Modern hierarchical, agglomerative clustering algorithms

This paper presents algorithms for hierarchical, agglomerative clustering which perform most efficiently in the general-purpose setup that is given in modern standard software. Requirements are: (1) the input data is given by pairwise dissimilarities between data points, but extensions to vector data are also discussed (2) the output is a "stepwise dendrogram", a data structure which is shared by all implementations in current standard software. We present algorithms (old and new) which perform clustering in this setting efficiently, both in an asymptotic worst-case analysis and from a practical point of view. The main contributions of this paper are: (1) We present a new algorithm which is suitable for any distance update scheme and performs significantly better than the existing algorithms. (2) We prove the correctness of two algorithms by Rohlf and Murtagh, which is necessary in each case for different reasons. (3) We give well-founded recommendations for the best current algorithms for the various agglomerative clustering schemes.

==> xy.tex <==
%% xy.tex from $Id: xy.doc,v 3.31 2011/05/27 04:51:17 krisrose Exp $
%%
%% Basic Xy-pictures: Xy-pic bootstrap and kernel macros.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined\else\message{not reloaded}\endinput\fi
\let\xyloaded=\relax
\message{Bootstrap\string'ing\string:}
{\catcode96 12\catcode`\#6\catcode`\.12\catcode`\:12\catcode`\'12\catcode`\@11
\ifx\xywarnifdefined\undefined\else \immediate\write16{}%
 \immediate\write16{Xy-pic Warning: \string\xywarnifdefined\space redefined.}%
 \immediate\write16{}\fi
\gdef\xywarnifdefined#1{\ifx#1\undefined\else \immediate\write16{}%
 \immediate\write16{Xy-pic Warning: `\string#1' redefined.}%
 \immediate\write16{}\fi}
\xywarnifdefined\xydef@ \gdef\xydef@#1{\xywarnifdefined#1\gdef#1}
\xywarnifdefined\xylet@ \gdef\xylet@#1{\xywarnifdefined#1\global\let#1}
\xywarnifdefined\xynew@
 \gdef\xynew@#1#2{\xywarnifdefined#2\csname new#1\endcsname#2}}
\message{catcodes\string,}
\xywarnifdefined\xyuncatcodes
\xywarnifdefined\xyreuncatcodes \def\xyreuncatcodes{\edef\xyuncatcodes{%
 \catcode92 0 \catcode123 1 \catcode125 2 \catcode37 14
 \catcode 9 \the\catcode 9 \catcode10 \the\catcode10 \catcode12 \the\catcode12
 \catcode35 \the\catcode35 \catcode36 \the\catcode36 \catcode38 \the\catcode38
 \catcode43 \the\catcode43 \catcode45 \the\catcode45 \catcode46 \the\catcode46
 \catcode47 \the\catcode47
 \catcode60 \the\catcode60 \catcode61 \the\catcode61 \catcode62 \the\catcode62
 \catcode64 \the\catcode64 \catcode96 \the\catcode96
 \newlinechar \the\newlinechar \endlinechar \the\endlinechar }}
\xyreuncatcodes
\xywarnifdefined\xycatcodes \def\xycatcodes{%
 \catcode 9 10
 \catcode 35 6 \catcode 36 3 \catcode 38 4
 \catcode 43 12 \catcode 45 12 \catcode 46 12 \catcode 47 12
 \catcode 60 12 \catcode 61 12 \catcode 62 12
 \catcode 64 11 \catcode 96 12 }
\xycatcodes
\message{docmode,}
{\catcode`\|0 \xywarnifdefined|DOCMODE
\gdef|DOCMODE#1{\ifx(#1\relax \xycatcodes \expandafter\ignorespaces
 \else \skipspecials@ \expandafter\docm@\fi}%
\xywarnifdefined\skipspecials@
\gdef\skipspecials@{%
 \catcode`\\12 \catcode`\{12 \catcode`\}12 \catcode`\#12 \catcode`\%12
 \catcode`\^^L12 \endlinechar`\^^J }%
\catcode`\/=12 \lccode`\/`\\%
\lccode`\D`\D \lccode`\O`\O \lccode`\C`\C \lccode`\M`\M \lccode`\E`\E
\lowercase{%
\xywarnifdefined\docm@ \gdef\docm@{\docm@i}%
\xywarnifdefined\docm@i \gdef\docm@i#1^^J{\docm@ii#1/DOCMODE\docm@iii}%
\xywarnifdefined\docm@ii
 \gdef\docm@ii#1/DOCMODE{\def\next@{#1}\futurelet\next\docm@iii}%
\xywarnifdefined\docm@iii \gdef\docm@iii#1\docm@iii{%
 \ifx\next\docm@iii \let\next\next@ \docecho@ \let\next@\docm@
 \else\ifx\next@\empty \let\next@\docfinish@
 \else \edef\next@{\noexpand\docm@iv\next@/DOCMODE#1\noexpand\docm@iv}%
 \fi\fi \next@}%
\xywarnifdefined\docm@iv
 \gdef\docm@iv#1/DOCMODE\docm@iv{\def\next{#1}\docecho@ \docm@}}%
\xywarnifdefined\docecho@ \global\let\docecho@\relax
\xywarnifdefined\docfinish@ \gdef\docfinish@{\xyuncatcodes|DOCMODE\next}}
\xydef@\xydefcsname@#1{\DN@{#1}\DNii@##1{%
 \ifx ##1\relax\else \xywarning@{\string`\string##1\string' redefined}\fi
 \def##1}%
 \expandafter\nextii@\csname\codeof\next@\endcsname}
\xydef@\xyletcsnamecsname@#1#2{\def\1{#1}\def\2{#2}\DN@##1##2{%
 \ifx ##1\relax\else \xywarning@{`\string##1\string' redefined}\fi
 \let##1=##2}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\csname\expandafter\codeof\expandafter\1\expandafter\endcsname
 \csname\codeof\2\endcsname}
\xywarnifdefined\codeof
\xywarnifdefined\codeof@
{\catcode`\:=12
 \gdef\codeof#1{\expandafter\codeof@\meaning#1<-:}
 \gdef\codeof@#1:->#2<-:{#2}}
\xywarnifdefined\addAT@
\xywarnifdefined\addHASH@
\xywarnifdefined\addDOLL@
\xywarnifdefined\addAND@
\xywarnifdefined\addRQ@
\xywarnifdefined\addPLUS@
\xywarnifdefined\addDASH@
\xywarnifdefined\addDOT@
\xywarnifdefined\addLT@
\xywarnifdefined\addEQ@
\xywarnifdefined\addGT@
\xywarnifdefined\addLQ@
\xydef@\xymakeADD@#1#2 #3 {\ifnum\catcode#3=6 \def#1##1{##1#2#2}%
 \else \def#1##1{##1#2}\fi}
\xydef@\xyrecat@{\xymakeADD@\addAT@}
\xydef@\xyrecat{\xyrecat@}
\xydef@\xyresetcatcodes{\def\xyrecat{\xyrecat@}\xyreuncatcodes
 \input xyrecat \relax \xyuncatcodes}
\xyuncatcodes \xyresetcatcodes \xycatcodes
\xydef@\testAND@{{\aftergroup\ifx 
 \addAND@\ifx\next\addFalse@\else\addTrue@\fi}}
\xydef@\addFalse@{\aftergroup\iffalse}
\xydef@\addTrue@{\aftergroup\iftrue}
\input xyidioms
\xydef@\stripRCS$#1${\stripRCS@#1: @@ @@@}
\xydef@\stripRCS@#1: #2@ #3@@@{%
 \ifx @#2\string?\else\ifx :#2\else\stripRCS@@#2\fi\fi}
\xydef@\stripRCS@@#1 #2: @{#1}
\xydef@\xyversion{3.8.6}
\edef\next{\stripRCS$Date: 2011/05/27 04:51:17 $}
\xylet@\xydate=\next
\xydef@\Xygreet@{%
 \W@{}%
 \W@{ Xy-pic version \xyversion\space<\xydate>}%
 \W@{ Copyright (c) 1991-2011 by Kristoffer H. Rose <krisrose@tug.org>}%
 \W@{ Xy-pic is free software: see the User\string's Guide for details.}%
 \W@{}}
\Xygreet@
\expandafter\everyjob\expandafter{\the\everyjob\Xygreet@}
\message{Loading kernel:}
\xydef@\Xy@{\leavevmode
 \hbox{\kern-.1em X\kern-.3em\lower.4ex\hbox{Y\kern-.15em}}}
\ifx\undefined\DeclareRobustCommand\let\Xy=\Xy@
\else\DeclareRobustCommand{\Xy}{\Xy@}\fi
\message{messages;}
\xywarnifdefined\thelineno@
\ifx\inputlineno\undefined \edef\thelineno@{\string?}
\else \def\thelineno@{\the\inputlineno}\fi
\xydef@\xytracelineno@{ \string[\jobname:\thelineno@\string]}
\xydef@\xywarning@#1{{\newlinechar=10
 \W@{}\W@{Xy-pic Warning: #1\xytracelineno@.}\W@{}}}
\xydef@\xyerror@#1#2{\if\inxy@\xy@{ERROR #1}{}\fi
 {\def\2{#2}\newlinechar=10
 \ifx\2\empty \errhelp{See the Xy-pic manual for further information.}%
 \else \errhelp{#2}\fi
 \errmessage{Xy-pic error: #1}}}
\xydef@\xybug@#1{{\newlinechar=10
 \errhelp{This is a bug in Xy-pic and should not happen!^^J%
If it did then please send a bug report with the offending Xy-pic code^^J%
to the author of Xy-pic, krisrose@tug.org.}%
 \errmessage{Xy-pic BUG: #1 -- notify krisrose@tug.org.}}}
\message{fonts;}
\xydef@\xyfont@#1{\ifx#1\undefined \DN@{\global\font#1}\expandafter\next@
 \else \xywarning@{Using previously loaded \string#1\space font}\fi}
\xyfont@\xydashfont=xydash10
\xydef@\xydashl@{\fontdimen6\xydashfont}
\xydef@\xydashh@{\fontdimen5\xydashfont}
\xydef@\xydashw@{\fontdimen8\xydashfont}
\xyfont@\xyatipfont=xyatip10
\xyfont@\xybtipfont=xybtip10
\xyfont@\xybsqlfont=xybsql10
\xydef@\xybsqll@{\fontdimen6\xybsqlfont}
\xydef@\xybsqlh@{\fontdimen5\xybsqlfont}
\xydef@\xybsqlw@{\fontdimen8\xybsqlfont}
\xyfont@\xycircfont=xycirc10
\message{allocations:}
\message{state,}
\xynew@{dimen}\X@c
\xynew@{dimen}\Y@c
\xynew@{dimen}\U@c
\xynew@{dimen}\D@c
\xynew@{dimen}\L@c
\xynew@{dimen}\R@c
\xynew@{toks}\Edge@c
\xynew@{dimen}\X@p
\xynew@{dimen}\Y@p
\xynew@{dimen}\U@p
\xynew@{dimen}\D@p
\xynew@{dimen}\L@p
\xynew@{dimen}\R@p
\xynew@{toks}\Edge@p
\xynew@{dimen}\X@origin \X@origin=\z@
\xynew@{dimen}\Y@origin \X@origin=\z@
\xynew@{dimen}\X@xbase \X@xbase=1mm
\xynew@{dimen}\Y@xbase \Y@xbase=\z@
\xynew@{dimen}\X@ybase \X@ybase=\z@
\xynew@{dimen}\Y@ybase \Y@ybase=1mm
\xynew@{dimen}\X@min
\xynew@{dimen}\Y@min
\xynew@{dimen}\X@max
\xynew@{dimen}\Y@max
\xynew@{box}\lastobjectbox@
\xynew@{box}\zerodotbox@
\setbox\zerodotbox@=\hbox{\dimen@=.5\xydashw@
 \kern-\dimen@ \vrule width\xydashw@ height\dimen@ depth\dimen@}
\wd\zerodotbox@=\z@ \ht\zerodotbox@=\z@ \dp\zerodotbox@=\z@
\xynew@{dimen}\almostz@ \almostz@=50sp
\xydef@\zz@#1{\ifdim#1<\z@-\fi#1<\almostz@\relax}
\xynew@{if}\iftmp@
\message{direction,}
\xynew@{dimen}\d@X
\xynew@{dimen}\d@Y
\xydef@\sd@X{}
\xydef@\sd@Y{}
\xynew@{count}\K@ \K@=1024
\xynew@{count}\KK@ \KK@=32
\xynew@{count}\Direction
\xynew@{dimen}\K@dXdY
\xynew@{dimen}\K@dYdX
\xydef@\cosDirection{}
\xydef@\sinDirection{}
\xywarnifdefined\DirectionChar
\xywarnifdefined\SemiDirectionChar
\xynew@{read}\xyread@
\xynew@{write}\xywrite@
\xynew@{count}\csp@
\xynew@{dimen}\quotPTK@
\message{utility macros;}
\xydef@\addtotoks@#1{\toks@=\expandafter{\the\toks@#1}}
\xydef@\xyinputorelse@#1#2{%
 \expandafter\let\expandafter\next@\csname#1loaded\endcsname
 \ifx\next@\empty \else
 \DN@{\xyinputorelse@@{#1}{\xyinputorelse@@{#1.doc}{#2}}}%
 \fi \next@}
\xydef@\xyinputorelse@@#1#2{\openin\xyread@=#1
 \ifeof\xyread@ \DN@{#2}\else \DN@{\closein\xyread@\input#1 }\fi \next@}
\global\csp@=\z@
\xydef@\enter@#1{\global\advance\csp@\@ne
 \expandafter\xdef\csname cs@\number\csp@\endcsname{#1}\ignorespaces}
\xydef@\nter@#1{\global\advance\csp@\@ne
 \expandafter\gdef\csname cs@\number\csp@\endcsname{#1}\ignorespaces}
\xydef@\dontleave@{\csname cs@\number\csp@\endcsname}
\xydef@\unenter@{\global\advance\csp@\m@ne}
\xydef@\leave@{\expandafter\unenter@\csname cs@\number\csp@\endcsname}
\quotPTK@=\p@ \divide\quotPTK@\K@
\xylet@\quotsign@@=\empty
\xywarnifdefined\removePT@
{\catcode`p=12 \catcode`t=12 \gdef\removePT@#1pt{#1}}
\xydef@\quotient@#1#2#3{\A@=#2\relax \B@=#3\relax
 \ifdim\A@<\z@\def\quotsign@@{-}\else\def\quotsign@@{+}\fi
 \ifdim\quotsign@@\A@<15pt \multiply\A@\K@
 \else\ifdim\quotsign@@\A@<511pt \multiply\A@\KK@
 \advance\B@\ifdim\B@<\z@-\fi 16sp \divide\B@\KK@
 \else
 \advance\B@\ifdim\B@<\z@-\fi 512sp \divide\B@\K@
 \fi\fi
 \ifdim\ifdim\B@<\z@-\fi\B@<\quotPTK@ \xywarning@{division overflow}%
 \else \advance\A@.5\B@ \divide\A@\B@ \fi
 \multiply\A@\quotPTK@ \edef#1{\expandafter\removePT@\the\A@}}
\xydef@\quotient@@#1#2#3{\A@=#2\relax \B@=#3\relax \multiply\A@\KK@
 \advance\B@\ifdim\B@<\z@-\fi 128sp \divide\B@\KK@ \divide\B@ 8
 \ifdim\B@=\z@\else \advance\A@.5\B@ \divide\A@\B@ \fi
 \B@=.125\quotPTK@ \multiply\A@\B@ \edef#1{\expandafter\removePT@\the\A@}}
\xydef@\loop@#1\repeat@{\def\body@{#1}\iterate@}\xylet@\repeat@=\fi
\xydef@\iterate@{\body@\expandafter\iterate@\else\fi}
\xydef@\xyinitial@#1#2{\DN@{#1}%
 \xyerror@{command used out of context: \codeof\next@}{}}
\xylet@\xy@=\xyinitial@
\xylet@\oxy@=\xy@
\xydef@\change@oxy@#1{\let\oxy@=#1\relax
}
\xydef@\inxy@{T\ifx\xy@\xyinitial@ F\else T\fi}
\xydef@\xyxy@@ix@{\begingroup
 \xyuncatcodes\afterassignment\endgroup\global\toks9=}
\xydef@\xy@@{\xy@{}}
\xydef@\plainxy@{\let\xy@=\xyxy@ \change@oxy@\xy@ \let\xy@@ix@=\xyxy@@ix@}
\message{pictures: \string\xy,}
\xydef@\xy{\ifmmode\expandafter\xymath@\else\expandafter\xynomath@\fi}
\xydef@\xymath@{\hbox\bgroup \dimen@=\the\fontdimen22\textfont\tw@ \xyinside@}
\xydef@\xynomath@{\hbox\bgroup \dimen@=\z@ \xyinside@}
\xydef@\xyinside@{%
 \saveXyStyle@ \aftergroup\xycheck@end
 \setboxz@h\bgroup
 \plainxy@
 \X@c=\z@ \Y@c=\z@ \czeroEdge@
 \X@p=\z@ \Y@p=\z@ \U@p=\z@ \D@p=\z@ \L@p=\z@ \R@p=\z@ \Edge@p={\zeroEdge}%
 \X@min=\hsize \X@max=-\hsize \Y@min=\hsize \Y@max=-\hsize
 \mathsurround=\z@
 \expandafter\POS\everyxy@@}
\xydef@\czeroEdge@{\U@c=\z@ \D@c=\U@c \L@c=\U@c \R@c=\U@c \Edge@c={\zeroEdge}}
\xydef@\xyxy@#1#2{#2}
\xywarnifdefined\everyxy
\expandafter\def\addEQ@\everyxy#1{\def\everyxy@@{#1}\ignorespaces}
\xylet@\everyxy@@=\empty
\xydef@\endxy{\if\inxy@\else\xyerror@{Unexpected \string\endxy}{}\fi
 \relax
 \dimen@=\Y@max \advance\dimen@-\Y@min
 \ifdim\dimen@<\z@ \dimen@=\z@ \Y@min=\z@ \Y@max=\z@ \fi
 \dimen@=\X@max \advance\dimen@-\X@min
 \ifdim\dimen@<\z@ \dimen@=\z@ \X@min=\z@ \X@max=\z@ \fi
 \edef\tmp@{\egroup
 \setboxz@h{\kern-\the\X@min\boxz@}%
 \ht\z@=\the\Y@max \dp\z@=-\the\Y@min \wdz@=\the\dimen@
 \noexpand\maybeunraise@ \raise\dimen@\boxz@
 \noexpand\recoverXyStyle@ \egroup \noexpand\xy@end
 \U@c=\the\Y@max \D@c=-\the\Y@min \L@c=-\the\X@min \R@c=\the\X@max}\tmp@}
\xydef@\maybeunraise@{\if\inxy@\else \dimen@ii=\dp\z@
 \ifdim\dimen@ii<\z@ \advance\dimen@\dimen@ii \fi\fi}
\xydef@\xycheck@end{\xyFN@\xycheck@end@}
\xydef@\xycheck@end@{\ifx\next\xy@end\DN@\xy@end{}\else\DN@{\xy@end}\fi\next@}
\xydef@\xy@end{%
 \xyerror@{An \string\xy\space environment is not closed correctly.}%
 {I expected \string\endxy. You probably have an umatched {} grouping.}}
\message{positions,}
\xydef@\POS{\afterPOS{}}
\xydef@\afterPOS#1{%
 \DN@##1{\def\afterPOS@{\def\afterPOS@{##1}#1}}%
 \expandafter\next@\expandafter{\afterPOS@}%
 \afterCOORD{\xyFN@\POS@}}
\xylet@\afterPOS@=\empty
\xydef@\afterCOORD#1{%
 \DN@##1{\def\afterCOORD@{\def\afterCOORD@{##1}#1}}%
 \expandafter\next@\expandafter{\afterCOORD@}%
 \afterVECTORorEMPTY{\xy@@\czeroEdge@ \afterCOORD@}{\xyFN@\COORD@}}
\xylet@\afterCOORD@=\empty
\xydef@\afterVECTORorEMPTY#1#2{%
 \DN@##1{\def\afterVECTOR@{\def\afterVECTOR@{##1}%
 \ifVECTORempty@\DN@{#2}\else\DN@{#1}\fi \next@}}%
 \expandafter\next@\expandafter{\afterVECTOR@}%
 \xyFN@\VECTOR@}
\xynew@{if}\ifVECTORempty@
\xylet@\afterVECTOR@=\empty
\xydef@\xyVECTOR@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\VECTOR@}%
 \else \ifcat A\noexpand\next \let\next@=\VECTOR@letter
 \else \let\next@=\VECTOR@other \fi\fi \next@}
\xylet@\VECTOR@=\xyVECTOR@
\def\notrelaxorelse@#1#2{\ifx#1\relax \expandafter#2\else\expandafter#1\fi}
\xydef@\VECTOR@letter{%
 \ifx a\next \expandafter\VECTOR@a \else \expandafter\CORNER@ \fi}
\xydef@\VECTOR@a a(#1){\xy@{a(#1)}{\vfromcartesianangle@{#1}}%
 \VECTORempty@false \afterVECTOR@}
\xydef@\CORNER@{%
 \xy@{}{\A@=-.5\L@c \advance\A@.5\R@c \B@=-.5\D@c \advance\B@.5\U@c
 \let\nextii@=\zeroit@}%
 \VECTORempty@true\CORNER@i}
\xydef@\zeroit@#1{#1=\z@}
\xydef@\CORNER@i{%
 \ifx D\next \DN@ D{\xy@{D}{\Y@c=-\D@c \nextii@\X@c \B@=\Y@c}\CORNER@ii}%
 \else\ifx U\next \DN@ U{\xy@{U}{\Y@c= \U@c \nextii@\X@c \B@=\Y@c}\CORNER@ii}%
 \else\ifx L\next \DN@ L{\xy@{L}{\X@c=-\L@c \nextii@\Y@c \A@=\X@c}\CORNER@ii}%
 \else\ifx R\next \DN@ R{\xy@{R}{\X@c= \R@c \nextii@\Y@c \A@=\X@c}\CORNER@ii}%
 \else\ifx C\next \DN@ C{\xy@{C}{\X@c= \A@ \Y@c= \B@}\CORNER@ii}%
 \else\ifx E\next \DN@ E{\xy@{E}{%
 \A@=\X@c \B@=\Y@c \the\Edge@c\z@ \advance\X@c-\A@ \advance\Y@c-\B@}%
 \CORNER@ii}%
 \else\ifx P\next \DN@ P{\xy@{P}{%
 \A@=\X@c \B@=\Y@c \the\Edge@c\thr@@ \advance\X@c-\A@ \advance\Y@c-\B@}%
 \CORNER@ii}%
 \else\ifx (\next
 \DN@(##1){\xy@{(##1)}{\X@c=##1\X@c \Y@c=##1\Y@c}\afterVECTOR@}%
 \else\ifx A\next \DN@ A{\xy@{A}{\Y@c=\fontdimen22\textfont\tw@ \nextii@\X@c \B@=\Y@c}\CORNER@ii}%
 \else\ifx V\next \DN@ V{\xy@{V}{\nextii@\X@c \Y@c=\U@p}\CORNER@ii}%
 \else\ifx H\next \DN@ H{\xy@{H}{\nextii@\Y@c \X@c=\R@p}\CORNER@ii}%
 \else \let\next@=\afterVECTOR@
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\CORNER@ii{\xy@@{\let\nextii@=\eat@}%
 \VECTORempty@false \xyFN@\CORNER@i}
\xydef@\VECTOR@other{%
 \addLT@\ifx \next
 \addGT@{\addLT@\DN@##1}{\xy@{<##1>}{\vfromabsolute@{##1}}%
 \VECTORempty@false\afterVECTOR@}%
 \else\ifx (\next
 \DN@({\xyFN@\VECTOR@other@open}%
 \else\ifx /\next
 \DN@/##1/{\xy@@ix@{{##1}}%
 \xy@{/##1/}{\expandafter\vfromslide@\the\toks9 }%
 \VECTORempty@false\afterVECTOR@}%
 \else\ifx 0\next
 \DN@ 0{\xy@{0}{\X@c=\z@ \Y@c=\z@}\VECTORempty@false\afterVECTOR@}%
 \else
 \DN@{\VECTORempty@true\afterVECTOR@}%
 \fi\fi\fi\fi \next@}
\xydef@\VECTOR@other@open{%
 \ifx *\next \DN@{\VECTORempty@true \xyFN@\afterVECTOR@(}%
 \else
 \DN@##1){\xy@{(##1)}{\vfromcartesian@{##1}}\VECTORempty@false\afterVECTOR@}%
 \fi \next@}
\xydef@\xyCOORD@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\COORD@}%
 \else \ifcat A\noexpand\next \let\next@=\xyCOORD@letter
 \else \let\next@=\xyCOORD@other \fi\fi \next@}
\xylet@\COORD@=\xyCOORD@
\xydef@\xyCOORD@letter{%
 \ifx c\next
 \DN@ c{\xy@{c}{}\afterCOORD@}%
 \else\ifx p\next
 \DN@ p{\xy@{p}\cfromp@ \afterCOORD@}%
 \else\ifx x\next
 \DN@ x{\xy@{x}{\R@c=\X@xbase \U@c=\Y@xbase \intersect@}\afterCOORD@}%
 \else\ifx y\next
 \DN@ y{\xy@{y}{\R@c=\X@ybase \U@c=\Y@ybase \intersect@}\afterCOORD@}%
 \else\ifx s\next
 \DN@ s##1{\xy@{s{##1}}{\cfroms@{##1}}\afterCOORD@}%
 \else \let\next@=\afterCOORD@ \fi\fi\fi\fi\fi \next@}
\xydef@\xyCOORD@other{%
 \ifx "\next
 \DN@"##1"{\xy@{"##1"}{\cfromid@{##1}}\afterCOORD@}%
 \else\ifx \bgroup\next
 \DN@##1{\xy@{{##1}}{\enter@{\pfromthep@\basefromthebase@}}%
 \silencexy@ \POS##1\relax \unsilencexy@ \xy@@\leave@ \afterCOORD@}%
 \else\ifx (\next
 \DN@({\xyFN@\xyCOORD@other@open}%
 \else \let\next@=\afterCOORD@ \fi\fi\fi \next@}
\xynew@{if}\ifsilentxy@
\xydef@\silencexy@{%
 \ifsilentxy@ \nter@{}%
 \else \nter@{\silentxy@false \let\xy@=\unsilent@@xy@}
 \silentxy@true \let\unsilent@@xy@=\xy@ \def\xy@##1##2{\unsilent@@xy@{}{##2}}%
 \fi}
\xydef@\unsilencexy@{\leave@}
\xydef@\xyCOORD@other@open{%
 \ifx *\next
 \DN@*##1*){\xy@{(*}{\enter@{\pfromthep@\basefromthebase@}}%
 \POS##1\relax \xy@{*)}\leave@ \afterCOORD@}%
 \else \DN@{\xyFN@\afterCOORD@(}%
 \fi \next@}
\xydef@\xyPOS@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\POS@}%
 \else\addPLUS@\ifx \next
 \addPLUS@\DN@{\xy@+{\enter@\cplusthec@}%
 \afterCOORD{\xy@@\leave@ \xyFN@\POS@}}%
 \else\addDASH@\ifx \next
 \addDASH@\DN@{\xy@-{\enter@\cplusthec@}%
 \afterCOORD{\xy@@{\X@c=-\X@c \Y@c=-\Y@c\leave@}\xyFN@\POS@}}%
 \else\ifx !\next
 \DN@ !{\xy@!{\enter@\cskewthec@}\afterCOORD{\xy@@\leave@ \xyFN@\POS@}}%
 \else\addDOT@\ifx \next
 \addDOT@\DN@{\xy@.{\enter@\cmergethec@}\afterCOORD{\xy@@\leave@ \xyFN@\POS@}}%
 \else\ifx ,\next
 \DN@ ,{\xy@,{\comma@@}\afterCOORD{\xyFN@\POS@}}%
 \else\ifx ;\next
 \DN@ ;{\xy@;{\swap@}\afterCOORD{\xyFN@\POS@}}%
 \else\ifx :\next
 \DN@ :{\xyFN@\POS@colon}%
 \else\addEQ@\ifx \next
 \addEQ@\DN@{\xyFN@\saveid@}%
 \else\ifx *\next
 \DN@ *{\xyFN@\POS@star}%
 \else\ifx ?\next
 \DN@ ?{\xy@?{}\afterPLACE{\xyFN@\POS@}}%
 \else \addAT@\ifx \next
 \addAT@\DN@{\xyFN@\STACK@}%
 \else
 \let\next@=\afterPOS@
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xylet@\comma@@=\relax
\xylet@\POS@=\xyPOS@
\xydef@\POS@colon{\DNii@{\afterCOORD{\xyFN@\POS@}}%
 \ifx :\next \xy@{::}{\setbase@@\X@c\Y@c}\DN@:{\nextii@}%
 \else \xy@:{\setbase@\X@p\Y@p\X@c\Y@c}\let\next@=\nextii@ \fi
 \next@}
\xydef@\POS@star{%
 \ifx *\next
 \DN@*##1##{\nextii@{##1}}%
 \DNii@##1##2{\xy@@ix@{{##1}{##2}}%
 \xy@{**##1{##2}}{\expandafter\connect@\the\toks9 }\xyFN@\POS@}%
 \else
 \DN@##1##{\nextii@{##1}}%
 \DNii@##1##2{\xy@@ix@{{##1}{##2}}%
 \xy@{*##1{##2}}{\expandafter\drop@\the\toks9 }\xyFN@\POS@}%
 \fi
 \next@}
\xydef@\cfromp@{\X@c=\X@p \Y@c=\Y@p \U@c=\U@p \D@c=\D@p \L@c=\L@p \R@c=\R@p
 \Edge@c=\expandafter{\the\Edge@p}}
\xydef@\pfromc@{\X@p=\X@c \Y@p=\Y@c \U@p=\U@c \D@p=\D@c \L@p=\L@c \R@p=\R@c
 \Edge@p=\expandafter{\the\Edge@c}}
\xydef@\swapdimen@#1#2{\dimen@=#1\relax #1=#2\relax #2=\dimen@}
\xynew@{toks}\swaptoks@@
\xydef@\swap@{\swapdimen@\X@c\X@p \swapdimen@\Y@c\Y@p
 \swapdimen@\U@c\U@p\swapdimen@\D@c\D@p \swapdimen@\L@c\L@p\swapdimen@\R@c\R@p
 \swaptoks@@=\Edge@c \Edge@c=\Edge@p \Edge@p=\swaptoks@@}
\xydef@\vfromabsolute@#1{\vfromabsolute@@#1,@}
\xydef@\vfromabsolute@@#1,#2@{\X@c=#1\relax
 \DN@{#2}\ifx\next@\empty \Y@c=\X@c
 \else \DN@##1,{\Y@c=##1}\next@#2\relax \fi
}
\xydef@\cfromthec@{\X@c=\the\X@c \Y@c=\the\Y@c
 \U@c=\the\U@c \D@c=\the\D@c \L@c=\the\L@c \R@c=\the\R@c
 \Edge@c={\expandafter\noexpand\the\Edge@c}}
\xydef@\cfromthep@{\X@c=\the\X@p \Y@c=\the\Y@p
 \U@c=\the\U@p \D@c=\the\D@p \L@c=\the\L@p \R@c=\the\R@p
 \Edge@c={\expandafter\noexpand\the\Edge@p}}
\xydef@\pfromthep@{\X@p=\the\X@p \Y@p=\the\Y@p
 \U@p=\the\U@p \D@p=\the\D@p \L@p=\the\L@p \R@p=\the\R@p
 \Edge@p={\expandafter\noexpand\the\Edge@p}}
\xydef@\pfromthec@{\X@p=\the\X@c \Y@p=\the\Y@c
 \U@p=\the\U@c \D@p=\the\D@c \L@p=\the\L@c \R@p=\the\R@c
 \Edge@p={\expandafter\noexpand\the\Edge@c}}
\xydef@\cplusthec@{\advance\X@c\the\X@c \advance\Y@c\the\Y@c}
\xydef@\cskewthec@{%
 \noexpand\cskew@{\the\Y@c}{\the\X@c}{\the\D@c}{\the\U@c}{\the\L@c}{\the\R@c}}
\xydef@\cskew@#1#2#3#4#5#6{%
 \D@c=#3\advance\D@c \Y@c \ifdim\D@c<\z@ \D@c=\z@ \fi
 \U@c=#4\advance\U@c-\Y@c \ifdim\U@c<\z@ \U@c=\z@ \fi
 \advance\Y@c#1%
 \L@c=#5\advance\L@c \X@c \ifdim\L@c<\z@ \L@c=\z@ \fi
 \R@c=#6\advance\R@c-\X@c \ifdim\R@c<\z@ \R@c=\z@ \fi
 \advance\X@c#2%
 \Edge@c={\rectangleEdge}}
\xydef@\cmergethec@{%
 \noexpand\cmerge@{\the\Y@c}{\the\X@c}{\the\D@c}{\the\U@c}{\the\L@c}{\the\R@c}}
\xydef@\cmerge@#1#2#3#4#5#6{\the\Edge@c4%
 \A@=#2\advance\A@-\X@c \B@=#1\advance\B@-\Y@c
 \dimen@=#5\advance\L@c \A@ \ifdim\L@c<\dimen@ \L@c=\dimen@ \fi
 \dimen@=#6\advance\R@c-\A@ \ifdim\R@c<\dimen@ \R@c=\dimen@ \fi
 \dimen@=#3\advance\D@c \B@ \ifdim\D@c<\dimen@ \D@c=\dimen@ \fi
 \dimen@=#4\advance\U@c-\B@ \ifdim\U@c<\dimen@ \U@c=\dimen@ \fi
 \advance\X@c\A@ \advance\Y@c\B@}
\xydef@\halfroottwo{.70710678}
\xydef@\partroottwo{.29289322}
\xydef@\halfrootthree{.8660254}
\xydef@\vfromcartesian@#1{\vfromcartesian@@#1@}
\xydef@\vfromcartesian@@#1,#2@{%
 \X@c=\X@origin \advance\X@c#1\X@xbase \advance\X@c#2\X@ybase
 \Y@c=\Y@origin \advance\Y@c#1\Y@xbase \advance\Y@c#2\Y@ybase}
\xydef@\setbase@#1#2#3#4{%
 \X@origin=#1\relax \Y@origin=#2\relax
 \X@xbase=#3\relax \advance\X@xbase-\X@origin
 \Y@xbase=#4\relax \advance\Y@xbase-\Y@origin
 \X@ybase=-\Y@xbase \Y@ybase=\X@xbase}
\xydef@\setbase@@#1#2{%
 \X@ybase=#1\relax \advance\X@ybase-\X@origin
 \Y@ybase=#2\relax \advance\Y@ybase-\Y@origin}
\xydef@\basefromthebase@{\X@origin=\the\X@origin \Y@origin=\the\Y@origin
 \X@xbase=\the\X@xbase \Y@xbase=\the\Y@xbase
 \X@ybase=\the\X@ybase \Y@ybase=\the\Y@ybase}
\xydef@\vfromcartesianangle@#1{\enter@\basefromthebase@ \R@=#1\p@
 \B@=360\p@
 \loop@ \ifdim\R@<\z@ \advance\R@\B@ \repeat@
 \loop@ \ifdim\R@>\B@ \advance\R@-\B@ \repeat@
 \ifdim\R@<.5\B@\else \R@=-\R@ \advance\R@\B@
 \X@ybase=-\X@ybase \Y@ybase=-\Y@ybase \fi
 \B@=180\p@
 \ifdim\R@<.5\B@\else \R@=-\R@ \advance\R@\B@
 \X@xbase=-\X@xbase \Y@xbase=-\Y@xbase \fi
 \B@=90\p@
 \ifdim\R@<.5\B@ \let\nextiii@=\literal@
 \else \R@=-\R@ \advance\R@\B@ \def\nextiii@##1,##2@{##2,##1@}\fi
 \dimen@=\z@ \DN@{1,0@}%
 \dimen@ii=45\p@ \DNii@{.70710678,.70710678@}%
 \chooseangleinterval@
 {\chooseangleinterval@
 {\chooseangleinterval@
 {\chooseangleinterval@
 {\chooseangleinterval@
 {}%
 {4.090909}{.99677570,.08023846@}%
 {}}%
 {6}{.99452190,.10452846@}%
 {\chooseangleinterval@
 {}%
 {8.181818}{.98982144,.14231484@}%
 {}}}%
 {10}{.98480775,.17364818@}%
 {\chooseangleinterval@
 {}%
 {12.857143}{.97492791,.22252093@}%
 {}}}%
 {15}{.96592583,.25881905@}%
 {\chooseangleinterval@
 {\chooseangleinterval@
 {}%
 {16.363636}{.95949297,.28173256@}%
 {}}%
 {18}{.95105652,.30901699@}%
 {\chooseangleinterval@
 {}%
 {20}{.93969262,.34202014@}%
 {}}}}%
 {22.5}{.92387953,.38268343@}%
 {\chooseangleinterval@
 {\chooseangleinterval@
 {\chooseangleinterval@
 {}%
 {24.545455}{.90963200,.41541501@}%
 {}}%
 {25.714286}{.90096887,.43388374@}%
 {}}%
 {30}{.86602540,.5@}%
 {\chooseangleinterval@
 {\chooseangleinterval@
 {}%
 {32.727273}{.84125353,.54064082@}%
 {}}%
 {36}{.80901699,.58778525@}%
 {\chooseangleinterval@
 {\chooseangleinterval@
 {}%
 {38.571429}{.78183148,.62348980@}%
 {}}%
 {40.909091}{.75574957,.65486073@}%
 {\chooseangleinterval@
 {}%
 {40}{.76604444,.64278761@}%
 {}}}}}%
 \A@=\R@ \advance\A@-\dimen@
 \ifdim\ifdim\A@<\z@-\fi\A@<.01\p@ \edef\next@{\expandafter\nextiii@\next@}%
 \else \B@=\dimen@ii \advance\B@-\R@ 
 \ifdim\A@<\B@ \dimen@=\toradians@\A@
 \edef\next@{\next@ \expandafter\removePT@\the\dimen@ @}%
 \else \dimen@=-\toradians@\B@
 \edef\next@{\nextii@ \expandafter\removePT@\the\dimen@ @}%
 \fi
 \expandafter\interpolatepoint@\next@
 \edef\next@{\expandafter\nextiii@\next@}%
 \fi 
 \expandafter\vfromcartesian@@\next@
 \leave@}
\xydef@\chooseangleinterval@#1#2#3#4{%
 \B@=#2\p@ \def\next{#3}%
 \ifdim\R@<\B@ \dimen@ii=\B@ \let\nextii@=\next #1%
 \else \dimen@=\B@ \let\next@=\next \ifdim\B@<\R@ #4\fi\fi}
\xydef@\interpolateinterval@#1,#2@#3,#4@{%
 \A@=#1\p@ \dimen@=#3\p@ \advance\dimen@-\A@ \advance\A@\next\dimen@
 \B@=#2\p@ \dimen@=#4\p@ \advance\dimen@-\B@ \advance\B@\next\dimen@
 \edef\next@{\expandafter\removePT@\the\A@,\expandafter\removePT@\the\B@ @}}
\xydef@\toradians@{0.01745329}
\xydef@\interpolatepoint@#1,#2@#3@{%
 \A@=#1\p@ \dimen@ii=#3\A@ \dimen@ii=-.5\dimen@ii \advance\A@#3\dimen@ii
 \dimen@=-#2\p@ \advance\A@#3\dimen@
 \B@=#2\p@ \dimen@ii=#3\B@ \dimen@ii=-.5\dimen@ii \advance\B@#3\dimen@ii
 \dimen@=#1\p@ \advance\B@#3\dimen@
 \edef\next@{\expandafter\removePT@\the\A@,\expandafter\removePT@\the\B@ @}}
\xydef@\drop@#1#2{%
 \global\setbox\lastobjectbox@=\object#1{#2}%
 \ifHidden@ \dimen@=\X@c \advance\dimen@-\L@c \else
 \dimen@=\Y@c \advance\dimen@ \U@c \ifdim\Y@max<\dimen@ \Y@max=\dimen@ \fi
 \dimen@=\Y@c \advance\dimen@-\D@c \ifdim\dimen@<\Y@min \Y@min=\dimen@ \fi
 \dimen@=\X@c \advance\dimen@ \R@c \ifdim\X@max<\dimen@ \X@max=\dimen@ \fi
 \dimen@=\X@c \advance\dimen@-\L@c \ifdim\dimen@<\X@min \X@min=\dimen@ \fi
 \fi
 \ifInvisible@\else
 \setboxz@h{\kern\dimen@ \raise\Y@c\box\lastobjectbox@}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ {\Drop@@}\fi}
\xydef@\connect@#1#2{\setupDirection@ \enter@{\cfromthec@}%
 \global\setbox\lastobjectbox@=\object#1{#2}\leave@
 \Connect@@}
\xydef@\preconnect@#1#2{\setupDirection@ \enter@{\cfromthec@}%
 \global\setbox\lastobjectbox@=\object#1{#2}\leave@ \connectStore@
 \ifInvisible@ \Connect@@ \else \Invisible@true\Connect@@\Invisible@false \fi}
\xynew@{box}\connectobjectbox@@
\xylet@\connectDrop@@=\empty
\xylet@\connectpreXY@style@=\empty
\xylet@\connectpostXY@style@=\empty
\xylet@\connectRest@@=\empty
\xydef@\connectStore@{%
 \global\setbox\connectobjectbox@@=\copy\lastobjectbox@
 \let\connectDrop@@=\Drop@@
 \let\connectpreXY@style@ =\preXY@style@ 
 \let\connectpostXY@style@=\postXY@style@
 \xdef\connectRest@@{%
 \def\noexpand\Upness@{\Upness@}%
 \def\noexpand\Leftness@{\Leftness@}%
 \ifInvisible@ \noexpand\Invisible@true \else \noexpand\Invisible@false \fi
 \ifHidden@ \noexpand\Hidden@true \else \noexpand\Hidden@false \fi}}
\xydef@\connectRestore@{%
 \ifvbox\connectobjectbox@@
 \setbox\lastobjectbox@=\copy\voidb@x
 \else
 \global\setbox\lastobjectbox@=\copy\connectobjectbox@@
 \fi
 \let\Drop@@=\connectDrop@@
 \global\let\preXY@style@ =\connectpreXY@style@ 
 \global\let\postXY@style@=\connectpostXY@style@
 \connectRest@@}
\xydef@\afterPLACE#1{%
 \DN@##1{\def\afterPLACE@{\xy@@\leave@ \def\afterPLACE@{##1}#1}}%
 \expandafter\next@\expandafter{\afterPLACE@}%
 \def\PLACEf@{{.5}}%
 \xy@@{\enter@{\pfromthep@}%
 \Creset@@ \def\PLACEf@{{.5}}%
 \let\PLACEedgep@@=\PLACEedgep@ \let\PLACEedgec@@=\PLACEedgec@}%
 \xyFN@\PLACE@}
\xydef@\PLACEf@{}
\xydef@\PLACEedgep@@{}
\xydef@\PLACEedgec@@{}
\xydef@\PLACEedgep@{\Cshavep@@ \def\PLACEedgep@@{\Cslidep@@\jot}}
\xydef@\PLACEedgec@{\Cshavec@@ \def\PLACEedgec@@{\Cslidec@@{-\jot}}}
\xylet@\afterPLACE@=\empty
\xydef@\PLACE@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PLACE@}%
 \else\addLT@\ifx \next
 \addLT@\DN@{\addLT@\xy@{\def\PLACEf@{{0}}\PLACEedgep@@}\xyFN@\PLACE@}%
 \else\addGT@\ifx \next
 \addGT@\DN@{\addGT@\xy@{\def\PLACEf@{{1}}\PLACEedgec@@}\xyFN@\PLACE@}%
 \else\ifx (\next
 \DN@(##1){\def\PLACEf@{{##1}}\xy@{(##1)}{\def\PLACEf@{{##1}}}\xyFN@\PLACE@}%
 \else\ifx !\next
 \DN@!{\xyFN@\PLACE@intercept}%
 \else
 \DN@{\xy@@{\expandafter\Calong@@\PLACEf@ \czeroEdge@}\PLACE@@}%
 \fi\fi\fi\fi\fi \next@}
\xydef@\PLACE@intercept{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PLACE@intercept}%
 \else\ifx \bgroup\next
 \DN@##1{\xy@{!{##1}}{}\PLACE@intercept@{##1}}%
 \else\ifx (\next
 \DN@(*##1*){\xy@{!(*##1*)}{}\PLACE@intercept@{##1}}%
 \else \DN@{\xyerror@{{<pos>} expected after ! in <place>}{}}%
 \fi\fi\fi \next@}
\xydef@\PLACE@intercept@#1{%
 \xy@@{\enter@{\pfromthep@\basefromthebase@}\begingroup}%
 \xy@@ix@{#1}\xy@@{\plainxy@ \expandafter\POS\the\toks9\relax
 \edef\next@{\endgroup
 \X@c =\the\X@c \Y@c=\the\Y@c \X@p=\the\X@p \Y@p=\the\Y@p}%
 \next@ \Cintercept@@ \leave@}%
 \PLACE@@}
\xydef@\PLACE@@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PLACE@@}%
 \else\ifx /\next \DN@/##1/{\xy@{/##1/}{\Cslidec@@{##1}}\afterPLACE@}%
 \else \let\next@=\afterPLACE@
 \fi\fi \next@}
\xydef@\intersect@{%
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p
 \A@=\X@c \advance\A@-\X@origin \B@=\Y@c \advance\B@-\Y@origin
 \edef\next@{\expandafter\removePT@\the\R@c}%
 \edef\nextii@{\expandafter\removePT@\the\U@c}%
 \D@c=\next@\d@Y \advance\D@c-\nextii@\d@X \divide\D@c\KK@
 \L@c=\next@\B@ \advance\L@c-\nextii@\A@ \divide\L@c\KK@
 \ifdim\D@c=\z@\zeroDivide@\else \quotient@\next@\L@c\D@c \fi
 \advance\X@c-\next@\d@X \advance\Y@c-\next@\d@Y
 \czeroEdge@}
\xydef@\zeroDivide@@{\zeroDivide@message{\intersect@}{treated as 0}\DN@{0}}
\xydef@\zeroDivide@message#1#2{\xywarning@{division by 0 in \string#1, #2}}
\xylet@\zeroDivide@=\zeroDivide@@
\xydef@\zeroDivideLimit@@{\ifdim\L@c=\z@ \DN@{0}%
 \else\ifdim\L@c<\z@\DN@{-\zeroDivide@Limit}%
 \else\DN@{\zeroDivide@Limit}\fi\fi
 \zeroDivide@message{\intersect@}{replaced by \zeroDivide@Limit}}
\xydef@\zeroDivideLimit@#1{\edef\zeroDivide@Limit{#1}%
 \let\zeroDivide@=\zeroDivideLimit@@}
\xylet@\zeroDivideLimit=\zeroDivideLimit@
\xydef@\vfromslide@#1{\enter@\DirectionfromtheDirection@ \begingroup
 \plainxy@\afterDIRECTIONorEMPTY\vfromslide@i\vfromslide@i#1@}
\xydef@\vfromslide@i#1@{\DN@{#1}%
 \edef\next{\endgroup
 \ifx\next@\empty \dimen@=.5pc \else \dimen@=#1\relax \fi
 \X@c=\cosDirection\dimen@ \Y@c=\sinDirection\dimen@}\next
 \leave@}
\xydef@\s@bot{-1}
\xydef@\s@top{-1}
\xydef@\cfroms@#1{\tests@{#1}\runs@\outofranges@}
\xydef@\tests@#1#2#3{\DN@{#3}%
 \count@=\s@top \advance\count@-#1\relax
 \ifnum\count@>\s@bot\relax \ifnum\count@>\s@top\else\DN@{#2}\fi\fi
 \next@}
\xydef@\runs@{\csname S@\the\count@\endcsname}
\xydef@\outofranges@{\count@=\s@top \advance\count@-\s@bot
 \xyerror@{stack index out of range (should be 0..\the\count@)}{}}
\xydef@\STACK@{%
 \addPLUS@\ifx\next
 \addPLUS@\DN@{\xy@{@+}{}\afterCOORD{\xy@@\spushc@ \xyFN@\POS@}}%
 \else\addDASH@\ifx\next
 \addDASH@\DN@{\xy@{@-}{}\afterCOORD{\xy@@\spop@ \xyFN@\POS@}}%
 \else \ifx i\next \DN@ i{\xy@{@i}\sinit@ \xyFN@\POS@}%
 \else \ifx (\next \DN@ ({\xy@{@(}\senter@ \xyFN@\POS@}%
 \else \ifx )\next \DN@ ){\xy@{@)}\sleave@ \xyFN@\POS@}%
 \else\addEQ@\ifx\next \addEQ@\DN@{\STACK@load}%
 \else\addAT@\ifx\next \addAT@\DN@{\xy@{@@}{}\smap@}%
 \else \DN@##1{\xyerror@{illegal stack command ##1}{}\afterCOORD{\xyFN@\POS@}}%
 \fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\STACK@load{\xy@{@=}{%
 \if\sempty@\else \xywarning@{loading on top of non-empty stack}\sinit@ \fi
 \let\comma@@=\spushc@}%
 \afterCOORD{\xy@@{\spushc@ \let\comma@@=\relax}\xyFN@\POS@}}
\xydef@\spushc@{%
 \count@=\s@top \advance\count@\@ne \edef\s@top{\the\count@}%
 \expandafter\edef\csname S@\s@top\endcsname{\cfromthec@}}
\xydef@\spushid@#1{\DNii@{#1}\edef\nextii@{\codeof\nextii@}%
 \expandafter\let\expandafter\next@\csname Q@\nextii@\endcsname
 \ifx\next@\relax \xyerror@{<pos> \string"\nextii@\string" not defined}{}%
 \else
 \count@=\s@top \advance\count@\@ne \edef\s@top{\the\count@}%
 \DNii@##1{\expandafter\def\csname S@\s@top\endcsname{##1}}%
 \expandafter\nextii@\expandafter{\next@}%
 \fi}
\xydef@\idfroms@#1#2{%
 \tests@{#2}{\DN@{\idfromxy@{#1}}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\expandafter{\csname S@\the\count@\endcsname}%
 }\outofranges@}
\xydef@\spop@{\count@=\s@top
 \ifnum\count@>\s@bot \advance\count@\m@ne \edef\s@top{\the\count@}%
 \else \xyerror@{nothing to pop from stack}{}\fi}
\xydef@\sinit@{\edef\s@top{\s@bot}}
\xydef@\senter@{%
 \count@=\s@top \advance\count@\@ne
 \expandafter\edef\csname S@\the\count@\endcsname{\s@bot}%
 \edef\s@bot{\the\count@}\edef\s@top{\the\count@}}
\xydef@\sleave@{%
 \ifnum\s@bot=\s@top\else \xywarning@{leaving non-empty stack}\sinit@ \fi
 \ifnum\s@bot>\m@ne \edef\s@bot{\csname S@\s@top\endcsname}%
 \count@=\s@top \advance\count@\m@ne \edef\s@top{\the\count@}%
 \edef\sbot{\the\count@}\fi}
\xydef@\sempty@{\ifnum\s@top=\s@bot TT\else TF\fi}
\xydef@\xytotoks@#1#2{\addtotoks@{#2}}
\xydef@\xytotoks@@toksix@#1{\addtotoks@{\toks9={#1}}}
\xydef@\smap@{%
 \begingroup \toks@={}\let\xy@=\xytotoks@ \change@oxy@\xy@
 \let\xy@@ix@=\xytotoks@@toksix@
 \afterCOORD{\expandafter\endgroup
 \expandafter\smapxy@@\expandafter{\the\toks@}\xyFN@\POS@}}
\xydef@\smapxy@@#1{\xy@@{\edef\smapp@@{\s@bot}\smapxy@i{#1}}}
\xylet@\smapp@@=\empty
\xydef@\smapxy@i#1{%
 \ifnum\smapp@@<\s@top
 \count@=\smapp@@ \advance\count@\@ne \edef\smapp@@{\the\count@}%
 \DN@{\csname S@\smapp@@\endcsname #1\relax \smapxy@i{#1}}%
 \else \let\next@=\relax
 \fi \next@}
\xydef@\saveid@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\saveid@}%
 \else \ifx "\next\DN@"##1"{\xy@{="##1"}{\idfromc@{##1}}\xyFN@\POS@}%
 \else \ifx :\next\DN@:##1"##2"{\xy@{=:"##2"}{\idfrombase@{##2}}\xyFN@\POS@}%
 \else\addAT@\ifx\next
 \addAT@\DN@"##1"{\xy@{=@"##1"}{\idfromstack@{##1}}\xyFN@\POS@}%
 \else \ifx s\next
 \DN@ s##1"##2"{\xy@{=s##1"##2"}{\idfroms@{##2}{##1}}\xyFN@\POS@}%
 \else\addEQ@\ifx\next \let\saveid@COORD@@=\saveid@COORDii
 \addEQ@\DN@{\xyFN@\saveid@COORD}%
 \else \let\saveid@COORD@@=\saveid@COORDi \let\next@=\saveid@COORD
 \fi\fi\fi\fi\fi\fi \next@}
\xylet@\saveid@COORD@@=\relax
\xydef@\idfromc@#1{\DN@{#1}%
 \expandafter\edef\csname Q@\codeof\next@\endcsname{\cfromthec@}}
\xydef@\idfrombase@#1{\DN@{#1}%
 \expandafter\edef\csname Q@\codeof\next@\endcsname{\basefromthebase@}}
\xydef@\idfromstack@#1{%
 \toks@={\if\sempty@\else
 \xywarning@{loading on top of non-empty stack}\sinit@ \fi}%
 \count@=\s@bot \advance\count@\@ne
 \ifnum\count@>\s@top\else
 \loop@
 \expandafter\let\expandafter\next@\csname S@\the\count@\endcsname
 \expandafter\addtotoks@\expandafter{\next@}%
 \ifnum\count@<\s@top \advance\count@\@ne \addtotoks@{\spushc@}\repeat@
 \fi
 \DN@{#1}\edef\next@##1{%
 \def\expandafter\noexpand\csname Q@\codeof\next@\endcsname{##1}}%
 \expandafter\next@\expandafter{\the\toks@}}
\xydef@\saveid@COORD{%
 \begingroup \toks@={}\let\xy@=\xytotoks@ \change@oxy@\xy@
 \let\xy@@ix@=\xytotoks@@toksix@
 \afterCOORD{\expandafter\saveid@COORDi\expandafter{\the\toks@}}}
\xydef@\saveid@COORDi#1#2"#3"{\endgroup \xy@@{\idfromxy@{#3}{#1}}\xyFN@\POS@}
\xydef@\saveid@COORDii#1#2"#3"{\endgroup \xy@@{\idfromcxy@{#3}{#1}}\xyFN@\POS@}
\xydef@\idfromxy@#1#2{\DN@{#1}%
 \expandafter\def\csname Q@\codeof\next@\endcsname{#2}}
\xydef@\idfromcxy@#1#2{\DN@{#1}%
 \expandafter\edef\csname Q@\codeof\next@\endcsname{\cfromthec@#2}}
\xydef@\cfromid@#1{\DNii@{#1}\edef\nextii@{\codeof\nextii@}%
 \expandafter\let\expandafter\next@\csname Q@\nextii@\endcsname
 \ifx\next@\relax \xyerror@{<pos> \string"\nextii@\string" not defined}{}%
 \else \expandafter\next@\fi}
\message{objects,}
\xydef@\OBJECT@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\OBJECT@}%
 \else\ifcat A\noexpand\next \let\next@=\OBJECT@letter
 \else \let\next@=\OBJECT@other \fi\fi \next@}
\xydef@\OBJECT@letter{%
 \ifx i\next \DN@ i{\addtotoks@\Invisible@true \xyFN@\OBJECT@}%
 \else\ifx h\next\DN@ h{\addtotoks@\Hidden@true \xyFN@\OBJECT@}%
 \else\ifx o\next\DN@ o{\xywarning@{Obsolete o modifier used}\OBJECT@shape{o}}%
 \else\ifx x\next\DN@ x{\xywarning@{Obsolete x modifier used}\OBJECT@shape{}}%
 \else\ifx @\next\DN@ @##1##{%
\xywarning@{Impossible @ (letter) should not be here!!}
 \OBJECT@@{\dir##1}}%
 \else \let\next@=\OBJECT@direction
 \fi\fi\fi\fi\fi \next@}
\xydef@\OBJECT@other{%
 \ifx !\next \DN@!{\OBJECT@shift}%
 \else\addPLUS@\ifx \next \DN@{\OBJECT@change}%
 \else\addDASH@\ifx \next \DN@{\OBJECT@change}%
 \else\addEQ@\ifx \next \DN@{\OBJECT@set}%
 \else\ifx [\next
 \DN@[##1]{\xy@{[##1]}{\OBJECT@shape{##1}}}%
 \else\ifx ^\next \let\next@=\OBJECT@direction
 \else\ifx _\next \let\next@=\OBJECT@direction
 \else\ifx :\next \let\next@=\OBJECT@direction
 \else\ifx ?\next
 \DN@ ?{\xywarning@{\string? modifier used}\xyFN@\OBJECT@direction}%
 \else\ifx (\next
 \let\next@=\OBJECT@direction
 \else\addAT@\ifx\next \addAT@\DN@##1##{\OBJECT@@{\dir##1}}%
 \else \DN@##1##{\OBJECT@@{##1}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\prevEdge@@{\zeroEdge}
\xydef@\OBJECT@@#1#2{%
 \expandafter\def\expandafter\prevEdge@@\expandafter{\the\Edge@c}%
 \expandafter\Edge@c\expandafter{\objectEdge}%
 \Invisible@false\Hidden@false
 \def\Leftness@{.5}\def\Upness@{.5}%
 \gdef\preXY@style@{}\gdef\postXY@style@{}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\relax}%
 \DN@{#1}\ifx\next@\empty \DNii@{#2}%
 \ifx\nextii@\empty \DN@{\hbox\bgroup\no@}\else \let\next@=\objectbox \fi\fi
 \setbox\z@=\next@{#2}\L@c=\Leftness@\wdz@ \R@c=\wdz@ \advance\R@c-\L@c
 \D@c=\dp\z@ \advance\D@c\ht\z@ \U@c=\Upness@\D@c \advance\D@c-\U@c
 \R@p=\z@ \L@p=\L@c \U@p=\U@c \advance\U@p-\ht\z@ \D@p=-\U@p
 \the\toks@\toks@={}\setboxz@h{\kern\R@p \raise\U@p\boxz@}%
 \checkZeroEdge@
 \dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@ \ht\z@=\U@c \dp\z@=\D@c \boxz@
 \OBJECT@x}
\xydef@\adjustLR@{%
 \ifdim\zz@\wdz@ \L@c=\z@ \R@c=\z@ \dimen@=\Leftness@\p@
 \ifdim\dimen@<\z@ \L@c=\dimen@ \R@c=-\L@c
 \else\ifdim\dimen@>\p@ \L@c=\dimen@ \advance\L@c-\p@ \R@c=-\L@c \fi\fi
 \else \L@c=\Leftness@\wdz@ \R@c=\wdz@ \advance\R@c-\L@c \fi}
\xydef@\adjustUD@{\dimen@=\ht\z@ \advance\dimen@\dp\z@
 \ifdim\zz@\dimen@ \U@c=\z@ \D@c=\z@ \dimen@=\Upness@\p@
 \ifdim\dimen@<\z@ \U@c=\dimen@ \D@c=-\L@c
 \else\ifdim\dimen@>\p@ \U@c=\dimen@ \advance\U@c-\p@ \D@c=-\L@c \fi\fi
 \else \D@c=\dimen@ \U@c=\Upness@\dimen@ \advance\D@c-\U@c \fi}
\def\checkZeroEdge@{%
 \expandafter\DN@\expandafter{\the\Edge@c}\def\nextii@{\zeroEdge}%
 \ifx\next@\nextii@\Edge@c={\rectangleEdge}\fi
 \DN@{}\def\nextii@{}%
 \ifdim\zz@\L@c \ifdim\zz@\R@c \ifdim\zz@\U@c \ifdim\zz@\D@c
 \DN@{\Edge@c={\zeroEdge}}\fi\fi\fi\fi
 \next@}
\xydef@\OBJECT@x{\toks@={\egroup\def\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Drop@@}\def\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Connect@@}}%
 \edef\tmp@{\D@c=\the\D@c \U@c=\the\U@c \L@c=\the\L@c \R@c=\the\R@c
 \Edge@c={\expandafter\noexpand\the\Edge@c}%
 \ifInvisible@\noexpand\Invisible@true\else\noexpand\Invisible@false\fi
 \ifHidden@\noexpand\Hidden@true\else\noexpand\Hidden@false\fi
 \def\noexpand\Leftness@{\Leftness@}\def\noexpand\Upness@{\Upness@}}%
 \expandafter\addtotoks@\expandafter{\tmp@}\the\toks@}
\xynew@{if}\ifInvisible@
\xynew@{if}\ifHidden@
\xydef@\Leftness@{}
\xydef@\Upness@{}
\xydef@\Drop@@{\styledboxz@}
\xydef@\Connect@@{}
\xydef@\objectbox#1{\hbox{$\m@th\objectstyle{#1}$}}
\xylet@\objectstyle=\textstyle
\xydef@\object{\hbox\bgroup\resetStyle@\object@}
\xydef@\object@{%
 \edef\next@{={\DirectionfromtheDirection@}}\expandafter\toks@\next@
 \plainxy@ \xyFN@\OBJECT@}
\xydef@\composite#1#{\hbox\bgroup\composite@{#1}}
\xydef@\composite@#1#2{%
 \DN@{#1}\ifx\next@\empty\else\xywarning@{no variants of
 \string\composite\space allowed}\fi
 \global\setbox9=\hbox\bgroup
 \D@p=-\maxdimen \U@p=-\maxdimen \L@p=-\maxdimen \R@p=-\maxdimen
 \xyFN@\composite@i#2@}
\xydef@\composite@i{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\composite@i}%
 \else\ifx *\next \DN@ *{\xyFN@\composite@i}%
 \else\ifx @\next \DN@ @{\composite@x}%
 \xyerror@{<composite> object expected}{}\czeroEdge@
 \else \DN@{\composite@ii}\fi\fi\fi \next@}
\xydef@\composite@ii#1#{\composite@iii{#1}}
\xydef@\composite@iii#1#2{%
 \setbox\z@=\object#1{#2}%
 \ifInvisible@ \setboxz@h{}\else
 \setboxz@h{\kern-\L@c \boxz@}\ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ {\Drop@@}\fi
 \ifHidden@\else
 \ifdim\U@p<\U@c \U@p=\U@c \fi \ifdim\D@p<\D@c \D@p=\D@c \fi
 \ifdim\R@p<\R@c \R@p=\R@c \fi \ifdim\L@p<\L@c \L@p=\L@c \fi
 \fi
 \xyFN@\composite@iv}
\xydef@\composite@iv{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\composite@iv}%
 \else \ifx @\next \DN@ @{\composite@x}%
 \else \let\next@=\composite@i \fi\fi \next@}
\xydef@\composite@x{%
 \edef\tmp@{\egroup
 \D@c=\the\D@p \U@c=\the\U@p \L@c=\the\L@p \R@c=\the\R@p}\tmp@
 \setboxz@h{\kern\L@c\box9}\ht\z@=\U@c \dp\z@=\D@c
 \dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@
 \Edge@c={\rectangleEdge}\computeLeftUpness@ \boxz@
 \OBJECT@x}
\xydef@\computeLeftUpness@{%
 \dimen@=\L@c \advance\dimen@\R@c
 \ifdim\zz@\dimen@ \def\Connect@@{\straight@{\dottedSpread@\jot}}%
 \ifdim\zz@\L@c\else
 \DN@{\zeroEdge}\expandafter\DNii@\expandafter{\the\Edge@c}%
 \ifx\next@\nextii@\Edge@c={\rectangleEdge}\fi\fi
 \else \quotient@\Leftness@\L@c\dimen@ \fi
 \dimen@=\U@c \advance\dimen@\D@c 
 \ifdim\zz@\dimen@ \def\Connect@@{\straight@{\dottedSpread@\jot}}%
 \ifdim\zz@\U@c\else
 \DN@{\zeroEdge}\expandafter\DNii@\expandafter{\the\Edge@c}%
 \ifx\next@\nextii@\Edge@c={\rectangleEdge}\fi\fi
 \else \quotient@\Upness@\U@c\dimen@ \fi}
\xydef@\xybox#1{\xy#1\endxy \Edge@c={\rectangleEdge}\computeLeftUpness@}
\xydef@\OBJECT@shift{%
 \let\xy@=\xytotoks@ \afterVECTORorEMPTY
 {\OBJECT@shift@}%
 {\addtotoks@{\X@c=-\L@c \advance\X@c\R@p \advance\X@c\L@p \Y@c=\U@p}%
 \OBJECT@shift@}}
\xydef@\OBJECT@shift@{%
 \addtotoks@{\advance\U@p-\Y@c
 \advance\L@c\X@c \advance\R@c-\X@c \advance\D@c\Y@c \advance\U@c-\Y@c
 \computeLeftUpness@}%
 \let\xy@=\oxy@ \xyFN@\OBJECT@}
\xylet@\objectmargin@=\jot
\xylet@\objectwidth@=\z@
\xylet@\objectheight@=\z@
\xydef@\objectmargin{\afterADDOP{\Addop@@\objectmargin@}}
\xydef@\objectwidth{\afterADDOP{\Addop@@\objectwidth@}}
\xydef@\objectheight{\afterADDOP{\Addop@@\objectheight@}}
\xydef@\OBJECT@change{%
 \afterADDOP{%
 \addEQ@\ifx \next
 \addtotoks@{\X@c=\D@c \advance\X@c\U@c \Y@c=\L@c \advance\Y@c\R@c}%
 \else
 \addtotoks@{\X@c=\objectmargin@ \advance\X@c\X@c \Y@c=\X@c}%
 \fi
 \let\xy@=\xytotoks@ 
 \afterVECTORorEMPTY\OBJECT@change@\OBJECT@change@}}
\xydef@\OBJECT@set{%
 \afterADDOP{%
 \let\xy@=\xytotoks@ \afterVECTORorEMPTY\OBJECT@change@
 {\addtotoks@{\X@c=\objectwidth@ \Y@c=\objectheight@}\OBJECT@change@}}}
\xydef@\OBJECT@change@{%
 \addtotoks@{\advance\R@c\L@c \advance\R@p-\L@c \let\tmp@=\R@c}%
 \expandafter\addtotoks@\expandafter{\Addop@@\tmp@\X@c\R@c=\tmp@
 \L@c=\Leftness@\R@c \advance\R@p\L@c \advance\R@c-\L@c}%
 \addtotoks@{\advance\D@c\U@c \let\tmp@=\D@c}%
 \expandafter\addtotoks@\expandafter{\Addop@@\tmp@\Y@c\D@c=\tmp@
 \U@c=\Upness@\D@c \advance\D@c-\U@c}%
 \let\xy@=\oxy@ \xyFN@\OBJECT@}
\xydef@\afterADDOP#1{\def\afterADDOP@{#1}\xyFN@\ADDOP@}
\xylet@\afterADDOP@=\empty
\xydef@\ADDOP@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\ADDOP@}%
 \else\addPLUS@\ifx \next \addPLUS@\DN@{\xyFN@\ADDOP@plus}%
 \else\addDASH@\ifx \next \addDASH@\DN@{\xyFN@\ADDOP@minus}%
 \else\addEQ@\ifx \next
 \addEQ@\DN@{\def\Addop@@{\Addop@0+=}\afterADDOP@}%
 \else
 \DN@{\def\Addop@@{\Addop@0+=}\afterADDOP@}%
 \fi\fi\fi\fi \next@}
\xydef@\ADDOP@plus{%
 \addEQ@\ifx \next
 \addEQ@\DN@{\def\Addop@@{\Addop@0+<}\afterADDOP@}%
 \else
 \DN@{\def\Addop@@{\Addop@1+=}\afterADDOP@}%
 \fi \next@}
\xydef@\ADDOP@minus{%
 \addEQ@\ifx \next
 \addEQ@\DN@{\def\Addop@@{\Addop@0+>}\afterADDOP@}%
 \else
 \DN@{\def\Addop@@{\Addop@1-=}\afterADDOP@}%
 \fi \next@}
\xydef@\Addop@#1#2#3#4#5{%
 \dimen@=#4\relax \edef#4{\the\dimen@}%
 \dimen@=#1\dimen@ \advance\dimen@#2#5\relax
 \ifdim\dimen@#3#4\else \edef#4{\the\dimen@}\fi
 \ifx\xy@\xyinitial@\else \DN@##1{\xy@@{\edef#4{##1}\checkZeroEdge@}}%
 \expandafter\next@\expandafter{#4}\fi}
\xydef@\objectEdge{\rectangleEdge}
\xydefcsname@{shape [r]}{\advance\U@p\D@c \centerobject@
 \ifdim\L@c>\D@c
 \advance\R@c\L@c \L@c=.5\U@c \advance\L@c.5\D@c \advance\R@c-\L@c \fi
 \advance\U@p-\D@c}
\xydefcsname@{shape [l]}{\advance\U@p\D@c \centerobject@
 \ifdim\L@c>\D@c
 \advance\L@c\R@c \R@c=.5\U@c \advance\R@c.5\D@c \advance\L@c-\R@c \fi
 \advance\U@p-\D@c}
\xydefcsname@{shape [u]}{\advance\U@p\D@c \centerobject@
 \ifdim\D@c>\L@c
 \advance\U@c\D@c \D@c=.5\L@c \advance\D@c.5\R@c \advance\U@c-\D@c \fi
 \advance\U@p-\D@c}
\xydefcsname@{shape [d]}{\advance\U@p\D@c \centerobject@
 \ifdim\D@c>\L@c
 \advance\D@c\U@c \U@c=.5\L@c \advance\U@c.5\R@c \advance\D@c-\U@c \fi
 \advance\U@p-\D@c}
\xydefcsname@{shape [c]}{\advance\U@p\D@c \centerobject@ \advance\U@p-\D@c}
\xydef@\centerobject@{%
 \advance\D@c\U@c \D@c=.5\D@c \U@c=\D@c \advance\L@c\R@c \L@c=.5\L@c \R@c=\L@c}
\xydef@\OBJECT@shape#1{\DN@{shape [#1]}%
 \expandafter\let\expandafter\nextii@\csname\codeof\next@\endcsname
 \ifx\nextii@\relax\DN@{style [#1]}%
 \expandafter\let\expandafter\nextii@\csname\codeof\next@\endcsname
 \ifx\nextii@\relax \DN@{\OBJECT@shapei[#1]}%
 \else\DN@{\nextii@\xyFN@\OBJECT@}\fi
 \else \expandafter\addtotoks@\expandafter{\nextii@}%
 \DN@{\xyFN@\OBJECT@}%
 \fi \next@}
\xydefcsname@{shape []}{\the\Edge@c5\relax}%
\xydefcsname@{shape [Outer]}{\the\Edge@c5\relax}%
\xydefcsname@{shape [Inner]}{\the\Edge@c4\relax}%
\xydefcsname@{shape [o]}{\Edge@c={\circleEdge}\the\Edge@c5\relax 
 \Edge@c={\circleEdge}\def\prevEdge@@{\circleEdge}}
\xydefcsname@{shape [.]}{\czeroEdge@}
\def\OBJECT@shapei[#1#2]{\DN@{shape [#1...]}%
 \expandafter\let\expandafter\next\csname\codeof\next@\endcsname
 \ifx\next\relax\DN@{*stylechar@#1@}%
 \expandafter\let\expandafter\next\csname\codeof\next@\endcsname
 \ifx\next\relax\DNii@{shape [#1#2]}%
 \xywarning@{illegal [<shape>] ignored: \codeof\nextii@\space not defined}%
 \DN@{\xyFN@\OBJECT@}%
 \else% Delete this: \expandafter\addtotoks@\expandafter{\next{#2}}%
 \DN@{\next{#2}\xyFN@\OBJECT@}%
 \fi
 \else
\expandafter\addtotoks@\expandafter{\next{#2}}\DN@{\next{#2}\xyFN@\OBJECT@}%
 \fi \next@}
\xydef@\preXY@style@{}
\xydef@\postXY@style@{}
\xydef@\resetStyle@{\gdef\preXY@style@{}\gdef\postXY@style@{}}
\xynew@{toks}{\styletoks@}
\xydef@\addtostyletoks@#1{%
 \expandafter\styletoks@\expandafter{\the\styletoks@#1}}
\xydef@\styledboxz@{%
 \xypre@Style@@
 \boxz@
 \xypost@Style@@}
\xydef@\xypre@Style@{\styletoks@={}\saveXyStyle@\preXY@style@
 \expandafter\DN@\expandafter{\the\styletoks@}%
 \ifx\next@\empty \DN@{\let\xypre@Style@@=\relax 
 \let\xypost@Style@@=\relax \xypre@skipStyle@}%
 \else
 \let\xypre@Style@@=\relax \let\xypost@Style@@=\xypost@Style@
 \DN@{\expandafter\xydoprestyles@\expandafter{\the\styletoks@}}%
 \fi \next@ }
\xydef@\xypost@Style@{\styletoks@={}\postXY@style@
 \expandafter\xydopoststyles@\expandafter{\the\styletoks@}%
 \let\xypost@Style@@=\relax \let\xypre@Style@@=\xypre@Style@ }
\xydef@\xypre@skipStyle@#1\xypost@Style@@{#1\relax 
 \let\xypre@Style@@=\xypre@Style@ }
\xydef@\xydoprestyles@@{\literal@}
\xydef@\xydopoststyles@@{\literal@}
\xylet@\xydoprestyles@=\xydoprestyles@@
\xylet@\xydopoststyles@=\xydopoststyles@@
\xydef@\modXYstyle@{%
 \ifx\xy@style@\empty\resetStyle@\fi \checkXyStyle@
 \expandafter\expandafter\expandafter\DN@
 \expandafter\expandafter\expandafter{\preXYstyle@@}%
 \ifx\next@\empty\else\DN@{\modXYstyle@@}\fi \next@ }
\xydef@\modXYstyle@@{%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{##1}}%
 \expandafter\next@\expandafter{\preStyle@@}%
 \DN@##1{\expandafter\gdef\expandafter\preXY@style@\expandafter{%
 \preXY@style@ ##1}}\expandafter\next@\expandafter{\tmp@}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{##1}}%
 \expandafter\next@\expandafter{\postStyle@@}%
 \DN@##1{\expandafter\gdef\expandafter\postXY@style@\expandafter{%
 \tmp@ ##1}}\expandafter\next@\expandafter{\postXY@style@}}
\xydef@\xy@style@{}
\xydef@\checkXyStyle@{\ifx\xy@style@\empty\resetStyle@\fi
 \let\xy@style@=\relax}
\xydef@\preStyle@@{}
\xydef@\postStyle@@{}
\xydef@\preXYstyle@@{\relax}
\xydef@\loadxystyle@{%
 \let\xypre@Style@@=\xypre@Style@ \def\preXYstyle@@{\preStyle@@}}
\loadxystyle@
\xydef@\Unloadstyle@{%
 \let\xypre@Style@@=\relax \let\xypost@Style@@=\relax
 \def\preXYstyle@@{\relax}}
\xydefcsname@{shape [=...]}#1{\checkXyStyle@ \addtotoks@{\xynamestyle@{#1}}}
\xydef@\xynamestyle@#1{\checkXyStyle@
 \expandafter\DNii@\expandafter{\csname shape [#1]\endcsname}%
 \expandafter\ifx\nextii@\relax
 \else\xywarning@{Redefining style [#1]}\fi
 \expandafter\xynamestyle@@\csname shape [#1]\endcsname }
\xydef@\xynamestyle@@#1{%
 \expandafter\def\expandafter\tmp@\expandafter{\preXY@style@}%
 \DN@##1{\def\tmp@{\checkXyStyle@\gdef\preXY@style@{##1}}}%
 \expandafter\next@\expandafter{\preXY@style@}%
 \DN@##1{\expandafter\gdef\expandafter#1\expandafter{\tmp@
 \gdef\postXY@style@{##1}}}%
 \expandafter\next@\expandafter{\postXY@style@}\DN@{}}
\xydef@\prevXypreStyle@@{}
\xydef@\prevXypostStyle@@{}
\xydef@\saveXyStyle@{\expandafter
 \def\expandafter\prevXypreStyle@@\expandafter{\preXY@style@}%
 \expandafter\def\expandafter\prevXypostStyle@@\expandafter{%
 \postXY@style@}}
\xydef@\recoverXyStyle@{\expandafter
 \gdef\expandafter\preXY@style@\expandafter{\prevXypreStyle@@}%
 \expandafter\gdef\expandafter\postXY@style@\expandafter{%
 \prevXypostStyle@@}}
\xydef@\newxystyle#1#2#3{%
 \DN@{#3}\ifx\next@\empty 
 \xydefcsname@{shape [#1]}{\csname xyshape@#1@\endcsname}%
 \else \expandafter\def\csname shape [#1]\endcsname{%
 \csname xyshape@#1@\endcsname}\fi
 \DN@{#2}\ifx\next@\empty
 \expandafter\def\csname xyshape@#1@\endcsname{%
 \xyundefinedStyle@{#1}{}@@}%
 \else \expandafter\def\csname xyshape@#1@\endcsname{#2}\fi}
\xydef@\xyundefinedStyle@#1#2@@{%
 \xywarning@{style #1 not defined, nothing to apply}}
\xydef@\applyFIFOstyle@#1#2#3#4{\bgroup
 \styletoks@={\egroup\gdef\preXY@style@}%
 \expandafter\toks@\expandafter{\preXY@style@}%
 \expandafter\addtotoks@\expandafter{\expandafter#1\expandafter{#2}}%
 \expandafter\addtostyletoks@\expandafter{\expandafter{\the\toks@}%
 \gdef\postXY@style@}%
 \expandafter\toks@\expandafter{\expandafter#3\expandafter{#4}}%
 \expandafter\addtotoks@\expandafter{\postXY@style@}%
 \expandafter\addtostyletoks@\expandafter{\expandafter{\the\toks@}}%
 \the\styletoks@ }
\xydef@\applyLIFOstyle@#1#2#3#4{\bgroup
 \styletoks@={\egroup\gdef\preXY@style@}%
 \expandafter\toks@\expandafter{\expandafter#1\expandafter{#2}}%
 \expandafter\addtotoks@\expandafter{\preXY@style@}%
 \expandafter\addtostyletoks@\expandafter{\expandafter{\the\toks@}%
 \gdef\postXY@style@}%
 \expandafter\toks@\expandafter{\postXY@style@}%
 \expandafter\addtotoks@\expandafter{\expandafter#3\expandafter{#4}}%
 \expandafter\addtostyletoks@\expandafter{\expandafter{\the\toks@}}%
 \the\styletoks@ }
\xydef@\OBJECT@direction{\afterDIRECTIONorEMPTY{%
 \edef\next@{{\DirectionfromtheDirection@}}\expandafter\addtotoks@\next@
 \xyFN@\OBJECT@}%
 {\xyFN@\OBJECT@}}
\xydef@\afterDIRECTIONorEMPTY#1#2{%
 \DN@##1{\def\afterDIRECTION@{\def\afterDIRECTION@{##1}%
 \ifDIRECTIONempty@\DN@{#2}\else\DN@{#1}\fi \next@}}%
 \expandafter\next@\expandafter{\afterDIRECTION@}%
 \xyFN@\DIRECTION@}
\xylet@\afterDIRECTION@=\empty
\xynew@{if}\ifDIRECTIONempty@
\xydef@\DIRECTION@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\DIRECTION@}%
 \else\ifx v\next \DN@ v{\DIRECTION@v}%
 \else\ifx \bgroup\next \let\next@=\DIRECTION@group
 \else\ifx (\next \DN@({\xyFN@\DIRECTION@open}%
 \else
 \DN@{\count@=8
 \afterDIAG{\ifnum\count@=8 \DN@{\DIRECTIONempty@true \xyFN@\DIRECTION@i}%
 \else \DN@{\xy@@{\dimen@=\xydashl@}\Directionfromdiag@}\fi \next@}}%
 \fi\fi\fi\fi \next@}
\xydef@\DIRECTION@open{%
 \ifx *\next \DN@*##1*){\DIRECTION@group{##1}}%
 \else \DN@{\xyerror@{(* <pos> *) expected}{} \xyFN@\DIRECTION@i}%
 \fi \next@}
\def\afterDIAG#1{\def\afterDIAG@{#1}\xyFN@\DIAG@}
\xydef@\DIAG@{%
 \ifx d\next \DN@ d{\count@=1 \xyFN@\DIAG@@}%
 \else\ifx r\next \DN@ r{\count@=3 \xyFN@\DIAG@@}%
 \else\ifx u\next \DN@ u{\count@=5 \xyFN@\DIAG@@}%
 \else\ifx l\next \DN@ l{\count@=7 \xyFN@\DIAG@@}%
 \else \let\next@=\afterDIAG@
 \fi\fi\fi\fi \next@}
\xydef@\DIAG@@{\ifcase\count@ \or
 \DIAG@@@ l0r2\or\or \DIAG@@@ d2u4\or\or \DIAG@@@ r4l6\or\or \DIAG@@@ u6d0%
 \else\xybug@{impossible <diag> number}\fi
 \next@}
\xydef@\DIAG@@@#1#2#3#4{%
 \ifx #1\next \count@=#2\DN@#1{\afterDIAG@}%
 \else \ifx #3\next \count@=#4\DN@#3{\afterDIAG@}%
 \else \let\next@=\afterDIAG@ \fi\fi}
\xydef@\Directionfromdiag@{\ifcase\count@
 \xy@@{\dlDirection@\dimen@}%
 \or \xy@@{\dDirection@\dimen@}%
 \or \xy@@{\drDirection@\dimen@}%
 \or \xy@@{\rDirection@\dimen@}%
 \or \xy@@{\urDirection@\dimen@}%
 \or \xy@@{\uDirection@\dimen@}%
 \or \xy@@{\ulDirection@\dimen@}%
 \or \xy@@{\lDirection@\dimen@}%
 \or
 \else\xybug@{impossible <diag>}\fi
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}
\xydef@\DIRECTION@v{%
 \xy@{v}{\enter@{\cfromthec@ \X@origin=\the\X@origin \Y@origin=\the\Y@origin
 \X@p=\the\X@p \Y@p=\the\Y@p}%
 \X@origin=\z@ \Y@origin=\z@}%
 \afterVECTORorEMPTY
 {\xy@@{\X@p=\z@ \Y@p=\z@ \setupDirection@ \leave@}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}%
 {\xy@@\leave@ \xyerror@{<vector> expected after v}{}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}}
\xydef@\DIRECTION@group#1{%
 \xy@@{\begingroup}\xy@@ix@{#1}\xy@@{\plainxy@\expandafter\POS\the\toks9\relax
 \setupDirection@\edef\next@{\endgroup \DirectionfromtheDirection@}\next@}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}
\xydef@\DIRECTION@i{%
 \ifx ^\next \DN@ ^{\xy@^{\aboveDirection@\xydashl@}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}%
 \else\ifx _\next \DN@ _{\xy@_{\belowDirection@\xydashl@}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}%
 \else\ifx :\next \DN@ :{%
 \xy@{:}{\enter@{\cfromthec@ \basefromthebase@ \X@p=\the\X@p \Y@p=\the\Y@p}%
 \X@origin=\z@ \Y@origin=\z@
 \X@xbase=\cosDirection\xydashl@ \Y@xbase=\sinDirection\xydashl@
 \X@ybase=-\Y@xbase \Y@ybase=\X@xbase}%
 \afterVECTORorEMPTY
 {\xy@@{\X@p=\z@ \Y@p=\z@ \setupDirection@ \leave@}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}%
 {\xy@@\leave@ \xyerror@{<vector> expected after :}{}%
 \DIRECTIONempty@false \xyFN@\DIRECTION@i}}%
 \else
 \let\next@=\afterDIRECTION@
 \fi\fi\fi \next@}
\message{decorations;}
\xydef@\drop#1#{\DN@##1{\xy@@ix@{{#1}{##1}}%
 \xy@{\drop#1{##1}}{\expandafter\drop@\the\toks9 }\ignorespaces}\next@}
\xydef@\connect#1#{\DN@##1{\xy@@ix@{{#1}{##1}}%
 \xy@{\connect#1{##1}}{\expandafter\connect@\the\toks9 }\ignorespaces}\next@}
\xydef@\preconnect#1#{\DN@##1{\xy@@ix@{{#1}{##1}}%
 \xy@{\connect#1{##1}}{\expandafter\preconnect@\the\toks9 }\ignorespaces}\next@}
\xydef@\save{\relax\saveC}
\xydef@\saveC{\xy@\save\save@ \POS}
\xydef@\save@{\enter@{\cfromthec@ \pfromthep@ \basefromthebase@}}
\xydef@\restore{\xy@\restore\leave@ \ignorespaces}
\xydef@\xyecho{%
 \xy@\xyecho{\let\xy@=\xyecho@ \message{\string\xyecho}}\POS}
\xydef@\xyecho@#1#2{{\def\1{#1}\ifx\1\empty\else\message{\codeof\1}\fi}%
 \oxy@{#1}{#2}}
\xydef@\xyverbose{%
 \xy@\xyverbose{\let\xy@=\xyverbose@
 \W@{Xy: \string\xyverbose\xytracelineno@}}\POS}
\xydef@\xyverbose@#1#2{%
 {\def\1{#1}\ifx\1\empty\else\W@{Xy: \codeof\1\xytracelineno@}\fi}%
 \oxy@{#1}{#2}}
\xydef@\xytracing{%
 \xy@\xytracing{\let\xy@=\xytracing@
 \W@{Xy TRACE: \string\xytracing\xytracelineno@}\xystatus@:}\POS}
\xydef@\xytracing@#1#2{{\def\1{#1}\def\2{#2}%
 \W@{Xy TRACE: \codeof\1 {\codeof\2}\xytracelineno@}}\oxy@{#1}{#2}\xystatus@:}
\xydef@\xystatus@#1{\xystatus@cp{#1}%
 \W@{#1 d=<\the\d@X,\the\d@Y>
 Direction=\the\Direction=\string(\cosDirection,\sinDirection\string)}%
 \W@{#1 base=<\the\X@origin,\the\Y@origin>+%
 <\the\X@xbase,\the\Y@xbase>x+<\the\X@ybase,\the\Y@ybase>y}%
 \W@{#1 min/max=<\the\X@min,\the\Y@min>/<\the\X@max,\the\Y@max>
 S=\the\csp@}}
\xydef@\xystatus@cp#1{%
 \W@{#1 c=<\the\X@c,\the\Y@c> \expandafter\string\the\Edge@c
 \string[\the\L@c+\the\R@c,\the\D@c+\the\U@c\string]
 \ifInvisible@ I\fi\ifHidden@ H\fi}%
 \W@{#1 p=<\the\X@p,\the\Y@p> \expandafter\string\the\Edge@p
 \string[\the\L@p+\the\R@p,\the\D@p+\the\U@p\string]}}
\xydef@\xystatus@c#1{%
 \W@{#1<\the\X@c,\the\Y@c> \expandafter\string\the\Edge@c
 \string[\the\L@c+\the\R@c,\the\D@c+\the\U@c\string]}}
\xydef@\xyquiet{\xy@\xyquiet{\let\xy@=\oxy@}}
\xydef@\xyignore#1{\xy@\xyignore{\xyignore@{#1}}\ignorespaces}
\xydef@\xyignore@#1{{\let\xy@=\xyeat@ \change@oxy@\xy@ \POS#1\relax}}
\xydef@\xyeat@#1#2{}
\xydef@\xycompile@@{\jobname-}
\xydef@\xycompileno@@{0}
\xydef@\CompilePrefix#1{%
 \def\xycompile@@{#1}\xdef\xycompile@@{\codeof\xycompile@@}%
 \xdef\xycompileno@@{0}}
\xydef@\xycompile{%
 \count@=\xycompileno@@ \advance\count@\@ne
 \xdef\xycompileno@@{\ifnum10>\count@ 0\fi \the\count@}%
 \edef\next{\noexpand\xycompileto{\xycompile@@\xycompileno@@}}\next}
\xylet@\compilename@@=\empty
\xylet@\xyrecompile@@=\relax
\xydef@\xycompileto#1#2{%
 \if\inxy@ \DN@{\xy@@{\nter@{}}}%
 \else \DN@{\xy \xy@@{\nter@{\endxy}}}\fi \next@
 \ifxysaving@ \xyerror@{Compilations can not be nested}{}\fi
 \DN@{#1}\edef\compilename@@{\codeof\next@}\DNii@{#2}%
 \def\xyrecompile@@{recompiling TRUNCATED}%
 \expandafter\xyinputorelse@@\expandafter{\compilename@@.xyc}%
 {\def\xyrecompile@@{compiling to}}%
 \ifx\xyrecompile@@\relax \else \expandafter\xyrecompile@ \fi
 \xy@@\leave@ \ignorespaces}
\xydef@\xyrecompile@{%
 \message{(\xyrecompile@@\space\string`\compilename@@.xyc\string'}%
 \DN@{\immediate\openout\xywrite@=}\expandafter\next@\compilename@@.xyc
 \immediate\write\xywrite@{%
 \string\xycompiled{\compilename@@}%
 {\the\year/\the\month/\the\day\string:\the\time\xytracelineno@}%
 {Xy-pic \xyversion}\xycomment@}%
 \immediate\write\xywrite@{{\codeof\nextii@}\relax}%
 {\xysaving@ \expandafter\POS\nextii@ \relax}%
 \immediate\write\xywrite@{\string\xyendcompiled}%
 \immediate\closeout\xywrite@ \message{done)}%
 \expandafter\input\compilename@@.xyc
 \outlines@@\writeoutline@\writeoutline@}
\xydef@\xysaving@{\let\xy@=\xysave@ \change@oxy@\xy@
 \let\xy@@ix@=\xysave@@toksix@ \xysaving@true}
\xynew@{if}\ifxysaving@ \xysaving@false
\xydef@\xysave@#1#2{{\DN@{{#1}{#2}}%
 \immediate\write\xywrite@{\string\xy@\codeof\next@\xycomment@}}}
\xydef@\xysave@@toksix@#1{{\DN@{{#1}}%
 \immediate\write\xywrite@{\string\xy@@ix@\codeof\next@\relax}}}
\xywarnifdefined\xycomment@
{\catcode`\%=12 \catcode`\(=1 \catcode`\)=2 \gdef\xycomment@(%)}
\xydef@\xycompiled#1#2#3#4{\DN@{#1}\edef\next@{\codeof\next@}%
 \ifx\next@\compilename@@\else
 \xywarning@{This file does not contain the result of
 \string\xycompileto{\compilename@@}{...}^^J%
 but of \string\xycompileto{\next@}}\fi
 \edef\next{Xy-pic \xyversion}\DN@{#3}\ifx\next\next@
 \DN@{#4}\ifx\next@\nextii@ \xycatcodes \outlines@@\relax\readoutline@
 \else \def\xyrecompile@@{recompiling to}\endinput \fi
 \else \def\xyrecompile@@{Xy-pic version change - recompiling}\endinput \fi}
\xydef@\xyendcompiled{\let\xyrecompile@@=\relax \xyuncatcodes\endinput}
\xydef@\CompileFixPoint#1{%
 \expandafter\ifx\csname#1FIX@@\endcsname\relax
 \expandafter\xdef\csname#1FIX@@\endcsname{\xycompileno@@}%
 \else
 \xdef\xycompileno@@{\csname#1FIX@@\endcsname}\fi}
\xydef@\outlines@no#1#2{}
\xydef@\outlines@make#1#2{#1}
\xydef@\outlines@only#1#2{#2}
\xylet@\outlines@@=\outlines@no
\xylet@\writeoutline@@=\relax
\xylet@\readoutline@@=\relax
\xydef@\MakeOutlines{\let\outlines@@=\outlines@make}
\xydef@\OnlyOutlines{\xywarning@{Compiled pictures only shown as outlines}%
 \let\outlines@@=\outlines@only}
\xydef@\ShowOutlines{\let\readoutline@@=\typesetoutline@}
\xydef@\NoOutlines{\let\outlines@@=\outlines@no}
\xydef@\writeoutline@{%
 \DN@{\immediate\openout\xywrite@=}\expandafter\next@\compilename@@.xyd
 \immediate\write\xywrite@{\xycomment@\space\compilename@@.xyd}
 \immediate\write\xywrite@{%
 \string\X@min=\the\X@min \string\X@max=\the\X@max
 \string\Y@min=\the\Y@min \string\Y@max=\the\Y@max \string\relax}%
 \writeoutline@@
 \immediate\closeout\xywrite@}
\xynew@{if}\ifoutlineread@
\xydef@\readoutline@{\outlineread@true
 \expandafter\xyinputorelse@@\expandafter{\compilename@@.xyd}%
 {\def\xyrecompile@@{outline missing - recompiling to}\outlineread@false}%
 \ifoutlineread@ \readoutline@@
 \writeoutline@\expandafter\xyendcompiled\fi}
\xydef@\typesetoutline@{%
 \xy@@{\czeroEdge@ \U@p=\z@ \D@p=\z@ \L@p=\z@ \R@p=\z@ \Edge@p={\zeroEdge}%
 \X@p=\X@min \Y@p=\Y@min \X@c=\X@min \Y@c=\Y@max \connect@\dir{.}%
 \X@p=\X@c \Y@p=\Y@c \X@c=\X@max \Y@c=\Y@max \connect@\dir{.}%
 \X@p=\X@c \Y@p=\Y@c \X@c=\X@max \Y@c=\Y@min \connect@\dir{.}%
 \X@p=\X@c \Y@p=\Y@c \X@c=\X@min \Y@c=\Y@min \connect@\dir{.}}}
\message{kernel objects:}
\message{directionals,}
\xydef@\dir{\hbox\bgroup\xyFN@\dir@i}
\xydef@\dir@i{\ifx *\next \DN@*{\resetStyle@\object@}%
 \else \let\next@=\dir@ii \fi \next@}
\xydef@\dir@ii#1#{\dir@{#1}}
\xydef@\dir@#1#2{\DN@{dir#1{#2}}%
 \expandafter\let\expandafter\next\csname\codeof\next@\endcsname
 \ifx\next\relax \DN@{dir{#2}}%
 \expandafter\let\expandafter\next\csname\codeof\next@\endcsname
 \ifx\next\relax \DN@{\dir#1{#2}}%
 \xyerror@{illegal <dir>: \codeof\next@\space not defined}{}%
 \let\next=\no@ \fi\fi \next}
\xydefcsname@{dir{}}{\no@}
\xyletcsnamecsname@{dir0{}}{dir{}}
\xyletcsnamecsname@{dir1{}}{dir{}}
\xyletcsnamecsname@{dir^{}}{dir{}}
\xyletcsnamecsname@{dir_{}}{dir{}}
\xyletcsnamecsname@{dir2{}}{dir{}}
\xyletcsnamecsname@{dir3{}}{dir{}}
\xyletcsnamecsname@{dir{ }}{dir{}}
\xydef@\no@{\egroup \czeroEdge@
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\setbox\z@=\copy\voidb@x}\def\Connect@@{\no@@}}
\xydefcsname@{dir1{-}}{\line@}
\xydefcsname@{dir2{-}}{\line@ \double@\xydashh@}
\xydefcsname@{dir3{-}}{\line@ \triple@\xydashh@}
\xyletcsnamecsname@{dir0{-}}{dir{}}
\xyletcsnamecsname@{dir{-}}{dir1{-}}
\xyletcsnamecsname@{dir{=}}{dir2{-}}
\xydef@\line@{\dimen@=\sd@Y\sinDirection\xydashl@
 \ifnum\SemiDirectionChar<31 \D@c=\z@ \U@c=\dimen@ \DN@{\d@Y<\z@}%
 \else\ifnum\SemiDirectionChar<64 \D@c=\dimen@ \U@c=\z@ \DN@{\z@<\d@Y}%
 \else\ifnum\SemiDirectionChar<96 \D@c=\dimen@ \U@c=\z@ \DN@{\d@X<\z@}%
 \else \D@c=\z@ \U@c=\dimen@ \DN@{\d@X<\z@}\fi\fi\fi
 \setboxz@h{\line@@}\ht\z@=\U@c \dp\z@=\D@c
 \L@c=\z@ \R@c=\wdz@
 \ifdim\next@ \dimen@=\R@c \R@c=\L@c \L@c=\dimen@
 \dimen@=\U@c \U@c=\D@c \D@c=\dimen@ \advance\dimen@-\U@c
 \lower\dimen@\boxz@
 \else \boxz@ \fi
 \edef\tmp@{\egroup \U@c=\the\U@c \D@c=\the\D@c \L@c=\the\L@c \R@c=\the\R@c}%
 \tmp@
 \Edge@c={\rectangleEdge}%
 \ifdim\z@<\U@c \def\Upness@{1}\else \def\Upness@{0}\fi
 \ifdim\z@<\L@c \def\Leftness@{1}\else \def\Leftness@{0}\fi
 \def\Drop@@{\styledboxz@}\def\Connect@@{\solid@}}
\xydef@\line@@{{\xydashfont\SemiDirectionChar\/}}
\xydef@\solid@{%
 \checkXy@rules@\solidhrule@\solidvrule@{\straight@\solidSpread@}}
\xydef@\checkXy@rules@#1#2#3{%
 \dimen@=\Y@c \advance\dimen@-\Y@p
 \ifjusthvtest@.05pt>\ifdim\dimen@<\z@-\fi\dimen@ \DN@{#1}%
 \else \dimen@=\X@c \advance\dimen@-\X@p
 \ifjusthvtest@.05pt>\ifdim\dimen@<\z@-\fi\dimen@ \DN@{#2}%
 \else \DN@{#3}\fi\fi \next@}
\xydef@\solidSpread@{\ifnum\z@<\count@@ \advance\count@@\@ne \fi}
\xylet@\ifjusthvtest@=\ifdim
\xydef@\NoRules{\let\ifjusthvtest@=\iffalse}
\xydef@\UseRules{\let\ifjusthvtest@=\ifdim}
\xydef@\solidvrule@{\no@@ \solidvrule@typeset \ifHidden@\else\noinsert@\fi
 \solidvrule@pre}
\xydef@\solidvrule@pre{%
 \def\Cbreak@@{%
 \connectRestore@ \swap@\lastbreak@@\swap@
 \solidvrule@typeset \edef\lastbreak@@{\cfromthec@}\Creset@@}%
 \def\Clast@@{%
 \connectRestore@ \Creset@@\swap@\lastbreak@@\swap@
 \solidvrule@typeset \Creset@@ \edef\lastbreak@@{\cfromthep@}}%
}
\xydef@\solidvrule@typeset{%
 \ifInvisible@ \let\next@=\relax \else \let\next@=\solidvrule@typeset@ \fi
 \checkoverlap@@ \next@}
\xydef@\solidvrule@typeset@{{%
 \advance\X@c\X@p \X@c=.5\X@c \X@p=\X@c
 \advance\X@c-.5\xydashw@ \advance\X@p.5\xydashw@
 \ifdim\Y@c<\Y@p \advance\Y@c\U@c \advance\Y@p-\D@p
 \else \swapdimen@\Y@c\Y@p \advance\Y@c\U@p \advance\Y@p-\D@c \fi
 \Droprule@}}
\xydef@\solidhrule@{\no@@ \solidhrule@typeset \ifHidden@\else\noinsert@\fi
 \solidhrule@pre}
\xydef@\solidhrule@pre{%
 \def\Cbreak@@{%
 \connectRestore@ \swap@\lastbreak@@\swap@
 \solidhrule@typeset \edef\lastbreak@@{\cfromthec@}\Creset@@}%
 \def\Clast@@{%
 \connectRestore@ \Creset@@\swap@\lastbreak@@\swap@
 \solidhrule@typeset \Creset@@ \edef\lastbreak@@{\cfromthep@}}%
}
\xydef@\solidhrule@typeset{%
 \ifInvisible@ \let\next@=\relax \else \let\next@=\solidhrule@typeset@ \fi
 \checkoverlap@@ \next@}
\xydef@\solidhrule@typeset@{{%
 \ifdim\X@c<\X@p \advance\X@c\R@c \advance\X@p-\L@p
 \else \swapdimen@\X@c\X@p \advance\X@c\R@p \advance\X@p-\L@c \fi
 \advance\Y@c\Y@p \Y@c=.5\Y@c \Y@p=\Y@c
 \advance\Y@c-.5\xydashw@ \advance\Y@p.5\xydashw@
 \Droprule@}}
\xydef@\Droprule@{\advance\X@p-\X@c
 \setboxz@h{\kern\X@c \vrule width\X@p depth-\Y@c height\Y@p}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ \Drop@@}
\xydef@\zerodot{\copy\zerodotbox@}
\xydefcsname@{dir1{.}}{\point@}
\xydefcsname@{dir2{.}}{\point@ \double@\xydashh@}
\xydefcsname@{dir3{.}}{\point@ \triple@\xydashh@}
\xyletcsnamecsname@{dir0{.}}{dir{}}
\xyletcsnamecsname@{dir{.}}{dir1{.}}
\xyletcsnamecsname@{dir{:}}{dir2{.}}
\xydef@\point@{\pointlike@\zerodot\p@}
\xydef@\pointlike@#1#2{%
 \setboxz@h{#1}\wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@\egroup
 \def\Leftness@{.5}\def\Upness@{.5}\ctipEdge@
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@{#2}}}}
\xydef@\dottedSpread@#1{%
 \dimen@=#1\relax \DN@{\A@=2\A@ \B@=2\B@ \dottedSpread@i}%
 \A@=\sd@X\cosDirection\dimen@ \B@=\sd@Y\sinDirection\dimen@
 \dimen@=\A@ \advance\dimen@\B@
 \dimen@ii=\sd@X\d@X \advance\dimen@ii\sd@Y\d@Y
 \ifdim\dimen@>\dimen@ii \DN@{\count@@=\z@}\fi
 \next@}
\xydef@\dottedSpread@i{%
 \global\setbox8=\hbox to\A@{\hss
 \kern.5\A@\box\lastobjectbox@\kern.5\A@\hss}\dp8=.5\B@ \ht8=.5\B@
 \advance\d@X\sd@X\A@ \advance\d@Y\sd@Y\B@
 \advance\X@c\sd@X.5\A@ \advance\Y@c\sd@Y.5\B@
 \ifdim\sd@Y\d@Y<\sd@X\d@X \dimen@=\sd@X\d@X
 \ifdim\zz@\A@\else \divide\dimen@\A@ \fi \count@@=\dimen@
 \else \dimen@=\sd@Y\d@Y
 \ifdim\zz@\B@\else \divide\dimen@\B@ \fi \count@@=\dimen@
 \fi \advance\count@@\@ne}
\xydefcsname@{dir1{~}}{\squiggle@}
\xydefcsname@{dir2{~}}{\squiggle@ \double@\xybsqlh@}
\xydefcsname@{dir3{~}}{\squiggle@ \triple@\xybsqlh@}
\xyletcsnamecsname@{dir0{~}}{dir{}}
\xyletcsnamecsname@{dir{~}}{dir1{~}}
\xydef@\squiggle@{\xybsqlfont
 \dimen@=\sd@X\cosDirection\xybsqll@ \advance\dimen@.1\p@
 \dimen@ii=\sd@Y\sinDirection\xybsqll@
 \kern\dimen@\squiggle@@
 \edef\tmp@{\egroup \U@c=\the\dimen@ii \L@c=\the\dimen@}\tmp@
 \wdz@=2\L@c \R@c=\L@c \ht\z@=\U@c \D@c=\U@c \dp\z@=\U@c
 \Edge@c={\rectangleEdge}%
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\squiggledSpread@}}
\xydef@\squiggle@@{\DirectionChar \count@=\DirectionChar
 \advance\count@-64 \ifnum\count@<\z@ \advance\count@128 \fi \char\count@}
\xydef@\squiggledSpread@{%
 \dimen@=\d@X \advance\dimen@-\sd@X\count@@\A@ \advance\dimen@\sd@X.3\p@
 \advance\X@c-.5\dimen@ \advance\d@X-\dimen@
 \dimen@=\d@Y \advance\dimen@-\sd@Y\count@@\B@ \advance\dimen@\sd@Y.3\p@
 \advance\Y@c-.5\dimen@ \advance\d@Y-\dimen@}
\xydef@\double@#1{\edef\Drop@@{\dimen@=#1\relax
 \dimen@=.5\dimen@ \A@=-\sinDirection\dimen@ \B@=\cosDirection\dimen@
 \setboxz@h{\setbox2=\hbox{\kern\A@\raise\B@\copy\z@}%
 \dp2=\z@ \ht2=\z@ \wd2=\z@ \box2
 \setbox2=\hbox{\kern-\A@\raise-\B@ \noexpand\boxz@}%
 \dp2=\z@ \ht2=\z@ \wd2=\z@ \box2 }%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \noexpand\styledboxz@}}
\xydef@\triple@#1{\edef\Drop@@{\dimen@=#1\relax
 \A@=-\sinDirection\dimen@ \B@=\cosDirection\dimen@
 \setboxz@h{\setbox2=\hbox{\kern\A@\raise\B@\copy\z@}%
 \dp2=\z@ \ht2=\z@ \wd2=\z@ \box2
 \setbox2=\hbox{\kern-\A@\raise-\B@\copy\z@}%
 \dp2=\z@ \ht2=\z@ \wd2=\z@ \box2
 \dp\z@=\z@ \ht\z@=\z@ \wdz@=\z@ \noexpand\boxz@}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \noexpand\styledboxz@}}
\xydefcsname@{dir1{--}}{\dash@}
\xydefcsname@{dir2{--}}{\dash@ \double@\xydashh@}
\xydefcsname@{dir3{--}}{\dash@ \triple@\xydashh@}
\xyletcsnamecsname@{dir0{--}}{dir{}}
\xyletcsnamecsname@{dir{--}}{dir1{--}}
\xyletcsnamecsname@{dir{==}}{dir2{--}}
\xydef@\dash@{\line@ \wdz@=2\wdz@ \ht\z@=2\ht\z@ \dp\z@=2\dp\z@
 \multiply\D@c\tw@ \multiply\U@c\tw@ \multiply\L@c\tw@ \multiply\R@c\tw@
 \def\Connect@@{\straight@\dashedSpread@}}
\xydef@\dashedSpread@{\ifnum\z@<\count@@ \advance\count@@\@ne \fi
 \advance\d@X\sd@X.5\A@ \advance\d@Y\sd@Y.5\B@
 \ifdim\z@<\d@X \advance\X@c.5\A@ \fi \advance\Y@c\sd@Y.5\B@}
\xydefcsname@{dir1{~~}}{\dashsquiggle@}
\xydefcsname@{dir2{~~}}{\dashsquiggle@ \double@\xybsqlh@}
\xydefcsname@{dir3{~~}}{\dashsquiggle@ \triple@\xybsqlh@}
\xyletcsnamecsname@{dir0{~~}}{dir{}}
\xyletcsnamecsname@{dir{~~}}{dir1{~~}}
\xydef@\dashsquiggle@{\squiggle@
 \multiply\D@c\tw@ \multiply\U@c\tw@ \multiply\L@c\tw@ \multiply\R@c\tw@
 \dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@ \ht\z@=\U@c \dp\z@=\D@c
 \def\Connect@@{\straight@\dashsquiggledSpread@}}
\xydef@\dashsquiggledSpread@{\ifnum\z@<\count@@ \advance\count@@\@ne \fi
 \advance\X@c.5\A@ \advance\d@X.5\A@ \advance\Y@c.25\B@ \advance\d@Y.5\B@}
\xyletcsnamecsname@{dir1{..}}{dir{.}}
\xyletcsnamecsname@{dir2{..}}{dir2{.}}
\xyletcsnamecsname@{dir3{..}}{dir3{.}}
\xyletcsnamecsname@{dir{..}}{dir1{.}}
\xyletcsnamecsname@{dir{::}}{dir2{.}}
\xylet@\ctipEdge@=\czeroEdge@
\xydefcsname@{dir1{>}}{\tip@}
\xydefcsname@{dir^{>}}{\atip@}
\xydefcsname@{dir_{>}}{\btip@}
\xyletcsnamecsname@{dir0{>}}{dir{}}
\xyletcsnamecsname@{dir{>}}{dir1{>}}
\xydefcsname@{dir1{<}}{\reverseDirection@\tip@}
\xydefcsname@{dir^{<}}{\reverseDirection@\btip@}
\xydefcsname@{dir_{<}}{\reverseDirection@\atip@}
\xyletcsnamecsname@{dir0{<}}{dir{}}
\xyletcsnamecsname@{dir{<}}{dir1{<}}
\xydef@\tip@{\tip@x\tip@@}
\xydef@\atip@{\tip@x\atip@@}
\xydef@\btip@{\tip@x\btip@@}
\xydef@\tip@x#1{#1\egroup
 \ctipEdge@
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@\jot}}}
\xydef@\tip@@{\atip@@\btip@@}
\xydef@\atip@@{\xyatipfont\DirectionChar}
\xydef@\btip@@{\xybtipfont\DirectionChar}
\xydefcsname@{dir2{>}}{\Tip@}
\xydefcsname@{dir2{<}}{\reverseDirection@\Tip@}
\xydef@\Tip@{\kern2.5pt \vrule height2.5pt depth2.5pt width\z@
 \Tip@@ \kern2.5pt \egroup
 \U@c=2.5pt \D@c=2.5pt \L@c=2.5pt \R@c=2.5pt \Edge@c={\circleEdge}%
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@\jot}}}
\xydef@\Tip@@{\count@=\DirectionChar
 \advance\count@-4 \ifnum\count@<\z@ \advance\count@128 \fi
 \xyatipfont\char\count@
 \advance\count@ 8 \ifnum127<\count@ \advance\count@-128 \fi
 \xybtipfont\char\count@}
\xydefcsname@{dir3{>}}{\Ttip@}
\xydefcsname@{dir3{<}}{\composite@{}{:(-1,0)\dir3{>}}}
\xydef@\Ttip@{\kern3.2pt \vrule height3.2pt depth3.2pt width\z@
 \Ttip@@ \kern3.2pt \egroup
 \U@c=3.2pt \D@c=3.2pt \L@c=3.2pt \R@c=3.2pt \Edge@c={\circleEdge}%
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@\jot}}}
\xydef@\Ttip@@{%
 \setboxz@h\bgroup\reverseDirection@\line@ \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@
 \kern-\L@c \boxz@ \kern\L@c
 {\vDirection@(1,-.31)\xydashl@ \xyatipfont\char\DirectionChar}%
 {\vDirection@(1,+.31)\xydashl@ \xybtipfont\char\DirectionChar}}
\xydefcsname@{dir1{|}}{\stopper@}
\xydefcsname@{dir^{|}}{\aboveDirection@\xydashl@
 \shiftdir@\line@\z@ \pointlike@{}\xydashh@}
\xydefcsname@{dir_{|}}{\belowDirection@\xydashl@
 \shiftdir@\line@\z@ \pointlike@{}\xydashh@}
\xydefcsname@{dir2{|}}{\stopper@ \double@\xydashh@}
\xydefcsname@{dir3{|}}{\stopper@ \double@{2\xydashh@}}
\xyletcsnamecsname@{dir0{|}}{dir{}}
\xyletcsnamecsname@{dir{|}}{dir1{|}}
\xydef@\stopper@{\tip@x\stopper@@}
\xydef@\stopper@@{\setboxz@h{\count@=\SemiDirectionChar \advance\count@64
 \ifnum127<\count@ \advance\count@-128 \fi \xydashfont\char\count@\/}%
 \setboxz@h{\kern-.5\wdz@ \dimen@=\sd@Y\cosDirection\xydashl@ 
 \ifnum\SemiDirectionChar=95 \dimen@=\sd@X\sd@Y\dimen@ \fi
 \raise.5\dimen@\boxz@}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydefcsname@{dir1{(}}{\hook@}
\xydefcsname@{dir^{(}}{\ahook@}
\xydefcsname@{dir_{(}}{\bhook@}
\xyletcsnamecsname@{dir0{(}}{dir{}}
\xyletcsnamecsname@{dir{(}}{dir1{(}}
\xydefcsname@{dir1{)}}{\reverseDirection@\hook@}
\xydefcsname@{dir^{)}}{\reverseDirection@\bhook@}
\xydefcsname@{dir_{)}}{\reverseDirection@\ahook@}
\xyletcsnamecsname@{dir0{)}}{dir{}}
\xyletcsnamecsname@{dir{)}}{dir1{)}}
\xydef@\hook@{\tip@x\hook@@}
\xydef@\hook@@{\setboxz@h{\xybsqlfont
 \vDirection@(1,-1){.707107\xybsqll@}%
 \hbox{\DirectionChar
 \kern-\d@Y\raise\d@X\hbox{\count@=\DirectionChar \advance\count@-32
 \ifnum\count@<\z@ \advance\count@128 \fi \char\count@}}}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\ahook@{\tip@x\ahook@@}
\xydef@\ahook@@{\setboxz@h{\xybsqlfont
 \vDirection@(1,-1){.707107\xybsqll@}\kern-\d@X
 \lower\d@Y\hbox{\DirectionChar
 \kern-\d@Y\raise\d@X\hbox{\count@=\DirectionChar \advance\count@-32
 \ifnum\count@<\z@ \advance\count@128 \fi \char\count@}}}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\bhook@{\tip@x\bhook@@}
\xydef@\bhook@@{\setboxz@h{\xybsqlfont
 \vDirection@(-1,-1){.707107\xybsqll@}\DirectionChar
 \kern\d@X\raise\d@Y\hbox{\count@=\DirectionChar \advance\count@-96
 \ifnum\count@<\z@ \advance\count@128 \fi \char\count@}}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydefcsname@{dir^{'}}{\reverseDirection@\bturn@}
\xydefcsname@{dir_{'}}{\reverseDirection@\aturn@}
\xydefcsname@{dir^{`}}{\aturn@}
\xydefcsname@{dir_{`}}{\bturn@}
\xydef@\aturn@{\tip@x\aturn@@}
\xydef@\aturn@@{\setboxz@h{\xybsqlfont
 \vDirection@(1,-1){.707107\xybsqll@}\kern-\d@X
 \lower\d@Y\hbox{\DirectionChar}}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\bturn@{\tip@x\bturn@@}
\xydef@\bturn@@{\setboxz@h{\xybsqlfont
 \vDirection@(-1,-1){.707107\xybsqll@}\DirectionChar}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\newdir#1#{\newdir@{#1}}
\xydef@\newdir@#1#2#3{\xydefcsname@{dir#1{#2}}{\composite@{}{#3}}}
\xydef@\shiftdir@#1#2{%
 \setbox\z@=\hbox\bgroup#1\relax
 \setboxz@h{\dimen@ii=#2\relax
 \dimen@=-\cosDirection\dimen@ii \advance\dimen@-\L@c
 \kern\dimen@ \lower\sinDirection\dimen@ii\boxz@}%
 \wdz@\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xylet@\tipjot@=\jot
\xydefcsname@{dir1{>>}}{\shiftdir@\tip@\tipjot@ \tip@}
\xydefcsname@{dir^{>>}}{\shiftdir@\atip@\tipjot@ \atip@}
\xydefcsname@{dir_{>>}}{\shiftdir@\btip@\tipjot@ \btip@}
\xydefcsname@{dir2{>>}}{\composite@{}{h!/\tipjot@/\dir2{>}*\dir2{>}}}
\xydefcsname@{dir3{>>}}{\composite@{}{h!/\tipjot@/\dir3{>}*\dir3{>}}}
\xyletcsnamecsname@{dir0{>>}}{dir{}}
\xyletcsnamecsname@{dir{>>}}{dir1{>>}}
\xydefcsname@{dir1{<<}}{\reverseDirection@ \shiftdir@\tip@\tipjot@ \tip@}
\xydefcsname@{dir^{<<}}{\reverseDirection@ \shiftdir@\btip@\tipjot@ \btip@}
\xydefcsname@{dir_{<<}}{\reverseDirection@ \shiftdir@\atip@\tipjot@ \atip@}
\xydefcsname@{dir2{<<}}{\composite@{}{h!/-\tipjot@/\dir2{<}*\dir2{<}}}
\xydefcsname@{dir3{<<}}{\composite@{}{h!/-\tipjot@/\dir3{<}*\dir3{<}}}
\xyletcsnamecsname@{dir0{<<}}{dir{}}
\xyletcsnamecsname@{dir{<<}}{dir1{<<}}
\xydefcsname@{dir1{||}}{\shiftdir@\stopper@\xydashh@ \shiftdir@\stopper@\z@
 \pointlike@{}\jot}
\xydefcsname@{dir^{||}}{\shiftdir@{\aboveDirection@\xydashl@\line@}\xydashh@
 \shiftdir@{\aboveDirection@\xydashl@\line@}\z@ \pointlike@{}\jot}
\xydefcsname@{dir_{||}}{\shiftdir@{\belowDirection@\xydashl@\line@}\xydashh@
 \shiftdir@{\belowDirection@\xydashl@\line@}\z@ \pointlike@{}\jot}
\xydefcsname@{dir2{||}}{\shiftdir@\stopper@\xydashh@ \shiftdir@\stopper@\z@
 \pointlike@{}\jot \double@\xydashh@}
\xydefcsname@{dir3{||}}{\shiftdir@\stopper@\xydashh@ \shiftdir@\stopper@\z@
 \pointlike@{}\jot \double@{2\xydashh@}}
\xyletcsnamecsname@{dir0{||}}{dir{}}
\xyletcsnamecsname@{dir{||}}{dir1{||}}
\xydefcsname@{dir1{>|}}{\shiftdir@\stopper@\z@ \tip@}
\xydefcsname@{dir2{>|}}{\composite@{}{\dir2{>}*\dir2{|}}}
\xydefcsname@{dir3{>|}}{\composite@{}{\dir3{>}*\dir3{|}}}
\xyletcsnamecsname@{dir0{>|}}{dir{}}
\xyletcsnamecsname@{dir{>|}}{dir1{>|}}
\xydefcsname@{dir1{>>|}}{\shiftdir@\stopper@\z@ \shiftdir@\tip@\tipjot@ \tip@}
\xydefcsname@{dir2{>>|}}{\composite@{}{h!/\tipjot@/\dir2{>}*\dir2{>}*\dir2{|}}}
\xydefcsname@{dir3{>>|}}{\composite@{}{h!/\tipjot@/\dir3{>}*\dir3{>}*\dir3{|}}}
\xyletcsnamecsname@{dir0{>>|}}{dir{}}
\xyletcsnamecsname@{dir{>>|}}{dir1{>>|}}
\xydefcsname@{dir1{|<}}{\reverseDirection@ \shiftdir@\stopper@\z@ \tip@}
\xydefcsname@{dir2{|<}}{\reverseDirection@ \shiftdir@\stopper@\z@ \Tip@}
\xydefcsname@{dir3{|<}}{\reverseDirection@ \shiftdir@\stopper@\z@ \Ttip@}
\xyletcsnamecsname@{dir0{|<}}{dir{}}
\xyletcsnamecsname@{dir{|<}}{dir1{|<}}
\xydefcsname@{dir1{|<<}}{\reverseDirection@
 \shiftdir@\stopper@\z@ \shiftdir@\tip@\tipjot@ \tip@}
\xydefcsname@{dir2{|<<}}{%
 \composite@{}{h!/-\tipjot@/\dir2{<}*\dir2{<}*\dir2{|}}}
\xydefcsname@{dir3{|<<}}{%
 \composite@{}{h!/-\tipjot@/\dir3{<}*\dir3{<}*\dir3{|}}}
\xyletcsnamecsname@{dir0{|<<}}{dir{}}
\xyletcsnamecsname@{dir{|<<}}{dir1{|<<}}
\xydefcsname@{dir1{|-}}{\shiftdir@\stopper@\z@
 \shiftdir@\line@\z@ \pointlike@{}\jot}
\xydefcsname@{dir^{|-}}{\shiftdir@{\aboveDirection@\xydashl@ \line@}\z@
 \shiftdir@\line@\z@ \pointlike@{}\jot}
\xydefcsname@{dir_{|-}}{\shiftdir@{\belowDirection@\xydashl@ \line@}\z@
 \shiftdir@\line@\z@ \pointlike@{}\jot}
\xydefcsname@{dir2{|-}}{\shiftdir@\stopper@\z@
 \shiftdir@\line@\z@ \pointlike@{}\jot \double@\xydashh@}
\xydefcsname@{dir3{|-}}{\shiftdir@\stopper@\z@
 \shiftdir@\line@\z@ \pointlike@{}\jot \triple@\xydashh@}
\xyletcsnamecsname@{dir0{|-}}{dir{}}
\xyletcsnamecsname@{dir{|-}}{dir1{|-}}
\xyletcsnamecsname@{dir{|=}}{dir2{|-}}
\xydefcsname@{dir{+}}{%
 \DN@##1{\composite@{}{##10\dir{|}*!C##10\dir{-}}}\addEQ@\next@}
\xyletcsnamecsname@{dir0{+}}{dir{}}
\xydefcsname@{dir{x}}{\vDirection@(1,1)\jot
 \DN@##1{\composite@{}{##10\dir{|}*!C##10\dir{-}}}\addEQ@\next@}
\xyletcsnamecsname@{dir0{x}}{dir{}}
\xydefcsname@{dir{/}}{\vDirection@(1,-.3)\jot \stopper@}
\xyletcsnamecsname@{dir0{/}}{dir{}}
\xydefcsname@{dir{//}}{\vDirection@(1,-.3)\jot
 \shiftdir@\stopper@\xydashh@ \stopper@}
\xyletcsnamecsname@{dir0{//}}{dir{}}
\xydefcsname@{dir{*}}{\solidpoint@}
\xydef@\solidpoint@{%
 \pointlike@{\kern-1.8pt\lower1.8pt\hbox{$\scriptstyle\bullet$}}\jot}
\xyletcsnamecsname@{dir0{*}}{dir{}}
\xydefcsname@{dir{o}}{\hollowpoint@}
\xydef@\hollowpoint@{%
 \pointlike@{\kern-1.8pt\lower1.8pt\hbox{$\scriptstyle\circ$}}\jot}
\xyletcsnamecsname@{dir0{o}}{dir{}}
\message{circles,}
\xydef@\cir#1#{\hbox\bgroup
 \afterVECTORorEMPTY{\xy@@{\R@=\X@c}\cir@}{\xy@@{\R@=\R@c}\cir@}#1@}
\xydef@\cir@#1@#2{%
 \DN@{#1}\ifx\next@\empty\else \xyerror@{illegal circle <radius>: must be
 <vector> or <empty>}{}\fi
 \afterCIRorDIAG{\xyFN@\cir@cir}{\xyFN@\cir@diag}#2@}
\xydef@\cir@cir{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\cir@cir}%
 \else \ifx @\next \DN@ @{\cir@i}%
 \else \xyerror@{illegal <cir>: must have form <diag><orient><diag> or
 <empty>}{}%
 \fi\fi \next@}
\xydef@\cir@diag{%
 \DN@{\xyerror@{illegal <cir>: must have form <diag><orient><diag> or
 <empty>}{}}%
 \ifx @\next \ifnum\count@=8
 \DN@ @{\def\CIRin@@{0}\def\CIRorient@@{\CIRfull@}\def\CIRout@@{7}\cir@i}%
 \fi\fi \next@}
\xydef@\cir@i{%
 \ifnum\CIRin@@=8 \xyerror@{incomplete <cir> specification}{%
The <cir> you specified as <diag><orient><diag> is not sufficiently specific.}%
 \def\CIRin@@{0}\fi
 \ifdim\R@<.5\p@ \R@=\z@ \zerodot
 \else \CIRorient@@ \cirbuild@ \fi
 \L@c=\R@ \R@c=\R@ \D@c=\R@ \U@c=\R@ \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\relax}%
 \Edge@c={\circleEdge}\OBJECT@x}
\xydef@\CIRin@@{3}
\xydef@\CIRout@@{3}
\xylet@\CIRorient@@=\empty
\xydef@\afterCIRorDIAG#1#2{\def\afterCIR@{#1}\def\afterCIRDIAG@{#2}\xyFN@\CIR@}
\xylet@\afterCIR@=\empty
\xylet@\afterCIRDIAG@=\empty
\xydef@\CIR@{\count@=8 \afterDIAG{\edef\CIRin@@{\the\count@}\xyFN@\CIR@@}}
\xydef@\CIR@@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\CIR@@}%
 \else\ifx ^\next
 \DN@ ^{\def\CIRorient@@{\CIRacw@}%
 \afterDIAG{\edef\CIRout@@{\the\count@}\afterCIR@}}%
 \else\ifx _\next
 \DN@_{\def\CIRorient@@{\CIRcw@}%
 \afterDIAG{\edef\CIRout@@{\the\count@}\afterCIR@}}%
 \else
 \DN@{\def\CIRorient@@{\relax}\afterCIRDIAG@}%
 \fi\fi\fi \next@}
\xylet@\CIRtest@@=\relax
\xydef@\CIRlo@@{0}
\xydef@\CIRhi@@{0}
\xydef@\CIRfull@{\def\CIRtest@@##1##2{##2}}
\xydef@\cirbuild@{\cirrestrict@@ \multiply\count@8
 \circhar@0\circhar@7\kern\dimen@
 \circhar@1\circhar@6\kern\dimen@
 \circhar@2\circhar@5\kern\dimen@
 \circhar@3\circhar@4\kern\dimen@}
\xydef@\circhar@#1{%
 \setboxz@h{\circhar@@{#1}}\dimen@=\wdz@ \wdz@=\z@ \ht\z@=\R@ \dp\z@=\R@
 \CIRtest@@#1{\styledboxz@}\setbox\z@=\copy\voidb@x}
\xydef@\circhar@@#1{{\xycircfont \advance\count@#1\relax \char\count@}}
\xydef@\cirrestrict@@{\begingroup \dimen@=\R@
 \setboxz@h{\xycircfont\char\z@\char\@ne}\A@=\wdz@
 \ifdim\R@<8\A@ \count@=\dimen@ \divide\count@\A@ \advance\count@\m@ne
 \else\ifdim\R@<16\A@ \count@=\dimen@
 \dimen@=2\A@ \divide\count@\dimen@ \advance\count@3
 \else\ifdim\R@<32\A@ \count@=\dimen@
 \dimen@=4\A@ \divide\count@\dimen@ \advance\count@7
 \else \count@=15 \fi\fi\fi
 \R@=\A@
 \ifnum\count@<8 \multiply\R@\count@ \advance\R@\A@
 \else\ifnum\count@<12 \multiply\R@\count@ \multiply\R@\tw@ \advance\R@-6\A@
 \else\ifnum\count@<16 \multiply\R@\count@ \multiply\R@ 4 \advance\R@-28\A@
 \else \multiply\R@ 32 \fi\fi\fi
 \edef\@tmp{\endgroup \R@=\the\R@ \count@=\the\count@}\@tmp}
\xydef@\CIRacw@{\count@@=\CIRin@@ \count@=\CIRout@@
 \ifnum\count@=8 \count@=\count@@
 \ifnum\count@<6 \advance\count@\tw@ \else \advance\count@-6 \fi \fi
 \ifnum\count@@<\@ne \advance\count@@7 \else \advance\count@@\m@ne \fi
 \ifnum\count@<\@ne \advance\count@7 \else \advance\count@\m@ne \fi
 \ifnum\count@@>\count@ \let\CIRtest@@=\CIRtest@outside
 \edef\CIRlo@@{\the\count@}\edef\CIRhi@@{\the\count@@}%
 \else \let\CIRtest@@=\CIRtest@inside
 \edef\CIRlo@@{\the\count@@}\edef\CIRhi@@{\the\count@}%
 \fi}
\xydef@\CIRcw@{\count@@=\CIRin@@ \count@=\CIRout@@
 \ifnum\count@=8 \count@=\count@@
 \ifnum\count@>\@ne \advance\count@-\tw@ \else \advance\count@6 \fi \fi
 \ifnum\count@@<5 \advance\count@@\thr@@ \else \advance\count@@-5 \fi
 \ifnum\count@<5 \advance\count@\thr@@ \else \advance\count@-5 \fi
 \ifnum\count@@<\count@ \let\CIRtest@@=\CIRtest@outside
 \edef\CIRlo@@{\the\count@@}\edef\CIRhi@@{\the\count@}%
 \else \let\CIRtest@@=\CIRtest@inside
 \edef\CIRlo@@{\the\count@}\edef\CIRhi@@{\the\count@@}%
 \fi}
\xydef@\CIRtest@inside#1#2{\let\next@=\relax
 \ifnum\CIRlo@@>#1\else \ifnum#1<\CIRhi@@\DN@{#2}\fi\fi \next@}
\xydef@\CIRtest@outside#1#2{\let\next@=\relax
 \ifnum\CIRlo@@>#1\DN@{#2}\else \ifnum#1<\CIRhi@@\else\DN@{#2}\fi\fi \next@}
\message{text;}
\xydef@\txt{\hbox\bgroup \xyFN@\txt@}
\xydef@\txt@{%
 \addLT@\ifx\next \addGT@{\addLT@\DN@##1}{\A@=##1\txt@i}%
 \else \DN@{\A@=\maxdimen \txt@i}\fi \next@}
\xydef@\txt@i#1#{%
 \setboxz@h{#1\mathstrut}\dimen@=\ht\z@ \advance\dimen@\dp\z@
 \baselineskip=1.1\dimen@ \lineskip=.2\dimen@ \lineskiplimit=\lineskip
 \def\txtline@@##1{\txtline@{#1}{##1}}\object@\txt@ii}
\xylet@\txtline@@=\eat@
\xydef@\txtline@#1#2{\relax\setboxz@h{#1{\ignorespaces #2\unskip}}%
 \ifdim\A@<\wdz@ \setboxz@h{\hsize=\A@
 \leftskip=0pt plus4em \rightskip=\leftskip
 \parfillskip=0pt \parindent=0pt
 \spaceskip=.3333em \xspaceskip=.5em
 \pretolerance=9999 \tolerance=9999
 \hyphenpenalty=9999 \exhyphenpenalty=9999
 \vbox{#1\noindent\ignorespaces #2\unskip}}%
 \else\ifdim\A@<\maxdimen\setboxz@h to\A@{\hfil\boxz@\hfil}\fi\fi
 \boxz@}
\xydef@\txt@ii#1{\vbox{%
 \let\\=\cr
 \tabskip=\z@skip \halign{\relax\hfil\txtline@@{##}\hfil\cr\leavevmode#1\crcr}}}
\message{options;}
\xylet@\xyoption@@=\relax
\xydef@\xyoption#1{\DN@{#1}\edef\next@{\codeof\next@}%
 \csname xyeveryrequest@\next@ @\endcsname
 \xyinputorelse@{xy#1}{\xyoption@truncated#1@@@@@@@@@,#1@}%
 \def\xyoption@@{#1}\edef\xyoption@@{\codeof\xyoption@@}
 \expandafter\let\expandafter\next@\csname xy\xyoption@@ version\endcsname
 \expandafter\let\csname xy\xyoption@@ loaded\endcsname=\next@
 \runxywith@ \ignorespaces}
\xydef@\xyoption@truncated#1#2#3#4#5#6#7@#8,#9@{%
 \DN@{#7}\ifx\next@\empty \DN@##1##2{##2}\else\let\next@=\xyinputorelse@ \fi
 \next@{xy#1#2#3#4#5#6}%
 {\DN@{#1#2#3#4#5#6}\edef\next@{\codeof\next@}%
 \xyerror@{No `\next@' option}{%
Your \xyoption{#9} request could not be granted: the required^^J%
file `xy#9.tex' could not be located. Please make sure that it is^^J%
properly installed before continuing.}}}
\xydef@\xyrequire#1{\DN@{#1}\edef\next@{\codeof\next@}%
 \csname xyeveryrequest@\next@ @\endcsname
 \expandafter\let\expandafter\next@\csname xy\codeof\next@ loaded\endcsname
 \ifx \next@\relax \DN@{\xyoption{#1}}\else \DN@{\ignorespaces}\fi \next@}
\xylet@\xywith@@=\empty
\xydef@\runxywith@{\let\xywithdo@@=\xywithtest@ \xywith@@}
\xydef@\xywithoption#1#2{\DN@{#1}\edef\next@{\codeof\next@}%
 \expandafter\let\expandafter\nextii@\csname xy\next@ loaded\endcsname
 \ifx \nextii@\relax
 \expandafter\def\expandafter\xywith@@\expandafter{\xywith@@ 
 \xywithdo@@{#1}{#2}}%
 \else \expandafter\xywithrun@\expandafter{\next@}{#2}\fi}
\xydef@\xywithtest@#1#2{\DN@{#1}\edef\next@{\codeof\next@}%
 \ifx\next@\xyoption@@ \expandafter\xywithrun@\expandafter{\next@}{#2}\fi}
\xydef@\xywithrun@#1#2{\csname xyeverywithoption@#1@\endcsname #2}
\xydef@\xyevery@#1#2#3{\DN@{#2}\edef\next@{\codeof\next@}%
 \expandafter\ifx\csname xyevery#1@\next@ @\endcsname\relax
 \expandafter\let\csname xyevery#1@\next@ @\endcsname=\empty \fi
 \DNii@##1{\expandafter\def\expandafter##1\expandafter{##1#3}}%
 \expandafter\nextii@\csname xyevery#1@\next@ @\endcsname}
\xydef@\xyeveryrequest{\xyevery@{request}}
\xydef@\xyeverywithoption{\xyevery@{withoption}}
\xydef@\xyprovide#1#2#3#4#5#6{%
 \def\xyoption@@{#1}\edef\xyoption@@{\codeof\xyoption@@}\edef\next@{#3}%
 \message{ Xy-pic option: #2 v.\next@}%
 \expandafter\let\expandafter\nextii@\csname xy\xyoption@@ loaded\endcsname
 \ifx \next@\nextii@ \message{not reloaded}\endinput
 \else
 \ifx \nextii@\relax\else \xyerror@{Option `\xyoption@@' version mismatch}{%
You previously loaded, or the format has preloaded, a different version^^J%
of this option. Just continue to try to load this version instead (and^^J%
be prepared for a lot of warnings about redefinitions).}%
 \fi
 \expandafter\let\csname xy\xyoption@@ version\endcsname=\next@
 \expandafter\let\expandafter\xyenddocmode@\csname DOCMODE\endcsname
 \expandafter\let\csname DOCMODE\endcsname\xyprovidedocmode@
 \xycatcodes
 \fi \ignorespaces}
\xydef@\xyendinput{\expandafter\let\csname DOCMODE\endcsname=\xyenddocmode@
 \message{loaded}\xyuncatcodes\endinput}
\expandafter\xylet@\expandafter\xyprovidedocmode@\csname DOCMODE\endcsname
\xylet@\xyenddocmode@=\relax
\xydef@\xydriversloaded@none{\do{unload}}
\xylet@\xydriversloaded@@=\xydriversloaded@none
\xylet@\xydriversselected@@=\empty
\xylet@\xydriver@unload@support@@=\empty
\xydef@\selectdriver@#1{\DN@{#1}\edef\next@{\codeof\next@}%
 \expandafter\selectdriver@@\expandafter{\next@}}
\xydef@\selectdriver@single#1{\xysetup@@{\def\xydriversselected@@{\do{#1}}%
 \xyLoadDrivers@}\let\selectdriver@@=\changedriver@single}
\xydef@\changedriver@single#1{\xysetup@@{\def\xydriversselected@@{\do{#1}}%
 \xyReloadDrivers@}}
\xydef@\selectdriver@multiple#1{\expandafter\xysetup@@\expandafter{%
 \expandafter\def\expandafter\xydriversselected@@\expandafter{%
 \xydriversselected@@ \do{#1}}%
 \let\do=\activatedriver@ \xydriversselected@@}}
\xydef@\UseSingleDriver{\let\selectdriver@@=\selectdriver@single}
\xydef@\MultipleDrivers{\let\selectdriver@@=\selectdriver@multiple}
\xydef@\xyLoadDrivers@{\let\do=\activatedriver@ \xydriversselected@@}
\xydef@\xyReloadDrivers@{\activatedriver@{unload}\xyLoadDrivers@}
\xylet@\xyReloadDrivers=\xyReloadDrivers@
\xydef@\activatedriver@#1{%
 \let\doii=\activatedriversupport@ \csname xydriver@#1@support@@\endcsname}
\xydef@\activatedriversupport@#1#2{%
 \expandafter\ifx\csname xy#1loaded\endcsname\relax\DN@{}%
 \else\DN@{#2}\fi \next@}
\UseSingleDriver
\xydef@\xyselectoptionsupport@{\let\do=\activatedriver@ \xydriversselected@@}
\xydef@\xyShowDrivers{{\W@{Loaded:}\let\do=\doShow \xydriversloaded@@
 \let\next@=\empty
 \def\do##1{\ifx\next@\empty \DN@{##1}%
 \else \expandafter\DN@\expandafter{\next@, ##1}\fi}%
 \xydriversselected@@\W@{Selected: \next@.}}}
\def\doShow#1{\let\next@=\empty
 \def\doii##1##2{\ifx\next@\empty \DN@{##1}%
 \else \expandafter\DN@\expandafter{\next@, ##1}\fi}%
 \csname xydriver@#1@support@@\endcsname
 \W@{ <driver> #1 supports \next@.}}
\xydef@\newdriver#1{%
 \def\nextiii@##1{%
 \expandafter\def\expandafter\xydriversloaded@@
 \expandafter{\xydriversloaded@@\do{##1}}%
 \expandafter\let\csname xydriver@\xyoption@@ @support@@\endcsname=\empty}%
 \def\do##1{\DNii@{##1}\ifx\xyoption@@\nextii@ \let\nextiii@=\eat@ \fi}%
 \xydriversloaded@@ \expandafter\nextiii@\expandafter{\xyoption@@}%
 #1\relax
 \DN@##1{\xywithoption{##1}{%
 \selectdriver@{##1}\xyeveryrequest{##1}{\selectdriver@{##1}}}}%
 \expandafter\next@\expandafter{\xyoption@@}\ignorespaces}
\xydef@\xyaddsupport{\expandafter\xyadddriversupport@\expandafter{\xyoption@@}}
\xydef@\xyaddunsupport{\xyadddriversupport@{unload}}
\xydef@\xyadddriversupport@#1#2#3{%
 \DNii@{#1}\edef\nextii@{\codeof\nextii@}%
 \def\nextiii@{#2}\edef\nextiii@{\codeof\nextiii@}%
\def\next{\xybug@{<driver> \nextii@\space not loaded}}%
\def\do##1{\DN@{##1}\edef\next@{\codeof\next@}%
 \ifx\next@\nextii@ \let\next=\relax \fi}\xydriversloaded@@ \next
\def\next{\xybug@{<driver> \nextii@\space already supports \nextiii@}}%
\def\doii##1##2{\DN@{##1}\edef\next@{\codeof\next@}%
 \ifx\next@\nextiii@ \let\next=\relax \fi}\xydriversloaded@@ \next
 \DN@##1##2{\ifx##1\relax \let##1=\empty \fi
 \expandafter\def\expandafter##1\expandafter{##1\doii{##2}{#3}}}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\csname xydriver@\nextii@ @support@@\endcsname
 \expandafter{\nextiii@}%
 \DN@##1{\expandafter\xyeverywithoption\expandafter{\nextiii@}{%
 \xytestforsupport@{##1}}}%
 \expandafter\next@\expandafter{\nextii@}\xydriversloaded@@
 \ignorespaces}
\xydef@\xytestforsupport@#1{\def\do##1{\DN@{##1}\DNii@{#1}%
 \ifx\next@\nextii@ \expandafter\xyselectoptionsupport@ \fi}}
\xynew@{if}\ifunsupportwarnings@
\xydef@\xyunsupportwarning@#1#2{{%
 \DN@{#1}\edef\next@{\codeof\next@}
 \expandafter\ifx\csname xywarn@unload@\next@ @\endcsname\relax
 \expandafter\gdef\csname xywarn@unload@\next@ @\endcsname{}%
 \ifunsupportwarnings@ \xyclosedown@@\xyunsupportwarnings@@ \fi
 \global\unsupportwarnings@true
 \expandafter\gdef\expandafter\xyunsupportwarnings@@\expandafter{%
 \xyunsupportwarnings@@ \W@{ #2.}}%
 \W@{}%
 \W@{Xy-pic Warning: `\next@' reproduction is NOT EXACT\xytracelineno@:}%
 \W@{ #2.}%
 \W@{}%
 \fi}}
\xydef@\xyunsupportwarnings@@{\W@{}%
 \W@{Xy-pic Warning: The produced DVI file is NOT EXACT:}}
\xynew@{if}\ifsupportwarnings@
\xydef@\xysupportwarning@#1#2{{%
 \DN@{#1}\edef\next@{\codeof\next@}\DNii@{#2}\edef\nextii@{\codeof\nextii@}%
 \expandafter\ifx\csname xywarn@\next@ @\nextii@ @\endcsname\relax
 \expandafter\gdef\csname xywarn@\next@ @\nextii@ @\endcsname{}%
 \ifsupportwarnings@ \xyclosedown@@\xysupportwarnings@@ \fi
 \global\supportwarnings@true
 \expandafter\gdef\expandafter\xysupportwarnings@@\expandafter{%
 \xysupportwarnings@@ \driverextensioncomplain@{#1}{#2}}%
 \W@{}%
 \W@{Xy-pic Warning: The produced DVI file is NOT PORTABLE\xytracelineno@:}%
 \driverextensioncomplain@{#1}{#2}%
 \W@{}%
 \fi}}
\xydef@\xysupportwarnings@@{%
 \W@{Xy-pic Warning: The produced DVI file is NOT PORTABLE:}}
\xydef@\driverextensioncomplain@#1#2{%
 \DN@{#1}\edef\next@{\codeof\next@}\DNii@{#2}\edef\nextii@{\codeof\nextii@}%
 \W@{ It contains <driver> `\next@' \string\special s for the `\nextii@'
 extension.}}
\xydef@\dvimessage@#1#2{\xysupportwarning@{#1}{#2}}
\xynew@{if}\ifxydrivernoloads@
\xydef@\xydrivernoload@#1{\xyerror@{Could not load xy#1.tex}{}%
 \xydrivernoloads@true}
\xydef@\xydriverfail@#1{\xyerror@{Sorry, #1 not supported.}{}}
\xydef@\xyunload@#1{\xywarning@{Unloading #1.}}
\message{algorithms: directions,}
\xydef@\DirectionfromtheDirection@{\noexpand\Direction=\the\Direction
 \noexpand\d@X=\the\d@X \noexpand\d@Y=\the\d@Y
 \def\noexpand\sd@X{\sd@X}\def\noexpand\sd@Y{\sd@Y}%
 \noexpand\K@dXdY=\the\K@dXdY \noexpand\K@dYdX=\the\K@dYdX
 \chardef\noexpand\DirectionChar=\the\DirectionChar
 \chardef\noexpand\SemiDirectionChar=\the\SemiDirectionChar
 \def\noexpand\cosDirection{\cosDirection}%
 \def\noexpand\sinDirection{\sinDirection}%
 \noexpand\resetupDirection@}
\xydef@\Directiontest@@#1#2{#2}
\xydef@\setupDirection@{%
 \d@X=\X@c\advance\d@X-\X@p \d@Y=\Y@c\advance\d@Y-\Y@p
 \Directiontest@@\relax\setupDirection@i}
\xydef@\setupDirection@i{\DN@{\setupDirection@ii}%
 \ifdim\d@X=\d@Y
 \ifdim\zz@\d@Y \DN@{}%
 \else\ifdim\d@X<\z@ \DN@{\dlDirection@{-1.4142\d@X}}%
 \else \DN@{\urDirection@{1.4142\d@X}}\fi\fi
 \else\ifdim\d@X<\d@Y
 \ifdim\zz@\d@X \DN@{\uDirection@\d@Y}%
 \else\ifdim\zz@\d@Y \DN@{\lDirection@{-\d@X}}%
 \else\ifdim-\d@X=\d@Y \DN@{\ulDirection@{-1.4142\d@X}}\fi\fi\fi
 \else
 \ifdim\zz@\d@X \DN@{\dDirection@{-\d@Y}}%
 \else\ifdim\zz@\d@Y \DN@{\rDirection@\d@X}%
 \else\ifdim\d@X=-\d@Y \DN@{\drDirection@{1.4142\d@X}}\fi\fi\fi
 \fi\fi \next@}
\xydef@\dlDirection@{\Direction=\z@
 \def\cosDirection{-.7071}\def\sinDirection{-.7071}\def\sd@X{-}\def\sd@Y{-}%
 \chardef\DirectionChar=127\relax\chardef\SemiDirectionChar=127\relax
 \K@dXdY=1\K@ \K@dYdX=1\K@ \fixedDirection@}
\xydef@\dDirection@{\Direction=\K@
 \def\cosDirection{0}\def\sinDirection{-1}\def\sd@Y{-}%
 \edef\sd@X{\ifdim\X@c<\X@p-\else+\fi}%
 \chardef\DirectionChar=15\relax\chardef\SemiDirectionChar=31\relax
 \K@dXdY=\z@ \K@dYdX=\KK@\K@ \fixedDirection@}
\xydef@\drDirection@{\dimen@ii=2\K@ \Direction=\dimen@ii
 \def\cosDirection{+.7071}\def\sinDirection{-.7071}\def\sd@X{+}\def\sd@Y{-}%
 \chardef\DirectionChar=31\relax\chardef\SemiDirectionChar=63\relax
 \K@dXdY=-1\K@ \K@dYdX=-1\K@ \fixedDirection@}
\xydef@\rDirection@{\dimen@ii=3\K@ \Direction=\dimen@ii
 \def\cosDirection{+1}\def\sinDirection{0}\def\sd@X{+}%
 \edef\sd@Y{\ifdim\Y@c<\Y@p-\else+\fi}%
 \chardef\DirectionChar=47\relax\chardef\SemiDirectionChar=95\relax
 \K@dXdY=\KK@\K@ \K@dYdX=\z@ \fixedDirection@}
\xydef@\urDirection@{\dimen@ii=4\K@ \Direction=\dimen@ii
 \def\cosDirection{+.7071}\def\sinDirection{+.7071}\def\sd@X{+}\def\sd@Y{+}%
 \chardef\DirectionChar=63\relax\chardef\SemiDirectionChar=127\relax
 \K@dXdY=1\K@ \K@dYdX=1\K@ \fixedDirection@}
\xydef@\uDirection@{\dimen@ii=-3\K@ \Direction=\dimen@ii
 \def\cosDirection{0}\def\sinDirection{+1}\def\sd@Y{+}%
 \edef\sd@X{\ifdim\X@c<\X@p-\else+\fi}%
 \chardef\DirectionChar=79\relax\chardef\SemiDirectionChar=31\relax
 \K@dXdY=\z@ \K@dYdX=\KK@\K@ \fixedDirection@}
\xydef@\ulDirection@{\dimen@ii=-2\K@ \Direction=\dimen@ii
 \def\cosDirection{-.7071}\def\sinDirection{+.7071}\def\sd@X{-}\def\sd@Y{+}%
 \chardef\DirectionChar=95\relax\chardef\SemiDirectionChar=63\relax
 \K@dXdY=-1\K@ \K@dYdX=-1\K@ \fixedDirection@}
\xydef@\lDirection@{\Direction=-\K@
 \def\cosDirection{-1}\def\sinDirection{0}\def\sd@X{-}%
 \edef\sd@Y{\ifdim\Y@c<\Y@p-\else+\fi}%
 \chardef\DirectionChar=111\relax\chardef\SemiDirectionChar=95\relax
 \K@dXdY=\KK@\K@ \K@dYdX=\z@ \fixedDirection@}
\xydef@\fixedDirection@#1{\dimen@ii=#1\relax
 \d@X=\cosDirection\dimen@ii \d@Y=\sinDirection\dimen@ii
 \resetupDirection@}
\xydef@\setupDirection@ii{%
 \ifdim\d@X<\z@ \def\sd@X{-}\else \def\sd@X{+}\fi
 \ifdim\d@Y<\z@ \def\sd@Y{-}\else \def\sd@Y{+}\fi
 \K@dXdY=\sd@X\d@X \ifdim\K@dXdY<500pt \multiply\K@dXdY\KK@ \fi
 \dimen@=\sd@Y\d@Y
 \advance\dimen@\ifdim\dimen@<\z@-\fi.5\KK@ \divide\dimen@\KK@
 \ifdim\dimen@=\z@\else
 \advance\K@dXdY by.5\dimen@\relax \divide\K@dXdY\dimen@
 \fi \K@dXdY=\sd@X\sd@Y\K@dXdY
 \K@dYdX=\sd@Y\d@Y \ifdim\K@dYdX<500pt \multiply\K@dYdX\KK@ \fi
 \dimen@=\sd@X\d@X
 \advance\dimen@\ifdim\dimen@<\z@-\fi.5\KK@ \divide\dimen@\KK@
 \ifdim\dimen@=\z@\else
 \advance\K@dYdX by.5\dimen@\relax \divide\K@dYdX\dimen@
 \fi \K@dYdX=\sd@X\sd@Y\K@dYdX
 \Direction=\maxdimen
 \ifnum\K@dXdY<-\K@ \else \ifnum\K@<\K@dXdY \else
 \ifdim \d@Y<\z@
 \Direction=\K@ \advance\Direction-\K@dXdY
 \else
 \Direction=\K@ \multiply\Direction-\thr@@ \advance\Direction-\K@dXdY
 \fi\fi\fi
 \ifnum-\K@<\K@dYdX \ifnum\K@dYdX<\K@
 \ifdim \d@X<\z@
 \Direction=-\K@ \advance\Direction\K@dYdX
 \else
 \Direction=\K@ \multiply\Direction\thr@@ \advance\Direction\K@dYdX
 \fi\fi\fi
 \ifnum\Direction=\maxdimen
 \Direction=\K@dYdX \advance\Direction-\K@dXdY 
 \advance\Direction\ifnum\Direction<\z@-\fi\@ne \divide\Direction\tw@ 
 \ifnum\K@dXdY<\z@ \advance\Direction\K@ \advance\Direction\K@
 \else \advance\Direction-\K@ \advance\Direction-\K@ \fi
 \fi
 \imposeDirection@i
 \resetupDirection@
 }
\xydef@\imposeDirection@{\count@@=\Direction 
 \loop@\ifnum\count@@>4096 \advance\count@@-8192 \repeat@
 \loop@\ifnum\count@@<-4096 \advance\count@@8192 \repeat@
 \def\sd@X{+}\ifnum\count@@<\K@ \relax
 \ifnum\count@@>-3072 \def\sd@X{-}\fi\fi
 \def\sd@Y{+}\ifnum\count@@<3072 \relax
 \ifnum\count@@>-\K@ \relax\def\sd@Y{-}\fi\fi
 \imposeDirection@i
 \d@X=\cosDirection\xydashl@ \d@Y=\sinDirection\xydashl@
 \resetupDirection@}
\xydef@\imposeDirection@i{%
 \count@@=\K@ \multiply\count@@ by8 \advance\count@@\Direction
 \count@=\count@@ \advance\count@\KK@ \divide\count@64 \advance\count@\m@ne
 \loop@\ifnum127<\count@ \advance\count@-128 \repeat@
 \chardef\DirectionChar\count@
 \advance\count@@16 \divide\count@@\KK@ \advance\count@@\m@ne
 \loop@\ifnum127<\count@@ \advance\count@@-128 \repeat@
 \chardef\SemiDirectionChar\count@@
 \setbox8=\hbox{\xydashfont\SemiDirectionChar\/}%
 \quotient@@\cosDirection{\sd@X\wd8}\xydashl@
 \setbox8=\hbox{\xydashfont\count@=\SemiDirectionChar\advance\count@-64
 \ifnum\count@<\z@ \advance\count@128 \fi \char\count@\/}%
 \quotient@@\sinDirection{\sd@Y\wd8}\xydashl@}
\xydef@\getxyDirection@#1{\xy@@\bgroup\xy@@ix@{#1}%
 \xy@@{\expandafter\POS\the\toks9\relax\setupDirection@
 \edef\next@{\egroup \Direction=\the\Direction}\next@ \imposeDirection@ }}
\xydef@\reverseDirection@{%
 \d@X=-\d@X \d@Y=-\d@Y
 \ifdim\d@X<\z@ \def\sd@X{-}\else \def\sd@X{+}\fi
 \ifdim\d@Y<\z@ \def\sd@Y{-}\else \def\sd@Y{+}\fi
 \dimen@=4\K@ \ifnum\Direction<\z@ \advance\Direction\dimen@
 \else \advance\Direction-\dimen@ \fi
 \count@=\DirectionChar \ifnum\count@<64 \advance\count@64
 \else \advance\count@-64 \fi \chardef\DirectionChar=\count@
 \edef\cosDirection{\if-\cosDirection\else-\cosDirection\fi}%
 \edef\sinDirection{\if-\sinDirection\else-\sinDirection\fi}%
 \resetupDirection@}
\xydef@\aboveDirection@#1{%
 \dimen@=\d@X \d@X=-\d@Y \d@Y=\dimen@
 \dimen@=\K@dXdY \K@dXdY=-\K@dYdX \K@dYdX=-\dimen@
 \ifdim\d@X<\z@ \def\sd@X{-}\else \def\sd@X{+}\fi
 \ifdim\d@Y<\z@ \def\sd@Y{-}\else \def\sd@Y{+}\fi
 \dimen@=2\K@ \ifdim 1\Direction<\dimen@\else \dimen@=-6\K@ \fi
 \advance\Direction\dimen@
 \count@=\DirectionChar \ifnum\count@<96 \advance\count@32
 \else \advance\count@-96 \fi \chardef\DirectionChar=\count@
 \count@=\SemiDirectionChar \ifnum\count@<64 \advance\count@64
 \else \advance\count@-64 \fi \chardef\SemiDirectionChar=\count@
 \let\tmp@=\cosDirection
 \edef\cosDirection{\if-\sinDirection\else-\sinDirection\fi}%
 \let\sinDirection=\tmp@
 \dimen@=#1\relax \d@X=\cosDirection\dimen@ \d@Y=\sinDirection\dimen@
 \resetupDirection@}
\xydef@\belowDirection@#1{%
 \dimen@=\d@X \d@X=\d@Y \d@Y=-\dimen@
 \dimen@=\K@dXdY \K@dXdY=-\K@dYdX \K@dYdX=-\dimen@
 \ifdim\d@X<\z@ \def\sd@X{-}\else \def\sd@X{+}\fi
 \ifdim\d@Y<\z@ \def\sd@Y{-}\else \def\sd@Y{+}\fi
 \dimen@=-2\K@\ifdim 1\Direction<\dimen@\dimen@=6\K@\fi
 \advance\Direction\dimen@
 \count@=\DirectionChar \ifnum\count@<32 \advance\count@96
 \else \advance\count@-32 \fi \chardef\DirectionChar=\count@
 \count@=\SemiDirectionChar \ifnum\count@<64 \advance\count@64
 \else \advance\count@-64 \fi \chardef\SemiDirectionChar=\count@
 \let\tmp@=\sinDirection
 \edef\sinDirection{\if-\cosDirection\else-\cosDirection\fi}%
 \let\cosDirection=\tmp@
 \dimen@=#1\relax \d@X=\cosDirection\dimen@ \d@Y=\sinDirection\dimen@
 \resetupDirection@}
\xydef@\vDirection@(#1,#2)#3{\dimen@ii=#3\relax
 \dimen@=#1\dimen@ii \dimen@ii=#2\dimen@ii
 \d@X=\cosDirection\dimen@ \advance\d@X-\sinDirection\dimen@ii
 \d@Y=\sinDirection\dimen@ \advance\d@Y \cosDirection\dimen@ii
 \X@p=\X@c \advance\X@p-\d@X \Y@p=\Y@c \advance\Y@p-\d@Y
 \setupDirection@\ignorespaces}
\xydef@\resetDirection@{%
 \d@X=\X@c\advance\d@X-\X@p \d@Y=\Y@c\advance\d@Y-\Y@p
 \let\next@=\resetupDirection@
 \ifdim\sd@X\d@X<\z@ \let\next@=\setupDirection@i \fi
 \ifdim\sd@Y\d@Y<\z@ \let\next@=\setupDirection@i \fi
 \next@}
\xydef@\resetupDirection@{%
 \edef\Directiontest@@##1##2{\noexpand\DN@{##2}%
 \noexpand\ifdim\noexpand\d@X=\the\d@X\relax
 \noexpand\ifdim\noexpand\d@Y=\the\d@Y\relax \noexpand\DN@{##1}%
 \noexpand\fi\noexpand\fi \noexpand\next@}}
\xydef@\unsetupDirection@{\def\Directiontest@@##1##2{##2}}
\uDirection@\xydashl@
\message{edges,}
\xynew@{if}\ifInside@
\xydef@\zeroEdge#1{%
 \ifcase#1\relax \or \Inside@false \or \dimen@=\z@
 \or \else \Edge@c={\rectangleEdge}\fi}
\xydef@\circleEdge#1{\ifcase#1\expandafter\circleEdge@
 \or \expandafter\circleUnder@ \or \dimen@=\R@c
 \or \expandafter\circleProp@ \or \expandafter\circleInner@
 \else \expandafter\circleOuter@ \fi}
\xydef@\circleEdge@{\DN@{\ellipseEdge@}%
 \ifdim\R@c=\L@c\relax \ifdim\U@c=\D@c\relax
 \ifdim\R@c=\U@c\DN@{\circlecentredEdge@}%
 \else\DN@{\ellipsecentredEdge@}\fi
 \fi\fi \next@}
\xydef@\circleProp@{\DN@{\reverseDirection@\ellipseEdge@}%
 \ifdim\R@c=\L@c\relax \ifdim\U@c=\D@c\relax
 \ifdim\R@c=\U@c\DN@{\reverseDirection@\circlecentredEdge@}%
 \else\DN@{\reverseDirection@\ellipsecentredEdge@}\fi
 \fi\fi \next@}
\xydef@\circleUnder@{\Inside@false
 \ifdim\X@p=\X@c \relax \ifdim\Y@p=\Y@c \Inside@true \fi \fi 
 \ifInside@ \else \expandafter \circleCentre@ \fi}
\xydef@\circleCentre@{{%
 \ifdim\L@c=\R@c \relax\else
 \dimen@=\R@c\advance\dimen@-\L@c \divide\dimen@\tw@
 \advance\X@c\dimen@ \advance\R@c-\dimen@ \fi
 \d@X=\X@c \advance\d@X-\X@p \d@X=\ifdim\d@X<\z@-\fi\d@X
 \ifdim\U@c=\D@c\relax \else
 \dimen@=\U@c\advance\dimen@-\D@c \divide\dimen@\tw@
 \advance\Y@c\dimen@ \advance\U@c-\dimen@ \fi
 \d@Y=\Y@c \advance\d@Y-\Y@p \d@Y=\ifdim\d@Y<\z@-\fi\d@Y
 \DN@{}\ifdim\d@X>\R@c \relax \else \ifdim\d@Y>\U@c \relax 
 \else \ifdim\U@c=\R@c \DN@{\circlecentredUnder@}%
 \else \DN@{\ellipsecentredUnder@}\fi
 \fi\fi \next@}}
\xydef@\circleInner@{\DN@{\ellipseInner@}%
 \ifdim\R@c=\L@c\relax \ifdim\U@c=\D@c\relax
 \ifdim\R@c=\U@c\DN@{\circlecentredInner@}%
 \else\DN@{\ellipsecentredInner@}\fi
 \fi\fi \next@}
\xydef@\circleOuter@{\DN@{\ellipseOuter@}%
 \ifdim\R@c=\L@c\relax \ifdim\U@c=\D@c\relax
 \ifdim\R@c=\U@c\DN@{\circlecentredOuter@}%
 \else\DN@{\ellipsecentredOuter@}\fi
 \fi\fi \next@}
\xydef@\circlecentredEdge@{%
 \dimen@=-\cosDirection\R@c \advance\X@c\dimen@
 \dimen@=-\sinDirection\R@c \advance\Y@c\dimen@}
\xydef@\circlecentredUnder@{%
 \loop\ifdim\R@c>100\p@ \circlescale@ \repeat
 \edef\tmp@{\expandafter\removePT@\the\R@c}\dimen@=\tmp@\R@c 
 \edef\tmp@{\expandafter\removePT@\the\d@X}\advance\dimen@-\tmp@\d@X
 \edef\tmp@{\expandafter\removePT@\the\d@Y}\advance\dimen@-\tmp@\d@Y
 \ifdim\dimen@>\z@ \aftergroup\Inside@true \fi}
%%\xydef@\circlescale@{\divide\R@c\KK@ \divide\d@X\KK@ \divide\d@Y\KK@ }
\xydef@\circlescale@{\divide\R@c\KK@ \divide\d@X\KK@ \divide\d@Y\KK@ }
\xydef@\circlecentredInner@{%
 \L@c=\sd@X\cosDirection\R@c \D@c=\sd@Y\sinDirection\R@c
 \R@c=\L@c \U@c=\D@c \Edge@c={\rectangleEdge}}
\xydef@\circlecentredOuter@{%
 \L@c=\R@c \D@c=\R@c \U@c=\D@c \Edge@c={\rectangleEdge}}
\xydef@\ellipsecentredEdge@{\bgroup \X@p=\X@c \Y@p=\Y@c 
 \ifdim\U@c>\R@c
 \X@c=\cosDirection\U@c \Y@c=\sinDirection\U@c
 \quotient@\tmp@\U@c\R@c \X@c=\tmp@\X@c \R@c=\U@c 
 \else
 \X@c=\cosDirection\R@c \Y@c=\sinDirection\R@c
 \quotient@\tmp@\R@c\U@c \Y@c=\tmp@\Y@c 
 \fi
 \advance\X@c\X@p \advance\Y@c\Y@p 
 \setupDirection@ \X@c=\X@p \Y@c=\Y@p \circlecentredEdge@
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p 
 \ifdim\U@c>\L@c \quotient@\tmp@\L@c\U@c \d@X=\tmp@\d@X
 \else \quotient@\tmp@\U@c\R@c \d@Y =\tmp@\d@Y \fi
 \X@c=\X@p \advance\X@c\d@X \Y@c=\Y@p \advance\Y@c\d@Y 
 \edef\next@{\egroup \X@c=\the\X@c \Y@c=\the\Y@c}\next@ }%
\xydef@\ellipsecentredUnder@{%
 \ifdim\R@c>64\p@ \circlescale@ \divide\U@c\KK@ 
 \else \ifdim\U@c>64\p@ \circlescale@ \divide\U@c\KK@ \fi\fi
 \edef\tmp@{\expandafter\removePT@\the\R@c}\d@Y=\tmp@\d@Y 
 \edef\tmp@{\expandafter\removePT@\the\U@c}\d@X=\tmp@\d@X 
 \R@c=\tmp@\R@c \circlecentredUnder@ }
\xydef@\ellipsecentredOuter@{\Edge@c={\rectangleEdge}}
\xydef@\ellipsecentredInner@{%
 \bgroup \X@p=\X@c \Y@p=\Y@c \ellipsecentredEdge@
 \advance\X@c-\X@p \L@c=\ifdim\X@c<\z@-\fi\X@c
 \advance\Y@c-\Y@p \D@c=\ifdim\Y@c<\z@-\fi\Y@c
 \edef\next@{\egroup \L@c=\the\L@c \D@c=\the\D@c}\next@
 \R@c=\L@c \U@c=\D@c \Edge@c={\rectangleEdge}}
\xydef@\ellipseEdge@{\bgroup
 \A@=\R@c \B@=\U@c
 \ifdim\R@c=\L@c \d@X=\z@ 
 \else \d@X=.5\R@c \advance\d@X-.5\L@c 
 \advance\A@\L@c \divide\A@\tw@ \fi
 \ifdim\U@c=\D@c \d@Y=\z@ 
 \else \d@Y=.5\U@c \advance\d@Y-.5\D@c 
 \advance\B@\D@c \divide\B@\tw@ \fi
 \bgroup
 \L@c=\A@ \U@c=\B@
 \R@p=\U@c \advance\R@p\L@c \multiply\R@p\tw@
 \ifdim\B@<\A@ \quotient@\tmp@\U@c\L@c \R@c=\tmp@\p@ \D@c=\p@
 \quotient@\tmp@\R@p\L@c \R@p=\tmp@\p@
 \else
 \ifdim\A@<\B@ \quotient@\tmp@\L@c\U@c \D@c=\tmp@\p@ \R@c=\p@
 \quotient@\tmp@\R@p\U@c \R@p=\tmp@\p@
 \else
 \R@c=\p@ \D@c=\p@ \quotient@\tmp@\R@p\U@c \R@p=\tmp@\p@
 \fi\fi
 \quotient@\sd@X\d@X\L@c \d@X=\sd@X\p@
 \quotient@\sd@Y\d@Y\U@c \d@Y=\sd@Y\p@
 \loop
 \bgroup \U@p=-\p@ \D@p=\z@
 \ifdim\R@c<\p@
 \edef\tmp@{\expandafter\removePT@\the\R@c}\dimen@=\tmp@\R@p 
 \advance\d@X\cosDirection\dimen@
 \else \advance\d@X\cosDirection\R@p \fi
 \edef\sd@X{\expandafter\removePT@\the\d@X}%
 \advance\U@p\sd@X\d@X
 \ifdim\R@c<\p@
 \edef\tmp@{\expandafter\removePT@\the\R@c}\dimen@=\tmp@\d@X 
 \advance\D@p\cosDirection\dimen@
 \else \advance\D@p\cosDirection\d@X \fi
 \ifdim\D@c<\p@
 \edef\tmp@{\expandafter\removePT@\the\D@c}\dimen@=\tmp@\R@p 
 \advance\d@Y\sinDirection\dimen@
 \else \advance\d@Y\sinDirection\R@p \fi
 \edef\sd@Y{\expandafter\removePT@\the\d@Y}%
 \advance\U@p\sd@Y\d@Y
 \ifdim\D@c<\p@
 \edef\tmp@{\expandafter\removePT@\the\D@c}\dimen@=\tmp@\d@Y 
 \advance\D@p\sinDirection\dimen@
 \else \advance\D@p\sinDirection\d@Y \fi
 \multiply\D@p\tw@ 
 \dimen@=\ifdim\U@p<\z@-\fi\U@p 
 \ifdim\dimen@<.01\p@ \U@p=\z@ 
 \else
 \quotient@\tmp@\U@p\D@p \U@p=\tmp@\p@
 \ifdim\U@p<\z@\xywarning@{poor convergence}\U@p=\z@
 \else \advance\R@p-\U@p \U@p=\ifdim\U@p<\z@-\fi\U@p 
 \fi \fi
 \edef\next@{\egroup \R@p=\the\R@p \U@p=\the\U@p \D@p=\the\D@p}\next@
 \ifdim\U@p>\z@ \repeat
 \edef\next@{\egroup \dimen@=\the\R@p}\next@
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \ifdim\B@<\A@ \dimen@=\tmp@\B@ \else \dimen@=\tmp@\A@ \fi
 \dimen@=-\dimen@
 \advance\X@c\cosDirection\dimen@
 \advance\Y@c\sinDirection\dimen@
 \edef\next@{\egroup \X@c=\the\X@c \Y@c=\the\Y@c}\next@ }%
\xydef@\ellipseOuter@{\Edge@c={\rectangleEdge}}
\xydef@\ellipseInner@{%
 \bgroup \X@p=\X@c \Y@p=\Y@c \ellipseEdge@
 \d@X=\X@c\advance\d@X-\X@p
 \ifdim\d@X>\z@ \R@p=\d@X \L@p=\R@p
 \ifdim\L@c=\R@c\else\advance\L@p\L@c \advance\L@p-\R@c \fi
 \else \L@p=-\d@X \R@p=\L@p
 \ifdim\L@c=\R@c \else\advance\R@p\R@c \advance\R@p-\L@c \fi
 \fi
 \d@Y=\Y@c\advance\d@Y-\Y@p
 \ifdim\d@Y>\z@ \U@p=\d@Y \D@p=\U@p
 \ifdim\D@c=\U@c\else\advance\D@p\D@c \advance\D@p-\U@c \fi
 \else \D@p=-\d@Y \U@p=\D@p
 \ifdim\D@c=\U@c\else\advance\U@p\U@c \advance\U@p-\D@c \fi
 \fi
 \edef\next@{\egroup
 \L@c=\the\L@p \D@c=\the\D@p \R@c=\the\R@p \U@c=\the\U@p}%
 \next@ \Edge@c={\rectangleEdge}}
\xydef@\rectangleEdge#1{\ifcase#1\expandafter\rectangleEdge@
 \or \expandafter\rectangleUnder@ \or \expandafter\rectangleDist@
 \or \expandafter\rectangleProp@
 \else \relax \fi}
\xydef@\rectangleEdge@{%
 \ifdim\d@Y<-.05\p@ \rectangleEdge@i
 \else\ifdim\d@Y<.05\p@ \rectangleEdge@ii
 \else \rectangleEdge@iii\fi\fi
 \resetupDirection@}
\xydef@\rectangleEdge@i{%
 \ifdim\d@X<-.05\p@
 \settomin@\X@c+\R@c\U@c\d@X\d@Y \settomin@\Y@c+\U@c\R@c\d@Y\d@X%1a
 \else\ifdim\d@X<.05\p@ \advance\Y@c\U@c
 \else \settomin@\X@c-\L@c\U@c\d@X\d@Y \settomin@\Y@c+\U@c\L@c\d@Y\d@X
 \fi\fi}
\xydef@\rectangleEdge@ii{%
 \ifdim\d@X<-.05\p@ \advance\X@c\R@c
 \else\ifdim\d@X<.05\p@
 \else \advance\X@c-\L@c
 \fi\fi}
\xydef@\rectangleEdge@iii{%
 \ifdim\d@X<-.05\p@
 \settomin@\X@c+\R@c\D@c\d@X\d@Y \settomin@\Y@c-\D@c\R@c\d@Y\d@X%3a
 \else\ifdim\d@X<.05\p@ \advance\Y@c-\D@c
 \else \settomin@\X@c-\L@c\D@c\d@X\d@Y \settomin@\Y@c-\D@c\L@c\d@Y\d@X
 \fi\fi}
\xydef@\settomin@#1#2#3#4#5#6{%
 \edef\nextii@{\A@=\the\A@ \B@=\the\B@}\quotient@\next@{#5}{#6}\nextii@
 \dimen@=\sd@X\sd@Y\next@#4\relax
 \ifdim#3<\dimen@ \dimen@=#3\fi \advance#1#2\dimen@}
\xydef@\rectangleUnder@{\Inside@false
 \ifdim\X@p=\X@c \ifdim\Y@p=\Y@c \Inside@true \fi\fi 
 \ifInside@ \else
 \dimen@=\X@p \advance\dimen@-\X@c 
 \ifdim \dimen@>-\L@c \relax \ifdim\dimen@<\R@c 
 \dimen@=\Y@p \advance\dimen@-\Y@c 
 \ifdim \dimen@>-\D@c \relax \ifdim\dimen@<\U@c 
 \Inside@true 
 \fi\fi\fi\fi\fi }
\xydef@\rectangleDist@{\let\next@=\rectangleDist@i
 \ifdim\d@X<-.05\p@ \dimen@=\R@c
 \else\ifdim\d@X<.05\p@ \dimen@=\z@ \DN@{\dimen@=\dimen@ii}%
 \else \dimen@=\L@c \fi\fi
 \ifdim\d@Y<-.05\p@ \dimen@ii=\U@c
 \else\ifdim\d@Y<.05\p@ \DN@{}%
 \else \dimen@ii=\D@c \fi\fi
 \next@}
\xydef@\rectangleDist@i{%
 \begingroup \quotient@\next\p@{\sd@X\cosDirection\p@}%
 \edef\next{\endgroup \dimen@=\next\dimen@}\next
 \begingroup \quotient@\next\p@{\sd@Y\sinDirection\p@}%
 \edef\next{\endgroup \dimen@ii=\the\dimen@ii}\next
 \ifdim\dimen@ii<\dimen@ \dimen@=\dimen@ii \fi}
\xydef@\rectangleProp@{%
 \enter@{\A@=\the\A@ \B@=\the\B@ \DirectionfromtheDirection@}%
 \reverseDirection@
 \dimen@=1\Direction \count@=\K@ \multiply\count@\tw@
 \ifnum \Direction>\count@
 \DN@{0}%
 \advance\dimen@-2\K@ \quotient@\nextii@{\dimen@}{2\K@}%
 \else\ifnum \Direction>\z@
 \dimen@=-\dimen@ \advance\dimen@2\K@ \quotient@\next@{\dimen@}{2\K@}%
 \DNii@{0}%
 \else\ifnum \Direction>-\count@
 \DN@{1}%
 \quotient@\nextii@{-\dimen@}{2\K@}%
 \else
 \advance\dimen@4\K@ \quotient@\next@{\dimen@}{2\K@}%
 \DNii@{1}%
 \fi\fi\fi
 \advance\X@c-\L@c \dimen@=\L@c \advance\dimen@\R@c 
 \ifdim\dimen@=\z@ \advance\X@c 2\L@c \else \advance\X@c\next@\dimen@ \fi
 \advance\Y@c+\U@c \dimen@=\D@c \advance\dimen@\U@c 
 \ifdim\dimen@=\z@ \advance\Y@c-2\U@c \advance\Y@c\Upness@\U@c
 \else \advance\Y@c-\nextii@\dimen@ \fi
 \leave@}
\message{connections;}
\xydef@\Creset@@{}
\xydef@\Cshavep@@{\noCshavep@@}
\xydef@\Cshavec@@{\noCshavec@@}
\xydef@\Cslidep@@{\noCslidep@@}
\xydef@\Cslidec@@{\noCslidec@@}
\xydef@\Calong@@{\noCalong@@}
\xydef@\Cintercept@@{\noCintercept@@}
\xydef@\Cbreak@@{\noCbreak@@}
\xydef@\Clast@@{\noClast@@}
\xylet@\lastbreak@@=\empty
\xydef@\noCshavep@@{\setupDirection@
 \enter@{\cfromthec@ \DirectionfromtheDirection@}%
 \reverseDirection@ \cfromp@ \the\Edge@c\z@
 \pfromc@ \leave@ \resetDirection@}
\xydef@\noCshavec@@{\setupDirection@ \the\Edge@c\z@ \resetDirection@}
\xydef@\noCslidep@@#1{\dimen@=#1\relax
 \advance\X@p\cosDirection\dimen@ \advance\Y@p\sinDirection\dimen@
 \resetDirection@}
\xydef@\noCslidec@@#1{\dimen@=#1\relax
 \advance\X@c\cosDirection\dimen@ \advance\Y@c\sinDirection\dimen@
 \resetDirection@}
\xydef@\noCalong@@#1{%
 \d@X=#1\d@X \d@Y=#1\d@Y \X@c=\X@p \Y@c=\Y@p \advance\X@c\d@X \advance\Y@c\d@Y
 \resetupDirection@}
\xydef@\noCintercept@@{\enter@{\pfromthep@}%
 \begingroup\Creset@@ \edef\tmp@{\endgroup
 \X@origin=\the\X@p \Y@origin=\the\Y@p \R@c=\the\d@X \U@c=\the\d@Y}\tmp@
 \loop@\dimen@=\ifdim\R@c<\z@-\fi\R@c \advance\dimen@\ifdim\U@c<\z@-\fi\U@c
 \ifdim\dimen@>10\p@ \advance\R@c \ifdim\R@c<\z@-\fi 16sp \divide\R@c\KK@ 
 \advance\U@c \ifdim\U@c<\z@-\fi 16sp \divide\U@c\KK@ \repeat@
 \intersect@ \leave@}
\xydef@\noCbreak@@{\edef\lastbreak@@{\cfromthec@}}
\xydef@\noClast@@{\Creset@@ \edef\lastbreak@@{\cfromthep@}}
\xydef@\no@@{\setupDirection@ \edef\lastbreak@@{\cfromthep@}%
 \enter@{\cfromthec@\pfromthep@\DirectionfromtheDirection@}%
 \edef\Creset@@{\cfromthec@ \pfromthep@ \DirectionfromtheDirection@}%
 \edef\next@{{\sd@X}{\sd@Y}}\expandafter\straightcheckoverlap@\next@
 \setupDirection@ \the\Edge@c\z@
 \swap@\reverseDirection@\the\Edge@c\z@\swap@\reverseDirection@
 \resetDirection@
 \edef\Cshavep@@{\DirectionfromtheDirection@
 \pfromthep@\noexpand\resetDirection@}%
 \edef\Cshavec@@{\DirectionfromtheDirection@
 \cfromthec@\noexpand\resetDirection@}%
 \leave@
 \def\Cslidep@@{\noCslidep@@}\def\Cslidec@@{\noCslidec@@}%
 \def\Calong@@{\noCalong@@}\def\Cintercept@@{\noCintercept@@}%
 \def\Cbreak@@{\noCbreak@@}\def\Clast@@{\noClast@@}\noinsert@}
\xydef@\noinsert@{\ifHidden@\else
 \ifdim\Y@c>\Y@max \Y@max=\Y@c \fi \ifdim\Y@p>\Y@max \Y@max=\Y@p \fi
 \ifdim\Y@c<\Y@min \Y@min=\Y@c \fi \ifdim\Y@p<\Y@min \Y@min=\Y@p \fi
 \ifdim\X@c>\X@max \X@max=\X@c \fi \ifdim\X@p>\X@max \X@max=\X@p \fi
 \ifdim\X@c<\X@min \X@min=\X@c \fi \ifdim\X@p<\X@min \X@min=\X@p \fi
 \fi}
\xydef@\Spread@@{}
\xydef@\checkoverlap@@{}
\xydef@\straight@#1{\setupDirection@ \def\Spread@@{#1}%
 \edef\Creset@@{\cfromthec@ \pfromthep@ \DirectionfromtheDirection@}%
 \edef\lastbreak@@{\cfromthep@}%
 \edef\next@{{\sd@X}{\sd@Y}}\expandafter\straightcheckoverlap@\next@
 \setupDirection@ \the\Edge@c\z@
 \swap@\reverseDirection@\the\Edge@c\z@\swap@\reverseDirection@
 \resetDirection@
 \edef\Cshavep@@{\DirectionfromtheDirection@
 \pfromthep@\noexpand\resetDirection@}%
 \edef\Cshavec@@{\DirectionfromtheDirection@
 \cfromthec@\noexpand\resetDirection@}%
 \noinsert@
 \straight@typeset
 \def\Cbreak@@{\straightCbreak@}\def\Clast@@{\straightClast@}%
 \def\Cslidep@@{\noCslidep@@}\def\Cslidec@@{\noCslidec@@}%
 \def\Calong@@{\noCalong@@}\def\Cintercept@@{\noCintercept@@}%
 \Creset@@}
\xydef@\straightcheckoverlap@#1#2{\def\checkoverlap@@{%
 \ifdim#1\X@p>#1\X@c \let\next@=\relax \fi
 \ifdim#2\Y@p>#2\Y@c \let\next@=\relax \fi}}
\xydef@\straight@typeset{%
 \ifInvisible@ \let\next@=\relax
 \else\ifdim 1\Direction<-2\K@ \DN@{\straightv@}%
 \else\ifdim 1\Direction<\z@ \DN@{\straighth@}%
 \else\ifdim 1\Direction<2\K@ \DN@{\straightv@}%
 \else \DN@{\straighth@}%
 \fi\fi\fi\fi \checkoverlap@@ \next@}
\xylet@\nextbreak@@=\empty
\xydef@\straightCbreak@{\connectRestore@
 \edef\nextbreak@@{\cfromthec@}%
 \Creset@@ \swap@ \the\Edge@c4\enter@{\cmergethec@}\lastbreak@@ \leave@
 \swap@ \the\Edge@c4\enter@{\cmergethec@}\nextbreak@@ \leave@
 \setupDirection@
 \the\Edge@c\z@
 \swap@ \reverseDirection@ \the\Edge@c\z@ \swap@ \reverseDirection@
 \resetDirection@ \noinsert@ \straight@typeset
 \Creset@@ \let\lastbreak@@=\nextbreak@@}
\xydef@\straightClast@{\connectRestore@
 \Creset@@ \swap@ \the\Edge@c4\enter@{\cmergethec@}\lastbreak@@ \leave@
 \swap@
 \setupDirection@
 \the\Edge@c\z@
 \swap@\reverseDirection@ \the\Edge@c\z@ \swap@\reverseDirection@
 \resetDirection@ \noinsert@ \straight@typeset
 \Creset@@ \edef\lastbreak@@{\cfromthep@}}
\xydef@\straighth@{\setbox\z@=\hbox{%
 \setbox8=\copy\lastobjectbox@
 \A@=\wd8\relax \B@=\dp8\relax \advance\B@\ht8\relax
 \ifdim \A@=\z@ \count@@=\m@ne
 \else \dimen@=\sd@X\d@X \divide\dimen@\A@ \count@@=\dimen@ \fi
 \Spread@@
 \ifdim\d@X>\z@ \advance\X@c-\wd8\relax\fi
 \dimen@=-\sd@X\wd8\relax
 \multiply\dimen@\K@dYdX \divide\dimen@\K@
 \ifdim\d@X>\z@ \advance\Y@c\dimen@ \advance\Y@c-\Leftness@\dimen@
 \else \advance\Y@c\Leftness@\dimen@ \fi
 \dimen@=\wd8\relax \A@=\sd@X\d@X \advance\A@-\dimen@
 \B@=\sd@X\dimen@ \multiply\B@\K@dYdX \divide\B@\K@
 \advance\B@-\d@Y \B@=\sd@Y\B@
 \count@=\count@@ \advance\count@\m@ne
 \ifnum\z@<\count@ \divide\A@\count@ \divide\B@\count@ \fi
 \A@=-\sd@X\A@ \B@=\sd@Y\B@ \wd8=\A@
 \kern\X@c \count@=\z@
 \loop@\ifnum\count@<\count@@ \advance\count@\@ne
 \raise\Y@c\copy8\relax \advance\Y@c\B@ \repeat@}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ {\Drop@@}}
\xydef@\straightv@{\setbox\z@=\vtop{%
 \setbox8=\copy\lastobjectbox@
 \A@=\wd8\relax \B@=\dp8\relax \advance\B@\ht8\relax
 \ifdim \B@=\z@ \count@@=\m@ne
 \else \dimen@=\sd@Y\d@Y \divide\dimen@\B@ \count@@=\dimen@ \fi
 \Spread@@
 \dimen@=\dp8\relax \advance\dimen@\ht8\relax
 \B@=\sd@Y\d@Y \advance\B@-\dimen@
 \A@=\sd@Y\dimen@ \multiply\A@\K@dXdY \divide\A@\K@ \advance\A@-\d@X
 \A@=\sd@X\A@ \count@=\count@@ \advance\count@\m@ne
 \ifnum\z@<\count@ \divide\B@\count@ \divide\A@\count@ \fi
 \B@=\sd@Y\B@ \A@=\sd@X\A@ \ht8=\B@ \dp8=\z@
 \ifdim\d@Y<\z@ 
 \advance\Y@c\dimen@ \advance\Y@c\Upness@\B@
 \else
 \advance\dimen@\Upness@\B@ \advance\Y@c-\dimen@ \advance\Y@c\B@
 \fi
 \advance\Y@c\B@ 
 \ifdim\d@X<\z@ \else \advance\X@c-\wd8\relax \fi
 \null \kern-\Y@c \count@=\z@
 \loop@\ifnum\count@<\count@@ \advance\count@\@ne
 \nointerlineskip \moveright\X@c\copy8\relax \advance\X@c\A@
 \repeat@}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ {\Drop@@}}
\message{ Xy-pic loaded}\xyuncatcodes \endinput


==> xy16textures.tex <==
%% xy16textures.tex from $Id: xy16textures.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Textures v1.6'' driver interface option.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{16textures}{Textures v1.6 driver}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\oldTextures@@#1{\dvimessage@{Textures v1.6}{#1}}
\newdriver{%
 \xyaddsupport{color}\oldtexturesColor@@
 \xyaddsupport{crayon}\oldtexturesCrayon@@
 \xyaddsupport{ps}\oldtexturesPS@@
 \xyaddsupport{rotate}\oldtexturesRotate@@
 \xyaddsupport{line}\oldtexturesLine@@
 \xyaddsupport{frame}\oldtexturesFrames@@
 \xyaddsupport{tile}\oldtexturesTiles@@
 \xyaddsupport{cmtip}\relax
}
\xydef@\oldTexturesColours@{\oldtexturesPStypes@
 \let\xylocalColor@=\xyNoColor@@ \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}%
 \installPScolor@ }\else\DN@{}\fi \next@
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\oldtexturesCrayon@@{}}%
 \else\let\next@=\xystandardcolors@ \fi \next@ 
 \let\xycolorwarning@=\relax
 \let\oldtexturesColor@@=\relax
 \let\UnloadColor@@=\NooldTexturesColor@
 }
\xydef@\oldtexturesColor@@{\oldTexturesColours@}
\xydef@\NooldTexturesColor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\oldtexturesColor@@=\oldTexturesColours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\oldtexturesCrayon@@{\oldtexturesColor@@\oldtexturesCrayon@}
\xydef@\oldtexturesCrayon@{\installCrayolaColors@}%
\xydef@\oldtexturesPS@@{\oldtexturesPS@}
\xydef@\oldtexturesPSunload@{\UnloadPS@
 \ifx\xyrealshipout@\undefined\else
 \ifx\shipout\xyrealshipout@
 \else \let\shipout=\xyrealshipout@\fi\fi
 \let\installxyps@@=\relax
 \let\UnloadPS@@=\UnloadPS@
 \let\oldtexturesPS@@=\oldtexturesPS@ }
\xydef@\oldTexturesSpecial@#1{\firstPS@@\special{postscript #1}}
\xydef@\oldTexturesMacro@#1{\special{postscript {#1}xy}}
\xydef@\oldTexturesInclude@#1{\firstPS@@\special{rawpostscriptfile #1}}
\xydef@\oldTexturesRaw@#1{\firstPS@@\special{rawpostscript #1}}
\xydef@\oldtexturesPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\oldTexturesSpecial@\else
 \let\PSspecial@@=\oldTexturesSpecial@
 \let\PSmacro@@=\oldTexturesMacro@
 \let\PSdict@@=\oldTexturesRaw@
 \let\PSraw@@=\oldTexturesRaw@
 \let\PSinclude@@=\oldTexturesInclude@
 \let\PSspecialdict@@=\oldTexturesRaw@
 \let\xyPSobeylines@@=\obeyoldTextureslines@
 \oldTextures@@{PostScript}%
 \fi 
 \oldtexturesCurrpt@ \@PSshipout }
{\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\par \obeyspaces}}
\xylet@\obeyoldTextureslines@=\next
\xydef@\oldtexturesCurrpt@{\let\xyPScurrpt@@=\oldtexturesCurrpt@@}%
\xydef@\oldtexturesCurrpt@@{\PSspecial@@{xyi}\PSraw@@{userdict begin xyx end}}
\xydef@\oldtexturesPS@{\oldtexturesPStypes@ 
 \let\oldtexturesPS@@=\relax
 \let\UnloadPS@@=\oldtexturesPSunload@ 
 \let\installxyps@@=\@PSshipout \installxyps@ }
\xydef@\oldtexturesRotate@@{\oldtexturesRotate@}
\xydef@\oldtexturesRotate@{\oldtexturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \xyRotScale@@ \installPSrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}\UnloadRotate@\relax}\fi
 \next@ }
\xydef@\oldtexturesLine@@{\oldtexturesLine@}
\xydef@\oldtexturesLine@{\oldtexturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}%
 \installPSline@ }%
 \else\DN@{\xydriverfail@{line-styles are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\oldtexturesFrames@@{\oldtexturesFrames@}
\xydef@\oldtexturesFrames@{\oldtexturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}%
 \installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadPSFrames@\relax}\fi
 \next@ }
\xydef@\oldtexturesTiles@@{\oldtexturesTiles@}
\xydef@\oldtexturesTiles@{\oldtexturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}%
 \installPSpatterns@ \xystandardpatterns@}%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xyendinput


==> xy17oztex.tex <==
%% xy17oztex.tex from $Id: xy17oztex.doc,v 3.8 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``OzTeX v1.7'' driver interface option.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{17oztex}{OzTeX v1.7 driver}{\stripRCS$Revision: 3.8 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\OzTeX@@#1{\dvimessage@{OzTeX v1.7}{#1}}
\newdriver{%
 \xyaddsupport{color}\oldoztexColor@@
 \xyaddsupport{crayon}\oldoztexCrayon@@
 \xyaddsupport{ps}\oldoztexPS@@
 \xyaddsupport{rotate}\oldoztexRotate@@
 \xyaddsupport{line}\oldoztexLine@@
 \xyaddsupport{frame}\oldoztexFrames@@
 \xyaddsupport{tile}\oldoztexTiles@@
 \xyaddsupport{cmtip}\relax
}
\xydef@\oldoztexColor@@{\oldOzTeXColours@}
\xydef@\oldOzTeXColours@{\oldOzTeXPStypes@
 \let\xylocalColor@=\xyNoColor@@ \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}%
 \installPScolor@ }\else\DN@{}\fi \next@
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\oldOzTeXCrayon@@{}}%
 \else\let\next@=\xystandardcolors@\fi \next@
 \let\xycolorwarning@=\relax
 \let\oldoztexColor@@=\relax
 \let\UnloadColor@@=\NooldOzTeXColor@
 }
\xydef@\NooldOzTeXColor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\oldoztexColor@@=\oldOzTeXColours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\oldOzTeXCrayon@@{\installCrayolaColors@}
\xydef@\oldoztexPS@@{\oldoztexPS@}
\xydef@\oldoztexPSunload@{\UnloadPS@
 \def\xyPSdictname{}\UsePSdict@@false
 \let\installxyps@@=\relax
 \let\UnloadPS@@=\UnloadPS@
 \xyPSshapes@true 
 \let\oldoztexPS@@=\oldoztexPS@ }
\xydef@\oldOzTeXSpecial@#1{\special{empty.ps {#1}xy}}
\xydef@\oldOzTeXMacro@#1{\special{empty.ps {#1}xy}}
\xydef@\oldOzTeXDict@#1{\special{empty.ps @obxy{#1}stopped pop @eoxy}}
\xydef@\oldOzTeXinclude@#1{\special{#1}}
\xydef@\oldOzTeXraw@#1{\special{empty.ps @boxy #1 @eoxy}}%
\xydef@\oldOzTeXPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\oldOzTeXSpecial@\else
 \let\PSspecial@@=\oldOzTeXSpecial@
 \let\PSmacro@@=\oldOzTeXMacro@
 \let\PSdict@@=\oldOzTeXDict@
 \let\PSraw@@=\oldOzTeXraw@
 \let\PSinclude@@=\oldOzTeXinclude@
 \let\xyPSobeylines@@=\obeyoldOzTeXlines@
 \let\PSspecialdict@@=\oldOzTeXDict@
 \oldOzTeX@@{PostScript}%
 \fi
 \oldOzTeXCurrpt@ }
{\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\space \obeyspaces}}
\xylet@\obeyoldOzTeXlines@=\next
\xydef@\oldOzTeXCurrpt@{\let\xyPScurrpt@@=\OzTeXCurrpt@@}%
\xydef@\oldOzTeXCurrpt@@{}
\xydef@\oldoztexPS@@{\oldOzTeXPStypes@ 
 \let\installxyps@@=\old@OzTeX@PS@
 \installxyps@ }
\xydef@\old@OzTeX@PS@{\UsePSdict@@true
 \let\includePSmessage@=\xyoldOzTeXheader 
 \ifx\undefined\xyPSdictname\def\xyPSdictname{global.ps}\fi}
\xydef@\xyoldOzTeXheader#1#2#3{\UsePSdict@@true}
\xydef@\oldoztexLine@@{\oldoztexLine@}
\xydef@\oldoztexLine@{\oldOzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}\installPSline@ }%
 \else\DN@{\xydriverfail@{line-styles are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\oldoztexFrames@@{\oldOzTeXFrames@}
\xydef@\oldOzTeXFrames@{\oldOzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}\installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadPSFrames@\relax}\fi
 \next@ }
\xydef@\oldoztexTiles@@{\oldOzTeXTiles@}
\xydef@\oldOzTeXTiles@{\oldOzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}\installPSpatterns@
 \xystandardpatterns@ }%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xydef@\oldoztexRotate@@{\oldOzTeXRotate@}
\xydef@\oldOzTeXRotate@{\oldOzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \xyRotScale@@ \installPSrotscale@ \xyPSshapes@false }%
 \else\DN@{\xydriverfail@{rotations are}\UnloadRotate@\relax}\fi
 \next@ }
\xyendinput


==> xy2cell.tex <==
%% xy2cell.tex from $Id: xy2cell.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``2-cell'' feature.
%% Copyright (c) 1993-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this macro package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{2cell}{Two-cell feature}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xyrequire{curve}\xycatcodes
\message{two-cells,}
\xydef@\UseTwocells{\definesupermorphism{twocell}{%
 \xy@{start of 2-cell}{\begingroup}%
 \twocell@}}
\xydef@\UseHalfTwocells{%
 \definesupermorphism{uppertwocell}{%
 \xy@{start of 2-cell}{\begingroup}%
 \uppertwocell@}%
 \definesupermorphism{lowertwocell}{%
 \xy@{start of 2-cell}{\begingroup}%
 \lowertwocell@}}
\xydef@\UseCompositeMaps{\definesupermorphism{compositemap}{%
 \xy@{start composite-map}{\begingroup}%
 \compositemap@}}
\xydef@\UseAllTwocells{%
 \UseTwocells \UseHalfTwocells \UseCompositeMaps }
\xydef@\supermorphism#1[#2]#3{\def\afterMORPHISM{[#2]#3}#1}
\xydef@\afterMORPHISM{}
\xydef@\definesupermorphism#1#2{%
 \expandafter\def\csname x#1\endcsname{\supermorphism{#2}}%
 \expandafter\def\csname u#1\endcsname{\supermorphism{#2}[-1,0]{}}%
 \expandafter\def\csname d#1\endcsname{\supermorphism{#2}[1,0]{}}%
 \expandafter\def\csname l#1\endcsname{\supermorphism{#2}[0,-1]{}}%
 \expandafter\def\csname r#1\endcsname{\supermorphism{#2}[0,1]{}}%
 \expandafter\def\csname uu#1\endcsname{\supermorphism{#2}[-2,0]{}}%
 \expandafter\def\csname dd#1\endcsname{\supermorphism{#2}[2,0]{}}%
 \expandafter\def\csname ll#1\endcsname{\supermorphism{#2}[0,-2]{}}%
 \expandafter\def\csname rr#1\endcsname{\supermorphism{#2}[0,2]{}}%
 \expandafter\def\csname ur#1\endcsname{\supermorphism{#2}[-1,1]{}}%
 \expandafter\def\csname ul#1\endcsname{\supermorphism{#2}[-1,-1]{}}%
 \expandafter\def\csname dr#1\endcsname{\supermorphism{#2}[1,1]{}}%
 \expandafter\def\csname dl#1\endcsname{\supermorphism{#2}[1,-1]{}}%
 \expandafter\def\csname uul#1\endcsname{\supermorphism{#2}[-2,-1]{}}%
 \expandafter\def\csname uur#1\endcsname{\supermorphism{#2}[-2,1]{}}%
 \expandafter\def\csname ull#1\endcsname{\supermorphism{#2}[-1,-2]{}}%
 \expandafter\def\csname urr#1\endcsname{\supermorphism{#2}[-1,2]{}}%
 \expandafter\def\csname ddl#1\endcsname{\supermorphism{#2}[2,-1]{}}%
 \expandafter\def\csname ddr#1\endcsname{\supermorphism{#2}[2,1]{}}%
 \expandafter\def\csname dll#1\endcsname{\supermorphism{#2}[1,-2]{}}%
 \expandafter\def\csname drr#1\endcsname{\supermorphism{#2}[1,2]{}}%
 \expandafter\def\csname uull#1\endcsname{\supermorphism{#2}[-2,-2]{}}%
 \expandafter\def\csname uurr#1\endcsname{\supermorphism{#2}[-2,2]{}}%
 \expandafter\def\csname ddll#1\endcsname{\supermorphism{#2}[2,-2]{}}%
 \expandafter\def\csname ddrr#1\endcsname{\supermorphism{#2}[2,2]{}}}
\newdir{=>}{!/5pt/\dir{=}!/2.5pt/\dir{=}*!/-5pt/\dir2{>}}
\xydef@\arrowobject#1{\def\Arrowobject@{#1}}
\xydef@\Arrowobject@{\dir{=>}}
\xydef@\twocell@{\toks6={3.5}\toks5={@}\toks7={@}\toks8={@}\toks3={f}%
 \tw@cell@ }
\xydef@\uppertwocell@{\toks6={7}\toks5={@}\toks7={@}\toks8={@}\toks3={o}%
 \tw@cell@ }
\xydef@\lowertwocell@{\toks6={-7}\toks5={@}\toks7={@}\toks8={@}\toks3={o}%
 \tw@cell@ }
\xydef@\compositemap@{\toks6={3.5}\toks5={@}\toks7={@}\toks8={@}\toks3={t}%
 \tw@cell@ }
\xydef@\tw@cell@@@{%
 \expandafter\ifx\the\toks6\omit\relax\toks6={}\else
 \expandafter\ifx\expandafter @\the\toks7\relax\expandafter\dimen@\the\toks6\p@
 \expandafter\if\the\toks3t\relax\dimen@=\p@
 \else\expandafter\if\the\toks3o\divide\dimen@\tw@
 \ifdim\dimen@<\z@ \dimen@ii-\p@ \advance\dimen@ii\dimen@
 \dimen@=\dimen@ii \else \dimen@\p@ \fi
 \else\dimen@\p@
 \fi\fi
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter\toks\expandafter7\expandafter{\tmp@}\fi
 \expandafter\ifx\expandafter @\the\toks8\relax
 \expandafter\dimen@\the\toks6\p@
 \expandafter\if\the\toks3t\relax\dimen@\p@
 \else\expandafter\if\the\toks3o\divide\dimen@\tw@
 \ifdim\dimen@<\z@ \dimen@ii-\p@ \advance\dimen@ii\dimen@
 \dimen@=\dimen@ii \else \dimen@\p@ \fi
 \else\dimen@\p@
 \fi\fi
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter\toks\expandafter8\expandafter{\tmp@}\fi
 \expandafter\ifx\expandafter @\the\toks5\relax
 \expandafter\dimen@\the\toks6\p@
 \expandafter\if\the\toks3o\divide\dimen@ by-4\relax
 \else\dimen@\z@\fi
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter\toks\expandafter5\expandafter{\tmp@}\fi
 \fi
 \twocellmod@ 
 \expandafter\if\the\toks3t\relax
 \edef\tmp@{.[\noexpand\twocell@@@@{\the\toks6}{\the\toks5}%
 {\the\toks7}{\the\toks8}{\the\toks3}%
 {\the\toks2}{\the\toks1}{\the\toks@}{\the\toks4}!!!].\afterMORPHISM}%
 \else
 \edef\tmp@{.[\noexpand\twocell@@@@{\the\toks6}{\the\toks5}%
 {\the\toks7}{\the\toks8}{\the\toks3}%
 {\the\toks1}{\the\toks2}{\the\toks@}{\the\toks4}!!!].\afterMORPHISM}%
 \fi 
 \toks@={\endgroup}%
 \expandafter\def\expandafter\next@\expandafter{%
 \expandafter\def\expandafter\twocellhead@\expandafter{\twocellhead@}}%
 \expandafter\addtotoks@\expandafter{\next@}%
 \expandafter\def\expandafter\next@\expandafter{%
 \expandafter\def\expandafter\twocelltail@\expandafter{\twocelltail@}}%
 \expandafter\addtotoks@\expandafter{\next@}%
 \expandafter\addtotoks@\expandafter{\expandafter\twocellPATH\tmp@}%
 \the\toks@ }%
\xydef@\twocellstyle{\scriptstyle}
\xydef@\droptwocelllabel@#1{\xyFN@\droptwocelllabel@@#1@!}
\xydef@\droptwocelllabel@@{%
 \ifx*\next\DN@*{\droptwocelldrop@}%
 \else\DN@##1@!{\droptwocelltext@{##1}}%
 \fi \next@ }
{\xyuncatcodes \gdef\next#1{\drop+!C{\twocellstyle #1}}}
\xylet@\droptwocelltext@=\next
\xydef@\droptwocelldrop@#1@!{\bgroup \let\xy@=\oxy@ 
 \let\objectstyle=\twocellstyle \drop#1{}%
 \edef\tmp@{\egroup \X@min=\the\X@min \X@max=\the\X@max
 \Y@min=\the\Y@min \Y@max=\the\Y@max}\tmp@ }
\xydef@\twocellhead#1{\def\twocellhead@{#1}}
\xydef@\twocelltail#1{\def\twocelltail@{#1}}
\xydef@\twocellhead@{\dir{>}}
\xydef@\twocelltail@{}
\xywarnifdefined\twocellmod@
\xydef@\tw@cell@{\begingroup
 \toks@={{}}\toks1={{}}\toks2={{}}\toks4={{}}%
 \def\twocellmod@{}\xyFN@\tw@@cell@}%
\xydef@\tw@@cell@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\tw@@cell@}%
 \else\ifx\bgroup\next \let\next@=\toks@\afterassignment\tw@@cell@@
 \else\ifx ^\next \DN@^##1{\toks@={##1}\nudgepos@71\tw@@cell@}%
 \else\ifx _\next \DN@_##1{\toks@={##1}\nudgepos@82\tw@@cell@}%
 \else\addLT@\ifx \next \addGT@{\addLT@\DN@##1}{%
 \toks6={##1}\ifx\omit##1\relax\toks3={t}\toks5={0}\fi\xyFN@\tw@@cell@}%
 \else\ifx\omit\next \DN@\omit{\omitarrows@\xyFN@\tw@@cell@}%
 \else\ifx~\next \DN@~{\xyFN@\whichCurveObject@}%
 \else \DN@{\xyFN@\tw@cell@@\empty @}%
 \fi\fi\fi\fi\fi\fi\fi%
 \next@ }
\xydef@\whichCurveObject@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\whichCurveObject@}%
 \else\ifx\next^\DN@^##1{\xy@{~^{##1}}{\uppercurveobject{##1}}\xyFN@\tw@@cell@}%
 \else\ifx\next_\DN@_##1{\xy@{~_{##1}}{\lowercurveobject{##1}}\xyFN@\tw@@cell@}%
 \else\addRQ@\ifx\next \addRQ@\DN@##1{%
 \xy@{~'{##1}}{\def\twocellhead@{##1}}\xyFN@\tw@@cell@}%
 \else\addLQ@\ifx\next \addLQ@\DN@##1{%
 \xy@{~`{##1}}{\def\twocelltail@{##1}}\xyFN@\tw@@cell@}%
 \else\ifx!\next \DN@!{\xyFN@\checkmodmap@}%
 \else\ifx\next\bgroup\DN@##1{\xy@{~{##1}}{\curveobject{##1}}\xyFN@\tw@@cell@}%
 \else\DN@##1{\xy@{~##1}{\curveobject{##1}}\xyFN@\tw@@cell@}%
 \fi\fi\fi\fi \fi\fi\fi 
 \next@ }
\xydef@\checkmodmap@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\checkmodmap@}%
 \else \def\twocellmod@{\modmap@}%
 \ifx\next!\DN@!##1{%
 \xy@{~!!{##1}}{\def\modmapobject@{##1}}\xyFN@\tw@@cell@}%
 \else \DN@{\xyFN@\tw@@cell@}\fi
 \fi \next@ }
\xydef@\omitarrows@{\toks5={0}\toks6={}\toks7={0}\toks8={0}}
\xydef@\tw@@cell@@{\expandafter\xyFN@\expandafter\tw@cell@@\the\toks@ @}
\xydef@\tw@cell@@{\ifx \space@\next\expandafter\DN@\space{\xyFN@\tw@cell@@}%
 \else\ifx ^\next 
 \DN@^##1@{\toks@={##1}\toks4={^}\nudgepos@50\tw@cell@@@}%
 \else\addEQ@\ifx\next 
 \addEQ@\DN@##1@{\toks@={##1}\toks4={=}\nudgepos@50\tw@cell@@@}%
 \else\ifx _\next 
 \DN@_##1@{\toks@={##1}\toks4={_}\nudgepos@50\tw@cell@@@}%
 \else\addLT@\ifx \next 
 \DN@##1@{\toks@={##1}\toks4={_}\nudgepos@50\tw@cell@@@}%
 \else\ifx\omit\next \DN@\omit##1@{\toks4={@}\toks@={##1}\tw@cell@@@}%
 \else\addRQ@\ifx\next \addRQ@\DN@##1@{\toks4={@}\toks3={/}\toks@={##1}%
 \nudgepos@50\tw@cell@@@}%
 \else\addLQ@\ifx\next \addLQ@\DN@##1@{\toks4={@}\toks3={b}\toks@={##1}%
 \nudgepos@50\tw@cell@@@}%
 \else\ifx"\next \DN@"##1@{\toks4={@}\toks3={B}\toks@={##1}%
 \nudgepos@50\tw@cell@@@}%
 \else\ifx!\next \DN@!##1@{\toks4={@}\toks3={@}\toks@={##1}%
 \nudgepos@50\tw@cell@@@}%
 \else\ifx\next\empty\DN@##1@{\toks@={{}}\toks4={_}\tw@cell@@@}%
 \else\DN@##1@{\toks@={##1}\toks4={_}\tw@cell@@@}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@ }
\xywarnifdefined\whichnudge
\xywarnifdefined\whichinfo
\xywarnifdefined\afternudge
\xydef@\nudgepos@#1#2#3{\def\whichnudge{\toks#1}\def\whichinfo{\toks#2}%
 \def\afternudge{#3}\expandafter\xyFN@\expandafter\nudgepos@@\the\toks@ @}
\xydef@\nudgepos@@{\ifx \space@\next\expandafter\DN@\space{\xyFN@\nudgepos@}%
 \else\addLT@\ifx \next
 \addGT@{\addLT@\DN@##1}##2@{%
 \ifx\omit##1\relax\whichnudge={0}\whichinfo={}%
 \else\whichnudge={##1}\whichinfo={##2}\fi\xyFN@\afternudge}%
 \else \DN@##1@{\whichinfo={##1}\xyFN@\afternudge}%
 \fi\fi \next@ }
\xydef@\modmap@{%
 \expandafter\ifx\the\toks4@\toks4={!}%
 \else\expandafter\ifx\the\toks4=\toks4={H}%
 \else\expandafter\ifx\the\toks4^\toks4={A}%
 \else\expandafter\ifx\the\toks4_\toks4={V}\fi\fi\fi\fi 
 \expandafter\DN@\expandafter{\the\toks6}%
 \ifx\next@\empty\relax\else\expandafter\moddefs@\fi}
\xydef@\moddefs@{%
 \expandafter\dimen@\the\toks6\p@
 \ifdim\dimen@=\z@\relax
 \expandafter\dimen@\the\toks7\p@
 \ifdim\dimen@<\z@\advance\dimen@.5\p@\else\advance\dimen@-.5\p@\fi
 \edef\tmp@{\noexpand\toks7={\expandafter\removePT@\the\dimen@}}\tmp@
 \expandafter\dimen@\the\toks8\p@
 \ifdim\dimen@<\z@\advance\dimen@-.5\p@\else\advance\dimen@.5\p@\fi
 \expandafter\ifx\the\toks3t\advance\dimen@-1\p@\fi
 \edef\tmp@{\noexpand\toks8={\expandafter\removePT@\the\dimen@}}\tmp@
 \else
 \ifdim\dimen@<\z@\advance\dimen@-.5\p@\else\advance\dimen@.5\p@\fi
 \edef\tmp@{\noexpand\toks6={\expandafter\removePT@\the\dimen@}}\tmp@
 \expandafter\dimen@\the\toks7\p@
 \ifdim\dimen@<\z@\advance\dimen@-.5\p@\else\advance\dimen@.5\p@\fi
 \expandafter\ifx\the\toks3t\advance\dimen@-2\p@\fi
 \edef\tmp@{\noexpand\toks7={\expandafter\removePT@\the\dimen@}}\tmp@
 \expandafter\dimen@\the\toks8\p@
 \ifdim\dimen@<\z@\advance\dimen@-.5\p@\else\advance\dimen@.5\p@\fi
 \expandafter\ifx\the\toks3t\advance\dimen@-2\p@\fi
 \edef\tmp@{\noexpand\toks8={\expandafter\removePT@\the\dimen@}}\tmp@
 \fi }%
\xydef@\modmapobject#1{\def\modmapobject@{#1}}
\xydef@\modmapobject@{\dir{|}}
\xydef@\@modmapobject@{{\if\@mod@\relax\expandafter\empty
 \else\expandafter\modmapobject@\fi}} 
\xydef@\curveobject#1{\def\ucurveObject@{~*#1}\def\dcurveObject@{~*#1}}
\xydef@\uppercurveobject#1{\def\ucurveObject@{~*#1}}
\xydef@\lowercurveobject#1{\def\dcurveObject@{~*#1}}
\xydef@\ucurveObject@{}
\xydef@\dcurveObject@{}
\xydef@\savetwocellobjects{%
 \xy@{twocell objects}{%
 \expandafter\uppercurveobject\expandafter{\ucurveObject@}%
 \expandafter\lowercurveobject\expandafter{\dcurveObject@}%
 \expandafter\modmapobject\expandafter{\modmapobject@}%
 \expandafter\twocellhead\expandafter{\twocellhead@}%
 \expandafter\twocelltail\expandafter{\twocelltail@}%
 \expandafter\arrowobject\expandafter{Arrowobject@}%
 }}
\xydef@\twocell@path.[#1].{%
 \expandafter\ifx\csname Q@@c\endcsname\relax
 \DN@{\enter@{\cfromthec@ \pfromthep@ \basefromthebase@}%
 \xy@{}{\expandafter\edef\csname Q@@\endcsname{\cfromthec@}}%
 \afterPOS{\xy@{}%
 {\expandafter\edef\csname Q@@c\endcsname{\cfromthec@}}%
 \xy@{}%
 {\cfromid@{@}\expandafter\edef\csname Q@@p\endcsname{\cfromthec@}}%
 \xy@{twocell #1}{#1}\leave@\aftertwoCELL};p,}%
 \else 
 \DN@{\enter@{\cfromthec@ \pfromthep@ \basefromthebase@}%
 \xy@{twocell #1}{#1}\leave@\aftertwoCELL}%
 \fi \next@ }
\xydef@\twocellpath.[#1].{%
 \expandafter\edef\csname Q@@p\endcsname{\cfromthec@}%
 \xy@{}{\enter@{\pfromthep@}}%
 \xy@{}{\enter@{\cfromthec@ \pfromthep@ \basefromthebase@}%
 \enter@{\pfromthec@}}%
 \afterPOS{\xy@{}{\leave@\setupDirection@}#1\restore\restore
 \xy@{end of 2-cell}\xysaveMinMax@ }}%
\xydef@\xysaveMinMax@{\edef\tmp@{\endgroup
 \noexpand\ifdim\X@max<\the\X@max \X@max=\the\X@max\noexpand\fi 
 \noexpand\ifdim\X@min>\the\X@min \X@min=\the\X@min\noexpand\fi 
 \noexpand\ifdim\Y@max<\the\Y@max \Y@max=\the\Y@max\noexpand\fi 
 \noexpand\ifdim\Y@min>\the\Y@min \Y@min=\the\Y@min\noexpand\fi 
 }\tmp@ }
\xylet@\twocellPATH=\twocellpath
\xydef@\aftertwo@CELL{\let\twocellPATH=\twocellpath \def\aftertwoCELL{}}
\xydef@\aftertwoCELL{}
\xydef@\twocell@@@@#1!!!{\xy@{twocell #1}{\twocell@@#1!!!}}
\let\xystatus=\xystatus@
\xydef@\twocell{\hbox\bgroup\@twocell}
\xydef@\uppertwocell{\hbox\bgroup\@uppertwocell}
\xydef@\lowertwocell{\hbox\bgroup\@lowertwocell}
\xydef@\compositemap{\hbox\bgroup\@compositemap}
\xydef@\twocelll#1#{\hbox\bgroup\xy@\save\save@\@twocelll{#1}}
\xydef@\@twocelll#1#2{%
 \afterPOS{\@twocelll@\xyFN@\twocell@#1{#2}}}
\xydef@\uppertwocelll#1#{\hbox\bgroup\xy@\save\save@\@uppertwocelll{#1}}
\xydef@\@uppertwocelll#1#2{%
 \afterPOS{\@twocelll@\xyFN@\uppertwocell@#1{#2}}}
\xydef@\lowertwocelll#1#{\hbox\bgroup\xy@\save\save@\@lowertwocelll{#1}}
\xydef@\@lowertwocelll#1#2{%
 \afterPOS{\@twocelll@\xyFN@\lowertwocell@#1{#2}}}
\xydef@\compositemapp#1#{\hbox\bgroup\xy@\save\save@\@compositemapp{#1}}
\xydef@\@compositemapp#1#2{%
 \afterPOS{\@twocelll@\xyFN@\compositemap@#1{#2}}}
\xydef@\@twocelll@{%
 \expandafter\edef\csname Q@@c\endcsname{\cfromthec@}\swap@
 \expandafter\edef\csname Q@@p\endcsname{\cfromthec@}\swap@
 \let\twocellPATH=\twocell@path
 \def\aftertwoCELL{\twocell@DONE \xy@\restore \leave@ 
 }}
\xydef@\@twocell#1{\DN@{\@twocell@\twocell@}\xyFN@\next@[#1]}
\xydef@\@uppertwocell#1{\DN@{\@twocell@\uppertwocell@}\xyFN@\next@[#1]}
\xydef@\@lowertwocell#1{\DN@{\@twocell@\lowertwocell@}\xyFN@\next@[#1]}
\xydef@\@compositemap#1{\DN@{\@twocell@\compositemap@}\xyFN@\next@[#1]}
\xydef@\@twocell@#1{\ifx\next[\DN@[{\toks@={#1}\xyFN@\@@twocell@}%
 \else\DN@{#1{}}\fi
%% 
 \expandafter\edef\csname Q@@c\endcsname{\cfromthec@}\swap@
 \expandafter\edef\csname Q@@p\endcsname{\cfromthec@}\swap@
 \let\twocellPATH=\twocell@path
 \def\aftertwoCELL{\twocell@DONE}\next@}
\xydef@\@@twocell@{\ifx\next\bgroup\DN@##1]{\the\toks@{##1}}%
 \else\DN@##1]{\the\toks@##1}\fi\next@}
%% \DN@{\twocell}%
%% \expandafter\def\csname*dir@@\codeof\next@ @\endcsname{\@twocell}
%% \DN@{\uppertwocell}%
%% \expandafter\def\csname*dir@@\codeof\next@ @\endcsname{\@uppertwocell}
%% \DN@{\lowertwocell}%
%% \expandafter\def\csname*dir@@\codeof\next@ @\endcsname{\@lowertwocell}
%% \DN@{\compositemap}%
%% \expandafter\def\csname*dir@@\codeof\next@ @\endcsname{\@compositemap}
\xydef@\twocell@DONE{%
 \edef\tmp@{\egroup \X@min=\the\X@min \X@max=\the\X@max
 \Y@min=\the\Y@min \Y@max=\the\Y@max}\tmp@
 \L@c=\X@c \advance\L@c-\X@min \R@c=\X@max \advance\R@c-\X@c
 \D@c=\Y@c \advance\D@c-\Y@min \U@c=\Y@max \advance\U@c-\Y@c
 \ht\z@=\U@c \dp\z@=\D@c \dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@
 \computeLeftUpness@
\setboxz@h{\kern-\X@p \raise-\Y@c\boxz@ }%
\dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@ \ht\z@=\U@c \dp\z@=\D@c 
 \Edge@c={\rectangleEdge}\Invisible@false \Hidden@false
 \edef\Drop@@{\noexpand\drop@Twocell
 \noexpand\def\noexpand\Leftness@{\Leftness@}%
 \noexpand\def\noexpand\Upness@{\Upness@}}%
 \edef\Connect@@{\noexpand\connect@Twocell
 \noexpand\ifdim\X@max<\the\X@max \X@max=\the\X@max\noexpand\fi 
 \noexpand\ifdim\X@min>\the\X@min \X@min=\the\X@min\noexpand\fi 
 \noexpand\ifdim\Y@max<\the\Y@max \Y@max=\the\Y@max\noexpand\fi 
 \noexpand\ifdim\Y@min>\the\Y@min \Y@min=\the\Y@min\noexpand\fi }}%
\xydef@\drop@Twocell{\boxz@ }
\xydef@\connect@Twocell{%
 \setboxz@h{\kern\X@p \raise\Y@c\box\lastobjectbox@ }%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \Drop@@ }
\xywarnifdefined\@mod@
\xywarnifdefined\Arrowtok@
\xydef@\twocell@@#1#2#3#4#5#6#7#8#9!!!{%
 \def\@mod@{@}\DN@{#9}%
 \ifx #9!\def\Arrowtok@{@}\else\ifx #9A\def\Arrowtok@{^}%
 \else\ifx #9V\def\Arrowtok@{_}\else\ifx #9H\def\Arrowtok@{=}%
 \else\def\@mod@{\relax}%
 \ifx #5/\def\Arrowtok@{@}\else\ifx #5b\def\Arrowtok@{@}%
 \else\ifx #5B\def\Arrowtok@{@}\else\ifx #5@\def\Arrowtok@{@}%
 \else\def\Arrowtok@{#9}%
 \fi\fi\fi\fi\fi\fi\fi\fi
 \addEQ@\ifx #9\def\Arrowtok@{=}\fi
 \DN@{\omit}\ifx\next@\Arrowtok@\def\Arrowtok@{}\else
 \edef\Arrowtok@{\codeof\Arrowtok@}\fi
 \save@ \idfromc@{@c}\swap@\idfromc@{@p}\swap@
 \cfromid@{@c}\no@@
 \ifdim \X@c<\X@p \X@min=\X@c \X@max=\X@p \else \X@min=\X@p \X@max=\X@c \fi
 \ifdim \Y@c<\Y@p \Y@min=\Y@c \Y@max=\Y@p \else \Y@min=\Y@p \Y@max=\Y@c \fi
 \Calong@@{.5}\idfromc@{@m}\idfromc@{@m1}\idfromc@{@m2}%
 \ifx #5t\relax 
 \enter@{\cplusthec@\pfromthep@}%
 \enter@\DirectionfromtheDirection@ \begingroup\aboveDirection@ \xydashl@
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\p@\fi
 \ifdim\dimen@=\z@ \DN@{\vfromslide@i{\xydashl@}@}\relax
 \else\DN@{\vfromslide@i{#1\xydashl@}@}\fi \next@
 \czeroEdge@ \leave@ \no@@ \drop@{+}{}\idfromc@{@m1}%
 \DN@{#1}\ifx\next@\empty\DN@{\no@@}\else\DN@{\connect@{\dir}{-}}\fi
 \else 
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\p@\fi
 \ifdim\dimen@=\z@ \enter@{\cplusthec@\pfromthep@}%
 \enter@\DirectionfromtheDirection@ \begingroup\aboveDirection@\xydashl@
 \vfromslide@i{\xydashl@}@\czeroEdge@ \leave@ \idfromc@{@m1}%
 \cfromid@{@p}\swap@\cfromid@{@c}%
 \DN@{#1}\ifx\next@\empty\DN@{\no@@}\else\DN@{\connect@{\dir}{-}}\fi
 \else \DN@{\enter@\cplusthec@ 
 \enter@\DirectionfromtheDirection@ \begingroup\aboveDirection@ \xydashl@
 \vfromslide@i{#1\xydashl@}@\czeroEdge@ \leave@
 \idfromc@{@m1}\cfromid@{@p}\swap@\cfromid@{@c}%
 \edef\next@{\codeof\ucurveObject@}%
 \ifx\next@\empty\DN@{\connect@\crv{"@m1"}}%
 \else 
 \DNii@####1{\connect@\crv{####1}}\expandafter\DN@\expandafter{%
 \expandafter\nextii@\expandafter{\ucurveObject@"@m1"}}%
 \fi \next@ }%
%% \ifx\next@\empty\def\ucurveObject@{.}\fi
%% \enter@\cfromthec@\sinit@\cfromid@{@m1}\senter@\leave@
%% \expandafter\connect@\expandafter\crvs\expandafter{\ucurveObject@}%
%% \sinit@\sleave@ }%
 \fi
 \fi \next@ 
 \DN@{#1}\ifx\next@\empty\relax\else
 \if\@mod@ @\relax 
 \enter@\pfromthep@ \Creset@@
 \ifx #5t\relax
 \PLACEedgec@ \PLACEedgep@ \def\PLACEf@{{.5}}%
 \else \def\next@{\crvreset@}%
 \ifx\next@\Creset@@
 \gettwocelledges@ \edef\PLACEf@{{\expandafter\removePT@\the\dimen@}}%
 \else \PLACEedgec@ \PLACEedgep@ \def\PLACEf@{{.5}}\fi 
 \fi
 \expandafter\Calong@@\PLACEf@ \czeroEdge@ \leave@
 \edef\tmp@{\codeof\modmapobject@}%
 \ifx\tmp@\empty \DN@{\drop@{\dir}{|}}%
 \else \DNii@##1##{\drop@{##1}}%
 \DN@{\expandafter\nextii@\modmapobject@{}}%
 \fi \next@ 
 \fi\fi
 \DN@{#6}\ifx\next@\empty\DN@{\relax}\else
 \DNii@{{}}\ifx\next@\nextii@\DN@{\relax}\else
 \ifx @#3\relax\DN@{\relax}\else
 \DN@{\enter@\pfromthep@ \Creset@@
 \Calong@@{.5}\czeroEdge@ \leave@
 \enter@\cplusthec@ 
 \enter@\DirectionfromtheDirection@\begingroup
 \DN@{#1}\ifx\next@\empty\dimen@\z@\else\dimen@=#1\p@\fi
 \ifdim\dimen@<\z@ \belowDirection@ \xydashl@ 
 \else \aboveDirection@ \xydashl@ \fi
 \dimen@=#3\p@ \if\@mod@ @\relax 
 \advance\dimen@\ifdim\dimen@<\z@-\fi.5\p@\fi
 \edef\next@{\expandafter\removePT@\the\dimen@}%
 \expandafter\vfromslide@i\expandafter{\next@\xydashl@}@\leave@
 \droptwocelllabel@{#6}}%
 \fi\fi\fi \next@ 
 \DN@{#1}\ifx\next@\empty\relax\else
 \ifx #5b\relax
 \enter@ {\pfromthep@ }\Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty \DN@{\dir{>}}%
 \ifx\next@\twocellhead@\drop@{\dir}{<}%
 \else 
 \reverseDirection@ \DNii@##1##{\drop@{##1}}%
 \expandafter\nextii@\twocellhead@{}\reverseDirection@
 \fi
 \else 
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocelltail@{}%
 \fi
 \else\ifx #5@\relax
 \else
 \enter@\pfromthep@ \Creset@@ \PLACEedgec@
 \Calong@@{1}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocellhead@}%
 \ifx\next@\empty\drop@{\dir}{>}%
 \else 
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocellhead@{}%
 \fi
 \ifx #5B\relax
 \enter@ {\pfromthep@ }\Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty \DN@{\dir{>}}%
 \ifx\next@\twocellhead@\drop@{\dir}{<}%
 \else 
 \reverseDirection@\DNii@##1##{\drop@{##1}}%
 \expandafter\nextii@\twocellhead@{}\reverseDirection@
 \fi
 \else 
 \DNii@##1##{\drop@{##1}}\expandafter\drop\twocelltail@{}%
 \fi
 \else\ifx #5/\relax
 \else \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty\relax\else 
 \enter@\pfromthep@ \Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocelltail@{}%
 \fi\fi\fi
 \fi\fi\fi 
 \cfromid@{@p}\swap@\cfromid@{@c}\no@@ \cfromid@{@m}%
 \ifx #5t\relax 
 \idfromc@{@m2}\cfromid@{@m1}\swap@ \cfromid@{@c}\no@@
 \DN@{#1}\ifx\next@\empty\DN@{\no@@}\else\DN@{\connect@{\dir}{-}}\fi
 \else\ifx #5o\relax
 \idfromc@{@m2}\DN@{}%
 \else
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\p@\fi
 \ifdim\dimen@=\z@
 \enter@{\cplusthec@\pfromthep@}%
 \enter@\DirectionfromtheDirection@ \begingroup \belowDirection@\xydashl@
 \vfromslide@i{\xydashl@}@\czeroEdge@ \leave@ \idfromc@{@m2}%
 \DN@{\cfromid@{@p}\swap@\cfromid@{@c}\no@@}%
 \else \DN@{\enter@\cplusthec@
 \enter@\DirectionfromtheDirection@ \begingroup \belowDirection@ \xydashl@
 \vfromslide@i{#1\xydashl@}@\czeroEdge@ \leave@
 \idfromc@{@m2}\cfromid@{@p}\swap@\cfromid@{@c}%
 \edef\next@{\codeof\dcurveObject@}%
 \ifx\next@\empty\DN@{\connect@\crv{"@m2"}}%
 \else 
 \DNii@####1{\connect@\crv{####1}}\expandafter\DN@\expandafter{%
 \expandafter\nextii@\expandafter{\dcurveObject@"@m2"}}%
 \fi \next@ }\fi
%% \enter@\cfromthec@\sinit@\cfromid@{@m2}\senter@\leave@
%% \expandafter\connect@\expandafter\crvs\expandafter{\dcurveObject@}%
%% \sinit@\sleave@ 
%% }\fi
 \fi\fi \next@ 
 \DN@{#1}\ifx\next@\empty\relax\else \ifx #5o\relax\else
 \if\@mod@ @\DN@{\enter@\pfromthep@ \Creset@@ 
 \ifx #5t\relax
 \PLACEedgec@ \PLACEedgep@ \def\PLACEf@{{.5}}%
 \else \def\next@{\crvreset@}%
 \ifx\next@\Creset@@
 \gettwocelledges@ \edef\PLACEf@{{\expandafter\removePT@\the\dimen@}}%
 \else \PLACEedgec@ \PLACEedgep@ \def\PLACEf@{{.5}}\fi 
 \fi
 \expandafter\Calong@@\PLACEf@ \czeroEdge@ \leave@
 \edef\tmp@{\codeof\modmapobject@}\ifx\tmp@\empty\DN@{\drop@{\dir}{|}}%
 \else \DNii@####1####{\drop@{####1}}%
 \DN@{\expandafter\nextii@\modmapobject@{}}\fi
 \next@ }\else\DN@{\relax}\fi
 \next@ \fi\fi
 \DN@{#7}\ifx\next@\empty\DN@{\relax}\else
 \DNii@{{}}\ifx\next@\nextii@\DN@{\relax}\else
 \ifx @#4\relax\DN@{\relax}\else
 \DN@{\enter@\pfromthep@ \Creset@@
 \Calong@@{.5}\czeroEdge@ \leave@
 \enter@\cplusthec@ 
 \enter@\DirectionfromtheDirection@ \begingroup
 \DN@{#1}\ifx\next@\empty\dimen@\z@ \else\dimen@=#1\p@\fi
 \ifx #5t\relax \ifdim\dimen@<\z@ \belowDirection@ \xydashl@
 \else \aboveDirection@ \xydashl@ \fi
 \else \ifdim\dimen@<\z@ \aboveDirection@ \xydashl@ 
 \else \belowDirection@ \xydashl@ \fi
 \fi \dimen@=#4\p@ \if\@mod@ @\relax 
 \advance\dimen@\ifdim\dimen@<\z@-\fi.5\p@\fi
 \edef\next@{\expandafter\removePT@\the\dimen@}%
 \expandafter\vfromslide@i\expandafter{\next@\xydashl@}@\leave@
 \droptwocelllabel@{#7}}%
 \fi\fi\fi \next@
 \DN@{#1}\ifx\next@\empty\relax\else
 \ifx #5o\relax
 \else\ifx #5b\relax
 \enter@ {\pfromthep@ }\Creset@@ \PLACEedgec@ 
 \Calong@@{1}\czeroEdge@ \leave@ 
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty \DN@{\dir{>}}%
 \ifx\next@\twocellhead@\drop@{\dir}{>}%
 \else 
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocellhead@{}%
 \fi
 \else
 \DNii@##1##{\drop@{##1}}\expandafter\drop\twocelltail@{}%
 \fi
 \else\ifx #5/\relax
 \enter@{\pfromthep@}\Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty \DN@{\dir{>}}%
 \ifx\next@\twocellhead@\drop@{\dir}{<}%
 \else 
 \reverseDirection@\DNii@##1##{\drop@{##1}}%
 \expandafter\nextii@\twocellhead@{}\reverseDirection@
 \fi
 \else
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocelltail@{}%
 \fi
 \else\ifx #5@\relax
 \else
 \enter@\pfromthep@ \Creset@@ \PLACEedgec@
 \Calong@@{1}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocellhead@}%
 \ifx\next@\empty\drop@{\dir}{>}%
 \else
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocellhead@{}%
 \fi
 \ifx #5B\relax
 \enter@ {\pfromthep@ }\Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty\DN@{\dir{>}}%
 \ifx\next@\twocellhead@\drop@{\dir}{<}%
 \else 
 \reverseDirection@\DNii@##1##{\drop@{##1}}%
 \expandafter\nextii@\twocellhead@{}\reverseDirection@
 \fi
 \else
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocelltail@{}%
 \fi
 \else
 \edef\next@{\codeof\twocelltail@}%
 \ifx\next@\empty\relax\else
 \enter@ {\pfromthep@ }\Creset@@ \PLACEedgep@
 \Calong@@{0}\czeroEdge@ \leave@
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\twocelltail@{}%
 \fi\fi
 \fi\fi\fi
 \fi\fi
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\p@\fi
 \ifdim\dimen@<\z@ \cfromid@{@m2}\swap@\cfromid@{@m1}%
 \else \cfromid@{@m1}\swap@\cfromid@{@m2}%
 \fi \no@@ \cfromid@{@m}%
 \ifx\Arrowtok@\empty
 \else\DN@{_}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \enter@{\pfromthep@ \cplusthec@}\dimen@=#2\xydashl@ 
 \enter@\DirectionfromtheDirection@ \begingroup
 \expandafter\vfromslide@i\expandafter{\the\dimen@}@\czeroEdge@
 \leave@ \idfromc@{@m}%
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\Arrowobject@{}%
 \else\DN@{^}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \DN@{_}\edef\Arrowtok@{\codeof\next@}%
 \enter@{\pfromthep@ \cplusthec@}\dimen@=#2\xydashl@ 
 \enter@\DirectionfromtheDirection@ \begingroup
 \expandafter\vfromslide@i\expandafter{\the\dimen@}@\czeroEdge@
 \leave@ \idfromc@{@m}\reverseDirection@
 \DNii@##1##{\drop@{##1}}\expandafter\nextii@\Arrowobject@{}%
 \else \DN@{=}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \enter@{\pfromthep@ \cplusthec@}%
 \dimen@=#2\xydashl@ \advance\dimen@\xydashl@ 
 \enter@\DirectionfromtheDirection@ \begingroup
 \expandafter\vfromslide@i\expandafter{\the\dimen@}@\czeroEdge@
 \leave@ \idfromc@{@m2}%
 \cfromid@{@m}%
 \enter@{\pfromthep@ \cplusthec@}%
 \dimen@=#2\xydashl@ \advance\dimen@-\xydashl@ 
 \enter@\DirectionfromtheDirection@ \begingroup
 \expandafter\vfromslide@i\expandafter{\the\dimen@}@\czeroEdge@
 \leave@ \idfromc@{@m1}%
 \cfromid@{@m2}\swap@\cfromid@{@m1}\connect@{\dir 2}{-}%
 \fi\fi\fi\fi
 \DN@{#8}\ifx\next@\empty\DN@{}\else\DN@{%
 \ifx\Arrowtok@\empty
 \Calong@@{.5}%
 \else\DN@{=}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \Calong@@{.5}%
 \else\DN@{_}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \cfromid@{@m}%
 \fi\fi\fi
 \enter@\cplusthec@
 \enter@\DirectionfromtheDirection@ \begingroup \aboveDirection@\xydashl@
 \ifx\Arrowtok@\empty
 \def\tmp@{0pt}%
 \else\DN@{=}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \def\tmp@{\xydashl@}%
 \else\DN@{_}\edef\next@{\codeof\next@}\ifx\next@\Arrowtok@
 \def\tmp@{1.2\xydashl@}%
 \else\def\tmp@{0pt}%
 \fi\fi\fi
 \expandafter\vfromslide@i\expandafter{\tmp@}@\czeroEdge@ \leave@
 \droptwocelllabel@{#8}%
 }\fi \next@ 
 \leave@ }%
\xydef@\gettwocelledges@{%
 \bgroup \the\crvpts@ 
 \edef\next@{\edges@}%
 \expandafter\gettwocelledges@@\next@ }
\xydef@\gettwocelledges@@#1;#2,#3;#4,{%
 \dimen@=#2\advance\dimen@-#4\relax
 \advance\dimen@ 2\p@ \divide\dimen@ by4 \relax
 \edef\next@{\egroup\dimen@=\the\dimen@ }\next@}%
\xyendinput


==> xyall.tex <==
%% xyall.tex from $Id: xyall.doc,v 3.8 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``All features'' option.
%% Copyright (c) 1993-1996 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{all}{All features}{\stripRCS$Revision: 3.8 $}%
 {Kristoffer H.~Rose}{krisrose@tug.org}%
 {IBM T.~ J.\ Watson Research Center, P.O.~Box 704, Yorktown Heights, NY 10598 (USA)}
\xyrequire{curve}
\xyrequire{frame}
\xyrequire{cmtip}
\xyrequire{line}
\xyrequire{rotate}
\xyrequire{color}
\xyrequire{matrix}
\xyrequire{arrow}
\xyrequire{graph}
\xyendinput


==> xyarc.tex <==
%% xyarc.tex from $Id: xyarc.doc,v 3.8 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Circles, Ellipses and Arcs'' feature.
%% Copyright (c) 1995-1997 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The XY-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The XY-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{arc}{Circle, Ellipse, Arc feature}{\stripRCS$Revision: 3.8 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xyrequire{curve}
\xycatcodes
\xydef@\ellipse#1#{\xy@{ELLIPSE}{\hbox\bgroup\save@}%
 \let\endarc@=\endellipse@@ \xyFN@\preARC@ #1@}
\xydef@\endellipse@@{\xy@{endELLIPSE}{\leave@\origDirection@
 \edef\next@{\egroup \X@min=\the\X@min \X@max=\the\X@max
 \Y@min=\the\Y@min \Y@max=\the\Y@max }\next@}\let\bstartPLACE@=\relax}
\xydef@\preARC@{%
 \ifx\next\space@ \expandafter\DN@\space{\xyFN@\preARC@}%
 \else\ifx\next @\DN@{\xy@{ellipseARC}\ellipticARC@ \arc@}%
 \else\ifx\next ~\DN@~##1{\tildeARC@{##1}}%
 \else\DN@{\xy@{ellipticARC}\ellipticARC@ \arc@}%
 \fi\fi\fi \next@ }
\xydef@\arc@#1@#2{\DN@{#2}%
 \ifx\next@\empty \xy@{arcSTYLE}{\def\arcSTYLE{-}}%
 \else \xy@{arcSTYLE}{\def\arcSTYLE{#2}}\fi \arc@i
 \DNii@{#1}%
 \ifx\nextii@\empty \DN@{\fullCircle@}%
 \else \DN@{_}%
 \ifx\next@\nextii@ \xy@{_}{\def\arcOrient@@{_}}%
 \let\arcOrient@@=\next@ \DN@{\fullCircle@}%
 \else \DN@{^}%
 \ifx\next@\nextii@ \xy@{^}{\def\arcOrient@@{^}}%
 \let\arcOrient@@=\next@ \DN@{\fullCircle@}%
 \else \DN@{\def\afterARCextents@@{%
 \xy@{aftARCext}{\let\doCircleArc@=\doCircleArc@@}%
 \ellipseArc@ \xy@{doCircARCs}{\doCircleArcs@}\endarc@ }%
 \xyFN@\getarcparams@#1@}\fi\fi\fi
 \next@ }
\xydef@\arc@i{\xy@{ARCi}{%
 \save@\idfromc@{0@c}\cfromp@\idfromc@{0@p}%
 \enter@\cplusthec@ \enter@\relax\begingroup\vfromslide@i{}@\czeroEdge@ 
 \leave@\idfromc@{0@m}\leave@ \zeroDivideLimit@{50}%
 \edef\origDirection@{\Direction=\the\Direction
 \relax\noexpand\imposeDirection@}%
 \let\startDirection@=\origDirection@ \def\startDirection@@{}%
 \def\endDirection@{}\def\endDirection@@{}\def\arcOrient@@{^}}%
 \def\arcOrient@@{^}\let\processDirections@=\checkstartDirection@ 
 \def\arcRadius@{}\def\ellipseRatio@{}\def\arcScale@{\arcScale@@}}
\message{circles,}
\xydef@\fullCircle@{\xy@{fullCIRC}{\let\endDirection@=\relax
 \let\doCircleArc@=\doMergeEndArc@@}\circleArc@ }%
\xydef@\getarcparams@{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\getarcparams@}%
 \else\addLT@\ifx \next \xy@{<}{}%
 \addGT@{\addLT@\DN@##1}{\splitRadius@dim##1,,@}%
 \else\ifx\next (\DN@({\xyFN@\checkRadOpen@}%
 \else\ifx\next @\xy@{@}{}\DN@ @{\fullEllipse@}%
 \else \addLQ@\ifx \next \addLQ@\DN@{\xy@`{}\ARCturn@}%
 \else \DN@{\getarcExtents@}%
 \fi\fi\fi\fi\fi \next@ }
\xydef@\checkRadOpen@{%
 \ifx\next *\DN@{\xyFN@\getarcExtents@ (}%
 \else \xy@{(}{}\DN@##1){\splitRadius@##1,,@}%
 \fi \next@ }
\xydef@\fixedRadiusArc@{%
 \xy@{fixRadArc}{\save@ \idfromc@{0@0}\cfromp@\idfromc@{0@c}\leave@}%
 \xyFN@\fixedRadiusArc@i }
\xydef@\fixedRadiusArc@i{%
 \ifx\next\space@ \expandafter\DN@\space{\xyFN@\fixedRadiusArc@i}%
 \else\ifx\next @\xy@{@}{}\DN@ @{\fullEllipse@}%
 \else\DN@{\let\processDirections@=\processArcDirections@
 \def\afterARCextents@@{\xy@{aftARCext}{\let\doCircleArc@=\doCircleArc@@ 
 \ellipseSector@}}\xyFN@\getarcExtents@}%
 \fi\fi \next@ }
\xydef@\arcScale@@{\xy@{arcSCALE@@}{\save@
 \cfromid@{0@0}\pfromc@\cfromid@{0@p}\setbase@\X@p\Y@p\X@c\Y@c}}
\xydef@\arcScale@dim#1{\xy@{arcSCALEdim}{\save@
 \cfromid@{0@0}\pfromc@ \cfromid@{0@p}\setupDirection@\cfromp@
 \enter@\cplusthec@ \begingroup\vfromslide@i#1@%
 \setbase@\X@p\Y@p\X@c\Y@c \idfromc@{0@p}}}
\xydef@\ellipseScale@dim#1{\xy@{ellSCALEdim}{\setupDirection@\cfromp@ 
 \enter@\cplusthec@ \aboveDirection@\xydashl@ \vfromslide@{#1}\leave@
 \setbase@@\X@c\Y@c}}
\xydef@\ellipseScale@#1{\xy@{ellSCALE@}%
 {\vfromcartesian@@0,#1@\setbase@@\X@c\Y@c}}
\xydef@\splitRadius@dim#1,#2,#3@{%
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\relax%\splinetracing 
 \expandafter\def\expandafter\arcRadius@
 \expandafter{\arcScale@dim{#1}}\fi
 \DN@{#2}\ifx\next@\empty\dimen@ii=\z@\def\ellipseRatio@{}%
 \else\dimen@ii=#2\relax \expandafter
 \def\expandafter\ellipseRatio@\expandafter{\ellipseScale@dim{#2}}%
 \fi \fixedRadiusArc@ }
\xydef@\splitRadius@#1,#2,#3@{%
 \DN@{#1}\ifx\next@\empty\dimen@=\z@\else\dimen@=#1\p@\relax\fi
 \DN@{#2}\ifx\next@\empty\dimen@ii=\z@\else\dimen@ii=#2\p@\relax\fi 
 \ifdim\dimen@=\z@ \ifdim\dimen@ii=\z@\else \expandafter
 \def\expandafter\ellipseRatio@\expandafter{\ellipseScale@{#2}}\fi
 \else
 \ifdim\dimen@ii=\z@
 \def\arcScale@{\xy@{arcSCALE@}{\save@\cfromid@{0@0}%
 \X@origin=\X@c \Y@origin=\Y@c
 \X@xbase=#1\X@xbase \Y@xbase=#1\Y@xbase
 \X@ybase=#1\X@ybase \Y@ybase=#1\Y@ybase 
 \advance\X@c\X@xbase \advance\Y@c\Y@xbase \czeroEdge@
 \idfromc@{0@p}\idfromc@{0@c}}}%
 \else
 \def\arcScale@{\xy@{arcSCALE@}{\save@\cfromid@{0@0}%
 \X@origin=\X@c \Y@origin=\Y@c
 \X@xbase=#1\X@xbase \Y@xbase=#1\Y@xbase
 \X@ybase=#2\X@ybase \Y@ybase=#2\Y@ybase 
 \advance\X@c\X@xbase \advance\Y@c\Y@xbase \czeroEdge@
 \idfromc@{0@p}\idfromc@{0@c}}}%
 \fi
 \fi \fixedRadiusArc@ }
\xydef@\baseOrient@{\DN@{_}\ifx\next@\arcOrient@@
 \X@ybase=-\X@ybase \Y@ybase=-\Y@ybase \fi }
\message{ellipses,}
\xydef@\fullEllipse@{\xy@{fullELLIPSE}%
 {\def\startDirection@{}\let\doCircleArc@=\doMergeEndArc@@}%
 \ellipseArc@
 \xy@{doCIRCarcs}{\leave@ \doCircleArcs@}\endarc@ }
\xydef@\ellipseArc@{%
 \arcScale@ \arcRadius@ \ellipseRatio@
 \xy@{arcCONTROLS}{\baseOrient@ \arcControls@ \let\bstartPLACE@=\relax }}
\xydef@\cubicARCcontrols@@{\czeroEdge@
 \vfromcartesian@@0,1@\idfromc@{1@c}%
 \vfromcartesian@@-1,0@\idfromc@{2@c}%
 \vfromcartesian@@0,-1@\idfromc@{3@c}%
 \vfromcartesian@@1,\arcparam@ @\idfromc@{1@m}%
 \vfromcartesian@@\arcparam@,1@\idfromc@{2@m}%
 \vfromcartesian@@-\arcparam@,1@\idfromc@{3@m}%
 \vfromcartesian@@-1,\arcparam@ @\idfromc@{4@m}%
 \vfromcartesian@@-1,-\arcparam@ @\idfromc@{5@m}%
 \vfromcartesian@@-\arcparam@,-1@\idfromc@{6@m}%
 \vfromcartesian@@\arcparam@,-1@\idfromc@{7@m}%
 \vfromcartesian@@1,-\arcparam@ @\idfromc@{8@m}%
 }
\xydef@\doCircleArc@@#1#2{\save@ \ifcase#2\relax
 \doCircleArc@@@{0@p}{1@m}{2@m}{1@c}{#1}\or
 \doCircleArc@@@{1@c}{3@m}{4@m}{2@c}{#1}\or
 \doCircleArc@@@{2@c}{5@m}{6@m}{3@c}{#1}\or
 \doCircleArc@@@{3@c}{7@m}{8@m}{0@p}{#1}\or
 \doCircleArc@@@{0@p}{1@m}{2@m}{1@c}{#1}\or
 \doCircleArc@@@{1@c}{3@m}{4@m}{2@c}{#1}\or
 \doCircleArc@@@{2@c}{5@m}{6@m}{3@c}{#1}\or
 \doCircleArc@@@{3@c}{7@m}{8@m}{0@p}{#1}\fi \leave@ }
\xydef@\doCircleArc@@@#1#2#3#4#5{%
 \cfromid@{#1}\pfromc@\senter@
 \cfromid@{#2}\spushc@\cfromid@{#3}\spushc@\cfromid@{#4}%
 \connect@\crvs{#5}\relax\sinit@\sleave@}
\xydef@\doMergeEndArc@@#1#2{\save@\ifcase#2\relax
 \doMergeEnd@@@{0@p}{1@m}{2@m}{1@c}{#1}\relax\or
 \doMergeEnd@@@{1@c}{3@m}{4@m}{2@c}{#1}\relax\or
 \doMergeEnd@@@{2@c}{5@m}{6@m}{3@c}{#1}\relax\or
 \doMergeEnd@@@{3@c}{7@m}{8@m}{0@p}{#1}@\fi \leave@ }
\xydef@\doMergeEnd@@@#1#2#3#4#5#6{%
 \cfromid@{#1}\pfromc@\senter@
 \cfromid@{#2}\spushc@\cfromid@{#3}\spushc@\cfromid@{#4}%
 \ifx#6\relax
 \L@c=.1\p@ \R@c=\L@c \U@c=\L@c \D@c=\L@c \Edge@c={\rectangleEdge}\fi
 \enter@\cmergethec@\cfromid@{0@c}\leave@
 \enter@\cmergethec@\cfromcontrols@{#1}{#2}{#3}{#4}\leave@
 \connect@\crvs{#5}\relax
 \sinit@\sleave@}
\xydef@\doMergeStartArc@#1#2{\save@\ifcase#2\relax
 \doMergeStart@@{0@p}{1@m}{2@m}{1@c}{#1}@\or
 \doMergeStart@@{1@c}{3@m}{4@m}{2@c}{#1}\relax\or
 \doMergeStart@@{2@c}{5@m}{6@m}{3@c}{#1}\relax\or
 \doMergeStart@@{3@c}{7@m}{8@m}{0@p}{#1}\relax\fi \leave@ }
\xydef@\doMergeStart@@#1#2#3#4#5#6{%
 \cfromid@{#1}\ifx#6\relax
 \L@c=.1\p@ \R@c=\L@c \U@c=\L@c \D@c=\L@c \Edge@c={\rectangleEdge}\fi
 \enter@\cmergethec@\cfromid@{0@x}\leave@
 \enter@\cmergethec@\cfromcontrols@{#4}{#3}{#2}{#1}\leave@
 \pfromc@
 \senter@ \cfromid@{#2}\spushc@\cfromid@{#3}\spushc@\cfromid@{#4}%
 \connect@\crvs{#5}\relax\sinit@\sleave@}
\xydef@\doMergeBothArc@#1#2{\save@\ifcase#2\relax
 \doMergeBoth@@{0@p}{1@m}{2@m}{1@c}{#1}@\or
 \doMergeBoth@@{1@c}{3@m}{4@m}{2@c}{#1}\relax\or
 \doMergeBoth@@{2@c}{5@m}{6@m}{3@c}{#1}\relax\or
 \doMergeBoth@@{3@c}{7@m}{8@m}{0@p}{#1}\relax\fi \leave@ }
\xydef@\doMergeBoth@@#1#2#3#4#5#6{%
 \cfromid@{#1}\ifx#6\relax
 \L@c=.1\p@ \R@c=\L@c \U@c=\L@c \D@c=\L@c \Edge@c={\rectangleEdge}\fi
 \enter@\cmergethec@\cfromid@{0@x}\leave@
 \enter@\cmergethec@\cfromcontrols@{#4}{#3}{#2}{#1}\leave@
 \pfromc@
 \senter@ \cfromid@{#2}\spushc@\cfromid@{#3}\spushc@\cfromid@{#4}%
 \enter@\cmergethec@\cfromid@{0@c}\leave@ 
 \enter@\cmergethec@\cfromcontrols@{#1}{#2}{#3}{#4}\leave@
 \connect@\crvs{#5}\relax\sinit@\sleave@}
\xydef@\doMergeEndArc@#1#2{\count@@=#2\relax
 \ifnum\count@@>\thr@@ \advance\count@@-4\fi\relax
 \doMergeEndArc@@{#1}\count@@ }
\xydef@\doStraightArc@@#1{\xy@{STRAITarc}{\save@
 \cfromid@{0@p}\pfromc@\cfromid@{0@c}%
 \senter@\connect@\crvs{#1}\sinit@\sleave@\leave@}}
\xydef@\cfromcontrols@#1#2#3#4{\bgroup
 \cfromid@{#1}\L@p=\X@c \U@p=\Y@c
 \cfromid@{#4}\R@p=\X@c \D@p=\Y@c
 \cfromid@{#3}\A@=\X@c \B@=\Y@c \cfromid@{#2}%
 \ifdim\R@p>\L@p \ifdim\A@>\R@p \R@p=\A@
 \ifdim\X@c>\R@p \R@p=\X@c\fi\fi
 \else \ifdim\A@<\R@p \R@p=\A@
 \ifdim\X@c<\R@p \R@p=\X@c\fi\fi
 \fi
 \ifdim\D@p>\U@p \ifdim\B@>\D@p \D@p=\B@
 \ifdim\Y@p>\D@p \D@p=\Y@p\fi\fi
 \else \ifdim\B@<\D@p \D@p=\B@
 \ifdim\Y@p<\D@p \D@p=\Y@p\fi\fi
 \fi 
 \edef\next@{\egroup \X@c=\the\R@p \Y@c=\the\D@p}\next@ }
\xydef@\doCircleArcs@{\save@
 \cfromid@{0@0}\pfromc@\cfromid@{0@p}\setupDirection@
 \startDirection@ \edef\startDirection@@{\the\Direction}%
 \cfromid@{1@c}\setupDirection@ \edef\quadDirection@{\the\Direction}\relax 
 \count@=\quadDirection@ \relax\def\nextii@{^}%
 \let\preDirection@@=\startDirection@@ 
 \ifx\nextii@\arcOrient@@
 \ifnum\quadDirection@>\startDirection@@ \relax
 \else \advance\count@ by8192 \relax\edef\quadDirection@{\the\count@}\fi
 \ifx\endDirection@@\empty
 \ifx\endDirection@\relax
 \bgroup\cfromid@{0@c}\setupDirection@
 \edef\next@{\egroup \count@@=\the\Direction}\next@ \relax
 \ifnum\count@@<\startDirection@@ \advance\count@@ 8192 \fi
 \edef\endDirection@@{\the\count@@}%
 \else
 \count@@=\startDirection@@
 \advance\count@@ by8192 \edef\endDirection@@{\the\count@@}%
 \fi
 \else 
 \count@@=\endDirection@@ \relax\ifnum\count@@<\startDirection@@ \relax
 \advance\count@@ by8192 \edef\endDirection@@{\the\count@@}\fi
 \fi
 \ifnum\endDirection@@>\quadDirection@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{0}}%
 \else
 \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{0}}%
 \fi
 \else
 \ifnum\count@<\startDirection@@\relax\else\advance\count@ by-8192 \relax
 \edef\quadDirection@{\the\count@}\fi
 \ifx\endDirection@@\empty
 \ifx\endDirection@\relax
 \bgroup\cfromid@{0@c}\setupDirection@
 \edef\next@{\egroup \count@@=\the\Direction}\next@ \relax
 \ifnum\count@@>\startDirection@@ \advance\count@@-8192 \fi
 \edef\endDirection@@{\the\count@@}%
 \else
 \count@@=\startDirection@@
 \advance\count@@ by-8192 \edef\endDirection@@{\the\count@@}%
 \fi
 \else 
 \count@@=\endDirection@@ \relax \ifnum\count@@>\startDirection@@
 \advance\count@@ by-8192 \edef\endDirection@@{\the\count@@}\fi
 \fi
 \ifnum\endDirection@@<\quadDirection@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{0}}%
 \else \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{0}}\fi
 \fi
 \next@ \relax
 \count@=\quadDirection@ \relax\def\nextii@{^}\DN@{}%
 \ifx\nextii@\arcOrient@@
 \count@@=\startDirection@@ \advance\count@@ by4096 \relax
 \ifnum \count@<\endDirection@@ \relax
 \ifnum\endDirection@@>\count@@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{1}}%
 \else \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{1}}\fi
 \fi
 \else 
 \count@@=\startDirection@@ \advance\count@@ by-4096 \relax
 \ifnum \count@>\endDirection@@ \relax 
 \ifnum\endDirection@@<\count@@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{1}}%
 \else \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{1}}\fi
 \fi\fi 
 \next@ \relax
 \ifx\next@\empty \else \relax
 \count@=\startDirection@@ \relax\def\nextii@{^}\DN@{}%
 \ifx\nextii@\arcOrient@@ \advance\count@ by4096 \relax
 \count@@=\quadDirection@ \advance\count@@ by4096 \relax
 \ifnum \count@<\endDirection@@ 
 \ifnum\endDirection@@>\count@@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{2}}%
 \else \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{2}}\fi
 \fi
 \else \advance\count@ by-4096 \relax
 \count@@=\quadDirection@ \advance\count@@ by-4096 \relax
 \ifnum \count@>\endDirection@@ \relax
 \ifnum\endDirection@@<\count@@
 \DN@{\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{2}}%
 \else \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{2}}\fi
 \fi\fi 
 \next@ \relax
 \fi
 \ifx\next@\empty \else \relax
 \count@=\quadDirection@ \def\nextii@{^}\DN@{}%
 \ifx\nextii@\arcOrient@@ \advance\count@ by4096 \relax
 \ifnum \count@<\endDirection@@
 \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{3}}\fi
 \else \advance\count@ by-4096 \relax
 \ifnum \count@>\endDirection@@ 
 \DN@{\expandafter\doCircleArc@\expandafter{\arcSTYLE}{3}}\fi
 \fi \next@ \relax
 \fi
 \leave@ }
\message{elliptical arcs,}
\xydef@\arcmagic@@{0.5517847}
\xylet@\arcmagic=\arcmagic@@
\xydef@\tildeARC@#1{%
 \if q#1\DN@{\xy@{quadARC}\quadARC@ \arc@}%
 \else\if c#1\DN@{\xyFN@\cubicARC@i}%
 \else\if e#1\DN@{\xy@{ellipticARC}\ellipticARC@ \arc@}%
 \else\if i#1\DN@{\xy@{interpARC}\interpARC@ \arc@}%
 \else\if p#1\DN@{\xy@{cuspidalARC}\cuspidalARC@ \arc@}%
 \else\xywarning@{unknown arc type: #1 }%
 \DN@{\xy@{ellipticARC}\ellipticARC@ \arc@}%
 \fi\fi\fi\fi\fi \next@ }
\xydef@\cubicARC@i{%
 \ifx\next\space@ \expandafter\DN@\space{\xyFN@\cubicARC@i}%
 \else\ifx\next (\DN@(##1){\xy@{cubicARC(##1)}{\cubicARC@{##1}}\arc@}%
 \else \DN@{\xy@{cubicARC(1)}{\cubicARC@{1}}\arc@}%
 \fi\fi \next@ }
\xydef@\ellipticARC@{\let\arcControls@=\cubicARCcontrols@@
 \edef\arcparam@{\arcmagic@@}}
\xydef@\cubicARC@#1{\let\arcControls@=\cubicARCcontrols@@
 \dimen@=#1\p@ \edef\arcparam@{\expandafter\removePT@\the\dimen@}}
\xydef@\quadARC@{\let\arcControls@=\cubicARCcontrols@@
 \def\arcparam@{.66667}}
\xydef@\cuspidalARC@{\let\arcControls@=\cubicARCcontrols@@
 \def\arcparam@{2}}
\xydef@\interpARC@{\let\arcControls@=\cubicARCcontrols@@
 \def\arcparam@{1.33333}}
\xydef@\ARCturn@{\xy@@\bgroup\afterCOORD{%
 \xy@@{\edef\next@{\egroup \A@=\the\X@c \B@=\the\Y@c}\next@}\ARCturn@@}}
\xydef@\ARCturn@@#1@{\DN@{#1}\DNii@{^}%
 \ifx\next@\nextii@ \xy@{^}{\def\arcOrient@@{^}}%
 \else\DNii@{_}\ifx\next@\nextii@ \xy@{_}{\def\arcOrient@@{_}}%
 \else\xy@{}{\def\arcOrient@@{}}\fi\fi
 \xy@@\ARCturn@@@ \processDirections@@ }
\xydef@\ARCturn@@@{%
 \bgroup\cfromid@{0@p}\X@p=\X@c \Y@p=\Y@c \X@c=\A@ \Y@c=\B@
 \setupDirection@ \edef\next@{\egroup\count@=\the\Direction}\next@\relax
 \edef\startDirection@@{\the\count@ }%
 \bgroup\cfromid@{0@c}\X@p=\A@ \Y@p=\B@
 \setupDirection@ \edef\next@{\egroup\count@=\the\Direction}\next@\relax
 \edef\endDirection@@{\the\count@}%
 \ifx\arcOrient@@\empty
 \bgroup\cfromid@{0@p}\X@p=\X@c \Y@p=\Y@c \cfromid@{0@c}%
 \setupDirection@ \edef\next@{\egroup\count@@=\the\Direction}\next@\relax
 \count@=-\count@@ \advance\count@\startDirection@@ \relax \count@=-\count@
 \ifnum\count@>4096 \def\arcOrient@@{_}%
 \else\ifnum\count@<-4096 \def\arcOrient@@{^}%
 \else\ifnum\count@>\z@ \def\arcOrient@@{^}%
 \else\def\arcOrient@@{_}\fi\fi\fi
 \fi }
\xydef@\circleArc@{%
 \xy@{circARC@}{\cfromid@{0@p}\pfromc@\cfromp@\startDirection@ 
 \arcCenter@\idfromc@{0@0}%
 \def\startDirection@{\bgroup
 \cfromid@{0@0}\pfromc@\cfromid@{0@p}\setupDirection@ 
 \edef\next@{\egroup \Direction=\the\Direction}\next@
 \relax\imposeDirection@}}%
 \ifx\endDirection@@\empty
 \ifx\arcRadius@\empty \ifx\ellipseRatio@\empty\else
 \DN@{\arcScale@@}\ifx\arcScale@\next@\else
 \xy@@{\bgroup\cfromid@{0@0}\pfromc@\cfromid@{0@c}\setupDirection@
 \edef\next@{\egroup \Direction=\the\Direction}\next@ 
 \edef\endDirection@@{\the\Direction}}\fi\fi\fi\fi
 \ellipseArc@ \xy@@{\leave@ \doCircleArcs@}\endarc@ }
\xydef@\arcbisector{%
 \cfromid@{0@p}\pfromc@\cfromid@{0@c}\setupDirection@
 \advance\X@c\X@p\divide\X@c\tw@ 
 \advance\Y@c\Y@p\divide\Y@c\tw@ \czeroEdge@ \pfromc@
 \enter@\cplusthec@ \enter@\relax\begingroup
 \aboveDirection@\xydashl@ \vfromslide@i{}@\leave@ }
\xydef@\arcCenter@{%
 \cfromid@{0@p}\pfromc@\cfromid@{0@m}\setupDirection@
 \cfromp@\enter@\cplusthec@ \enter@\relax\begingroup
 \aboveDirection@\xydashl@ \vfromslide@i{}@\leave@\no@@
 \arcCenter@i }
\xydef@\arcCenter@i{%
 \enter@{\pfromthep@}\setupDirection@ \Creset@@
 \let\PLACEedgep@@=\PLACEedgep@ \let\PLACEedgec@@=\PLACEedgec@
 \enter@{\pfromthep@\basefromthebase@}\bgroup 
 \arcbisector \edef\next@{\egroup 
 \X@c =\the\X@c \Y@c=\the\Y@c \X@p=\the\X@p \Y@p=\the\Y@p }%
 \next@ \Cintercept@@ \leave@\leave@ }
\xydef@\getarcExtents@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\getarcExtents@}%
 \else\ifx\next @\xy@{@}{}\DN@ @{\fullEllipse@}%
 \else\DN@{\xy@{arcEXTENTs}{\save@ 
 \def\startDirection@{\Direction=\startDirection@@ \imposeDirection@}}%
 \xyFN@\getarcExtents@ii}\fi\fi \next@ }
\xydef@\getarcExtents@ii{%
 \ifx\next!\xy@{![[}{}\DN@![[##1]]{\getxyDirection@{##1}\getarcExtents@iv}%
 \else\DN@{\getarcExtents@iv}\fi \next@ }
\xydef@\getarcExtents@iv{\afterDIRECTIONorEMPTY
 {\xy@{startDIR}{\edef\startDirection@@{\the\Direction}\leave@}%
 \xyFN@\getarcOrientation@}%
 {\xy@{startDIR}{\edef\startDirection@@{\the\Direction}\leave@}%
 \xyFN@\getarcOrientation@}}
\xydef@\getarcOrientation@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\getarcOrientation@}%
 \else\ifx\next @\xy@{@}{}\DN@{\getEndDirection@x}%
 \else\ifx\next,\xy@{,}{}\DN@,{\xyFN@\getarcOrientation@i}%
 \else\DN@{\getarcOrientation@i}\fi\fi\fi \next@ }%
\xydef@\getarcOrientation@i{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\getarcOrientation@i}%
 \else\ifx\next @\xy@{@}{}\DN@{\getEndDirection@x}%
 \else\ifx\next^{}\DN@##1{\xy@{^}{\def\arcOrient@@{^}}%
 \def\arcOrient@@{^}\xyFN@\getEndDirection@}%
 \else\ifx\next_\DN@##1{\xy@{_}{\def\arcOrient@@{_}}%
 \def\arcOrient@@{_}\xyFN@\getEndDirection@}%
 \else\DN@{\xyFN@\getEndDirection@}%
 \fi\fi\fi\fi \next@ }
\xydef@\getEndDirection@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\getEndDirection@}%
 \else\ifx\next,\DN@,{\xy@{,}{}\xyFN@\getEndDirection@}%
 \else\addEQ@\ifx\next\addEQ@\DN@{\xy@{=}{\save@\startDirection@}%
 \xyFN@\getEqDirection@}%
 \else \ifx\next!\DN@![[##1]]{\xy@{![[}{\save@}\getxyDirection@{##1}%
 \xy@{endDIR}{\edef\endDirection@@{\the\Direction}}%
 \xyFN@\getEndDirection@i}%
 \else \DN@{\xy@{origDIR}{\save@\origDirection@}\getEndDirection@i}%
 \fi\fi\fi\fi \next@ }
\xydef@\getEqDirection@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\getEqDirection@}%
 \else\ifx\next @\xy@{@}{}\DN@ @{%
 \xy@{sameDIR}{\edef\endDirection@@{\startDirection@@}\leave@}%
 \parEllipse@{1}{}}%
 \else\ifx\next (\DN@({\xyFN@\checkEqOpen@}%
 \else \DN@{\getEndDirection@i}\fi\fi\fi \next@ }
\xydef@\checkEqOpen@{%
 \ifx\next *\DN@{\getEndDirection@i (}%
 \else \DN@##1)##2@{\xy@{()}\leave@ \parEllipse@{##1}{##2}}%
 \fi \next@ }
\xydef@\getEndDirection@i{\afterDIRECTIONorEMPTY
 {\xy@{endDIR}{\edef\endDirection@@{\the\Direction}\leave@}%
 \getEndDirection@x }%
 {\xy@{endDIR}\leave@ \getEndDirection@x }}
\xydef@\getEndDirection@x#1@{%
 \DN@{#1}\ifx\next@\empty\relax \else\xywarning@{\omittingTokens@}\fi
 \processDirections@ }
\xydef@\omittingTokens@{omitting unused tokens: \codeof\next@ }
\xydef@\processDirections@@{%
 \ifx\endDirection@@\empty \skewCircle@
 \else \skewEllipse@ \expandafter \afterARCextents@@ \fi }
\xydef@\processArcDirections@{%
 \xy@{ARCdirs}{\ifx\endDirection@@\empty
 \origDirection@ \edef\endDirection@@{\the\Direction}\fi}%
 \ellipseArc@ 
 \xy@{procARCdirs}\processArcDirections@@
 \let\arcScale@\ellsave@ \let\arcRadius@\ellsave@ \def\ellipseRatio@{}%
 \xy@{circSECTORS}{\doCircleSectors@}\endarc@ }
\xydef@\ellsave@{\xy@@{\save@}}
\xydef@\processArcDirections@@{\save@
 \bgroup \cfromid@{0@0}\pfromc@ \Direction=\startDirection@@ 
 \DN@{_}\ifx\next@\arcOrient@@
 \advance\Direction \ifnum\Direction<\z@-\fi 4096 \relax\fi 
 \imposeDirection@
 \d@X=\cosDirection\Y@ybase \advance\d@X-\sinDirection\X@ybase
 \d@Y=-\cosDirection\Y@xbase \advance\d@Y\sinDirection\X@xbase
 \setupDirection@i
 \d@X=-\cosDirection\X@ybase \advance\d@X\sinDirection\X@xbase
 \d@Y=-\cosDirection\Y@ybase \advance\d@Y\sinDirection\Y@xbase
 \enter@\cplusthec@\X@c=\d@X \Y@c=\d@Y \leave@ \czeroEdge@
 \setupDirection@i 
 \czeroEdge@
 \edef\next@{\egroup \cfromthec@ \count@=\the\Direction}\next@
 \edef\startDirection@@{\the\count@}\idfromc@{0@x}%
 \bgroup \cfromid@{0@0}\pfromc@ \Direction=\endDirection@@
 \DN@{_}\ifx\next@\arcOrient@@
 \advance\Direction \ifnum\Direction<\z@-\fi 4096 \relax\fi 
 \imposeDirection@ 
 \d@X=\cosDirection\Y@ybase \advance\d@X-\sinDirection\X@ybase
 \d@Y=-\cosDirection\Y@xbase \advance\d@Y\sinDirection\X@xbase
 \setupDirection@i
 \d@X=-\cosDirection\X@ybase \advance\d@X\sinDirection\X@xbase
 \d@Y=-\cosDirection\Y@ybase \advance\d@Y\sinDirection\Y@xbase
 \enter@\cplusthec@\X@c=\d@X \Y@c=\d@Y \leave@
 \czeroEdge@ 
 \setupDirection@i 
 \edef\next@{\egroup \cfromthec@ \count@=\the\Direction}\next@
 \edef\endDirection@@{\the\count@}\idfromc@{0@c}%
 \count@=\startDirection@@ \relax \count@@=\endDirection@@ \relax
 \DN@{^}\ifx\arcOrient@@\next@
 \ifnum\count@@>\count@ \else\advance\count@@ 8192 \relax\fi
 \else
 \ifnum\count@@<\count@ \else\advance\count@@-8192 \relax\fi\fi
 \edef\startDirection@@{\the\count@}%
 \edef\endDirection@@{\the\count@@}}%
\xydef@\doCircleSectors@{%
 \let\doCircleArc@=\doMergeEndArc@@ \leave@ \leave@
 \cfromid@{0@0}\pfromc@\cfromid@{0@p}\setupDirection@ 
 \count@=\Direction \DN@{^}\ifx\arcOrient@@\next@
 \ifnum\count@>\startDirection@@ \advance\count@-8192 \fi\relax
 \count@@=\count@ \advance\count@@ 8192 \relax
 \ifnum\count@@<\endDirection@@ \advance\count@@ 8192 \fi\relax
 \else 
 \ifnum\count@<\startDirection@@ \advance\count@ 8192 \fi\relax
 \count@@=\count@ \advance\count@@-8192 \relax
 \ifnum\count@@>\endDirection@@ \advance\count@@-8192 \fi\relax
 \fi \relax
 \edef\preDirection@@{\the\count@}\edef\postDirection@@{\the\count@@}%
 \cfromid@{1@c}\setupDirection@ \count@=\Direction 
 \def\nextii@{^}\ifx\nextii@\arcOrient@@
 \DN@{\forwardSectors@\doEllipseSectors@}%
 \ifnum\count@<\preDirection@@ \advance\count@ 8192 \relax
 \else \count@@=\count@\advance\count@-8192 \relax
 \ifnum\count@@<\preDirection@@ \else\count@=\count@@ \fi\fi
 \else
 \DN@{\backwardSectors@\doEllipseSectors@}%
 \ifnum\count@>\preDirection@@ \advance\count@-8192 \relax
 \else \count@@=\count@\advance\count@ 8192 \relax
 \ifnum\count@@>\preDirection@@ \else\count@=\count@@ \fi\fi
 \fi \edef\quadDirection@{\the\count@}%
 \next@ }
\xydef@\forwardSectors@{%
 \ifnum \startDirection@@<\quadDirection@ \def\startSector@@{0}%
 \else\count@=\preDirection@@ \advance\count@ 4096 \relax
 \ifnum \startDirection@@<\count@ \def\startSector@@{1}%
 \else\count@=\quadDirection@ \advance\count@ 4096 \relax
 \ifnum\startDirection@@<\count@ \def\startSector@@{2}%
 \else \def\startSector@@{3}\fi\fi\fi 
 \ifnum\quadDirection@ <\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@ 4096 \relax
 \ifnum\count@<\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@ 4096 \relax
 \ifnum\count@<\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@ 8192 \relax
 \ifnum\count@<\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@ 8192 \relax
 \ifnum\count@<\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@ 12288 \relax
 \ifnum\count@<\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@ 12288 \relax
 \ifnum\count@<\endDirection@@ \def\endSector@@{7}%
 \else \def\endSector@@{6}\fi
 \else \def\endSector@@{5}\fi
 \else \def\endSector@@{4}\fi
 \else \def\endSector@@{3}\fi
 \else \def\endSector@@{2}\fi
 \else \def\endSector@@{1}\fi
 \else \def\endSector@@{0}\fi }
\xydef@\backwardSectors@{%
 \ifnum \startDirection@@>\quadDirection@ \def\startSector@@{0}%
 \else\count@=\preDirection@@ \advance\count@-4096 \relax
 \ifnum \startDirection@@>\count@ \def\startSector@@{1}%
 \else\count@=\quadDirection@ \advance\count@-4096 \relax
 \ifnum\startDirection@@>\count@ \def\startSector@@{2}%
 \else \def\startSector@@{3}\fi\fi\fi 
 \ifnum\quadDirection@>\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@-4096 \relax
 \ifnum\count@>\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@-4096 \relax
 \ifnum\count@>\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@-8192 \relax
 \ifnum\count@>\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@-8192 \relax
 \ifnum\count@>\endDirection@@ \relax
 \count@=\preDirection@@ \advance\count@-12288 \relax
 \ifnum\count@>\endDirection@@ \relax
 \count@=\quadDirection@ \advance\count@-12288 \relax
 \ifnum\count@>\endDirection@@ \def\endSector@@{7}%
 \else \def\endSector@@{6}\fi
 \else \def\endSector@@{5}\fi
 \else \def\endSector@@{4}\fi
 \else \def\endSector@@{3}\fi
 \else \def\endSector@@{2}\fi
 \else \def\endSector@@{1}\fi
 \else \def\endSector@@{0}\fi }
\xydef@\doEllipseSectors@{%
 \ifx\startSector@@\endSector@@
 \DN@{\expandafter\doMergeBothArc@\expandafter{\arcSTYLE}{\endSector@@}}%
 \else
 \expandafter\doMergeStartArc@\expandafter{\arcSTYLE}{\startSector@@}%
 \edef\countArcs@@{\startSector@@}%
 \loop@ \count@=\countArcs@@ \relax \advance\count@\@ne
 \ifnum \count@ < \endSector@@ \edef\countArcs@@{\the\count@}%
 \bgroup\expandafter\doCircleArc@@\expandafter{\arcSTYLE}{\countArcs@@}%
 \egroup 
 \repeat@
 \DN@{\expandafter\doMergeEndArc@\expandafter{\arcSTYLE}{\endSector@@}}%
 \fi \next@ }
\xydef@\checkstartDirection@{%
 \bgroup\no@@ \edef\next@{\egroup\count@@=\the\Direction}\next@\relax
 \ifnum\count@@=\startDirection@@ \relax \DN@{\straightArc@}%
 \else \advance\count@@-\startDirection@@ \relax
 \ifnum\count@@=\ifnum\count@@<\z@-\fi 4096 \relax \DN@{\straightArc@}%
 \else \DN@{\processDirections@@}\fi\fi \next@ }
\xydef@\straightArc@{\xywarning@{straight arc encountered}%
 \xy@@{\let\bstartPLACE@=\relax 
 \expandafter\doStraightArc@@\expandafter{\arcSTYLE}}\endarc@ }%
\xydef@\skewEllipse@{\xy@@{\doskewEllipse@}%
 \def\afterARCextents@@{\xy@{aftARCext}{\let\doCircleArc@=\doMergeEndArc@@}%
 \ellipseArc@ \xy@{doCircARCs}{\doCircleArcs@}\endarc@ }%
 \let\arcScale@=\relax \def\arcRadius@{}\def\ellipseRatio@{}}
\xydef@\skewCircle@{\xy@@{\setupDirection@}%
 \ifnum\Direction=\startDirection@@\relax\DN@{\halfEllipse@{1}}%
 \else
 \xy@@{\def\startDirection@{\Direction=\startDirection@@\imposeDirection@}%
 \cfromid@{0@p}\enter@\cplusthec@ \startDirection@
 \enter@\relax\begingroup\vfromslide@i{}@\czeroEdge@\leave@\idfromc@{0@m}%
 \let\endDirection@=\relax \let\doCircleArc@=\doMergeEndArc@@}%
 \DN@{\circleArc@}%
 \fi \next@ }
\xydef@\doskewEllipse@{%
 \def\startDirection@{\Direction=\startDirection@@ \relax
 \imposeDirection@}\startDirection@ \cfromid@{0@p}%
 \enter@\cplusthec@ \enter@\relax\begingroup\vfromslide@i{}@\leave@ 
 \idfromc@{0@x}%
 \ifx\endDirection@@\empty \parallelDirection@
 \else
 \def\endDirection@{\Direction=\endDirection@@ \relax
 \imposeDirection@ }\endDirection@ \skewEllB@ 
 \bgroup\setupDirection@\edef\next@{\egroup\count@@=\the\Direction}\next@
 \edef\endDirection@@{\the\count@@}%
 \fi
 \cfromid@{0@p}\bgroup \setupDirection@
 \edef\next@{\egroup \count@@=\the\Direction}\next@
 \edef\startDirection@@{\the\count@@}}
\xydef@\halfEllipse@#1{\xy@@{%
 \cfromid@{0@p}\pfromc@\cfromid@{0@c}\no@@
 \edef\endDirection@@{\the\Direction}%
 \advance\X@c\X@p \divide\X@c\tw@ \advance\Y@c\Y@p \divide\Y@c\tw@
 \idfromc@{0@0}\pfromc@ \cfromid@{0@p}\setbase@\X@p\Y@p\X@c\Y@c 
 \dimen@=\X@origin \advance\dimen@-\X@c \dimen@ii=\cosDirection\dimen@
 \dimen@=\Y@origin \advance\dimen@-\Y@c \advance\dimen@ii \sinDirection\dimen@
 \X@c=\X@origin \Y@c=\Y@origin \enter@\cplusthec@ 
 \dimen@=#1\p@ \ifdim\dimen@<\z@ \DN@{^}\dimen@ii=-#1\dimen@ii
 \ifx\next@\arcOrient@@\def\arcOrient@@{_}\else\def\arcOrient@@{^}\fi
 \else \dimen@ii=#1\dimen@ii\fi 
 \startDirection@ \enter@\relax\begingroup\expandafter
 \vfromslide@i\expandafter{\the\dimen@ii}@\leave@
 \idfromc@{1@c}\setbase@@ \X@c \Y@c \adjustBaseOrient@
 \count@@=\endDirection@@ \relax
 \DN@{^}\advance\count@@\ifx\arcOrient@@\next@\else-\fi 4096 \relax
 \edef\startDirection@@{\the\count@@}%
 \def\startDirection@{\Direction=\startDirection@@ \imposeDirection@ }%
 \let\doCircleArc@=\doMergeEndArc@@ }%
 \let\arcScale@=\relax \ellipseArc@
 \xy@@{\doCircleArcs@}\endarc@ }
\xydef@\parallelDirection@{\show\parallelDirection@}%
\xydef@\parEllipse@#1#2{\DN@{#2}\ifx\next@\empty 
 \else\xywarning@{\omittingTokens@ }\fi \halfEllipse@{#1}}
\xydef@\skewEllB@{\cfromid@{0@c}\pfromc@\enter@\cplusthec@
 \enter@\relax\begingroup\vfromslide@i{}@\leave@
 \enter@{\pfromthep@\basefromthebase@}\no@@
 \bgroup \cfromid@{0@p}\pfromc@\cfromid@{0@x}\edef\next@{\egroup 
 \X@c =\the\X@c \Y@c=\the\Y@c \X@p=\the\X@p \Y@p=\the\Y@p }\next@
 \Cintercept@@\leave@ \idfromc@{0@x}\cfromid@{0@p}\enter@\cplusthec@
 \cfromid@{0@c}\leave@ \enter@\cplusthec@ \cfromid@{0@x}%
 \X@c=-\X@c \Y@c=-\Y@c \leave@ \idfromc@{0@0}\pfromc@\cfromid@{0@p}%
 \setbase@\X@p\Y@p\X@c\Y@c \cfromid@{0@c}\setbase@@\X@c\Y@c
 \adjustBaseOrient@ }
\xydef@\adjustBaseOrient@{%
 \edef\tmp@{\expandafter\removePT@\the\X@xbase}\dimen@=\Y@ybase
 \divide\dimen@ 64 \relax \dimen@ii=\tmp@\dimen@
 \edef\tmp@{\expandafter\removePT@\the\X@ybase}\dimen@=\Y@xbase
 \divide\dimen@ 64 \relax \dimen@=\tmp@\dimen@
 \ifdim\dimen@>\dimen@ii \X@ybase=-\X@ybase \Y@ybase=-\Y@ybase \fi }
\xyendinput


==> xyarrow.tex <==
%% xyarrow.tex from $Id: xyarrow.doc,v 3.9 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Arrows and Paths'' feature.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{arrow}{Arrow and Path feature}{\stripRCS$Revision: 3.9 $}%
 {Kristoffer H.~Rose}{krisrose@tug.org}%
 {IBM T.~ J.\ Watson Research Center, P.O.~Box 704, Yorktown Heights, NY 10598 (USA)}
\message{path,}
\xydef@\PATH{\afterPATH{}}
\xylet@\afterPATH@=\empty
\xydef@\afterPATH#1{\save
 \DN@##1{\def\afterPATH@{\restore \def\afterPATH@{##1}#1}}%
 \expandafter\next@\expandafter{\afterPATH@}%
 \let\PATHfail@@=\empty
 \let\PATHbefore@@=\empty
 \let\PATHafter@@=\empty
 \let\PATHlabelsevery@@=\empty
 \let\PATHlabelsnext@@=\empty
 \let\PATHlabelslast@@=\empty
 \xy@{\afterPATH{#1}}{\def\PATHslide@@{\z@}}%
 \def\PATHcontinue@@{\xyFN@\PATH@}%
 \xyFN@\PATH@}
\xynew@{if}\ifPATHsingle@
\xydef@\PATH@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATH@}%
 \else\ifPATHsingle@ \let\next@=\PATH@single
 \else \let\next@=\PATH@normal \fi\fi \next@}
\xydef@\PATH@normal{%
 \ifx ~\next \DN@ ~{\xyFN@\PATHsetting@}%
 \else \addRQ@\ifx \next \addRQ@\DN@{\xy@'{}\xyFN@\PATHstraight@}%
 \else \addLQ@\ifx \next \addLQ@\DN@{\xy@`{}\xyFN@\PATHturn@}%
 \else\ifx \PATHfail@@\PATH@x \DN@{\xyFN@\PATHfinal@}%
 \else
 \DNii@{\let\PATHfail@@=\PATH@x \xyFN@\PATH@}%
 \DN@{\expandafter\nextii@\PATHfail@@}%
 \fi\fi\fi\fi \next@}
\xylet@\PATHfail@@=\empty
\xylet@\PATHbefore@@=\empty
\xylet@\PATHafter@@=\empty
\xylet@\PATHlabelsevery@@=\empty
\xylet@\PATHlabelsnext@@=\empty
\xylet@\PATHlabelslast@@=\empty
\xydef@\PATHsetting@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHsetting@}%
 \else\ifx \bgroup\next
 \DN@##1{\xy@{~{##1}}{}\def\PATHfail@@{##1}\xyFN@\PATH@}%
 \else \addEQ@\ifx \next
 \addEQ@\DN@##1{\xy@{~={##1}}{}\def\PATHbefore@@{##1}\xyFN@\PATH@}%
 \else \addLT@\ifx \next
 \addLT@\DN@##1{\xy@{~<{##1}}{}\def\PATHlabelsnext@@{##1}\xyFN@\PATH@}%
 \else \addGT@\ifx \next
 \addGT@\DN@##1{\xy@{~>{##1}}{}\def\PATHlabelslast@@{##1}\xyFN@\PATH@}%
 \else \addPLUS@\ifx \next
 \addPLUS@\DN@##1{\xy@{~+{##1}}{}\def\PATHlabelsevery@@{##1}\xyFN@\PATH@}%
 \else \ifx /\next
 \DN@/##1{\xy@{~/{##1}}{}\def\PATHafter@@{##1}\xyFN@\PATH@}%
 \else \addDASH@\ifx \next
 \xywarning@{Obsolete `-' PATH <action> translated to `='.}%
 \addDASH@\DN@##1{\xy@{~-{##1}}{}\def\PATHbefore@@{##1}\xyFN@\PATH@}%
 \else
 \xyerror@{Unknown \string~ setting: \meaning\next}%
 {See the Xy-pic arrow feature documentation for help.}%
 \fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xylet@\PATHinit@@=\empty
\xylet@\PATHextra@@=\empty
\xylet@\PATHpost@@=\empty
\xylet@\PATHcontinue@@=\empty
\xydef@\PATHstraight@{%
 \def\PATHinit@@{\PATHinitstraight@}%
 \let\PATHextra@@=\empty
 \let\PATHpost@@=\empty
 \let\PATHlabelsextra@@=\relax
 \xy@@\pfromc@ \PATHafterPOS{\xyFN@\PATHsegment@}}
\xydef@\PATHfinal@{%
 \def\PATHinit@@{\PATHinitstraight@}%
 \def\PATHextra@@{\let\PATHcontinue@@=\afterPATH@}%
 \let\PATHpost@@=\empty
 \let\PATHlabelsextra@@=\PATHlabelsextralast@
 \xy@@\pfromc@ \PATHafterPOS{\xyFN@\PATHsegment@}}
\xydef@\PATHlabelsextralast@{\let\PATHlabelsextra@@=\relax
 \expandafter\xyFN@\expandafter\PATHlabels@\PATHlabelslast@@}
\xydef@\PATHinitstraight@{\xy@@{\setupDirection@ \dimen@=\PATHslide@@
 \dimen@ii=-\sinDirection\dimen@
 \ifPATHomitslide@@\else\advance\X@p\dimen@ii\fi \advance\X@c\dimen@ii
 \dimen@ii= \cosDirection\dimen@
 \ifPATHomitslide@@\else\advance\Y@p\dimen@ii\fi \advance\Y@c\dimen@ii
 \PATHomitslide@@false \resetupDirection@}}
\xydef@\PATHslide@@{\z@}
\xynew@{if}\ifPATHomitslide@@
\xydef@\PATHsegment@{%
 \addLT@\ifx\next
 \addGT@{\addLT@\DN@##1}{%
 \xy@{<##1>}{\dimen@=##1\relax \edef\PATHslide@@{\the\dimen@}}%
 \xyFN@\PATHsegment@@}%
 \else \let\next@=\PATHsegment@@
 \fi \next@}
\xydef@\PATHsegment@@{\PATHinit@@ \addEQ@\PATHaction@\PATHbefore@@ \PATHextra@@
 \expandafter\toks@\expandafter{\PATHlabelsnext@@}\let\PATHlabelsnext@@=\empty
 \expandafter\addtotoks@\expandafter{\PATHlabelsevery@@}%
 \expandafter\def\expandafter\PATHlabels@@\expandafter{\the\toks@}%
 \toks@={}\expandafter\xyFN@\expandafter\PATHlabels@\PATHlabels@@}
\xylet@\PATHlabelit@@=\empty
\xydef@\PATHlabels@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHlabels@}%
 \else \ifx ^\next 
 \DN@##1{\xy@^{}\let\PATHlabelit@@=\PATHlabelabove@@
 \DNii@{}\xyFN@\PATHanchor@}%
 \else \ifx _\next
 \DN@##1{\xy@_{}\let\PATHlabelit@@=\PATHlabelbelow@@
 \DNii@{}\xyFN@\PATHanchor@}%
 \else \ifx |\next
 \DN@##1{\xy@|{}\let\PATHlabelit@@=\PATHlabelbreak@
 \DNii@{}\xyFN@\PATHanchor@}%
 \else \let\next@=\PATHfinishsegments@ \fi\fi\fi\fi \next@}
\xydef@\PATHanchor@{\begingroup \toks@={}\PATHanchor@i}
\xydef@\PATHanchor@i{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHanchor@i}%
 \else\addDASH@\ifx \next
 \addDASH@\DN@{\expandafter\addtotoks@\expandafter{\PATHanchor@toks}%
 \xyFN@\PATHanchor@i}%
 \else
 \DNii@##1{\endgroup\afterPLACE{\xyFN@\PATHit@}##1}%
 \DN@{\expandafter\nextii@\expandafter{\the\toks@}}%
 \fi\fi \next@}
{\xyuncatcodes \gdef\next{<>(.5)}}
\xylet@\PATHanchor@toks=\next
\xylet@\PATHitshapes@@=\empty
\xydef@\PATHit@{\let\PATHitshape@@=\empty \xyFN@\PATHit@i}
\xydef@\PATHit@i{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHit@i}%
 \else \ifx *\next \DN@*##1##{\PATHlabelit@@{!C##1}}%
 \else \addAT@\ifx\next \addAT@\DN@##1##{\PATHlabelit@@{\dir##1}}%
 \else \ifx [\next \DN@[##1]{%
 \expandafter\def\expandafter\PATHitshape@@\expandafter{\PATHitshape@@[##1]}%
 \xyFN@\PATHit@i}%
 \else \DN@{\PATHlabelit@@{}}%
 \fi\fi\fi\fi \next@}
\xydef@\PATHfinishsegments@{%
 \ifx\PATHlabelsextra@@\relax \expandafter\PATHfinishsegments@i
 \else
 \expandafter\PATHlabelsextra@@ \fi}
\xydef@\PATHfinishsegments@i{%
 \xy@@{\Clast@@}\the\toks@ \toks@={}%
 \xy@@\setupDirection@
 \PATHpost@@ \PATHaction@/\PATHafter@@
 \PATHcontinue@@}
\xydef@\PATHaction@default#1#2{\xy@{PATHaction#1{#2}}{}\POS#2\relax}
\xylet@\PATHaction=\PATHaction@default
\xydef@\PATHaction@#1#2{\expandafter\PATHaction\expandafter#1\expandafter{#2}}
\xylet@\PATHafterPOS@default=\afterPOS
\xylet@\PATHafterPOS=\PATHafterPOS@default
\xydef@\PATHlastout@@{3}
\xydef@\PATHturn@{\afterCIRorDIAG\PATHturn@cir\PATHturn@diag}
\xydef@\PATHturn@cir{\toks@={\xy@@{%
 \count@=\CIRin@@ \ifnum\count@<4\else\advance\count@-4\fi
 \count@@=\CIRout@@ \ifnum\count@@<4\else\advance\count@@-4\fi
 \ifnum\count@=\count@@ \xyerror@{<turn> cannot be half or full}{%
You asked for a <turn>ed segment with parallel in- and out-direction.^^J%
This is not allowed because it is not possible to position it uniquely.}\fi}}%
 \edef\next@{{\CIRin@@}{\expandafter\noexpand\CIRorient@@}{\CIRout@@}}%
 \expandafter\PATHturn@i\next@}
\xydef@\PATHturn@diag{\toks@={\xy@@{%
 \setupDirection@ \count@=\CIRin@@ \dimen@=\xydashl@ \ABfromdiag@
 \ifdim \sinDirection\A@>\cosDirection\B@ \def\CIRorient@@{\CIRacw@}%
 \advance\count@\ifnum\count@<6 \tw@ \else -6\fi
 \else \def\CIRorient@@{\CIRcw@}%
 \advance\count@\ifnum\count@>\@ne -\tw@ \else 6\fi
 \fi
 \edef\CIRout@@{\the\count@}}}%
 \edef\next@{{\CIRin@@}{}{}}%
 \expandafter\PATHturn@i\next@}
\xylet@\PATHpostpos@@=\empty
\xydef@\PATHturn@i#1#2#3{%
 \DN@##1{\def\PATHinit@@{\xy@@{%
 \def\CIRin@@{#1}\def\CIRorient@@{#2}\def\CIRout@@{#3}%
 \ifnum\CIRin@@=8 \let\CIRin@@=\PATHlastout@@ \fi
 \R@=\turnradius@
 ##1\relax}%
 \xy@@{\count@=\CIRin@@
 \ifPATHomitslide@@ \dimen@=-\PATHslide@@
 \ABfromdiag@ \advance\X@p-\B@ \advance\Y@p\A@ \fi
 \enter@{\pfromthep@ \basefromthebase@}}%
 \xy@@{\dimen@=\expandafter\ifx\CIRorient@@\CIRcw@-\fi\R@
 \ABfromdiag@ \advance\X@p-\B@ \advance\Y@p\A@
 \X@origin=\X@p \Y@origin=\Y@p}%
 \xy@@{\dimen@=\xydashl@ \ABfromdiag@ \R@c=\A@ \U@c=\B@
 \count@=\CIRout@@
 \dimen@=\expandafter\ifx\CIRorient@@\CIRcw@-\fi\R@
 \ABfromdiag@ \advance\X@c-\B@ \advance\Y@c\A@
 \dimen@=\xydashl@ \X@p=\X@c \Y@p=\Y@c
 \ABfromdiag@ \advance\X@p-\A@ \advance\Y@p-\B@
 \intersect@
 \count@=\CIRin@@ \dimen@=\p@ \ABfromdiag@}%
 \xy@@{\edef\next@{\expandafter\removePT@\the\A@}%
 \edef\nextii@{\expandafter\removePT@\the\B@}%
 \A@=\X@c \advance\A@-\X@origin \B@=\Y@c \advance\B@-\Y@origin
 \ifdim \next@\A@<-\nextii@\B@
 \dontleave@ \cfromp@
 \count@=\CIRin@@ \advance\count@\ifnum\count@<4 +4\else -4\fi
 \dimen@=\xydashl@ \Directionfromdiag@
 \the\Edge@c\z@
 \count@=\CIRin@@ \dimen@=\expandafter\ifx\CIRorient@@\CIRcw@-\fi\R@
 \ABfromdiag@ \advance\X@c-\B@ \advance\Y@c\A@
 \dimen@=5sp \ABfromdiag@ \advance\X@c\A@ \advance\Y@c\B@
 \fi
 \dimen@ii=\expandafter\ifx\CIRorient@@\CIRacw@-\fi\PATHslide@@
 \advance\R@\dimen@ii
 \drop@\literal@{\hbox\bgroup\cir@i}}%
 \xy@@{\X@p=\X@c \Y@p=\Y@c
 \count@=\CIRout@@
 \dimen@=\expandafter\ifx\CIRorient@@\CIRacw@-\fi\R@c
 \ABfromdiag@ \advance\X@p-\B@ \advance\Y@p\A@
 \edef\PATHpostpos@@{\X@c=\the\X@p \Y@c=\the\Y@p \noexpand\czeroEdge@
 \noexpand\PATHomitslide@@true}}%
 \xy@@{\count@=\CIRin@@
 \dimen@=\expandafter\ifx\CIRorient@@\CIRacw@-\fi\R@c
 \ABfromdiag@ \advance\X@c-\B@ \advance\Y@c\A@ \czeroEdge@}%
 \xy@@{\leave@
 \count@=\CIRin@@ \dimen@=\PATHslide@@
 \ABfromdiag@ \advance\X@p-\B@ \advance\Y@p\A@
 \edef\PATHlastout@@{\CIRout@@}%
 \count@=\CIRout@@ \dimen@=\xydashl@ \Directionfromdiag@}}}%
 \expandafter\next@\expandafter{\the\toks@}\toks@={}%
 \let\PATHextra@@=\empty
 \def\PATHpost@@{\xy@@\PATHpostpos@@}%
 \let\PATHlabelsextra@@=\relax
 \xyFN@\PATHturn@ii}
\xydef@\PATHturn@ii{%
 \ifx /\next
 \DN@ /{\afterassignment\nextii@\dimen@=}%
 \DNii@{%
 \edef\next@{\noexpand\xy@@{\edef\noexpand\turnradius@{\the\dimen@}}}\next@
 \xy@@\pfromc@ \PATHafterPOS{\xyFN@\PATHsegment@}}%
 \else \DN@{\xy@@\pfromc@ \PATHafterPOS{\xyFN@\PATHsegment@}}\fi
 \next@}
\xydef@\ABfromdiag@{\ifcase\count@\relax
 \A@=-.7071\dimen@ \B@=-.7071\dimen@ \or \A@=\z@ \B@=-\dimen@
 \or \A@=+.7071\dimen@ \B@=-.7071\dimen@ \or \A@=\dimen@ \B@=\z@
 \or \A@=+.7071\dimen@ \B@=+.7071\dimen@ \or \A@=\z@ \B@=+\dimen@
 \or \A@=-.7071\dimen@ \B@=+.7071\dimen@ \or \A@=-\dimen@ \B@=\z@
 \else\xybug@{impossible <diag>?}\fi}
\xydef@\turnradius@{10pt}
\xydef@\turnradius{\afterADDOP{\Addop@@\turnradius@}}
\xydef@\PATHlabelabove@#1#2{\droplabel@\belowDirection@{#1}{#2}%
 \let\afteraliases@@=\empty \xyFN@\PATHlabelalias@}
\xydef@\PATHlabelbelow@#1#2{\droplabel@\aboveDirection@{#1}{#2}%
 \let\afteraliases@@=\empty \xyFN@\PATHlabelalias@}
\xylet@\PATHlabelabove@@=\PATHlabelabove@
\xylet@\PATHlabelbelow@@=\PATHlabelbelow@
\xydef@\droplabel@#1#2#3{\xy@@{\enter@\DirectionfromtheDirection@}%
 \DN@{#2}\ifx\next@\empty
 \expandafter\xy@@ix@\expandafter{\PATHitshape@@\labelbox{#3}}%
 \else \expandafter\xy@@ix@\expandafter{\PATHitshape@@#2{#3}}\fi
 \xy@@{\setbox\z@=\expandafter\object\the\toks9
 \advance\L@c\labelmargin@ \advance\R@c\labelmargin@
 \advance\D@c\labelmargin@ \advance\U@c\labelmargin@ 
 \setboxz@h{\kern\labelmargin@\boxz@\kern\labelmargin@}%
 \A@=\X@c \B@=\Y@c #1\xydashl@ \the\Edge@c\thr@@ 
 \advance\A@-\X@c \advance\B@-\Y@c \advance\X@c 2\A@ \advance\Y@c 2\B@
 \ht\z@=\U@c \dp\z@=\D@c \dimen@=\L@c \advance\dimen@\R@c \wd\z@=\dimen@ 
 \setbox\lastobjectbox@=\hbox{\X@c=\L@c \Y@c=\z@ \Drop@@}%
 \drop@{\box\lastobjectbox@}{}%
 \leave@}}
\xydef@\PATHlabelbreak@#1#2{%
 \DN@{#1}\ifx\next@\empty \drop\labelbox{#2}\else \drop#1{#2}\fi
 \def\afteraliases@@{\xy@@\Cbreak@@}\xyFN@\PATHlabelalias@}
\xylet@\labelmargin@=\objectmargin@
\xydef@\labelmargin{\afterADDOP{\Addop@@\labelmargin@}}
\xydef@\hole{\hbox{\dimen@=\objectmargin@ \kern2\dimen@
 \vrule height\dimen@ depth\dimen@ width\z@}}
\xylet@\labelstyle=\scriptstyle
\xydef@\labelbox#1{\hbox{$\m@th\labelstyle{#1}$}}
\xydef@\PATHlabelalias@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHlabelalias@}%
 \else \addEQ@\ifx \next
 \addEQ@\DN@"##1"{\savealias@{##1}\xyFN@\PATHlabelalias@}%
 \else \DN@{\afteraliases@@\PATHlabels@}\fi\fi \next@}
\xylet@\afteraliases@@=\empty
\xydef@\savealias@#1{\xy@@{\enter@\cfromthec@
 \advance\X@c-\L@c \advance\L@c\R@c \L@c=.5\L@c \R@c=\L@c \advance\X@c\L@c 
 \advance\Y@c-\D@c \advance\D@c\U@c \D@c=.5\D@c \U@c=\D@c \advance\Y@c\D@c 
 \idfromc@{#1}\leave@}}
\message{\string\ar,}
\xylet@\arvariant@@=\empty
\xylet@\arstemprefix@@=\empty
\xylet@\artail@@=\empty
\xylet@\arstem@@=\empty
\xylet@\arhead@@=\empty
\xylet@\armodifiers@@=\empty
\xylet@\arlabels@@=\empty
\xylet@\arafterPOS@@=\empty
\xylet@\arinit@@=\empty
\xylet@\arexit@@=\empty
\xylet@\arcomponent@@=\relax
\xylet@\arcomponenttype@@=\relax
\xylet@\afterar@@=\relax
\xydef@\ar{\relax\arSAFE}
\xydef@\arSAFE{%
 \let\arvariant@@=\empty
 \def\arstemprefix@@{\dir}%
 \edef\artail@@{\arvariant@@{}}%
 \edef\arstem@@{\arvariant@@{-}}%
 \edef\arhead@@{\arvariant@@{>}}%
 \def\armodifiers@@{}%
 \def\arafterPOS@@{}%
 \def\arlabels@@{}%
 \def\arinit@@{}%
 \def\arexit@@{}%
 \let\PATHlabelabove@@=\PATHlabelabove@
 \let\PATHlabelbelow@@=\PATHlabelbelow@
 \xyFN@\ar@}
\xydef@\ar@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\ar@}%
 \else \addAT@\ifx\next \addAT@\DN@{\xyFN@\ar@form}%
 \else\ifx |\next
 \DN@ |{\ar@anchor|}%
 \else\ifx ^\next
 \DN@ ^{\ar@anchor^}%
 \else\ifx _\next
 \DN@ _{\ar@anchor_}%
 \else \let\next@=\ar@x \fi\fi\fi\fi\fi \next@}
\xydef@\addtoarinit@#1{%
 \expandafter\def\expandafter\arinit@@\expandafter{\arinit@@ #1}}
\xydef@\addtoarlabels@#1{%
 \expandafter\def\expandafter\arlabels@@\expandafter{\arlabels@@ #1}}
\xydef@\ar@anchor#1{\begingroup
 \def\PATHlabelit@@##1##2{%
 \DN@{##1}\ifx\next@\empty
 \DN@####1{\expandafter\endgroup\expandafter\addtoarlabels@
 \expandafter{\the\toks@####1{##2}}\xyFN@\ar@}%
 \else
 \DN@####1{\expandafter\endgroup\expandafter\addtoarlabels@
 \expandafter{\the\toks@*!C####1##1{##2}}\xyFN@\ar@}\fi
 \expandafter\next@\expandafter{\PATHitshape@@}}%
 \toks@={#1}%
 \def\xy@##1##2{\addtotoks@{##1}}\change@oxy@\xy@ \let\xy@@ix@=\eat@
 \DNii@{}\xyFN@\PATHanchor@}
\xydef@\ar@form{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\ar@form}%
 \else\ifx ^\next \DN@ ^{\xyFN@\ar@style}\edef\arvariant@@{\string^}%
 \else\ifx _\next \DN@ _{\xyFN@\ar@style}\edef\arvariant@@{\string_}%
 \else\ifx 0\next \DN@ 0{\xyFN@\ar@style}\def\arvariant@@{0}%
 \else\ifx 1\next \DN@ 1{\xyFN@\ar@style}\def\arvariant@@{1}%
 \else\ifx 2\next \DN@ 2{\xyFN@\ar@style}\def\arvariant@@{2}%
 \else\ifx 3\next \DN@ 3{\xyFN@\ar@style}\def\arvariant@@{3}%
 \else\ifx \bgroup\next \let\next@=\ar@style
 \else\ifx [\next \DN@[##1]{\ar@modifiers{[##1]}}%
 \else\ifx *\next \DN@ *{\ar@modifiers}%
 \else\addLT@\ifx\next \let\next@=\ar@slide
 \else\ifx /\next \let\next@=\ar@curveslash
 \else\ifx (\next \let\next@=\ar@curveinout
 \else\addRQ@\ifx\next \addRQ@\DN@{\ar@curve@}%
 \else\addLQ@\ifx\next \addLQ@\DN@{\xyFN@\ar@curve}%
 \else\addDASH@\ifx\next \addDASH@\DN@{\defarstem@-\xyFN@\ar@}%
 \else\addEQ@\ifx\next \addEQ@\DN@{\def\arvariant@@{2}\defarstem@-\xyFN@\ar@}%
 \else\addDOT@\ifx\next \addDOT@\DN@{\defarstem@.\xyFN@\ar@}%
 \else\ifx :\next \DN@:{\def\arvariant@@{2}\defarstem@.\xyFN@\ar@}%
 \else\ifx ~\next \DN@~{\defarstem@~\xyFN@\ar@}%
 \else\ifx !\next \DN@!{\dasharstem@\xyFN@\ar@}%
 \else\ifx ?\next \DN@?{\ar@upsidedown\xyFN@\ar@}%
 \else \let\next@=\ar@error
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\defarstem@#1{\edef\arstem@@{\arvariant@@{\string#1}}%
 \DNii@##1##{\next@}%
 \edef\next@##1{\def\noexpand\artail@@{\arvariant@@{##1}}}%
 \expandafter\nextii@\artail@@
 \edef\next@##1{\def\noexpand\arhead@@{\arvariant@@{##1}}}%
 \expandafter\nextii@\arhead@@}
\xydef@\dasharstem@{%
 \DN@##1##{\nextii@{##1}}\DNii@##1##2{\def\arstem@@{##1{##2##2}}}%
 \expandafter\next@\arstem@@}
\xydef@\ar@error#1{\xyerror@{Illegal <form>ation (\meaning\next)}{}%
 \xyFN@\ar@}
\xydef@\ar@style{%
 \ifx \bgroup\next \def\artail@@{{}}%
 \edef\arstem@@{\arvariant@@{-}}\edef\arhead@@{\arvariant@@{>}}%
 \expandafter\ar@i
 \else \resetvariant@\artail@@ \resetvariant@\arstem@@ \resetvariant@\arhead@@
 \expandafter\xyFN@\expandafter\ar@ \fi}
\xydef@\resetvariant@#1{%
 \DN@##1##{\DN@{##1}\ifx\next@\empty
 \DN@{\expandafter\nextii@\expandafter{\arvariant@@}}%
 \else \DN@{\nextii@{##1}}\fi \next@}%
 \DNii@##1##2{\def#1{##1{##2}}}%
 \expandafter\next@#1}
\xydef@\ar@i#1{\DN@{#1}%
 \ifx\next@\empty \edef\arstem@@{\arvariant@@{}}\edef\arhead@@{\arvariant@@{}}%
 \DN@{\xyFN@\ar@}%
 \else
 \let\arcomponent@@=\ar@ii \let\arcomponenttype@@=\artip@
 \DN@{\xyFN@\arcomponent@#1$}%
 \fi \next@}
\xydef@\ar@ii{\ifx $\next \let\next@=\ar@iv
 \else \expandafter\def\expandafter\artail@@\expandafter{\the\toks@}%
 \let\arcomponent@@=\ar@iii \let\arcomponenttype@@=\arconn@
 \DN@{\xyFN@\arcomponent@}\fi \next@}
\xydef@\ar@iii{%
 \expandafter\def\expandafter\arstem@@\expandafter{\the\toks@}%
 \resetvariant@\artail@@
 \let\arcomponent@@=\ar@iv \let\arcomponenttype@@=\artip@
 \xyFN@\arcomponent@}
\xydef@\ar@iv{%
 \expandafter\def\expandafter\arhead@@\expandafter{\the\toks@}%
 \ifx $\next \DN@ ${\xyFN@\ar@}%
 \else \xyerror@{illegal <arrow>: \meaning\next\space not valid}{}\fi \next@}
\xydef@\ar@x{%
 \let\arsavedPATHafterPOS@@=\PATHafterPOS \let\PATHafterPOS=\arafterPOS@
 \toks@={\ar@PATH}%
 \expandafter\addtotoks@\expandafter{\expandafter{\artail@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arstem@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arstemprefix@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arhead@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\armodifiers@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arinit@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arexit@@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\arlabels@@}}%
 \addtotoks@{\afterar@@}%
 \expandafter\DNii@\expandafter{\the\toks@}\toks@={}%
 \nextii@}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{%
 \def\next{%
 \afterPATH{#9}%
 ~={#6\preconnect#5#3#2}%
 ~/{#7}%
 ~<{|<*h#5\dir#1}%
 ~>{|>*h#5\dir#4}%
 ~+{#8}%
 }%
 \next}}
\xylet@\ar@PATH=\next
\xydef@\arafterPOS@#1{%
 \arsavedPATHafterPOS@@{\let\PATHafterPOS=\arsavedPATHafterPOS@@
 \DN@{#1}\expandafter\next@\arafterPOS@@}}%
\xylet@\arsavedPATHafterPOS@@=\relax
\xydef@\arcomponent@{%
 \ifx ^\next \toks@ii={^}\DN@ ^{\xyFN@\arcomponent@i}%
 \else\ifx _\next \toks@ii={_}\DN@ _{\xyFN@\arcomponent@i}%
 \else\ifx 1\next \toks@ii={1}\DN@ 1{\xyFN@\arcomponent@i}%
 \else\ifx 2\next \toks@ii={2}\DN@ 2{\xyFN@\arcomponent@i}%
 \else\ifx 3\next \toks@ii={3}\DN@ 3{\xyFN@\arcomponent@i}%
 \else\ifx \bgroup\next \expandafter\toks@ii\expandafter{\arvariant@@}%
 \let\next@=\arcomponent@i
 \else\ifx *\next \DN@*##1##{\arcomponent@ii{##1}}%
 \else \expandafter\toks@ii\expandafter{\arvariant@@}\toks@={}%
 \let\next@=\arcomponenttype@@
 \fi\fi\fi\fi\fi\fi\fi
 \next@}
\xydef@\arcomponent@i#1{\toks@={#1}\arcomponent@x}
\xydef@\arcomponent@ii#1#2{\toks@={*#1{#2}}\xyFN@\arcomponent@@}
\xydef@\artip@{%
 \addGT@\ifx\next \addGT@\addtotoks@ \addGT@\DN@{\xyFN@\artip@}%
 \else\addLT@\ifx\next \addLT@\addtotoks@ \addLT@\DN@{\xyFN@\artip@}%
 \else\ifx (\next \addtotoks@(\DN@({\xyFN@\artip@}%
 \else\ifx )\next \addtotoks@)\DN@){\xyFN@\artip@}%
 \else\ifx |\next \addtotoks@|\DN@|{\xyFN@\artip@}%
 \else\addLQ@\ifx\next \addLQ@\addtotoks@ \addLQ@\DN@{\xyFN@\artip@}%
 \else\addRQ@\ifx\next \addRQ@\addtotoks@ \addRQ@\DN@{\xyFN@\artip@}%
 \else\addPLUS@\ifx \next \addPLUS@\addtotoks@ \addPLUS@\DN@{\xyFN@\artip@}%
 \else\ifx /\next \addtotoks@/\DN@/{\xyFN@\artip@}%
 \else\ifcat A\noexpand\next \DN@##1{\addtotoks@{##1}\xyFN@\artip@}%
 \else\ifx\space@\next \addtotoks@{ }\expandafter\DN@\space{\xyFN@\artip@}%
 \else \let\next@=\arcomponent@x
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\arconn@{%
 \addDASH@\ifx\next \addDASH@\addtotoks@ \addDASH@\DN@{\xyFN@\arconn@}%
 \else\addEQ@\ifx\next \addEQ@\addtotoks@ \addEQ@\DN@{\xyFN@\arconn@}%
 \ifx\arvariant@@\empty \def\arvariant@@{2}\fi
 \else\addDOT@\ifx\next \addDOT@\addtotoks@ \addDOT@\DN@{\xyFN@\arconn@}%
 \else\ifx :\next \addtotoks@:\DN@:{\xyFN@\arconn@}%
 \ifx\arvariant@@\empty \def\arvariant@@{2}\fi
 \else\ifx ~\next \addtotoks@~\DN@~{\xyFN@\arconn@}%
 \else \let\next@=\arcomponent@x
 \fi\fi\fi\fi\fi \next@}
\xydef@\arcomponent@x{%
 \DN@##1{\toks@=\expandafter{\the\toks@ii{##1}}}%
 \expandafter\next@\expandafter{\the\toks@}%
 \xyFN@\arcomponent@@}
\xydef@\ar@curveslash/#1/{\expandafter\ar@curve@\ar@slashing{#1}}
\xydef@\ar@slashing#1{{\xy@{**{} ?+/#1/+/#1/ @+c}{\setupDirection@
 \vfromslide@{#1}%
 \X@c=2\X@c \advance\X@c\X@p \advance\X@c.5\d@X
 \Y@c=2\Y@c \advance\Y@c\Y@p \advance\Y@c.5\d@Y
 \czeroEdge@
 \spushc@}}}
{\xyuncatcodes \catcode`\#=6
 \gdef\next(#1,#2){{+/#1 3pc/,p+/#2 3pc/}}}
\xylet@\ar@curveinout@=\next
\xydef@\ar@curveinout{\expandafter\ar@curve@load\ar@curveinout@}
\xydef@\ar@curve{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\ar@curve}%
 \else\ifx \bgroup\next \let\next@=\ar@curve@load
 \else\ifx "\next \DN@"##1"{\ar@curve@{"##1"}}%
 \else \xyerror@{@= <form> must be followed by \string"<id>\string" or
 {<control point list>}}{}%
 \fi\fi\fi \next@}
{\xyuncatcodes \gdef\next#1#2{\def#1##1{#2{;@={##1}}}}}
\next\ar@curve@load\ar@curve@
\xydef@\ar@curve@#1{\curve@check
 \setcurvearinit@{#1}\setcurvearexit@\arexit@@
 \def\arstemprefix@@{\crvi}\xyFN@\ar@}
{\xyuncatcodes \gdef\next#1{\save @(,#1\restore}}
\xylet@\setcurvearinit@i=\next
\xydef@\setcurvearinit@#1{%
 \expandafter\addtoarinit@\expandafter{\setcurvearinit@i{#1}}}
{\xyuncatcodes \gdef\next#1{\def#1{\POS @i @) }}}
\xylet@\setcurvearexit@=\next
\xydef@\curve@check{%
 \xyerror@{Forms @/.../, @(...), and @`{...}, only available when curve
 extension loaded}{}}
\xywithoption{curve}{\let\curve@check=\relax}
\xydef@\ar@modifiers#1{%
 \expandafter\def\expandafter\armodifiers@@\expandafter{\armodifiers@@#1}%
 \xyFN@\ar@}
{\xyuncatcodes \catcode`\#=6 \catcode`\@=11
 \gdef\next<#1>{\def\arafterPOS@@{<#1>}\xyFN@\ar@}}
\xylet@\ar@slide=\next
\xydef@\ar@upsidedown{\let\next=\PATHlabelabove@@
 \let\PATHlabelabove@@=\PATHlabelbelow@@ \let\PATHlabelbelow@@=\next}
\xyendinput


==> xycmactex.tex <==
%% xycmactex.tex from $Id: xycmactex.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``CMacTeX'' driver interface option.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{cmactex}{CMacTeX driver}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xyrequire{dvips}
\xyendinput


==> xycmtip.tex <==
%% xycmtip.tex from $Id: xycmtip.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Computer Modern tips'' extension.
%% Copyright (c) 1992-1996 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{cmtip}{Computer Modern tip extension}{\stripRCS$Revision: 3.7 $}%
 {Kristoffer H.~Rose}{krisrose@tug.org}%
 {IBM T.~ J.\ Watson Research Center, P.O.~Box 704, Yorktown Heights, NY 10598 (USA)}
\xyrequire{tips}\xycatcodes
\xydef@\UseComputerModernTips{\SelectTips{cm}{10}\UseTips}
\xydef@\NoComputerModernTips{\NoTips}
\xyendinput


==> xycolor.tex <==
%% xycolor.tex from $Id: xycolor.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Colour extension'' option.
%% Copyright (c) 1993-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{color}{Colour extension}{\stripRCS$Revision: 3.11 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\xycolorwarning@@{\xycolormessage@
 \gdef\xycolorwarning@{\xycolormessage@
 \xywarning@{...no further colour warnings will be given.}%
 \global\let\xycolorwarning@=\relax }}
\xylet@\xycolorwarning@=\xycolorwarning@@
\xydef@\xycolormessage@{%
 \xywarning@{Current driver does not support colour.}}%
\xydef@\xyNoColor@#1{}
\xylet@\xycolor@@=\xyNoColor@
\xydef@\xyNoColor@@#1#2{\xycolorwarning@}
\xydef@\xycolor@{\xycolor@@}
\xylet@\xylocalColor@=\xyNoColor@@
\xydef@\UnloadColor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@ }
\xylet@\UnloadColor@@=\UnloadColor@
\xyaddunsupport{color}{\UnloadColor@@\relax}
\ifx\current@color\undefined \xydef@\xybasecolor@{}%
\else \def\xybasecolor@{\current@color}\fi
\xydef@\xystackcolor@{\bgroup \DN@##1##2{\egroup}%
 \ifInvisible@\else\ifHidden@\else\DNii@{\no@@}\ifx\nextii@\Connect@@ 
 \else\DN@{\xystackcolor@i}\fi\fi\fi \next@ } 
\xydef@\xystackcolor@i#1#2{\checkXyStyle@ 
 \DN@{#2}\ifx\next@\empty
 \def\tmp@##1{\DN@{\xycolor@push{#1}##1\xycolor@pop}}%
 \else\def\tmp@##1{\DN@{\xycolor@push{#2 #1}##1\xycolor@pop}}\fi
 \toks@={\egroup \let\xy@style@=\relax \def\Drop@@}%
 \expandafter\tmp@\expandafter{\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}\def\Connect@@}%
 \expandafter\tmp@\expandafter{\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}}%
 \the\toks@ }%
\xydef@\xycolor@push@@#1{\special{color push #1}}
\xydef@\xycolor@pop{\special{color pop}}
\xylet@\xycolor@push=\xycolor@push@@
\xydef@\newxycolor#1#2{\newxyColor{#1}{}{}{#2}{}}
\xydef@\newxyColor#1#2#3#4{\newxycolor@{#1}{#2}{#3}{#4}{}}
\xydef@\newxycolor@#1#2#3#4#5{%
 \expandafter\let\expandafter\next@\csname shape [#1]\endcsname
 \ifx\next@\relax
 \DN@{#4}\ifx\next@\empty
 \DN@{#2}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalColor@{}{#3}\xycolor@{#3}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalColor@{#2}{#3}\xycolor@{#2 #3}}}%
 \fi
 \else\DN@{#2#3}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalColor@{#4}{}\xycolor@{#4}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalColor@{#2}{#3}\xycolor@{#4}}}%
 \fi \fi 
 \else \def\tmp@{\relax}\DNii@{#5}%
 \ifx\nextii@\tmp@
 \DN@{#4}\ifx\next@\empty
 \DN@{#2}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalColor@{}{#3}\xycolor@{#3}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalColor@{#2}{#3}\xycolor@{#2 #3}}}%
 \fi
 \else
 \DN@{#2#3}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalColor@{#4}{}\xycolor@{#4}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalColor@{#2}{#3}\xycolor@{#4}}}%
 \fi \fi 
 \else\DN@{}\fi\fi \next@\relax}
\xydef@\xystandardcolors@{%
 \newxycolor@{black}{0. 0. 0.}{rgb}{}\relax
 \newxycolor@{white}{1. 1. 1.}{rgb}{}\relax
 \newxycolor@{gray}{.5}{gray}{}\relax
 \newxycolor@{grey}{.5}{gray}{}\relax
 \newxycolor@{red}{1. 0. 0.}{rgb}{}\relax
 \newxycolor@{green}{0. 1. 0.}{rgb}{}\relax
 \newxycolor@{blue}{0. 0. 1.}{rgb}{}\relax
 \newxycolor@{cyan}{0. 1. 1.}{rgb}{}\relax
 \newxycolor@{magenta}{1. 0. 1.}{rgb}{}\relax
 \newxycolor@{yellow}{1. 1. 0.}{rgb}{}\relax
 \xyuncatcodes }
\xydef@\UseCrayolaColors{\xyrequire{crayon}\xyuncatcodes}%
\xydef@\xyBEcolorcheck@{\ifx\xycolor@@\xyNoColor@\else
 \xywarning@{PostScript colour support should be OK.}\fi }%
\xywithoption{ps}{%
 \xyinputorelse@{xyps-c}{\xyerror@{Could not load xyps-c}{}}}%
 \xycatcodes
\xyendinput


==> xycrayon.tex <==
%% xycrayon.tex from $Id: xycrayon.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Crayola colours'' PostScript backend support.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{crayon}{Crayola Colours}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\installCrayolaColors@{%
 \xyinputorelse@{xyps-col}{\xyerror@{Could not load Crayola colours}{}}%
 \let\installCrayolaColors@=\relax
 \xyuncatcodes }
\xyendinput
#


==> xycurve.tex <==
%% xycurve.tex from $Id: xycurve.doc,v 3.12 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Curves and Splines'' extension.
%% Copyright (c) 1993-1997 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{curve}{Curve and Spline extension}{\stripRCS$Revision: 3.12 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\message{curve,}
\xynew@{count}\crv@cnt@
\xydef@\xynumctrlpts@{\the\crv@cnt@}
\xynew@{toks}\crvpts@
\xydef@\setcurve@{%
 \edef\xysplineparams@{%
 \expandafter\noexpand\csname params@\endcsname}%
 \edef\xysplineedges@{%
 \expandafter\noexpand\csname edges@\endcsname}%
 \edef\xycrvcnt@{%
 \expandafter\noexpand\csname crvcnt@\endcsname}%
 \expandafter\edef\xycrvcnt@{\number\crv@cnt@}%
 \ifcase\crv@cnt@
 \expandafter\xycvxhull@\or
 \expandafter\xyquadbezier@\or
 \expandafter\xycubicbezier@\or
 \expandafter\xybspline@iii\or
 \expandafter\xybspline@iv\else
 \expandafter\xybspline@
 \fi}
\xydef@\curve{\connect\crv}
\xydef@\crv#1#{\hbox \bgroup \crvresetbreaks@ \initshape@
 \def\pure@crv{\crv@saveStyles@}\crv@{#1}}
\xydef@\crv@#1#2{%
 \DN@{#1}\ifx\empty\next@
 \DN@{\def\afterCURVEaction@{}\parsecurve@\xycurve@@}%
 \else\DN@{\parseCURVE@#1\parsecurve@\curveSTYLE@}\fi
 \next@ #2\@endcurve\endcrv@ }
\xydef@\curveSTYLE@{\xycurve@@}%
\xydef@\afterCURVEaction@{}%
\xydef@\@endcurve{}%
\xydef@\endcrv@@{\endcrv@\POS}%
\xydef@\pure@crv{\relax}
\xywarnifdefined\crv@normaltemplate
\xywarnifdefined\crv@othertemplate
\xywarnifdefined\crv@specialtemplate@@
{\xyuncatcodes \catcode`\@=11 \catcode`\#=6
 \gdef\crv@normaltemplate#1{{}{~**#1\xy@@crvaddstack@}}
 \gdef\crv@othertemplate#1{{}{~*=<2\jot>{}~**#1\xy@@crvaddstack@}}
 \gdef\crv@specialtemplate@@#1{{}{~**\dir{#1}\xy@@crvaddstack@}}
}
\xydef@\crvs#1#{\hbox \bgroup \def\pure@crv{\relax}\crvs@{#1}}%
\xydef@\crvi#1#{\hbox \bgroup \def\pure@crv{\relax}\invisbreaks@ \crvs@{#1}}%
\xydef@\crvs@#1{\DN@{\initshape@ \@crv@{#1}}%
 \def\crv@defaultshape{-}%
 \ifx\bstartPLACE@\relax \else
 \ifx\bstartPLACE@\empty \Invisible@true \else
\splinetrace@{bstartPLACE@=\bstartPLACE@, bendPLACE@=\bendPLACE@}%
 \DN@{\let\xy@@crvaddstack@=\xy@@samecurve@
 \let\saveshape@=\savesame@ 
 \let\savectrlptsnum@=\relax
 \let\startxycurve@=\recovercurve@ 
 \crv@cnt@=\xycrvptsnum@\relax \@crv@{#1}}%
 \fi \fi \next@ }
\xydef@\xy@@samecurve@{\xyFN@\checkendcurve@}
\xydef@\savesame@{\egroup }
\xydef@\recovercurve@{%
 \crv@cnt@=\xycrvptsnum@ \splinereset@ \recovercv@end
 \ifx\bendPLACE@\relax \def\bendPLACE@{1}\fi
 \ifdim\zz@\R@c \ifdim\zz@\L@c \ifdim\zz@\D@c \ifdim\zz@\U@c
 \Edge@c={\zeroEdge}\fi\fi\fi\fi
 \edef\cv@end{\cfromthec@}\edef\cv@start{\cfromthep@}}
\xydef@\recovercv@end{\count@=\ptsnum@\relax\advance\count@\@ne
 \edef\tmp@{\the\count@}\csname cv@\tmp@\endcsname}%
\xydef@\crvSTYLE@@{}
\expandafter\xydef@\expandafter\crv@defaultshape\expandafter{\addDASH@{}}
\xydef@\crv@noobject{\Invisible@true}
\xydef@\@crv@#1#2{\DN@{#1#2}%
 \ifx\next@\empty \edef\next@{\crv@defaultshape}%
 \ifx\bstartPLACE@\empty \xdef\crvSTYLE@@{{\crv@defaultshape}}\fi
 \else 
 \ifx\bstartPLACE@\empty \gdef\crvSTYLE@@{#1{#2}}\fi
 \fi
 \ifx\next@\empty \crv@noobject \DN@{\crv@{}{\xy@@crvaddstack@}}%
 \else\def\tmp@{-}\ifx\next@\tmp@ \DN@{\crv@{}{\xy@@crvaddstack@}}%
 \else\def\tmp@{=}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir{=}}}%
 \else\def\tmp@{2-}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir{2.}}}%
 \else\def\tmp@{3-}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir{3.}}}%
 \else\def\tmp@{--}\ifx\next@\tmp@
 \DN@{\expandafter\crv@\crv@specialtemplate@{--}}%
 \else\def\tmp@{==}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir2{--}}}%
 \else\def\tmp@{2--}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir2{--}}}%
 \else\def\tmp@{3--}\ifx\next@\tmp@ 
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir3{--}}}%
 \else\def\tmp@{.}\ifx\next@\tmp@
 \DN@{\expandafter\crv@\crv@specialtemplate@{.}}%
 \else\def\tmp@{:}\ifx\next@\tmp@
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir{:}}}%
 \else\def\tmp@{2.}\ifx\next@\tmp@
 \DN@{\expandafter\crv@\crv@normaltemplate{\dir{:}}}%
 \else\def\tmp@{..}\ifx\next@\tmp@
 \DN@{\expandafter\crv@\crv@specialtemplate@{.}}%
 \else
 \DN@{\expandafter\crv@\crv@othertemplate{\dir#1{#2}}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xylet@\crv@specialtemplate@=\crv@specialtemplate@@
\xydef@\crv@special#1{}
\xydef@\parseCURVE@{\def\curveSTYLE@{\xycurve@@}\def\afterCURVEaction@{}%
 \xyFN@\parseCURVE@@}
\xydef@\parseCURVE@@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\parseCURVE@@}%
 \else\ifx ~\next \DN@ ~{\xy@~{}\xyFN@\setcurveSTYLE@@}%
 \else\ifx\parsecurve@\next\DN@{}%
 \else\ifcat\active\noexpand\next\DN@{\xyactive@Warning}%
 \else\ifcat a\noexpand\next\DN@##1{\xytilde@Warning\setcurveSTYLE@{##1}%
 \xyFN@\parseCURVE@@}%
 \else\DN@{}\fi\fi\fi\fi\fi \next@ }%
\xydef@\xyactive@Warning{\xywarning@{expandable control sequences should 
 not be here, results are unpredictable in diagrams.}}%
\xydef@\xytilde@Warning{Please use ~ to set curve style.}%
\xydef@\setcurveSTYLE@#1{\xyFN@\setcurveSTYLE@@#1}
\xydef@\setcurveSTYLE@@{%
 \ifx\next p\def\curveSTYLE@{\xyc@trlpts@@}%
 \DN@ p{\xyFN@\setafterCURVEaction@}%
 \else\ifx\next P\def\curveSTYLE@{\xyc@trlpts@}%
 \DN@ P{\xyFN@\setafterCURVEaction@}%
 \else\ifx\next l\def\curveSTYLE@{\xyc@vxhull@@}%
 \DN@ l{\xyFN@\setafterCURVEaction@}%
 \else\ifx\next L\def\curveSTYLE@{\xyc@vxhull@}%
 \DN@ L{\xyFN@\setafterCURVEaction@}%
 \else\ifx\next c\def\curveSTYLE@{\xycurve@@}%
 \DN@ c{\xyFN@\setafterCURVEaction@}%
 \else\ifx\next C\def\curveSTYLE@{\xycurve@@}%
 \DN@ C{\xyFN@\setafterCURVEaction@}%
 \else \DN@##1{\xywarning@{unknown curve style ##1}\xyFN@\parseCURVE@@}%
 \fi\fi\fi\fi\fi\fi \next@ }
\xydef@\setafterCURVEaction@{%
 \ifx\next~\DN@~{\xyFN@\setcurveSTYLE@@}%
 \else\ifcat a\noexpand\next\DN@{\setafterCURVEaction@@}%
 \else\DN@{\xyFN@\parseCURVE@@}%
 \fi\fi \next@}
\xydef@\setafterCURVEaction@@{%
 \ifx\next c\DN@ c{%
 \def\afterCURVEaction@{\noexpand\endcurve\noexpand\xy@curve@}%
 \xyFN@\parseCURVE@@ }%
 \else\ifx\next C\DN@ C{%
 \def\afterCURVEaction@{\noexpand\endcurve\noexpand\xy@curve@@}%
 \xyFN@\parseCURVE@@ }%
 \else \DN@##1{\xywarning@{unknown after-curve action ##1}%
 \xyFN@\parseCURVE@@ }%
 \fi\fi \next@ }
\xydef@\parsecurve@{\xyFN@\parsecurve@@}
\xydef@\parsecurve@@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\parsecurve@@}%
 \else\ifx\next\@endcurve\DN@\@endcurve{\checkafterCURVE@}%
 \else\ifcat\active\noexpand\next\DN@{\relax}%
 \else\DN@{\xycurve@@}\fi\fi\fi\next@}%
\xydef@\xycurve@{\begingroup\afterCURVE{\setcurve@\endgroup}\crvobjects@
 \startxycurve@\xycrvmods@}
\xydef@\xycurve@@{\afterCURVE{\setcurve@}\crvobjects@\startxycurve@
 \xycrvmods@}
\xydef@\xy@curve@{\xy@curve@@@{\splinedefaulttol@\crvobjects@}}
\xydef@\xy@curve@@{\xy@curve@@@{\resetcrvobjects@}}
\xydef@\xy@curve@@@#1{\ifx\cv@start\relax
 \DN@{\xywarning@{There is no curve to plot}}.
 \else\DN@{\begingroup\afterCURVE{\setcurve@\endgroup}#1\cv@end}%
 \fi \next@ }
\xydef@\crvobjects@{\def\xycrvdrop@{}\def\xycrvconn@{}}
\xydef@\resetcrvobjects@{\crvobjects@}
\xylet@\savecurve=\xycurve@@
\xylet@\samecurve=\xy@curve@
\xydef@\xycrvmods@{\xyFN@\xy@crvmods@}%
\xydef@\xy@crvmods@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\xy@crvmods@}%
 \else\ifx\next ~\DN@ ~{\xyFN@\xy@crvmods@@}%
 \else\DN@{\xy@crvmods@@@@}\fi\fi \next@}%
\xydef@\xy@crvmods@@@@{\xyFN@\checkendcurve@}%
\xydef@\xy@crvmods@@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\xy@crvmods@@}%
 \else\ifx\next *\DN@ *{\xyFN@\xy@@crvmods@}%
 \else\addAT@\ifx\next\addAT@\DN@{\xyFN@\xy@@crvaddstack}%
 \else\DN@{\xywarning@{badly-formed curve option}\xyFN@\xy@crvmods@}%
 \fi\fi\fi \next@}%
\xydef@\xy@@crvmods@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\xy@@crvmods@}%
 \else\ifx\next *\DN@ *{\xyFN@\xy@@crvmods@@}%
 \else\DN@{\xy@crv@mods@@}\fi\fi \next@}%
\xydef@\xy@crv@mods@@#1#{\DN@##1{\xy@crvmods@@@{#1}{##1}}\next@}%
\xydef@\xy@crvmods@@@#1#2{%
 \DN@{#1#2}\ifx\next@\empty \def\xycrvdrop@{ #1{\zerodot}}%
 \else \def\xycrvdrop@{ #1{#2}}\fi
 \xyFN@\xy@crvmods@ }%
\xydef@\xy@@crvmods@@#1#{\DN@##1{\xy@@crvmods@@@{#1}{##1}}\next@}%
\xydef@\xy@@crvmods@@@#1#2{\def\xycrvconn@{ #1{#2}}\xyFN@\xy@crvmods@ }%
\xydef@\checkendcurve@{%
 \ifx\space@\next\expandafter\DN@\space{\xyFN@\checkendcurve@}%
 \else\ifx\next\endcurve\DN@\endcurve{\clearsearchflag@\endxycurve@}%
 \else\ifx\next\@endcurve\DN@\@endcurve{\checkafterCURVE@}%
 \else\ifx\next\xy@@crvaddstack@\DN@{}%
 \else\ifx\next\endxy\DN@{\clearsearchflag@\sloppyendcrv@}%
 \else\testAND@\iffalse \DN@##1{\clearsearchflag@\searchnextpt@}%
 \else\ifx ~\next\DN@ ~{\xyFN@\checkcrvtilde@}%
 \else\ifx\next\relax\DN@\relax{\clearsearchflag@\searchnextpt@}%
 \else\ifx\next\\\DN@\\{\clearsearchflag@\searchnextpt@}%
 \else\ifx\searchflag@\relax
 \DN@{\setsearchflag@\searchnextpt@}%
 \else\DN@##1{\flagwarn@{##1}}\fi
 \fi\fi\fi\fi\fi\fi\fi\fi\fi \next@ }
\xydef@\searchnextpt@{\afterPOS{\xy@@\addtocrv@ \xyFN@\checkendcurve@}}
\xydef@\checkafterCURVE@{%
 \edef\tmp@{\noexpand\xyFN@\noexpand\checkendcurve@
 \afterCURVEaction@\noexpand\endcurve}\tmp@ }
\xylet@\searchflag@=\relax
\xydef@\setsearchflag@{\let\searchflag@=@}
\xydef@\clearsearchflag@{\let\searchflag@=\relax}
\xydef@\flagwarn@#1{%
 \ifx\next\@endcurve\DN@{\xyFN@\checkendcurve@\endcurve}%
 \else\setsearchflag@\DN@{\xyFN@\checkendcurve@}%
 \xywarning@{skipping invalid token \string#1\space in curve}%
 \fi \next@ }
\xydef@\sloppyendcrv@{%
\xywarning@{Please use \string\endcurve\space to end the curve.}\endxycurve@}
\xydef@\endcrv@{\saveshape@
 \Edge@c={\splineEdge}\Invisible@false\Hidden@false
 \edef\Drop@@{\noexpand\ifInvisible@ \setbox\z@=\copy\voidb@x
 \noexpand\else
 \noexpand\wdz@=\z@
 \noexpand\ht\z@=\z@ \noexpand\dp\z@=\z@
 \noexpand\splineDrop@
 \noexpand\fi }%
 \edef\Connect@@{%
 \noexpand\setbox\z@=\noexpand\box\lastobjectbox@
 \noexpand\wdz@=\z@
 \noexpand\ht\z@=\z@ \noexpand\dp\z@=\z@
 \expandafter\noexpand\pure@crv
 \noexpand\ifInvisible@ \noexpand\crv@saveStyles@ \noexpand\else 
 \noexpand\crv@getStyles@\noexpand\styledboxz@ \noexpand\fi
 \noexpand\ifHidden@\noexpand\else 
 \noexpand\ifx\noexpand\COORD@\noexpand\xymatrixCOORD@ \noexpand\else
 \noexpand\X@min=\the\X@min \noexpand\X@max=\the\X@max 
 \noexpand\Y@min=\the\Y@min \noexpand\Y@max=\the\Y@max
 \noexpand\fi \noexpand\fi
 \savecrvparams@ \noexpand\crvconnect@
 }%
 \wdz@=\z@
 \ht\z@=\z@ \dp\z@=\z@ }
\xydef@\crvXY@pre@{}
\xydef@\crvXY@post@{}
\xydef@\crv@saveStyles@{\def\xy@style@{}%
 \expandafter\def\expandafter\crvXY@pre@\expandafter{\preXY@style@}%
 \expandafter\def\expandafter\crvXY@post@\expandafter{\postXY@style@}}
\xydef@\crv@getStyles@{\def\xy@style@{}%
 \gdef\preXY@style@{\crvXY@pre@}\gdef\postXY@style@{\crvXY@post@}}
\xydef@\initshape@{\savescope@ 
 \ifdim\X@c>\X@p \X@min=\X@p \X@max=\X@c \else \X@max=\X@p \X@min=\X@c \fi
 \ifdim\Y@c>\Y@p \Y@min=\Y@p \Y@max=\Y@c \else \Y@max=\Y@p \Y@min=\Y@c \fi }
\xydef@\saveshape@{\savectrlptsnum@ 
 \R@c=\X@max \advance\R@c-\X@c \L@c=\X@c \advance\L@c-\X@min
 \U@c=\Y@max \advance\U@c-\Y@c \D@c=\Y@c \advance\D@c-\Y@min
 \edef\tmp@{\egroup \U@c=\the\U@c \D@c=\the\D@c \L@c=\the\L@c \R@c=\the\R@c
 \noexpand\ifdim\noexpand\X@min>\the\X@min\noexpand\X@min=\the\X@min\noexpand\fi
 \noexpand\ifdim\noexpand\Y@min>\the\Y@min\noexpand\Y@min=\the\Y@min\noexpand\fi
 \noexpand\ifdim\noexpand\X@max<\the\X@max\noexpand\X@max=\the\X@max\noexpand\fi
 \noexpand\ifdim\noexpand\Y@max<\the\Y@max\noexpand\Y@max=\the\Y@max\noexpand\fi
 \savecrvparams@ \def\noexpand\pure@crv{\expandafter\noexpand\pure@crv}}%
 \tmp@ }
\xydef@\savecrvparams@{\crvpts@={\the\crvpts@}%
 \noexpand\def\noexpand\crvconnect@{\expandafter\noexpand\crvconnect@}}%
\xydef@\splineEdge{\rectangleEdge}
\xydef@\xy@@crvaddstack{%
 \ifx\next ~\xywarning@{there should be a poslist here, \string~@ ignored}%
 \DN@{\xy@crvmods@}%
 \else\DN@{\xy@@crvaddstack@}\fi \next@}
\xydef@\xy@@crvaddstack@{\smapxy@@\addtocrv@ \xyFN@\checkendcurve@}
\xydef@\checkcrvtilde@{%
 \addAT@\ifx\next\addAT@\DN@{\xy@@crvaddstack@}%
 \else\xywarning@{invalid token after ~, ignored}%
 \DN@##1{\xyFN@\checkendcurve@}%
 \fi \next@ }
\xydef@\crvconnect@@{%
 \def\Creset@@{\crvreset@}%
 \def\Cshavep@@{\crvshavep@}%
 \def\Cshavec@@{\crvshavec@}%
 \def\Cslidep@@{\crvslidep@}%
 \def\Cslidec@@{\crvslidec@}%
 \def\Calong@@{\crvalong@}%
 \def\Cintercept@@{\crvintercept@}%
 \def\Cbreak@@{\crvbreak@}%
 \def\Clast@@{\crvlast@}%
}
\xydef@\straitconnect@{\crvconnect@@ 
 \let\crvreset@=\straitreset@
 \let\crvshavep@=\straitshavep@
 \let\crvshavec@=\straitshavec@
 \let\crvslidep@=\straitslidep@
 \let\crvslidec@=\straitslidec@
 \let\crvalong@=\straitalong@
 \let\crvintercept@=\straitintercept@
 \let\crvbreak@=\straitbreak@
 \let\crvlast@=\straitlast@
}
\xydef@\straitreset@{\the\crvpts@ 
 \edef\xycrvptsnum@{\csname ptsnum@\endcsname}%
 \def\segmentnum@{0}}
\xydef@\straitslidep@{\setupDirection@ii \noCslidep@@ }
\xydef@\straitslidec@{\setupDirection@ii \noCslidec@@ }
\xydef@\straitshavep@{%
 \expandafter\ifnum\xycrvptsnum@>\z@
 \def\segmentnum@{0}%
 \csname cv@1\endcsname 
 \resetDirection@ \setupDirection@ii 
 \fi \noCshavep@@ }
\xydef@\straitshavec@{%
 \expandafter\ifnum\xycrvptsnum@>\z@
 \expandafter\count@@\xycrvptsnum@\relax 
 \bgroup \csname cv@\number\count@@\endcsname 
 \edef\tmp@{\egroup \X@p=\the\X@c \Y@p=\the\Y@c}\tmp@ 
 \edef\segmentnum@{\xycrvptsnum@}%
 \resetDirection@ \setupDirection@ii 
 \fi \noCshavec@@ }
\xydef@\straitalong@#1{%
 \ifdim#1\p@<\z@ 
 \xywarning@{parameter value #1 is negative, using 0}%
 \cfromp@ \def\PLACEf@{{0}}%
 \else 
 \dimen@=#1\p@ \count@=\dimen@ \divide\count@\p@ 
 \expandafter\count@@\xycrvptsnum@\relax \advance\count@@\@ne
 \advance\dimen@\segmentnum@\p@ 
 \advance\count@\segmentnum@\relax 
 \def\segmentnum@{0}%
 \ifnum\count@@<\count@
 \xywarning@{parameter value #1 too large, using \the\count@@}%
 \count@=\count@@ \advance\count@\m@ne \edef\PLACEf@{{1}}%
 \else
 \advance\dimen@-\count@\p@ 
 \ifdim\zz@\dimen@\ifnum\count@>\z@
 \advance\count@\m@ne \advance\dimen@\p@ \fi\fi
 \edef\PLACEf@{{\expandafter\removePT@\the\dimen@}}%
 \fi
 \ifnum\count@=\z@\else \bgroup
 \csname cv@\number\count@\endcsname 
 \edef\tmp@{\egroup \X@p=\the\X@c \Y@p=\the\Y@c}\tmp@
 \fi
 \advance\count@\@ne
 \ifnum\count@<\count@@
\splinetrace@{find place \the\dimen@\space along straight segment 
 \the\count@}%
 \csname cv@\number\count@\endcsname
 \fi
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p 
 \fi \expandafter\noCalong@@\PLACEf@ \czeroEdge@ }
\xydef@\straitintercept@{\noCintercept@@}
\xydef@\straitbreak@{\straightCbreak@@}
\xydef@\straitlast@{\straightClast@@}
\xydef@\splineconnect@{%
 \let\crvreset@=\splinereset@
 \let\crvshavep@=\splineshavep@
 \let\crvshavec@=\splineshavec@
 \let\crvslidep@=\splineslidep@
 \let\crvslidec@=\splineslidec@
 \let\crvalong@=\splinealong@
 \let\crvintercept@=\splineintercept@
 \let\crvbreak@=\splinebreak@
 \let\crvlast@=\splinelast@
}
\xydef@\splinereset@{\the\crvpts@ 
 \edef\xycrvptsnum@{\csname ptsnum@\endcsname}%
 \edef\xysplineparams@{%
 \expandafter\noexpand\csname params@\endcsname}%
 \edef\xysplineedges@{%
 \expandafter\noexpand\csname edges@\endcsname}%
 \def\segmentnum@{1}\def\splinecorrect@p{0}\def\splinecorrect@c{0}%
 \splinelength@=\z@ \def\splineplace@f{.5}%
}
\xydef@\splineshavep@{\begingroup 
 \edef\xysplineedges@{%
 \expandafter\noexpand\csname edges@\endcsname}%
 \expandafter\expandafter\expandafter\getsplineedges@safe\xysplineedges@ @@%
 \edef\tmp@{\noexpand\removePT@\the\dimen5}%
 \edef\tmp@{\endgroup 
 \noexpand\def\noexpand\splinecorrect@p{\tmp@}}\tmp@ 
 \setupDirection@ii }
\xydef@\splineshavec@{\begingroup 
 \edef\xysplineedges@{%
 \expandafter\noexpand\csname edges@\endcsname}%
 \expandafter\expandafter\expandafter\getsplineedges@safe\xysplineedges@ @@%
 \dimen@=-\dimen7\relax \advance\dimen@\p@
%% \getcrvsegsnum@ \advance\dimen@\count@\p@
 \edef\tmp@{\noexpand\removePT@\the\dimen@}%
 \edef\tmp@{\endgroup 
 \noexpand\def\noexpand\splinecorrect@c{\tmp@}}\tmp@ 
 \setupDirection@ii }
\xydef@\splineslidep@#1{\enter@{\pfromthep@}%
 \begingroup \splinealong@@{0}{#1}+\splineslidep@@@
 \setupDirection@ii \leave@ }%
\xydef@\splineslidep@@@{%
 \d@X=\dimen5 \d@Y=\dimen7 \edef\tmp@{\postfind@}\tmp@ \dimen@=\splineval@
 \expandafter\count@\xycrvptsnum@\relax
 \ifnum\count@>\tw@ \advance\count@\m@ne 
 \advance\dimen@\segmentnum@\p@ \advance\dimen@-\p@ 
 \fi 
 \edef\tmp@{\endgroup \endgroup
 \noexpand\def\noexpand\xysplineval@{\the\splineval@}%
 \noexpand\def\noexpand\splinecorrect@p{\expandafter\removePT@\the\dimen@}%
\splinetrace@{slide = \the\splinelength@}%
 \X@c=\dimen@i \Y@c=\dimen3
 \d@X=\the\d@X \d@Y=\the\d@Y
 \noexpand\def\noexpand\segmentnum@{\segmentnum@}}\tmp@ }
\xydef@\splineslidec@#1{\enter@{\pfromthep@}%
 \begingroup
 \expandafter\splinealong@@\PLACEf@{#1}+\splineslidec@@@
 \setupDirection@ii \leave@ }
\xydef@\splineslidec@@@{%
 \d@X=\dimen5 \d@Y=\dimen7 \edef\tmp@{\postfind@}\tmp@ \dimen@=\splineval@
 \expandafter\count@\xycrvptsnum@\relax
 \ifnum\count@>\tw@ \advance\count@\m@ne 
 \advance\dimen@\segmentnum@\p@ \advance\dimen@-\p@ 
 \dimen@=-\dimen@ \advance\dimen@\count@\p@
 \else \dimen@=-\dimen@ \advance\dimen@\p@ \fi
%% splinecorrect@c is probably wrong here!!
 \edef\tmp@{\endgroup \endgroup
 \noexpand\def\noexpand\xysplineval@{\the\splineval@}%
 \noexpand\def\noexpand\splinecorrect@c{\expandafter\removePT@\the\dimen@}%
\splinetrace@{slide = \the\splinelength@; correct@c=\noexpand\splinecorrect@c}%
 \X@c=\dimen@i \Y@c=\dimen3
 \d@X=\the\d@X \d@Y=\the\d@Y
 \noexpand\def\noexpand\segmentnum@{\segmentnum@}}\tmp@ }
\xydef@\checkslidemore@#1{%
 \dimen@ii=-#1\relax\ifdim\dimen@ii<\z@\multiply\dimen@ii\m@ne\fi
 \dimen@=-\splinelength@ \advance\dimen@\dimen@ii\relax 
 \ifdim\dimen@<\z@\dimen@ii=-\dimen@\else\dimen@ii=\dimen@\fi
 \ifdim\dimen@ii<.2\p@\DN@{\splineslidec@@ \leave@}%
 \else \splinetrace@{not found yet, \the\dimen@ii\space still to go}%
 \dimen@ii=#1\relax\ifdim\dimen@ii<\z@\multiply\dimen@\m@ne\fi
 \DN@{\expandafter\splineslidemore@\expandafter{\the\dimen@}}\fi 
 \next@}%
\xydef@\splineslidemore@#1{%
 \expandafter\count@\segmentnum@\relax
 \ifdim#1<\z@\advance\count@\m@ne\dimen@=\p@
 \else\advance\count@\@ne\dimen@=\z@\fi
 \ifnum\count@<\@ne
 \expandafter\splinesegment@\expandafter{\segmentnum@}%
 \DN@{\xywarning@{cannot slide beyond start of curve}%
 \spline@find{\z@}{\z@}{}\splineslidec@@ \leave@ }%
 \else \expandafter\count@@\xycrvptsnum@\relax\advance\count@@\m@ne
 \expandafter\ifnum\count@@<\count@\relax
 \expandafter\splinesegment@\expandafter{\segmentnum@}%
 \DN@{\xywarning@{cannot slide beyond end of curve}%
 \spline@find{\p@}{\z@}{}\splineslidec@@ \leave@ }%
 \else
 \edef\segmentnum@{\the\count@}%
 \expandafter\splinesegment@\expandafter{\segmentnum@}%
\splinetrace@{sliding onto segment \segmentnum@}%
 \expandafter\spline@find\expandafter{\the\dimen@}{#1}{}%
 \DN@{\checkslidemore@{#1}}%
 \fi\fi \next@ }
\xydef@\splineslidec@@{%
 \dimen@=\splineval@ \advance\dimen@\segmentnum@\p@\advance\dimen@-\p@ 
 \edef\tmp@{\endgroup 
 \noexpand\def\noexpand\xysplineval@{\the\dimen@}%
\splinetrace@{slide = \the\splinelength@}%
 \X@c=\the\dimen@i \Y@c=\the\dimen3 \d@X=\the\dimen5 \d@Y=\the\dimen7 \postfind@ 
 \noexpand\def\noexpand\segmentnum@{\segmentnum@}}\tmp@
 \setupDirection@ii}
\xydef@\splinealong@#1{\def\postfind@{}\splinealong@@{#1}\z@+%
 \splineslidec@@ 
 \dimen@=\xysplineval@\relax 
 \count@=\xycrvptsnum@\relax \ifnum\count@>\@ne \advance\count@\m@ne\fi
 \ifnum\count@>\@ne \dimen@nth\count@\dimen@
 \fi \edef\bthisPLACE@{\expandafter\removePT@\the\dimen@}%
\splinetrace@{bthisPLACE@=\bthisPLACE@}}%
\xydef@\splinealong@@#1#2#3{%
 \edef\tmp@{#1}\relax \dimen@ii\tmp@\p@ 
%% \getcrvsegsnum@
%% \dimen@=-\count@\p@ 
 \dimen@=-\p@
 \expandafter\advance\expandafter\dimen@\splinecorrect@p\p@
 \expandafter\advance\expandafter\dimen@\splinecorrect@c\p@
 \edef\tmp@{#1}\relax \dimen@=-\tmp@\dimen@ \relax
 \expandafter\advance\expandafter\dimen@\splinecorrect@p\p@
 \getcrvsegsnum@ \multiply \dimen@ by\count@\relax
\splinetrace@{actual:\the\dimen@; f:\the\dimen@ii; p:\splinecorrect@p, c:\splinecorrect@c}%
 \count@=\dimen@ \divide\count@\p@ \DN@{\relax}%
 \def\tmp@{\relax}\ifx\next@\tmp@
 \expandafter\ifnum\xycrvptsnum@<\count@
 \xywarning@{parameter value #1 too large}%
 \DNii@{\relax}\DN@{\begingroup}%
 \else
 \edef\xysplineval@{\the\dimen@}%
 \advance\dimen@-\count@\p@ 
 \ifdim\dimen@=\z@ 
\splinetrace@{find knot point \the\count@}%
 \ifnum\count@=\z@ \count@=\@ne \else \dimen@=\p@ \fi
 \else \advance\count@\@ne
\splinetrace@{find point \the\dimen@\space on spline segment \the\count@}%
 \fi 
 \edef\segmentnum@{\the\count@}%
 \edef\next@{\begingroup\noexpand\splinesegment@{\the\count@}}%
 \edef\nextii@{%
 \noexpand\spline@find{\the\dimen@}{#2}{}\noexpand\checksplinefind@{#2}}%
 \ifx>#3\relax 
 \edef\nextii@{%
 \noexpand\spline@find{\the\dimen@}{#2}#3\noexpand\checksplinefind@{#2}}%
 \else\ifx-#3\relax \ifdim\dimen@>\z@\relax \ifdim\dimen@<\p@
 \dimen@=-\dimen@ \advance\dimen@\p@
 \edef\nextii@{\noexpand\splinereverse@ 
 \noexpand\spline@find{\the\dimen@}{#2}{}\noexpand\checksplinefind@{#2}}%
 \fi\fi
 \else\ifx<#3\relax \ifdim\dimen@>\z@\relax \ifdim\dimen@<\p@
 \dimen@=-\dimen@ \advance\dimen@\p@
 \edef\nextii@{\noexpand\splinereverse@ 
 \noexpand\spline@find{\the\dimen@}{#2}#3\noexpand\checksplinefind@{#2}}%
 \fi\fi
 \fi\fi\fi
 \fi\fi \expandafter\next@\nextii@ }
\xydef@\checksplinefind@#1{%
 \dimen@ii=#1\relax \dimen@=\splinelength@
 \ifdim\dimen@ii=\z@\DN@{}%
 \else
 \ifdim\dimen@ii<\z@\advance\dimen@\dimen@ii
 \else\advance\dimen@-\dimen@ii\fi
 \ifdim\dimen@<\z@\multiply\dimen@\m@ne\fi
 \ifdim\dimen@<.2\p@\DN@{}%
 \else
 \count@=\segmentnum@\relax 
 \ifdim\dimen@ii<\z@\advance\dimen@ii\splinelength@
 \ifnum\count@>\@ne\advance\count@\m@ne
 \edef\next@{\noexpand\splinesegment@{\the\count@}%
 \noexpand\spline@find\p@{\the\dimen@ii}{}%
 \noexpand\checksplinefind@{\the\dimen@ii}}%
 \else
 \xywarning@{cannot slide \the\dimen@ii\space before start}%
 \DN@{\splinesegment@\@ne \spline@find\z@\z@{}}\fi
 \else\advance\dimen@ii-\splinelength@
 \count@@=\numcontrolpts 
 \ifnum\count@<\count@@ \advance\count@\@ne
 \edef\next@{\noexpand\splinesegment@{\the\count@}%
 \noexpand\spline@find\z@{\the\dimen@ii}{}%
 \noexpand\checksplinefind@{\the\dimen@ii}}%
 \else
 \xywarning@{cannot slide \the\dimen@ii\space beyond end}%
 \DN@{\splinesegment@{\the\count@@}\spline@find\p@\z@{}}\fi
 \fi
 \fi\fi \next@ }
\xydef@\resetbreaks@{%
 \let\bstartPLACE@=\relax \let\bthisPLACE@=\empty
 \let\bendPLACE@=\relax \let\bprevPLACE@=\relax}
\xydef@\invisbreaks@{\resetbreaks@ \let\bstartPLACE@=\empty}
\xydef@\crvresetbreaks@{\resetbreaks@ \let\bstartPLACE@=\relax }
\xydef@\initbreaks@{\xy@@{\ifx\bstartPLACE@\relax
 \def\bstartPLACE@{0}\def\bendPLACE@{1}\else
 \ifx\bstartPLACE@\empty\def\bstartPLACE@{0}\def\bendPLACE@{1}%
 \fi\fi}}
\xydef@\lastbreaks@{\ifx\bprevPLACE@\relax \def\bstartPLACE@{0}%
 \else \expandafter \bprevPLACE@ \fi 
 \let\bprevPLACE@\relax \let\bendPLACE@\relax}
\xylet@\bstartPLACE@\relax
\xylet@\bendPLACE@\relax
\xylet@\bprevPLACE@\relax
\xydef@\bthisPLACE@{1}
\xydef@\splinebreak@{%
\splinetrace@{***new break*** this:\bthisPLACE@ }%
 \ifx\bthisPLACE@\empty\def\bendPLACE@{1}%
 \else\edef\bendPLACE@{\bthisPLACE@}\let\bthisPLACE@\empty\fi
 \ifx\bprevPLACE@\relax\def\bstartPLACE@{0}\else\expandafter\bprevPLACE@\fi
 \edef\bprevPLACE@{\def\noexpand\bstartPLACE@{\bendPLACE@}\pfromthec@}%
\splinetrace@{splineBREAK: \bstartPLACE@ <> \bendPLACE@}%
 \edef\cv@brend{\cfromthec@}%
 \edef\cv@brstart{\cfromthep@}%
 \expandafter\connect\expandafter\crvs\crvSTYLE@@{}%
 \let\cv@brend=\relax
 \let\cv@brstart=\relax
\splinetrace@{**break done**}%
} 
\xydef@\splinelast@{\splinereset@ \lastbreaks@
\splinetrace@{splineLAST}%
 \edef\cv@brend{\cfromthec@}%
 \edef\cv@brstart{\cfromthep@}%
 \expandafter\connect\expandafter\crvs\crvSTYLE@@{}%
 \let\cv@brend=\relax
 \let\cv@brstart=\relax
\splinetrace@{**last done**}%
 \resetbreaks@}
\xydef@\splineNointercept@{\enter@{\pfromthep@}%
 \begingroup \splinereset@ \csname cv@0\endcsname \swap@ 
 \count@=\ptsnum@ \advance\count@\@ne \csname cv@\the\count@\endcsname 
 \edef\tmp@{\endgroup \X@origin=\the\X@p \Y@origin=\the\Y@p
 \R@c=\the\d@X \U@c=\the\d@Y}\tmp@
 \loop@
 \dimen@=\ifdim\R@c<\z@-\fi\R@c
 \advance\dimen@ \ifdim\U@c<\z@-\fi\U@c
 \ifdim\dimen@>10\p@
 \advance\R@c \ifdim\R@c<\z@-\fi 16sp \divide\R@c\KK@ 
 \advance\U@c \ifdim\U@c<\z@-\fi 16sp \divide\U@c\KK@
 \repeat@
 \intersect@ \leave@}
\xydef@\splineintercept@{\Hidden@true\Invisible@true\splineintercept@i}
\xydef@\splineintercept@i{\enter@{\pfromthep@}\begingroup 
 \R@p=\X@c \L@p=\X@p \d@X=\R@p \advance\d@X-\L@p
 \D@p=\Y@c \U@p=\Y@p \d@Y=\D@p \advance\d@Y-\U@p
 \dimen@nth\KK@\d@X \edef\sd@X{\expandafter\removePT@\the\d@X}%
 \dimen@nth\KK@\d@Y \edef\sd@Y{\expandafter\removePT@\the\d@Y}%
 \dimen@=\sd@Y\L@p \advance\dimen@-\sd@X\U@p 
 \edef\sideOffset@{\the\dimen@}\def\closestseg@{1}%
 \let\crvconnect@@=\relax \crvconnect@
 \let\spline@end=\splinef@end
 \def\spline@start{\bgroup \def\prevnext@{+-}%
 \def\splinerec@{\let\splinerec@=\splineIrec@ \splineinterceptTest@}%
 \def\splinedecast@{\let\splinedecast@=\splinedecast@@
 \def\splineadvance@{\splineIadvance@@}\splinedecast@@}%
 \def\splineadvance@{\intercepthull@}%
 \global\let\splinepoint=\splineIpt@@
 \global\let\splinegoal@=\splinef@pt
 \global\let\splinefinish@=\splinefinish@@}%
 \begingroup \splineIsegment@ 
 \splinesetparams@ \splined@@ \def\postfind@{}\splineIplace@
 \setupDirection@ii \leave@ }
\xydef@\splineIplace@{%
 \d@X=\dimen5 \d@Y=\dimen7 \dimen@=\splineval@
 \expandafter\count@\xycrvptsnum@\relax
 \ifnum\count@>\tw@ \advance\count@\m@ne
 \advance\dimen@\segmentnum@\p@ \advance\dimen@-\p@ 
 \dimen@nth\count@\dimen@
 \fi \edef\tmp@{\endgroup \endgroup
 \def\noexpand\PLACEf@{{\expandafter\removePT@\the\dimen@}}%
 \X@c=\dimen@i \Y@c=\dimen3
 \d@X=\the\d@X \d@Y=\the\d@Y }\tmp@
\splinetrace@{PLACE = \PLACEf@:(\the\X@c, \the\Y@c)}%
 \expandafter\edef\expandafter\bthisPLACE@\PLACEf@
 }
\xydef@\splineIrec@{\splineinterceptTest@ }
\xydef@\squineIpt@{\edef\tmp@{\endgroup
 \def\noexpand\prevnext@{\next}\begingroup}\tmp@ }
\xydef@\squineIadvance@{\edef\tmp@{\endgroup
 \def\noexpand\prevnext@{\next}\def\noexpand\howclose@{\howclose@}}%
 \tmp@ \splineadvance@@\begingroup}
\xydef@\cubicIpt@{\edef\tmp@{\endgroup
 \def\noexpand\prevnext@{\next}\begingroup}\tmp@ }
\xydef@\cubicIadvance@{\edef\tmp@{\egroup
 \def\noexpand\prevnext@{\next}\def\noexpand\howclose@{\howclose@}}%
 \tmp@ \splineadvance@@\bgroup}
\xydef@\splineIsegment@{\DN@{\splinesegment@\@ne}%
 \ifx\splinesegment@\squinesegment@\else
 \ifx\splinesegment@\cubicsegment@\else\DN@{\findIsegment@}%
 \fi\fi\next@}
\xydef@\findIsegment@{\expandafter\count@\xycrvptsnum@ \count@@\z@ 
 \loop@ \advance\count@@\@ne \bgroup 
 \expandafter\splinesegment@\expandafter{\the\count@@}%
 \xysidesofinterval@
 \findIsegment@i \repeat@ 
 \expandafter\dimen@\prevhowclose@ \relax
 \ifdim\dimen@=\z@ \edef\closestseg@{\the\count@@}\fi
 \expandafter\splinesegment@\expandafter{\closestseg@}}
\xydef@\findIsegment@i{%
 \expandafter\ifx\next \expandafter\findIsegment@ii
 \else\expandafter\findIsegment@x\fi \next@ }
\xydef@\findIsegment@ii{\expandafter\count@\xycrvptsnum@ \relax
 \advance\count@\m@ne \ifnum\count@>\segmentnum@\relax
 \expandafter\findIsegment@y\else\expandafter\findIsegment@x\fi}
\xydef@\findIsegment@x{%
 \edef\next@{\egroup\def\noexpand\next{\next}%
 \def\noexpand\prevhowclose@{\prevhowclose@}%
 \def\noexpand\closestseg@{\closestseg@}\noexpand\iffalse}}
\xydef@\findIsegment@y{%
 \edef\next@{\egroup\def\noexpand\next{\next}%
 \def\noexpand\prevhowclose@{\prevhowclose@}%
 \def\noexpand\closestseg@{\closestseg@}\noexpand\iftrue}}
\xydef@\xysidesofinterval@{\bgroup 
 \L@p=\sd@X\Y@p \advance\L@p-\sd@Y\X@p \advance\L@p\sideOffset@
 \U@p=\sd@X\Y@c \advance\U@p-\sd@Y\X@c \advance\U@p\sideOffset@
 \def\this@{}\ifdim\L@p>\almostz@ \ifdim\U@p>\almostz@ \def\next{++}\else
 \ifdim\U@p<-\almostz@ \def\next{+-}\else\def\next{+0}\def\this@{-}\fi\fi
 \else\ifdim\L@p<-\almostz@ \ifdim\U@p>\almostz@ \def\next{-+}\else
 \ifdim\U@p<-\almostz@ \def\next{--}\else\def\next{-0}\def\this@{+}\fi\fi
 \else \ifdim\U@p>\almostz@ \def\next{0+}\else
 \ifdim\U@p<-\almostz@ \def\next{0-}\else\def\next{00}\def\this@{+}\fi\fi
 \fi\fi
 \ifx\this@\empty
 \L@p=\ifdim\L@p<\z@-\fi\L@p \U@p=\ifdim\U@p<\z@-\fi\U@p 
 \ifdim\L@p<\U@p \edef\howclose@{\the\L@p}\def\this@{-}%
 \else \edef\howclose@{\the\U@p}\def\this@{+}\fi
 \else\def\howclose@{0.0pt}\fi 
\splinetrace@{\next:\this@:\howclose@;\the\splineval@:%
 (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c)}%
 \ifdim\howclose@<\prevhowclose@\relax 
 \edef\tmp@{\egroup\def\noexpand\this@{\this@}\def\noexpand\next{\next}%
 \def\noexpand\howclose@{\howclose@}\def\noexpand\prevhowclose@{\howclose@}%
 \def\noexpand\closestseg@{\segmentnum@}}%
\splinetrace@{closest yet: \howclose@, in segment \segmentnum@}%
 \else
 \edef\tmp@{\egroup\def\noexpand\this@{\this@}\def\noexpand\next{\next}%
 \def\noexpand\howclose@{\howclose@}}%
 \fi \tmp@ }
\xydef@\splineinterceptTest@{%
 \xysidesofinterval@ \DN@{\splineadvance@}%
 \DNii@{0.0pt}\ifx\howclose@\nextii@ \DN@{\splineclosest@}%
 \else\expandafter\ifx\next \expandafter\ifx\prevnext@
 \ifx\next\prevnext@\else\DN@{\X@c=\X@p \Y@c=\Y@p 
 \splinefinishf@}\fi\fi
 \else \DN@{\splinedecast@}\fi\fi 
 {\splinefar@false \splinenear@\X@p\X@c\Y@p\Y@c 
 \ifsplinefar@ \aftergroup\next@
 \else\aftergroup\splineclosest@
\splinetrace@{too close: (\the\X@p,\the\Y@p)::(\the\X@c,\the\Y@c)}%
 \fi}}
\xydef@\splineclosest@{%
 \expandafter\ifx\this@-\relax
 \X@c=\X@p \Y@c=\Y@p \global\advance\splineval@-\splinedepth@
 \fi \splinefinishf@ }%
\xydef@\squinetestcvxhull@{\begingroup
\splinetrace@{hull: closest in segment \closestseg@}%
 \expandafter\splinesegment@\ifx\undefined\closestseg@\@ne\else\closestseg@\fi
 \X@c=\L@c \Y@c=\U@c \xysidesofinterval@ 
 \expandafter\ifx\next \expandafter\splineoutsidehull@@
 \else \expandafter\splineinsidehull@\fi}
\xydef@\cubictestcvxhull@{\begingroup
 \expandafter\splinesegment@\ifx\undefined\closestseg@\@ne\else\closestseg@\fi
 \X@c=\L@c \Y@c=\U@c \xysidesofinterval@ 
 \expandafter\ifx\next \expandafter\cubictestcvxhull@i
 \else \expandafter\splineinsidehull@\fi}
\xydef@\cubictestcvxhull@i{%
 \X@c=\R@c \Y@c=\D@c \xysidesofinterval@ 
 \expandafter\ifx\next \expandafter\splineoutsidehull@@
 \else \expandafter\splineinsidehull@\fi}
\xydef@\xysidesofhull@{\bgroup 
 \L@p=\sd@X\Y@p \advance\L@p-\sd@Y\X@p \advance\L@p\sideOffset@
 \U@p=\sd@X\Y@c \advance\U@p-\sd@Y\X@c \advance\U@p\sideOffset@
 \L@p=\ifdim\L@p<\z@-\fi\L@p \U@p=\ifdim\U@p<\z@-\fi\U@p 
 \ifdim\L@p<\U@p \edef\howclose@{\the\L@p}\def\this@{-}%
 \else \edef\howclose@{\the\U@p}\def\this@{+}\fi
 \ifx\splinedecast@\squinedecast@ \D@c=\U@c \R@c=\L@c \fi
 \L@p=\sd@X\U@c \advance\L@p-\sd@Y\L@c \advance\L@p\sideOffset@
 \L@p=\ifdim\L@p<\z@-\fi\L@p 
 \expandafter\if\this@-%
 \ifdim\L@p<\prevhowclose@ \def\next{-+}\else \def\next{--}\fi
 \else
 \ifdim\L@p<\howclose@ \def\next{-+}\else 
 \U@p=\sd@X\D@c \advance\U@p-\sd@Y\R@c \advance\U@p\sideOffset@
 \U@p=\ifdim\U@p<\z@-\fi\U@p
 \ifdim\U@p<\howclose@ \def\next{+-}\else \def\next{++}\fi
 \fi\fi
 \edef\tmp@{\egroup\def\noexpand\this@{\this@}\def\noexpand\next{\next}%
 \def\noexpand\howclose@{\howclose@}}\tmp@ }
\def\PLACE@intercept@#1{%
 \xy@@{\enter@{\pfromthep@\basefromthebase@}\begingroup}%
 \xy@@ix@{#1}\xy@@{\plainxy@ \def\Creset@@{}%
 \expandafter\POS\the\toks9\relax
 \DNii@{\crvreset@}\ifx\nextii@\Creset@@ \edef\next@{\endgroup
 \def\noexpand\xyinterceptpts@{\the\crvpts@}%
 \X@c =\the\X@c \Y@c=\the\Y@c \X@p=\the\X@p \Y@p=\the\Y@p
 \noexpand\CCintercept@@ }%
 \else \edef\next@{\endgroup
 \X@c =\the\X@c \Y@c=\the\Y@c \X@p=\the\X@p \Y@p=\the\Y@p
 \noexpand\Cintercept@@ }%
 \fi \next@ \leave@}%
 \PLACE@@}
\xydef@\CCintercept@@{\splineSintercept@}
\xydef@\splineSintercept@{\enter@{\pfromthep@}\begingroup 
 \Creset@@ \edef\connect@pts{\cfromthec@ \pfromthep@}%
 \xyinterceptpts@ \splinereset@ \connect@pts \splineintercept@
 \edef\next@{\endgroup \cfromthec@ \DirectionfromtheDirection@ }%
 \next@ \let\xyinterceptpts@=\empty \leave@}
\xydef@\nointerceptwarning@{\let\nointerceptwarning@=\relax
 \xywarning@{perhaps no curve intersection, or many. }}
\xydef@\intercepthull@{\nointerceptwarning@ 
 \expandafter\def\expandafter\prevnext@\expandafter{\next}%
 \splinetestcvxhull@}
\xydef@\splinetestcvxhull@{\begingroup 
 \X@c=\L@c \Y@c=\U@c \splinetrace@{hull:}\xysidesofinterval@ 
 \expandafter\ifx\next \expandafter\splineoutsidehull@@
 \else \expandafter\splineinsidehull@\fi}
\xydef@\splineinsidehull@{\edef\tmp@{\endgroup 
 \def\noexpand\howcvxclose@{\howclose@}%
 \noexpand\interceptinsidehull@}\tmp@ }
\xydef@\interceptinsidehull@{\edef\prevhowclose@{\howclose@}%
 \splinedecast@@ }
{\xdef\next{\the\maxdimen}}
\xylet@\prevhowclose@=\next
\xydef@\splineoutsidehull@{\edef\tmp@{\endgroup
 \def\noexpand\howcvxclose@{\howclose@}%
 \noexpand\interceptoutsidehull@}\tmp@}
\xylet@\splineoutsidehull@@=\splineoutsidehull@
\xydef@\interceptoutsidehull@{\dimen@=\howcvxclose@ \relax
\splinetrace@{OUTSIDE HULL: \the\dimen@ : (\howclose@)(\prevhowclose@)}%
 \let\splinedecast@=\splinedecast@@
 \let\splinerec@\splineHnear@test
 \let\splineadvance@\splineIadvance@@
 \splinedecast@@ }
\xydef@\splineHnear@test{%
 \xysidesofhull@ \DN@{\splinedecast@}%
 \ifdim\howclose@<\prevhowclose@\edef\howclose@{\prevhowclose@}\fi
 \expandafter\if\this@-%
 \expandafter\ifx\next\DN@{\splineclosest@}\fi
 \else
 \expandafter\ifx\next\DN@{\splineadvance@}\fi
 \fi
 {\splinefar@false \splinenear@\X@p\X@c\Y@p\Y@c 
 \ifsplinefar@ \aftergroup\next@
 \else\aftergroup\splineclosest@
\splinetrace@{too close: (\the\X@p,\the\Y@p)::(\the\X@c,\the\Y@c)}%
 \fi}}
\xydef@\cubicoutsidehull@{\edef\tmp@{\endgroup
 \def\noexpand\howcvxclose@{\howclose@}}\tmp@
 \edef\prevhowcvxclose@{\howcvxclose@}\begingroup 
 \X@p=\R@c \Y@p=\D@c \splinetrace@{hullii:}\xysidesofinterval@ 
 \expandafter\ifx\next \expandafter\cubicoutsidehull@i
 \else \expandafter\cubicinsidehull@\fi} 
\xydef@\cubicinsidehull@{\edef\tmp@{\endgroup
 \def\noexpand\howclose@{\howclose@}}\tmp@
 \cubicoutsidehull@ii }
\xydef@\cubicoutsidehull@i{\edef\tmp@{\endgroup
 \def\noexpand\howcvxclose@{\howclose@}}\tmp@
 \dimen@=\prevhowcvxclose@\relax 
 \ifdim\dimen@<\howcvxclose@ \relax
 \edef\howcvxclose@{\the\dimen@}\expandafter\interceptoutsidehull@
 \else \expandafter\cubicoutsidehull@ii\fi }
\xydef@\cubicoutsidehull@ii{%
 \def\splineadvance@{\splineadvance@@}%
 \def\splinepoint\endgroup{\endgroup
 \global\let\splinepoint=\relax
 \def\splineadvance@{\intercepthull@}}%
 \splinedecast@@ }%
\xydef@\splineHadvance@{\futurelet\next@\splineHadvance@i}
\xydef@\splineHadvance@i{\ifx\next@\endgroup
 \expandafter\splineHadvance@x\else\expandafter\splineclosest@\fi}
\xydef@\splineHadvance@x{\edef\tmp@{\endgroup
 \def\noexpand\prevhowclose@{\prevhowclose@}%
 \def\noexpand\prevnext@{\next}\def\noexpand\howcvxclose@{\howclose@}}%
 \tmp@ \dimen@=\prevhowclose@ \relax
 \ifdim\dimen@<\howclose@ \relax \DN@{\splineclosest@\begingroup}%
 \else\ifdim\howcvxclose@=\dimen@\DN@{\splineclosest@\begingroup}%
 \else\DN@{\splineadvance@@\begingroup}\fi\fi \next@ }
\xydef@\xyclearcrv@{\cv@end\cv@restore\loop@
 \expandafter\let\csname cv@\number\crv@cnt@\endcsname\relax
 \ifnum\crv@cnt@>0\advance\crv@cnt@\m@ne\repeat@
 \let\cv@start=\relax \let\cv@end=\relax \let\cv@restore=\relax \POS}
\xylet@\clearcurve=\xyclearcrv@
\xylet@\numcontrolpts=\xynumctrlpts@
\xydef@\xycontrolpt@#1{{%
 \ifnum#1<\z@\aftergroup\cv@restore\aftergroup\cv@start
 \else
 \expandafter\count@\xycrvptsnum@\relax \advance\count@\@ne
 \ifnum#1>\count@ \ifx\cv@end\relax 
 \expandafter\aftergroup\csname cv@\number#1\endcsname
 \else\aftergroup\cv@end\fi
 \else 
 \expandafter\ifx\csname cv@\number#1\endcsname\relax
 \ifnum#1=\z@\aftergroup\cv@start\else\aftergroup\cv@end\fi
 \else\expandafter\aftergroup\csname cv@\number#1\endcsname
 \fi\fi\fi}}%
\xylet@\xycontrolpt=\xycontrolpt@
\xydef@\startxycurve@@{\crv@cnt@=\z@
 \edef\cv@start{\cfromthep@}%
 \ifdim\zz@\R@c \ifdim\zz@\L@c \ifdim\zz@\D@c \ifdim\zz@\U@c
 \Edge@c={\zeroEdge}\fi\fi\fi\fi
 \edef\cv@end{\cfromthec@}%
 \edef\cv@restore{\pfromthep@\basefromthebase@}}
\xylet@\startxycurve@=\startxycurve@@
\xylet@\cv@start=\relax
\xylet@\cv@end=\relax
\xylet@\cv@restore=\relax
\xydef@\readxycurve@{\startxycurve@\xycrvmods@}
\xylet@\readxycurve=\readxycurve@
\xydef@\addtocrv@{\advance\crv@cnt@\@ne 
 \edef\tmp@{%
 \expandafter\noexpand\csname cv@\number\crv@cnt@\endcsname}%
 \expandafter\edef\tmp@{\cfromthec@}%
 \edef\tmp@{\noexpand\addtocrvpts@{\noexpand\def
 \expandafter\noexpand\tmp@{\X@c=\the\X@c \Y@c=\the\Y@c }}}\tmp@
 \edef\xycrvptsnum@{\the\crv@cnt@}%
}
\xydef@\xycrvdrop@{ {\zerodot}}
\xydef@\xycrvconn@{}
\xydef@\xyc@trlpts@{\def\xycrvdrop@{ \dir{x}}\def\xycrvconn@{}%
 \afterCURVE{\savecrvobjects@\xyctrlpts@}\readxycurve@}
\xydef@\xyc@trlpts@@{%
 \afterCURVE{\savecrvobjects@\def\xycrvdrop@{ \dir{x}}%
 \def\xycrvconn@{}\xyctrlpts@}\readxycurve@}
\xydef@\xyc@vxhull@{\def\xycrvdrop@{ {}}%
 \edef\xycrvconn@{ \noexpand\dir{\addDASH@{}}}%
 \afterCURVE{\savecrvobjects@\xycvxhull@}\readxycurve@}
\xydef@\xyc@vxhull@@{%
 \afterCURVE{\savecrvobjects@\def\xycrvdrop@{ {}}%
 \edef\xycrvconn@{ \noexpand\dir{\addDASH@{}}}\xycvxhull@}\readxycurve@}
\xylet@\controlpts=\xyc@trlpts@
\xylet@\convexhull=\xyc@vxhull@
\xydef@\savecrvobjects@{\bgroup 
 \expandafter\toks@\expandafter{\xycrvdrop@}%
 \expandafter\toks@ii\expandafter{\xycrvconn@}%
 \edef\tmp@{\egroup\noexpand\def\noexpand\resetcrvobjects@{%
 \noexpand\def\noexpand\xycrvdrop@{\the\toks@}%
 \noexpand\def\noexpand\xycrvconn@{\the\toks@ii}%
 }}\tmp@}
\xydef@\afterCURVE#1{\def\afterCURVE@{#1}}
\xydef@\endxycurve@{\cv@end\savectrlptsnum@
 \expandafter\def\csname params@\endcsname{\the\crvpts@}%
 \cv@restore\afterCURVE@\POS}
\xylet@\endcurve=\endxycurve@
\xydef@\xyctrlpts@{\cv@end \cv@restore
 \def\crvconnect@{\straitconnect@}%
 \ifnum\crv@cnt@>\z@ 
 \count@@@=\@ne \DN@{\loop@\xycontrolpt@{\count@@@}\relax
 \expandafter\xycvxhulldrop@\xycrvdrop@
 \ifnum\crv@cnt@>\count@@@\advance\count@@@\@ne\repeat@ 
 \cv@end \cv@restore }%
 \else\DN@{\relax}\fi \next@ }
\xylet@\xyctrlpts=\xyctrlpts@
\xydef@\addtocrvpts@#1{\crvpts@=\expandafter{\the\crvpts@#1}}
\xydef@\savescope@{\crvpts@={}%
 \edef\tmp@{\expandafter\noexpand\csname cv@0\endcsname}%
 \edef\tmp@{\noexpand\addtocrvpts@{\noexpand\def
 \expandafter\noexpand\tmp@{\X@c=\the\X@p \Y@c=\the\Y@p}}}%
 \tmp@ }
\xydef@\savectrlptsnum@{%
 \advance\crv@cnt@\@ne \edef\tmp@{%
 \expandafter\noexpand\csname cv@\number\crv@cnt@\endcsname}%
 \edef\tmp@{\noexpand\addtocrvpts@{\noexpand\def
 \expandafter\noexpand\tmp@{\X@c=\the\X@c \Y@c=\the\Y@c}}}\tmp@
 \advance\crv@cnt@\m@ne 
 \edef\tmp@{\expandafter\noexpand\csname ptsnum@\endcsname}%
 \edef\tmp@{\noexpand\addtocrvpts@{%
 \noexpand\def\expandafter\noexpand\tmp@{\number\crv@cnt@}}}%
 \tmp@ }
\xydef@\xycvxhull@{\cv@end \cv@restore 
 \addtocrvpts@{\def\crvconnect@{\straitconnect@}}%
 \def\crvconnect@{\straitconnect@}%
 \ifnum\crv@cnt@>\z@ 
 \count@@@=\@ne\relax \DN@{\loop@\xycontrolpt@{\count@@@}\relax
 \expandafter\xycvxhulldrop@\xycrvdrop@
 {\expandafter\connect\xycrvconn@{}}\pfromc@
 \ifnum\crv@cnt@>\count@@@\relax \advance\count@@@\@ne\repeat@ 
 \cv@end }%
 \else
 \ifx\empty\xycrvconn@
 \edef\xycrvconn@{\noexpand!C\noexpand\dir{\addDASH@{}}}\fi
 \DN@{\relax}\fi \next@ 
 {{\expandafter\connect\xycrvconn@{}}}%
 \cv@end \cv@restore }
\xylet@\xycvxhull=\xycvxhull@
\xydef@\xycvxhulldrop@#1#{\drop@{#1}}
\xydef@\savespline@{%
\splinetrace@{savespline@:}%
 \edef\endspline@{\endgroup 
 \savesplineparams@ \savesplinerefs@
 \X@min=\the\X@min\relax \X@max=\the\X@max\relax
 \Y@min=\the\Y@min\relax \Y@max=\the\Y@max\relax
 \ifInvisible@\noexpand\Invisible@true
 \else\noexpand\Invisible@false\fi
 }\endspline@ 
 \edef\tmp@{\noexpand\addtocrvpts@{\savesplineparams@}}\tmp@
 \xycontrolpt@\z@ \cv@end }
\xydef@\savesplineparams@{%
 \noexpand\def\expandafter\noexpand\xysplineedges@{\xysplineedges@}}
\xydef@\savesplinerefs@{%
 \noexpand\def\noexpand\xysplineparams@{%
 \expandafter\noexpand\xysplineparams@}%
 \noexpand\def\noexpand\xysplineedges@{%
 \expandafter\noexpand\xysplineedges@}%
}
\xynew@{box}\splinebox@ 
\xynew@{dimen}\splineval@ 
\xynew@{dimen}\splinedepth@ 
\xynew@{dimen}\splinetol@ 
\xynew@{dimen}\splinelength@ 
\xynew@{if}\ifsplinefar@
\xynew@{if}\ifsplineplot@
\xydef@\splinetracing{\let\splinetrace@=\W@}
\xydef@\splineignore@#1{}
\xylet@\splinetrace@=\splineignore@
\xydef@\readsplineparams@{%
 \expandafter\expandafter\expandafter\getsplineparams@\xysplineparams@
 \expandafter\expandafter\expandafter\getsplineedges@safe\xysplineedges@ @@}
\xydef@\getsplineedges@safe#1@@{\DN@{#1}%
 \ifx\next@\empty \DN@{\getsplineedges@.0pt;0.0pt,0.0pt;0.0pt,}%
 \else \DN@{\getsplineedges@safe@#1@@}\fi \next@}
\xydef@\getsplineedges@safe@#1;#2,#3@@{\DN@{#3}%
\splinetrace@{getsplineedges@safe}%
 \ifx\next@\empty \DN@{\getsplineedges@#1;#2,0.0pt;0.0pt,}%
 \else \DN@{\getsplineedges@#1;#2,#3}\fi \next@}
\xydef@\getsplineedges@#1;#2,#3;#4,{%
 \global\dimen@i=#1\global\dimen5=#2\relax
 \dimen@=#3\multiply\dimen@\m@ne \advance\dimen@\splinelength@
 \global\dimen3=\dimen@
 \dimen@=#4\relax 
 \ifdim\dimen@>\p@ \xywarning@{edge out-of-range: \the\dimen@}%
 \count@=\dimen@ \divide\count@\p@
 \advance\dimen@-\count@\p@ \multiply\dimen@\m@ne
 \advance\dimen@ \count@\p@ \advance\dimen@\p@
\splinetrace@{\the\dimen@}%
 \else
 \multiply\dimen@\m@ne \advance\dimen@\p@
 \fi
 \global\dimen7=\dimen@ }
\xydef@\dimen@half{%
 \advance\dimen@ \ifdim\dimen@<\z@-\fi 1sp \divide\dimen@\tw@}
\xydef@\halve@dimen#1{\dimen@=#1\relax \dimen@half #1=\dimen@}
\xydef@\dimen@nth#1#2{\dimen@=#2\relax \dimen@ii=#1sp
 \advance\dimen@ \ifdim\dimen@<\z@-\fi.5\dimen@ii 
 \divide\dimen@ by#1\relax #2=\dimen@}
\xydef@\splinetolerance@#1{\dimen@=#1\relax
 \ifdim\dimen@>\z@ \splinetol@=\dimen@
 \else\splinetol@=.4\p@\fi}
\xylet@\splinedefaulttol@=\relax
\xydef@\splinetolerance#1{\splinetolerance@{#1}%
 \edef\splinedefaulttol@{\splinetol@=\the\splinetol@}}
\splinetolerance\z@
\xydef@\SloppyCurves{\splinetolerance{.8\p@}}
\xydef@\xylowtolerance@{\splinedefaulttol@
 \ifdim\splinetol@<\p@ \divide\splinetol@\tw@ \fi}
\xywarnifdefined\splinedrop@
\xydef@\setstdsplinedrop@{%
 \setbox\splinebox@=\hbox\bgroup
 \setboxz@h{\expandafter\object\xycrvdrop@{}}%
 \splinedefaulttol@ \dimen@=\wd\z@ \dimen@ii=\ht\z@ \advance\dimen@ii\dp\z@
 \ifdim\dimen@ii>\dimen@ \dimen@=\dimen@ii \fi \dimen@=1.4142\dimen@
 \ifdim\dimen@>\splinetol@ \splinetol@=\dimen@\else\dimen@=\splinetol@\fi
 \dimen@=.5\wd\z@ 
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \kern-\dimen@ \Drop@@ \kern\dimen@
 \edef\tmp@{\egroup \splinetol@=\the\splinetol@
 \ifInvisible@\noexpand\Invisible@true
 \else\noexpand\Invisible@false\fi}\tmp@
 \edef\splinedefaulttol@{\splinetol@=\the\splinetol@}%
 \def\splinedrop@{\copy\splinebox@\splineextra@@}}
\xywarnifdefined\splineconn@
\xydef@\stdsplineconn@{{\setsplinedir@
 \setboxz@h\bgroup\expandafter\object\xycrvconn@{}%
 \edef\tmp@{\egroup\L@c=\the\L@c \R@c=\the\R@c \D@c=\the\D@c \U@c=\the\U@c
 \noexpand\def\noexpand\Drop@@}\expandafter\tmp@\expandafter{\Drop@@}%
 \setboxz@h{\kern-\L@c \boxz@}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \Drop@@}}
\xydef@\setcrvobjects@{\setstdsplinedrop@ \def\splineconn@{\stdsplineconn@}}
\xylet@\splineextra@@=\relax
\xydef@\splinenear@#1#2#3#4{{\d@X=#1\advance\d@X-#2%
 \ifdim\d@X<\z@ \d@X=-\d@X\fi
 \ifdim\splinetol@<\d@X \aftergroup\splinefar@true
 \else \d@Y=#3\advance\d@Y-#4\ifdim\d@Y<\z@ \d@Y=-\d@Y\fi
 \ifdim\splinetol@<\d@Y\aftergroup\splinefar@true
 \else \xydist@\d@X\d@Y
 \ifdim\splinetol@<\dimen@ \aftergroup\splinefar@true
 \else 
 \ifdim\dimen@<.1\splinetol@\aftergroup\splinetooclose@\fi
 \fi\fi\fi}}
\xydef@\splineadvance@@{\global\advance\splineval@\splinedepth@}
\xydef@\splinetooclose@{\aftergroup\aftergroup\aftergroup\splinetooclose@@}
\xydef@\splinetooclose@@{\def\splineplotpt@{\relax}}
\xydef@\splinepoint@@{%
\splinetrace@{P@:(\the\X@c,\the\Y@c)::\the\splineval@;\the\splinedepth@}%
 {\splinetest@\ifsplineplot@\relax\else\aftergroup\splinecontinue\fi}}
\xydef@\splinepoint@{%
 {\splinetest@\ifsplineplot@\aftergroup\splinecontinue\fi}}
\xylet@\splinepoint=\splinepoint@
\xydef@\splinecontinue@{%
 \global\let\splinepoint=\splinepoint@@
 \global\let\splinecontinue=\splinecontinue@@}
\xydef@\splinecontinue@@{%
 \global\let\splinepoint=\splinepoint@
 \global\let\splinecontinue=\relax}
\xylet@\splinecontinue=\splinecontinue@
\xydef@\splineknotpoint@{{\X@p=\X@c \Y@p=\Y@c \cv@start 
 \the\Edge@c\@ne \ifInside@\else\aftergroup\splineknotpoint@@\fi}}%
\xydef@\splineknotpoint@@{{\X@p=\X@c \Y@p=\Y@c \cv@end 
 \the\Edge@c\@ne \ifInside@\else \aftergroup\splinepoint\fi}}%
\xylet@\firstsplinepoint@=\splineknotpoint@
\xylet@\lastsplinepoint@= \splineknotpoint@
\xydef@\splined@@@{%
\splinetrace@{finding end types}%
\splinetrace@{bstartPLACE@:\bstartPLACE@; bendPLACE@:\bendPLACE@}%
 \DN@{\splinescan@}\ifx\bstartPLACE@\empty
 \ifx\bendPLACE@\relax\def\bendPLACE@{1}\fi
 \else\ifx\bstartPLACE@\relax
 \else\ifx\bstartPLACE@\undefined
 \else 
 \DN@{\splinescanbreak@}\ifx\bendPLACE@\relax\def\bendPLACE@{1}\fi
 \DNii@{0}\ifx\bstartPLACE@\nextii@
 \DNii@{1}\ifx\bendPLACE@\nextii@\DN@{}%
 \fi\fi
 \fi\fi\fi \next@ }%
\xydef@\splineStarttest@{{\X@p=\X@c \Y@p=\Y@c \cv@start \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}%
\xydef@\splineEndtest@{{\X@p=\X@c \Y@p=\Y@c \cv@end \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}%
\xydef@\splineBreakStarttest@{{\X@p=\X@c \Y@p=\Y@c \cv@brstart \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}%
\xydef@\splineBreakEndtest@{{\X@p=\X@c \Y@p=\Y@c \cv@brend \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}%
\xylet@\splineStarttest=\splineStarttest@
\xylet@\splineEndtest=\splineEndtest@
\xydef@\splineSlowStarttest{{\X@p=\X@c \Y@p=\Y@c \cv@start \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@maybe@@\else\aftergroup\splineplot@true\fi}}%
\xydef@\splineSlowEndtest{{\X@p=\X@c \Y@p=\Y@c \cv@end \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@maybe@@\else\aftergroup\splineplot@true\fi}}%
\xydef@\splineplot@maybe{\splineplot@false}%
\xylet@\splineplot@maybe@@=\splineplot@maybe
\xydef@\splinescan@{\bgroup%
 \expandafter\def\xysplineedges@{\z@;\z@,\z@;\z@,}%
 \bgroup \cv@start 
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ \gdef\splineedges@{\z@;\z@,}%
 \else\aftergroup\splinestartScan@\fi
 \egroup \relax
 \bgroup \cv@end 
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ 
 \getcrvsegsnum@ \edef\segmentnum@{\the\count@}%
 \splineval@=\z@ \splineRecordEndValue@
 \else\aftergroup\splineendScan@\fi
 \egroup \egroup
 \expandafter\testsplineedges@\splineedges@;,@@%
 \expandafter\edef\xysplineedges@{\splineedges@}%
 \global\let\splineedges@=\relax
\splinetrace@{edge params: \xysplineedges@}}%
\xydef@\testsplineedges@#1;#2,#3;#4,#5@@{%
 \DN@{#5}\ifx\next@\empty
 \DNii@{#4}\ifx\nextii@\empty
 \xynoedgespline@{end}\def\splineedges@{#1;#2,\z@;\z@,}\fi
 \DNii@{#2}\ifx\nextii@\empty
 \xynoedgespline@{start}\def\splineedges@{\z@;\z@,\z@;\z@,}\fi
 \fi }
\xydef@\xynoedgespline@#1{\xywarning@{#1 edge of spline not found}}%
\xydef@\splinestartScan@{\bgroup
\splinetrace@{scan for start}%
 \global\let\splineadvance@=\splineadvance@@
 \let\spline@start=\splinefindStart@
 \let\spline@end=\spline@end@@
 \let\splinefinish@=\splinefinish@@
 \let\splinewhich=\relax
 \global\splinelength@=\z@
 \def\splinerec@{\let\splinerec@=\splineSrec@ \splinedecast@@}%
 \edef\splineedges@{}%
 \expandafter\let\xysplineedges@\relax
 \xylowtolerance@ \splined@@ 
 \ifx\splineedges@\empty\expandafter\splineslowScan@\fi
 \ifx\splineedges@\relax\expandafter\splinenostart@\fi
 \egroup }%
\xydef@\splineslowScan@{%
 \let\splineStarttest=\splineSlowStarttest 
 \let\splinescanStarttest=\relax 
 \def\splinerec@{\let\splinerec@=\splineSrec@ \splinedecast@@}%
 \splined@@ }
\xydef@\splineslowEnd@{%
 \global\let\splineEndtest=\splineSlowEndtest 
 \let\splinescanEndtest=\relax 
 \def\splinerec@{\let\splinerec@=\splineErec@ \splinedecast@@}%
 \splined@@ }
\xydef@\splinenostart@{%
 \def\segmentnum@{1}\splinelength@=\z@ \splineval@=\z@
 \xynoedgespline@{start}\splineRecordValue@ }
\xydef@\splineendScan@{\bgroup
 \bgroup
\splinetrace@{scan for end}%
 \global\let\splineadvance@=\splineadvance@@
 \let\spline@start=\splinefindEnd@
 \let\spline@end=\spline@end@@ 
 \let\splinefinish@=\splinefinish@@
 \let\splinewhich=\relax
 \global\splinelength@=\z@ 
 \global\let\splineEndtest=\splineEndtest@ 
 \def\splinerec@{\let\splinerec@=\splineErec@ \splinedecast@@}%
 \expandafter\def\expandafter\prevedges@\expandafter{\splineedges@}%
 \xylowtolerance@ \splined@@ 
 \ifx\splineedges@\prevedges@\expandafter\splineslowScan@\fi
 \egroup \egroup}
\xydef@\splinescanbreak@{%
\splinetrace@{SCANBREAK}%
 \gdef\breakedges@{}%
 \DN@{0}\ifx\next@\bstartPLACE@
 \DN@{\bgroup \def\tmp@####1;####2,####3;####4,{%
 \global\splineval@=####2\relax}%
 \expandafter\expandafter\expandafter\tmp@\xysplineedges@
 \def\segmentnum@{1}\splineRecordBreakValue@ \egroup}%
 \else
 \bgroup \cv@start 
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ \aftergroup\splinezerostart
 \else\aftergroup\splinewidestart\fi
 \egroup 
 \fi \next@ 
 \DN@{1}\ifx\next@\bendPLACE@ 
 \DN@{\bgroup \def\tmp@####1;####2,####3;####4,{%
 \global\splineval@=####4\relax}%
 \expandafter\expandafter\expandafter\tmp@\xysplineedges@
%% \multiply\splineval@\m@ne \advance\splineval@\p@
%% \def\segmentnum@{1}
 \getcrvsegsnum@ \edef\segmentnum@{\the\count@}%
 \global\multiply\splineval@\count@ 
 \splineRecordEndBreakValue@ \egroup}%
 \else
 \bgroup \cv@end 
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ \aftergroup\splinezeroend
 \else\aftergroup\splinewideend\fi
 \egroup 
 \fi \next@ 
 \expandafter\def\expandafter
 \xybreakedges@\expandafter{\breakedges@}%
 \global\let\breakedges@=\relax
\splinetrace@{break params: \xybreakedges@::\bstartPLACE@--\bendPLACE@}%
 \expandafter\let\xysplineedges@\xybreakedges@ }
\xydef@\getcrvsegsnum@{%
 \count@=\ptsnum@\relax \ifnum\count@>\@ne\advance\count@\m@ne\fi}
\xydef@\splinezerostart{\DN@{\bgroup 
\splinetrace@{splinezerostart:}%
 \dimen@=\bstartPLACE@\p@ 
 \global\splineval@=\dimen@ 
 \splineRecordBreakValue@ \egroup }}
\xydef@\splinezeroend{\DN@{\bgroup 
\splinetrace@{splinezeroend:}%
 \dimen@=\bendPLACE@\p@
 \multiply\dimen@\m@ne \advance\dimen@\p@
 \def\segmentnum@{0}\global\splineval@=\dimen@ 
 \splineRecordEndBreakValue@ \egroup }}
\xydef@\splinewidestart{\DN@{\bgroup 
 \splinetrace@{scan for start}%
 \let\splinefbcontinue@=\breakstartcontinue@
 \let\splinef@pt=\splinef@breakpt
 \let\splinef@end=\break@start
 \edef\tmp@{{\bstartPLACE@}}%
 \expandafter\splinealong@@\tmp@\z@>\endgroup\egroup }}
\xydef@\splinewideend{\DN@{\bgroup 
 \splinetrace@{scan for wide end}%
 \let\splinefbcontinue@=\breakendcontinue@
 \let\splinef@pt=\splinef@breakpt
 \let\splinef@end=\break@end
 \edef\tmp@{{\bendPLACE@}}%
 \expandafter\splinealong@@\tmp@\z@<\endgroup\egroup }}
\xydef@\splineSrec@{{%
\splinetrace@{v=\the\splineval@ + d=\the\splinedepth@ :
 (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c):Srec }%
 \splineStarttest
 \ifsplineplot@ 
 \ifdim\splinedepth@<.0001\p@ \aftergroup\splinefinish@
 \global\advance\splineval@ .5\splinedepth@
 \else\aftergroup\splinedecast@@ \fi
 \else \aftergroup\splineadvance@ \fi}}
\xydef@\splinefindStart@@{\bgroup \bgroup 
 \expandafter\expandafter\expandafter\getsplineparams@\xysplineparams@
 \global\let\splineadvance@=\splineadvance@@
 \global\let\splinepoint=\relax
 \let\splinegoal@=\splineRecordValue@ \global\dimen5=\z@ 
 {\X@c=\X@p \Y@c=\Y@p \splinescanStarttest }%
} 
\xydef@\splinefindStart@{%
 \expandafter\crv@cnt@\xycrvptsnum@\relax
 \ifnum\crv@cnt@>\tw@
 \crv@cnt@=\@ne \splineplot@false \splinesegment@{\crv@cnt@}%
 {\splineStarttest
 \ifsplineplot@\aftergroup\splineplot@true\fi}%
 \ifsplineplot@ \else \searchforStartsegment@ \fi 
 \splinesegment@{\crv@cnt@}%
\splinetrace@{start is in segment \segmentnum@}%
 \else \splinesegment@\@ne \fi
 \splineplot@false \splinefindStart@@
}
\xydef@\searchforStartsegment@{\splineplot@true\loop@ 
 \advance\crv@cnt@\@ne 
 \expandafter\count@\xycrvptsnum@\relax
 \ifnum\count@=\crv@cnt@\expandafter\splineplot@false
 \else 
 \splinesegment@{\crv@cnt@}{\splineStarttest
 \ifsplineplot@\aftergroup\splineplot@false
 \else\aftergroup\splineplot@true\fi }%
 \fi \ifsplineplot@\repeat@ 
}
\xydef@\splinefindEnd@@{\bgroup \bgroup
 \expandafter\expandafter\expandafter\getsplineparams@\xysplineparams@
\splinetrace@{params:\xysplineparams@}%
 \splinereverse@@
\splinetrace@{params:\xysplineparams@}%
 \global\let\splineadvance@=\splineadvance@@
 \global\let\splinepoint=\splinescanEndtest 
 \let\splinegoal@=\splineRecordEndValue@ \global\dimen5=\z@ 
 {\X@c=\X@p \Y@c=\Y@p \splinescanEndtest }%
}
\xydef@\splinereverse@@{\splinereverse@@@}
\xydef@\splinereverse@@@{%
 \def\postspline@{\d@X=-\d@X \d@Y=-\d@Y}%
 \dimen@ii=\X@c \X@c=\X@p \X@p=\dimen@ii 
 \dimen@ii=\Y@c \Y@c=\Y@p \Y@p=\dimen@ii 
 \global\dimen5=-\dimen5\relax 
 \global\advance\dimen5\splinelength@ }
\xydef@\postspline@{}
\xydef@\splineErec@{{%
 \dimen@=\splineval@ \advance\dimen@\splinedepth@
\splinetrace@{ER (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c);;;
\the\dimen@,\the\splinedepth@}%
 \splineEndtest
 \ifsplineplot@ 
 \ifdim\splinedepth@<.0001\p@ \aftergroup\splinefinish@
 \else\aftergroup\splinedecast@@ \fi
 \else \aftergroup\splineadvance@ \fi}}
\xydef@\splinefindEnd@{%
 \expandafter\crv@cnt@\xycrvptsnum@\relax 
 \ifnum\crv@cnt@>\tw@
 \advance\crv@cnt@\m@ne 
 \splineplot@false \splinesegment@{\crv@cnt@}%
 {\X@c=\X@p \Y@c=\Y@p \splineEndtest
 \ifsplineplot@\aftergroup\splineplot@true\fi }%
 \ifsplineplot@ 
 \else \searchforEndsegment@ \fi 
 \splinesegment@{\crv@cnt@}%
\splinetrace@{end is in segment: \segmentnum@ }%
 \else \splinesegment@\@ne \fi
 \splineplot@false\splinefindEnd@@
}
\xydef@\searchforEndsegment@{\splineplot@true\loop@ 
 \advance\crv@cnt@\m@ne 
 \ifnum\crv@cnt@=\z@\expandafter\splineplot@false
 \else 
 \splinesegment@{\crv@cnt@}{\X@c=\X@p \Y@c=\Y@p \splineEndtest
 \ifsplineplot@\aftergroup\splineplot@false
 \else\aftergroup\splineplot@true\fi}%
 \fi \ifsplineplot@\repeat@ 
}
\xydef@\splinescanStarttest{%
\splinetrace@{SST (\the\X@c,\the\Y@c); \the\splinelength@, \the\splineval@}%
 {\splineplot@false\splineStarttest
 \ifsplineplot@\expandafter\splinefinish@\fi}}
\xydef@\splinescanEndtest{%
\splinetrace@{SET (\the\X@c,\the\Y@c); \the\splinelength@, \the\splineval@}%
 {\splineplot@false\splineEndtest 
 \ifsplineplot@\expandafter\splinefinish@\fi}}
\xydef@\splineBrec@{{%
 \dimen@=\splineval@ \advance\dimen@\splinedepth@
\splinetrace@{BR (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c);;;
\the\dimen@,\the\splinedepth@}%
 \splineEndtest
 \ifsplineplot@ \aftergroup\splineadvance@ \else
 \ifdim\splinedepth@<.0001\p@ \aftergroup\splinefinish@
 \else\aftergroup\splinedecast@@ \fi \fi}}
\xydef@\splineBSrec@{{%
\splinetrace@{SR (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c);;;
\the\dimen@,\the\splinedepth@:SR}%
 \splineStarttest
 \ifsplineplot@ 
 \ifdim\splinedepth@<.0001\p@ \aftergroup\splinefinish@
 \global\advance\splineval@ .5\splinedepth@
 \else \advance\splineval@\splinedepth@
 \splinetest@ \advance\splineval@-\splinedepth@
 \ifsplineplot@\aftergroup\splineadvance@
 \else\aftergroup\splinedecast@@\fi
 \fi
 \else
 \global\advance\splineval@\splinedepth@
 \aftergroup\splinefinish@ \fi }}
\xydef@\splineBErec@{{%
 \dimen@=\splineval@ \advance\dimen@\splinedepth@
\splinetrace@{BE (\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c);;;
 \the\dimen@,\the\splinedepth@}%
 \splineEndtest
 \ifsplineplot@ 
 \ifdim\splinedepth@<.0001\p@ \aftergroup\splinefinish@
 \global\advance\splineval@ .5\splinedepth@
 \else \advance\splineval@\splinedepth@
 \splinetest@ \advance\splineval@-\splinedepth@
 \ifsplineplot@\aftergroup\splineadvance@
 \else\aftergroup\splinedecast@@\fi
 \fi
 \else
 \ifdim\splinedepth@<\p@ \global\advance\splineval@\splinedepth@ \fi
 \aftergroup\splinefinish@ \fi }}
\xydef@\splinef@breakpt#1{%
 \ifdim\splineval@>\z@
\splinetrace@{found: val=\the\splineval@;(\the\X@c,\the\Y@c)}%
 \else
\splinetrace@{found: val=\the\splineval@;(\the\X@p,\the\Y@p)}%
 \fi \splinefbcontinue@ }
\xydef@\splinef@pt@@{%
 \ifdim\splineval@>\z@ 
\splinetrace@{found: val=\the\splineval@;c:(\the\X@c,\the\Y@c)}%
 \global\dimen@i=\X@c \global\dimen3=\Y@c 
 \else
\splinetrace@{found: val=\the\splineval@;p:(\the\X@p,\the\Y@p)}%
 \fi
 \setsplinedir@ \global\dimen5=\d@X \global\dimen7=\d@Y 
 \global\splineval@=\splineval@
 \aftergroup\splinefocus@ }
\xydef@\findbreakwarning@#1{%
 \xywarning@{#1 of break not found: bSTART=\bstartPLACE@, bEND=\bendPLACE@}%
 \DN@{#1}\def\DNii@{start}\ifx\next@\nextii@\splineRecordBreakValue@
 \else\splineRecordEndBreakValue@\fi\egroup}%
\xydef@\breakstartcontinue@{\bgroup \cv@start
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ \aftergroup\breakstartfound@
 \else \aftergroup\breakstartcontinue@i\fi \egroup }%
\xydef@\breakstartcontinue@i{%
\splinetrace@{move to start edge, from (\the\X@c,\the\Y@c): val=\the\splineval@ }%
 \global\let\splineEndtest=\splineBreakStarttest@
 \global\let\splinetest@=\splineBreakStarttest@
 \gdef\splinerec@{\global\let\splinerec@=\splineSrec@ \splinedecast@@}%
 \global\let\splinepoint=\relax
 \global\let\spline@end=\checkfoundSbreak@ 
 \global\let\splinegoal@=\splineRecordSBreakValue@ 
 \global\let\splinefinish@=\splinefinish@@ }
\xydef@\breakstartfound@{%
\splinetrace@{found start edge, at (\the\X@c,\the\Y@c): val=\the\splineval@ }%
 \global\let\splinetest@=\splineStarttest
 \gdef\splinerec@{\splinegoal@ \global\let\splinerec@=\splinefinish@ }%
 \global\let\splinepoint=\relax
 \global\let\spline@end=\relax
 \global\let\splinegoal@=\splineRecordBreakValue@ 
 \global\let\splinefinish@=\splinefinish@@
 }
\xydef@\checkfoundSbreak@{%
 \ifnum\xycrvptsnum@<\thr@@\DN@{\findbreakwarning@{start}}%
 \else\DN@{\searchBreakSsegment@}\fi \next@ }%
\xydef@\searchBreakSsegment@{%
 \crv@cnt@=\segmentnum@ \DN@{}\count@=\crv@cnt@
 \DNii@{}\ifnum\splineval@=\z@ \ifnum\crv@cnt@=\@ne
 \ifnum\xycrvptsnum@=\@ne\count@=\z@\DNii@{\egroup}\fi
 \else \DN@{\egroup}\fi 
 \else \ifnum\splineval@=\m@ne 
 \else \advance\crv@cnt@\@ne \fi \fi
 \ifnum\crv@cnt@=\xycrvptsnum@\relax
 \ifnum\xycrvptsnum@>\tw@ \DNii@{\egroup}\fi
 \DN@{\expandafter\splineRecordBreakValue@\nextii@}%
 \else
 \DN@{\splinesegment@{\crv@cnt@}\splinesetparams@
 \splined@@ \egroup}%
 \fi \next@ }
\xydef@\checkfoundEbreak@{%
 \ifnum\xycrvptsnum@<\thr@@\DN@{\findbreakwarning@{end}}%
 \else\DN@{\searchBreakEsegment@}\fi \next@ }%
\xydef@\searchBreakEsegment@{%
 \crv@cnt@=\segmentnum@ \DN@{}\count@=\crv@cnt@
 \DNii@{}\ifnum\splineval@=\z@ \ifnum\crv@cnt@=\@ne
 \ifnum\xycrvptsnum@=\@ne\count@=\z@\DNii@{\egroup}\fi
 \else\DN@{\egroup}\fi
 \else \advance\crv@cnt@\m@ne \fi 
 \ifnum\count@=\z@
 \ifnum\xycrvptsnum@>\tw@ \splineval@=\m@ne\p@
 \DNii@{\egroup}\fi
 \DN@{\expandafter\splineRecordEndBreakValue@\nextii@}\else
 \DN@{\splinesegment@{\crv@cnt@}\splinereverse@
 \readsplineparams@ \splined@@ \egroup}%
 \fi \next@ }
\xydef@\break@start{\egroup \egroup 
\splinetrace@{scan for start}%
 \global\let\splineadvance@=\splineadvance@@
 \let\spline@start=\splinefindBStart@
 \let\spline@end=\egroup
 \let\splinefinish@=\splinefinish@@
 \let\splinewhich=\relax
 \global\let\splineadvance@=\splineadvance@@
 \global\let\splinepoint=\relax
 \let\splinegoal@=\splineRecordBreakValue@
 \global\dimen5=\z@ \global\splinelength@=\z@
 \let\splinerec@=\splineSrec@ 
 \def\breakedges@{}%
 \bgroup \bgroup \splined@@ }
\xydef@\splinefindBStart@{\bgroup
 \global\splineval@=\z@ \splinedepth@=.5\p@}
\xydef@\breakendcontinue@{\bgroup
 \edef\tmp@{\X@p = \the\X@c \Y@p=\the\Y@c}\cv@end\tmp@
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\zeroEdge}%
 \ifx\next@\nextii@ \aftergroup\breakendfound@
 \else\aftergroup\breakendcontinue@i\fi \egroup }%
\xydef@\breakendcontinue@i{%
\splinetrace@{move to end edge, from (\the\X@c,\the\Y@c): val=\the\splineval@ }%
 \global\let\splineEndtest=\splineBreakEndtest@
 \global\let\splinetest@=\splineBreakEndtest@
 \gdef\splinerec@{\global\let\splinerec@=\splineErec@\splinedecast@@}%
 \global\let\splinepoint=\relax
 \global\let\spline@end=\checkfoundEbreak@ 
 \global\let\splinegoal@=\splineRecordEBreakValue@ 
 \global\let\splinefinish@=\splinefinish@@ 
 \splinerec@ }
\xydef@\splineRecordEBreakValue@{%
\splinetrace@{\the\count@\space segments, \the\splineval@}%
 \splineRecordEndBreakValue@ }
\xydef@\splineRecordSBreakValue@{\getcrvsegsnum@
 \dimen@=\splineval@ 
 \advance\dimen@\segmentnum@\p@ \advance\dimen@-\p@
 \dimen@nth\count@\dimen@
 \global\splineval@=\dimen@ \def\segmentnum@{1}%
 \splineRecordBreakValue@ }
\xydef@\breakendfound@{%
\splinetrace@{found end edge, at (\the\X@c,\the\Y@c): val=\the\splineval@ }%
 \global\let\splinetest@=\splineEndtest
 \gdef\splinerec@{\splinegoal@ \global\let\splinerec@=\splinefinish@}%
 \global\let\splinepoint=\relax
 \global\let\spline@end=\relax
 \global\let\splinegoal@=\splineRecordEndBreakValue@ 
 \global\let\splinefinish@=\splinefinish@@ }
\xydef@\break@end{\egroup \egroup
 \global\let\splineadvance@=\splineadvance@@
 \let\spline@start=\splinefindBEnd@
 \let\spline@end=\egroup 
 \let\splinefinish@=\splinefinish@@
 \let\splinewhich=\relax
 \global\let\splineadvance@=\splineadvance@@
 \global\let\splinegoal@=\splineRecordEndBreakValue@
 \global\splinelength@=\z@ 
 \let\splinerec@=\splineErec@ 
 \global\let\splineEndtest=\splineEndtest@ 
 \bgroup \splined@@ }
\xydef@\splinefindBEnd@{\bgroup\bgroup 
 \splinereverse@ \readsplineparams@ 
 \global\splineval@=\z@ }
\xydef@\splineRecordValue@{%
 \ifx\unknown\segmentnum@\relax
 \else
 \getcrvsegsnum@ 
 \dimen@=\splineval@ \advance\dimen@ \segmentnum@\p@
 \advance\dimen@-\p@ \dimen@nth\count@\dimen@
 \global\splineval@=\dimen@
 \fi
 \xdef\splineedges@{\splineedges@\the\splinelength@;\the\splineval@,}%
\splinetrace@{found edge: \splineedges@}}
\xydef@\splineRecordEndValue@{%
 \ifx\unknown\segmentnum@\relax
 \else
 \getcrvsegsnum@
 \dimen@=\splineval@ \advance\dimen@ \count@\p@
 \advance\dimen@-\segmentnum@\p@ \dimen@nth\count@\dimen@
 \global\splineval@=\dimen@
 \fi
 \xdef\splineedges@{\splineedges@\the\splinelength@;\the\splineval@,}%
\splinetrace@{found edge: \splineedges@}}
\xydef@\splineRecordBreakValue@{%
 \ifx\unknown\segmentnum@\relax
 \else\expandafter\advance\expandafter\splineval@\segmentnum@\p@
 \count@=\segmentnum@\relax 
 \ifnum\count@>0 \advance\splineval@-\p@ \fi\fi
 \xdef\breakedges@{\breakedges@\the\splinelength@;\the\splineval@,}%
 \global\let\spline@end=\egroup
\splinetrace@{found break edge: \breakedges@}}
\xydef@\splineRecordEndBreakValue@{%
 \ifx\unknown\segmentnum@\relax 
 \else\count@=\segmentnum@\relax \ifnum\count@=\z@
 \else \getcrvsegsnum@ 
 \count@@=\count@ \advance\count@@-\segmentnum@\relax
 \dimen@=\splineval@ \advance\dimen@ \count@@\p@
 \dimen@nth\count@\dimen@
 \global\splineval@=\dimen@
 \fi\fi
 \ifdim\splineval@<\z@ \relax\splineval@=\z@ \fi
 \ifx\breakedges@\relax\relax\else\ifx\breakedges@\empty\else
 \ifdim\splineval@<\p@\relax \ifdim\splineval@>\z@ 
 \expandafter\testbreakedges@\breakedges@ @%
 \fi\fi\fi\fi
 \xdef\breakedges@{\breakedges@\the\splinelength@;\the\splineval@,}%
 \global\let\spline@end=\egroup
\splinetrace@{found break edge: \breakedges@}}
\xydef@\testbreakedges@#1;#2,#3@{\bgroup \dimen@=#2\relax
 \advance\dimen@\splineval@ \advance\dimen@-\p@
\splinetrace@{testbreak: #1;#2,#3@ \the\splineval@::\the\dimen@}%
 \DN@{\egroup}\ifdim\dimen@>\z@
 \edef\next@{\egroup\def\noexpand\breakedges@{#1;1pt,#3}}%
 \else\ifdim\zz@\dimen@ 
 \edef\next@{\egroup\def\noexpand\breakedges@{#1;1pt,#3}}%
 \fi \fi \next@ }
\xydef@\splineRecordBreakEValue{%
 \ifdim\splineval@>\z@
 \splineval@=-\splineval@ \advance\splineval@\p@ \fi
 \splineRecordBreakValue@ }%
\xydef@\xydist@#1#2{\ifdim#1>#2\relax
 \quotient@@\tmp@#2#1\expandafter\dimen@ii\tmp@#2\relax
 \ifdim\dimen@ii>.41422#1\relax
 \dimen@=1.060665#1\advance\dimen@ .353555\dimen@ii\relax
 \else \dimen@=#1\advance\dimen@.5\dimen@ii\fi
 \else 
 \quotient@@\tmp@#1#2\expandafter\dimen@ii\tmp@#1\relax
 \ifdim\dimen@ii>.41422#2\relax
 \dimen@=1.060665#2\advance\dimen@ .353555\dimen@ii\relax
 \else \dimen@=#2\advance\dimen@.5\dimen@ii\fi
 \fi}
\xydef@\splineDadvance@{\splineadvance@@
 \expandafter\splineDadvance@@\splineDadvance@@@}
\xydef@\splineDadvance@@#1#2#3#4{%
 {\d@X=#1\advance\d@X-#2\ifdim\d@X<\z@ \d@X=-\d@X\fi 
 \d@Y=#3\advance\d@Y-#4\ifdim\d@Y<\z@ \d@Y=-\d@Y\fi
 \xydist@\d@X\d@Y 
 \global\advance\splinelength@\dimen@ 
\splinetrace@{d=(\the\d@X,\the\d@Y): v=\the\splineval@: l=\the\splinelength@}%
}}
\xydef@\spline@end@{\lastsplinepoint@ \egroup \egroup
 \ht\z@=\z@ \dp\z@=\z@ \wdz@=\z@ \boxz@}%
\gdef\splinetest@{\splineplot@true}
\xydef@\spline@end@@{\egroup \egroup}
\xydef@\splinefrec@{{%
 \advance\splineval@\splinedepth@
\splinetrace@{F:(\the\X@p,\the\Y@p);(\the\X@c,\the\Y@c);;
\the\splineval@;\the\splinedepth@}%
 \ifdim\dimen5=\splineval@ \aftergroup\splinefinishf@ 
 \else \dimen@=\dimen5\advance\dimen@-\splineval@
 \ifdim\dimen@<\z@ \dimen@=-\dimen@ \fi
 \ifdim\dimen@<.0001\p@ \aftergroup\splinefinishf@
 \else
 \ifdim\dimen5<\splineval@\aftergroup\splinedecast@@
 \else \aftergroup\splineadvance@ 
 \fi\fi\fi}}
\xydef@\splinefinishf@{\global\advance\splineval@\splinedepth@
 \splinefinish@}%
\xydef@\spline@find#1#2#3{%
\splinetrace@{spline@find #1 #2 #3}%
 \readsplineparams@
 \global\let\splinefinish@=\splinefinish@@
 \global\let\splinegoal@=\splinef@pt 
 \global\let\splinepoint=\relax
 \dimen@=#1\relax\dimen@ii=#2\relax
 \ifdim\dimen@ii=\z@ \def\postfind@{}%
 \else\def\postfind@{}%
 \ifdim\dimen@ii<\z@ \splinereverse@ 
 \readsplineparams@ 
\splinetrace@{reverse orientation: (\the\X@p,\the\Y@p),(\the\X@c,\the\Y@c)}%
 \dimen@=#1\relax\dimen@ii=#2\relax
 \multiply\dimen@\m@ne \advance\dimen@\p@ \multiply\dimen@ii\m@ne
 \def\postfind@{\d@X=-\the\d@X \d@Y=-\the\d@Y \noexpand\reversesplineval@}%
 \fi\fi
 \expandafter\splinetrace@\expandafter{\xysplineparams@}%
 \edef\next@{\noexpand\spline@@find{\the\dimen@}{\the\dimen@ii}{#3}}%
 \next@ }
\xydef@\reversesplineval@{\splineval@=-\splineval@ \advance\splineval@\p@ }
\xydef@\spline@@find#1#2#3{%
\splinetrace@{spline@@find #1 #2 #3}%
 \let\splinerec@=\splinefrec@ 
 \global\let\splineadvance@=\splineadvance@@
 \dimen5=#1\relax
 \ifdim #2=\z@\relax
 \ifdim #1=\z@\relax \bgroup 
 \let\splined@@=\spline@@knot
 \global\splineval@=\m@ne\p@ 
 \else\ifdim #1=\p@\relax \bgroup
 \let\splined@@=\spline@@knot 
 \global\splineval@=\z@ 
 \else 
 \global\splineval@=\z@ 
 \global\let\splineadvance@=\splineadvance@@
 \DN@{#3}\ifx\next@\empty \setsplinetest@\splineval@>{#1}{}%
 {{\ifdim\splineval@=\dimen5\aftergroup\splineplot@false\fi}}%
 \else\DNii@{>}\ifx\next@\nextii@
 \setsplineundertest@\splineval@>{#1}{}{}%
 \let\splinerec@=\splineBSrec@ 
 \else\DNii@{<}\ifx\next@\nextii@
 \setsplineundertest@\splineval@>{#1}{}{}%
 \let\splinerec@=\splineBErec@ 
 \else\xywarning@{unknown find-mode: #3}\fi\fi\fi
 \fi\fi
 \else 
 \global\splineval@=\z@ 
 \def\splineslidetest@@{%
 \setsplinetest@\splinelength@<{#2}{}{}}%
 \let\splinefinish@=\splinefcontinue@
 \fi
 \let\spline@end=\splinef@end
 \let\splinepoint@=\relax
 \splinelength@=\z@ 
 \def\spline@start{\bgroup\xylowtolerance@}%
 \splined@@ }
\xydef@\spline@@knot{%
 \let\setsplinedir@=\setsplineknotdir@
 \splinesetparams@\spline@start
 \splinedepth@=\p@
 \global\dimen@i=\X@p \global\dimen3=\Y@p 
 \splinefinishf@ \spline@end \egroup }
\xydef@\splinefcontinue@{%
\splinetrace@{sliding... from (\the\X@c,\the\Y@c): val=\the\splineval@ }%
 \global\let\splinerec@=\splinerec@@
 \global\splinelength@=\z@
 \global\splineval@=\splineval@
 \global\let\splinepoint=\splinefindtest@
 \global\let\splinegoal@=\splinef@pt 
 \global\let\splineadvance@=\splineDadvance@
 \global\let\splinefinish@=\splinefinish@@ 
 \splineslidetest@@ 
 }
\xydef@\splinefindtest@{%
\splinetrace@{SFT (\the\X@c,\the\Y@c); \the\splinelength@, \the\splineval@}%
 {\splineplot@false\splinetest@ 
 \ifsplineplot@\expandafter\splinefinishf@\fi}}
\def\setsplineundertest@#1#2#3#4#5{%
\splinetrace@{setsplineundertest@: #1,#2,#3,#4,#5,}%
 \DNii@{\gdef\splinetest@}%
 \DN@##1\next{\def\tmp@{{\splineplot@false 
 \ifdim#1#2##1\relax #4\else\splineplot@true#5\fi }}}%
 \next@#3\relax\next
 \expandafter\nextii@\tmp@ }
\xydef@\splinef@end{\edef\tmp@{\egroup\splinelength@=\the\splinelength@}\tmp@}
\xydef@\splinef@pt{%
 \ifdim\splineval@>\z@ 
\splinetrace@{found: val=\the\splineval@;c:(\the\X@c,\the\Y@c)}%
 \global\dimen@i=\X@c \global\dimen3=\Y@c 
 \else
\splinetrace@{found: val=\the\splineval@;p:(\the\X@p,\the\Y@p)}%
 \fi
 \setsplinedir@ \global\dimen5=\d@X \global\dimen7=\d@Y 
 \global\splineval@=\splineval@
 \aftergroup\splinefocus@ }
\def\setsplinetest@#1#2#3#4#5{%
 \DNii@{\gdef\splinetest@}%
 \DN@##1\next{\def\tmp@{{\splineplot@false \ifdim#1#2##1\relax
 #4\else\splineplot@true#5\fi}}}%
 \next@#3\relax\next
 \expandafter\nextii@\tmp@ }%
\xydef@\splinefocus@{%
 \d@X=\dimen5\relax \d@Y=\dimen7\relax \setsplinedir@ }
\xydef@\splinesegment@#1{}
\xydef@\xyprecurve@{}
\xydef@\xypostcurve@{}
\xydef@\splineset@{%
\splinetrace@{splineset@:}%
 \ifx\bstartPLACE@\empty
 \DN@{\xyprecurve@ 
 \edef\tmp@{\egroup \X@max=\the\X@max \X@min=\the\X@min
 \Y@max=\the\Y@max \Y@min=\the\Y@min}\tmp@ \xypostcurve@ }%
 \else
 \DN@{\xyprecurve@ \xysplinespecialcases@
 \edef\tmp@{\egroup \X@max=\the\X@max \X@min=\the\X@min
 \Y@max=\the\Y@max \Y@min=\the\Y@min}\tmp@ \xypostcurve@ }%
 \fi
 \next@ }
\xydef@\xysplinespecialcases@{%
 \ifx\empty\xycrvdrop@ 
 \ifx\empty\xycrvconn@ \DN@{\splinesolid@}%
 \else \DN@{ \dir{-}}\ifx\next@\xycrvconn@ \DN@{\splinesolid@}%
 \else \DN@{ \dir 2{-}}\ifx\next@\xycrvconn@ \DN@{\splinedoubled@}%
 \else \DN@{ \dir{=}}\ifx\next@\xycrvconn@ \DN@{\splineribboned@}%
 \else \DN@{ \dir {2.}}\ifx\next@\xycrvconn@ \DN@{\splinedoubled@}%
 \else \DN@{ \dir 3{-}}\ifx\next@\xycrvconn@ \DN@{\splinetrebled@}%
 \else \DN@{ \dir {3.}}\ifx\next@\xycrvconn@ \DN@{\splinetrebled@}%
 \else \DN@{ \dir{--}}\ifx\next@\xycrvconn@ \DN@{\splinedashed@}%
 \else \DN@{ \dir{.}}\ifx\next@\xycrvconn@ \DN@{\splinedotted@}%
 \else \DN@{ \dir{:}}\ifx\next@\xycrvconn@ \DN@{\splinedbldotted@}%
 \else \ifdim\splinetol@>\z@ \else \splinedefaulttol@ \fi
 \DN@{\splineset@@}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
 \else
 \DN@{\splineset@@}%
 \fi \ifInvisible@\DN@{}\fi \next@ }
\xydef@\splinesolid@{\setbox\splinebox@=\zerodot \def\xycrvdrop@{ }%
 \def\xycrvconn@{}\splineset@@}
\xydef@\splinedoubled@{\splinedefaulttol@\def\xycrvdrop@{ }\def\splinedrop@{}%
 \def\xycrvconn@{!C\dir2{.}}\splineset@@}
\xydef@\splineribboned@{\splinedefaulttol@\def\xycrvdrop@{ }\def\splinedrop@{}%
 \def\xycrvconn@{!C\dir{:}}\splineset@@}
\xydef@\splinetrebled@{\splinedefaulttol@\def\xycrvdrop@{ }\def\splinedrop@{}%
 \def\xycrvconn@{!C\dir3{.}}\splineset@@}
\xydef@\splinedashed@{\splinetol@=1.5pc \def\xycrvdrop@{ }%
 \def\splinedrop@{}\edef\xycrvconn@{\noexpand!C\noexpand\dir{\addDASH@{}}}%
 \splineset@@}
\xydef@\splinedotted@{\setbox\splinebox@=\zerodot \def\xycrvdrop@{ }%
 \splinetol@=1.5\jot \def\xycrvconn@{}\splineset@@}
\xydef@\splinedbldotted@{\def\xycrvdrop@{ }\def\splinedrop@{}%
 \splinetol@=1.5\jot \def\xycrvconn@{!C\dir{:}}\splineset@@}
\xydef@\splineset@@{%
 \readsplineparams@
 \ifx\xycrvdrop@\empty \splinetol@=7.5\p@
 \def\splinedefaulttol@{\splinetol@=7.5\p@}\def\splinedrop@{}%
 \else\edef\splinedefaulttol@{\splinetol@=\the\splinetol@}\fi
 \ifx\xycrvconn@\empty \def\splineconn@{}\fi
\splinetrace@{set the curve: >\the\dimen5, <\the\dimen7}%
 \global\let\splineadvance@=\splineadvance@@
 \let\splinerec@=\splineTrec@
 \def\splineStarttest{\splinetest@}%
 \global\let\splinepoint=\relax
 \let\spline@start=\spline@start@
 \let\spline@end=\spline@end@
 \ifdim\dimen7=\p@ 
 \gdef\splinecontinue{\splinesetting@
 \global\let\splinetest@=\splineplot@true}%
 \else
 \ifdim\dimen7=\tw@\p@
%% \ifdim\bendPLACE@\p@=\z@ \emptyspline@ \else
 \ifdim\bendPLACE@\p@=\p@
 \fi
 \else
 \xdef\splinecontinue{\noexpand\setsplinetest@
 \splineval@>{\the\dimen7}{\noexpand\splinebreakcancel@}{}%
 \noexpand\splinesetting@ }%
 \fi\fi
 \ifdim\dimen7>\z@ \DN@{\splinesetting@\splinecontinue}%
 \ifdim\zz@{\dimen5}%
 \else 
 \edef\next@{\noexpand\setsplinetest@
 \splineval@<{\the\dimen5}{}%
 {\noexpand\expandafter\noexpand\splinecontinue}%
 \noexpand\splinesetting@ }%
 \fi
 \else\DN@{\dimen5=\p@}\fi
 \next@
 \ifdim\dimen5=\p@\DN@{}\else\DN@{\splined@@}\fi \next@ 
 }
\xydef@\emptyspline@{\xywarning@{empty curve subsegment}%
\splinetrace@{bstartPLACE@=\bstartPLACE@, bendPLACE@=\bendPLACE@, 
 empty segment}%
 \gdef\splinecontinue{\splinesetting@
 \global\let\splinetest@=\splineplot@false
 \global\dimen5=\z@ }}
\xydef@\splineTrec@{{%
 \advance\splineval@\splinedepth@
 \ifdim\dimen5=\splineval@
 \aftergroup\splinecontinue
 \else \dimen@=\dimen5\advance\dimen@-\splineval@
 \ifdim\dimen@<\z@ \dimen@=-\dimen@ \fi
 \ifdim\dimen@<.001\p@
 \aftergroup\splinecontinue
 \else
 \ifdim\dimen5<\splineval@\aftergroup\splinedecast@@
 \else \aftergroup\splineadvance@
 \fi\fi\fi}}
\xydef@\splinesetting@{\splinesetting@@}
\xydef@\splinesetting@@{%
\splinetrace@{splinesetting@@:}%
 \ifdim\splinedepth@=\z@ \splinedepth@=\p@ \fi
 \ifdim\splinedepth@=\p@
 \def\splinerec@{\global\let\splinerec@=\splinerec@@\splinedecast@@}%
 \else \global\let\splinerec@=\splinerec@@ \fi
 \gdef\splinepoint{\splineplotpt@}}
\xydef@\splineplotpt@{{\global\advance\dimen@i-\X@c 
 \splinetest@ \DN@{\splineglue@}\ifsplineplot@ 
 \DN@{\dosplineplotpt@}%
 \fi \next@ \global\dimen@i=\X@c \global\dimen3=\Y@c }}
\xydef@\splineglue@{\hglue-\dimen@i
\splinetrace@{N:(\the\X@c,\the\Y@c);;\the\dimen@i;\the\dimen3%
 ,\the\splinelength@,\the\splineval@,\the\splinedepth@}}
\xydef@\dosplineplotpt@{\ifdim\dimen@i<\z@
 \raise\Y@c\hbox to-\dimen@i{\hfill\splinedrop@}%
 \else \kern-\dimen@i\raise\Y@c\hbox{\splinedrop@}\fi
 \ifx\splineconn@\relax\else\raise\Y@c\hbox{%
 \setboxz@h{\splineconn@}\Drop@@}\fi
\splinetrace@{P:(\the\X@c,\the\Y@c);;\the\dimen@i;\the\dimen3
 ,\the\splinelength@,\the\splineval@,\the\splinedepth@}}
\xydef@\splinefinish@@{\postspline@ \splinegoal@ \splinecancel@ }
\xydef@\splinecancel@{%
 \global\let\splinerec@=\relax
 \global\let\splinepoint=\relax 
 \global\let\splinecontinue=\relax
 \global\let\splinedecast@=\relax
 }
\xydef@\splinebreakcancel@{\bsplinecancel@ \splinecancel@}
\xydef@\bsplinecancel@{\gdef\lastbspline@{\leave@\leave@}%
 \global\let\middlebspline@=\lastbspline@ }
\xydef@\splinegoal@{\ifdim\splineval@>\z@
 \global\dimen@i=\X@c \global\dimen3=\Y@c \fi
 \global\splineval@=\splineval@ \global\splinelength@=\splinelength@
 \splinesetdir@ }
\xylet@\splinefinish@\splinefinish@@
\xylet@\splinewhich\splineDwhich@
\xydef@\squinewhich@{%
 \ifdim\dimen5>\squinelength
 \d@X=\X@c \d@Y=\Y@c \advance\d@X-\L@c \advance\d@Y-\U@c 
 \advance\squineval-\squinedepth 
 \else \X@c=\X@p \Y@c=\Y@p \advance\squineval-\squinedepth
 \d@X=\L@c \d@Y=\U@c \advance\d@X-\X@p \advance\d@Y-\Y@p \fi
 \d@X=-\d@X \d@Y=-\d@Y
 \squinefinish}
\xydef@\squineDwhich@{%
 \ifdim\dimen5>\squinelength
 \d@X=\X@c \d@Y=\Y@c \advance\d@X-\L@c \advance\d@Y-\U@c 
 \else \X@c=\X@p \Y@c=\Y@p \advance\squineval-\squinedepth
 \d@X=\L@c \d@Y=\U@c \advance\d@X-\X@p \advance\d@Y-\Y@p \fi
 \d@X=-\d@X \d@Y=-\d@Y
 \squinefinish}
\xydef@\xyquadbezier@{%
 \global\let\splinerec@=\relax
 \addtocrvpts@{\def\crvconnect@{\squineconnect@}}%
 \xyquadmethods@ \let\splinesegment@=\squinesegment@
 \begingroup\setcrvobjects@ \xysplineparams@ \splined@@@
 \bgroup \setupsquine@ \squined@ \splineset@ \savespline@ }
\xydef@\xyquadmethods@{%
 \def\crvconnect@{\squineconnect@}%
 \def\splinereverse@@{\splinereverse@@@}%
 \let\getsplineparams@=\getsquineparams@
 \let\spline@start@=\squine@start@
 \let\splinedecast@@=\squinedecast@
 \let\splinerec@@=\squinerec@
 \let\splined@@=\squined@@
 \let\splineIpt@@=\squineIpt@
 \let\splineIadvance@@=\squineIadvance@
 \let\splineinfo@=\squineinfo@
 \let\setsplinedir@=\setsquinedir@
 \let\splinetestcvxhull@=\squinetestcvxhull@
 \let\setsplineknotdir@=\setsquineknotdir@
 \let\splinereverse@=\squinereverse@
 \let\splineDadvance@@@=\squineDadvance@@@
 \let\splinesetparams@=\squinesetparams@
 \let\splineplot@maybe@@=\squineplot@maybe
}
\xydef@\squineconnect@{\splineconnect@ \crvconnect@@ 
 \let\splinesegment@=\squinesegment@ }%
\xydef@\squinesegment@#1{\xyquadmethods@ \def\segmentnum@{1}%
 \setupsquine@ \squined@ }
\xydef@\setupsquine@{%
 \xycontrolpt@\z@ \X@p=\X@c \Y@p=\Y@c
 \xycontrolpt@\@ne \A@=\X@c \B@=\Y@c 
 \xycontrolpt@\tw@ 
 \ifdim \A@>\X@max
 \dimen@=\X@p\advance\dimen@\A@ \dimen@half
 \ifdim \dimen@>\X@max \X@max=\dimen@ \fi
 \dimen@=\X@c\advance\dimen@\A@ \dimen@half
 \ifdim \dimen@>\X@max \X@max=\dimen@ \fi
 \else \ifdim \A@<\X@min 
 \dimen@=\X@p\advance\dimen@\A@ \dimen@half
 \ifdim \dimen@<\X@min \X@min=\dimen@ \fi
 \dimen@=\X@c\advance\dimen@\A@ \dimen@half
 \ifdim \dimen@>\X@min \X@min=\dimen@ \fi
 \fi\fi
 \ifdim \B@>\Y@max 
 \dimen@=\Y@p\advance\dimen@\B@ \dimen@half
 \ifdim \dimen@>\Y@max \Y@max=\dimen@ \fi
 \dimen@=\Y@c\advance\dimen@\B@ \dimen@half
 \ifdim \dimen@>\Y@max \Y@max=\dimen@ \fi
 \else \ifdim \B@<\Y@min
 \dimen@=\Y@p\advance\dimen@\B@ \dimen@half
 \ifdim \dimen@<\Y@min \Y@min=\dimen@ \fi
 \dimen@=\Y@c\advance\dimen@\B@ \dimen@half
 \ifdim \dimen@>\Y@min \Y@min=\dimen@ \fi
 \fi\fi }
\xydef@\squinedecast@{\halve@dimen\splinedepth@
 \R@c=\L@c \advance\L@c\X@p \halve@dimen\L@c
 \advance\R@c\X@c \halve@dimen\R@c
 \A@=\L@c \advance\A@\R@c \halve@dimen\A@
 \D@c=\U@c \advance\U@c\Y@p \halve@dimen\U@c
 \advance\D@c\Y@c \halve@dimen\D@c
 \B@=\U@c \advance\B@\D@c \halve@dimen\B@
 \begingroup \X@c=\A@ \Y@c=\B@ \splinerec@ \endgroup
 \begingroup \X@c=\A@ \Y@c=\B@ \splinepoint \endgroup
 \X@p=\A@ \L@c=\R@c \Y@p=\B@ \U@c=\D@c \splinerec@}
\xydef@\squinerec@{{\splinefar@false \splinenear@\X@p\X@c\Y@p\Y@c 
 \ifsplinefar@ \aftergroup\squinedecast@ 
 \else \aftergroup\splineadvance@ \fi}}
\xydef@\squineDadvance@@@{\X@p\L@c\Y@p\D@c}
\xydef@\squineplot@maybe{{\X@p=\L@c \Y@p=\U@c \cv@start \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}
\xydef@\setsquinedir@{%
 \d@X=\X@c \advance\d@X-\L@c \d@Y=\Y@c \advance\d@Y-\U@c 
 \dimen@=\ifdim\d@X<\z@-\fi\d@X \ifdim\dimen@<.02\p@
 \dimen@=\ifdim\d@Y<\z@-\fi\d@Y \ifdim\dimen@<.02\p@ 
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p \fi\fi
 \ifdim\X@c=\X@p \ifdim\Y@c=\Y@p 
 \d@X=\L@c \advance\d@X-\X@p \d@Y=\U@c \advance\d@Y-\Y@p \fi\fi
 \setupDirection@ii } 
\xydef@\setsquineknotdir@{%
 \ifdim\zz@\splineval@ \expandafter \setsquinezerodir@
 \else\expandafter \setsquinedir@ \fi } 
\xydef@\setsquinezerodir@{%
 \d@X=\L@c \advance\d@X-\X@p \d@Y=\U@c \advance\d@Y-\Y@p 
 \ifdim\zz@\d@X \ifdim\zz@\d@Y 
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p 
 \fi\fi \setupDirection@ii }
\xydef@\getsquineparams@#1,#2,#3,#4,#5,#6,#7,{%
 \splinelength@=#1\relax\X@p=#2\relax\Y@p=#3\relax
 \A@=#4\relax\B@=#5\relax\X@c=#6\relax\Y@c=#7\relax
}
\xydef@\squineinfo@{%
\expandafter\removePT@\the\X@c\space
\expandafter\removePT@\the\Y@c\space
\expandafter\removePT@\the\A@\space
\expandafter\removePT@\the\B@\space
\expandafter\removePT@\the\X@p\space
\expandafter\removePT@\the\Y@p\space
\expandafter\removePT@\the\dimen5\space\space
\expandafter\removePT@\the\dimen7\space
 }%
\xydef@\squinereverse@{\readsplineparams@
 \expandafter\edef\xysplineparams@{\the\splinelength@,%
 \the\X@c,\the\Y@c,\the\A@,\the\B@,\the\X@p,\the\Y@p,}}%
\xydef@\squine@start@{\setboxz@h\bgroup
 \global\splinelength@=\z@ \global\dimen@i=\z@ \global\dimen3=\z@
 \kern\X@p
 {\squinesetparams@ \X@c=\X@p \Y@c=\Y@p \firstsplinepoint@
 }\bgroup }
\xydef@\squinesetparams@{%
 \global\dimen@i=\X@p \global\dimen3=\Y@p 
 \L@c=\A@ \U@c=\B@ \R@c=\L@c \D@c=\U@c }%
\xydef@\squined@{%
 \expandafter\edef\xysplineparams@{%
 \the\z@,\the\X@p,\the\Y@p,\the\A@,\the\B@,\the\X@c,\the\Y@c,}}
\xydef@\squined@@{%
 \splinedepth@=\p@ 
 \global\splineval@=\z@ 
 \global\dimen@i=\X@p \global\dimen3=\Y@p
 \spline@start 
 \ifx\splinerec@\relax \let\splinerec@=\squinerec@\fi
 \L@c=\A@ \U@c=\B@ \R@c=\L@c \D@c=\U@c 
 \splinerec@ \spline@end }
\xydef@\xycubicbezier@{%
 \addtocrvpts@{\def\crvconnect@{\cubicconnect@}}%
 \xycubicmethods@ \let\splinesegment@=\cubicsegment@
 \begingroup \setcrvobjects@ \xysplineparams@ \splined@@@ 
 \bgroup \setupcubic@ \cubiced@ \splineset@ \savespline@ }
\xydef@\xycubicmethods@{%
 \def\crvconnect@{\cubicconnect@}%
 \def\splinereverse@@{\cubicreverse@@}%
 \let\getsplineparams@=\getcubicparams@
 \let\spline@start@=\cubic@start@
 \let\splinedecast@@=\cubicdecast@
 \let\splinerec@@=\cubicrec@
 \let\splined@@=\cubiced@@
 \let\splineIpt@@=\cubicIpt@
 \let\splineIadvance@@=\cubicIadvance@
 \let\splineoutsidehull@@=\cubicoutsidehull@
 \let\splinetestcvxhull@=\cubictestcvxhull@
 \let\splineinfo@=\cubicinfo@
 \let\setsplinedir@=\setcubicdir@
 \let\setsplineknotdir@=\setcubicknotdir@
 \let\splinereverse@=\cubicreverse@ 
 \let\splineDadvance@@@=\cubicDadvance@@@
 \let\splinesetparams@=\cubicsetparams@
 \let\splineplot@maybe@@=\cubicplot@maybe
 }
\xydef@\cubicconnect@{\splineconnect@ \crvconnect@@
 \let\splinesegment@=\cubicsegment@ }%
\xydef@\cubicsegment@#1{\xycubicmethods@ \def\segmentnum@{1}%
 \setupcubic@ \cubiced@ }
\xydef@\setupcubic@{%
 \xycontrolpt@\z@ \X@p=\X@c \Y@p=\Y@c
 \xycontrolpt@\@ne \A@=\X@c \B@=\Y@c 
 \xycontrolpt@\tw@ \global\dimen3=\X@c \global\dimen5=\Y@c
 \xycontrolpt@\thr@@ 
 \adjustmaxmin@ }
\xydef@\adjustmaxmin@{%
 \ifdim \A@>\X@max \dimen@=\A@ \advance\dimen@\X@p \dimen@half 
 \ifdim\dimen@>\X@max \X@max=\dimen@ \fi \else
 \ifdim \A@<\X@min \dimen@=\A@ \advance\dimen@\X@p \dimen@half 
 \ifdim\dimen@<\X@min \X@min=\dimen@ \fi \fi\fi
 \ifdim \B@>\Y@max \dimen@=\B@ \advance\dimen@\Y@p \dimen@half 
 \ifdim\dimen@>\Y@max \Y@max=\dimen@ \fi \else
 \ifdim \B@<\Y@min \dimen@=\B@ \advance\dimen@\Y@p \dimen@half 
 \ifdim\dimen@<\Y@min \Y@min=\dimen@ \fi \fi\fi
 \ifdim \dimen3>\X@max \dimen@=\dimen3\advance\dimen@\X@c \dimen@half 
 \ifdim\dimen@>\X@max \X@max=\dimen@ \fi \else
 \ifdim \dimen3<\X@min \dimen@=\dimen3\advance\dimen@\X@c \dimen@half 
 \ifdim\dimen@<\X@min \X@min=\dimen@ \fi \fi\fi
 \ifdim \dimen5>\Y@max \dimen@=\dimen5\advance\dimen@\Y@c \dimen@half 
 \ifdim\dimen@>\Y@max \Y@max=\dimen@ \fi \else
 \ifdim \dimen5<\Y@min \dimen@=\dimen5\advance\dimen@\Y@c \dimen@half 
 \ifdim\dimen@<\Y@min \Y@min=\dimen@ \fi \fi\fi
 \dimen@=\A@ \advance\dimen@\dimen3 \dimen@half
 \ifdim\dimen@>\X@max \X@max=\dimen@
 \else \ifdim\dimen@<\X@min \X@min=\dimen@ \fi\fi
 \dimen@=\B@ \advance\dimen@\dimen5 \dimen@half
 \ifdim\dimen@>\Y@max \Y@max=\dimen@
 \else \ifdim\dimen@<\Y@min \Y@min=\dimen@ \fi\fi
}
\xydef@\cubicdecast@{\halve@dimen\splinedepth@
 \A@=\L@c \advance\A@\R@c \halve@dimen\A@
 \advance\R@c\X@c \halve@dimen\R@c
 \B@=\U@c \advance\B@\D@c \halve@dimen\B@
 \advance\D@c\Y@c \halve@dimen\D@c
 \advance\L@c\X@p \halve@dimen\L@c
 \advance\U@c\Y@p \halve@dimen\U@c
 \begingroup 
 \X@c=\R@c \advance\X@c\L@c \halve@dimen\X@c
 \advance\X@c\A@ \halve@dimen\X@c
 \Y@c=\D@c \advance\Y@c\U@c \halve@dimen\Y@c
 \advance\Y@c\B@ \halve@dimen\Y@c
 \R@c=\L@c \advance\R@c\A@ \halve@dimen\R@c
 \D@c=\U@c \advance\D@c\B@ \halve@dimen\D@c
 \bgroup \splinerec@ 
 \egroup \splinepoint \endgroup 
 \X@p=\L@c \advance\X@p\R@c \halve@dimen\X@p
 \advance\X@p\A@ \halve@dimen\X@p
 \L@c=\R@c \advance\L@c\A@ \halve@dimen\L@c
 \Y@p=\U@c \advance\Y@p\D@c \halve@dimen\Y@p
 \advance\Y@p\B@ \halve@dimen\Y@p
 \U@c=\D@c \advance\U@c\B@ \halve@dimen\U@c
 \splinerec@ }
\xydef@\cubicrec@{{\splinefar@false \splinenear@\X@p\X@c\Y@p\Y@c 
 \ifsplinefar@ \aftergroup\cubicdecast@
 \else \aftergroup\splineadvance@ \fi}}
\xydef@\cubicDadvance@@@{\X@p\X@c\Y@p\Y@c}
\xydef@\cubicplot@maybe{{\X@p=\L@c \Y@p=\U@c \cv@start \the\Edge@c\@ne 
 \ifInside@\aftergroup\cubicplot@maybeii\else\aftergroup\splineplot@true\fi}}
\xydef@\cubicplot@maybeii{{\X@p=\R@c \Y@p=\D@c \cv@start \the\Edge@c\@ne 
 \ifInside@\aftergroup\splineplot@false\else\aftergroup\splineplot@true\fi}}
\xydef@\cubiced@@{%
 \splinedepth@=\p@ 
 \global\splineval@=\z@ 
 \spline@start 
 \global\dimen@i=\X@p \global\dimen3=\Y@p
 \splinerec@ \spline@end }
\xydef@\setcubicdir@{%
 \ifdim\splinedepth@<.001\p@\DN@{\cubiccoarsedir@}%
 \else\DN@{\cubicfinedir@}\fi \next@ }
\xydef@\cubicfinedir@{%
 \d@X=\X@c \advance\d@X-\R@c \d@Y=\Y@c \advance\d@Y-\D@c 
 \ifdim\zz@\d@X \ifdim\zz@\d@Y 
 \d@X=\X@c \advance\d@X-\L@c \d@Y=\Y@c \advance\d@Y-\U@c 
 \ifdim\zz@\d@X \ifdim\zz@\d@Y 
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p 
 \fi\fi \fi\fi
 \setupDirection@ii 
\splinetrace@{dir:(\the\d@X,\the\d@Y),\the\Direction; depth:\the\splinedepth@}%
} 
\xydef@\cubiccoarsedir@{%
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p \setupDirection@ii
 \global\dimen5=\d@X \global\dimen7=\d@Y
\splinetrace@{dir:(\the\d@X,\the\d@Y),\the\Direction; depth:\the\splinedepth@}%
}
\xydef@\setcubicknotdir@{%
 \ifdim\zz@\splineval@ \DN@{\setcubiczerodir@}%
 \else \DN@{\cubicfinedir@}\fi \next@ } 
\xydef@\setcubiczerodir@{%
 \d@X=\L@c \advance\d@X-\X@p \d@Y=\U@c \advance\d@Y-\Y@p 
 \ifdim\zz@\d@X \ifdim\zz@\d@Y 
 \d@X=\R@c \advance\d@X-\X@p \d@Y=\D@c \advance\d@Y-\Y@p 
 \ifdim\zz@\d@X \ifdim\zz@\d@Y 
 \d@X=\X@c \advance\d@X-\X@p \d@Y=\Y@c \advance\d@Y-\Y@p 
 \fi\fi \fi\fi \setupDirection@ii }
\xydef@\getcubicparams@#1,#2,#3,#4,#5,#6,#7,#8,#9,{%
 \splinelength@=#1\relax\X@p=#2\relax\Y@p=#3\relax\L@c=#4\relax
 \U@c=#5\relax\R@c=#6\relax\D@c=#7\relax\X@c=#8\relax\Y@c=#9\relax
}%
\xydef@\cubicinfo@{%
\expandafter\removePT@\the\X@p\space
\expandafter\removePT@\the\Y@p\space
\expandafter\removePT@\the\L@c\space
\expandafter\removePT@\the\U@c\space
\expandafter\removePT@\the\R@c\space
\expandafter\removePT@\the\D@c\space
\expandafter\removePT@\the\X@c\space
\expandafter\removePT@\the\Y@c\space
\expandafter\removePT@\the\dimen5\space\space
\expandafter\removePT@\the\dimen7\space
 }%
\xydef@\cubicreverse@{\readsplineparams@
 \expandafter\edef\xysplineparams@{\the\splinelength@,%
 \the\X@c,\the\Y@c,\the\R@c,\the\D@c,\the\L@c,\the\U@c,\the\X@p,\the\Y@p,}}%
\xydef@\cubicreverse@@{%
 \splinereverse@@@ 
 \dimen@ii=\L@c \L@c=\R@c \R@c=\dimen@ii 
 \dimen@ii=\U@c \U@c=\D@c \D@c=\dimen@ii }
\xydef@\cubic@start@{\setboxz@h\bgroup
 \global\splinelength@=\z@ \global\dimen@i=\z@ \global\dimen3=\z@
 \kern\X@p
 {\cubicsetparams@ \X@c=\X@p \Y@c=\Y@p \R@c=\X@c \D@c=\Y@c
 \firstsplinepoint@ }\bgroup 
}
\xydef@\cubicsetparams@{%
 \expandafter\expandafter\expandafter\getsplineparams@\xysplineparams@
 \global\dimen@i=\X@p \global\dimen3=\Y@p }
\xydef@\cubiced@{%
 \expandafter\edef\xysplineparams@{\the\z@,\the\X@p,\the\Y@p
 ,\the\A@,\the\B@,\the\dimen3,\the\dimen5,\the\X@c,\the\Y@c,}%
 }%
\xydef@\xybspline@iii{%
 \addtocrvpts@{\def\crvconnect@{\bsplineiiiconnect@}}%
 \def\crvconnect@{\bsplineiiiconnect@}\xybsplinemethods@ 
 \let\splinesegment@=\bsplinesegment@iii
 \begingroup\setcrvobjects@ \dobspline@ \savespline@ }
\xydef@\bsplineiiiconnect@{\splineconnect@ \crvconnect@@
 \let\splinesegment@=\bsplinesegment@iii }%
\xydef@\xybspline@iv{%
 \addtocrvpts@{\def\crvconnect@{\bsplineivconnect@}}%
 \def\crvconnect@{\bsplineivconnect@}\xybsplinemethods@
 \let\splinesegment@=\bsplinesegment@iv
 \begingroup\setcrvobjects@ \dobspline@ \savespline@ }
\xydef@\bsplineivconnect@{\splineconnect@ \crvconnect@@
 \let\splinesegment@=\bsplinesegment@iv }%
\xydef@\xybspline@{%
\splinetrace@{B-spline with \numcontrolpts\space control points.}%
 \addtocrvpts@{\def\crvconnect@{\bsplineconnect@}}%
 \def\crvconnect@{\bsplineconnect@}\xybsplinemethods@ 
 \let\splinesegment@=\bsplinesegment@ 
 \begingroup\setcrvobjects@
 \dobspline@ \savespline@ }
\xydef@\xybsplinemethods@{%
 \def\splinereverse@@{\cubicreverse@@}%
 \let\getsplineparams@=\getbsplineparams@
 \let\spline@start@=\cubic@start@
 \let\splinedecast@@=\cubicdecast@
 \let\splinerec@@=\cubicrec@
 \let\splineIpt@@=\cubicIpt@
 \let\splineIadvance@@=\cubicIadvance@
 \let\splined@@=\bsplined@@
 \let\splineinfo@=\cubicinfo@
 \let\setsplinedir@=\setcubicdir@
 \let\setsplineknotdir@=\setcubicknotdir@
 \let\splinereverse@=\cubicreverse@ 
 \let\splineDadvance@@@=\cubicDadvance@@@
 \let\splinesetparams@=\cubicsetparams@
 \global\let\lastbspline@=\lastbspline@@
 \global\let\middlebspline@=\middlebspline@@
}
\xydef@\bsplined@@{%
 \splinedepth@=\p@ 
 \global\splineval@=\z@ 
 \spline@start 
 \global\dimen@i=\X@p \global\dimen3=\Y@p
 \splinerec@ \spline@end }
\xydef@\bsplineconnect@{\splineconnect@ \crvconnect@@
 \let\splinesegment@=\bsplinesegment@ }%
\xydef@\getbsplineparams@{\getcubicparams@}
\xydef@\dobspline@{\xysplineparams@ \scanbspline@ \firstbspline@ }%
\xydef@\firstbspline@{%
 \enter@{\pfromthep@ \cfromthec@}\enter@{\cfromthec@}\bgroup
 \def\segmentnum@{1}\xycontrolpt@\z@ \X@p=\X@c \Y@p=\Y@c
\splinetrace@{0: \the\X@p, \the\Y@p}%
 \xycontrolpt@\@ne \A@=\X@c \B@=\Y@c 
\splinetrace@{1: \the\X@c, \the\Y@c}%
 \xycontrolpt@\tw@ 
\splinetrace@{2: \the\X@c, \the\Y@c}%
 \dimen@=\X@c \advance\dimen@\A@ \dimen@half
 \global\dimen3=\dimen@
 \dimen@=\Y@c \advance\dimen@\B@ \dimen@half
 \global\dimen5=\dimen@
 \xycontrolpt@{3}%
\splinetrace@{3: \the\X@c, \the\Y@c}%
 \expandafter\count@\xycrvcnt@\relax
 \ifnum\count@=3\relax 
 \advance\X@c-\A@ \dimen@nth4\X@c
 \advance\X@c\dimen3\relax
 \advance\Y@c-\B@ \dimen@nth4\Y@c
 \advance\Y@c\dimen5\relax
 \enter@{\X@p=\the\X@c \Y@p=\the\Y@c \crv@cnt@=\@ne\relax
 \noexpand\lastbspline@ }%
 \else 
 \advance\X@c 7\dimen3 \advance\X@c-2\A@ 
 \dimen@nth6\X@c
 \advance\Y@c 7\dimen5 \advance\Y@c-2\B@ 
 \dimen@nth6\Y@c
 \enter@{\X@p=\the\X@c \Y@p=\the\Y@c \crv@cnt@=\@ne\relax
 \noexpand\middlebspline@ }%
 \fi \adjustmaxmin@ \czeroEdge@
 \bsplined@ \splineset@ \leave@ }
\xydef@\lastbspline@@{\bgroup 
 \advance\crv@cnt@\@ne \edef\segmentnum@{\the\crv@cnt@}%
\splinetrace@{<: \the\X@p, \the\Y@p}%
 \advance\crv@cnt@\@ne \xycontrolpt@{\crv@cnt@}%
 \global\dimen3=\X@c \global\dimen5=\Y@c
\splinetrace@{\the\crv@cnt@: \the\X@c, \the\Y@c}%
 \advance\crv@cnt@\m@ne \xycontrolpt@{\crv@cnt@}%
\splinetrace@{\the\crv@cnt@: \the\X@c, \the\Y@c}%
 \A@=\X@c \advance\A@\dimen3 \halve@dimen\A@
 \B@=\Y@c \advance\B@\dimen5 \halve@dimen\B@
 \adjustmaxmin@ \leave@ \relax \cv@end
\splinetrace@{>: \the\X@c, \the\Y@c}%
 \bsplined@ \splineset@ \leave@ }%
\xylet@\lastbspline@=\lastbspline@@
\xydef@\middlebspline@@{%
 \advance\crv@cnt@\@ne \edef\segmentnum@{\the\crv@cnt@}%
\splinetrace@{<: \the\X@p, \the\Y@p}%
 \bgroup 
 \xycontrolpt@{\crv@cnt@}\A@=2\X@c \B@=2\Y@c
\splinetrace@{\the\crv@cnt@: \the\X@c, \the\Y@c}%
 \advance\crv@cnt@\@ne \xycontrolpt@{\crv@cnt@}%
\splinetrace@{\the\crv@cnt@: \the\X@c, \the\Y@c}%
 \advance\A@\X@c \dimen@nth3\A@
 \advance\B@\Y@c \dimen@nth3\B@
 \advance\X@c\A@ \halve@dimen\X@c
 \advance\Y@c\B@ \halve@dimen\Y@c
 \global\dimen3=\X@c \global\dimen5=\Y@c 
 \advance\crv@cnt@\@ne \xycontrolpt@{\crv@cnt@}%
\splinetrace@{\the\crv@cnt@: \the\X@c, \the\Y@c}%
 \expandafter\count@\xycrvcnt@\relax 
 \ifnum\crv@cnt@<\count@\relax 
 \advance\X@c 7\dimen3\advance\X@c-2\A@
 \dimen@nth6\X@c
 \advance\Y@c 7\dimen5\advance\Y@c-2\B@
 \dimen@nth6\Y@c
 \enter@{\X@p=\the\X@c \Y@p=\the\Y@c \crv@cnt@=\segmentnum@\relax
 \noexpand\middlebspline@}%
 \else 
 \advance\X@c-\A@ \dimen@nth4\X@c
 \advance\X@c \dimen3\relax
 \advance\Y@c-\B@ \dimen@nth4\Y@c
 \advance\Y@c \dimen5\relax
 \enter@{\X@p=\the\X@c \Y@p=\the\Y@c \noexpand\lastbspline@}%
 \fi \adjustmaxmin@ 
 \bsplined@ \splineset@ \leave@ } 
\xylet@\middlebspline@=\middlebspline@@
\xydef@\scanbspline@{\splined@@@}
\xydef@\bsplined@{\cubiced@ 
 \expandafter\ifx\xysplineedges@\relax\relax\DN@{}%
 \else\DN@{\adjustbsplineedges@}\fi \next@ }
\xydef@\adjust@forsegments@{\getcrvsegsnum@ 
 \ifnum\count@>\@ne
\splinetrace@{adjust for \the\count@\space segments:
 \the\dimen5, \the\dimen7}%
 \multiply\dimen5 by \count@\relax \dimen@=\segmentnum@\p@
 \ifnum\dimen5>\dimen@ \relax\dimen5=\p@
 \else \advance\dimen5-\segmentnum@\p@ \advance\dimen5 by\p@ \fi
 \ifnum\dimen5<\z@ \relax\dimen5=\z@\relax\fi
 \multiply\dimen7 by \count@\relax
 \dimen@=\segmentnum@\p@
 \ifnum\dimen7<\dimen@ \advance\dimen@-\p@
 \ifnum\dimen7>\dimen@ \advance\dimen7-\dimen@
 \else \dimen7=\z@ \fi
 \else \dimen7=\p@ \fi
\splinetrace@{adjusted for \the\count@\space segments:
 \the\dimen5, \the\dimen7}%
 \fi}
\xydef@\adjustbsplineedges@{\bgroup
\splinetrace@{** adjusting edges **}%
 \readsplineparams@ \adjust@forsegments@
\splinetrace@{params:\xysplineparams@}%
\splinetrace@{segment \segmentnum@:<\the\dimen5,\the\dimen7>:\xysplineedges@}%
 \multiply\dimen7by\m@ne \advance\dimen7by\p@
 \expandafter\edef\xysplineedges@{%
 \noexpand\z@;\the\dimen5,\noexpand\z@;\the\dimen7,}%
 \edef\tmp@{\egroup 
 \noexpand\def\expandafter\noexpand\xysplineedges@{\xysplineedges@}}%
 \tmp@ }
\xydef@\bsegment@@ii@iii{%
 \xycontrolpt@{\count@@}\global\dimen3=\X@c \global\dimen5=\Y@c
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \advance\count@@\@ne \xycontrolpt@{\count@@}\A@=\X@c \B@=\Y@c
 \advance\A@ by2\dimen3 \dimen@nth3\A@
 \advance\B@ by2\dimen5 \dimen@nth3\B@
 \dimen@=\dimen3 \advance\dimen@ by2\X@c
 \dimen@nth3\dimen@
 \global\dimen3=\dimen@
 \dimen@=\dimen5 \advance\dimen@ by2\Y@c
 \dimen@nth3\dimen@
 \global\dimen5=\dimen@
\splinetrace@{<: \the\dimen3, \the\dimen5}%
\splinetrace@{>: \the\A@, \the\B@}%
 \advance\count@@\m@ne }
\xydef@\bsegment@@i{\bgroup
 \advance\count@@\m@ne \xycontrolpt@{\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \edef\tmp@{\egroup \X@p=\the\X@c \Y@p=\the\Y@c}\tmp@
 \advance\X@p-2\dimen3\advance\X@p by7\A@
 \dimen@nth6\X@p
 \advance\Y@p-2\dimen5\advance\Y@p by7\B@ 
 \dimen@nth6\Y@p
}
\xydef@\bsegment@@iv{%
 \advance\count@@\tw@ \xycontrolpt@{\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \advance\X@c by7\dimen3\advance\X@c-2\A@ 
 \dimen@nth6\X@c
 \advance\Y@c by7\dimen5\advance\Y@c-2\B@ 
 \dimen@nth6\Y@c
\splinetrace@{>>: \the\X@c, \the\Y@c }%
}
\xydef@\bsegment@@ii@i{\bgroup
 \advance\count@@\m@ne \xycontrolpt@{\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \edef\tmp@{\egroup \X@p=\the\X@c \Y@p=\the\Y@c}\tmp@
 \advance\X@p-\dimen3\advance\X@p by4\A@ 
 \dimen@nth4\X@p
 \advance\Y@p-\dimen5\advance\Y@p by4\B@ 
 \dimen@nth4\Y@p
\splinetrace@{<<: \the\X@p, \the\Y@p}%
}
\xydef@\bsegment@@y@iv{%
 \advance\count@@\tw@ \xycontrolpt@{\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \advance\X@c by4\dimen3\advance\X@c-\A@ 
 \dimen@nth4\X@c
 \advance\Y@c by4\dimen5\advance\Y@c-\B@ 
 \dimen@nth4\Y@c
}
\xydef@\bsegment@i{%
 \xycontrolpt@\z@ \X@p=\the\X@c \Y@p=\the\Y@c
\splinetrace@{0: \the\X@p \the\Y@p}%
 \xycontrolpt@\@ne
\splinetrace@{1: \the\X@c, \the\Y@c}\A@=\X@c \B@=\Y@c 
 \xycontrolpt@\tw@
 \dimen@=\X@c \advance\dimen@\A@ \dimen@half
 \global\dimen3=\dimen@
\splinetrace@{2: \the\X@c, \the\Y@c}%
 \dimen@=\Y@c \advance\dimen@\B@ \dimen@half
 \global\dimen5=\dimen@ }
\xydef@\bsegment@i@iv{%
 \xycontrolpt@{3}%
\splinetrace@{3: \the\X@c, \the\Y@c}%
 \advance\X@c by7\dimen3\advance\X@c-2\A@ 
 \dimen@nth6\X@c
 \advance\Y@c by7\dimen5\advance\Y@c-2\B@ 
 \dimen@nth6\Y@c
 }
\xydef@\bsegment@z{%
 \expandafter\count@@\xycrvptsnum@ \advance\count@@\@ne 
 \xycontrolpt@{\the\count@@}\relax
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \advance\count@@\m@ne
 \bgroup
 \xycontrolpt@{\the\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \global\dimen3=\X@c \global\dimen5=\Y@c
 \advance\count@@\m@ne \xycontrolpt@{\the\count@@}%
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \A@=\X@c \advance\A@\dimen3 \halve@dimen\A@
 \B@=\Y@c \advance\B@\dimen5 \halve@dimen\B@
 \edef\tmp@{\egroup \A@=\the\A@ \B@=\the\B@ \count@@=\the\count@@}%
 \tmp@ }
\xydef@\bsegment@z@i{%
 \expandafter\count@@\xycrvptsnum@\relax\advance\count@@-\tw@ 
 \bgroup
 \xycontrolpt@{\count@@}\X@p=\the\X@c \Y@p=\the\Y@c
\splinetrace@{\the\count@@: \the\X@c, \the\Y@c}%
 \advance\X@p by7\A@ \advance\X@p-2\dimen3 \dimen@nth6\X@p
 \advance\Y@p by7\B@ \advance\Y@p-2\dimen5 \dimen@nth6\Y@p
 \edef\tmp@{\egroup \X@p=\the\X@p \Y@p=\the\Y@p}%
 \tmp@ }
\xydef@\bsplinesegment@#1{\xybsplinemethods@ 
 \count@@=#1\relax 
 \ifnum\count@@=\@ne
 \bsegment@i \bsegment@i@iv
 \else\ifnum\count@@=\tw@
 \bsegment@@ii@iii \bsegment@@ii@i \bsegment@@iv
 \else\expandafter\count@\xycrvptsnum@\advance\count@\m@ne
 \ifnum\count@@=\count@
 \bsegment@z \bsegment@z@i 
 \else\advance\count@\m@ne
 \ifnum\count@@=\count@
 \bsegment@@ii@iii \bsegment@@i \bsegment@@y@iv
 \else
 \bsegment@@ii@iii \bsegment@@i \bsegment@@iv
 \fi\fi\fi\fi 
 \expandafter\def\expandafter\segmentnum@\expandafter{\number#1}%
 \bsplined@ }
\xydef@\bsplinesegment@iii#1{\xybsplinemethods@ 
\splinetrace@{2 segments; \number#1}%
 \count@@=#1\relax 
 \ifnum\count@@=\@ne \bsegment@i 
 \xycontrolpt@{3}%
\splinetrace@{3: \the\X@c, \the\Y@c}%
 \advance\X@c 4\dimen3\advance\X@c-\A@ 
 \dimen@nth4\X@c
 \advance\Y@c 4\dimen5\advance\Y@c-\B@ 
 \dimen@nth4\Y@c
 \else\ifnum\count@@=\tw@ \bsegment@z 
 \bgroup\xycontrolpt@{\@ne}%
\splinetrace@{1: \the\X@c, \the\Y@c}%
 \edef\tmp@{\egroup \X@p=\the\X@c \Y@p=\the\Y@c}\tmp@
 \advance\X@p 4\A@ \advance\X@p-\dimen3
 \dimen@nth4\X@p
 \advance\Y@p 4\B@ \advance\Y@p-\dimen5
 \dimen@nth4\Y@p
 \fi\fi
 \expandafter\def\expandafter\segmentnum@\expandafter{\number#1}%
 \bsplined@ }
\xydef@\bsplinesegment@iv#1{\xybsplinemethods@ 
\splinetrace@{3 segments; \number#1}%
 \count@@=#1\relax
 \ifnum\count@@=\@ne \bsegment@i \bsegment@i@iv
 \else\ifnum\count@@=\tw@
 \bsegment@@ii@iii \bsegment@@ii@i \bsegment@@y@iv
 \else\ifnum\count@@=3\relax
 \bsegment@z \bsegment@z@i
 \fi\fi\fi 
 \expandafter\def\expandafter\segmentnum@\expandafter{\number#1}%
 \bsplined@ }
\message{circles,}
\xydef@\Circmagic@@{0.5517847}
\xylet@\Circmagic=\Circmagic@@
\xydef@\twoPi@{6.2831852}
\xydef@\fullPi@{3.1415926}
\xydef@\halfPi@{1.5707963}
\xynew@{dimen}\L@
\xydef@\xycircle#1#{\hbox\bgroup\afterVECTORorEMPTY{%
 \xy@@{\R@=\X@c \L@=\Y@c}\xycircle@}{\xy@@{\R@=\R@c \L@=\L@c}\xycircle@}#1@}
\xydef@\xycircle@#1@#2{%
 \DN@{#1}\ifx\next@\empty\def\onlyQuad@{}\else \count@=#1\relax 
 \ifnum\count@<5 \advance\count@-3\relax 
 \ifnum\count@<\z@ \advance\count@ 4\relax\fi \edef\onlyQuad@{\the\count@}%
 \else\xyerror@{illegal circle <radius>: must be <vector> or <empty>}{}\fi
 \fi \xy@@{\def\circleSTYLE@{#2}}\def\circleSTYLE@{#2}\xycircle@i}
\xydef@\xycircle@i{\hbox{\vbox{\vskip\L@
 \hbox to2\R@{\hfill \buildcircle@ \hfill}\vskip\L@ }}%
 \L@c=\R@ \R@c=\R@ \D@c=\L@ \U@c=\L@ \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\relax}\Edge@c={\circleEdge}%
 \OBJECT@x}
\xydef@\adjustMinMaxcirc@#1#2{%
 \dimen@=\X@c \advance\dimen@#1\relax\ifdim\dimen@>\X@max \X@max=\dimen@\fi
 \dimen@=\X@c \advance\dimen@-#1\relax\ifdim\dimen@<\X@min \X@min=\dimen@\fi
 \dimen@=\Y@c \advance\dimen@#2\relax\ifdim\dimen@>\Y@max \Y@max=\dimen@\fi
 \dimen@=\Y@c \advance\dimen@-#2\relax\ifdim\dimen@<\Y@min \Y@min=\dimen@\fi
}
%% \cubicCircleControls@@ 
\xydef@\cubicCircleControls@@{\X@origin=\z@ \Y@origin=\z@
 \X@xbase=\R@ \Y@xbase=\z@ \X@ybase=\z@ \Y@ybase=\L@
 \vfromcartesian@@1,0@\czeroEdge@\idfromc@{0@c}%
 \vfromcartesian@@0,1@\czeroEdge@\idfromc@{1@c}%
 \vfromcartesian@@-1,0@\czeroEdge@\idfromc@{2@c}%
 \vfromcartesian@@0,-1@\czeroEdge@\idfromc@{3@c}%
 \vfromcartesian@@1,\Circmagic@@ @\czeroEdge@\idfromc@{1@m}%
 \vfromcartesian@@\Circmagic@@,1@\czeroEdge@\idfromc@{2@m}%
 \vfromcartesian@@-\Circmagic@@,1@\czeroEdge@\idfromc@{3@m}%
 \vfromcartesian@@-1,\Circmagic@@ @\czeroEdge@\idfromc@{4@m}%
 \vfromcartesian@@-1,-\Circmagic@@ @\czeroEdge@\idfromc@{5@m}%
 \vfromcartesian@@-\Circmagic@@,-1@\czeroEdge@\idfromc@{6@m}%
 \vfromcartesian@@\Circmagic@@,-1@\czeroEdge@\idfromc@{7@m}%
 \vfromcartesian@@1,-\Circmagic@@ @\czeroEdge@\idfromc@{8@m}%
 }
\xydef@\doCircleQuadrant@@#1#2{\save@ \ifcase#2\relax
 \doCircleQuadrant@@@{0@c}{1@m}{2@m}{1@c}{#1}\or
 \doCircleQuadrant@@@{1@c}{3@m}{4@m}{2@c}{#1}\or
 \doCircleQuadrant@@@{2@c}{5@m}{6@m}{3@c}{#1}\or
 \doCircleQuadrant@@@{3@c}{7@m}{8@m}{0@c}{#1}\or
 \doCircleQuadrant@@@{0@c}{1@m}{2@m}{1@c}{#1}\or
 \doCircleQuadrant@@@{1@c}{3@m}{4@m}{2@c}{#1}\or
 \doCircleQuadrant@@@{2@c}{5@m}{6@m}{3@c}{#1}\or
 \doCircleQuadrant@@@{3@c}{7@m}{8@m}{0@c}{#1}\fi \leave@ }
\xydef@\doCircleQuadrant@@@#1#2#3#4#5{%
 \cfromid@{#1}\pfromc@\senter@
 \cfromid@{#2}\spushc@\cfromid@{#3}\spushc@\cfromid@{#4}%
 \let\bstartPLACE@=\empty \connect@\crvs{#5}\relax\sinit@\sleave@
 \resetbreaks@}
\xydef@\dosolidcircle@#1{%
 \cubicCircleControls@@ 
 \doCircleQuadrant@@{#1}1 \relax\Clast@@
 \doCircleQuadrant@@{#1}2 \relax\Clast@@
 \doCircleQuadrant@@{#1}3 \relax\Clast@@
 \doCircleQuadrant@@{#1}4 \relax\Clast@@}%
\xydef@\solidcircle@{\dosolidcircle@@}
\xylet@\dosolidcircle@@=\dosolidcircle@
\xydef@\circledobjects@{\cubicCircleControls@@ 
 \setboxz@h{\expandafter\object\circleSTYLE@{}}%
 \ifdim\L@>\R@ \dimen@ii=\ht\z@ \advance\dimen@ii \dp\z@
 \ifdim\zz@\dimen@ii \dimen@ii=\wdz@\fi
 \else \dimen@ii=\wdz@ 
 \ifdim\zz@\dimen@ii \dimen@ii=\ht\z@ \advance\dimen@ii \dp\z@\fi
 \fi \ifdim\zz@\dimen@ii \dimen@ii=2\jot\fi
 \expandafter\dimen@\ifdim\L@>\R@ \twoPi@\L@\else \twoPi@\R@\fi
 \advance\dimen@.5\dimen@ii
 \count@@=\dimen@ \count@=\dimen@ii \divide\count@@\count@
 \edef\numobjects{\the\count@@}\dimen@=4\p@
 \dimen@nth\numobjects\dimen@
 \edef\circleseparation@{\expandafter\removePT@\the\dimen@}%
 \edef\circleplace@{-\circleseparation@}\placeQuadrants@}%
\xydef@\placeQuadrants@{\DN@{\placeAllQuadrants@}%
 \ifx\onlyQuad@\undefined\else\ifx\onlyQuad@\empty\else
 \DN@{\expandafter\placeCircQuadrant@\expandafter{\onlyQuad@}}%
 \fi\fi \next@ }%
\xydef@\placeAllQuadrants@{%
 \placeCircQuadrant@{1}%
 \advance\dimen@-\p@\advance\dimen@-\circleseparation@\p@
 \edef\circleplace@{\expandafter\removePT@\the\dimen@}%
 \placeCircQuadrant@{2}%
 \advance\dimen@-\p@\advance\dimen@-\circleseparation@\p@
 \edef\circleplace@{\expandafter\removePT@\the\dimen@}%
 \placeCircQuadrant@{3}%
 \advance\dimen@-\p@\advance\dimen@-\circleseparation@\p@
 \edef\circleplace@{\expandafter\removePT@\the\dimen@}%
 \placeCircQuadrant@{4}}
\xydef@\placeCircQuadrant@#1{%
 \let\bstartPLACE@=\relax \doCircleQuadrant@@{}#1%
 \loop@
 \expandafter\dimen@\circleplace@\p@
 \advance\dimen@\circleseparation@\p@
 \edef\circleplace@{\expandafter\removePT@\the\dimen@}%
 \ifdim\dimen@<\p@ \placeCircObject@
 \repeat@ }
\xydef@\placeCircObject@{\begingroup
 \crvconnect@@ \Creset@@ \Invisible@false
 \expandafter\splinealong@\expandafter{\circleplace@}%
 \expandafter\drop\circleSTYLE@{}\endgroup }
\xydef@\buildcircle@{\save@
 \DNii@{\circledobjects@}%
 \ifx\circleSTYLE@\empty\DNii@{\solidcircle@{}}%
 \else \expandafter\DN@\expandafter{\addDASH@{}}\relax
 \ifx\next@\circleSTYLE@ \DNii@{\solidcircle@{}}%
 \else \expandafter\DN@\expandafter{\addEQ@{}}%
 \ifx\next@\circleSTYLE@ 
 \expandafter\circletemplate@\expandafter{\addEQ@{}}{}%
 \else \expandafter\DN@\expandafter{\addDASH@ 2}%
 \ifx\next@\circleSTYLE@ \DNii@{\doublecircle@{}}%
 \else \expandafter\DN@\expandafter{\addDASH@ 3}%
 \ifx\next@\circleSTYLE@ \DNii@{\triplecircle@{}}%
 \else \expandafter\expandafter\expandafter\DN@\expandafter\expandafter
 \expandafter{\expandafter\addDASH@\addDASH@{}}%
 \ifx\next@\circleSTYLE@ \DNii@{\dashedcircle@{}}%
 \else \expandafter\expandafter\expandafter\DN@\expandafter\expandafter
 \expandafter{\expandafter\addEQ@\addEQ@{}}%
 \ifx\next@\circleSTYLE@ \expandafter\expandafter\expandafter
 \circletemplate@\expandafter\expandafter\expandafter{%
 \expandafter\addEQ@\addEQ@{}}2%
 \else \expandafter\expandafter\expandafter\DN@\expandafter\expandafter
 \expandafter{\expandafter\addEQ@\addEQ@2}%
 \ifx\next@\circleSTYLE@ \expandafter\expandafter\expandafter
 \circletemplate@\expandafter\expandafter\expandafter{%
 \expandafter\addEQ@\addEQ@{}}2%
 \else \expandafter\expandafter\expandafter\DN@\expandafter\expandafter
 \expandafter{\expandafter\addEQ@\addEQ@3}%
 \ifx\next@\circleSTYLE@ \expandafter\expandafter\expandafter
 \circletemplate@\expandafter\expandafter\expandafter{%
 \expandafter\addEQ@\addEQ@{}}3%
 \else \expandafter\DN@\expandafter{\addDOT@{}}\relax
 \ifx\next@\circleSTYLE@ \DNii@{\dottedcircle@{}}%
 \else \expandafter\DN@\expandafter{\addDOT@2}\relax
 \ifx\next@\circleSTYLE@ \DNii@{\dbldottedcircle@{}}%
 \else \expandafter\DN@\expandafter{\addDOT@3}\relax
 \ifx\next@\circleSTYLE@ \DNii@{\trpldottedcircle@{}}%
 \else \DN@{:}\relax
 \ifx\next@\circleSTYLE@ \DNii@{\dbldottedcircle@{}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \nextii@ \leave@}
\xydef@\circletemplate@#1#2{\def\circleSTYLE@{\dir#2{#1}}}
\xydef@\doublecircle@#1{%
 \advance\R@-\p@ \advance\L@-\p@ \solidcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \solidcircle@{}}
\xydef@\triplecircle@#1{%
 \advance\R@-2\p@ \advance\L@-2\p@ \solidcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \solidcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \solidcircle@{}}
\xydef@\dottedcircle@#1{%
 \expandafter\def\expandafter\circleSTYLE@\expandafter{%
 \zerodot@i}%
 \circledobjects@}
\xydef@\dashedcircle@#1{%
 \expandafter\def\expandafter\circleSTYLE@\expandafter{\zerodash@i}%
 \circledobjects@}
\xydef@\dbldottedcircle@#1{%
 \advance\R@-\p@ \advance\L@-\p@ \dottedcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \dottedcircle@{}}
\xydef@\trpldottedcircle@{%
 \advance\R@-2\p@ \advance\L@-2\p@ \dottedcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \dottedcircle@{}%
 \advance\R@ 2\p@ \advance\L@ 2\p@ \dottedcircle@{}}
{\xyuncatcodes \gdef\next{=<.75\jot>{\zerodot}}}
\xylet@\zerodot@i=\next
{\dimen0=2\xydashl@ \xyuncatcodes 
\expandafter\gdef\expandafter\next\expandafter{\expandafter
 =\expandafter<\the\dimen0 >_\dir{|}}}
\xylet@\zerodash@i=\next
{\xyuncatcodes\gdef\next{--}}
\xylet@\dashcorntemp@@=\next
{\xyuncatcodes\gdef\next{.}}
\xylet@\dotcorntemp@@=\next
\xydef@\dotcorner@#1{%
 \expandafter\circleCorner@\expandafter{\dotcorntemp@@}{#1}}%
\xydef@\dashcorner@#1{%
 \expandafter\circleCorner@\expandafter{\dashcorntemp@@}{#1}}
\xydef@\circleCorner@#1#2{\setboxz@h\bgroup 
 \edef\next{#2\relax\R@=\the\R@\relax\L@=\R@ }%
 \expandafter\xycircle@\next @{#1}%
 \ifcase#2\or \setboxz@h{\lower\R@\boxz@\kern\X@c}%
 \or \setboxz@h{\kern-\R@\lower\R@\boxz@\kern\R@\kern\X@c}%
 \or \setboxz@h{\kern-\R@\lower\R@\boxz@\kern\R@\kern\X@c}%
 \or \setboxz@h{\lower\R@\boxz@\kern\X@c}\fi
 \wdz@=\R@ \ht\z@=\R@ \dp\z@=\R@ \boxz@
 }
\xydef@\qspline{\hbox\bgroup\crvresetbreaks@ \xy@spline@}
\xydef@\xy@spline@#1#{\if\sempty@ \DN@{\crvs@{}\resetbreaks@}%
 \else\DN@{\xy@spline@i{#1}}\fi \next@ }%
\xydef@\xy@spline@i#1#2{\def\splineSTYLE@{#2}%
 \DN@{\xy@spline@ii}\DNii@{#1}%
 \ifx\nextii@\empty\DN@{\xy@spline@ii@@}\fi \next@ }
\xydef@\xy@spline@ii{\save@ \cfromp@\idfromc@{@p}%
 \enter@\cplusthec@ \count@@=\s@top\advance\count@@\m@ne
 \cfroms@{\count@@}\leave@
 \halve@dimen\X@c
 \halve@dimen\Y@c
 \czeroEdge@ \idfromc@{@c}%
 \expandafter\doSplineStraight@\expandafter{\splineSTYLE@}%
 \count@=\@ne \edef\next@{\the\count@}%
 \ifx\next@\s@top\DN@{\xy@spline@iv}\else\DN@{\xy@spline@iii}\fi 
 \next@ }
\xylet@\xy@spline@ii@@=\xy@spline@ii
\xydef@\xy@spline@iii{\crv@cnt@=\s@top 
 \loop \advance\crv@cnt@\m@ne \xy@spline@g \ifnum\crv@cnt@>\@ne\repeat
 \xy@spline@iv}
\xydef@\xy@spline@g{\cfromid@{@c}\idfromc@{@p}%
 \count@@=\crv@cnt@\cfroms@{\count@@}\idfromc@{@m}%
 \enter@\cplusthec@ \count@@=\crv@cnt@ \advance\count@@\m@ne
 \cfroms@{\count@@}\leave@
 \halve@dimen\X@c
 \halve@dimen\Y@c
 \czeroEdge@\idfromc@{@c}%
 \expandafter\doSplineSegment@\expandafter{\splineSTYLE@}}
\xydef@\xy@spline@iv{\cfromid@{@c}\idfromc@{@p}%
 \cfroms@{\z@}\idfromc@{@m}\leave@ \save@
 \enter@\cplusthec@ \cfromid@{@m}\leave@
 \halve@dimen\X@c
 \halve@dimen\Y@c
 \czeroEdge@\idfromc@{@c}%
 \expandafter\doSplineSegment@\expandafter{\splineSTYLE@}%
 \xy@spline@v }
\xydef@\xy@spline@v{\cfromid@{@c}\idfromc@{@p}%
 \leave@ \save@ \idfromc@{@c}%
 \expandafter\doSplineStraight@\expandafter{\splineSTYLE@}%
 \xy@spline@x }
\xydef@\xy@spline@x{\leave@ 
 \def\Drop@@{\splineDrop@ \resetbreaks@}%
 \def\Connect@@{\straight@\relax\splineConnect@ \resetbreaks@}%
 \OBJECT@x}
\xydef@\splineDrop@{\ifInvisible@\setboxz@h{}%
 \else\setboxz@h{\kern-\the\X@c\raise-\the\Y@c\hbox{\styledboxz@}}\fi
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@ }
\xydef@\splineConnect@{%
 \ifInvisible@\else\box\lastobjectbox@\fi }%
\xydef@\doSplineStraight@#1{\begingroup \sinit@
 \cfromid@{@p}\pfromc@\cfromid@{@c}%
 \connect@\crvs{#1}\relax\sleave@\endgroup }
\xydef@\doSplineSegment@#1{\begingroup \sinit@
 \cfromid@{@p}\pfromc@\senter@\cfromid@{@m}\spushc@\cfromid@{@c}%
 \connect@\crvs{#1}\relax\sinit@\sleave@\endgroup }
\xyendinput


==> xydummy.tex <==
%% xydummy.tex from $Id: xydummy.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Dummy'' option.
%% Copyright (c) 1993-1996 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{dummy}{Dummy option}{\stripRCS$Revision: 3.7 $}%
 {Kristoffer H.~Rose}{krisrose@tug.org}%
 {IBM T.~ J.\ Watson Research Center, P.O.~Box 704, Yorktown Heights, NY 10598 (USA)}
\xynew@{count}\xydummyrequires@@
\xyeveryrequest{dummy}{\global\advance\xydummyrequires@@\@ne
 \W@{The `dummy' option was used \the\xydummyrequires@@\space times!}}
\xyendinput


==> xydvidrv.tex <==
%% xydvidrv.tex from $Id: xydvidrv.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``dvidrv-driver'' option.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{dvidrv}{dvidrv driver}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\dvidrv@@#1{\dvimessage@{dvidrv}{#1}}
\newdriver{%
 \xyaddsupport{emtex}\dvidrvEmTeX@@
 \xyaddsupport{line}\dvidrvLine@@
}
\xydef@\dvidrvEmTeX@@{\dvidrvEmTeX@}%
\xydef@\dvidrvEmTeX@{\setupxyEMTeX@}%
\xydef@\dvidrvLine@@{\dvidrvLine@}%
\xydef@\dvidrvLine@{\xywithoption{emtex}{\installEMline@}}%
\xyendinput


==> xydvips.tex <==
%% xydvips.tex from $Id: xydvips.doc,v 3.9 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``dvips-driver'' option.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{dvips}{DVIPS driver}{\stripRCS$Revision: 3.9 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\dvips@@#1{\dvimessage@{dvips}{#1}}
\newdriver{%
 \xyaddsupport{color}\dvipsColor@@
 \xyaddsupport{crayon}\dvipsCrayola@@
 \xyaddsupport{ps}\dvipsPS@@
 \xyaddsupport{rotate}\dvipsRotate@@
 \xyaddsupport{line}\dvipsLine@@
 \xyaddsupport{frame}\dvipsFrames@@
 \xyaddsupport{tile}\dvipsTiles@@
 \xyaddsupport{tpic}\dvipsTPIC@ 
 \xyaddsupport{emtex}\dvipsEM@
 \xyaddsupport{tips}\dvipsTIPS@
}
\xydef@\dvips@Color@{\dvipsPStypes@ 
 \let\xylocalColor@=\xystackcolor@ 
 \let\xycolor@push\xycolor@push@@
 \def\xycolor@{\xycolor@@}\let\xycolorwarning@=\relax
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}\installPScolor@ }%
 \else\DN@{}\fi \next@ 
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\dvipsCrayola@{}}%
 \else \DN@{\xystandardcolors@}\fi \next@
 \let\dvipsColor@@=\relax
 \let\UnloadColor@@=\NoDVIPScolor@
 }%
\xydef@\dvipsColor@@{\dvips@Color@}
\xydef@\NoDVIPScolor@{%
 \def\xycolor@{\xycolor@@}%
 \let\xycolor@@=\xyNoColor@
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\dvipsColor@@=\dvips@Color@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\NoDVIPScolordvi@{\xywarning@{%
 Neither colordvi.tex nor colordvi.sty could be found.}%
 \xyBEcolorcheck@}%
\xydef@\dvipsCrayola@@{\dvipsColor@@\dvipsCrayola@}
\xydef@\dvipsCrayola@{%
 \let\prevxycolor@=\newxycolor@
 \def\newxyDVIPScolor@##1##2##3{\prevxycolor@{##1}{}{##1}}%
 \let\newxycolor@=\newxyDVIPScolor@ \dvipsInclude@{color.pro}%
 \installCrayolaColors@
 \let\newxycolor@=\prevxycolor@ }%
\xydef@\dvipsPS@@{\dvipsPS@}
\xydef@\dvipsPS@unload{\UnloadPS@
 \let\UnloadPS@@=\UnloadPS@
 \let\dvipsPS@@=\dvipsPS@ }
\xydef@\dvipsPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\dvipsSpecial@\else
 \let\PSspecial@@=\dvipsSpecial@
 \let\PSmacro@@=\dvipsMacro@
 \let\PSdict@@=\dvipsDict@
 \let\PSspecialdict@@=\dvipsDict@
 \let\PSraw@@=\dvipsRaw@
 \let\PSinclude@@=\dvipsInclude@
 \let\xyPSobeylines@@=\obeyDVIPSlines@
 \let\xyPScurrpt@@=\dvipsCurrpt@@
 \dvips@@{PostScript}%
 \fi
 \XYpredict@ }
\xywarnifdefined\dvipsSpecial@
\xywarnifdefined\dvipsMacro@
\xywarnifdefined\dvipsDict@
\xywarnifdefined\dvipsInclude@
\xywarnifdefined\dvipsRaw@
{\catcode`\"=11 \catcode`\!=11 \catcode`\:=11
 \gdef\dvipsSpecial@#1{\special{ps:: SDict begin #1 end}}
 \gdef\dvipsMacro@#1{\firstPS@@\special{" {#1}xy}}
 \gdef\dvipsDict@#1{\special{! #1}}
 \gdef\dvipsInclude@#1{\special{header=#1}}
 \gdef\dvipsRaw@#1{\special{ps: SDict begin #1 end}}
\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\space }}%
\xylet@\obeyDVIPSlines@=\next
\xydef@\dvipsCurrpt@{\let\xyPScurrpt@@=\dvipsCurrpt@@}%
\xydef@\dvipsCurrpt@@{\PSraw@@{xyp}}
\xydef@\dvipsPS@{\dvipsPStypes@ 
 \let\dvipsPS@@=\PSspecials@true
 \let\UnloadPS@@=\dvipsPS@unload 
 \let\installxyps@@=\relax \installxyps@ }
\xydef@\dvipsRotate@@{\dvipsRotate@}
\xydef@\dvipsRotate@{\dvipsPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \dvipsCurrpt@ \dvipsRotScale@ \installPSrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}UnloadRotate@\relax}\fi
 \next@ }
\xydef@\dvipsRotScale@{%
 \def\xyrot@start(##1){{xyct ##1\space xyrs }}%
 \def\xyrot@end{}%
 \def\xyscale@start(##1,##2){{xyct ##1\space##2\space xyss }}%
 \def\xyscale@end{}}
\xydef@\dvipsLine@@{\dvipsLine@}
\xydef@\dvipsLine@{\dvipsPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}\installPSline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\dvipsFrames@@{\dvipsFrames@}
\xydef@\dvipsFrames@{\dvipsPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}\installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadFrames@\relax}\fi
 \next@ }
\xydef@\dvipsTiles@@{\dvipsTiles@}
\xydef@\dvipsTiles@{\dvipsPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}\installPSpatterns@ }%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xydef@\dvipsTPIC@@{\dvipsTPIC@}
\xydef@\dvipsTPIC@{\setupxyTPIC@}
\xydef@\dvipsEM@@{\dvipsEM@}
\xydef@\dvipsEM@{\setupxyEMTeX@}
\xydef@\dvipsTIPS@{
 \PSdict@@{/XYdict where pop begin XYdict begin}%
 \PSdict@@{%
 /lu{0.04 0.0 -0.16 0.125 -0.11 0.0
 1 1 6{pop xyfsize mul 6 1 roll}for
 lineto lineto lineto closepath fill
 0 0 0 0 0 0}def
 }%
 \PSdict@@{end end}%
}
\xyendinput


==> xydvitops.tex <==
%% xydvitops.tex from $Id: xydvitops.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``DVITOPS-driver'' option.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{dvitops}{DVITOPS driver}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\dvitops@@#1{\dvimessage@{DVITOPS}{#1}}
\newdriver{%
 \xyaddsupport{color}\dvitopsColor@@
 \xyaddsupport{crayon}\dvitopsCrayon@@
 \xyaddsupport{ps}\dvitopsPS@@
 \xyaddsupport{rotate}\dvitopsRotate@@
 \xyaddsupport{line}\dvitopsLine@@
 \xyaddsupport{frame}\dvitopsFrames@@
 \xyaddsupport{tile}\dvitopsTiles@@
 \xyaddsupport{cmtip}\relax
}
\xydef@\dvitopsColor@@{\dvitops@Color@}
\xydef@\dvitops@Color@{\dvitopsPStypes@ 
 \let\xylocalColor@=\xyDVITOPScolor@ 
 \let\xycolor@push\xycolor@push@@
 \def\xycolor@{\xycolor@@}\let\xycolorwarning@=\relax
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}\xycatcodes
 \installPScolor@ }\else\DN@{}\fi \next@
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\dvitopsCrayon@{}}%
 \else\let\next@=\xystandardcolors@
 \fi \next@
 \let\dvitops@Color@@=\relax
 \let\UnloadColor@@=\NoDVITOPScolor@
 }%
\xydef@\NoDVITOPScolor@{%
 \def\xycolor@{\xycolor@@}%
 \let\xycolor@@=\xyNoColor@
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\dvitops@Color@@=\dvitops@Color@
 }
\xydef@\xyDVITOPScolor@{\bgroup \DN@##1##2{\egroup}%
 \ifInvisible@\else\ifHidden@\else\DNii@{\no@@}\ifx\nextii@\Connect@@ 
 \else\DN@{\xyDVITOPScolor@i}\fi\fi\fi \next@ }
\xydef@\xyDVITOPScolor@i#1#2{\checkXyStyle@ 
 \DN@{#2}\ifx\next@\empty
 \def\tmp@##1{\DN@{\xycolor@begin##1\xycolor@end{#1}}}%
 \else\DNii@{gray}\ifx\next@\nextii@
 \def\tmp@##1{\DN@{\xycolor@begin##1\xycolor@end{gray}{#1}}}%
 \else\DNii@{rgb}\ifx\next@\nextii@
 \def\tmp@##1{\DN@{\xycolor@begin##1\xycolor@end{rgbcolor}{#1}}}%
 \else\DNii@{hsb}\ifx\next@\nextii@
 \def\tmp@##1{\DN@{\xycolor@begin##1\xycolor@end{hsbcolor}{#1}}}%
 \else \DN@{\xywarning@{DVITOPS cannot support color: #2 #1}}%
 \fi\fi\fi\fi
 \toks@={\egroup \let\xy@style@=\relax \def\Drop@@}%
 \expandafter\tmp@\expandafter{\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}\def\Connect@@}%
 \expandafter\tmp@\expandafter{\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}}%
 \the\toks@ }%
\xydef@\xycolor@begin{\dvitopsBegin@{color}}
\xydef@\xycolor@end{\dvitopsEnd@{color}\dvitopsColor@x}
\xydef@\dvitopsCrayon@@{\dvitopsColor@@\dvitopsCrayon@}
\xydef@\dvitopsCrayon@{\installCrayolaColors@}%
\xydef@\dvitopsPS@@{\dvipsPS@}
\xydef@\dvitopsPS@unload{\UnloadPS@
 \let\UnloadPS@@=\UnloadPS@
 \let\dvitopsPS@@=\dvitopsPS@ }
\xydef@\dvitopsPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\dvitopsSpecial@\else
 \let\PSspecial@@=\dvitopsSpecial@
 \let\PSmacro@@=\dvitopsMacro@
 \let\PSdict@@=\dvitopsDict@
 \let\PSspecialdict@@=\dvitopsDict@
 \let\PSraw@@=\dvitopsRaw@
 \let\PSinclude@@=\dvitopsInclude@
 \let\xyPSobeylines@@=\obeyDVIPSlines@
 \let\xyPScurrpt@@=\dvitopsCurrpt@@
 \dvitops@@{PostScript}%
 \fi
 \XYpredict@ }
\xywarnifdefined\dvitopsSpecial@
\xywarnifdefined\dvitopsMacro@
\xywarnifdefined\dvitopsDict@
\xywarnifdefined\dvitopsInclude@
\xywarnifdefined\dvitopsRaw@
\xywarnifdefined\dvitopsOrigin@
\xywarnifdefined\dvitopsBegin@
\xywarnifdefined\dvitopsEnd@
\xywarnifdefined\dvitopsRotate@x
\xywarnifdefined\dvitopsTransform@x
\xywarnifdefined\dvitopsColor@x
{\catcode`\:=11
 \gdef\dvitopsSpecial@#1{\special{dvitops: inline #1}}
 \gdef\dvitopsMacro@#1{\special{dvitops: inline {#1}xy}}
 \gdef\dvitopsDict@#1{\special{dvitops: inline #1}}
 \gdef\dvitopsInclude@#1{\special{dvitops: prolog #1}}
 \gdef\dvitopsRaw@#1{\special{dvitops: inline #1}}
 \gdef\dvitopsOrigin@#1{\special{dvitops: origin #1}}
 \gdef\dvitopsBegin@#1{\special{dvitops: begin #1}}
 \gdef\dvitopsEnd@#1{\special{dvitops: end #1}}
 \gdef\dvitopsRotate@x#1{\special{dvitops: rotate #1}}
 \gdef\dvitopsTransform@x#1{\special{dvitops: transform #1}}
 \gdef\dvitopsColor@x#1#2{\special{dvitops: #1 color #2}}
}
\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\space }}%
\xylet@\obeyDVIPSlines@=\next
\xydef@\dvitopsCurrpt@{\global\let\xyPScurrpt@@=\relax}%
\xydef@\dvitopsPS@{\dvitopsPStypes@ 
 \let\installxyps@@=\relax \installxyps@ }
\xydef@\dvitopsRotate@@{\dvitopsRotate@}
\xydef@\dvitopsRotate@{\dvitopsPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty
 \DN@{\xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \installDVITOPSrotate@ }%
 \else\DN@{\xydriverfail@{rotations are}\UnloadRotate@\relax}\fi
 \next@ }
\xydef@\dvitopsRotScale@{%
 \def\xyrot@start{\dvitopsBegin@{rot}\dvitopsOrigin@{rot}}%
 \def\xyrot@end(##1){\dvitopsEnd@{rot}\dvitopsRotate@x{##1}}%
 \def\xyscale@start{\dvitopsBegin@{scal}\dvitopsOrigin@{scal}}%
 \def\xyscale@end(##1,##2){%
 \dvitopsEnd@{scal}\dvitopsTransform@x{##1 0 ##2 0}}%
 }
\xydef@\installDVITOPSrotate@{\installPSstyle@
 \let\xyRotate@@=\dvitopsRotate@
 \let\doSpecialRotate@@=\dvitopsSpecialRotate@
 \let\xyscale@@=\dvitopsScale@
 \dvitopsCurrpt@
 \dvitopsRotScale@ \xyPSshapes@true }
\xydef@\UnloadDVITOPSrotate@{\UnloadRotate@\relax}
 \xydef@\dvitopsRotate@#1{\xyPSsplitPS@
 {\dvitopsBegin@{rot}\dvitopsOrigin@{rot}}%
 {\dvitopsEnd@{rot}\dvitopsRotate@x{#1}}}%
 \xydef@\dvitopsScale@#1#2{\xyPSsplitPS@
 {\dvitopsBegin@{scal}\dvitopsOrigin@{scal}}%
 {\dvitopsEnd@{scal}\dvitopsTransform@x{#1 0 #2 0}}}
 \xydef@\dvitopsSpecialRotate@#1@@{\dvitopsRotate@{#1}}
\xydef@\dvitopsLine@@{\dvitopsLine@}
\xydef@\dvitopsLine@{\dvitopsPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}\installPSline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\dvitopsFrames@@{\dvitopsFrames@}
\xydef@\dvitopsFrames@{\dvitopsPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}\installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadFrames@\relax}\fi
 \next@ }
\xydef@\dvitopsTiles@{\dvitopsPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}\installPSpatterns@ }%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xydef@\dvitopsTPIC@@{\dvitopsTPIC@}
\xydef@\dvitopsTPIC@{\setupxyTPIC@}
\xyendinput


==> xyemtex.tex <==
%% xyemtex.tex from $Id: xyemtex.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``em-TeX'' back-end extension.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{emtex}{em-TeX backend}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xynew@{if}\ifEMspecials@
\xydef@\UseEMspecials{\EMspecials@true}
\xydef@\NoEMspecials{\EMspecials@false}
\xydef@\xyemtex@lineto{\xyEM@special{lineto}} 
\xydef@\xyemtex@moveto{\xyEM@special{moveto}} 
\xydef@\xyemtex@line#1{\xyEM@special{line #1}} 
\xydef@\xyemtex@point#1{\xyEM@special{point #1}} 
\xydef@\xyemtex@pen#1{\addtostyletoks@{\xyEM@special{linewidth #1}}}
{\catcode`:=12 \gdef\next#1{\special{em:#1}}}
\xylet@\xyEM@special=\next
{\catcode`:=12 \gdef\next#1{%
 \W@{EM:#1 (\the\X@p,\the\Y@p),(\the\X@c,\the\Y@c)}\special{em:#1}}}
\xylet@\xyEM@noisy=\next
\xydef@\NoisyEMTeX{\let\xyEM@special=\xyEM@noisy}
\xydef@\EMalternative@#1#2{%
\expandafter\global\expandafter\let\csname origxy#2@\endcsname=#1%
 \xdef#1{\noexpand\ifEMspecials@
 \noexpand\expandafter\expandafter\noexpand\csname xyemtex@#2@\endcsname
 \noexpand\else
 \noexpand\expandafter\expandafter\noexpand\csname origxy#2@\endcsname
 \noexpand\fi}}%
\xydef@\setupxyEMTeX@{\xywarning@{using em-TeX specials}%
 \EMalternative@{\solid@}{solid}%
 \EMalternative@{\splinesolid@}{splinesolid}%
 \let\setupxyEM@=\reloadxyEM@ 
 \activateEM@ }
\xydef@\xyunloadEM@{\xywarning@{EM specials turned off}%
 \xywithoption{line}{\xysetup@@\uninstallEMline@ }%
 \EMspecials@false
 \let\setupxyEM@=\reloadxyEM@ }
\xydef@\activateEM@{%
 \xywithoption{line}{\xysetup@@\installEMline@}%
 \EMspecials@true }
\xydef@\reloadxyEM@{\xywarning@{EM specials back on}\activateEM@ }
\xydef@\xyemtex@solid@{%
 \ifInvisible@ \let\next@=\no@@
 \else \DN@{\xyEMstraight@}\fi
 \next@ }
\xydef@\xyEMstraight@{\setupDirection@
 \edef\Creset@@{\cfromthec@ \pfromthep@ \DirectionfromtheDirection@}%
 \DN@##1##2{\def\checkoverlap@@{%
 \ifdim##1\X@p>##1\X@c \let\next@=\relax \fi
 \ifdim##2\Y@p>##2\Y@c \let\next@=\relax \fi}}%
 \edef\nextii@{{\sd@X}{\sd@Y}}\expandafter\next@\nextii@
 \noCshavep@@ \edef\Cshavep@@{\pfromthep@ \noexpand\resetDirection@}%
 \noCshavec@@ \edef\Cshavec@@{\cfromthec@ \noexpand\resetDirection@}%
 \ifHidden@\else
 \ifdim\Y@c>\Y@max \Y@max=\Y@c \fi \ifdim\Y@p>\Y@max \Y@max=\Y@p \fi
 \ifdim\Y@c<\Y@min \Y@min=\Y@c \fi \ifdim\Y@p<\Y@min \Y@min=\Y@p \fi
 \ifdim\X@c>\X@max \X@max=\X@c \fi \ifdim\X@p>\X@max \X@max=\X@p \fi
 \ifdim\X@c<\X@min \X@min=\X@c \fi \ifdim\X@p<\X@min \X@min=\X@p \fi \fi
 \ifInvisible@\let\next@=\relax \else
 \DN@{%
 \setboxz@h{\kern\X@p \raise\Y@p\hbox{\xyemtex@moveto}}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@
 \setboxz@h{\boxz@ \kern\X@c \raise\Y@c\hbox{\xyemtex@lineto}}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ {\Drop@@}}%
 \fi 
 \checkoverlap@@
 \ifdim\d@X=\z@ \ifdim\d@Y=\z@ \DN@{\relax}\fi\fi \next@
 \def\Cslidep@@{\noCslidep@@}\def\Cslidec@@{\noCslidec@@}%
 \def\Calong@@{\noCalong@@}\Creset@@ }
\xydef@\xyemtex@splinesolid@{\setbox\splinebox@=\copy\voidb@x 
 \multiply\splinetol@\thr@@ 
 \gdef\splineextra@@{\xyemtex@moveto\gdef\splineextra@@{\xyemtex@lineto}}%
 \def\xycrvdrop@{ }\def\xycrvconn@{}\splineset@@ }
\xydef@\xyEMlinewidth@#1{\dimen@=#1\relax\edef\next@{\the\dimen@}}
\xydef@\installEMline@{%
 \let\xylinewidth@@=\xylinewidth@
 \let\xylineSpecial@@=\xyemtex@pen
 \let\transxyline@@=\xyEMlinewidth@ }
\xydef@\uninstallEMline@{\UnloadLine@\relax}%
\xydef@\UseEMlinewidth{\installEMline@}%
\xydef@\NoEMlinewidth{\uninstallEMline@}%
\xyendinput


==> xyframe.tex <==
%% xyframe.tex from $Id: xyframe.doc,v 3.13 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Frames and Brackets'' extension.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{frame}{Frame and Bracket extension}{\stripRCS$Revision: 3.13 $}%
 {Kristoffer H.~Rose}{krisrose@tug.org}%
 {IBM T.~ J.\ Watson Research Center, P.O.~Box 704, Yorktown Heights, NY 10598 (USA)}
\xydef@\frm{\hbox{}\dimen@=\L@c \advance\dimen@\R@c \wdz@=\dimen@
 \ht\z@=\U@c \dp\z@=\D@c \dimen@=\U@c \advance\dimen@\D@c
 \ifdim\wdz@=\z@ \def\Leftness@{.5}\else \quotient@\Leftness@\L@c\wdz@ \fi
 \ifdim\dimen@=\z@ \def\Upness@{.5}\else \quotient@\Upness@\U@c\dimen@ \fi
 \expandafter\Edge@c\expandafter{\prevEdge@@}\let\frmradius@@=\z@
 \def\Drop@@{}%
 \def\Connect@@{\xy@@{\save@\cmerge@\Y@p\X@p\D@p\U@p\L@p\R@p\Drop@@}\restore}%
 \xyFN@\frm@i}
\xylet@\frmradius@@=\z@
\xydef@\frm@i{%
 \addLT@\ifx\next \addGT@{\addLT@\DN@##1}{\def\frmradius@@{##1}\xyFN@\frm@i}%
 \else \DN@##1##{\frm@{##1}}\fi \next@}
\xydef@\frm@#1#2{\DNii@{frm#1{#2}}%
 \expandafter\let\expandafter\next@\csname\codeof\nextii@\endcsname
 \ifx\next@\relax \DNii@{frm{#2}}%
 \expandafter\let\expandafter\next@\csname\codeof\nextii@\endcsname
 \ifx\next@\relax \let\next@=\frm@generic \fi\fi \next@}
\xydef@\frm@generic{\xyerror@{No generic frames yet!}{}}
\xydef@\frmDrop@#1{%
 \ifx\frmradius@@\z@ \addtoDrop@@{\let\frmradius@@=\z@ #1}%
 \else \expandafter\addtoDrop@@\expandafter{%
 \expandafter\def\expandafter\frmradius@@\expandafter{\frmradius@@}#1}\fi}
\xydef@\EdgefromtheEdge@{%
 \U@c=\the\U@c \D@c=\the\D@c \L@c=\the\L@c \R@c=\the\R@c
 \Edge@c={\expandafter\noexpand\the\Edge@c}}
\xydef@\prevEdgefromtheEdge@{%
 \U@c=\the\U@c \D@c=\the\D@c \L@c=\the\L@c \R@c=\the\R@c
 \noexpand\def\noexpand\prevEdge@@{\expandafter\noexpand\the\Edge@c}}
\xydef@\addtoDrop@@#1{%
 \expandafter\def\expandafter\Drop@@\expandafter{\Drop@@#1}}
\xydef@\addbeforeDrop@@#1{\DNii@{#1}%
 \expandafter\DN@\expandafter{\expandafter\nextii@\Drop@@}%
 \expandafter\expandafter\expandafter\def
 \expandafter\expandafter\expandafter\Drop@@
 \expandafter\expandafter\expandafter{\next@}}
\xydefcsname@{frm{}}{}
\xyletcsnamecsname@{frm[]{}}{frm{}}
\xyletcsnamecsname@{frm[o]{}}{frm{}}
\xydefcsname@{frm{.}}{\frmDrop@{\let\zerocorner=\framezerodot@@
 \let\framehfill=\frm@doth@@ \let\framevfill=\frm@dotv@@
 \framed@@{\frmradius@@}}}
\xyletcsnamecsname@{frm[]{.}}{frm{.}}
\xydef@\frm@doth@@{\setboxz@h{\kern5\B@\framezerodot@@\kern5\B@}\ht\z@=\B@
 \dp\z@=\B@\kern5\B@\xleaders\boxz@\hss\kern5\B@}
\xydef@\frm@dotv@@{\setboxz@h to2\B@{\hss\framezerodot@@\hss}\ht\z@=5\B@
 \dp\z@=5\B@\kern5\B@\xleaders\boxz@\vss\kern5\B@}
\xyletcsnamecsname@{frm{..}}{frm{.}}
\xylet@\framezerodot@@=\zerodot
\xydefcsname@{frm{-}}{\frmDrop@{\framed@\frmradius@@}}
\xyletcsnamecsname@{frm[]{-}}{frm{-}}
\xydef@\framed@{\let\zerocorner=\framezerodot@@
 \let\framehfill=\frm@solidh@@ \let\framevfill=\frm@solidv@@ \framed@@}
\xylet@\framesetthick@=\relax
\xydef@\frm@solidh@@{\framesetthick@\leaders\hrule height\B@ depth\B@\hfill}
\xydef@\frm@solidv@@{\framesetthick@\leaders\vrule width2\B@\vfill}
\xydefcsname@{frm{=}}{\frmDrop@{\framed@\frmradius@@
 {\advance\L@c-2\p@ \advance\R@c-2\p@ \advance\U@c-2\p@ \advance\D@c-2\p@
 \dimen@=\frmradius@@
 \ifdim\dimen@>2\p@ \advance\dimen@-2\p@ \else \dimen@=\z@\fi
 \framed@\dimen@}}}
\xyletcsnamecsname@{frm[]{=}}{frm{=}}
\xydef@\framesetthick@line{\B@=.5\xylinethick@}
\xydef@\frm@thickc@@{\hbox{\framesetthick@line
 \vrule height.5\B@ depth.5\B@ width\B@}}
\xywithoption{line}{%
 \let\framezerodot@@\frm@thickc@@ \let\framesetthick@=\framesetthick@line}
\xydef@\framed@@#1{\setboxz@h{\R@=#1\relax 
 \dimen@=\L@c \advance\dimen@\R@c \dimen@ii=\U@c \advance\dimen@ii\D@c
 \ifdim.5\dimen@<\R@ \R@=.5\dimen@ \fi
 \ifdim.5\dimen@ii<\R@ \R@=.5\dimen@ii \fi
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@-\D@c
 \ifdim\R@<\p@\else \cirrestrict@@ \fi
 \dimen@=2\R@ \advance\dimen@-\L@c \advance\dimen@-\R@c
 \ifdim\dimen@>\z@ \advance\A@-.5\dimen@ \fi
 \dimen@=2\R@ \advance\dimen@-\U@c \advance\dimen@-\D@c
 \ifdim\dimen@>\z@ \advance\B@-.5\dimen@ \fi
 \kern\A@ \raise\B@\vbox to \dimen@ii{\framed@body@@}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\framed@body@{%
 \advance\dimen@ii.22\p@ \advance\dimen@-.2\p@ 
 \setboxz@h{\corn@@4\R@}\A@=-.5\wdz@ \B@=.5\xydashw@
 \dimen@=\L@c \advance\dimen@\R@c \advance\dimen@-.2\p@
 \setboxz@h to\dimen@{\kern\A@ \boxz@ \framehfill\corn@@3\R@\kern\A@}%
 \advance\dimen@ii-\dp\z@ \kern-\ht\z@ \nointerlineskip\boxz@
 \dimen@=\L@c \advance\dimen@\R@c \advance\dimen@-.2\p@
 \setboxz@h to\dimen@{\kern\A@\corn@@1\R@\framehfill\corn@@2\R@\kern\A@}%
 \advance\dimen@ii-\ht\z@
 \dimen@=\L@c \advance\dimen@\R@c \advance\dimen@.2\p@
 \nointerlineskip\hbox to\dimen@{%
 \setbox\z@=\vbox to\dimen@ii{\framevfill}\kern-.5\wdz@\copy\z@
 \hss \copy\z@\kern-.5\wdz@ }%
 \nointerlineskip\boxz@ \vss \kern\z@}
\xylet@\framed@body@@=\framed@body@
\xylet@\zerocorner=\framezerodot@@
\xydef@\solidcorner@#1#2{\hbox\bgroup \R@=#2\relax
 \ifdim\R@<\p@ \zerocorner
 \else \cirrestrict@@ \multiply\count@8
 \setboxz@h{\corn@x@@{#1}}\dimen@=\wdz@
 \ifcase#1\or \ht\z@=\z@ \kern\dimen@ \raise\dimen@\boxz@ 
 \or \ht\z@=\z@ \raise\dimen@\boxz@ \kern\dimen@
 \or \dp\z@=\z@ \lower\dimen@\boxz@ \kern\dimen@
 \or \dp\z@=\z@ \kern\dimen@ \lower\dimen@\boxz@ \fi
 \vrule height\dimen@ depth\dimen@ width\z@\fi
 \edef\tmp@{\egroup \U@c=\the\dimen@}\tmp@ \D@c=\U@c \L@c=\U@c \R@c=\U@c
 \Edge@c={\circleEdge}\ignorespaces}
\xydef@\corn@x@#1{\ifcase#1\or
 \circhar@@\z@ \circhar@@\@ne\or\circhar@@\tw@ \circhar@@3\or
 \circhar@@5\circhar@@4\or\circhar@@7\circhar@@6\fi}
\xylet@\corn@x@@=\corn@x@
\xydef@\corn@@{\DN@{\solidcorner@}%
 \ifx\framehfill\frm@doth@@ \DN@{\let\cirrestrict@@=\relax
 \let\corn@x@@=\dotcorner@@ \let\zerodot=\framezerodot@@
 \solidcorner@ }%
 \else\ifx\framehfill\frm@dashh@@ \DN@{\let\cirrestrict@@=\relax
 \let\corn@x@@=\dashcorner@@ \let\zerodot=\framezerodot@@
 \solidcorner@ }%
 \fi\fi \next@}
\xydef@\dotcorner@@#1{\zerocorner}
\xydef@\dashcorner@@#1{\zerocorner}
\xywithoption{curve}{%
 \let\dotcorner@@=\dotcorner@ \let\dashcorner@@=\dashcorner@}
\xydefcsname@{frm{--}}{%
 \frmDrop@{\let\zerocorner=\framezerodot@@ 
 \let\framehfill=\frm@dashh@@ \let\framevfill=\frm@dashv@@
 \framed@@\frmradius@@}}
\xyletcsnamecsname@{frm[]{--}}{frm{--}}
\xydef@\frm@dashh@@{\setboxz@h{\dashhfillchar}%
 \ht\z@=\B@ \dp\z@=\B@ \wdz@=2\xydashl@
 \copy\z@ \xleaders\copy\z@\hss \boxz@\kern-\xydashl@}
\xydef@\frm@dashv@@{\setboxz@h to2\B@{\hss\dashvfillchar\hss}\ht\z@=\z@
 \dp\z@=2\xydashl@ \nointerlineskip\copy\z@ \xleaders\copy\z@\vss
 \nointerlineskip\boxz@\kern-\xydashl@}%
\xydef@\dashhfillchar{{\rDirection@\xydashl@ \line@@}}
\xydef@\dashvfillchar{{\dDirection@\xydashl@ \line@@}}
\xydefcsname@{frm{o-}}{%
 \ifdim\frmradius@@<2\xydashl@\relax \dimen@=.8\xydashl@
 \expandafter\def\expandafter\frmradius@@\expandafter{\the\dimen@}\fi
 \frmDrop@{\let\zerocorner=\framezerodot@@ 
 \let\framehfill=\frm@rddashh@@ \let\framevfill=\frm@rddashv@@
 \framed@@\frmradius@@}}%
\xydef@\frm@rddashh@@{\setboxz@h{\kern\xydashl@\dashhfillchar}%
 \ht\z@=\B@ \dp\z@=\B@ \copy\z@ \xleaders\copy\z@\hss \boxz@ \kern\xydashl@}
\xydef@\frm@rddashv@@{\ifdim\dimen@ii<2\xydashl@\else
 \setbox\z@=\vbox to2\xydashl@{\hbox to2\B@{\hss\dashvfillchar\hss}\vss}%
 \kern\xydashl@ \copy\z@ \xleaders\copy\z@\vss
 {\ifdim\dimen@ii<2\xydashl@\else\aftergroup\boxz@\fi}\fi}
\xydefcsname@{frm{,}}{%
 \ifx\frmradius@@\z@ \shaded@{1.2\p@}\else \shaded@\frmradius@@ \fi}
\xydef@\shaded@#1{\frmDrop@{\R@=#1\relax
 {\advance\X@c\R@ \advance\Y@c-\D@c \U@c=\z@ \D@c=\R@ \blacked@}%
 {\advance\X@c\R@c \advance\Y@c-\R@ \L@c=\z@ \R@c=\R@ \blacked@}}}
\xydefcsname@{frm{-,}}{\addtoDrop@@{\drop\frm{-}\drop\frm{,}}}
\xydef@\blacked@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \dimen@=\L@c \advance\dimen@\R@c
 \B@=\Y@c \advance\B@-\D@c \dimen@ii=\Y@c \advance\dimen@ii\U@c
 \advance\A@-.5\xydashw@
 \kern\A@ \blacked@@ }%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\bblacked@{\setboxz@h{%
 \dimen@=\L@c \advance\dimen@\R@c \B@=-\D@c \dimen@ii=\U@c
 \kern-\L@c \blacked@@ \kern-\dimen@ \kern\L@c}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\blacked@@{\vrule width\dimen@ depth-\B@ height\dimen@ii}
\xydefcsname@{frm{o}}{%
 \ifx\frmradius@@\z@
 \frmDrop@{\dimen@=.5\L@c \advance\dimen@.5\R@c
 \let\framehfill=\frm@solidh@@ \let\framevfill=\frm@solidv@@
 \circled@\dimen@}%
 \else
 \frmDrop@{\let\framehfill=\frm@solidh@@
 \let\framevfill=\frm@solidv@@ \circled@\frmradius@@}%
 \fi}
\xydefcsname@{frm{oo}}{%
 \ifx\frmradius@@\z@
 \frmDrop@{\dimen@=.5\L@c \advance\dimen@.5\R@c
 \let\framehfill=\frm@solidh@@ \let\framevfill=\frm@solidv@@
 {\circled@\dimen@}\advance\dimen@-2.1\p@ \circled@\dimen@}%
 \else
 \frmDrop@{\dimen@=\frmradius@@
 \let\framehfill=\frm@solidh@@ \let\framevfill=\frm@solidv@@
 {\circled@\dimen@}\advance\dimen@-2.1\p@ \circled@\dimen@}%
 \fi}
\xydef@\circled@#1{\setboxz@h\bgroup \R@=#1\relax 
 \setboxz@h{\vbox{\circled@x@@}}%
 \A@=\X@c \advance\A@-.5\wd\z@
 \B@=\Y@c \advance\B@-.5\ht\z@ \advance\B@.5\dp\z@ \advance\B@.2\p@
 \edef\tmp@{\egroup\dimen@=\the\wdz@}%
 \kern\A@ \raise\B@\boxz@
 \tmp@ \divide\dimen@4 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\circled@x@{\hbox{\corn@@4\R@ \corn@@3\R@}%
 \nointerlineskip\hbox{\corn@@1\R@ \corn@@2\R@}}
\xylet@\circled@x@@=\circled@x@
\xydefcsname@{frm{.o}}{%
 \ifx\frmradius@@\z@ \frmDrop@{\let\framehfill=\frm@doth@@ 
 \dimen@=.5\L@c \advance\dimen@.5\R@c \circled@\dimen@}%
 \else
 \frmDrop@{\let\framehfill=\frm@doth@@ \circled@\frmradius@@}%
 \fi}
\xydefcsname@{frm{-o}}{%
 \ifx\frmradius@@\z@ \frmDrop@{\let\framehfill=\frm@dashh@@
 \dimen@=.5\L@c \advance\dimen@.5\R@c \circled@\dimen@}%
 \else
 \frmDrop@{\let\framehfill=\frm@dashh@@ \circled@\frmradius@@}%
 \fi}
\xydefcsname@{frm{e}}{\ellipse@whichfrm@\ellipsesolidframed@}%
\xydefcsname@{frm{.e}}{\ellipse@whichfrm@\ellipsedotframed@}%
\xydefcsname@{frm{-e}}{\ellipse@whichfrm@\ellipsedashframed@}%
\xydefcsname@{frm{ee}}{\ellipse@whichdblfrm@\ellipsesolidframed@}%
\xydefcsname@{frm2{.e}}{\ellipse@whichdblfrm@\ellipsedotframed@}%
\xydefcsname@{frm2{-e}}{\ellipse@whichdblfrm@\ellipsedashframed@}%
\xyletcsnamecsname@{frm[o]{-}}{frm{e}}
\xyletcsnamecsname@{frm[o]{=}}{frm{ee}}
\xyletcsnamecsname@{frm[o]{.}}{frm{.e}}
\xyletcsnamecsname@{frm[o]{--}}{frm{-e}}
\xydef@\ellipse@whichfrm@#1{%
 \ifx\frmradius@@\z@
 \frmDrop@{#1\dimen@=.5\L@c \advance\dimen@.5\R@c
 \dimen@ii=.5\U@c \advance\dimen@ii.5\D@c
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}\next@ }%
 \else
 \frmDrop@{#1\expandafter\ellipsed@i@\frmradius@@,,@@}%
 \fi}
\xydef@\ellipse@whichdblfrm@#1{%
 \ifx\frmradius@@\z@
 \frmDrop@{#1\dimen@=.5\L@c \advance\dimen@.5\R@c
 \dimen@ii=.5\U@c \advance\dimen@ii.5\D@c
 \edef\next@{\noexpand\ellipsed@e@{\the\dimen@}{\the\dimen@ii}}\next@ }%
 \else
 \frmDrop@{#1\expandafter\ellipsed@ei@\frmradius@@,,@@}%
 \fi}
\xydef@\ellipsed@i@#1,#2,#3@@{\DNii@{,}\DN@{#3}%
 \ifx\next@\nextii@
 \dimen@=#1\relax \dimen@ii=#2\relax
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}%
 \else \ifx\next@\empty \DN@{#2}%
 \ifx\next@\empty \DN@{#1}%
 \dimen@=.5\L@c \advance\dimen@.5\R@c
 \dimen@ii=.5\U@c \advance\dimen@ii.5\D@c
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}%
 \else \dimen@=#1\relax
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}%
 \fi
 \else\xywarning@{ignoring extra tokens in elliptical frame: #3 }%
 \dimen@=#1\relax \dimen@ii=#2\relax 
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}%
 \fi\fi \next@ }
\xydef@\ellipsed@ei@#1,#2,#3@@{\DNii@{,}\DN@{#3}%
 \ifx\next@\nextii@
 \dimen@=#1\relax \dimen@ii=#2\relax 
 \edef\next@{\noexpand\ellipsed@e@{\the\dimen@}{\the\dimen@ii}}%
 \else \ifx\next@\empty \DN@{#2}%
 \ifx\next@\empty \DN@{#1}%
 \dimen@=.5\L@c \advance\dimen@.5\R@c
 \dimen@ii=.5\U@c \advance\dimen@ii.5\D@c
 \edef\next@{\noexpand\ellipsed@e@{\the\dimen@}{\the\dimen@ii}}%
 \else 
 \dimen@=#1\relax 
 \edef\next@{\noexpand\ellipsed@e@{\the\dimen@}{\the\dimen@}}%
 \fi
 \else\xywarning@{ignoring extra tokens in elliptical frame: #3 }%
 \dimen@=#1\relax \dimen@ii=#2\relax 
 \edef\next@{\noexpand\ellipsed@e@{\the\dimen@}{\the\dimen@ii}}%
 \fi\fi \next@ }
\xydef@\ellipsed@e@#1#2{%
 \dimen@=#1\relax \dimen@ii=#2\relax 
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}\next@ 
 \dimen@=#1\relax \dimen@ii=#2\relax 
 \ifdim\dimen@>2\p@ \advance\dimen@-2\p@ \else \dimen@=\z@\fi
 \ifdim\dimen@ii>2\p@ \advance\dimen@ii-2\p@ \else \dimen@ii=\z@\fi
 \edef\next@{\noexpand\ellipsed@{\the\dimen@}{\the\dimen@ii}}\next@ }%
\xydef@\ellipsed@#1#2{\setboxz@h\bgroup \relax
 \setboxz@h{\vbox{\ellipsed@x@@{#1}{#2}}}%
 \A@=\X@c \advance\A@-.5\wd\z@
 \B@=\Y@c \advance\B@-.5\ht\z@ \advance\B@.5\dp\z@
 \edef\tmp@{\egroup\dimen@=\the\wdz@}%
 \kern\A@ \raise\B@\boxz@
 \tmp@ \divide\dimen@4 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\ellipsed@i#1#2{{\R@c=#1\relax\L@c=\R@c
 \U@c=#2\relax\D@c=\U@c \ellipsed@{#1}{#2}}}
\xydef@\ellipsed@x@#1#2{\R@=#1\relax\advance\R@#2\relax
 \divide\R@\tw@ \circled@x@@ }
\xylet@\ellipsed@x@@=\ellipsed@x@
\xydef@\ellipsesolidframed@{%
 \let\framehfill=\frm@solidh@@ \let\framevfill=\frm@solidv@@}
\xydef@\ellipsedotframed@{%
 \let\framehfill=\frm@doth@@ \let\framevfill=\frm@dotv@@}
\xydef@\ellipsedashframed@{%
 \let\framehfill=\frm@dashh@@ \let\framevfill=\frm@dashv@@}
\xydefcsname@{frm{\{}}{\addtoDrop@@{\lbraced}}
\xydefcsname@{frm{\}}}{\addtoDrop@@{\rbraced}}
\xydefcsname@{frm{^\}}}{\addtoDrop@@{\ubraced}}
\xydefcsname@{frm{_\}}}{\addtoDrop@@{\dbraced}}
\xydef@\dbraced{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracelu$}\dimen@=2\wdz@ \advance\B@-.5\ht\z@
 \ifdim\R@c<\dimen@ \R@c=\dimen@ \fi
 \ifdim\L@c<\dimen@ \advance\A@-\dimen@ \advance\A@\L@c \L@c=\dimen@ \fi
 \advance\A@-.25pt
 \kern\A@\raise\B@\hbox{%
 \hbox to\L@c{$\m@th\bracelu\leaders\vrule\hfil\bracerd$}%
 \kern.5pt
 \hbox to\R@c{$\m@th\braceld\leaders\vrule\hfil\braceru$}}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydef@\ubraced{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@\U@c
 \setboxz@h{$\m@th\bracelu$}\dimen@=2\wdz@
 \ifdim\R@c<\dimen@ \R@c=\dimen@ \fi
 \ifdim\L@c<\dimen@ \advance\A@-\dimen@ \advance\A@\L@c \L@c=\dimen@ \fi
 \advance\A@-.25pt
 \kern\A@\raise\B@\hbox{%
 \hbox to\L@c{$\m@th\braceld\leaders\vrule\hfil\braceru$}%
 \kern.5pt
 \hbox to\R@c{$\m@th\bracelu\leaders\vrule\hfil\bracerd$}}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
{\catcode`\"=12
 \global\mathchardef\braceur="338
 \global\mathchardef\braceul="339
 \global\mathchardef\bracedr="33A
 \global\mathchardef\bracedl="33B
 \global\mathchardef\bracecl="33C
 \global\mathchardef\bracecr="33D
 \global\mathchardef\bracec="33E }
\xydef@\lbraced{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracecl$}\dimen@ii=\dp\z@ \advance\A@-.5\wdz@
 \setboxz@h{$\m@th\bracec$}\dimen@=\dp\z@
 \ifdim\U@c<.5\dimen@ \U@c=.5\dimen@ \fi
 \ifdim\D@c<.5\dimen@ \advance\B@-.5\dimen@ \advance\B@\D@c \D@c=.5\dimen@ \fi
 \advance\U@c.6\p@ \advance\D@c.6\p@ \advance\B@-.6\p@
 \kern\A@\raise\B@\vbox{\vbox to\U@c{%
 \nointerlineskip\hbox{$\m@th\braceur$}%
 \kern-.61\dimen@ \cleaders\copy\z@\vfil \kern-.4\dimen@
 \nointerlineskip\hbox{$\m@th\bracecl$}\kern-.5\dimen@ii}%
 \nointerlineskip\vbox to\D@c{\kern.5\dimen@ii
 \kern-.4\dimen@ \cleaders\copy\z@\vfil \kern-.61\dimen@
 \nointerlineskip\hbox{$\m@th\bracedr$}\kern\z@}}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydef@\rbraced{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@\R@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracecr$}\dimen@ii=\dp\z@ \advance\A@-.5\wdz@
 \setboxz@h{$\m@th\bracec$}\dimen@=\dp\z@
 \ifdim\U@c<.5\dimen@ \U@c=.5\dimen@ \fi
 \ifdim\D@c<.5\dimen@ \advance\B@-.5\dimen@ \advance\B@\D@c \D@c=.5\dimen@ \fi
 \advance\U@c.6\p@ \advance\D@c.6\p@ \advance\B@-.6\p@
 \kern\A@\raise\B@\vbox{\vbox to\U@c{%
 \nointerlineskip\hbox{$\m@th\braceul$}%
 \kern-.61\dimen@ \cleaders\copy\z@\vfil \kern-.4\dimen@
 \nointerlineskip\hbox{$\m@th\bracecr$}\kern-.5\dimen@ii}%
 \nointerlineskip\vbox to\D@c{\kern.5\dimen@ii
 \kern-.4\dimen@ \cleaders\copy\z@\vfil \kern-.61\dimen@
 \nointerlineskip\hbox{$\m@th\bracedl$}\kern\z@}}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydefcsname@{frm{(}}{\addtoDrop@@{\lparenthesized}}
\xydefcsname@{frm{)}}{\addtoDrop@@{\rparenthesized}}
\xydefcsname@{frm{^)}}{\addtoDrop@@{\uparenthesized}}
\xydefcsname@{frm{_)}}{\addtoDrop@@{\dparenthesized}}
\xydef@\dparenthesized{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracelu$}\dimen@=2\wdz@ \advance\B@-.5\ht\z@
 \ifdim\R@c<\dimen@ \R@c=\dimen@ \fi
 \ifdim\L@c<\dimen@ \advance\A@-\dimen@ \advance\A@\L@c \L@c=\dimen@ \fi
 \dimen@=\L@c \advance\dimen@\R@c
 \kern\A@\raise\B@\hbox to\dimen@{%
 $\m@th\bracelu\leaders\vrule\hfil\braceru$}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydef@\uparenthesized{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@\U@c
 \setboxz@h{$\m@th\bracelu$}\dimen@=2\wdz@
 \ifdim\R@c<\dimen@ \R@c=\dimen@ \fi
 \ifdim\L@c<\dimen@ \advance\A@-\dimen@ \advance\A@\L@c \L@c=\dimen@ \fi
 \dimen@=\L@c \advance\dimen@\R@c
 \kern\A@\raise\B@\hbox to\dimen@{%
 $\m@th\braceld\leaders\vrule\hfil\bracerd$}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydef@\lparenthesized{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@-\L@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracecr$}\dimen@ii=\dp\z@ \advance\A@-.5\wdz@
 \setboxz@h{$\m@th\bracec$}\dimen@=\dp\z@
 \ifdim\U@c<.5\dimen@ \U@c=.5\dimen@ \fi
 \ifdim\D@c<.5\dimen@ \advance\B@-.5\dimen@ \advance\B@\D@c \D@c=.5\dimen@ \fi
 \advance\U@c.6\p@ \advance\D@c.6\p@ \advance\B@-.6\p@
 \dimen@ii\U@c \advance\dimen@ii\D@c
 \kern\A@\raise\B@\vbox to \dimen@ii{%
 \nointerlineskip\hbox{$\m@th\braceur$}%
 \kern-.61\dimen@ \cleaders\copy\z@\vfil \kern-.61\dimen@
 \nointerlineskip\hbox{$\m@th\bracedr$}\kern\z@}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydef@\rparenthesized{\xy@@{\setboxz@h{%
 \A@=\X@c \advance\A@\R@c \B@=\Y@c \advance\B@-\D@c
 \setboxz@h{$\m@th\bracecr$}\dimen@ii=\dp\z@ \advance\A@-.5\wdz@
 \setboxz@h{$\m@th\bracec$}\dimen@=\dp\z@
 \ifdim\U@c<.5\dimen@ \U@c=.5\dimen@ \fi
 \ifdim\D@c<.5\dimen@ \advance\B@-.5\dimen@ \advance\B@\D@c \D@c=.5\dimen@ \fi
 \advance\U@c.6\p@ \advance\D@c.6\p@ \advance\B@-.6\p@
 \dimen@ii\U@c \advance\dimen@ii\D@c
 \kern\A@\raise\B@\vbox to \dimen@ii{%
 \nointerlineskip\hbox{$\m@th\braceul$}%
 \kern-.61\dimen@ \cleaders\copy\z@\vfil \kern-.61\dimen@
 \nointerlineskip\hbox{$\m@th\bracedl$}\kern\z@}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}}
\xydefcsname@{frm{*}}{%
 \expandafter\frmDrop@\expandafter{%
 \expandafter\def\expandafter\prevEdge@@\expandafter{\prevEdge@@}%
 \frame@fill@@\frmradius@@}}
\xydefcsname@{frm{**}}{%
 \expandafter\frmDrop@\expandafter{%
 \expandafter\def\expandafter\prevEdge@@\expandafter{\prevEdge@@}%
 \frame@emph@@\frmradius@@}}
\xydef@\frame@fill@#1{\filled@{#1}\empty}
\xydef@\frame@emph@#1{\framed@\frmradius@@}
\xylet@\frame@fill@@=\frame@fill@
\xylet@\frame@emph@@=\frame@emph@
\xydef@\filled@#1{\R@=#1\relax 
 \expandafter\DNii@\expandafter{\prevEdge@@}%
 \DN@{\rectangleEdge}\ifx\next@\prevEdge@@
 \ifdim\R@=\z@ \DN@{\filled@Rectangle@}%
 \else \DN@{\filled@Oval@}\fi
 \else \DN@{\circleEdge}\ifx\next@\prevEdge@@
 \ifdim\R@=\z@ \DN@{\filled@Ellipse@}%
 \else \DN@{\restR@max\filled@Circle@}\fi
 \else 
 \ifdim\R@=\z@ \DN@{\filled@Rectangle@}%
 \else \DN@{\filled@Circle@}\fi
 \fi\fi \next@}
\xydef@\restR@max{%
 \dimen@=\L@c\advance\dimen@\R@c
 \dimen@ii=\U@c \advance\dimen@ii\D@c
 \ifdim\dimen@ii>\dimen@ \dimen@=\dimen@ii\fi
 \ifdim\dimen@>\z@ \divide\dimen@\tw@
 \ifdim\R@>\dimen@\R@=\dimen@\fi\fi }
\xylet@\filledRectangle@@=\bblacked@
\xylet@\filledCircle@@=\bblacked@
\xylet@\filledEllipse@@=\bblacked@
\xylet@\filledOval@@=\bblacked@
\xydef@\filled@Region@#1#2{\setboxz@h\bgroup 
 \setboxz@h{\vbox{#1#2\empty}}%
 \A@=\X@c \advance\A@-.5\wd\z@
 \B@=\Y@c \advance\B@-.5\ht\z@ \advance\B@.5\dp\z@ 
 \edef\tmp@{\egroup\dimen@=\the\wdz@}%
 \kern\A@ \raise\B@\boxz@ \kern-\A@
 \tmp@ \divide\dimen@\tw@ \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \styledboxz@}
\xydef@\filled@Rectangle@{\filled@Region@\filledRectangle@@}
\xydef@\filled@Oval@{\filled@Region@\filledOval@@}
\xydef@\filled@Circle@{\filled@Region@\filledCircle@@}
\xydef@\filled@Ellipse@{\filled@Region@\filledEllipse@@}
\xydefcsname@{shape [F...]}#1{\xyFN@\Fshape@#1:@}
\xylet@\whichframe@@=\empty
\xylet@\whichoptions@@=\empty
\xydef@\Fshape@#1:{\def\whichframe@@{{#1}}%
 \DN@{{}}\ifx\whichframe@@\next@ \def\whichframe@@{{-}}\fi
 \expandafter\DN@\expandafter{\the\Edge@c}\DNii@{\circleEdge}\ifx\next@\nextii@
 \DN@##1{\def\whichframe@@{[o]##1}}%
 \expandafter\next@\expandafter{\whichframe@@}\fi
 \let\whichoptions@@=\empty \xyFN@\Fshape@i}
\xydef@\Fshape@i{%
 \ifx @\next \let\next@=\Fshape@x
 \else\addLT@\ifx\next \let\next@=\Fshape@iii
 \else \let\next@=\Fshape@ii \fi\fi \next@}
\xydef@\Fshape@ii#1:{%
 \expandafter\def\expandafter\whichoptions@@\expandafter{\whichoptions@@[#1]}%
 \xyFN@\Fshape@i}
\xydef@\Fshape@iii#1:{\DN@##1{\def\whichframe@@{#1##1}}%
 \expandafter\next@\expandafter{\whichframe@@}\xyFN@\Fshape@i}
\xydef@\Fshape@x @{%
 \edef\next@##1{\noexpand\addbeforeDrop@@{{\EdgefromtheEdge@##1}}}%
 \DNii@##1##2{\next@{\saveframestyles@{\setbox\z@=\object##2\frm##1%
 \xypre@Style@@\Drop@@\xypost@Style@@\restoreframestyles@}}}%
 \expandafter\expandafter\expandafter\nextii@
 \expandafter\expandafter\expandafter{%
 \expandafter\whichframe@@\expandafter}\expandafter{\whichoptions@@}}
\xydef@\saveframestyles@{%
 \expandafter\def\expandafter\afterframe@preStyle@\expandafter{\preXY@style@}%
 \expandafter\def\expandafter\afterframe@postStyle@\expandafter{\postXY@style@}}
\xydef@\restoreframestyles@{%
 \expandafter\gdef\expandafter\preXY@style@\expandafter{\afterframe@preStyle@}%
 \expandafter\gdef\expandafter\postXY@style@\expandafter{\afterframe@postStyle@}%
 \def\afterframe@preStyle@{}\def\afterframe@postStyle@{}}
\xydef@\xycircleframe@x@{\L@=\R@ \xycircleframe@x@i}%
\xydef@\xyellipseframe@x@#1#2{\R@=#1\relax \L@=#2\relax \xycircleframe@x@i}
\xydef@\xycircleframe@x@i{%
 \ifx\framehfill\frm@solidh@@\def\circleSTYLE@{}%
 \else\ifx\framehfill\frm@doth@@
 \expandafter\def\expandafter\circleSTYLE@\expandafter{\addDOT@{}}%
 \else\ifx\framehfill\frm@dashh@@
 \expandafter\expandafter\expandafter\def\expandafter\expandafter
 \expandafter\circleSTYLE@\expandafter\expandafter\expandafter
 {\expandafter\addDASH@\addDASH@{}}%
 \fi\fi\fi \xycircleframe@x@x }
\xydef@\xycircleframe@x@x{\hbox{\vbox{\vskip\L@
 \hbox to2\R@{\hfill \buildcircle@ \hfill}\vskip\L@ }}}
\xydef@\UseCurveFrames@{%
 \let\circled@x@@=\xycircleframe@x@
 \let\ellipsed@x@@=\xyellipseframe@x@ }
\def\UseCurveFrames{\xywithoption{curve}{\UseCurveframes@}}%
\xydef@\UseFontFrames@{%
 \let\circled@x@@=\circled@x@
 \let\ellipsed@x@@=\ellipsed@x@ }
\xylet@\UseFontFrames=\UseFontFrames@
\xydef@\UnloadFrames@{%
 \let\framed@body@@=\framed@body@
 \let\circled@x@@=\circled@x@
 \let\ellipsed@x@@=\ellipsed@x@
 \let\frame@fill@@=\frame@fill@
 \let\frame@emph@@=\frame@emph@
 \let\filledRectangle@@=\bblacked@
 \let\filledCircle@@=\bblacked@
 \let\filledEllipse@@=\bblacked@
 \let\filledOval@@=\bblacked@
}
\xyaddunsupport{frame}\UnloadFrames@
\xyendinput


==> xygraph.tex <==
%% xygraph.tex from $Id: xygraph.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Graph Combinator feature'' option.
%% Copyright (c) 1994-1997 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{graph}{Graph feature}{\stripRCS$Revision: 3.11 $}%
 {Kristoffer H.~Rose}{krisrose@tug.org}%
 {IBM T.~ J.\ Watson Research Center, P.O.~Box 704, Yorktown Heights, NY 10598 (USA)}
\xyrequire{arrow}\xycatcodes
\xydef@\xygraph#1{\relax\graph#1\endgraph}
\xydef@\graph{\if\inxy@ \DN@{\xy@@{\nter@{}}}%
 \else \DN@{\xy \xy@\xy{\nter@\endxy}}\fi \next@
 \xy@\xygraph{\senter@ \idfromc@{?NODE}\spushc@
 \expandafter\let\expandafter\next@\csname Q@graphbase\endcsname
 \ifx\next@\relax \setbase@\z@\z@{3pc}\z@
 \else \expandafter\next@ \fi}%
 \GRAPH[]}
\xydef@\endgraph{\ignorespaces}
\xydef@\GRAPH{\xyFN@\GRAPH@}
\xydef@\GRAPH@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\GRAPH@}%
 \else\ifx :\next \DN@:{\xy@:{}\expandafter\GRAPHar@\GRAPHeveryarrow@@}%
 \else\addDASH@\ifx\next
 \addDASH@\DN@{\xy@-{}\expandafter\GRAPHar@\GRAPHeveryline@@}%
 \else\ifx (\next
 \DN@({\xy@({\spushid@{?NODE}\idfromc@{?NODE}}\xyFN@\GRAPH@}%
 \else\ifx ,\next
 \DN@,{\xy@,{\cfromid@{?NODE}}\xyFN@\GRAPH@}%
 \else\ifx )\next
 \DN@){\xy@){\cfromid@{?NODE}%
 \tests@\z@{\idfroms@{?NODE}\z@ \spop@}{\xyerror@{) without (}{}}}%
 \xyFN@\GRAPH@}%
 \else\ifx \endgraph\next \DN@{\xy@@{\tests@\z@\spop@\sleave@\leave@}}%
 \else\ifx \end\next \DN@{\xy@@{\tests@\z@\spop@\sleave@\leave@}}%
 \else\ifx ~\next
 \DN@~{\xy@@{\enter@\cfromthec@}\afterNODE{\leave@ \xyFN@\GRAPH@}!}%
 \else \DN@{\afterNODE{\xyFN@\GRAPH@}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xylet@\GRAPHsaved@PATHafterPOS=\PATHafterPOS
\xylet@\GRAPHsaved@afterar@@=\afterar@@
\xydef@\GRAPHar@{%
 \let\PATHafterPOS=\afterNODE \let\afterar@@=\GRAPHafterar@ \ar}
\xydef@\GRAPHafterar@{%
 \let\PATHafterPOS=\GRAPHsaved@PATHafterPOS
 \let\afterar@@=\GRAPHsaved@afterar@@
 \xy@@{\cfromid@{}}\xyFN@\GRAPH@}
\xylet@\afterNODE@@=\empty
\xydef@\afterNODE#1{\xy@@{\enter@\pfromthep@}%
 \DN@##1{\def\afterNODE@@{\xy@@\leave@ \def\afterNODE@@{##1}#1}}%
 \expandafter\next@\expandafter{\afterNODE@@}%
 \xyFN@\NODE@}
\xylet@\theMOVE@@=\relax
\xydef@\NODE@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\NODE@}%
 \else\ifx [\next \DN@[##1]{\xy@{[##1]}{}%
 \def\theMOVE@@{[##1]}\xyFN@\MOVE@##1]}%
 \else\ifx "\next \DN@ "##1"{%
 \xy@{"##1"}{\cfromid@{##1}}\def\theMOVE@@{"##1"}\xyFN@\NODE@i}%
 \else\ifx ?\next \DN@ ?{%
 \xy@?{\cfromid@{?NODE}}\def\theMOVE@@{?}\xyFN@\NODE@i}%
 \else\ifx !\next \def\theMOVE@@{[]}\let\next@=\NODE@i
 \else \testAND@\iffalse
 \DN@##1{\xy@{}{\pfromc@ \advance\X@c\X@xbase \advance\Y@c\Y@xbase
 \czeroEdge@}\jumpMOVE@ \xyFN@\NODE@i}%
 \else\ifx \\\next
 \DN@\\{\xy@\\{\pfromc@ \advance\X@c\X@xbase \advance\Y@c\Y@xbase
 \R@c=\X@ybase \U@c=\Y@ybase \intersect@
 \advance\X@c-\X@ybase \advance\Y@c-\Y@ybase
 \czeroEdge@}\def\theMOVE@@{\\}\xyFN@\NODE@i}%
 \else \xyerror@{Illegal <node>: \string`\meaning\next\string' unexpected}{}%
 \fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\jumpMOVE@@{&}
\xydef@\jumpMOVE@{\let\theMOVE@@=\jumpMOVE@@}
\xydef@\MOVE@{\xy@@{\count@=\z@ \count@@=\z@}%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\MOVE@}%
 \else\ifcat A\noexpand\next \let\next@=\MOVE@letter
 \else \let\next@=\MOVE@x \fi\fi \next@}
\xydef@\MOVE@letter{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\MOVE@letter}%
 \else\ifx u\next \DN@ u{\xy@@{\advance\count@\@ne}\xyFN@\MOVE@letter}%
 \else\ifx d\next \DN@ d{\xy@@{\advance\count@\m@ne}\xyFN@\MOVE@letter}%
 \else\ifx l\next \DN@ l{\xy@@{\advance\count@@\m@ne}\xyFN@\MOVE@letter}%
 \else\ifx r\next \DN@ r{\xy@@{\advance\count@@\@ne}\xyFN@\MOVE@letter}%
 \else \let\next@=\MOVE@x \fi\fi\fi\fi\fi \next@}
\xydef@\MOVE@x{%
 \ifx ]\next \DN@ ]{\MOVE@hop \xyFN@\NODE@i}%
 \else\ifx (\next \DN@{\MOVE@hop \xyFN@\MOVE@place}%
 \else\ifx !\next \DN@{\MOVE@hop \xyFN@\MOVE@place}%
 \else\ifx /\next \DN@{\MOVE@hop \xyFN@\MOVE@place}%
 \else\addLT@\ifx\next \DN@{\MOVE@hop \xyFN@\MOVE@place}%
 \else\addGT@\ifx\next \DN@{\MOVE@hop \xyFN@\MOVE@place}%
 \else\addDASH@\ifx\next \addDASH@\DN@{\xyerror@{- not implemented yet}{}}%
 \else \xyerror@{illegal <move>: \codeof\theMOVE@@}{}\let\next@=\NODE@i
 \fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\MOVE@hop{\xy@@{\pfromc@ \czeroEdge@
 \edef\next@{\the\count@@,\the\count@ @}\expandafter\vfromcartesian@@\next@
 \advance\X@c-\X@origin \advance\Y@c-\Y@origin
 \advance\X@c\X@p \advance\Y@c\Y@p}}
\xydef@\MOVE@place{\xy@@\no@@ \afterPLACE{\xyFN@\MOVE@}}
\xydef@\NODE@i{\let\next@=\NODE@x
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\NODE@i}%
 \else\addEQ@\ifx \next
 \addEQ@\DN@"##1"{\xy@{="##1"}{\idfromc@{##1}}\xyFN@\NODE@i}%
 \else\ifx !\next \DN@!{\xyFN@\NODE@escape}%
 \else\ifx :\next 
 \else\addDASH@\ifx\next
 \else\ifx (\next
 \else\ifx ,\next
 \else\ifx )\next
 \else\ifx ~\next
 \else\ifx [\next
 \else\ifx "\next
 \else\ifx ?\next
 \else\ifx ^\next
 \else\ifx _\next
 \else\ifx |\next
 \else\addLQ@\ifx\next
 \else\addRQ@\ifx\next
 \else \testAND@ \iffalse
 \else\ifx \\\next
 \else\ifx \endgraph\next
 \else\ifx \end\next
 \else \let\next@=\NODE@it
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\NODE@x{\xy@@{\idfromc@{}}\afterNODE@@}
\xydef@\NODE@it{\let\PATHlabelit@@=\NODEit@ \PATHit@}
{\xyuncatcodes \gdef\next{+}}
\xylet@\GRAPHnodemodifiers@@=\next
\xydef@\NODEit@#1{%
 \DN@{#1}\ifx\next@\empty
 \DN@{\expandafter\NODEit@i\expandafter{\GRAPHnodemodifiers@@}}%
 \else \DN@{\NODEit@i{#1}}\fi \next@}
\def\NODEit@i#1#2{\xy@{*#1{#2}}{\drop@{#1}{#2}}%
 \DN@{\addEQ@\ifx\next\else \xy@@{\idfromc@{#2}}\fi \NODE@i}%
 \xyFN@\next@}
\xydef@\NODE@escape{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\NODE@escape}%
 \else\ifcat A\noexpand\next \DN@##1{\rungraphescape@{##1}}%
 \else\ifcat !\noexpand\next \DN@##1{\rungraphescape@{##1}}%
 \else\ifx \bgroup\next \DN@##1{\xy@{!{##1}}{}\POS##1\relax \xyFN@\NODE@i}%
 \else\ifx ~\next \let\next@=\graphsetup@
 \else \DN@{\xyerror@{Unknown graph <escape>}{}\xyFN@\NODE@i}%
 \fi\fi\fi\fi\fi \next@}
\xydefcsname@{graph !M}#1#{\NODE@matrix{#1}}
\xydef@\NODE@matrix#1#2{\xyerror@{matrix feature not loaded}{}\xyFN@\GRAPH@}
\xydef@\NODE@matrix@#1#2{\xy@{!M#1{#2}}{}%
 \def\everyentry@{\GRAPHeveryentry}%
 \xymatrix#1{#2}%
 \let\everyentry@=\empty \insertmatrixingraph@ \xyFN@\NODE@i}
\xydef@\GRAPHeveryentry{\def\:{\ar}\def\="##1"{\xy@@{\idfromc@{##1}}}}
\xywithoption{matrix}{\let\NODE@matrix=\NODE@matrix@}
\xydef@\insertmatrixingraph@{%
 \xy@@{\enter@{\cfromthec@ \pfromthep@}%
 \expandafter\let\expandafter\next@\csname Q@1,1\endcsname
 \ifx\next@\relax\else
 \next@ \swap@
 \expandafter\let\expandafter\next@\csname Q@1,2\endcsname
 \ifx\next@\relax\else \next@ \setbase@\X@p\Y@p\X@c\Y@c
 \expandafter\let\expandafter\next@\csname Q@2,1\endcsname
 \ifx\next@\relax\else
 \next@ \setbase@@{-\X@c}{-\Y@c}\fi\fi\fi
 \leave@}}
\xydefcsname@{graph !P}#1#{\NODE@poly{#1}}
\xydef@\NODE@poly#1#2{\xyerror@{poly(gon) feature not loaded}{}\xyFN@\GRAPH@}
\xydef@\NODE@poly@#1#2{\xy@{!P#1{#2}}{}\xypoly@#1{#2}\xyFN@\NODE@i}
\xywithoption{poly}{\let\NODE@poly=\NODE@poly@}
\xydefcsname@{graph !E}#1#{\NODE@arc{#1}!}
\xydef@\NODE@arc#1#2{\xyerror@{(ellipse+)arc feature not loaded}{}%
 \xyFN@\GRAPH@}
\xydef@\NODE@arc@#1#2{\xy@{!E#1{#2}}{}\ellipse#1{#2}\xyFN@\NODE@i}
\xywithoption{arc}{\let\NODE@arc=\NODE@arc@}
\xylet@\GRAPHeveryarrow@@=\empty
{\xyuncatcodes \gdef\next{@{-}}}
\xylet@\GRAPHeveryline@@=\next
\xydef@\graphsetup@~{\xyFN@\graphsetup@i}
\xydef@\graphsetup@i{%
 \ifx :\next \DN@:##1{\def\GRAPHeveryarrow@@{##1}\xyFN@\NODE@i}%
 \else\addDASH@\ifx\next
 \addDASH@\DN@##1{\def\GRAPHeveryline@@{##1}\xyFN@\NODE@i}%
 \else\ifx *\next \DN@*##1{\def\GRAPHnodemodifiers@@{##1}\xyFN@\NODE@i}%
 \else\ifcat A\next \DN@##1##2{\newgraphescape{##1}{##2}\xyFN@\NODE@i}%
 \else \DN@{\xyerror@{illegal graph setup \codeof\next@}{}\xyFN@\NODE@i}%
 \fi\fi\fi\fi \next@}
\xydef@\newgraphescape#1{%
 \expandafter\let\expandafter\next\csname graph !#1\endcsname
 \ifx\next\relax\else \expandafter\let\csname G!#1\endcsname=\undefined
 \xywarning@{Redefining graph <escape> !#1}\fi
 \expandafter\gdef\csname graph !#1\endcsname{%
 \expandafter\let\expandafter\next\csname G!#1\endcsname
 \expandafter\xyFN@\expandafter\NODE@\next}%
 \DN@{\newgraphescape@{#1}}\xyFN@\next@}
\xydef@\newgraphescape@#1{%
 \ifx [\next
 \ifx\newcommand\undefined \xyerror@{[n] only with LaTeX}%
 \else
 \def\nextiv@{\expandafter\newcommand\expandafter{\csname G!#1\endcsname}}\fi
 \else \def\nextiv@{\expandafter\gdef\csname G!#1\endcsname}\fi \nextiv@}
\xydef@\rungraphescape@#1{%
 \expandafter\let\expandafter\next\csname graph !#1\endcsname
 \ifx\next\relax \xyerror@{Undefined graph <escape> !#1}\fi \next}
\xyendinput


==> xyidioms.tex <==
%% xyidioms.tex from $Id: xyidioms.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Format-dependent idioms for Xy-pic.
%% Copyright (c) 1991-1997 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyidiomsloaded\empty \message{not reloaded}\endinput \fi
\let\xyidiomsloaded=\empty
\xywarnifdefined\A@ \dimendef\A@=4
\xywarnifdefined\B@ \dimendef\B@=6
\xywarnifdefined\R@ \dimendef\R@=8
\ifx\undefined\AveryUNLIKELYc@ntr@lSEQUENCE@@\else
\errmessage{Xy-pic Error: \string\undefined\space defined.}\fi
\ifx\undefined\literal@ \def\literal@#1{#1}\fi
\ifx\undefined\eat@ \def\eat@#1{}\fi
\xydef@\xyFN@{\futurelet\next}
\ifx\undefined\DN@ \def\DN@{\def\next@}\fi
\ifx\undefined\DNii@ \def\DNii@{\def\nextii@}\fi
\ifx\undefined\setboxz@h\def\setboxz@h{\setbox\z@\hbox}\fi
\ifx\undefined\wdz@ \def\wdz@{\wd\z@}\fi
\ifx\undefined\boxz@ \def\boxz@{\box\z@}\fi
\ifx\undefined\W@ \def\W@{\immediate\write16 }\fi
\ifx\undefined\space@ \def\space@.{\futurelet\space@\relax}\space@. \fi
\ifx\undefined\notempty \def\notempty#1{T\if @#1@F\else T\fi}\fi
\xydef@\xysetup@dummy#1{\xyuncatcodes#1}
\xywarnifdefined\xysetup@@
\ifx\AtEndDocument\undefined
 \expandafter\ifx\csname amsppt.sty\endcsname\relax
 \let\xysetup@@=\xysetup@dummy
 \else
 \def\xysetup@@#1{%
 \expandafter\def\expandafter\topmatter\expandafter{\topmatter
 #1\xyuncatcodes}}\fi
\else
 \def\xysetup@@#1{\AtBeginDocument{#1\xyuncatcodes}}
\fi
\ifx\xysetup@@\xysetup@dummy\else
 \xysetup@@{\let\xysetup@@=\xysetup@dummy \xyuncatcodes}\fi
\xywarnifdefined\xyclosedown@@
\ifx\AtEndDocument\undefined \let\xyclosedown@@=\eat@
\else \def\xyclosedown@@#1{\AtEndDocument{#1}}\fi
\xylet@\xy@begindvi=\literal@
\ifx\undefined\AtBeginDvi\else
 \AtBeginDocument{\let\xy@begindvi=\AtBeginDvi}
 \AtBeginDvi{\global\let\xy@begindvi=\literal@}\fi
\ifx\amstexloaded@\relax
\xylet@\toks@ii=\toks@@ \endinput \fi
\ifx\@tempcnta\undefined
\xynew@{count}\count@@
\xynew@{count}\count@@@
\else
\xylet@\count@@=\@tempcnta
\xylet@\count@@@=\@tempcntb
\fi
\ifx\undefined\toks@ii \toksdef\toks@ii=2 \fi
\endinput


==> xyimport.tex <==
%% xyimport.tex from $Id: xyimport.doc,v 3.13 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Import feature'' option.
%% Copyright (c) 1993-1997 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{import}{Import graphics extension}{\stripRCS$Revision: 3.13 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\xyimport#1#{\xyimport@{#1}}
\xydef@\xyimport@#1#2{\xydelayimport@{#1}{#2}}
\xydef@\xydelayimport@#1#2{\xy@@ix@{#1{#2}}%
 \xy@@{\expandafter\xyextern@\the\toks9}}
\xydef@\xyextern@(#1,#2){\hbox\bgroup\R@c=#1\p@ \U@c=#2\p@\xyextern@i}
\xydef@\xyextern@i#1#{\DN@{#1}%
 \ifx\next@\empty \L@c=\z@ \D@c=\z@ \DN@{\xyextern@x}%
 \else \DN@{\xyextern@ii#1}\fi \next@ }
\xydef@\xyextern@ii(#1,#2){\L@c=#1\p@ \D@c=#2\p@ 
 \advance\R@c-\L@c \advance\U@c-\D@c \xyextern@x}
\xydef@\xyimportdefault@{3}
\xydef@\xyexportwarning@#1#2#3{\xywarning@{%
 #1 for import has zero #2; using \xyimportdefault@#3 default}}
\xydef@\xyextern@x#1{\toks@={\egroup\L@c=}\setboxz@h{#1}%
 \dimen@ii=\L@c \advance\dimen@ii\R@c \dimen@=\wdz@ 
 \ifdim\dimen@=\z@ \xyexportwarning@{graphic}{width}{cm}%
 \dimen@=\xyimportdefault@ cm\fi
 \ifdim\dimen@ii=\z@ \xyexportwarning@{coords}{width}{unit}%
 \dimen@ii=\xyimportdefault@\p@\fi
 \quotient@\next@\dimen@\dimen@ii \dimen@=\next@\p@
 \edef\tmp@{\expandafter\removePT@\the\L@c}\L@c=\tmp@\dimen@
 \expandafter\addtotoks@\expandafter{\the\L@c\relax\R@c=}%
 \edef\tmp@{\expandafter\removePT@\the\R@c}\R@c=\tmp@\dimen@
 \expandafter\addtotoks@\expandafter{\the\R@c\relax\setbase@\z@\z@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\the\dimen@}\z@\D@c=}%
 \dimen@ii=\U@c \advance\dimen@ii\D@c \dimen@=\ht\z@\advance\dimen@\dp\z@
 \ifdim\dimen@=\z@ \xyexportwarning@{graphic}{height}{cm}%
 \dimen@=\xyimportdefault@ cm\fi
 \ifdim\dimen@ii=\z@ \xyexportwarning@{coords}{height}{unit}%
 \dimen@ii=\xyimportdefault@\p@\fi
 \quotient@\next@\dimen@\dimen@ii \dimen@=\next@\p@
 \edef\tmp@{\expandafter\removePT@\the\D@c}\D@c=\tmp@\dimen@
 \expandafter\addtotoks@\expandafter{\the\D@c\relax\U@c=}%
 \edef\tmp@{\expandafter\removePT@\the\U@c}\U@c=\tmp@\dimen@
 \expandafter\addtotoks@\expandafter{\the\U@c\relax\setbase@@\z@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\the\dimen@}}%
 \setboxz@h{\kern-\L@c\lower\D@c\boxz@\kern\L@c}%
 \wd\z@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@ \the\toks@ \X@c=\z@ \Y@c=\z@
 \ifdim\X@min>-\L@c \X@min=-\L@c \fi \ifdim\X@max<\R@c \X@max=\R@c \fi
 \ifdim\Y@min>-\D@c \Y@min=-\D@c \fi \ifdim\Y@max<\U@c \Y@max=\U@c \fi
 \idfromc@{import}\POS }
\xyendinput


==> xyknot.tex <==
%% xyknot.tex from $Id: xyknot.doc,v 3.9 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Knots and Links'' feature.
%% Copyright (c) 1994-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this macro package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{knot}{Knots and Links feature}{\stripRCS$Revision: 3.9 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\message{knots and links,}
\xyrequire{arrow}\xycatcodes 
\xydef@\xykparsecross@{%
 \def\xykSCALE@@{}\edef\xyknotPLACE{\xykmidPLACE@}%
 \let\xykparser@=\xykparsecross@@
 \def\xykdefaultbreak@{\let\xykbreak@=\xykforetemp@
 \def\xyknotPLACE{(.5)}\appendtoholder@}%
 \xyFN@\xykparsescale@ }
{\xyuncatcodes \catcode`@=11
\gdef\next{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xykparsecross@@}%
 \else\addLT@\ifx\next \addLT@\DN@{\xyprecross@}%
 \else\addGT@\ifx\next \addGT@\DN@{\xypostcross@}%
 \else\addEQ@\ifx\next \addEQ@\DN@{\xyFN@\xykparsetips@@}%
 \else\ifx|\next\DN@|{\xymidcross@}%
 \else\addAT@\ifx\next \addAT@\DN@(##1){%
 \xyadjustBREAK@i##1@@\xyFN@\xykparsecross@@}%
 \else\DN@{\afterknot@}%
 \fi\fi\fi\fi\fi\fi \next@ }}
\xylet@\xykparsecross@@=\next
\xydef@\xyprecross@{%
 \def\xykholder@{\xykprebreak@@}%
 \edef\xyknotPLACE{\xykprePLACE@}%
 \xyFN@\xykparsebreak@}
\xydef@\xypostcross@{%
 \def\xykholder@{\xykpostbreak@@}%
 \edef\xyknotPLACE{\xykpostPLACE@}%
 \xyFN@\xykparsebreak@}
\xydef@\xymidcross@{%
 \def\xykholder@{\xykmidbreak@@}%
 \edef\xyknotPLACE{\xykmidPLACE@}%
 \xyFN@\xykparsebreak@}
\xydef@\xykcross@#1{\xykcheckTIPS@
 \expandafter\toks@\expandafter{\expandafter#1\knotSTYLE}}
\xydef@\xykoverstring@{\addtotoks@{{}}\xykmidbreak@ \xyknottips@}
\xydef@\xykunderstring@{\xykprebreak@ \xykpostbreak@ \xyknottips@}
\xydef@\vcross{\begingroup\def\afterknot@{\xyvcross}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\hcross{\begingroup\def\afterknot@{\xyhcross}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vcrossneg{\begingroup\def\afterknot@{\xyvcrossneg}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\hcrossneg{\begingroup\def\afterknot@{\xyhcrossneg}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vuncross{\begingroup\def\afterknot@{\xyvuncross}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\huncross{\begingroup\def\afterknot@{\xyhuncross}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xyvcross{\xykcross@\xykcrossv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhcross{\xykcross@\xykcrossh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyvcrossneg{\xykcross@\xykcrossv
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhcrossneg{\xykcross@\xykcrossh
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyvuncross{\xykcross@\xykuncrossv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhuncross{\xykcross@\xykuncrossh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz_\ar #1@'{"_<"**{}?(.25)@+,?+(.375,0)@+,
 "_>";"^>"**{}?-(.375,0)@+,?(.25)@+}"_>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"^<"**{}?(.25)@+,?+(.375,0)@+,
 "^>";"_>"**{}?-(.375,0)@+,?(.25)@+}"^>"#6#7#8}
 \restore\POS #9}}
\xylet@\xykcrossv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "_<",{\xykz_\ar #1@'{"_>"**{}?(.25)@+,?+(0,.375)@+,
 "^>";"^<"**{}?-(0,.375)@+,?(.25)@+}"^>"#3#4#5},
 "_>",{\xykz^\ar #2@'{"_<"**{}?(.25)@+,?+(0,.375)@+,
 "^<";"^>"**{}?-(0,.375)@+,?(.25)@+}"^<"#6#7#8}
 \restore\POS #9}}
\xylet@\xykcrossh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz^\ar #1@'{"_<"**{}?(.25)@+,?(.375)+(.375,0)@+,
 "^>";"_>"**{}?(.375)-(.375,0)@+,?(.25)@+}"^>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"^<"**{}?(.25)@+,?(.375)+(.375,0)@+,
 "_>";"^>"**{}?(.375)-(.375,0)@+,?(.25)@+}"_>"#6#7#8}
 \restore\POS #9}}
\xylet@\xykuncrossv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "_<",{\xykz^\ar #1@'{"_>"**{}?(.25)@+,?(.375)+(0,.375)@+,
 "^<";"^>"**{}?(.375)-(0,.375)@+,?(.25)@+}"^<"#3#4#5},
 "_>",{\xykz^\ar #2@'{"_<"**{}?(.25)@+,?(.375)+(0,.375)@+,
 "^>";"^<"**{}?(.375)-(0,.375)@+,?(.25)@+}"^>"#6#7#8}
 \restore\POS #9}}
\xylet@\xykuncrossh=\next
\xydef@\vover{\begingroup\def\afterknot@{\xyvover}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.8)}\def\xykpostbreak@@{|(.725)\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\hover{\begingroup\def\afterknot@{\xyhover}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.8)}\def\xykpostbreak@@{|(.725)\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vunder{\begingroup\def\afterknot@{\xyvunder}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.2)}\def\xykpostbreak@@{|(.275)\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\hunder{\begingroup\def\afterknot@{\xyhunder}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.2)}\def\xykpostbreak@@{|(.275)\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vunover{\begingroup\def\afterknot@{\xyvunover}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.8)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\hunover{\begingroup\def\afterknot@{\xyhunover}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.8)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xoverv{\begingroup\def\afterknot@{\xyxoverv}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.15)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\xunderv{\begingroup\def\afterknot@{\xyxunderv}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.15)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\xoverh{\begingroup\def\afterknot@{\xyxoverh}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.15)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\xunderh{\begingroup\def\afterknot@{\xyxunderh}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.85)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\xunover{\begingroup\def\afterknot@{\xyxunover}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.15)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xunoverv{\begingroup\def\afterknot@{\xyxunoverv}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.2)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xunoverh{\begingroup\def\afterknot@{\xyxunoverh}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.8)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xyvover{\xykcross@\xykoverv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhover{\xykcross@\xykoverh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyvunder{\xykcross@\xykoverv
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhunder{\xykcross@\xykoverh
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyvunover{\xykcross@\xykunoverv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhunover{\xykcross@\xykunoverh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyxoverv{\xykcross@\xykxoverv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyxunderv{\xykcross@\xykxoverv
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyxoverh{\xykcross@\xykxoverh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyxunderh{\xykcross@\xykxoverh
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyxunover{\xykcross@\xykxoverv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyxunoverv{\xykcross@\xykxunoverv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyxunoverh{\xykcross@\xykxunoverh
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz^\ar #1@'{"^>"**{}?(.25)@+,?(.625)+(0,-.125)@+,
 "_>";"^>"**{}?(.625)-(.125,0)@+,?(.25)@+}"_>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"^<"**{}?(.25)@+,?(.625)+(.125,0)@+,
 "^>";"^<"**{}?(.625)-(0,.125)@+,?(.25)@+}"^>"#6#7#8},\restore\POS#9}}
\xylet@\xykoverv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "_<",{\xykz^\ar #1@'{"^<"**{}?(.25)@+,?(.625)+(.125,0)@+,
 "^>";"^<"**{}?(.625)-(0,.125)@+,?(.25)@+}"^>"#3#4#5},
 "_>",{\xykz^\ar #2@'{"_<"**{}?(.25)@+,?(.625)+(0,.125)@+,
 "^<";"_<"**{}?(.625)+(.125,0)@+,?(.25)@+}"^<"#6#7#8},\restore\POS#9}}
\xylet@\xykoverh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz^\ar #1@'{"^>"**{}?(.25)@+,?-(0,.175)@+,?(.75)@+}
 "^>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"^<"**{}?(.25)@+,?+(.125,0)@+,
 "_>"**{}?+(0,.7)@+,"_>";"^>"**{}?-(.125,0)@+,?(.25)@+}
 "_>"#6#7#8},\restore\POS#9}}
\xylet@\xykunoverv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "_<",{\xykz^\ar #1@'{"^<"**{}?(.25)@+,?+(.175,0)@+,?(.75)@+}
 "^<"#3#4#5},
 "_>",{\xykz^\ar #2@'{"_<"**{}?(.25)@+,?+(0,.125)@+,
 "^>"**{}?-(.7,0)@+,"^>";"^<"**{}?-(0,.125)@+,?(.25)@+}
 "^>"#6#7#8},\restore\POS#9}}
\xylet@\xykunoverh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<";"^>"**{}?="^_","_<";"_>"**{}?;"^_",**{}?="^_",
 "^>",{\xykz^\ar #1@'{"^_"@+}"_<"#3#4#5},
 "^<",{\xykz_\ar #2@'{"^_"@+}"_>"#6#7#8},\restore\POS#9}}
\xylet@\xykxoverv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<";"_<"**{}?="^_","^>";"_>"**{}?;"^_",**{}?="^_",
 "^<",{\xykz_\ar #1@'{"^_"@+}"_>"#3#4#5},
 "_<",{\xykz_\ar #2@'{"^_"@+}"^>"#6#7#8},\restore\POS#9}}
\xylet@\xykxoverh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<";"^>"**{}?="^_","_<";"_>"**{}?;"^_",**{}?="^_",
 "^>",{\xykz^\ar #1@'{"^_"@+}"_>"#3#4#5},
 "^<",{\xykz^\ar #2@'{"^_"@+}"_<"#6#7#8},\restore\POS#9}}
\xylet@\xykxunoverv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<";"_<"**{}?="^_","^>";"_>"**{}?;"^_",**{}?="^_",
 "^<",{\xykz^\ar #1@'{"^_"@+}"^>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"^_"@+}"_>"#6#7#8},
 \restore\POS#9}}
\xylet@\xykxunoverh=\next
\xydef@\vtwist{\begingroup\def\afterknot@{\xyvtwist}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\htwist{\begingroup\def\afterknot@{\xyhtwist}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vtwistneg{\begingroup\def\afterknot@{\xyvtwistneg}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\htwistneg{\begingroup\def\afterknot@{\xyhtwistneg}%
 \def\xykprePLACE@{(.1)}\def\xykpostPLACE@{(.9)}%
 \def\xykmidPLACE@{(.9)}\def\xykpostbreak@@{|\knothole}%
 \xyFN@\xykparsecross@ }%
\xydef@\vuntwist{\begingroup\def\afterknot@{\xyvuntwist}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.85)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\huntwist{\begingroup\def\afterknot@{\xyhuntwist}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.85)}%
 \def\xykmidPLACE@{(.85)}\def\xykpostbreak@@{}%
 \xyFN@\xykparsecross@ }%
\xydef@\xyvtwist{\xykcross@\xyktwistv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyvtwistneg{\xykcross@\xyktwistv
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyvuntwist{\xykcross@\xykuntwistv
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(0,-1)}}
\xydef@\xyhtwist{\xykcross@\xyktwisth
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyhuntwist{\xykcross@\xykuntwisth
 \xykoverstring@ \xykunderstring@ \xykhvobject@{+(1,0)}}
\xydef@\xyhtwistneg{\xykcross@\xyktwisth
 \xykunderstring@ \xykoverstring@ \xykhvobject@{+(1,0)}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^>",{\xykz_\ar #1@'{"_>"**{}?(.25)@+,?-(.375,0)@+,
 "_<";"^<"**{}?+(.375,0)@+,?(.25)@+}"_<"#3#4#5},
 "^<",{\xykz^\ar #2@'{"_<"**{}?(.25)@+,?+(.375,0)@+,
 "_>";"^>"**{}?+(-.375,0)@+,?(.25)@+}"_>"#6#7#8}
 \restore\POS #9}}
\xylet@\xyktwistv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^>",{\xykz^\ar #1@'{"_>"**{}?(.125)@+,?(.375)-(.25,0)@+,
 ?(.625)-(.25,0)@+,?(.875)@+}"_>"#3#4#5},
 "^<",{\xykz^\ar #2@'{"_<"**{}?(.125)@+,?(.375)+(.25,0)@+,
 ?(.625)+(.25,0)@+,?(.875)@+}"_<"#6#7#8}
 \restore\POS #9}}
\xylet@\xykuntwistv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz_\ar #1@'{"^>"**{}?(.25)@+,?+(0,-.375)@+,
 "_>";"_<"**{}?+(0,.375)@+,?(.25)@+}"_>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"_>"**{}?(.25)@+,?+(0,.375)@+,
 "^>";"^<"**{}?-(0,.375)@+,?(.25)@+}"^>"#6#7#8}
 \restore\POS #9}}
\xylet@\xyktwisth=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\save,
 "^<",{\xykz^\ar #1@'{"^>",**{}?(.125)@+,?(.375)+(0,-.25)@+,
 ?(.625)+(0,-.25)@+,?(.875)@+}"^>"#3#4#5},
 "_<",{\xykz^\ar #2@'{"_>",**{}?(.125)@+,?(.375)+(0,.25)@+,
 ?(.625)+(0,.25)@+,?(.875)@+}"_>"#6#7#8},\restore\POS #9}}
\xylet@\xykuntwisth=\next
\xydef@\xykparsescale@{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xykparsescale@}%
 \else\addDASH@\ifx\next \addDASH@\DN@{\def\xykSCALE@@{-1}%
 \xyFN@\xykparser@}%
 \else\ifx[\next \DN@[##1]{\dimen@=##1\p@
 \ifdim\dimen@=\z@\xywarning@{\xykscaleerror@}%
 \else\edef\xykSCALE@@{\expandafter\removePT@\the\dimen@}\fi
 \xyFN@\xykparser@}%
 \else\ifx~\next \DN@~##1##2##3##4{%
 \def\xykSCALE@@{@{##1}{##2}{##3}{##4}}\xyFN@\xykparser@}%
 \else\DN@{\xyFN@\xykparser@}%
 \fi\fi\fi\fi \next@}
\xydef@\xykscaleerror@{Ignoring zero scale factor}
\xydef@\xykhobject@{\aftergroup\xykhadjust@
 \ifx\xykSCALE@@\empty\DN@{\xykkeepscale@}%
 \else \DN@{\xyksavescale@{}}%
 \fi \next@ }
\xydef@\xykvobject@{\aftergroup\xykvadjust@
 \ifx\xykSCALE@@\empty\DN@{\xykkeepscale@}%
 \else \DN@{\xyksavescale@{}}%
 \fi \next@ }
\xydef@\xykhvobject@{\aftergroup\xykhvadjust@
 \ifx\xykSCALE@@\empty\DN@{\xykkeepscale@}%
 \else \DN@{\xyksavescale@{}}%
 \fi \next@ }
\xydef@\xykhuobject@{\aftergroup\xykhuadjust@
 \ifx\xykSCALE@@\empty\DN@{\xykkeepscale@}%
 \else \DN@{\xyksavescale@{}}%
 \fi \next@ }
\xydef@\xyksavescale@#1#2{%
 \expandafter\ifx\the\Edge@c\zeroEdge\relax \def\xyksaveEdgec{}%
 \else
 \edef\xyksaveEdgec{\noexpand\Edge@c={\expandafter\noexpand\the\Edge@c}%
 \L@c=\the\L@c \R@c=\the\R@c \D@c=\the\D@c \U@c=\the\U@c}%
 \fi
 \edef\next@##1##2{\endgroup
 \def\noexpand\xyksaveEdgec{}%
 \def\noexpand\xykSCALE@@\noexpand{##1}%
 \def\noexpand\xykjoincontrol\noexpand{\xykjoincontrol}%
 \noexpand\toks@\noexpand{##2}%
 \noexpand\xy@@{\def\noexpand\xyksaveEdgec{}%
 \def\noexpand\xykSCALE@@{##1}%
 \def\noexpand\xykjoincontrol{\xykjoincontrol}}}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\expandafter{\expandafter\xykSCALE@@\expandafter}%
 \expandafter{\the\toks@}%
 \xykrescale@ #1\the\toks@\restore\POS#2}
\xydef@\xykkeepscale@{%
 \edef\next@##1{\endgroup \noexpand\toks@={##1}%
 \def\noexpand\xykjoincontrol{\xykjoincontrol}}%
 \expandafter\next@\expandafter{\the\toks@}%
 \def\xykSCALE@@{}\def\xyksaveEdgec{}%
 \xy@@{\def\xykSCALE@@{}\def\xyksaveEdgec{}}%
 \edef\next@{\def\noexpand\xykjoincontrol{\xykjoincontrol}}%
 \expandafter\xy@@\expandafter{\next@}%
 \xyknoflexscale@ \the\toks@}
\xydef@\xykrescale@{\expandafter\xykcheckscale@\xykSCALE@@ !}%
\xydef@\xykcheckscale@#1#2!{%
 \expandafter\DN@\expandafter{\codeof{#1}}%
 \expandafter\DNii@\expandafter{\codeof{@}}%
 \ifx\next@\nextii@\relax\DN@{\xykflexiscale@#2%
 \xy@@{\divide\X@xbase2\divide\X@ybase2\divide\Y@xbase2\divide\Y@ybase2%
 \def\xykSCALE@@{}}\def\xykSCALE@@{}%
 \expandafter\toks@\expandafter{\afterFLEX@}}%
 \else\DN@{\save \xykrescale@@}\fi \next@ }
\xydef@\xykflexiscale@{%
 \expandafter\def\expandafter\afterFLEX@\expandafter{\the\toks@}%
 \xykflexiscale@@ }
\xydef@\xykrescale@@{%
 \edef\next@{\X@xbase=\xykSCALE@@\X@xbase \X@ybase=\xykSCALE@@\X@ybase
 \Y@xbase=\xykSCALE@@\Y@xbase \Y@ybase=\xykSCALE@@\Y@ybase}%
 \expandafter\xy@@\expandafter{\next@}%
 \ifdim\xykSCALE@@\p@<\z@\relax \DN@{\xyknegflexscale@}%
 \else\DN@{\xyknoflexscale@}\fi \next@ }
{\xyuncatcodes \gdef\next#1#2#3#4{\save="@",
 #1,="^<",\POS"@",#2,="^>",\POS"@",#3,="_<",\POS"@",#4,="_>",
 (0,0);"^>"-"^<"+"_>"-"_<":"^<"-"_<"+"^>"-"_>"::}}
\xylet@\xykflexiscale@@=\next
{\xyuncatcodes \gdef\next{\save ="^<",
 +(1,0)="^>",-(1,1)="_<",+(1,0)="_>"\restore }}
\xylet@\xyknoflexscale@@=\next
\xylet@\xyknoflexscale@=\next
{\xyuncatcodes \gdef\next{\save ="_>",
 +(-1,1)="^<",+(1,0)="^>",-(1,1)="_<"\restore }}
\xylet@\xyknegflexscale@@=\next
\xylet@\xyknegflexscale@=\next
{\xyuncatcodes \gdef\next{\save ="_<",
 +(1,0)="_>",+(-1,1)="^<",+(1,0)="^>"\restore }}
\xylet@\xykhscale@@=\next
{\xyuncatcodes \gdef\next{\save ="^>",
 -(1,0)="^<",+(1,-1)="_>",-(1,0)="_<"\restore }}
\xylet@\xykvscale@@=\next
\xydef@\xykhadjust@{%
 \let\xyknoflexscale@=\xykhscale@@
 \let\xyknegflexscale@=\xyknegflexscale@@ }
\xydef@\xykvadjust@{%
 \let\xyknoflexscale@=\xyknoflexscale@@
 \let\xyknegflexscale@=\xykhscale@@ }
\xydef@\xykhvadjust@{%
 \let\xyknoflexscale@=\xyknoflexscale@@
 \let\xyknegflexscale@=\xyknegflexscale@@ }
\xydef@\xykhuadjust@{%
 \let\xyknoflexscale@=\xykhscale@@
 \let\xyknegflexscale@=\xykvscale@@ }
\xydef@\xykprebreak@{%
 \ifx\xykprebreak@@\empty\addtotoks@{{}}\else
 \expandafter\addtotoks@\expandafter{\expandafter{\xykprebreak@@}}\fi}
\xydef@\xykpostbreak@{%
 \ifx\xykpostbreak@@\empty\addtotoks@{{}}\else
 \expandafter\addtotoks@\expandafter{\expandafter{\xykpostbreak@@}}\fi}
\xydef@\xykmidbreak@{%
 \ifx\xykmidbreak@@\empty\addtotoks@{{}}\else
 \expandafter\addtotoks@\expandafter{\expandafter{\xykmidbreak@@}}\fi}
\xydef@\xykparsebreak@{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xykparsebreak@}%
 \else \addLT@\ifx\next 
 \expandafter\appendtoholder@\xykbacktemp@\next@
 \addLT@\DN@{\xyFN@\xykparser@}%
 \else \addGT@\ifx\next 
 \expandafter\appendtoholder@\xykforetemp@\next@
 \addGT@\DN@{\xyFN@\xykparser@}%
 \else \ifx|\next
 \expandafter\appendtoholer@\xyknulltemp@\next@
 \DN@|{\xyFN@\xykparser@}%
 \else \ifx\next \bgroup\DN@##1{\checkgroupbreak@##1@}%
 \else \ifx (\next\DN@(##1){\xyadjustknotPLACE@i##1@@%
 \xyFN@\xykparsebreak@}%
 \else \ifx\next \knothole@\DN@##1{\expandafter\appendtoholder@@
 \expandafter{\expandafter|\xyknotPLACE\knothole}\next@
 \xyFN@\xykparser@}%
 \else 
 \expandafter\xykdefaultbreak@\xykbreak@\next@
 \DN@{\xyFN@\xykparser@}%
 \fi\fi\fi\fi\fi\fi\fi \next@ }
{\xyuncatcodes \gdef\next{^>*\dir{>}}}
\xylet@\xykforetips@=\next
{\xyuncatcodes \gdef\next{^<*\dir{<}}}
\xylet@\xykbacktips@=\next
{\xyuncatcodes \gdef\next{*!/-1pt/=0\dir{>}}}
\xylet@\xykforetemp@=\next
{\xyuncatcodes \gdef\next{*!/1pt/=0\dir{<}}}
\xylet@\xykbacktemp@=\next
{\xyuncatcodes \gdef\next{*=<\xykholesize>[o]{}}}
\xylet@\xykholetemp@=\next
\xydef@\knothole@{\hbox to\xykholesize{%
 \dimen@=\xykholesize \divide\dimen@\tw@
 \hfill \vrule height\dimen@ depth\dimen@ width\z@ }}
\xylet@\knothole=\knothole@
\xylet@\khole=\knothole@
{\xyuncatcodes \gdef\next{*=<0pt>{}}}
\xylet@\xyknulltemp@=\next
\xylet@\xykbreak@=\xyknulltemp@
\xydef@\checkgroupbreak@#1#2@{%
 \ifx|#1\DN@{\appendtoholder@@#1#2\next@ \xyFN@\xykparser@}%
 \else \ifx_#1\DN@{\appendtoholder@@_#2\next@ \xyFN@\xykparser@}%
 \else \ifx^#1\DN@{\appendtoholder@@^#2\next@ \xyFN@\xykparser@}%
 \else 
 \def\next##1\next{\expandafter\DNii@\expandafter{\xyk@@##1}}%
 \expandafter\next\xyknotPLACE\next
 \ifx*#1%
 \expandafter\DN@\expandafter{%
 \expandafter\appendtoholder@@\nextii@#1#2\next@ \xyFN@\xykparser@}%
 \else
 \expandafter\DN@\expandafter{%
 \expandafter\appendtoholder@@\nextii@{#1#2}\next@ \xyFN@\xykparser@}%
 \fi\fi\fi\fi \next@ }
{\xyuncatcodes \gdef\next{%
 \expandafter{\expandafter^\xyknotPLACE##1}}}%
 \DN@{\xydef@\xykholder@@##1}\DNii@{\expandafter\toks@}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\expandafter{\expandafter\nextii@\next}
\xydef@\appendtoholder@#1\next@{\xykholder@@{#1}%
 \DN@##1{\expandafter\DN@\expandafter{\xykholder@##1}}%
 \expandafter\next@\expandafter{\the\toks@}\appendtoholder@@@ }
\xydef@\appendtoholder@@#1\next@{%
 \DN@##1\next@{\expandafter\DN@\expandafter{\xykholder@##1}}%
 \next@#1\next@ \appendtoholder@@@}%
\xydef@\appendtoholder@@@{%
 \expandafter\expandafter\expandafter\DN@
 \expandafter\expandafter\expandafter{\next@}%
 \DNii@{\expandafter\def\xykholder@}%
 \expandafter\nextii@\expandafter{\next@}}
{\xyuncatcodes \gdef\next{%
 \expandafter{\expandafter|\xyknotPLACE##1}}}%
\DN@{\xydef@\xykholer@@##1}\DNii@{\expandafter\toks@}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\expandafter{\expandafter\nextii@\next}
\xydef@\appendtoholer@#1\next@{\xykholer@@{#1}%
 \DN@##1{\expandafter\DN@\expandafter{\xykholder@##1}}%
 \expandafter\next@\expandafter{\the\toks@}\appendtoholder@@@ }
\xydef@\xykz#1{\let\xyk@@=#1\xy@@{\let\xyk@@=#1}}
{\xyuncatcodes \global\let\next=_}
\xylet@\xyk@@=\next
\xydef@\xyadjustknotPLACE@i{%
 \ifx\xyknotPLACE\empty\DN@{\dimen@=.5\p@}%
 \else\DN@{\expandafter\xygetknotPLACE@@\xyknotPLACE}%
 \fi \next@ \relax \let\xywhichknotPLACE@@=\xysetknotPLACE@@
 \xyFN@\xyadjustknotPLACE@}
\xydef@\xyadjustknotPLACE@{\expandafter\ifx\space@\next
 \expandafter\DN@\space{\xyFN@\xyadjustknotPLACE@}%
 \else\addDASH@\ifx\next\DN@{\xyadjustknotPLACE@@}%
 \else\addPLUS@\ifx\next\DN@{\xyadjustknotPLACE@@}%
 \else\addEQ@\ifx\next\addEQ@\DN@{\dimen@=\z@ \xyadjustknotPLACE@@}%
 \else \DN@{\dimen@=\z@ \xyadjustknotPLACE@@}%
 \fi\fi\fi\fi \next@}
\xydef@\xyadjustknotPLACE@@#1@@{\advance\dimen@#1\p@
 \expandafter\xysetknotPLACE@\expandafter{\the\dimen@}}
\xydef@\xysetknotPLACE@#1{%
 \expandafter\xywhichknotPLACE@@\expandafter{\removePT@#1}}
{\xyuncatcodes\gdef\next#1{\def\xyknotPLACE{(#1)}}}%
\xylet@\xysetknotPLACE@@=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next(#1){\DN@\next@{#1}\ifx\next@\empty
 \dimen@=\z@\else\dimen@=#1\p@ \fi}}%
\xylet@\xygetknotPLACE@@=\next 
\xydef@\xyadjustJOIN@i{%
 \ifx\xykjoincontrol\empty\DN@{\dimen@=.75\p@}%
 \else\DN@{\expandafter\xygetknotPLACE@@\expandafter(\xykjoincontrol)}%
 \fi \next@ \relax \let\xywhichknotPLACE@@=\xysetjoincontrol@
 \xyFN@\xyadjustknotPLACE@}
\xydef@\xyadjustBREAK@i{%
 \ifx\xykpostbreak@@\empty\DN@{\dimen@=.5\p@}%
 \else\DN@{\expandafter\xygetpostBREAK@\xykpostbreak@@}%
 \fi \next@ \relax \let\xywhichknotPLACE@@=\xysetpostbreak@
 \xyFN@\xyadjustknotPLACE@}
\xydef@\xygetpostBREAK@|#1\knothole{\DN@{#1}%
 \ifx\next@\empty\dimen@=.5\p@\else \xygetknotPLACE@@#1\fi}
\xydef@\xysetpostbreak@#1{\def\xykpostbreak@@{|(#1)\knothole}}
\xydef@\xysetjoincontrol@#1{\edef\xykjoincontrol{#1}}
\xydef@\xykparsetips@{%
 \def\xyknotTIPS@@{}\def\xyknotPLACE{}%
 \let\xykparser@=\xykparsetips@@
 \xyFN@\xykparser@ }
\xydef@\xykparsetips@@{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xykparsetips@@}%
 \else\addLT@\ifx\next
 \ifx\xyknotTIPS@@\empty \def\xyknotTIPS@@{TF}%
 \else\DN@{FF}\ifx\next@\xyknotTIPS@@ \def\xyknotTIPS@@{TF}%
 \else\DN@{FT}\ifx\next@\xyknotTIPS@@ \def\xyknotTIPS@@{TT}%
 \fi\fi\fi
 \addLT@\DN@{\xyFN@\xykparser@}%
 \else\addGT@\ifx\next
 \ifx\xyknotTIPS@@\empty \def\xyknotTIPS@@{FT}%
 \else\DN@{FF}\ifx\next@\xyknotTIPS@@ \def\xyknotTIPS@@{FT}%
 \else\DN@{TF}\ifx\next@\xyknotTIPS@@ \def\xyknotTIPS@@{TT}%
 \fi\fi\fi
 \addGT@\DN@{\xyFN@\xykparser@}%
 \else\addEQ@\ifx\next \def\xyknotTIPS@@{TT}%
 \addEQ@\DN@{\xyFN@\xykparser@}%
 \else \ifx!\next \def\xyknotTIPS@@{FF}\DN@!{\xyFN@\xykparser@}%
 \else\DN@{\xyFN@\xykparser@}%
 \fi\fi\fi\fi\fi \next@ }
\xydef@\xykcheckTIPS@{%
 \ifx\xyknotTIPS@@\empty \edef\xyknotTIPS@@{\xyknotTIPS@}\fi
 \DN@{FF}\ifx\next@\xyknotTIPS@@\def\tmp@{}%
 \else\DN@{FT}\ifx\next@\xyknotTIPS@@
 \expandafter\def\expandafter\tmp@\expandafter{\xykforetips@}%
 \else\DN@{TF}\ifx\next@\xyknotTIPS@@
 \expandafter\def\expandafter\tmp@\expandafter{\xykbacktips@}%
 \else 
 \DN@##1\next@{\DN@{\xykforetips@##1}}%
 \expandafter\next@\xykbacktips@\next@
 \DNii@{\expandafter\def\expandafter\tmp@\expandafter}%
 \expandafter\nextii@\expandafter{\next@}%
 \fi\fi\fi \def\xyknotTIPS@@{}}
\xydef@\xyknottips@{%
 \ifx\tmp@\empty\addtotoks@{{}}\else
 \expandafter\addtotoks@\expandafter{\expandafter{\tmp@}}\fi}
\xydef@\xykparsejoin@{%
 \def\xykSCALE@@{}%
 \edef\xyknotPLACE{\xykmidPLACE@}%
 \let\xykparser@=\xykparsejoin@@
 \def\xykdefaultbreak@{\let\xykbreak@=\xykforetemp@
 \def\xyknotPLACE{(.5)}\appendtoholder@}%
 \xyFN@\xykparsescale@ }
{\xyuncatcodes \catcode`@=11
\gdef\next{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xykparsejoin@@}%
 \else\addLT@\ifx\next \let\xykbreak@=\xykbacktemp@
 \def\xykdefaultbreak@{\def\xyknotPLACE{(.5)}%
 \appendtoholder@}\addLT@\DN@{\xyprecross@}%
 \else\addGT@\ifx\next \let\xykbreak@=\xykforetemp@
 \def\xykdefaultbreak@{\def\xyknotPLACE{(.5)}%
 \appendtoholder@}\addGT@\DN@{\xypostcross@}%
 \else\ifx|\next \let\xykbreak@=\xyknulltemp@
 \def\xykdefaultbreak@{\def\xyknotPLACE{(.5)}%
 \appendtoholer@}\DN@|{\xymidcross@}%
 \else\addEQ@\ifx\next \addEQ@\DN@{\xyFN@\xykparsetips@@}%
 \else\addAT@\ifx\next \addAT@\DN@(##1){%
 \xyadjustJOIN@i##1@@\xyFN@\xykparsejoin@@}%
 \else\DN@{\afterknot@}%
 \fi\fi\fi\fi\fi\fi \next@ }}
\xylet@\xykparsejoin@@=\next
\xydef@\xykjoincontrol@@{.75}%
\xydef@\xyk@joincontrol@#1{\DN@{#1}%
 \ifx\next@\empty\edef\xykjoincontrol@@{.75}%
 \else\dimen@=#1\p@
 \edef\xykjoincontrol@@{\expandafter\removePT@\the\dimen@}\fi}
\xylet@\xykjoincontrol\empty
\xydef@\xykjoincontrol@(#1){\DN@{#1}%
 \ifx\next@\empty\edef\xykjoincontrol{\xykjoincontrol@@}%
 \else\dimen@=#1\p@
 \edef\xykjoincontrol{\expandafter\removePT@\the\dimen@}%
 \fi \xyFN@\xykparsejoin@@ }
\xydef@\xykjoincontrol@i#1{\DN@{#1}%
 \ifx\next@\empty\edef\xykjoincontrol{\xykjoincontrol@@}%
 \else\dimen@=#1\p@
 \edef\xykjoincontrol{\expandafter\removePT@\the\dimen@}\fi}
\xydef@\xykjoin@#1{%
 \expandafter\toks@\expandafter{\expandafter#1\knotSTYLE}}
\xydef@\xyksetjoin@{\xykcheckTIPS@ 
 \xykprebreak@ \xykmidbreak@ \xykpostbreak@ \xyknottips@ }
\xydef@\hcap{\begingroup\def\afterknot@{\xyhcap}%
 \def\xykprePLACE@{(.385)}\def\xykpostPLACE@{(.615)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.25}%
 \xyFN@\xykparsejoin@ }%
\xydef@\vcap{\begingroup\def\afterknot@{\xyvcap}%
 \def\xykprePLACE@{(.385)}\def\xykpostPLACE@{(.615)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.25}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xcapv{\begingroup\def\afterknot@{\xyxcapv}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xcaph{\begingroup\def\afterknot@{\xyxcaph}%
 \def\xykprePLACE@{(.2)}\def\xykpostPLACE@{(.8)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xyvcap{\xykjoin@\xykcapv \xyksetjoin@ \xykhobject@{}}
\xydef@\xyhcap{\xykjoin@\xykcaph \xyksetjoin@ \xykvobject@{}}
\xydef@\xyxcapv{\xykjoin@\xykxcapv \xyksetjoin@ \xykvobject@{+(0,-1)}}
\xydef@\xyxcaph{\xykjoin@\xykxcaph \xyksetjoin@ \xykhobject@{+(1,0)}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_>",{\xyksaveEdgec},{\xykz_\ar #1@'{"^>"**{}?(\xykjoincontrol)@+
 ,?-(.25,0)@+,"_<";"^<"**{}?+(.25,0)@+,?(\xykjoincontrol)@+}
 "_<"#3#4#5#6},\restore \POS#7}}
\xylet@\xykcapv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_<",{\xyksaveEdgec},{\xykz_\ar #1@'{"_>"**{}?(\xykjoincontrol)@+,
 ?+(0,.25)@+,"^<";"^>"**{}?-(0,.25)@+,?(\xykjoincontrol)@+}
 "^<"#3#4#5#6}
 \restore \POS#7}}
\xylet@\xykcaph=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^>";"_>"**{}?="^_","^<";"_<"**{}?;"^_",**{}?(\xykjoincontrol)="^_",
 "_<",{\xyksaveEdgec},{\xykz_\ar #1@'{"^_"@+}
 "^<"#3#4#5#6},\restore \POS#7}}
\xylet@\xykxcapv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^<";"^>"**{}?="^_","_<";"_>"**{}?;"^_",**{}?(\xykjoincontrol)="^_",
 "_>",{\xyksaveEdgec},{\xykz_\ar #1@'{"^_"@+}
 "_<"#3#4#5#6},\restore \POS#7}}
\xylet@\xykxcaph=\next
\xydef@\hloop{\begingroup\def\afterknot@{\xyhloop}%
 \def\xykprePLACE@{(.07)}\def\xykpostPLACE@{(.93)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.75}%
 \xyFN@\xykparsejoin@ }%
\xydef@\vloop{\begingroup\def\afterknot@{\xyvloop}%
 \def\xykprePLACE@{(.07)}\def\xykpostPLACE@{(.93)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.75}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xyvloop{\xykjoin@\xykloopv \xyksetjoin@ \xykhobject@{}}
\xydef@\xyhloop{\xykjoin@\xyklooph \xyksetjoin@ \xykvobject@{}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_>",{\xykz_\ar #1@'{"^>"**{}?(\xykjoincontrol)@+,?(1.25)-(.25,0)@+,
 "_<";"^<"**{}?(1.25)+(.25,0)@+,?(\xykjoincontrol)@+}"_<"#3#4#5#6}
 \restore \POS#7}}
\xylet@\xykloopv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_<",{\xykz_\ar #1@'{"_>"**{}?(\xykjoincontrol)@+,?(1.25)+(0,.25)@+,
 "^<";"^>"**{}?(1.25)+(0,-.25)@+,?(\xykjoincontrol)@+}"^<"#3#4#5#6}
 \restore \POS#7}}
\xylet@\xyklooph=\next
\xydef@\zbendh{\begingroup\def\afterknot@{\xyzbendh}%
 \def\xykprePLACE@{(.25)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{\xykjoincontrol@@}%
 \xyFN@\xykparsejoin@ }%
\xydef@\sbendv{\begingroup\def\afterknot@{\xysbendv}%
 \def\xykprePLACE@{(.25)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{\xykjoincontrol@@}%
 \xyFN@\xykparsejoin@ }%
\xydef@\sbendh{\begingroup\def\afterknot@{\xysbendh}%
 \def\xykprePLACE@{(.25)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{\xykjoincontrol@@}%
 \xyFN@\xykparsejoin@ }%
\xydef@\zbendv{\begingroup\def\afterknot@{\xyzbendv}%
 \def\xykprePLACE@{(.25)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{\xykjoincontrol@@}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xbendr{\begingroup\def\afterknot@{\xyxbendr}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xbendl{\begingroup\def\afterknot@{\xyxbendl}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xbendu{\begingroup\def\afterknot@{\xyxbendu}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xbendd{\begingroup\def\afterknot@{\xyxbendd}%
 \def\xykprePLACE@{(.15)}\def\xykpostPLACE@{(.75)}%
 \def\xykmidPLACE@{(.5)}\edef\xykjoincontrol{.5}%
 \xyFN@\xykparsejoin@ }%
\xydef@\xyzbendh{\xykjoin@\xykzbendh \xyksetjoin@ \xykhvobject@{+(1,-1)}}
\xydef@\xysbendv{\xykjoin@\xyksbendv \xyksetjoin@ \xykhvobject@{+(1,-1)}}
\xydef@\xysbendh{\xykjoin@\xyksbendh \xyksetjoin@ \xykhuobject@{+(1,1)}}
\xydef@\xyzbendv{\xykjoin@\xykzbendv \xyksetjoin@ \xykhuobject@{+(1,1)}}
\xydef@\xyxbendr{\xykjoin@\xykxbendr \xyksetjoin@ \xykhvobject@{+(1,-1)}}
\xydef@\xyxbendl{\xykjoin@\xykxbendl \xyksetjoin@ \xykhvobject@{+(0,-1)}}
\xydef@\xyxbendu{\xykjoin@\xykxbendu \xyksetjoin@ \xykhvobject@{+(1,0)}}
\xydef@\xyxbendd{\xykjoin@\xykxbendd \xyksetjoin@ \xykhvobject@{+(1,-1)}}
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^<",{\xyksaveEdgec},
 {\xykz^\ar #1@'{"^>"**{}?(\xykjoincontrol)@+,
 "_>";"_<"**{}?(\xykjoincontrol)@+}"_>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykzbendh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^<",{\xyksaveEdgec},
 {\xykz_\ar #1@'{"_<"**{}?(\xykjoincontrol)@+,
 "_>";"^>"**{}?(\xykjoincontrol)@+}"_>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xyksbendv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_<",{\xyksaveEdgec},
 {\xykz_\ar #1@'{"_>"**{}?(\xykjoincontrol)@+,
 "^>";"^<"**{}?(\xykjoincontrol)@+}"^>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xyksbendh=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_<",{\xyksaveEdgec},
 {\xykz^\ar #1@'{"^<"**{}?(\xykjoincontrol)@+,
 "^>";"_>"**{}?(\xykjoincontrol)@+}"^>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykzbendv=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^<"-(0,.5),{\xyksaveEdgec},
 {\xykz_\ar #1@'{"_<";"_>"**{}?(\xykjoincontrol)@+,}"_>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykxbendr=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^>"-(0,.5),{\xyksaveEdgec},
 {\xykz^\ar #1@'{"_>";"_<"**{}?(\xykjoincontrol)@+,}"_<"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykxbendl=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "_<"+(.5,0),{\xyksaveEdgec},
 {\xykz_\ar #1@'{"_>";"^>"**{}?(\xykjoincontrol)@+,}"^>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykxbendu=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\save,
 "^<"+(.5,0),{\xyksaveEdgec},
 {\xykz^\ar #1@'{"^>";"_>"**{}?(\xykjoincontrol)@+,}"_>"#3#4#5#6}%
 \restore \POS#7}}
\xylet@\xykxbendd=\next
{\xyuncatcodes \gdef\next{{@{-}}{@{-}}}}
\xylet@\knotSTYLE=\next 
{\xyuncatcodes \gdef\next#1{\def\knotSTYLE{{@{#1}}{@{#1}}}}}
\xylet@\knotstyle=\next 
{\xyuncatcodes \gdef\next#1#2{\def\knotSTYLE{{@{#1}}{@{#2}}}}}
\xylet@\knotstyles=\next 
{\xyuncatcodes \gdef\next#1{\def\knotSTYLE{#1}}}
\xylet@\KNOTstyle=\next 
\xydef@\knotholesize@#1{\def\xykholesize{#1}}
\xydef@\xykholesize{5pt}
\xylet@\knotholesize=\knotholesize@
\xylet@\holesize=\knotholesize@
\xydef@\knottips#1{\def\xyknotTIPS@{#1}}
\xydef@\xyknotTIPS@{FF}
\xydef@\xyknotTIPS@@{}
\xydef@\xykSCALE@@{}
\xydef@\xykprebreak@@{}%
\xydef@\xykpostbreak@@{}%
\xydef@\xykmidbreak@@{}%
\xydef@\xykprePLACE@{(.25)}%
\xydef@\xykpostPLACE@{(.75)}%
\xydef@\xykmidPLACE@{}%
\xylet@\xykPLACE@=\xykmidPLACE@
{\gdef\next#1#2#3#4{%
 \save(0,0);"#2"-"#1"+"#4"-"#3":(.5,0):
 "#3"-"#1"+"#4"-"#2"::(0,.5)::}}
\xylet@\xykflexbase@=\next
\xylet@\xykflexbase=\xykflexbase@
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8{\xykflexbase{#1}{#2}{#3}{#4}%
 "#1",{\ar @{#5}@'{"#1"+(0,.125)@++(.1875,.125)@+,
 "#4"-(.1875,.25)@++(.1875,.125)@+}"#4" #6},
 "#2",{\ar @{#5}@'{"#2"+(0,.125)@++(-.1875,.125)@+,
 "#3"+(.1875,-.25)@++(-.1875,.125)@+}"#3" #7}%
\restore \POS#8}}
\xylet@\Xtwist=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8{\xykflexbase{#1}{#2}{#3}{#4}%
 "#1",{\ar @{#5}@'{"#1"+(0,.0625)@++(.1875,.0625)@+,
 "#3"+(.1875,-.125)@++(-.1875,.0625)@+}"#3" #6},
 "#2",{\ar @{#5}@'{"#2"+(0,.0625)@++(-.1875,.0625)@+,
 "#4"-(.1875,.125)@++(.1875,.0625)@+}"#4" #7}%
\restore \POS#8}}
\xylet@\Xuntwist=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\xykflexbase{#1}{#2}{#3}{#4}%
 "#1",{\ar @{#5}@'{"#1"+(.1875,.0625)@++(.1875,.1875)@+,
 "#4"+(-#9,-.125)@+}"#4" #6},
 "#2",{\ar @{#5}@'{"#2"+(-.1875,.0625)@++(-.1875,.1875)@+,
 "#3"+(#9,-.125)@+}"#3" #7}%
\restore \POS#8}}
\xylet@\Xover=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7#8#9{\xykflexbase{#1}{#2}{#3}{#4}%
 "#1",{\ar @{#5}@'{"#1"+(.1875,.0625)@++(.1875,.1875)@+,
 "#2"+(-.1875,.0625)@+}"#2" #6},
 "#3",{\ar @{#5}@'{"#3"+(#9,-.125)@+,"#3"+(.25,-.25)@+,
 "#4"+(-#9,-.125)@+}"#4" #7}%
\restore \POS#8}}
\xylet@\Xunover=\next
{\xyuncatcodes \gdef\next#1#2#3#4#5#6#7{\xykflexbase{#1}{#2}{#3}{#4}%
 "#1",{\ar @{#5}@'{"#1"+(0,.125)@++(.125,.25)@+,
 "#4"+(-.125,.375)@++(.125,-.25)@+}"#4" #6},
\restore \POS#7}}
\xylet@\Xcap=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3#4#5#6#7#8#9{\dimen@=#1\p@
 \ifdim\dimen@=\z@ \DN@{\Xunover{#2}{#3}{#4}{#5}{#8}{#6}{#7}{"#5"}}%
 \else\ifdim\dimen@>\z@
 \DNii@{#6}\ifx\nextii@\empty
 \DN@{\Xover{#2}{#3}{#4}{#5}{#8}{|(.45)\knothole}{#7}{"#5"}}%
 \else \DN@{\Xover{#2}{#3}{#4}{#5}{#8}{#6}{#7}{"#5"}}\fi
 \else
 \DNii@{#7}\ifx\nextii@\empty
 \DN@{\Xover{#2}{#3}{#4}{#5}{#8}{#6}{|(.45)\knothole}{"#5"}}%
 \else\DN@{\Xover{#2}{#3}{#4}{#5}{#8}{#6}{#7}{"#5"}}\fi
 \fi\fi 
 \def\tmp@{{#9}}\ifx\tmp@\empty\def\tmp@{{0}}\else\dimen@=#9\p@\fi
 \expandafter\next@\tmp@ }}
\xylet@\XXover=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3#4#5#6#7#8{\dimen@=#1\p@
 \ifdim\dimen@=\z@ \DN@{\Xuntwist{#2}{#4}{#3}{#5}{#8}{#6}{#7}{"#5"}}%
 \else\ifdim\dimen@>\z@
 \DNii@{#6}\ifx\nextii@\empty
 \DN@{\Xtwist{#2}{#4}{#3}{#5}{#8}{|(.45)\knothole}{#7}{"#5"}}%
 \else \DN@{\Xtwist{#2}{#4}{#3}{#5}{#8}{#6}{#7}{"#5"}}\fi
 \else
 \DNii@{#7}\ifx\nextii@\empty
 \DN@{\Xtwist{#2}{#4}{#3}{#5}{#8}{#6}{|(.45)\knothole}{"#5"}}%
 \else\DN@{\Xtwist{#2}{#4}{#3}{#5}{#8}{#6}{#7}{"#5"}}\fi
 \fi\fi \next@ }}
\xylet@\XXtwist=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3#4{\dimen@=#1\p@
 \ifdim\dimen@=\z@ \DN@{\xykuncrossv{#4}{#2}{#3}{+(0,-1)}}%
 \else\ifdim\dimen@>\z@
 \DNii@{#2}\ifx\nextii@\empty
 \DN@{\xyktwistv{#4}{|\knothole}{#3}{+(1,0)}}%
 \else \DN@{\xyktwistv{#4}{#2}{#3}{+(1,0)}}\fi
 \else
 \DNii@{#3}\ifx\nextii@\empty
 \DN@{\xyktwistv{#4}{#2}{|\knothole}{+(0,-1)}}%
 \else\DN@{\xyktwistv{#4}{#2}{#3}{+(0,-1)}}\fi
 \fi\fi \next@ }}
\xylet@\Vcross=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3#4{\dimen@=#1\p@
 \ifdim\dimen@=\z@ \DN@{\xykuncrossh{#4}{#2}{#3}{+(0,-1)}}%
 \else\ifdim\dimen@<\z@
 \DNii@{#2}\ifx\nextii@\empty
 \DN@{\xyktwisth{#4}{|\knothole}{#3}{+(1,0)}}%
 \else \DN@{\xyktwisth{#4}{#2}{#3}{+(1,0)}}\fi
 \else
 \DNii@{#3}\ifx\nextii@\empty
 \DN@{\xyktwisth{#4}{}{|\knothole}{+(1,0)}}%
 \else\DN@{\xyktwisth{#4}{#2}{#3}{+(1,0)}}\fi
 \fi\fi \next@ }}
\xylet@\Hcross=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3{\dimen@=#1\p@ \save
 \ifdim\dimen@<\z@
 \DN@{\POS="@",p="@@",(0,0);(-1,0):(0,-1)::"@@";"@",}%
 \else\DN@{}\fi
 \next@ \xykcaph{#3}{#2}\restore }}
\xylet@\Hcap=\next
{\xyuncatcodes \catcode`@=11
 \gdef\next#1#2#3{\dimen@=#1\p@ \save
 \ifdim\dimen@<\z@
 \DN@{\POS="@",p="@@",(0,0);(0,-1)::"@@";"@",}%
 \else\DN@{}\fi
 \next@ \xykcapv{#3}{#2}\restore }}
\xylet@\Vcap=\next
\xyendinput


==> xyline.tex <==
%% xyline.tex from $Id: xyline.doc,v 3.10 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Line Width'' extension.
%% Copyright (c) 1993-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{line}{Line styles extension}{\stripRCS$Revision: 3.10 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydefcsname@{*stylechar@|@}#1{\xyFN@\xywidthchar@#1@@}%
\xydefcsname@{style [thinner]}{\xyshape@thinner@}
\xydefcsname@{style [thicker]}{\xyshape@thicker@}
\xynew@{dimen}\xylinethick@ \xylinethick@=\xydashw@
\xydef@\xyshape@thicker@{\xylinewidth@i{\multiply\xylinethick@\tw@}}
\xydef@\xyshape@thinner@{\xylinewidth@i{\divide\xylinethick@\tw@}}
\xydef@\xylinewidth@i#1{\edef\xyprevwidth@@{\the\xylinethick@}%
 #1\edef\next@{\xylinethick@=\the\xylinethick@}%
 \edef\next@ii{\noexpand\addtotoks@{%
 \noexpand\xylinewidth@@{\next@}{\xyprevwidth@@}}}%
 \next@ii }
\xydef@\xywidthchar@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xywidthchar@}%
 \else\ifx @\next \DN@ @@{\checkXyStyle@}%
 \else\ifx (\next \DN@ (##1)##2@@{%
 \xylinewidth@i{\xylinethick@=##1\xydashw@}}%
 \else\addLT@\ifx \next \addGT@{\addLT@\DN@ ##1}##2@@{%
 \xylinewidth@i{\xylinethick@=##1\relax}}%
 \else\ifx *\next \DN@ *@@{\recoverXyStyle@}%
 \else\addEQ@\ifx \next \addEQ@\DN@##1@@{\checkXyStyle@
 \addtotoks@{\xynamestyle@{##1}}}%
 \else\ifx C\next \DN@ C##1@@{\xysetlinecap@{##1}@}%
 \else\ifx J\next \DN@ J##1@@{\xysetlinejoin@{##1}@}%
 \else\ifx M\next \DN@ M(##1)@@{\xymiterlimit@{##1}@}%
 \else \DN@##1@@{\xylinewidth@i{\xylinethick@=##1\relax}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\xylinecap@{2}
\xydef@\xylinejoin@{2}
\xydef@\xylinemiter@{10}
\xydefcsname@{style [bevel]}{\xyshape@bevel@}
\xydefcsname@{style [roundjoin]}{\xyshape@rdjoin@}
\xydefcsname@{style [miter]}{\xyshape@miter@}
\xydefcsname@{style [butt]}{\xyshape@butt@}
\xydefcsname@{style [roundcap]}{\xyshape@rdcap@}
\xydefcsname@{style [projcap]}{\xyshape@projcap@}
\xydef@\xyshape@butt@{\xysetlinecap@@0}
\xydef@\xyshape@rdcap@{\xysetlinecap@@1}
\xydef@\xyshape@projcap@{\xysetlinecap@@2}
\xydef@\xyshape@miter@{\xysetlinejoin@@0}
\xydef@\xyshape@rdjoin@{\xysetlinejoin@@1}
\xydef@\xyshape@bevel@{\xysetlinejoin@@2}
\xydef@\xysetlinecap@#1@{\DN@ii{#1}\count@=#1\relax
 \expandafter\DN@\expandafter{\the\count@}%
 \ifx\next@\next@ii\else
 \xywarning@{ignoring extra tokens in line-cap: \next@}\fi
 \expandafter\xysetlinecap@@\expandafter{\next@}}
\xydef@\xysetlinejoin@#1@{\DN@ii{#1}\count@=#1\relax
 \expandafter\DN@\expandafter{\the\count@}%
 \ifx\next@\next@ii\else
 \xywarning@{ignoring extra tokens in line-join: \next@}\fi
 \expandafter\xysetlinejoin@@\expandafter{\next@}}
\xydef@\xysetmiterlimit@#1@{\DN@ii{#1}\dimen@=#1\p@\relax
 \edef\next@{\expandafter\removePT@\the\dimen@}%
 \ifx\next@\next@ii\else
 \xywarning@{ignoring extra tokens in miter-limit: \next@}\fi
 \expandafter\xysetmiterlimit@@\expandafter{\next@}}
\xydef@\xysetlinecap@@#1{\xy@linecap@i{\def\xylinecap@{#1}}}
\xydef@\xysetlinejoin@@#1{\xy@linejoin@i{\def\xylinejoin@{#1}}}
\xydef@\xysetmiterlimit@@#1{%
 \xy@linemiter@i{\def\xylinemiter@{#1}}}
\xydef@\xy@linecap@i#1{#1\addtotoks@{\xy@linecap@@{#1}}}
\xydef@\xy@linejoin@i#1{#1\addtotoks@{\xy@linejoin@{#1}}}
\xydef@\xy@linemiter@i#1{#1\addtotoks@{\xy@linemiter@{#1}}}
\xydef@\xy@linecap@#1{\checkXyStyle@ \edef\xyprevcap@@{\xylinecap@}%
 #1\let\prexylinecap@=\prexylinecap@@ \let\postxylinecap@=\postxylinecap@@
 \applyLIFOstyle@\prexylinecap@{\xylinecap@}%
 \postxylinecap@{\xyprevcap@@}}
\xydef@\prexylinecap@@{\let\prexylinecap@=\eat@ 
 \let\postxylinecap@=\postxylinecap@@ \outputxylinecap@ }
\xydef@\postxylinecap@@{\let\postxylinecap@=\eat@ 
 \let\prexylinecap@=\prexylinecap@@ \resetxylinecap@@ }
\xylet@\prexylinecap@=\prexylinecap@@
\xylet@\postxylinecap@=\postxylinecap@@
\xydef@\outputxylinecap@#1{\xycapSpecial@@{#1}}
\xydef@\resetxylinecap@#1{\resetxylinecap@i{#1}\outputxylinecap@{#1}}
\xydef@\resetxylinecap@i#1{\def\xylinecap@{#1}}
\xylet@\resetxylinecap@@=\resetxylinecap@
\xylet@\xycapSpecial@@=\eat@
\xydef@\xy@linejoin@#1{\checkXyStyle@
 \edef\xyprevjoin@@{\xylinejoin@}#1%
 \let\prexylinejoin@=\prexylinejoin@@
 \let\postxylinejoin@=\postxylinejoin@@
 \applyLIFOstyle@\prexylinejoin@{\xylinejoin@}%
 \postxylinecap@{\xyprevjoin@@}}
\xydef@\prexylinejoin@@{\let\prexylinejoin@=\eat@ 
 \let\postxylinejoin@=\postxylinejoin@@ \outputxylinejoin@ }
\xydef@\postxylinejoin@@{\let\postxylinejoin@=\eat@ 
 \let\prexylinejoin@=\prexylinejoin@@ \resetxylinejoin@@ }
\xylet@\prexylinejoin@=\prexylinejoin@@
\xylet@\postxylinejoin@=\postxylinejoin@@
\xydef@\outputxylinejoin@#1{\xyjoinSpecial@@{#1}}
\xydef@\resetxylinejoin@#1{\resetxylinejoin@i{#1}\outputxylinejoin@{#1}}
\xydef@\resetxylinejoin@i#1{\def\xylinejoin@{#1}}
\xylet@\resetxylinejoin@@=\resetxylinejoin@
\xylet@\xyjoinSpecial@@=\eat@
\xydef@\xy@linemiter@#1{\checkXyStyle@
 \edef\xyprevmiter@@{\xylinemiter@}#1%
 \let\prexylinemiter@=\prexylinemiter@@
 \let\postxylinemiter@=\postxylinemiter@@
 \applyLIFOstyle@\prexylinemiter@{\xylinemiter@}%
 \postxylinecap@{\xyprevmiter@@}}
\xydef@\prexylinemiter@@{\let\prexylinemiter@=\eat@ 
 \let\postxylinemiter@=\postxylinemiter@@ \outputxylinemiter@ }
\xydef@\postxylinemiter@@{\let\postxylinemiter@=\eat@ 
 \let\prexylinemiter@=\prexylinemiter@@ \resetxylinemiter@@ }
\xylet@\prexylinemiter@=\prexylinemiter@@
\xylet@\postxylinemiter@=\postxylinemiter@@
\xydef@\outputxylinemiter@#1{\xymiterSpecial@@{#1}}
\xydef@\resetxylinemiter@#1{\resetxylinemiter@i{#1}\outputxylinemiter@{#1}}
\xydef@\resetxylinemiter@i#1{\def\xylinemiter@{#1}}
\xylet@\resetxylinemiter@@=\resetxylinemiter@
\xylet@\xymiterSpecial@@=\eat@
\xydef@\xypolyline#1{\xypolyline@{#1}}
\xydef@\xypolyline@#1{\hbox\bgroup
 \enter@{\pfromthep@ \basefromthebase@ \cfromthec@}%
 \def\xyps@list{}\edef\smapp@@{\s@bot}%
 \smapxy@i{\enter@{\pfromthep@ \basefromthebase@ }%
 \edef\xyps@list{\expandafter\removePT@\the\X@c\space
 \expandafter\removePT@\the\Y@c\space \xyps@list}\leave@}%
 \leave@ \xy@polystyle@@{#1}\xydopoly@style\egroup
 \def\Drop@@{\styledboxz@}\def\Connect@@{\styledboxz@}}%
\xylet@\xypolyline@Special=\eat@
\xylet@\xypolyfill@Special=\eat@
\xylet@\xypolyeofill@Special=\eat@
\xylet@\xypolydot@Special=\eat@
\xylet@\xypolydash@Special=\eat@
\xydef@\UnloadpolySpecials@{%
 \let\xypolyline@Special=\eat@
 \let\xypolyfill@Special=\eat@
 \let\xypolyeofill@Special=\eat@
 \let\xypolydot@Special=\eat@
 \let\xypolydash@Special=\eat@
}
\xydef@\xy@polystyle@#1{%
 \let\poly@style@@=\xypolyline@Special
 \DNii@{#1}\ifx\nextii@\empty 
 \else\DN@{*}\ifx\next@\nextii@ \let\poly@style@@=\xypolyfill@Special
 \else\DN@{?}\ifx\next@\nextii@ \let\poly@style@@=\xypolyeofill@Special
 \else\expandafter\DN@\expandafter{\addDOT@{}}\ifx\next@\nextii@
 \let\poly@style@@=\xypolydot@Special
 \else\expandafter\DN@\expandafter{\addDASH@{}}\ifx\next@\nextii@
 \let\poly@style@@=\xypolydash@Special
 \else\DN@{{*}}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{*}}%
 \else \def\poly@style@@{\xypolystraight@{#1}}%
 \fi\fi\fi\fi\fi\fi }
\xydef@\xydopoly@style{\expandafter\poly@style@@\expandafter{\xyps@list}}
\xydef@\xynopolystyle@#1#2{\xyundefinedLine@{polyline}{{#1}}@@}
\xydef@\xypolynospec@#1{\DNii@{#1}%
 \ifx\nextii@\empty\def\poly@style@@{\xypolystraight@{-}}%
 \else\DN@{.}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{.}}%
 \else\DN@{-}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{--}}%
 \else\DN@{*}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{.}}%
 \else\DN@{?}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{.}}%
 \else\DN@{{*}}\ifx\next@\nextii@ \def\poly@style@@{\xypolystraight@{*}}%
 \else \def\poly@style@@{\xypolystraight@{#1}}%
 \fi\fi\fi\fi\fi\fi }
\xydef@\xypolystraight@#1#2{%
 \enter@{\pfromthep@ \basefromthebase@ \cfromthec@}%
 \edef\smapp@@{\s@bot}\csname S@0\endcsname\czeroEdge@\pfromc@\def\smapp@@{0}%
 \smapxy@i{\czeroEdge@\enter@{\pfromthec@}{\connect@\dir{#1}}\leave@}\leave@ }
\xylet@\xy@polystyle@@=\xypolynospec@
\xydef@\UninstallPolylines@{%
 \UnloadpolySpecials@
 \let\xy@polystyle@@=\xypolynospec@ }
\UninstallPolylines@
\xydef@\xyundefinedLine@#1#2@@{%
 \xywarning@{The #1 #2 effect is not implemented with the current driver.}}%
\xydef@\xynolinewidth@#1#2{%
 \xyundefinedLine@{linewidth}{\the\xylinethick@}@@}%
\xydef@\xynolinecap@#1{\xyundefinedLine@{linecap}{\xylinecap@}@@}%
\xydef@\xynolinejoin@#1{\xyundefinedLine@{linejoin}{\xylinejoin@}@@}%
\xydef@\xynolinemiter@#1{\xyundefinedLine@{miterlimit}{\xylinemiter@}@@}%
\xylet@\xylinewidth@@=\xynolinewidth@
\xylet@\xy@linecap@@=\xynolinecap@
\xylet@\xy@linejoin@@=\xynolinejoin@
\xylet@\xy@linemiter@@=\xynolinemiter@
\xydef@\UnloadLine@#1{%
 \ifx#1\relax\else\xyunload@{line width extension}\fi
 \let\resetxyline@@=\resetxyline@
 \let\resetxylinecap@@=\resetxylinecap@
 \let\resetxylinejoin@@=\resetxylinejoin@
 \let\resetxylinemiter@@=\resetxylinemiter@
 \let\transxyline@@=\DN@
 \let\xylineSpecial@@=\eat@
 \let\xycapSpecial@@=\eat@
 \let\xyjoinSpecial@@=\eat@
 \let\xymiterSpecial@@=\eat@
 \let\xylinewidth@@=\xynolinewidth@
 \let\xy@linecap@@=\xynolinecap@
 \let\xy@linejoin@@=\xynolinejoin@
 \let\xy@linemiter@@=\xynolinemiter@
 \UninstallPolylines@ }
\xyaddunsupport{line}{\UnloadLine@\relax}
\xydef@\xylinewidth@#1#2{\checkXyStyle@
 #1\let\prexyline@=\prexyline@@ \let\postxyline@=\postxyline@@
 \applyLIFOstyle@\prexyline@{\the\xylinethick@}\postxyline@{#2}}
\xydef@\prexyline@@{\let\prexyline@=\eat@ 
 \let\postxyline@=\postxyline@@ \outputxyline@ }
\xydef@\postxyline@@{\let\postxyline@=\eat@ 
 \let\prexyline@=\prexyline@@ \resetxyline@@ }
\xylet@\prexyline@=\prexyline@@
\xylet@\postxyline@=\postxyline@@
\xydef@\resetxyline@#1{\resetxyline@i{#1}\outputxyline@{#1}}
\xydef@\resetxyline@i#1{\xylinethick@=#1\relax}
\xydef@\outputxyline@#1{\transxyline@@{#1}%
 \expandafter\xylineSpecial@@\expandafter{\next@}}
\xylet@\resetxyline@@=\resetxyline@
\xydef@\transxyline@#1{\edef\next@{\removePT@#1}}
\xylet@\transxyline@@=\DN@
\xylet@\xylineSpecial@@=\eat@
\xyendinput


==> xymatrix.tex <==
%% xymatrix.tex from $Id: xymatrix.doc,v 3.14 2011/03/31 06:10:57 krisrose Exp $
%%
%% Xy-pic ``Matrix'' feature.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{matrix}{Matrix feature}{\stripRCS$Revision: 3.14 $}%
 {Kristoffer H.~Rose}{krisrose@tug.org}%
 {IBM T.~ J.\ Watson Research Center, P.O.~Box 704, Yorktown Heights, NY 10598 (USA)}
\xynew@{count}\Row
\xynew@{count}\Col
\xydef@\maxrow@{0}
\xydef@\maxcol@{0}
\xydef@\maxcolrow@{0}
\xynew@{toks}\queue@
\xynew@{toks}\queue@@
\xynew@{count}\qcount@
\xynew@{count}\qcount@@
\xydef@\clearq@{%
 \global\queue@={}\global\qcount@=\@ne
 \global\queue@@={}\global\qcount@@=\z@}
\xydef@\addq@#1{\global\advance\matrixsize@\@ne
 \ifnum\qcount@@<\qcount@ \let\addq@@=\addq@i
 \else \let\addq@@=\addq@ii \fi
 \expandafter\addq@@\the\queue@@\addq@@{#1}}
\xylet@\addq@@=\relax
\xydef@\addq@i#1\addq@@#2{%
 \global\advance\qcount@@\@ne \global\queue@@={#1#2}}
\xydef@\addq@ii#1\addq@@#2{%
 \global\advance\qcount@\@ne \global\qcount@@=\z@ 
 \global\queue@=\expandafter{\the\queue@#1#2}\global\queue@@={}}
\xydef@\finishq@{\expandafter\addq@ii\the\queue@@\addq@@{}}
\xynew@{count}\matrixsize@
\xynew@{if}\ifnoisymatrices@ \noisymatrices@true
\xydef@\SilentMatrices{\noisymatrices@false}
\xydef@\NoisyMatrices{\noisymatrices@true}
\xydef@\xymatrixnocompile{\global\matrixsize@=\z@
 \ifnoisymatrices@\message{<xymatrix}\fi
 \if\inxy@
 \DN@{\nter@{}\xy@\xymatrix{\enter@{%
 \def\noexpand\xy@minX@@{\xy@minX@@}\def\noexpand\xy@maxX@@{\xy@maxX@@}%
 \def\noexpand\xy@minY@@{\xy@minY@@}\def\noexpand\xy@maxY@@{\xy@maxY@@}%
 \edef\noexpand\xymatrixprefix@@{\codeof\xymatrixprefix@@}}}}%
 \else \DN@{\xy \nter@\endxy \xy@\xymatrix{\nter@{}}}\fi \next@
 \xy@@{\save@ \edef\matrixorigin@{\X@c=\the\X@c \Y@c=\the\Y@c}%
 \edef\xy@minX@@{\the\X@c}\edef\xy@maxX@@{\the\X@c}%
 \edef\xy@minY@@{\the\Y@c}\edef\xy@maxY@@{\the\Y@c}}%
 \xdef\maxrow@{0}\xdef\maxcol@{0}\xdef\maxcolrow@{0}%
 \mkHWdefaults@ \xymatrix@prefix""}
\xylet@\xymatrix=\xymatrixnocompile
\xydef@\xymatrixprefix@@{}
\xydef@\xymatrix@prefix"#1"{\DN@{#1}\edef\xymatrixprefix@@{\codeof\next@}%
 \DNii@##1{\xy@{"#1"}{\edef\xymatrixprefix@@{##1}}}%
 \expandafter\nextii@\expandafter{\xymatrixprefix@@}%
 \xyFN@\xymatrix@setup}
\xydef@\xymatrix@setup{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@setup}%
 \else\ifx \bgroup\next \let\next@=\xymatrix@ii
 \else\addAT@\ifx\next \addAT@\DN@{\xy@{@}{}\xyFN@\xymatrix@at}%
 \else\ifx "\next \let\next@=\xymatrix@prefix
 \else \DN@{\xyerror@{\string\xymatrix<setup>{<rows>} expected}{}}%
 \fi\fi\fi\fi \next@}
\xydef@\xymatrix@ii#1{%
 \xymatrix@pretypeset{#1}%
 \ifnum\maxcol@=\z@ \mkWcol@ \mkWmax@ \mkHrow@ \mkHmax@
 \xdef\maxcol@{\the\Col}\xdef\maxcolrow@{\the\Row}\fi
 \ifnoisymatrices@\message{\maxcol@ x\maxrow@}\fi
 \xymatrix@measureit@@ \the\queue@ \global\queue@={}%
 \xymatrix@typeset{#1}\restore\xymatrix@insert
 \xy@@\leave@ \leave@
 \ifnoisymatrices@\message{\the\matrixsize@>}\fi \ignorespaces}
\xydef@\xymatrixcompile#1#{\xymatrixcompile@{#1}}
\xydef@\xymatrixcompile@#1#2{\xycompile{\xymatrixnocompile#1{#2}}}
\xydef@\CompileMatrices{\let\xymatrix=\xymatrixcompile}
\xydef@\NoCompileMatrices{\let\xymatrix=\xymatrixnocompile}
\xydef@\xy@cossign@@{+}
\xydef@\xy@sinsign@@{+}
\xydef@\xy@cosabs@@{1}
\xydef@\xy@sinabs@@{0}
\xydef@\xy@tanabs@@{0}
\xydef@\xy@cotabs@@{100}
\xydef@\xymatrix@rotation{%
 \xy@@{%
 \edef\xy@cossign@@{\ifdim\cosDirection\p@<\z@-\else+\fi}%
 \edef\xy@sinsign@@{\ifdim\sinDirection\p@<\z@-\else+\fi}%
 \edef\xy@cosabs@@{%
 \if\xy@cossign@@\cosDirection\else\xy@cossign@@\cosDirection\fi}%
 \edef\xy@sinabs@@{%
 \if\xy@sinsign@@\sinDirection\else\xy@sinsign@@\sinDirection\fi}%
 \dimen@=\xy@cosabs@@\p@ \dimen@ii=\xy@sinabs@@\p@
 \ifdim\dimen@ii<.01\p@ \def\xy@cotabs@@{100}%
 \else \quotient@\xy@cotabs@@\dimen@\dimen@ii \fi
 \dimen@=\xy@cosabs@@\p@ \dimen@ii=\xy@sinabs@@\p@
 \ifdim\dimen@<.01\p@ \def\xy@tanabs@@{100}%
 \else \quotient@\xy@tanabs@@\dimen@ii\dimen@ \fi}}
\xylet@\xymatrixsavedCOORD@=\relax
\xydef@\xymatrix@pretypeset#1{%
 \global\Row=\z@ \xdef\maxcol@{0}\clearq@
 \setbox8=\vtop{%
 \ifx\xymatrixsavedCOORD@\relax \let\xymatrixsavedCOORD@=\COORD@ \fi
 \let\COORD@=\xymatrixCOORD@
 \everycr{}\let\\=\cr \tabskip=\z@ \offinterlineskip
 \halign{\prentry@ ##!@&&\xyFN@\prentry@@##!@\cr#1\crcr}%
 \prentry@@@}%
 \xdef\maxrow@{\the\Row}%
 \finishq@}
\xydef@\prentry@{\relax
 \ifnum\Row>\z@
 \ifnum\maxcol@<\Col\xdef\maxcol@{\the\Col}\xdef\maxcolrow@{\the\Row}\fi
 \expandafter\xdef\csname maxcol@\the\Row\endcsname{\the\Col}\fi
 \global\advance\Row\@ne \global\Col=\z@ \xyFN@\prentry@@}
\xylet@\lastprentry@@=\relax
\xydef@\xyeatall@{\let\xy@=\xyeat@ \change@oxy@\xyeat@ \let\xy@@ix@=\eat@}
\xydef@\prentry@@{\global\advance\Col\@ne
 \let\next@=\prentry@@norm
 \ifoldxymatrix@\else \ifx *\next \DN@*{\xyFN@\prentry@@star}\fi \fi
 \next@}
\xydef@\prentry@@star{\ifx *\next \DN@*{\xyFN@\prentry@@star@ii}%
 \else \DN@##1##{\prentry@@star@i{##1}}\fi \next@}
\xydef@\prentry@@star@i#1#2#3!@{\gdef\lastprentry@@{*#1{#2}#3}%
 \setbox\lastobjectbox@=\object#1{#2}%
 \prentry@@x}
\xydef@\prentry@@star@ii{%
 \ifx [\next
 \DN@[##1]{\DN@####1{\def\entrymodifiers@{[##1]####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\prentry@@norm}%
 \else
 \DN@##1{\DN@####1{\def\entrymodifiers@{##1####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\prentry@@norm}%
 \fi \next@}
\xydef@\prentry@@norm#1!@{\gdef\lastprentry@@{#1}%
 \DN@{\setbox\lastobjectbox@=\object}%
 \expandafter\next@\entrymodifiers@{\xyeatall@ \everyentry@ #1}%
 \prentry@@x}
\xydef@\prentry@@x{%
 \edef\next@{{\noexpand\pre@emit{\the\Row}{\Upness@}{\the\Col}{\Leftness@}%
 {\the\L@c}{\the\R@c}{\the\D@c}{\the\U@c}{\expandafter\noexpand\the\Edge@c}}}%
 \expandafter\addq@\next@ \box\lastobjectbox@}
\xynew@{if}\ifoldxymatrix@ \oldxymatrix@false
\xydef@\prentry@@@{\relax \let\next@=\prentry@@@i
 \ifoldxymatrix@ \ifnum\Col=\@ne \ifx\lastprentry@@\empty
 \global\advance\Row\m@ne \let\next@=\relax \fi\fi\fi
 \global\let\lastprentry@@=\relax \next@}
\xydef@\prentry@@@i{%
 \ifnum\maxcol@<\Col \xdef\maxcol@{\the\Col}\xdef\maxcolrow@{\the\Row}\fi
 \expandafter\xdef\csname maxcol@\the\Row\endcsname{\the\Col}}
\xydef@\xy@minX@@{\z@}
\xydef@\xy@maxX@@{\z@}
\xydef@\xy@minY@@{\z@}
\xydef@\xy@maxY@@{\z@}
\xydef@\pre@emit#1#2#3#4#5#6#7#8#9{%
 \global\Row=#1\global\Col=#3\relax
 \ifnum#3=\@ne
 \ifnum#1=\@ne \xy@@{\matrixorigin@}%
 \else \count@@=#1\advance\count@@\m@ne
 \edef\next@{\noexpand\xy@@{\noexpand\cfromid@
 {\xymatrixprefix@@\the\count@@,1}}}\next@
 \pre@emit@ \W@maxout\Hrow@c@@\W@maxin\Hrow@in\xy@tanabs@@
 \X@c\xy@sinsign@@\xy@sinabs@@\xymatrixrowsep@
 \pre@emit@ \Hrow@c@@\W@maxout\Hrow@in\W@maxin\xy@cotabs@@
 \Y@c{-\xy@cossign@@}\xy@cosabs@@\xymatrixrowsep@
 \fi
 \else \count@@=#3\advance\count@@\m@ne
 \pre@emit@ \Wcol@c@@\H@maxout\Wcol@in\H@maxin\xy@cotabs@@
 \X@c\xy@cossign@@\xy@cosabs@@\xymatrixcolsep@
 \pre@emit@ \H@maxout\Wcol@c@@\H@maxin\Wcol@in\xy@tanabs@@
 \Y@c\xy@sinsign@@\xy@sinabs@@\xymatrixcolsep@
 \fi
 \DN@##1{\xy@@{\L@c=#5\R@c=#6\D@c=#7\U@c=#8\Edge@c={#9}\idfromc@{##1#1,#3}}}%
 \expandafter\next@\expandafter{\xymatrixprefix@@}%
 \xy@@{%
 \dimen@=\X@c \advance\dimen@-\L@c
 \ifdim\dimen@<\xy@minX@@ \edef\xy@minX@@{\the\dimen@}\fi
 \dimen@=\X@c \advance\dimen@+\R@c
 \ifdim\dimen@>\xy@maxX@@ \edef\xy@maxX@@{\the\dimen@}\fi
 \dimen@=\Y@c \advance\dimen@-\D@c
 \ifdim\dimen@<\xy@minY@@ \edef\xy@minY@@{\the\dimen@}\fi
 \dimen@=\Y@c \advance\dimen@+\U@c
 \ifdim\dimen@>\xy@maxY@@ \edef\xy@maxY@@{\the\dimen@}\fi}}
\xydef@\pre@emit@#1#2#3#4{#1\A@ #2\B@ #3\R@ #4\dimen@
 \edef\next@{{\the\A@}{\the\B@}{\the\R@}{\the\dimen@}}%
 \expandafter\pre@emit@i\next@}
\xydef@\pre@emit@i#1#2#3#4#5{\xy@@{%
 \dimen@=#2\R@=#5\dimen@ \dimen@=#1\relax \ifdim\R@>\dimen@ \R@=\dimen@ \fi
 \dimen@=#4\B@=#5\dimen@ \dimen@=#3\relax \ifdim\B@>\dimen@ \B@=\dimen@ \fi
 \advance\R@\B@}%
 \pre@emit@ii}
\xydef@\pre@emit@ii#1#2#3#4{\xy@@{%
 \dimen@=#4\dimen@=#3\dimen@ \advance\R@\dimen@ \advance#1#2\R@}}
\xydef@\Wcol@in#1{#1=\csname Wcol@\the\Col\endcsname #1=.5#1}
\xydef@\Wcol@out#1{#1=\csname Wcol@\the\Col\endcsname #1=.5#1}
\xydef@\Wcol@c@@#1{#1=\csname Wcol@\the\count@@\endcsname #1=.5#1}
\xydef@\W@maxin#1{#1=\W@max #1=.5#1}
\xydef@\W@maxout#1{#1=\W@max #1=.5#1}
\xydef@\Hrow@in#1{#1=\csname Hrow@\the\Row\endcsname #1=.5#1}
\xydef@\Hrow@out#1{#1=\csname Hrow@\the\Row\endcsname #1=.5#1}
\xydef@\Hrow@c@@#1{#1=\csname Hrow@\the\count@@\endcsname #1=.5#1}
\xydef@\H@maxin#1{#1=\H@max #1=.5#1}
\xydef@\H@maxout#1{#1=\H@max #1=.5#1}
\xydef@\H@max{\z@}
\xydef@\W@max{\z@}
\xydef@\HW@max{\z@}
\xydef@\mkHrow@{}
\xydef@\mkWcol@{}
\xydef@\mkHmax@{}
\xydef@\mkWmax@{}
\xydef@\mkHWmax@{}
\xydef@\mkHWdefaults@{\let\xymatrix@measureit@@=\xymatrix@measureit
 \let\mkHrow@=\Hrow@R \let\mkWcol@=\Wcol@C
 \def\mkHmax@{\ifdim\dimen@>\H@max\relax \xdef\H@max{\the\dimen@}\fi}%
 \def\mkWmax@{\ifdim\dimen@>\W@max\relax \xdef\W@max{\the\dimen@}\fi}%
 \let\mkHWmax@=\HWmax@max}
\xydef@\Hrow@R{\expandafter\xdef\csname Hrow@\the\Row\endcsname{\the\dimen@}}
\xydef@\Wcol@C{\expandafter\xdef\csname Wcol@\the\Col\endcsname{\the\dimen@}}
\xydef@\Hrow@max{\expandafter\gdef\csname Hrow@\the\Row\endcsname{\H@max}}
\xydef@\Wcol@max{\expandafter\gdef\csname Wcol@\the\Col\endcsname{\W@max}}
\xydef@\Hrow@HWmax{\expandafter\gdef\csname Hrow@\the\Row\endcsname{\HW@max}}
\xydef@\Wcol@HWmax{\expandafter\gdef\csname Wcol@\the\Col\endcsname{\HW@max}}
\xydef@\HWmax@max{%
 \ifdim\H@max>\W@max\global\let\HW@max=\H@max\else\global\let\HW@max=\W@max\fi}
\xydef@\HWmax@set#1{\gdef\HW@max{#1}%
 \global\let\H@max=\HW@max \global\let\W@max=\HW@max}
\xydef@\xymatrix@measureit{%
 \xdef\H@max{\z@}\xdef\W@max{\z@}%
 \setbox6=\vbox{\unvbox8 \global\Row=\maxrow@
 \loop@ \dimen@ii=\lastskip\unskip \ifnum\z@<\Row
 \setbox4=\lastbox \dimen@=\dp4 \advance\dimen@\ht4 \mkHrow@ \mkHmax@
 \ifnum\Row=\maxcolrow@
 \setbox2=\hbox{\unhbox4
 \global\Col=\maxcol@
 \loop@ \dimen@ii=\lastskip\unskip \ifnum\z@<\Col
 \setbox\z@=\lastbox \dimen@=\wdz@ \mkWcol@ \mkWmax@
 \global\advance\Col\m@ne
 \repeat@}\fi
 \global\advance\Row\m@ne
 \repeat@}%
 \mkHWmax@}
\xylet@\xymatrix@measureit@@=\relax
\xydef@\xymatrix@typeset#1{%
 \clearq@
 \hbox{\vtop{\xyqall@
 \xy@@{\ifx\xymatrixsavedCOORD@\relax
 \enter@{\noexpand\let\noexpand\COORD@\noexpand\xymatrixsavedCOORD@}%
 \let\xymatrixsavedCOORD@=\COORD@ \let\COORD@=\xymatrixCOORD@
 \else \enter@{}\fi}%
 \ifx\xymatrixsavedCOORD@\relax \let\xymatrixsavedCOORD@=\COORD@ \fi
 \let\COORD@=\xymatrixCOORD@
 \kern\z@ \global\Row=\z@
 \everycr{}\let\\=\cr \tabskip=\z@ \offinterlineskip
 \halign{\entry@##!@&&\entry@@##!@\cr#1\crcr}%
 \xy@@{\leave@}}}%
 \finishq@ \expandafter\xy@@\expandafter{\the\queue@}\global\queue@={}}
\xydef@\entry@{\relax \global\advance\Row\@ne \global\Col=\z@ \entry@@}
\xydef@\entry@@{\global\advance\Col\@ne
 \DN@##1,##2,##3@{\xy@{ENTRY "##3##1,##2"}{\Row=##1 \Col=##2\relax
 \cfromid@{##3##1,##2}\pfromc@}}%
 \edef\nextii@{\the\Row,\the\Col,\xymatrixprefix@@ @}%
 \expandafter\next@\nextii@
 \xyFN@\entry@@i}
\xydef@\entry@@i{\let\next@=\entry@@norm
 \ifoldxymatrix@\else \ifx *\next \DN@*{\xyFN@\entry@@star}\fi \fi
 \next@}
\xydef@\entry@@star{\ifx *\next \DN@*{\xyFN@\entry@@star@ii}%
 \else \DN@##1##{\entry@@star@i{##1}}\fi \next@}
\xydef@\entry@@star@i#1#2#3!@{%
 \xy@@ix@{{#1}{#2}}\xy@@{\expandafter\dropentry@\the\toks9}%
 \setboxz@h{\xyqall@
 \ifx\xymatrixsavedCOORD@\relax \let\xymatrixsavedCOORD@=\COORD@ \fi
 \let\COORD@=\xymatrixCOORD@ \everyentry@ #3}%
 \setbox\z@=\copy\voidb@x}
\xydef@\entry@@star@ii{%
 \ifx [\next
 \DN@[##1]{\DN@####1{\def\entrymodifiers@{[##1]####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\entry@@norm}%
 \else
 \DN@##1{\DN@####1{\def\entrymodifiers@{##1####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\entry@@norm}%
 \fi \next@}
\xydef@\entry@@norm#1!@{%
 \DN@##1{\expandafter\xy@@ix@
 \expandafter{\expandafter{\entrymodifiers@}{##1}}}%
 \expandafter\next@\expandafter{\everyentry@#1}%
 \xy@@{\expandafter\dropentry@\the\toks9}%
 \setbox\z@=\expandafter\object\entrymodifiers@{\xyqall@
 \ifx\xymatrixsavedCOORD@\relax \let\xymatrixsavedCOORD@=\COORD@ \fi
 \let\COORD@=\xymatrixCOORD@ \everyentry@ #1}%
 \setbox\z@=\copy\voidb@x}
\xydef@\dropentry@#1#2{\drop@{#1}{\xyeatall@
 \ifx\xymatrixsavedCOORD@\relax \let\xymatrixsavedCOORD@=\COORD@ \fi
 \let\COORD@=\xymatrixCOORD@ #2}}
\xydef@\xyqall@{%
 \ifxysaving@ \let\xy@=\xyqs@ \let\xy@@ix@=\xysave@@toksix@
 \else \let\xy@=\xyq@ \let\xy@@ix@=\xyq@@toksix@ \fi
 \change@oxy@\xy@}
\xydef@\xyq@#1#2{\addq@{#2}}
\xydef@\xyq@@toksix@{\begingroup
 \xyuncatcodes \afterassignment\xyq@@toksix@i \global\toks9=}
\xydef@\xyq@@toksix@i{%
 \DN@##1{\endgroup \xy@@{\global\toks9={##1}}}%
 \expandafter\next@\expandafter{\the\toks9}}
\xydef@\xyqs@{\global\advance\matrixsize@\@ne \xysave@}
\xydef@\xymatrix@insert{%
 \xy@@{\edef\nextii@{{\xy@minX@@}{\xy@maxX@@}{\xy@minY@@}{\xy@maxY@@}}%
 \expandafter\xymatrix@insert@\nextii@}}
\xydef@\xymatrix@insert@#1#2#3#4{\matrixorigin@
 \L@c=+\X@c \advance\L@c-#1\relax
 \R@c=-\X@c \advance\R@c+#2\relax
 \D@c=+\Y@c \advance\D@c-#3\relax
 \U@c=-\Y@c \advance\U@c+#4\relax
 \Edge@c={\rectangleEdge}}
\xylet@\thematrixCOORD@@=\relax
\xylet@\thematrixprefix@@=\relax
\xydef@\xymatrixCOORD@{%
 \ifx [\next
 \DN@[##1]{\xy@{[##1]}{\def\thematrixCOORD@@{[##1]}}%
 \xyFN@\xymatrixCOORD@i##1]}%
 \else \let\next@=\xymatrixsavedCOORD@ \fi \next@}
\xydef@\xymatrixCOORD@i{\count@=\Row \count@@=\Col
 \let\thematrixprefix@@=\xymatrixprefix@@
 \ifcat A\noexpand\next
 \DN@##1{\expandafter\notrelaxorelse@\csname xymatrixCOORD@i@##1\endcsname
 \xymatrixCOORD@other}%
 \else\ifx ]\next \DN@]{\xymatrixCOORD@x}%
 \else\ifx "\next \DN@"##1"{\DN@{##1}\edef\thematrixprefix@@{\codeof\next@}%
 \xyFN@\xymatrixCOORD@ii}%
 \else \let\next@=\xymatrixCOORD@other \fi\fi\fi \next@}
\xydef@\xymatrixCOORD@i@u{\advance\count@ \m@ne\xyFN@\xymatrixCOORD@ii}
\xydef@\xymatrixCOORD@i@d{\advance\count@ \@ne \xyFN@\xymatrixCOORD@ii}
\xydef@\xymatrixCOORD@i@l{\advance\count@@\m@ne\xyFN@\xymatrixCOORD@ii}
\xydef@\xymatrixCOORD@i@r{\advance\count@@\@ne \xyFN@\xymatrixCOORD@ii}
\xydef@\xymatrixCOORD@ii{%
 \ifcat A\noexpand\next
 \DN@##1{\expandafter\notrelaxorelse@\csname xymatrixCOORD@i@##1\endcsname
 \xymatrixCOORD@error}%
 \else\ifx ]\next \DN@]{\xymatrixCOORD@x}%
 \else \let\next@=\xymatrixCOORD@xx \fi\fi \next@}
\xydef@\xymatrixCOORD@error#1{\DN@{#1}%
 \xyerror@{illegal <coord> (\codeof\next@): illegal [...] target form}{}%
 \xyFN@\xymatrixCOORD@ii}
\xydef@\xymatrixCOORD@other#1,#2]{%
 \advance\count@#1\advance\count@@#2\xymatrixCOORD@x}
\xydef@\xymatrixCOORD@x{%
 \DN@##1{\xy@@{%
 \expandafter\let\expandafter\next@\csname Q@##1\endcsname
 \ifx\next@\relax \xyerror@RC{##1}\else \next@ \fi}%
 \afterCOORD@}%
 \edef\nextii@{{\thematrixprefix@@\the\count@,\the\count@@}}%
 \expandafter\next@\nextii@}
\xydef@\xymatrixCOORD@xx{%
 \DN@##1{\xy@@{%
 \expandafter\let\expandafter\next@\csname Q@##1\endcsname
 \ifx\next@\relax \xyerror@RC{##1}\else \next@\no@@ \fi}%
 \afterPLACE\xymatrixCOORD@after}%
 \edef\nextii@{{\thematrixprefix@@\the\count@,\the\count@@}}%
 \expandafter\next@\nextii@}
\xydef@\xymatrixCOORD@after{%
 \ifx ]\next \DN@]{\afterCOORD@}%
 \else \let\next@=\xymatrixCOORD@error \fi \next@}
\xydef@\xyerror@RC#1{\xyerror@{in entry \string"\the\Row,\the\Col\string":
 No \codeof\thematrixCOORD@@\space(is \string"#1\string") from here}{}}
\xylet@\xymatrix@addop@@=\relax
\xydef@\xymatrix@at{\def\xymatrix@addop@@{\xymatrix@R\xymatrix@C}%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@at}%
 \else\ifx !\next \DN@!{\xyFN@\xymatrix@fix}%
 \else\addPLUS@\ifx \next \let\next@=\xymatrix@addop
 \else\addDASH@\ifx \next \let\next@=\xymatrix@addop
 \else\addEQ@\ifx \next \let\next@=\xymatrix@addop
 \else\ifx 1\next \DN@1{%
 \let\objectmargin@=\p@ \xyFN@\xymatrix@setup}%
 \else\ifx R\next \def\xymatrix@addop@@{\xymatrix@R}\DN@ R{\xymatrix@addop}%
 \else\ifx C\next \def\xymatrix@addop@@{\xymatrix@C}\DN@ C{\xymatrix@addop}%
 \else\ifx M\next \def\xymatrix@addop@@{\xymatrix@M}\DN@ M{\xymatrix@addop}%
 \else\ifx L\next \def\xymatrix@addop@@{\xymatrix@L}\DN@ L{\xymatrix@addop}%
 \else\ifx H\next \def\xymatrix@addop@@{\xymatrix@H}\DN@ H{\xymatrix@addop}%
 \else\ifx W\next \def\xymatrix@addop@@{\xymatrix@W}\DN@ W{\xymatrix@addop}%
 \else\ifx *\next \DN@*{\xyFN@\xymatrix@mods}%
 \else \DN@{\afterDIRECTIONorEMPTY
 {\xymatrix@rotation \xyFN@\xymatrix@setup}{%
 \xyerror@{<addop> or <direction> or one of 1RCMLHW*! expected}{}%
 \xyFN@\xymatrix@setup}}%
 \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\xymatrix@fix{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@fix}%
 \else\ifx R\next \let\mkHrow@=\Hrow@max \DN@ R{\xyFN@\xymatrix@fix@}%
 \else\ifx C\next \let\mkWcol@=\Wcol@max \DN@ C{\xyFN@\xymatrix@fix@}%
 \else \let\mkHrow@=\Hrow@HWmax \let\mkWcol@=\Wcol@HWmax
 \let\next@=\xymatrix@fix@
 \fi\fi\fi \next@}
\xydef@\xymatrix@fix@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@fix@}%
 \else\ifx 0\next \def\mkHWmax@{\HWmax@set\z@}\DN@ 0{\xyFN@\xymatrix@setup}%
 \else\addEQ@\ifx\next \addEQ@\DN@{\afterassignment\xymatrix@fix@x\dimen@ii=}%
 \else \let\mkHWmax@=\HWmax@max \let\next@=\xymatrix@setup \fi\fi\fi \next@}
\xydef@\xymatrix@fix@x{%
 \edef\mkHWmax@{\noexpand\HWmax@set{\the\dimen@ii}}\xyFN@\xymatrix@setup}
\xydef@\xymatrix@addop{\afterADDOP{\xyFN@\xymatrix@addop@}}
\xydef@\xymatrix@addop@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@addop@}%
 \else\ifx R\next \DN@ R{\xy@{R}{}\dimen@ii=\xymatrixrowsep@\xymatrix@addop@x}%
 \else\ifx C\next \DN@ C{\xy@{C}{}\dimen@ii=\xymatrixcolsep@\xymatrix@addop@x}%
 \else \DN@{\afterassignment\xymatrix@addop@x\dimen@ii=}\fi\fi\fi \next@}
\xydef@\xymatrix@addop@x{\expandafter\xy@\expandafter{\the\dimen@ii}{}%
 \xymatrix@addop@@ \xyFN@\xymatrix@setup}
\xydef@\xymatrix@R{\Addop@@\xymatrixrowsep@\dimen@ii}
\xydef@\xymatrix@C{\Addop@@\xymatrixcolsep@\dimen@ii}
\xydef@\xymatrix@M{\Addop@@\objectmargin@\dimen@ii}
\xydef@\xymatrix@L{\Addop@@\labelmargin@\dimen@ii}
\xydef@\xymatrix@H{\Addop@@\objectheight@\dimen@ii}
\xydef@\xymatrix@W{\Addop@@\objectwidth@\dimen@ii}
\xydef@\xymatrixrowsep@{2pc}
\xydef@\xymatrixcolsep@{2pc}
\xydef@\xymatrixrowsep{\afterADDOP{\Addop@@\xymatrixrowsep@}}
\xydef@\xymatrixcolsep{\afterADDOP{\Addop@@\xymatrixcolsep@}}
\xydef@\xymatrix@mods{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xymatrix@mods}%
 \else\ifx [\next
 \DN@ [##1]{\xy@{[##1]}{}\DN@####1{\def\entrymodifiers@{[##1]####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\xyFN@\xymatrix@setup}%
 \else\addPLUS@\ifx \next \DN@##1{\DNii@{##1}\xyFN@\xymatrix@change}%
 \else\addDASH@\ifx \next \DN@##1{\DNii@{##1}\xyFN@\xymatrix@change}%
 \else\addEQ@\ifx \next \DN@##1{\DNii@{##1}\xymatrix@set}%
 \else \let\next@=\xymatrix@mods@error \fi\fi\fi\fi\fi \next@}
\xydef@\xymatrix@set{%
 \begingroup \plainxy@
 \afterVECTORorEMPTY\xymatrix@mods@x\xymatrix@mods@error}
\xydef@\xymatrix@change{%
 \addEQ@\ifx\next \DN@##1{\expandafter\DNii@\expandafter{\nextii@##1}%
 \expandafter\xy@\expandafter{\nextii@}{}\begingroup \plainxy@
 \afterVECTORorEMPTY\xymatrix@mods@x\xymatrix@mods@xx}%
 \else \DN@{\expandafter\xy@\expandafter{\nextii@}{}\begingroup \plainxy@
 \afterVECTORorEMPTY\xymatrix@mods@x\xymatrix@mods@xx}\fi
 \next@}
\xydef@\xymatrix@mods@x{\expandafter\xy@\expandafter{\nextii@}{}%
 \def\next@##1##2##3{\def\nextii@####1{##1##2####1##3}}%
 \addGT@{\addLT@{\expandafter\next@\expandafter{\nextii@}}}%
 \DN@##1{\gdef\tmp@@@{{##1}}}%
 \edef\nextiii@{{\the\X@c,\the\Y@c}}%
 \expandafter\expandafter\expandafter\next@
 \expandafter\expandafter\expandafter{\expandafter\nextii@\nextiii@}%
 \endgroup
 \DN@##1{\xy@{##1}{}\DN@####1{\def\entrymodifiers@{##1####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\xyFN@\xymatrix@setup}%
 \expandafter\next@\tmp@@@}
\xydef@\xymatrix@mods@xx{\expandafter\xy@\expandafter{\nextii@}{}%
 \expandafter\gdef\expandafter\tmp@@@\expandafter{\expandafter{\nextii@}}%
 \endgroup
 \DN@##1{\xy@{##1}{}\DN@####1{\def\entrymodifiers@{##1####1}}%
 \expandafter\next@\expandafter{\entrymodifiers@}\xyFN@\xymatrix@setup}%
 \expandafter\next@\tmp@@@}
\xydef@\xymatrix@mods@error{\endgroup
 \xyerror@{Impossible @*<addop><size> <setup>.}{}\xyFN@\xymatrix@setup}
\xywarnifdefined\entrymodifiers
\expandafter\def\addEQ@\entrymodifiers#1{\def\entrymodifiers@{#1}\ignorespaces}
\xydef@\entrymodifiers@{!V\entrybox}
\xydef@\entrybox#1{\hbox{\setbox\z@=\objectbox{#1}%
%%
%% \L@p=\wdz@ \D@p=\ht\z@ \advance\D@p\dp\z@
%% \dimen@=\objectwidth@ \advance\dimen@-\L@p
%% \ifdim\dimen@>\z@ \advance\L@p\dimen@ \R@p=.5\dimen@ \else \R@p=\z@ \fi
%% \dimen@=\objectheight@ \advance\dimen@-\D@p
%% \ifdim\dimen@>\z@ \advance\D@p\dimen@ \fi
%% \dimen@=\objectmargin@ \advance\L@p2\dimen@ \advance\D@p2\dimen@ 
%% \U@p=-.5\ht\z@ \advance\U@p.5\dp\z@ \advance\R@p\objectmargin@
%% \setboxz@h{\kern\R@p \raise\U@p\boxz@}%
%% \wdz@=\L@p \ht\z@=.5\D@p \dp\z@=.5\D@p
 \L@p=\wdz@ \R@p=\z@
 \dimen@=\objectwidth@ \advance\dimen@-\L@p
 \ifdim\dimen@>\z@ \advance\L@p\dimen@ \R@p=.5\dimen@ \fi
 \dimen@=\objectmargin@ \advance\L@p2\dimen@ \advance\R@p\dimen@
 \D@p=\ht\z@ \advance\D@p\dp\z@ \U@p=-\fontdimen22\textfont\tw@
 \dimen@=\objectheight@ \advance\dimen@-\D@p
 \ifdim\dimen@>\z@ \advance\D@p\dimen@ \fi
 \dimen@=\objectmargin@ \advance\D@p2\dimen@
 \setboxz@h{\kern\R@p \raise\U@p\boxz@}%
 \wdz@=\L@p
 \advance\D@p-\ht\z@ \advance\D@p-\dp\z@ \D@p=.5\D@p
 \dimen@=\ht\z@ \advance\dimen@\D@p \ht\z@=\dimen@
 \dimen@=\dp\z@ \advance\dimen@\D@p \dp\z@=\dimen@
 \boxz@}}
\xywarnifdefined\everyentry
\expandafter\def\addEQ@\everyentry#1{\def\everyentry@{#1}\ignorespaces}
\xylet@\everyentry@=\empty
\xyendinput


==> xymovie.tex <==
%% xymovie.tex from $Id: xymovie.doc,v 3.9 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Movie Storyboard extension'' option.
%% Copyright (c) 1996-1997 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{movie}{Movie Storyboard extension}{\stripRCS$Revision: 3.9 $}%
 {Kristoffer H.~Rose}{krisrose@tug.org}%
 {IBM T.~ J.\ Watson Research Center, P.O.~Box 704, Yorktown Heights, NY 10598 (USA)}
\xynew@{dimen}\m@height
\xynew@{dimen}\m@width
\xydef@\extractparameterm@#1#2#3{%
 \DN@##1,#1=##2,##3@{\csname m@#1\endcsname=##2\relax}%
 \next@,#2,#3,@}
\xydef@\MovieSetup#1{%
 \extractparameterm@{height}{#1}{height=2in}%
 \extractparameterm@{width}{#1}{width=2in}%
}
\xydef@\theScene{0}
\xydef@\theF{0}
\xydef@\theFr{1}
\xydef@\F#1{#1(0)}
\xydef@\Fr#1{#1(1)}
\xynew@{if}\iflastframe@
\xynew@{count}\m@scene
\xydef@\scene{\advance\m@scene\@ne
 \DN@{\ifx*\next \lastframe@true \DN@*{\xyFN@\scene@}%
 \else \let\next@=\scene@ \fi \next@}%
 \xyFN@\next@}
\xydef@\scene@{%
 \ifx[\next \DN@[##1]{\scene@i}\else \let\next@=\scene@i \fi \next@}
\long\def\scene@i#1{{%
 \def\caption##1{\gdef\m@caption{Scene \the\m@scene. ##1}}%
 \edef\theScene{\the\m@scene}%
 \def\theF{0}\def\theFr{1}%
 \def\F##1{##1(0)}\def\Fr##1{##1(1)}%
 \scene@frame{#1}%
 \iflastframe@
 \def\caption##1{}%
 \gdef\m@caption{The End.}%
 \def\theF{1}\def\theFr{0}%
 \def\F##1{##1(1)}\def\Fr##1{##1(0)}%
 \scene@frame{#1}%
 \fi
 }\ignorespaces}
\def\scene@frame#1{\vbox{\null
 \dimen@=\m@width \advance\dimen@2\xydashw@
 \hrule width\dimen@
 \hbox to\dimen@{\vrule width\xydashw@ \hss
 \vbox to\m@height{\hsize=\m@width \null\vfil{#1}\vfil\null}%
 \hss \vrule width\xydashw@}%
 \hrule width\dimen@
 \setbox0=\hbox{%
 \setbox0=\hbox to\m@width{\hss\strut \m@caption\hss}%
 \dimen0=\dp0 \ht0=0pt \dp0=0pt \raise\dimen0\box0}%
 \ht0=0pt \dp0=0pt \box0\relax
 \null}}
\xyendinput


==> xynecula.tex <==
%% xynecula.tex from $Id: xynecula.doc,v 3.4 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Necula extensions'' option.
%% Copyright (c) 1998 George C. Necula <necula@cs.cmu.edu>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{necula}{Necula's extensions}{\stripRCS$Revision: 3.4 $}%
 {George C. Necula}{necula@cs.cmu.edu}%
 {School of Computer Science,
 Carnegie Mellon University,
 5000 Forbes Avenue,
 Pittsburgh, PA 15213-3891, USA}
\def\expandbeforenext@#1{%
 \DN@ e|##1|{\edef\tmp@{##1}\expandafter\xyFN@\expandafter#1\tmp@}%
}
\xylet@\xy@oldOBJECT@=\OBJECT@
\xydef@\xy@newOBJECT@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xy@newOBJECT@}%
 \else\ifx e\next
 \expandbeforenext@\OBJECT@
 \else
 \DN@{\xy@oldOBJECT@}\fi\fi
 \next@}%
\let\OBJECT@=\xy@newOBJECT@
\xylet@\xy@oldCOORD@=\COORD@
\xydef@\xy@newCOORD@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xy@newCOORD@}%
 \else\ifx e\next
 \expandbeforenext@\COORD@
 \else
 \DN@{\xy@oldCOORD@}\fi\fi
 \next@}%
\let\COORD@=\xy@newCOORD@
\xydefcsname@{*stylechar@P@}#1{\Pshape@#1@}
\xynew@{count}\c@poly@count \c@poly@count=\z@
\xydef@\Pshape@:#1@{%
 \addtotoks@{%
 \def\poly@list{@}%
 \poly@parse #1,\relax,%Sets the poly@list
 \def\poly@cache{}%
 \edef\poly@id{\the\c@poly@count}%
 \global\advance\c@poly@count\@ne
 \poly@setEdge
 \edef\poly@saveLcshape{\the\L@c}%
 \polygonEdge@Outer% Set U,R,D,L
 \poly@setEdge
 \dimen@=\poly@saveLcshape\advance\dimen@-\L@c
 \advance\R@p -\dimen@
}}
\xydef@\poly@setEdge{\expandafter\poly@setEdge@\poly@list\poly@id}
\xydef@\poly@setEdge@#1@#2{\Edge@c={\polygonEdge#1@#2@}%
 \expandafter\xdef\csname poly@cache#2%
 \endcsname{\poly@cache}}
\xydefcsname@{frm[P]{-}}{\expandafter\draw@polyframe\the\Edge@c{-}}
\xydefcsname@{frm[P]{.}}{\expandafter\draw@polyframe\the\Edge@c{.}}
\xydefcsname@{frm[P]{=}}{\expandafter\draw@polyframe\the\Edge@c{=}}
\xydef@\draw@polyframe\polygonEdge#1@#2@#3{%
 \def\poly@dir{#3}%
 \def\poly@list{#1@}%
 \def\poly@id{#2}%
 \edef\poly@cache{\csname poly@cache\poly@id\endcsname}%
 \draw@polygon}
\xydef@\poly@empty{}
\xydef@\poly@map#1#2,#3;#4@{%
 #1{#2}{#3}%
 \def\tmp@{#4}%
 \ifx \poly@empty\tmp@ \else
 \poly@map@next#1#4@%
 \fi
}
\xydef@\poly@map@stop#1@{}
\xydef@\poly@mapExpand#1#2{%
 \edef\tmp@{\noexpand\poly@map\noexpand #1#2}%
 \tmp@}
\xydef@\poly@parse #1,{%
 \ifx #1\relax
 \poly@close
 \let\next@=\relax
 \else
 \save@
 \POS #1%
 \edef\tmp@{{\the\X@c}{\the\Y@c}}%
 \expandafter\poly@append\tmp@
 \restore
 \let\next@=\poly@parse
 \fi
 \next@
}
\xydef@\poly@append#1#2{\expandafter\poly@append@\poly@list{#1,#2;}}
\xydef@\poly@append@#1@#2{\global\def\poly@list{#1#2@}}
\xydef@\poly@close{\expandafter\poly@close@\poly@list}
\xydef@\poly@close@#1,#2;#3@{\poly@append{#1}{#2}}
\xydef@\draw@polygon{%
 \save@
 \X@origin=\X@c \Y@origin=\Y@c
 \poly@setp
 \U@c=\z@\R@c=\z@\D@c=\z@\L@c=\z@\U@p=\z@\R@p=\z@\D@p=\z@\L@p=\z@
 \Edge@c={\zeroEdge}\Edge@p={\zeroEdge}%
 \let\poly@map@next=\poly@map
 \poly@mapExpand\poly@drawseg\poly@rest
 \restore
}
\xydef@\poly@setp{\expandafter\poly@setp@\poly@list}
\xydef@\poly@setp@#1,#2;#3@{%
 \X@p=#1\advance\X@p\X@origin \Y@p=#2\advance\Y@p\Y@origin%
 \global\def\poly@rest{#3@}}
\xydef@\poly@drawseg#1#2{%
 \dimen@=#1\X@c=\the\dimen@\advance\X@c \X@origin
 \dimen@=#2\Y@c=\the\dimen@\advance\Y@c \Y@origin
 \expandafter\connect@\expandafter\dir\poly@dir%
 \X@p=\X@c\Y@p=\Y@c}
\xydef@\polygonEdge#1@#2@#3{%
 \def\poly@list{#1@}%
 \def\poly@id{#2}%
 \edef\poly@cache{\csname poly@cache\poly@id\endcsname}%
 \ifcase#3\relax
 \DN@{\polygonEdge@Inters
 }%
 \or \DN@{\polygonEdge@Under}%
 \or \DN@{\polygonEdge@Dist}%
 \or \DN@{\rectangleProp@}%
 \or \DN@{\polygonEdge@Inner}%
 \or \DN@{\polygonEdge@Outer}%
 \else \DN@{}\fi
 \next@}
\newif\ifpoly@badinters
\xydef@\polygonEdge@Inters{%
 \ifx\poly@cache\poly@empty
 \poly@intersdoit
 \else
 \expandafter\poly@intersprobecache\poly@cache @%
 \fi
}
\xydef@\poly@cachehit#1#2{%
 \X@c=#1\Y@c=#2}
\xydef@\poly@cachehitdisable#1#2{\poly@intersdoit}
\xydef@\poly@intersprobecache#1,#2,#3,#4,#5@{%
 \dimen@=#1\advance\dimen@-\d@X
 \ifdim\zz@\dimen@
 \dimen@=#2\advance\dimen@-\d@Y
 \ifdim\zz@\dimen@
 \poly@cachehit{#3}{#4}
 \else
 \poly@intersdoit
 \fi
 \else
 \poly@intersdoit
 \fi
}
\xydef@\poly@intersdoit{%
 \edef\polyoldA@{\the\A@}\edef\polyoldB@{\the\B@}%
 \def\poly@intersneg{}\def\poly@interspos{}%
 \save@
 \poly@setorigin
 \def\zeroDivide@{\poly@badinterstrue}%
 \let\poly@map@next=\poly@map
 \poly@mapExpand\poly@interseg\poly@rest
 \ifx\poly@intersneg\poly@empty
 \poly@badinterstrue
 \else
 \ifx\poly@interspos\poly@empty
 \poly@badinterstrue
 \else
 \poly@badintersfalse
 \fi
 \fi
 \restore
 \A@=\polyoldA@\B@=\polyoldB@
 \ifpoly@badinters \else
 \edef\tmp@{\poly@interspos,\poly@intersneg @}%
 \expandafter\poly@intersfinish\tmp@
 \fi
}
\xydef@\poly@intersfinish#1,#2,#3@{%
 \X@c=#1\Y@c=#2\relax
 \xdef\poly@cache{\the\d@X,\the\d@Y,#1,#2,#3}%
 \poly@setEdge
}
\xydef@\poly@setorigin{\expandafter\poly@setorigin@\poly@list}
\xydef@\poly@setorigin@#1,#2;#3@{%
 \X@origin=#1\advance\X@origin\X@c \Y@origin=#2\advance\Y@origin\Y@c%
 \global\def\poly@rest{#3@}}
\xydef@\poly@interseg#1#2{%
 \dimen@=#1\advance\dimen@\X@c \edef\poly@saveXcinters{\the\dimen@}%
 \dimen@=#2\advance\dimen@\Y@c \edef\poly@saveYcinters{\the\dimen@}%
 \save@
 \poly@badintersfalse
 \R@c=\poly@saveXcinters \advance\R@c -\X@origin
 \U@c=\poly@saveYcinters \advance\U@c -\Y@origin
 \intersect@
 \A@=\X@c \B@=\Y@c
 \restore
 \ifpoly@badinters
 \else
\poly@isonseg\X@origin\Y@origin\A@\B@\poly@saveXcinters\poly@saveYcinters
 \ifpoly@badinters
 \else
 \poly@isonray\X@c\Y@c\A@\B@\X@p\Y@p
 \ifpoly@badinters
 \edef\poly@intersneg{\the\A@,\the\B@}%
 \else
 \edef\poly@interspos{\the\A@,\the\B@}%
 \fi
 \fi
 \fi
 \X@origin=\poly@saveXcinters\Y@origin=\poly@saveYcinters
}
\xydef@\polygonEdge@Dist{\xyerror@{Dist is not yet implemented for polygons}}
\newif\ifpoly@closedrange
\xydef@\poly@isinrange#1#2#3{%
 \ifpoly@badinters \else
 \dimen@=#1\dimen@i=#2\dimen@ii=#3\relax
 \advance\dimen@ii -\dimen@ \advance\dimen@i -\dimen@
 \ifdim\dimen@ii<0pt\relax
 \ifdim\dimen@i>100\almostz@
 \poly@badinterstrue
 \fi
 \dimen@i=-\dimen@i \dimen@ii=-\dimen@ii
 \else
 \ifdim\dimen@i<-100\almostz@\relax
 \poly@badinterstrue
 \fi
 \fi
 \ifpoly@closedrange
 \advance\dimen@ii 100\almostz@
 \ifdim\dimen@i>\dimen@ii
 \poly@badinterstrue
 \fi
 \fi
 \fi}
\xydef@\poly@isonseg#1#2#3#4#5#6{%
 \poly@closedrangetrue
 \poly@isinrange{#1}{#3}{#5}%
 \poly@isinrange{#2}{#4}{#6}%
}
\xydef@\poly@isonray#1#2#3#4#5#6{%
 \poly@closedrangefalse
 \poly@isinrange{#1}{#3}{#5}%
 \poly@isinrange{#2}{#4}{#6}%
}
\xydef@\polygonEdge@Under{%
 \edef\polysaveA@under{\the\A@}\edef\polysaveB@under{\the\B@}%
 \edef\poly@saveXcUnder{\the\X@c}\edef\poly@saveYcUnder{\the\Y@c}%
 \polygonEdge@Inters
 \ifpoly@badinters% p is very close to c
 \Inside@true
 \else
 \A@=\X@c\B@=\Y@c
 \X@c=\poly@saveXcUnder\Y@c=\poly@saveYcUnder
 \poly@isonseg\X@c\Y@c\X@p\Y@p\A@\B@
 \ifpoly@badinters \Inside@false \else \Inside@true\fi
 \A@=\polysaveA@under\B@=\poly@saveB@under
 \fi
}
\xydef@\polygonEdge@Inner{%
 \enter@{\basefromthebase@ \pfromthep@ \DirectionfromtheDirection@}%
 \L@c=\X@c \D@c=\Y@c
 \polygonEdge@Inters
 \ifpoly@badinters
 \czeroEdge@
 \else
 \expandafter\poly@getinterspoints\poly@cache @%
 \ifdim\X@c>\R@c
 \L@c=\R@c \R@c=\X@c
 \else
 \L@c=\X@c
 \fi
 \X@c=0.5\L@c \advance\X@c 0.5\R@c \advance\R@c -\X@c \L@c=\R@c
 \ifdim\Y@c>\U@c
 \D@c=\U@c \U@c=\Y@c
 \else
 \D@c=\Y@c
 \fi
 \Y@c=0.5\D@c \advance\Y@c 0.5\U@c \advance\U@c -\Y@c \D@c=\U@c
 \Edge@c={\rectangleEdge}%
 \fi
 \leave@
}
\xydef@\poly@getinterspoints#1,#2,#3,#4,#5,#6@{%
 \R@c=#3\U@c=#4\X@c=#5\Y@c=#6}
\xydef@\polygonEdge@Outer{%
 \enter@{\basefromthebase@ \pfromthep@ \DirectionfromtheDirection@}%
 \czeroEdge@
 \let\poly@map@next=\poly@map
 \poly@mapExpand\poly@findextent\poly@list
 \Edge@c={\rectangleEdge}%
 \leave@
}
\xydef@\poly@findextent#1#2{%
 \dimen@=#1\dimen@=\the\dimen@% it fails if I remove the second assign
 \ifdim\dimen@>\R@c \R@c=\dimen@ \fi
 \ifdim -\dimen@>\L@c \L@c=-\dimen@ \fi
 \dimen@=#2\dimen@=\the\dimen@% it fails if I remove the second assign
 \ifdim\dimen@>\U@c \U@c=\dimen@ \fi
 \ifdim -\dimen@>\D@c \D@c=-\dimen@ \fi
}
\xydef@\Fshape@#1:{\def\whichframe@@{{#1}}\let\whichoptions@@=\empty
 \DN@{{}}\ifx\whichframe@@\next@ \def\whichframe@@{{-}}\fi
 \expandafter\xyFN@\expandafter\Fshape@whichframe\the\Edge@c}
\xydef@\Fshape@whichframe{%
 \ifx\next\circleEdge
 \edef\whichframe@@{[o]\whichframe@@}%
 \DN@##1{\xyFN@\Fshape@i}%
 \else
 \ifx\next\polygonEdge
 \edef\whichframe@@{[P]\whichframe@@}%
 \DN@\polygonEdge##1@##2@{\xyFN@\Fshape@i}%
 \else
 \DN@##1{\xyFN@\Fshape@i}%
 \fi\fi
 \next@
}
\xyendinput


==> xyoztex.tex <==
%% xyoztex.tex from $Id: xyoztex.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``OzTeX'' driver interface option.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{oztex}{OzTeX driver}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\OzTeX@@#1{\dvimessage@{OzTeX}{#1}}
\newdriver{%
 \xyaddsupport{color}\oztexColor@@
 \xyaddsupport{crayon}\oztexCrayon@@
 \xyaddsupport{ps}\oztexPS@@
 \xyaddsupport{rotate}\oztexRotate@@
 \xyaddsupport{line}\oztexLine@@
 \xyaddsupport{frame}\oztexFrames@@
 \xyaddsupport{tile}\oztexTiles@@
 \xyaddsupport{cmtip}\relax
}
\xydef@\oztexColor@@{\OzTeXColours@}
\xydef@\OzTeXColours@{\OzTeXPStypes@
 \let\xylocalColor@=\xyNoColor@@ \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}%
 \installPScolor@ }\else\DN@{}\fi \next@
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\OzTeXCrayon@@{}}%
 \else\let\next@=\xystandardcolors@\fi \next@
 \let\xycolorwarning@=\relax 
 \let\oztexColor@@=\relax
 \let\UnloadColor@@=\NoOzTeXColor@
}
\xydef@\NoOzTeXColor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\oztexColor@@=\OzTeXColours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\OzTeXCrayon@@{\installCrayolaColors@}
\xydef@\oztexPS@@{\oztexPS@}
\xydef@\oztexPSunload@{\UnloadPS@
 \def\xyPSdictname{}\UsePSdict@@false
 \let\installxyps@@=\relax
 \let\UnloadPS@@=\UnloadPS@
 \xyPSshapes@true 
 \let\oztexPS@@=\oztexPS@ }
\xydef@\OzTeXSpecial@#1{\special{empty.ps {#1}xy}}
\xydef@\OzTeXMacro@#1{\special{empty.ps {#1}xy}}
\xydef@\OzTeXDict@#1{\special{empty.ps @bxy{#1}stopped pop @exy}}
\xydef@\OzTeXinclude@#1{\special{#1}}
\xydef@\OzTeXraw@#1{\special{empty.ps @bxy #1 @exy}}%
\xydef@\OzTeXPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\OzTeXSpecial@\else
 \let\PSspecial@@=\OzTeXSpecial@
 \let\PSmacro@@=\OzTeXMacro@
 \let\PSdict@@=\OzTeXDict@
 \let\PSraw@@=\OzTeXraw@
 \let\PSinclude@@=\OzTeXinclude@
 \let\xyPSobeylines@@=\obeyOzTeXlines@
 \let\PSspecialdict@@=\OzTeXDict@
 \OzTeX@@{PostScript}%
 \fi
 \OzTeXCurrpt@ }
{\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\space \obeyspaces}}
\xylet@\obeyOzTeXlines@=\next
\xydef@\OzTeXCurrpt@{\let\xyPScurrpt@@=\OzTeXCurrpt@@}%
\xydef@\OzTeXCurrpt@@{\PSraw@@{xyp}}
\xydef@\oztexPS@{\OzTeXPStypes@ 
 \let\oztexPS@@=\relax
 \let\UnloadPS@@=\oztexPSunload@
 \let\installxyps@@=\@OzTeX@PS@
 \installxyps@ }
\xydef@\@OzTeX@PS@{\UsePSdict@@true
 \let\includePSmessage@=\xyOzTeXheader 
 \ifx\undefined\xyPSdictname\def\xyPSdictname{global.ps}\fi}
\xydef@\xyOzTeXheader#1#2#3{\UsePSdict@@true}
\xydef@\oztexLine@@{\oztexLine@}
\xydef@\oztexLine@{\OzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}\installPSline@ }%
 \else\DN@{\xydriverfail@{line-styles are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\oztexFrames@@{\OzTeXFrames@}
\xydef@\OzTeXFrames@{\OzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}\installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadPSFrames@\relax}\fi
 \next@ }
\xydef@\oztexTiles@@{\OzTeXTiles@}
\xydef@\OzTeXTiles@{\OzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}\installPSpatterns@
 \xystandardpatterns@ }%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xydef@\oztexRotate@@{\OzTeXRotate@}
\xydef@\OzTeXRotate@{\OzTeXPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \OzTeXRotScale@ \installPSrotscale@ \xyPSshapes@false }%
 \else\DN@{\xydriverfail@{rotations are}\UnloadRotate@\relax}\fi
 \next@ }
\xydef@\OzTeXRotScale@{%
 \def\xyrot@start(##1){%
 {xyp xyt ##1\space xyr}{OzXy begin gsave}}%
 \def\xyscale@start(##1,##2){%
 {xyp xyt ##1\space##2\space xys}{OzXy begin gsave}}%
 \def\xyrot@end{grestore end}\def\xyscale@end{grestore end}}
\let\OzTeXRotScale@=\xyRotScale@@
\xyendinput


==> xypdf-co.tex <==
%%
%% This is file `xypdf-co.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `color')
%% 
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://math.stanford.edu/~muellner>
%% --------------------------------------------------------------------------
%% 
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%% 
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%% 
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%% 
%% --------------------------------------------------------------------------
%% 
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%% 
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%% 
%% The files with the TeX code are generated by the following command:
%% 
%%    latex xypdf.ins
%% 
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%% 
%% --------------------------------------------------------------------------
%% 
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%% 
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%% 
\xycatcodes
\expandafter\let\csname xypdf-co@loaded\endcsname\@empty
\@ifdefinable\xP@colorname\relax
\@ifdefinable\xP@colA\relax
\@ifdefinable\xP@colB\relax
\@ifdefinable\xP@colC\relax
\@ifdefinable\xP@colD\relax
\xP@hook{color}{newxycolor}
\newcommand*\xP@newxycolor[2]{\def\xP@colorname{#1}\xP@parsecolor#2 @}
\xP@color@on
\@ifdefinable\xP@parsecolor\relax
\def\xP@parsecolor#1 #2 #3@{\def\xP@colA{#1}\def\xP@colB{#2}\ifx\xP@colB\xP@gray
\xP@newcolor\xP@colorname\xP@colA\xP@gray\newxycolor
\else
\xP@parsecolor@#3 @\fi
}
\@ifdefinable\xP@parsecolor@\relax
\def\xP@parsecolor@#1 #2 #3 #4@{\def\xP@colC{#1}\def\xP@colD{#2}\ifx\xP@colD\xP@rgb
\xP@newcolor\xP@colorname{\xP@colA,\xP@colB,\xP@colC}\xP@rgb\newxycolor
\else
\def\@tempa{#3}\ifx\@tempa\xP@cmyk
\xP@newcolor\xP@colorname{\xP@colA,\xP@colB,\xP@colC,\xP@colD}{cmyk}\newxycolor
\else
\PackageError{xypdf}{Syntax error in \string\newxycolor}{}\fi
\fi
}
\newcommand*\xP@gray{gray}
\newcommand*\xP@rgb{rgb}
\newcommand*\xP@cmyk{cmyk}
\xP@hook{color}{OBJECT@shape}
\newcommand*\xP@OBJECT@shape[1]{\DN@{shape [#1]}\expandafter\let\expandafter\nextii@\csname\codeof\next@\endcsname
\ifx\nextii@\relax\DN@{style [#1]}\expandafter\let\expandafter\nextii@\csname\codeof\next@\endcsname
\ifx\nextii@\relax\DN@{\xP@checkcolor{#1}}\else\DN@{\nextii@\xyFN@\OBJECT@}\fi
\else\expandafter\addtotoks@\expandafter{\nextii@}\DN@{\xyFN@\OBJECT@}\fi \next@}
\newcommand*\xP@checkcolor[1]{\@ifundefined{\string\color@\detokenize{#1}}{\OBJECT@shapei[#1]}{\xP@append\toks@{\noexpand\xP@color{{\detokenize{#1}}}}\xyFN@\OBJECT@
}}
\newcommand*\xP@color[1]{\def\preStyle@@{\addtostyletoks@{\bgroup\xP@protectedcolor#1}}\def\postStyle@@{\addtostyletoks@{\egroup}}\modXYstyle@
}
\@ifdefinable\xP@protectedcolor\relax
\protected\def\xP@protectedcolor{\@ifundefined{color}\xP@pdfcolor\color
}
\@ifdefinable\xP@pdfcolor\relax
\def\xP@pdfcolor[#1]#2{\edef\@tempa{#1}\ifx\@tempa\xP@gray
\DN@{\xP@graycolor{#2}}\else\ifx\@tempa\xP@rgb
\DN@{\xP@rgbcolor#2@}\else\ifx\@tempa\xP@cmyk
\DN@{\xP@cmykcolor#2@}\fi\fi\fi
\aftergroup\xP@resetcolor
\next@
}\newcommand*\xP@graycolor[1]{\xP@setcolor{#1}gG}\@ifdefinable\xP@rgbcolor\relax
\def\xP@rgbcolor#1,#2,#3@{\xP@setcolor{#1 #2 #3}{rg}{RG}}
\@ifdefinable\xP@cmykcolor\relax
\def\xP@cmykcolor#1,#2,#3,#4@{\xP@setcolor{#1 #2 #3 #4}kK}
\newcommand*\xP@newcolor[4]{\expandafter\let\expandafter\next@\csname shape [#1]\endcsname
\ifx\next@\relax
\@ifundefined{\string\color@#1}\relax
{\xP@warning{xypdf}{The color `#1' is overridden by \string#4}}\edef\next@{\noexpand\newxystyle{#1}{\noexpand\xP@unnamedcolor{#2}{#3}}}\else
\DN@{}\fi
\next@\relax}
\newcommand*\xP@unnamedcolor[2]{\xP@color{[#2]{#1}}}
\newcommand\xP@definecrayolacolor[2]{\xP@newcolor{#1}{#2}{cmyk}\UseCrayolaColors}\newcommand*\xP@installCrayolaColors{\xP@definecrayolacolor{GreenYellow}{.15,0,.69,0}\xP@definecrayolacolor{Yellow}{0,0,1,0}\xP@definecrayolacolor{Goldenrod}{0,.1,.84,0}\xP@definecrayolacolor{Dandelion}{0,.29,.84,0}\xP@definecrayolacolor{Apricot}{0,.32,.52,0}\xP@definecrayolacolor{Peach}{0,.5,.7,0}\xP@definecrayolacolor{Melon}{0,.46,.5,0}\xP@definecrayolacolor{YellowOrange}{0,.42,1,0}\xP@definecrayolacolor{Orange}{0,.61,.87,0}\xP@definecrayolacolor{BurntOrange}{0,.51,1,0}\xP@definecrayolacolor{Bittersweet}{0,.75,1,.24}\xP@definecrayolacolor{RedOrange}{0,.77,.87,0}\xP@definecrayolacolor{Mahogany}{0,.85,.87,.35}\xP@definecrayolacolor{Maroon}{0,.87,.68,.32}\xP@definecrayolacolor{BrickRed}{0,.89,.94,.28}\xP@definecrayolacolor{Red}{0,1,1,0}\xP@definecrayolacolor{OrangeRed}{0,1,.5,0}\xP@definecrayolacolor{RubineRed}{0,1,.13,0}\xP@definecrayolacolor{WildStrawberry}{0,.96,.39,0}\xP@definecrayolacolor{Salmon}{0,.53,.38,0}\xP@definecrayolacolor{CarnationPink}{0,.63,0,0}\xP@definecrayolacolor{Magenta}{0,1,0,0}\xP@definecrayolacolor{VioletRed}{0,.81,0,0}\xP@definecrayolacolor{Rhodamine}{0,.82,0,0}\xP@definecrayolacolor{Mulberry}{.34,.9,0,.02}\xP@definecrayolacolor{RedViolet}{.07,.9,0,.34}\xP@definecrayolacolor{Fuchsia}{.47,.91,0,.08}\xP@definecrayolacolor{Lavender}{0,.48,0,0}\xP@definecrayolacolor{Thistle}{.12,.59,0,0}\xP@definecrayolacolor{Orchid}{.32,.64,0,0}\xP@definecrayolacolor{DarkOrchid}{.4,.8,.2,0}\xP@definecrayolacolor{Purple}{.45,.86,0,0}\xP@definecrayolacolor{Plum}{.5,1,0,0}\xP@definecrayolacolor{Violet}{.79,.88,0,0}\xP@definecrayolacolor{RoyalPurple}{.75,.9,0,0}\xP@definecrayolacolor{BlueViolet}{.86,.91,0,.04}\xP@definecrayolacolor{Periwinkle}{.57,.55,0,0}\xP@definecrayolacolor{CadetBlue}{.62,.57,.23,0}\xP@definecrayolacolor{CornflowerBlue}{.65,.13,0,0}\xP@definecrayolacolor{MidnightBlue}{.98,.13,0,.43}\xP@definecrayolacolor{NavyBlue}{.94,.54,0,0}\xP@definecrayolacolor{RoyalBlue}{1,.5,0,0}\xP@definecrayolacolor{Blue}{1,1,0,0}\xP@definecrayolacolor{Cerulean}{.94,.11,0,0}\xP@definecrayolacolor{Cyan}{1,0,0,0}\xP@definecrayolacolor{ProcessBlue}{.96,0,0,0}\xP@definecrayolacolor{SkyBlue}{.62,0,.12,0}\xP@definecrayolacolor{Turquoise}{.85,0,.2,0}\xP@definecrayolacolor{TealBlue}{.86,0,.34,.02}\xP@definecrayolacolor{Aquamarine}{.82,0,.3,0}\xP@definecrayolacolor{BlueGreen}{.85,0,.33,0}\xP@definecrayolacolor{Emerald}{1,0,.5,0}\xP@definecrayolacolor{JungleGreen}{.99,0,.52,0}\xP@definecrayolacolor{SeaGreen}{.69,0,.5,0}\xP@definecrayolacolor{Green}{1,0,1,0}\xP@definecrayolacolor{ForestGreen}{.91,0,.88,.12}\xP@definecrayolacolor{PineGreen}{.92,0,.59,.25}\xP@definecrayolacolor{LimeGreen}{.5,0,1,0}\xP@definecrayolacolor{YellowGreen}{.44,0,.74,0}\xP@definecrayolacolor{SpringGreen}{.26,0,.76,0}\xP@definecrayolacolor{OliveGreen}{.64,0,.95,.4}\xP@definecrayolacolor{RawSienna}{0,.72,1,.45}\xP@definecrayolacolor{Sepia}{0,.83,1,.7}\xP@definecrayolacolor{Brown}{0,.81,1,.6}\xP@definecrayolacolor{Tan}{.14,.42,.56,0}\xP@definecrayolacolor{Gray}{0,0,0,.5}\xP@definecrayolacolor{Black}{0,0,0,1}\xP@definecrayolacolor{White}{0,0,0,0}}
\xywithoption{crayon}{\xP@installCrayolaColors
\renewcommand*\installCrayolaColors@{}}
\xyendinput





%%
%% End of file `xypdf-co.tex'.


==> xypdf-cu.tex <==
%%
%% This is file `xypdf-cu.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `curve')
%% 
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://math.stanford.edu/~muellner>
%% --------------------------------------------------------------------------
%% 
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%% 
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%% 
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%% 
%% --------------------------------------------------------------------------
%% 
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%% 
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%% 
%% The files with the TeX code are generated by the following command:
%% 
%%    latex xypdf.ins
%% 
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%% 
%% --------------------------------------------------------------------------
%% 
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%% 
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%% 
\xycatcodes
\expandafter\let\csname xypdf-cu@loaded\endcsname\@empty
\newcommand*\xP@tempvar[2]{\@ifdefinable#1\relax
\let#1#2}
\newcommand*\xP@oldornewdimen[2]{\@ifundefined{#2}{\xP@newdimen#1}{\expandafter\xP@tempvar\expandafter#1\csname#2\endcsname}}
\xP@tempvar\xP@bigdim\quotPTK@
\xP@tempvar\xP@parA\L@p
\xP@tempvar\xP@velA\U@p
\xP@tempvar\xP@parB\R@p
\xP@tempvar\xP@velB\D@p
\xP@tempvar\xP@parC\X@origin
\xP@tempvar\xP@velC\Y@origin
\xP@tempvar\xP@parD\X@xbase
\xP@tempvar\xP@velD\Y@xbase
\xP@tempvar\xP@parE\X@ybase
\xP@tempvar\xP@velE\Y@ybase
\xP@tempvar\xP@lenA\X@min
\xP@tempvar\xP@lenB\Y@min
\xP@tempvar\xP@partlen\X@max
\xP@tempvar\xP@oldpartlen\Y@max
\xP@tempvar\xP@tolerance\almostz@
\xP@tempvar\xP@A\L@p
\xP@tempvar\xP@B\U@p
\xP@tempvar\xP@C\R@p
\xP@tempvar\xP@D\D@p
\xP@tempvar\xP@E\X@origin
\xP@tempvar\xP@F\Y@origin
\xP@tempvar\xP@G\X@xbase
\xP@tempvar\xP@H\Y@xbase
\xP@tempvar\xP@I\X@ybase
\xP@tempvar\xP@J\Y@ybase
\xP@tempvar\xP@K\X@min
\xP@tempvar\xP@L\Y@min
\xP@tempvar\xP@fa\X@max
\xP@tempvar\xP@fd\Y@max
\xP@tempvar\xP@tm\almostz@
\xP@tempvar\xP@xm\K@dXdY
\xP@tempvar\xP@ym\K@dYdX
\xP@tempvar\xP@off\splineval@
\xP@tempvar\xP@ta\splinedepth@
\xP@tempvar\xP@tb\splinetol@
\xP@tempvar\xP@tc\splinelength@
\xP@tempvar\xP@M\L@
\@tempcnta\count11\relax
\xP@oldornewdimen\xP@oldobj{normallineskiplimit}
\xP@oldornewdimen\xP@Tax{@savsk}
\xP@oldornewdimen\xP@Tay{lower@bound}
\xP@oldornewdimen\xP@Tdx{upper@bound}
\xP@oldornewdimen\xP@Tdy{leftmargin}
\xP@oldornewdimen\xP@Tmx{rightmargin}
\xP@oldornewdimen\xP@Tmy{listparindent}
\xP@oldornewdimen\xP@xa{itemindent}
\xP@oldornewdimen\xP@ya{labelwidth}
\xP@oldornewdimen\xP@xb{labelsep}
\xP@oldornewdimen\xP@yb{linewidth}
\xP@oldornewdimen\xP@xc{@totalleftmargin}
\xP@oldornewdimen\xP@yc{leftmargini}
\xP@oldornewdimen\xP@xd{leftmarginii}
\xP@oldornewdimen\xP@yd{leftmarginiii}
\count11\@tempcnta
\xP@tempvar\xP@a\X@ybase
\xP@tempvar\xP@b\Y@ybase
\xP@tempvar\xP@c\X@min
\xP@tempvar\xP@valA\Y@min
\xP@tempvar\xP@valB\X@max
\xP@tempvar\xP@devA\Y@max
\xP@tempvar\xP@devB\almostz@
\xP@tempvar\xP@ti\K@dXdY
\xP@tempvar\xP@tip\K@dYdX
\xP@tempvar\xP@sa\xP@Tax
\xP@tempvar\xP@sb\xP@Tay
\xP@tempvar\xP@sc\xP@Tdx
\xP@tempvar\xP@Ab\xP@Tdy
\xP@tempvar\xP@AAb\xP@Tmx
\xP@tempvar\xP@Aba\xP@Tmy
\xP@tempvar\xP@Abb\xP@xa
\xP@tempvar\xP@Abc\xP@ya
\xP@tempvar\xP@AAba\xP@xb
\xP@tempvar\xP@AAbb\xP@yb
\xP@tempvar\xP@AAbc\xP@xc
\xP@tempvar\xP@dta\xP@yc
\xP@tempvar\xP@dtb\xP@xd
\xP@tempvar\xP@dtc\xP@yd
\xP@tempvar\xP@temppar\X@origin
\xP@tempvar\xP@tempvel\Y@origin
\xP@tempvar\xP@posX\X@xbase
\xP@tempvar\xP@posY\Y@xbase
\xP@tempvar\xP@oldpar\X@ybase
\xP@tempvar\xP@lastpar\Y@ybase
\xP@tempvar\xP@tempvel@\X@min
\xP@tempvar\xP@parinc\Y@min
\xP@tempvar\xP@squiglen\almostz@
\xP@tempvar\xP@scaleone\K@
\xP@tempvar\xP@scaletwo\KK@
\xP@tempvar\xP@scalethree\Direction
\xP@hook{curve}{splinesolid@}
\newcommand*\xP@splinesolid@{\xP@spline\xP@setsolidpat}
\xP@hook{curve}{splinedashed@}
\newcommand*\xP@splinedashed@{\xP@spline\xP@setdashpat}
\xP@hook{curve}{splinedotted@}
\newcommand*\xP@splinedotted@{\xP@spline\xP@setdottedpat}
\newcommand*\xP@spline[1]{\readsplineparams@
\ifdim\dimen5<\dimen7
\xP@preparespline
\ifdim\@tempdimb>\z@
#1\xP@stroke{\xP@coor\X@p\Y@p m \xP@coor\L@c\U@c\xP@coor\R@c\D@c\xP@coor\X@c\Y@c c}\xP@savec
\fi
\fi
}
\newcommand*\xP@preparespline{\ifx\splineinfo@\squineinfo@
\L@c\dimexpr(\X@p+2\A@)/3\relax
\U@c\dimexpr(\Y@p+2\B@)/3\relax
\R@c\dimexpr(\X@c+2\A@)/3\relax
\D@c\dimexpr(\Y@c+2\B@)/3\relax
\fi
\xP@shavespline
\xP@bezierlength
}
\newcommand*\xP@inibigdim{\xP@bigdim5040pt}
\newcommand*\xP@shavespline{\xP@shaveprec{\dimen5*\xP@bigdim/\p@}{\dimen7*\xP@bigdim/\p@}}
\newcommand*\xP@shaveprec[2]{{\xP@inibigdim
\A@\dimexpr#1\relax
\B@\dimexpr#2\relax
\@tempswatrue
\ifdim\A@=\z@\ifdim\B@=\xP@bigdim\@tempswafalse\fi\fi
\if@tempswa
\L@p\dimexpr\L@c-\X@p\relax
\U@p\dimexpr\R@c-\L@p-\L@c\relax
\R@p\dimexpr\X@c-3\R@c+3\L@c-\X@p\relax
\D@p\dimexpr\U@c-\Y@p\relax
\X@min\dimexpr\D@c-\D@p-\U@c\relax
\Y@min\dimexpr\Y@c-3\D@c+3\U@c-\Y@p\relax
\xdef\@gtempa{\X@p\the\dimexpr\X@p+(3\L@p+(3\U@p+\R@p*\A@/\xP@bigdim)*\A@/\xP@bigdim)*\A@/\xP@bigdim\relax
\Y@p\the\dimexpr\Y@p+(3\D@p+(3\X@min+\Y@min*\A@/\xP@bigdim)*\A@/\xP@bigdim)*\A@/\xP@bigdim\relax
\L@c\the\dimexpr\X@p+(2\A@+\B@)*\L@p/\xP@bigdim+((\A@+2\B@)*\U@p/\xP@bigdim+\R@p*\A@/\xP@bigdim*\B@/\xP@bigdim)*\A@/\xP@bigdim\relax
\U@c\the\dimexpr\Y@p+(2\A@+\B@)*\D@p/\xP@bigdim+((\A@+2\B@)*\X@min/\xP@bigdim+\Y@min*\A@/\xP@bigdim*\B@/\xP@bigdim)*\A@/\xP@bigdim\relax
\R@c\the\dimexpr\X@p+(2\B@+\A@)*\L@p/\xP@bigdim+((\B@+2\A@)*\U@p/\xP@bigdim+\R@p*\B@/\xP@bigdim*\A@/\xP@bigdim)*\B@/\xP@bigdim\relax
\D@c\the\dimexpr\Y@p+(2\B@+\A@)*\D@p/\xP@bigdim+((\B@+2\A@)*\X@min/\xP@bigdim+\Y@min*\B@/\xP@bigdim*\A@/\xP@bigdim)*\B@/\xP@bigdim\relax
\X@c\the\dimexpr\X@p+(3\L@p+(3\U@p+\R@p*\B@/\xP@bigdim)*\B@/\xP@bigdim)*\B@/\xP@bigdim\relax
\Y@c\the\dimexpr\Y@p+(3\D@p+(3\X@min+\Y@min*\B@/\xP@bigdim)*\B@/\xP@bigdim)*\B@/\xP@bigdim\relax}\else
\global\let\@gtempa\relax
\fi
}\@gtempa
}
\newcommand*\xP@bezierlength{{\xP@inibigdim
\@tempdimb\z@
\xP@parA\z@
\xP@velocity\z@\xP@velA
\xP@parC.5\xP@bigdim
\xP@velocity\xP@parC\xP@velC
\xP@velocity\xP@bigdim\xP@velE
\xP@oldpartlen\dimexpr(\xP@velA+4\xP@velC+\xP@velE)/6\relax
\xP@tolerance\xP@max{1sp}{\dimexpr\xP@oldpartlen/100000\relax}\xP@arclength\xP@parC\xP@velC\xP@bigdim\xP@velE\xP@oldpartlen
\global\dimen@i\@tempdimb
}\@tempdimb\dimen@i
}
\newcommand*\xP@velocity[2]{{\@tempdima\dimexpr#1\relax
\xP@tangent
\global\dimen@i\@tempdimb
}#2\dimen@i
}
\newcommand*\xP@tangent{\d@X3\xP@precbeziertan\X@p\L@c\R@c\X@c\@tempdima
\d@Y3\xP@precbeziertan\Y@p\U@c\D@c\Y@c\@tempdima
\xP@veclen
}
\newcommand*\xP@tangentvec[1]{{\@tempdima#1\relax
\xP@tangent
\ifdim\@tempdimb=\z@
\L@p\dimexpr\X@c-\X@p+(\L@c-\R@c)*3\relax
\U@p\dimexpr\Y@c-\Y@p+(\U@c-\D@c)*3\relax
\d@X\dimexpr\L@p*\@tempdima/\xP@bigdim+(\X@p-2\L@c+\R@c)\relax
\d@Y\dimexpr\U@p*\@tempdima/\xP@bigdim+(\Y@p-2\U@c+\D@c)\relax
\xP@veclen
\ifdim\@tempdimb=\z@
\d@X\L@p
\d@Y\U@p
\xP@veclen
\ifdim\@tempdimb=\z@
\xP@warning{xypdf}{Cannot determine a tangent vector to a curve}\@tempdimb\p@
\fi
\fi
\fi
\global\dimen@i\d@X
\global\dimen3\d@Y
\global\dimen5\@tempdimb
}\d@X\dimen@i
\d@Y\dimen3\relax
\@tempdimb\dimen5\relax
}
\newcommand*\xP@arclength[5]{\xP@parE#3\xP@velE#4\xP@parC#1\xP@velC#2\xP@oldpartlen#5\xP@parB\dimexpr(\xP@parC+\xP@parA)/2\relax
\xP@velocity\xP@parB\xP@velB
\xP@parD\dimexpr(\xP@parE+\xP@parC)/2\relax
\xP@velocity\xP@parD\xP@velD
\xP@lenA
\dimexpr(\xP@velA+4\xP@velB+\xP@velC)/6*(\xP@parC-\xP@parA)/\xP@bigdim\relax
\xP@lenB
\dimexpr(\xP@velC+4\xP@velD+\xP@velE)/6*(\xP@parE-\xP@parC)/\xP@bigdim\relax
\xP@partlen\dimexpr\xP@lenA+\xP@lenB\relax
{\@tempdima\dimexpr\xP@oldpartlen-\xP@partlen\relax
\expandafter}\ifdim\ifdim\@tempdima<\z@-\fi\@tempdima>\xP@tolerance
\edef\next@{\noexpand\xP@arclength\xP@parB\xP@velB\xP@parC\xP@velC\xP@lenA
\noexpand\xP@arclength{\the\xP@parD}{\the\xP@velD}{\the\xP@parE}{\the\xP@velE}{\the\xP@lenB}}\else
\xP@parA\xP@parE
\xP@velA\xP@velE
\advance\@tempdimb\xP@partlen
\DN@{}\fi
\next@
}
\xP@hook{curve}{@crv@}
\newcommand*\xP@@crv@[2]{\DN@{#1#2}\ifx\next@\@empty \edef\next@{\crv@defaultshape}\ifx\bstartPLACE@\@empty\xdef\crvSTYLE@@{{\crv@defaultshape}}\fi
\else
\ifx\bstartPLACE@\@empty\gdef\crvSTYLE@@{#1{#2}}\fi
\fi
\ifx\next@\@empty\crv@noobject \DN@{\crv@{}{\xy@@crvaddstack@}}\else\def\tmp@{-}\ifx\next@\tmp@ \DN@{\crv@{}{\xy@@crvaddstack@}}\else\def\tmp@{=}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{=}}}\else\def\tmp@{2-}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{2.}}}\else\def\tmp@{3-}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{3.}}}\else\def\tmp@{--}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@specialtemplate@{--}}\else\def\tmp@{==}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir2{--}}}\else\def\tmp@{2--}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir2{--}}}\else\def\tmp@{3--}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir3{--}}}\else\def\tmp@{.}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@specialtemplate@{.}}\else\def\tmp@{:}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{:}}}\else\def\tmp@{2.}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{:}}}\else\def\tmp@{3.}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir3{.}}}\else\def\tmp@{~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{~}}}\else\def\tmp@{2~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir2{~}}}\else\def\tmp@{3~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir3{~}}}\else\def\tmp@{~~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir{~~}}}\else\def\tmp@{2~~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir2{~~}}}\else\def\tmp@{3~~}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@normaltemplate{\dir3{~~}}}\else\def\tmp@{..}\ifx\next@\tmp@
\DN@{\expandafter\crv@\crv@specialtemplate@{.}}\else
\DN@{\expandafter\crv@\crv@othertemplate{\dir#1{#2}}}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\next@}
\xP@hook{curve}{xysplinespecialcases@}
\newcommand*\xP@xysplinespecialcases@{\ifx\@empty\xycrvdrop@
\ifx\@empty\xycrvconn@\DN@{\splinesolid@}\else\DN@{ \dir{-}}\ifx\next@\xycrvconn@\DN@{\splinesolid@}\else\DN@{ \dir2{-}}\ifx\next@\xycrvconn@\DN@{\splinedoubled@}\else\DN@{ \dir{=}}\ifx\next@\xycrvconn@\DN@{\splineribboned@}\else\DN@{ \dir{2.}}\ifx\next@\xycrvconn@\DN@{\splinedoubled@}\else\DN@{ \dir3{-}}\ifx\next@\xycrvconn@\DN@{\splinetrebled@}\else\DN@{ \dir{3.}}\ifx\next@\xycrvconn@\DN@{\splinetrebled@}\else\DN@{ \dir{--}}\ifx\next@\xycrvconn@\DN@{\splinedashed@}\else\DN@{ \dir{.}}\ifx\next@\xycrvconn@\DN@{\splinedotted@}\else\DN@{ \dir{:}}\ifx\next@\xycrvconn@\DN@{\splinedbldotted@}\else\DN@{ \dir2{.}}\ifx\next@\xycrvconn@\DN@{\splinedbldotted@}\else\DN@{ \dir3{.}}\ifx\next@\xycrvconn@\DN@{\xP@splinetrbldotted}\else\DN@{ \dir2{--}}\ifx\next@\xycrvconn@\DN@{\xP@splinedbldashed}\else\DN@{ \dir3{--}}\ifx\next@\xycrvconn@\DN@{\xP@splinetrbldashed}\else\DN@{ \dir{~}}\ifx\next@\xycrvconn@\DN@{\xP@splinesquiggled}\else\DN@{ \dir2{~}}\ifx\next@\xycrvconn@\DN@{\xP@splinedblsquiggled}\else\DN@{ \dir3{~}}\ifx\next@\xycrvconn@\DN@{\xP@splinetrblsquiggled}\else\DN@{ \dir{~~}}\ifx\next@\xycrvconn@\DN@{\xP@splinebrokensquiggled}\else\DN@{ \dir2{~~}}\ifx\next@\xycrvconn@\DN@{\xP@splinebrokendblsquiggled}\else\DN@{ \dir3{~~}}\ifx\next@\xycrvconn@\DN@{\xP@splinebrokentrblsquiggled}\else\ifdim\splinetol@>\z@\else\splinedefaulttol@\fi
\DN@{\splineset@@}\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\else
\DN@{\splineset@@}\fi
\ifInvisible@\DN@{}\fi
\next@
}
\xP@hook{curve}{splinedoubled@}
\newcommand*\xP@splinedoubled@{\xP@checkspline\xP@splinemultsolid\xP@doublestroke}
\xP@hook{curve}{splineribboned@}
\@ifdefinable\xP@splineribboned@\relax
\let\xP@splineribboned@\xP@splinedoubled@
\xP@hook{curve}{splinetrebled@}
\newcommand*\xP@splinetrebled@{\xP@checkspline\xP@splinemultsolid\xP@trblstroke}
\newcommand*\xP@doublestroke{\xydashh@/2,-\xydashh@/2}
\newcommand*\xP@trblstroke{\xydashh@,\z@,-\xydashh@}
\newcommand*\xP@checkspline[1]{\readsplineparams@
\let\next@\@gobble
\ifdim\dimen5<\dimen7
\xP@preparespline
\ifdim\@tempdimb>\z@
\ifdim\@tempdimb<2\dimexpr\xP@preclw\relax
\let\next@\xP@splinemultsolid
\else
\let\next@#1\fi
\fi
\fi
\next@
}
\newcommand*\xP@splinemultsolid[1]{{\xP@inibigdim
\@temptokena{}\xP@setsolidpat
\@for\@tempa:={#1}\do{\xP@paintsolid\z@\xP@bigdim}\xP@stroke{\the\@temptokena}}}
\newcommand*\xP@paintsolid[2]{{\xP@savepts
\xP@a#1\relax
\xP@c#2\relax
\xP@movetotrue
\xP@paintsolid@
\xdef\@gtempa{\the\@temptokena}}\@temptokena\expandafter{\@gtempa}}
\newcommand*\xP@paintsolid@{\xP@b\xP@c
\xP@off\dimexpr\@tempa\relax
\ifdim\xP@off=\z@
\xP@shaveprec\xP@a\xP@c
\else
\loop
\xP@restorepts
\xP@offsetsegment
\xP@testoffset
\unless\ifxP@offsetok
\xP@b\dimexpr\xP@a+(\xP@b-\xP@a)*7/10\relax
\repeat
\fi
\xP@append\@temptokena{\ifxP@moveto\xP@coor\X@p\Y@p m \fi
\xP@coor\L@c\U@c\xP@coor\R@c\D@c\xP@coor\X@c\Y@c c }\xP@movetofalse
\ifdim\xP@b<\xP@c\relax
\xP@a\xP@b
\expandafter\xP@paintsolid@
\fi
}
\@ifdefinable\ifxP@moveto\relax
\@ifdefinable\xP@movetotrue\relax
\@ifdefinable\xP@movetofalse\relax
\newif\ifxP@moveto
\newcommand*\xP@savepts{\xP@xa\X@p
\xP@ya\Y@p
\xP@xb\L@c
\xP@yb\U@c
\xP@xc\R@c
\xP@yc\D@c
\xP@xd\X@c
\xP@yd\Y@c
}
\newcommand*\xP@restorepts{\X@p\xP@xa
\Y@p\xP@ya
\L@c\xP@xb
\U@c\xP@yb
\R@c\xP@xc
\D@c\xP@yc
\X@c\xP@xd
\Y@c\xP@yd
}
\@ifdefinable\xP@tmx\relax
\@ifdefinable\xP@tmy\relax
\newcommand*\xP@Tmxy{*\xP@Tmx/\xP@Tmy}
\newcommand*\xP@Tmyx{*\xP@Tmy/\xP@Tmx}
\newcommand*\xP@Tmzero{*\z@}
\newcommand*\xP@offsetsegment{{\xP@tangentvec\xP@a
\xP@xa\dimexpr\xP@precbezierpoly\X@p\L@c\R@c\X@c\xP@a/8+\d@Y*\xP@off/\@tempdimb\relax
\xP@ya\dimexpr\xP@precbezierpoly\Y@p\U@c\D@c\Y@c\xP@a/8-\d@X*\xP@off/\@tempdimb\relax
\xP@scaleT
\xP@Tax\d@X
\xP@Tay\d@Y
\xP@E\@tempdimb
\xP@tangentvec\xP@b
\xP@xd\dimexpr\xP@precbezierpoly\X@p\L@c\R@c\X@c\xP@b/8+\d@Y*\xP@off/\@tempdimb\relax
\xP@yd\dimexpr\xP@precbezierpoly\Y@p\U@c\D@c\Y@c\xP@b/8-\d@X*\xP@off/\@tempdimb\relax
\xP@scaleT
\xP@Tdx-\d@X
\xP@Tdy-\d@Y
\xP@F\@tempdimb
\xP@M\z@
\xP@Max\xP@M\xP@Tdx
\xP@Max\xP@M\xP@Tdy
\xP@L\dimexpr\xP@Tax*\xP@Tdx/\xP@M+\xP@Tay*\xP@Tdy/\xP@M\relax
\xP@tm\dimexpr(\xP@a+\xP@b)/2\relax
\ifdim\xP@L>\dimexpr\xP@E*\xP@F/\xP@M*49/50\relax
\d@X-\dimexpr\xP@Tay+\xP@Tdy\relax
\d@Y\dimexpr\xP@Tax+\xP@Tdx\relax
\xP@veclen
\xP@A\dimexpr\X@c-\X@p\relax
\xP@B\dimexpr\Y@c-\Y@p\relax
\xP@M\z@
\xP@Max\xP@M\xP@A
\xP@Max\xP@M\xP@B
\ifdim\xP@M=\z@
\xP@A\dimexpr\R@c-\L@c\relax
\xP@B\dimexpr\D@c-\U@c\relax
\xP@Max\xP@M\xP@A
\xP@Max\xP@M\xP@B
\fi
\xP@M\dimexpr\d@X*\xP@A/\xP@M+\d@Y*\xP@B/\xP@M\relax
\ifdim\xP@M<\z@
\multiply\d@X\m@ne
\multiply\d@Y\m@ne
\fi
\else
\xP@tangentvec\xP@tm
\fi
\xP@xm\dimexpr\xP@precbezierpoly\X@p\L@c\R@c\X@c\xP@tm+8\d@Y*\xP@off/\@tempdimb\relax
\xP@ym\dimexpr\xP@precbezierpoly\Y@p\U@c\D@c\Y@c\xP@tm-8\d@X*\xP@off/\@tempdimb\relax
\xP@Tmx\d@X
\xP@Tmy\d@Y
\xP@ifabsless\xP@Tmy\xP@Tmx
\let\xP@tmy\xP@Tmyx
\let\xP@tmx\@empty
\else
\ifdim\xP@Tmy=\z@
\let\xP@tmx\xP@Tmzero
\let\xP@tmy\xP@Tmzero
\else
\let\xP@tmy\@empty
\let\xP@tmx\xP@Tmxy
\fi
\fi
\xP@fa\p@
\xP@fd\p@
\xP@tm\p@
\count@\z@
\loop
\xP@offsetpoints
\@tempswafalse
\ifnum10>\count@
\xP@objfun\xP@oldobj
\ifdim\xP@oldobj>\xP@maxobjfun\relax\@tempswatrue\fi
\fi
\if@tempswa
\xP@offsetloop
\repeat
\xdef\@gtempa{\X@p\the\xP@xa\Y@p\the\xP@ya
\L@c\the\xP@xb\U@c\the\xP@yb\R@c\the\xP@xc\D@c\the\xP@yc
\X@c\the\xP@xd\Y@c\the\xP@yd\relax}}\@gtempa
}
\newcommand*\xP@scaleT{\xP@B6.28\xP@off
\xP@abs\xP@B
\xP@C\dimexpr\d@X*\xP@B/\@tempdimb\relax
\xP@D\dimexpr\d@Y*\xP@B/\@tempdimb\relax
\xP@A\dimexpr\xP@b-\xP@a\relax
\d@X\dimexpr\xP@C+\d@X*\xP@A/\xP@bigdim\relax
\d@Y\dimexpr\xP@D+\d@Y*\xP@A/\xP@bigdim\relax
\@tempdimb\dimexpr\xP@B+\@tempdimb*\xP@A/\xP@bigdim\relax
}
\newcommand*\xP@offsetloop{\xP@C\dimexpr\xP@C/2\relax
\xP@G\dimexpr\xP@G/2\relax
\xP@ta\dimexpr2\p@-\xP@tm\relax
\xP@tb\dimexpr\xP@tm*\xP@ta/\p@\relax
\xP@A\dimexpr\xP@Tax*\xP@tb/\p@*\xP@ta/\p@\relax
\xP@B\dimexpr\xP@Tdx*\xP@tb/\p@*\xP@tm/\p@\relax
\xP@E\dimexpr\xP@Tay*\xP@tb/\p@*\xP@ta/\p@\relax
\xP@F\dimexpr\xP@Tdy*\xP@tb/\p@*\xP@tm/\p@\relax
\xP@tb\dimexpr2\p@-3\xP@tm\relax
\xP@tc\dimexpr\xP@tb+2\p@\relax
\xP@I\dimexpr(2\xP@Tay\xP@tmx-2\xP@Tax\xP@tmy)*\xP@tb/\p@*\xP@ta/\p@\relax
\xP@J\dimexpr(2\xP@Tdy\xP@tmx-2\xP@Tdx\xP@tmy)*\xP@tc/\p@*\xP@tm/\p@\relax
\xP@K\dimexpr((\xP@yd-\xP@ya+(\xP@yb-\xP@yc)*3)
*\xP@tm/\p@+(\xP@yc-2\xP@yb+\xP@ya)*2)*12\xP@tmx
-((\xP@xd-\xP@xa+(\xP@xb-\xP@xc)*3)
*\xP@tm/\p@+(\xP@xc-2\xP@xb+\xP@xa)*2)*12\xP@tmy\relax
\xP@solvelinearsystem
\ifxP@validsol
\xP@correctsol
\ifdim\xP@ta=\z@
\ifdim\xP@tb=\z@
\ifdim\xP@tc=\z@
\xP@validsolfalse
\fi\fi\fi
\fi
\ifxP@validsol
\else
\xP@applinsys
\advance\xP@fa-\xP@ta
\advance\xP@fd-\xP@tb
\advance\xP@tm-\xP@tc
\ifdim\xP@tm<\z@\xP@tm\z@\fi
\ifdim\xP@tm>2\p@\xP@tm2\p@\fi
\fi
\advance\count@\@ne
}
\newcommand*\xP@maxsol{3pt}
\newcommand*\xP@correctsol{\xP@M\z@
\xP@Max\xP@M\xP@ta
\xP@Max\xP@M\xP@tb
\xP@Max\xP@M\xP@tc
\ifdim\xP@M>\xP@maxsol
\xP@ta\dimexpr\xP@maxsol*\xP@ta/\xP@M\relax
\xP@tb\dimexpr\xP@maxsol*\xP@tb/\xP@M\relax
\xP@tc\dimexpr\xP@maxsol*\xP@tc/\xP@M\relax
\fi
\advance\xP@fa-\xP@ta
\advance\xP@fd-\xP@tb
\xP@M\xP@tm
\advance\xP@tm-\xP@tc
\ifdim\xP@tm<\z@\xP@tm\z@\fi
\ifdim\xP@tm>2\p@\xP@tm2\p@\fi
{\xP@offsetpoints
\xP@objfun\xP@M
\expandafter}\ifdim\xP@M>\xP@oldobj
\advance\xP@fa\xP@ta
\advance\xP@fd\xP@tb
\xP@tm\xP@M
\xP@validsolfalse
\fi
}
\newcommand*\xP@objfun[1]{\xP@D\dimexpr\xP@bezierpoly\xP@xa\xP@xb\xP@xc\xP@xd\xP@tm-\xP@xm\relax
\xP@H\dimexpr\xP@bezierpoly\xP@ya\xP@yb\xP@yc\xP@yd\xP@tm-\xP@ym\relax
\xP@C\xP@beziertan\xP@xa\xP@xb\xP@xc\xP@xd\xP@tm
\xP@G\xP@beziertan\xP@ya\xP@yb\xP@yc\xP@yd\xP@tm
\xP@L\dimexpr\xP@G\xP@tmx-\xP@C\xP@tmy\relax
#1\z@
\xP@Max#1\xP@D
\xP@Max#1\xP@H
\xP@Max#1\xP@L
#1\ifdim#1>4843165sp
\maxdimen
\else
\dimexpr\xP@D*\xP@D/\p@+\xP@H*\xP@H/\p@+\xP@L*\xP@L/\p@\relax
\fi
}
\newcommand*\xP@offsetpoints{\xP@xb\dimexpr\xP@xa+\xP@Tax*\xP@fa/196608\relax
\xP@yb\dimexpr\xP@ya+\xP@Tay*\xP@fa/196608\relax
\xP@xc\dimexpr\xP@xd+\xP@Tdx*\xP@fd/196608\relax
\xP@yc\dimexpr\xP@yd+\xP@Tdy*\xP@fd/196608\relax
}
\newcommand*\xP@bezierpoly[5]{\dimexpr(((#4-#1+(#2-#3)*3)*#5/\p@+(#1-2#2+#3)*6)*#5/\p@+(#2-#1)*12)*#5/\p@
+#1*8\relax
}
\newcommand*\xP@precbezierpoly[5]{\dimexpr(((#4-#1+(#2-#3)*3)*2*#5/\xP@bigdim+(#1-2#2+#3)*6)*2*#5/\xP@bigdim
+(#2-#1)*12)*2*#5/\xP@bigdim+#1*8\relax
}
\newcommand*\xP@beziertan[5]{\dimexpr((#4-#1+(#2-#3)*3)*3*#5/32768+(#1-2#2+#3)*24)*#5/\p@+(#2-#1)*24\relax
}
\newcommand*\xP@precbeziertan[5]{\dimexpr((#4-#1+(#2-#3)*3)*#5/\xP@bigdim+(#1-2#2+#3)*2)*#5/\xP@bigdim
+#2-#1\relax
}
\@ifdefinable\xP@varone\relax
\@ifdefinable\xP@vartwo\relax
\@ifdefinable\xP@varthree\relax
\@ifdefinable\ifxP@validsol\relax
\@ifdefinable\xP@validsoltrue\relax
\@ifdefinable\xP@validsolfalse\relax
\newif\ifxP@validsol
\newcommand*\xP@solvelinearsystem{{\xP@scalerow\xP@A\xP@B\xP@C\xP@D
\xP@scalerow\xP@E\xP@F\xP@G\xP@H
\xP@scalerow\xP@I\xP@J\xP@K\xP@L
\xP@scalecol\xP@A\xP@E\xP@I\xP@scaleone
\xP@scalecol\xP@B\xP@F\xP@J\xP@scaletwo
\xP@scalecol\xP@C\xP@G\xP@K\xP@scalethree
\let\xP@varone\xP@ta
\let\xP@vartwo\xP@tb
\let\xP@varthree\xP@tc
\count@\m@ne
\@tempcnta\m@ne
\xP@ifabsless\xP@A\xP@B\@tempcnta\z@\xP@M\xP@B
\else\xP@M\xP@A\fi
\xP@ifabsless\xP@M\xP@C\@tempcnta\@ne\xP@M\xP@C\fi
\xP@ifabsless\xP@M\xP@E\@tempcnta\m@ne\count@\z@\xP@M\xP@E\fi
\xP@ifabsless\xP@M\xP@F\@tempcnta\z@\count@\z@\xP@M\xP@F\fi
\xP@ifabsless\xP@M\xP@G\@tempcnta\@ne\count@\z@\xP@M\xP@G\fi
\xP@ifabsless\xP@M\xP@I\@tempcnta\m@ne\count@\@ne\xP@M\xP@I\fi
\xP@ifabsless\xP@M\xP@J\@tempcnta\z@\count@\@ne\xP@M\xP@J\fi
\xP@ifabsless\xP@M\xP@K\@tempcnta\@ne\count@\@ne\fi
\ifcase\count@
\xP@swapdim\xP@A\xP@E
\xP@swapdim\xP@B\xP@F
\xP@swapdim\xP@C\xP@G
\xP@swapdim\xP@D\xP@H
\or
\xP@swapdim\xP@A\xP@I
\xP@swapdim\xP@B\xP@J
\xP@swapdim\xP@C\xP@K
\xP@swapdim\xP@D\xP@L
\fi
\ifcase\@tempcnta
\xP@swapdim\xP@A\xP@B
\xP@swapdim\xP@E\xP@F
\xP@swapdim\xP@I\xP@J
\let\xP@varone\xP@tb
\let\xP@vartwo\xP@ta
\xP@swapnum\xP@scaleone\xP@scaletwo
\or
\xP@swapdim\xP@A\xP@C
\xP@swapdim\xP@E\xP@G
\xP@swapdim\xP@I\xP@K
\let\xP@varone\xP@tc
\let\xP@varthree\xP@ta
\xP@swapnum\xP@scaleone\xP@scalethree
\fi
\multiply\xP@E\m@ne
\multiply\xP@I\m@ne
\ifdim\xP@A=\z@
\else
\advance\xP@F\dimexpr\xP@B*\xP@E/\xP@A\relax
\advance\xP@G\dimexpr\xP@C*\xP@E/\xP@A\relax
\advance\xP@H\dimexpr\xP@D*\xP@E/\xP@A\relax
\advance\xP@J\dimexpr\xP@B*\xP@I/\xP@A\relax
\advance\xP@K\dimexpr\xP@C*\xP@I/\xP@A\relax
\advance\xP@L\dimexpr\xP@D*\xP@I/\xP@A\relax
\fi
\count@\m@ne
\xP@ifabsless\xP@F\xP@G\@tempcnta\z@\xP@M\xP@G
\else\@tempcnta\m@ne\xP@M\xP@F\fi
\xP@ifabsless\xP@M\xP@J\@tempcnta\m@ne\count@\z@\xP@M\xP@J\fi
\xP@ifabsless\xP@M\xP@K\@tempcnta\z@\count@\z@\fi
\ifnum\count@=\z@
\xP@swapdim\xP@F\xP@J
\xP@swapdim\xP@G\xP@K
\xP@swapdim\xP@H\xP@L
\fi
\ifnum\@tempcnta=\z@
\xP@swapdim\xP@B\xP@C
\xP@swapdim\xP@F\xP@G
\xP@swapdim\xP@J\xP@K
\let\@tempa\xP@varthree
\let\xP@varthree\xP@vartwo
\let\xP@vartwo\@tempa
\xP@swapnum\xP@scaletwo\xP@scalethree
\fi
\ifdim\xP@F=\z@
\else
\advance\xP@K\dimexpr-\xP@G*\xP@J/\xP@F\relax
\advance\xP@L\dimexpr-\xP@H*\xP@J/\xP@F\relax
\fi
\xP@ifabsless{\dimexpr\xP@L/60\relax}{\dimexpr\xP@K/\xP@scalethree\relax}\xP@validsoltrue
\xP@varthree\dimexpr\xP@L*(\xP@scalethree*\p@)/\xP@K\relax
\else
\xP@validsolfalse
\fi
\xP@checkabs{\xP@H/8191}{\xP@F/\xP@scaletwo}\xP@checkabs{\xP@G/\xP@scalethree/136}{\xP@F/\xP@scaletwo}\ifxP@validsol
\xP@vartwo\dimexpr\xP@H*(\xP@scaletwo*\p@)/\xP@F
-\xP@varthree*\xP@scaletwo/\xP@scalethree*\xP@G/\xP@F\relax
\xP@checkabs\xP@vartwo{60pt}\fi
\xP@checkabs{\xP@D/5461}{\xP@A/\xP@scaleone}\xP@checkabs{\xP@B/\xP@scaletwo/91}{\xP@A/\xP@scaleone}\xP@checkabs{\xP@C/\xP@scalethree/91}{\xP@A/\xP@scaleone}\ifxP@validsol
\xP@varone\dimexpr\xP@D*(\xP@scaleone*\p@)/\xP@A
-\xP@vartwo*\xP@scaleone/\xP@scaletwo*\xP@B/\xP@A
-\xP@varthree*\xP@scaleone/\xP@scalethree*\xP@C/\xP@A\relax
\xP@checkabs\xP@varone{60pt}\fi
\xdef\@gtempa{\ifxP@validsol
\xP@ta\the\xP@ta\relax
\xP@tb\the\xP@tb\relax
\xP@tc\the\xP@tc\relax
\noexpand\xP@validsoltrue
\else
\noexpand\xP@validsolfalse
\fi
}}\@gtempa
}
\newcommand*\xP@scalerow[4]{\xP@M\z@
\xP@Max\xP@M#1\xP@Max\xP@M#2\xP@Max\xP@M#3\xP@Max\xP@M#4\count@134217727
\loop
\divide\xP@M\tw@
\ifdim\xP@M>\z@
\divide\count@\tw@
\repeat
\advance\count@\@ne
\multiply#1\count@
\multiply#2\count@
\multiply#3\count@
\multiply#4\count@
}
\newcommand*\xP@scalecol[4]{\xP@M\z@
\xP@Max\xP@M#1\xP@Max\xP@M#2\xP@Max\xP@M#3#416777215
\loop
\divide\xP@M\tw@
\ifdim\xP@M>\z@
\divide#4\tw@
\repeat
\advance#4\@ne
\multiply#1#4\multiply#2#4\multiply#3#4}
\newcommand*\xP@checkabs[2]{\xP@ifabsless{\dimexpr#1\relax}{\dimexpr#2\relax}\else\xP@validsolfalse\fi}
\newcommand*\xP@applinsys{{\xP@applinsys@
\xP@ta\xP@dta
\xP@tb\xP@dtb
\xP@tc\xP@dtc
\xP@checkapp
\if@tempswa
\xP@modobj
\xP@applinsys@
\xP@checkapp
\if@tempswa
\xP@modsol
\xP@modobj
\xP@applinsys@
\xP@modsol
\fi
\fi
\xdef\@gtempa{\xP@ta\the\xP@ta\relax
\xP@tb\the\xP@tb\relax
\xP@tc\the\xP@tc\relax
}}\@gtempa
}
\newcommand*\xP@checkapp{\@tempswatrue
\ifdim\xP@dta=\z@
\ifdim\xP@dtb=\z@
\ifdim\xP@dtc=\z@
\@tempswafalse
\fi\fi\fi
}
\newcommand*\xP@modobj{\advance\xP@D
\dimexpr-\xP@A*\xP@dta/\p@-\xP@B*\xP@dtb/\p@-\xP@C*\xP@dtc/\p@\relax
\advance\xP@H
\dimexpr-\xP@E*\xP@dta/\p@-\xP@F*\xP@dtb/\p@-\xP@G*\xP@dtc/\p@\relax
\advance\xP@L
\dimexpr-\xP@I*\xP@dta/\p@-\xP@J*\xP@dtb/\p@-\xP@K*\xP@dtc/\p@\relax
}
\newcommand*\xP@modsol{\advance\xP@ta\xP@dta
\advance\xP@tb\xP@dtb
\advance\xP@tc\xP@dtc
}
\newcommand*\xP@applinsys@{{\xP@sa\z@
\xP@Max\xP@sa\xP@A
\xP@Max\xP@sa\xP@B
\xP@Max\xP@sa\xP@C
\xP@Max\xP@sa\xP@E
\xP@Max\xP@sa\xP@F
\xP@Max\xP@sa\xP@G
\xP@Max\xP@sa\xP@I
\xP@Max\xP@sa\xP@J
\xP@Max\xP@sa\xP@K
\xP@sa\ifdim\xP@sa<5460pt\thr@@\xP@sa\else\maxdimen\fi
\xP@sb\z@
\xP@Max\xP@sb\xP@D
\xP@Max\xP@sb\xP@H
\xP@Max\xP@sb\xP@L
\ifdim\xP@sb>\z@
\xP@D\dimexpr\xP@D*\maxdimen/\xP@sb\relax
\xP@H\dimexpr\xP@H*\maxdimen/\xP@sb\relax
\xP@L\dimexpr\xP@L*\maxdimen/\xP@sb\relax
\fi
\xP@Aba\dimexpr\xP@A*\xP@D/\xP@sa+\xP@E*\xP@H/\xP@sa+\xP@I*\xP@L/\xP@sa\relax
\xP@Abb\dimexpr\xP@B*\xP@D/\xP@sa+\xP@F*\xP@H/\xP@sa+\xP@J*\xP@L/\xP@sa\relax
\xP@Abc\dimexpr\xP@C*\xP@D/\xP@sa+\xP@G*\xP@H/\xP@sa+\xP@K*\xP@L/\xP@sa\relax
\xP@AAba\dimexpr\xP@A*\xP@Aba/\xP@sa+\xP@B*\xP@Abb/\xP@sa
+\xP@C*\xP@Abc/\xP@sa\relax
\xP@AAbb\dimexpr\xP@E*\xP@Aba/\xP@sa+\xP@F*\xP@Abb/\xP@sa
+\xP@G*\xP@Abc/\xP@sa\relax
\xP@AAbc\dimexpr\xP@I*\xP@Aba/\xP@sa+\xP@J*\xP@Abb/\xP@sa
+\xP@K*\xP@Abc/\xP@sa\relax
\xP@sc\z@
\xP@Max\xP@sc\xP@Aba
\xP@Max\xP@sc\xP@Abb
\xP@Max\xP@sc\xP@Abc
\xP@Max\xP@sc\xP@AAba
\xP@Max\xP@sc\xP@AAbb
\xP@Max\xP@sc\xP@AAbc
\ifdim\xP@sc=\z@
\xP@AAb\z@
\else
\xP@Ab\dimexpr\xP@Aba*\xP@bigdim/\xP@sc*\xP@Aba/\xP@sc
+\xP@Abb*\xP@bigdim/\xP@sc*\xP@Abb/\xP@sc
+\xP@Abc*\xP@bigdim/\xP@sc*\xP@Abc/\xP@sc
\relax
\xP@AAb\dimexpr\xP@AAba*\xP@bigdim/\xP@sc*\xP@AAba/\xP@sc
+\xP@AAbb*\xP@bigdim/\xP@sc*\xP@AAbb/\xP@sc
+\xP@AAbc*\xP@bigdim/\xP@sc*\xP@AAbc/\xP@sc
\relax
\fi
\xdef\@gtempa{\ifdim\xP@AAb=\z@
\xP@dta\z@
\xP@dtb\z@
\xP@dtc\z@
\else
\xP@dta\the\dimexpr\xP@Aba*\xP@sb/\xP@sa*\p@/\xP@AAb*\xP@Ab/\maxdimen
\relax
\xP@dtb\the\dimexpr\xP@Abb*\xP@sb/\xP@sa*\p@/\xP@AAb*\xP@Ab/\maxdimen
\relax
\xP@dtc\the\dimexpr\xP@Abc*\xP@sb/\xP@sa*\p@/\xP@AAb*\xP@Ab/\maxdimen
\relax
\fi
}}\@gtempa
}
\@ifdefinable\ifxP@offsetok\relax
\@ifdefinable\xP@offsetoktrue\relax
\@ifdefinable\xP@offsetokfalse\relax
\newif\ifxP@offsetok
\newcommand*\xP@maxdev{.1pt}
\newcommand*\xP@maxobjfun{.005pt}
\newcommand*\xP@testoffset{{\gdef\xP@afteroffsetok{\xP@offsetoktrue}\def\xP@offsetokif{\ifdim\xP@ti<1.85pt}\xP@ti.1pt
\loop
\xP@tip\dimexpr\xP@a+(\xP@b-\xP@a)*\xP@ti/131072\relax
\L@p\xP@precbezierpoly\xP@xa\xP@xb\xP@xc\xP@xd\xP@tip
\U@p\xP@precbezierpoly\xP@ya\xP@yb\xP@yc\xP@yd\xP@tip
\xP@valA\dimexpr\xP@bezierpoly\X@p\L@c\R@c\X@c\xP@ti-\L@p\relax
\xP@valB\dimexpr\xP@bezierpoly\Y@p\U@c\D@c\Y@c\xP@ti-\U@p\relax
\d@X3\xP@precbeziertan\xP@xa\xP@xb\xP@xc\xP@xd\xP@tip
\d@Y3\xP@precbeziertan\xP@ya\xP@yb\xP@yc\xP@yd\xP@tip
\xP@veclen
\@tempdimc\dimexpr(\xP@b-\xP@a)*\@tempdimb/\xP@bigdim\relax
\xP@abs\@tempdimc
\ifdim.01pt<\@tempdimc
\xP@devA\dimexpr\xP@valA*\d@X/\@tempdimb+\xP@valB*\d@Y/\@tempdimb\relax
\xP@devB\dimexpr\xP@valA*\d@Y/\@tempdimb-\xP@valB*\d@X/\@tempdimb-8\xP@off
\relax
\xP@abs\xP@devA
\xP@abs\xP@devB
\@tempdima\dimexpr\xP@devA+\xP@devB\relax
\else
\ifdim\@tempdimc=\z@
\@tempdima\z@
\else
{\d@X\xP@valA
\d@Y\xP@valB
\xP@veclen@
\global\dimen@i\@tempdimb
}\@tempdima\dimen@i
\advance\@tempdima\ifdim\xP@off>\z@-\fi8\xP@off
\xP@abs\@tempdima
\fi
\fi
\ifdim\@tempdima>\xP@maxdev
\divide\L@p-8\relax
\divide\U@p-8\relax
{\xP@transformcoor\X@p\Y@p
\xP@transformcoor\L@c\U@c
\xP@transformcoor\R@c\D@c
\xP@transformcoor\X@c\Y@c
\xP@findzero
}\fi
\xP@offsetokif
\advance\xP@ti.1pt
\repeat
\expandafter}\xP@afteroffsetok
}
\newcommand*\xP@afteroffsetok{}
\newcommand*\xP@offsetokif{}
\newcommand*\xP@transformcoor[2]{\advance#1\L@p
\advance#2\U@p
\@tempdima\dimexpr#1*\d@X/\@tempdimb+#2*\d@Y/\@tempdimb\relax
#2\dimexpr#2*\d@X/\@tempdimb-#1*\d@Y/\@tempdimb\relax
#1\@tempdima
}
\newcommand*\xP@findzero{\xP@setleftvalue{.05}\xP@setrightvalue{.05}\ifdim\xP@valB<\z@\xP@reversecoeff\fi
\ifdim\xP@valA>\z@
\@tempswatrue
\@for\@tempa:={.1,.15,.2,.25,.35,.5,1.1}\do{\if@tempswa
\xP@setleftvalue\@tempa
\ifdim\xP@valA<\z@\@tempswafalse\fi
\if@tempswa
\xP@setrightvalue\@tempa
\ifdim\xP@valB<\z@
\@tempswafalse
\xP@reversecoeff
\fi
\fi
\fi
}\if@tempswa
\L@p\xP@ti
\xP@valA\xP@bezierpoly\X@p\L@c\R@c\X@c\L@p
\ifdim\xP@valA<\z@
\xP@setrightvalue{.05}\else
\U@p\L@p
\xP@valB\xP@valA
\fi
\fi
\fi
\loop
\ifnum\numexpr\U@p-\L@p\relax>\@ne
\xP@ti\dimexpr(\L@p+\U@p)/2\relax
\xP@devA\xP@bezierpoly\X@p\L@c\R@c\X@c\xP@ti
\ifdim\xP@devA>\z@
\U@p\xP@ti
\xP@valB\xP@devA
\else
\L@p\xP@ti
\xP@valA\xP@devA
\fi
\repeat
\xP@ifabsless\xP@valB\xP@valA
\L@p\U@p
\xP@valA\xP@valB
\fi
\xP@valB\dimexpr\xP@bezierpoly\Y@p\U@c\D@c\Y@c\L@p+8\xP@off\relax
\xP@abs\xP@valA
\xP@abs\xP@valB
\ifdim\dimexpr\xP@valA+\xP@valB\relax>\xP@maxdev\relax
\xP@failed
\fi
}
\newcommand*\xP@failed{\global\let\xP@offsetokif\iffalse
\gdef\xP@afteroffsetok{\xP@offsetokfalse}}
\newcommand*\xP@reversecoeff{\multiply\X@p\m@ne
\multiply\L@c\m@ne
\multiply\R@c\m@ne
\multiply\X@c\m@ne
\multiply\xP@valA\m@ne
\multiply\xP@valB\m@ne
}
\newcommand*\xP@setleftvalue[1]{\L@p\dimexpr\xP@ti-#1\p@\relax
\ifdim\L@p<-.1pt\L@p-.1pt\fi
\xP@valA\xP@bezierpoly\X@p\L@c\R@c\X@c\L@p
}
\newcommand*\xP@setrightvalue[1]{\U@p\dimexpr\xP@ti+#1\p@\relax
\ifdim\U@p>2.1\p@\U@p2.1\p@\fi
\xP@valB\xP@bezierpoly\X@p\L@c\R@c\X@c\U@p
}
\newcommand*\xP@splinedbldashed{\xP@checkspline\xP@splinemultdashed\xP@doublestroke}
\newcommand*\xP@splinetrbldashed{\xP@checkspline\xP@splinemultdashed\xP@trblstroke}
\newcommand*\xP@splinemultdashed[1]{\xP@testcont\xP@dashmacro
\@tempcnta
\ifxP@splinecont
\numexpr2*((\@tempdimb-\xydashl@/3)/(2*\xydashl@))\relax
\else
\numexpr2*((\@tempdimb+\xydashl@)/(2*\xydashl@))-1\relax
\fi
\ifnum\@tempcnta>\@ne
\xP@splinemultdashed@#1\else
\ifnum\@tempcnta=\@ne
\xP@splinemultsolid#1
\else
\xP@savec
\fi
\fi
\global\let\xP@lastpattern\xP@dashmacro
}
\newcommand*\xP@splinemultdashed@[1]{{\xP@inibigdim
\@tempdima\dimexpr\@tempdimb/\@tempcnta\relax
\xP@temppar\z@
\toks@{}\xP@savec
\ifodd\@tempcnta
\else
\xP@slide
\fi
\@tempcnta\z@
\loop
\advance\@tempcnta\@ne
\xP@append\toks@{\ifodd\@tempcnta\noexpand\xP@paintdash\fi
{\the\xP@temppar}}\xP@oldpar\xP@temppar
\xP@slide
\ifdim\xP@temppar<\xP@bigdim
\repeat
\xP@lastpar
\ifodd\@tempcnta
\xP@temppar
\xP@append\toks@{{\the\xP@temppar}}\else
\xP@oldpar
\fi
\@temptokena{}\xP@setsolidpat
\global\let\xP@lastpattern\xP@dashmacro
\@for\@tempa:={#1}\do{\the\toks@}\xP@stroke{\the\@temptokena}}}
\newcommand*\xP@paintdash[2]{\xP@paintsolid{\dimexpr#1*\xP@bigdim/\xP@lastpar\relax}{\dimexpr#2*\xP@bigdim/\xP@lastpar\relax}}
\xP@hook{curve}{splinedbldotted@}
\newcommand*\xP@splinedbldotted@{\let\xP@normalmult\@ne
\xP@checkspline\xP@splinemultdotted\xP@doublestroke}
\newcommand*\xP@splinetrbldotted{\let\xP@normalmult\tw@
\xP@checkspline\xP@splinemultdotted\xP@trblstroke}
\newcommand*\xP@multidottedpat{\def\xP@pattern{0 J [\xP@coor\xP@preclw{\xydashh@-\xP@preclw}]0 d}\global\let\xP@lastpattern\xP@dotmacro
}
\@ifdefinable\xP@normalmult\relax
\newcommand\xP@splinemultdotted[1]{{\xP@inibigdim
\xP@temppar\z@
\xP@testcont\xP@dotmacro
\ifxP@splinecont
\@tempdimc\dimexpr\@tempdimb/(\@tempdimb/131072+1)\relax
\@tempdima\dimexpr\@tempdimc-\xP@preclw/2\relax
\xP@slide
\@tempdima\@tempdimc
\else
\@tempdima\dimexpr\xP@preclw/2\relax
\xP@slide
\@tempdima\dimexpr\@tempdimb-\xP@preclw\relax
\ifdim\@tempdima<\z@\@tempdima\z@\fi
\@tempdima\dimexpr\@tempdima/(\@tempdima/131072+1)\relax
\fi
\xP@savec
\toks@{}\ifdim\xP@temppar<\xP@bigdim
\loop
\xP@append\toks@{\noexpand\xP@paintdot{\the\xP@temppar}}\xP@oldpar\xP@temppar
\xP@slide
\ifdim\xP@temppar<\xP@bigdim
\repeat
\xP@velocity\xP@bigdim\xP@tempvel
\ifdim
\ifdim\xP@preclw<\xP@tempvel
\dimexpr2\xP@bigdim-\xP@oldpar-\xP@preclw*\xP@bigdim/\xP@tempvel\relax
\else
-\maxdimen
\fi<\xP@temppar
\xP@temppar\xP@oldpar
\else
\xP@append\toks@{\noexpand\xP@paintdot{\the\xP@temppar}}\fi
\@tempdima\dimexpr\xP@preclw/2\relax
\xP@slide
\xP@lastpar\xP@temppar
\@temptokena{}\the\toks@
\xP@multidottedpat
\xP@stroke{\the\@temptokena}\else
\global\let\xP@lastpattern\@empty
\fi
}}
\newcommand*\xP@slide{{\xP@slide@
\global\dimen@i\xP@temppar
}\xP@temppar\dimen@i
}
\newcommand*\xP@slide@{\xP@velocity\xP@temppar\xP@tempvel
\@tempdimc\dimexpr\xP@bigdim*\@tempdima/\@tempdimb\relax
\count@\z@
\@tempswatrue
\loop
\xP@velocity{\xP@temppar+\@tempdimc}\xP@tempvel@
\ifdim\dimexpr\@tempdima*4/13\relax>\xP@tempvel@
\@tempswafalse
\else
\xP@parinc\dimexpr\@tempdima*\xP@bigdim/\xP@tempvel@
-(\xP@tempvel+\xP@tempvel@)/2*\@tempdimc/\xP@tempvel@\relax
\advance\@tempdimc\xP@parinc
\ifdim\@tempdimc>.12\xP@bigdim
\@tempswafalse
\else
\ifdim\xP@parinc=\z@
\@tempswafalse
\else
\ifnum\count@=9\relax
\@tempswafalse
\fi
\fi
\fi
\fi
\if@tempswa
\advance\count@\@ne
\repeat
\ifdim\xP@temppar<5461pt
\ifdim\@tempdimc>.1\xP@bigdim
\@tempswatrue
\fi
\fi
\if@tempswa
{\dimen5\xP@temppar
\advance\xP@temppar.1\xP@bigdim
\ifdim\xP@temppar>5461pt\xP@temppar5461pt\fi
\dimen7\xP@temppar
\xP@shaveprec{\dimen5}{\dimen7}\xP@bezierlength
\global\dimen@i\dimexpr\@tempdima-\@tempdimb\relax
\global\dimen3\xP@temppar
}\@tempdima\dimen@i
\xP@temppar\dimen3\relax
\expandafter\xP@slide@
\else
\advance\xP@temppar\@tempdimc
\fi
}
\newcommand*\xP@paintdot[1]{\@tempdima\dimexpr#1*\xP@bigdim/\xP@lastpar\relax
\xP@tangent
\xP@posX\dimexpr\xP@precbezierpoly\X@p\L@c\R@c\X@c\@tempdima/8\relax
\xP@posY\dimexpr\xP@precbezierpoly\Y@p\U@c\D@c\Y@c\@tempdima/8\relax
\@tempdima\dimexpr(\xydashh@+\xP@preclw/\xP@normalmult)/2\relax
\L@p\dimexpr\d@Y*\@tempdima/\@tempdimb\relax
\U@p\dimexpr-\d@X*\@tempdima/\@tempdimb\relax
\xP@append\@temptokena{\xP@coor{\xP@posX+\L@p*\xP@normalmult}{\xP@posY+\U@p*\xP@normalmult}m \xP@coor{\xP@posX-\L@p*(\xP@normalmult+\@ne)}{\xP@posY-\U@p*(\xP@normalmult+\@ne)}l }}
\newcommand*\xP@splinesquiggled{\xP@checkspline\xP@splinesquiggled@\z@}
\newcommand*\xP@splinedblsquiggled{\xP@checkspline\xP@splinesquiggled@\xP@doublestroke}
\newcommand*\xP@splinetrblsquiggled{\xP@checkspline\xP@splinesquiggled@\xP@trblstroke}
\newcommand*\xP@splinesquiggled@[1]{{\xP@inibigdim
\xP@testcont\xP@oddsquigglemacro
\ifxP@splinecont
\def\xP@squigsign{-}\else
\let\xP@squigsign\@empty
\fi
\xP@savec
\@tempcnta=\numexpr\@tempdimb/\xybsqll@\relax
\ifnum\@tempcnta<\tw@\@tempcnta\tw@\fi
\multiply\@tempcnta\tw@
\@tempdima\dimexpr\@tempdimb/\@tempcnta\relax
\xP@squiglen\@tempdima
\xP@temppar\z@
\toks@{}\@tempcnta\z@
\loop
\advance\@tempcnta\@ne
\xP@append\toks@{\noexpand\xP@paintsquiggle{\the\xP@temppar}}\xP@oldpar\xP@temppar
\xP@slide
\ifdim\xP@temppar<\xP@bigdim
\repeat
\xP@lastpar
\ifodd\@tempcnta
\xP@oldpar
\advance\@tempcnta\m@ne
\else
\xP@temppar
\xP@append\toks@{\noexpand\xP@paintsquiggle{\the\xP@temppar}}\fi
\@temptokena{}\xP@setsolidpat
\global\expandafter\let\expandafter\xP@lastpattern
\ifodd\numexpr\@tempcnta/2\if\xP@squigsign-+1\fi\relax
\xP@oddsquigglemacro
\else
\xP@evensquigglemacro
\fi
\@for\@tempa:={#1}\do{\let\xP@dosquiggle\xP@dosquiggle@
\count@\z@
\the\toks@
}\xP@stroke{\the\@temptokena}}}
\newcommand*\xP@paintsquiggle[1]{\xP@squigglevectors{#1}\xP@dosquiggle
\ifnum\count@=\thr@@\relax\count@\z@\else\advance\count@\@ne\fi
}
\newcommand*\xP@squigglevectors[1]{\@tempdima\dimexpr#1*\xP@bigdim/\xP@lastpar\relax
\xP@tangent
\xP@posX\dimexpr\xP@precbezierpoly\X@p\L@c\R@c\X@c\@tempdima/8-\d@Y*(\@tempa)/\@tempdimb\relax
\xP@posY\dimexpr\xP@precbezierpoly\Y@p\U@c\D@c\Y@c\@tempdima/8+\d@X*(\@tempa)/\@tempdimb\relax
\L@p\dimexpr\d@X*\xP@squiglen/\@tempdimb\relax
\U@p\dimexpr\d@Y*\xP@squiglen/\@tempdimb\relax
\R@p\dimexpr\L@p*543339720/1311738121\relax
\D@p\dimexpr\U@p*543339720/1311738121\relax
\X@min\dimexpr\L@p*362911648/967576667\relax
\Y@min\dimexpr\U@p*362911648/967576667\relax
\X@max\dimexpr(\L@p+\xP@squigsign\U@p)*173517671/654249180\relax
\Y@max\dimexpr(\L@p-\xP@squigsign\U@p)*173517671/654249180\relax
}
\@ifdefinable\xP@dosquiggle@\relax
\newcommand*\xP@dosquiggle@{\edef\next@{\xP@coor{\xP@posX}{\xP@posY}m
\xP@coor{\xP@posX+\Y@max}{\xP@posY+\xP@squigsign\X@max}}\let\xP@dosquiggle\xP@dosquiggle@@
}
\newcommand*\xP@dosquiggle@@{\xP@append\@temptokena{\next@\expandafter\xP@coor
\ifcase\count@
{\xP@posX-\Y@max}{\xP@posY-\xP@squigsign\X@max}\xP@coor\xP@posX\xP@posY
\or
{\xP@posX-\xP@squigsign\D@p-\X@min}{\xP@posY+\xP@squigsign\R@p-\Y@min}\xP@coor{\xP@posX-\xP@squigsign\D@p}{\xP@posY+\xP@squigsign\R@p}\or
{\xP@posX-\X@max}{\xP@posY+\xP@squigsign\Y@max}\xP@coor\xP@posX\xP@posY
\or
{\xP@posX+\xP@squigsign\D@p-\X@min}{\xP@posY-\xP@squigsign\R@p-\Y@min}\xP@coor{\xP@posX+\xP@squigsign\D@p}{\xP@posY-\xP@squigsign\R@p}\fi c }\edef\next@{\expandafter\xP@coor
\ifcase\count@
{\xP@posX+\Y@max}{\xP@posY+\xP@squigsign\X@max}\or
{\xP@posX-\xP@squigsign\D@p+\X@min}{\xP@posY+\xP@squigsign\R@p+\Y@min}\or
{\xP@posX+\X@max}{\xP@posY-\xP@squigsign\Y@max}\or
{\xP@posX+\xP@squigsign\D@p+\X@min}{\xP@posY-\xP@squigsign\R@p+\Y@min}\fi
}}
\newcommand*\xP@splinebrokensquiggled{\xP@checkspline\xP@splinebrokensquiggled@\z@}
\newcommand*\xP@splinebrokendblsquiggled{\xP@checkspline\xP@splinebrokensquiggled@\xP@doublestroke}
\newcommand*\xP@splinebrokentrblsquiggled{\xP@checkspline\xP@splinebrokensquiggled@\xP@trblstroke}
\newcommand*\xP@splinebrokensquiggled@[1]{{\xP@inibigdim
\xP@testcont\xP@brokensquigglemacro
\ifxP@splinecont
\let\xP@squigsign\@firstoftwo
\else
\let\xP@squigsign\@secondoftwo
\fi
\xP@savec
\@tempcnta\numexpr(\@tempdimb\xP@squigsign{}{+2*\xybsqll@})/(4*\xybsqll@)\relax
\ifnum\@tempcnta<\@ne\@tempcnta\@ne\fi
\@tempdima\dimexpr\@tempdimb/(8*\@tempcnta\xP@squigsign{}{-4})\relax
\xP@squiglen\@tempdima
\xP@temppar\z@
\xP@squigsign{\xP@slide\xP@slide\xP@slide\xP@slide}{}\count@\z@
\toks@{}\loop
\xP@append\toks@{\noexpand\xP@paintbrokensquiggle{\the\xP@temppar}}\xP@slide
\xP@append\toks@{{\the\xP@temppar}}\xP@slide
\xP@append\toks@{{\the\xP@temppar}}\xP@slide
\xP@append\toks@{{\the\xP@temppar}}\xP@slide
\xP@append\toks@{{\the\xP@temppar}}\xP@lastpar\xP@temppar
\advance\count@\@ne
\ifnum\count@<\@tempcnta
\xP@slide
\xP@slide
\xP@slide
\xP@slide
\repeat
\@temptokena{}\xP@setsolidpat
\global\let\xP@lastpattern\xP@brokensquigglemacro
\let\xP@squigsign\@empty
\@for\@tempa:={#1}\do{\the\toks@}\xP@stroke{\the\@temptokena}}}
\newcommand*\xP@paintbrokensquiggle[5]{\xP@squigglevectors{#1}\xP@append\@temptokena{\xP@coor\xP@posX\xP@posY m \xP@coor{\xP@posX+\Y@max}{\xP@posY+\X@max}}\xP@squigglevectors{#2}\xP@append\@temptokena{\xP@coor{\xP@posX-\D@p-\X@min}{\xP@posY+\R@p-\Y@min}\xP@coor{\xP@posX-\D@p}{\xP@posY+\R@p}c \xP@coor{\xP@posX-\D@p+\X@min}{\xP@posY+\R@p+\Y@min}}\xP@squigglevectors{#3}\xP@append\@temptokena{\xP@coor{\xP@posX-\X@max}{\xP@posY+\Y@max}\xP@coor\xP@posX\xP@posY c \xP@coor{\xP@posX+\X@max}{\xP@posY-\Y@max}}\xP@squigglevectors{#4}\xP@append\@temptokena{\xP@coor{\xP@posX+\D@p-\X@min}{\xP@posY-\R@p-\Y@min}\xP@coor{\xP@posX+\D@p}{\xP@posY-\R@p}c \xP@coor{\xP@posX+\D@p+\X@min}{\xP@posY-\R@p+\Y@min}}\xP@squigglevectors{#5}\xP@append\@temptokena{\xP@coor{\xP@posX-\Y@max}{\xP@posY-\X@max}\xP@coor\xP@posX\xP@posY c }}
\xyendinput





%%
%% End of file `xypdf-cu.tex'.


==> xypdf-fr.tex <==
%%
%% This is file `xypdf-fr.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `frame')
%% 
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://math.stanford.edu/~muellner>
%% --------------------------------------------------------------------------
%% 
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%% 
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%% 
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%% 
%% --------------------------------------------------------------------------
%% 
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%% 
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%% 
%% The files with the TeX code are generated by the following command:
%% 
%%    latex xypdf.ins
%% 
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%% 
%% --------------------------------------------------------------------------
%% 
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%% 
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%% 
\xyrequire{curve}\xycatcodes
\expandafter\let\csname xypdf-fr@loaded\endcsname\@empty
\newcommand*\xP@framedrop[1]{\expandafter\frmDrop@\expandafter{\expandafter\def\expandafter\prevEdge@@\expandafter{\prevEdge@@}\setboxz@h{#1\frmradius@@}\styledboxz@}}
\xP@hook{frame}{frm{-}}
\expandafter\newcommand\expandafter*\csname xP@frm{-}\endcsname{\xP@framedrop\xP@solidframe
}
\newcommand*\xP@solidframe[1]{\R@#1\relax
\xP@setsolidpat
\let\xP@fillorstroke\xP@stroke
\xP@frameifnotzero\xP@oval
}
\newcommand*\xP@ifzerosize[2]{\@tempswafalse
\ifdim\L@c=\z@\ifdim\R@c=\z@\ifdim\U@c=\z@\ifdim\D@c=\z@
\@tempswatrue
\fi\fi\fi\fi
\if@tempswa#1\else#2\fi
}
\newcommand*\xP@frameifnotzero[1]{\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\xP@ifzerosize{}{#1}}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
}
\newcommand*\xP@oval{\hskip-\L@c
\lower\D@c\hbox{\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\R@\xP@min\R@{.5\dimen@}\R@\xP@min\R@{.5\dimen@ii}\@tempdimb\dimexpr2\dimen@+2\dimen@ii-\R@*696621973/405764219\relax
\ifdim\R@=\z@
\xP@fillorstroke{0 0 \xP@coor\dimen@\dimen@ii re}\else
\def\@tempa{*119763188/267309217}\xP@fillorstroke{\xP@dim\R@0 m \xP@dim{\R@\@tempa}0 0 \xP@dim{\R@\@tempa}0 \xP@dim\R@ c \ifdim2\R@=\dimen@ii\else
0 \xP@dim{\dimen@ii-\R@}l \fi
0 \xP@dim{\dimen@ii-\R@\@tempa}\xP@coor{\R@\@tempa}\dimen@ii
\xP@coor\R@\dimen@ii c \ifdim2\R@=\dimen@\else
\xP@coor{\dimen@-\R@}\dimen@ii l \fi
\xP@coor{\dimen@-\R@\@tempa}\dimen@ii
\xP@coor\dimen@{\dimen@ii-\R@\@tempa}\xP@coor\dimen@{\dimen@ii-\R@} c \ifdim2\R@=\dimen@ii\else
\xP@coor\dimen@\R@ l \fi
\xP@coor\dimen@{\R@\@tempa}\xP@dim{\dimen@-\R@\@tempa}0 \xP@dim{\dimen@-\R@}0 c h}\fi
}}
\xP@hook{frame}{frm[o]{-}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{-}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setsolidpat}}
\newcommand*\xP@ellipseframe[2]{\xP@getradii{#2}\xP@ifzerosize{}{\def\xP@fillorstroke{#1\xP@stroke}\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\xP@framedellipse}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
}}
\xP@hook{frame}{frm{.}}
\expandafter\newcommand\expandafter*\csname xP@frm{.}\endcsname{\xP@framedrop\xP@rectframedotted
}
\newcommand*\xP@rectframedotted[1]{\R@#1\relax
\xP@frameifnotzero{\ifdim\R@=\z@
\xP@dottedrect
\else
\xP@dottedoval
\fi
}}
\newcommand*\xP@dottedrect{\hskip-\L@c
\lower\D@c\hbox{\dimen@ii\dimexpr\U@c+\D@c\relax
\@tempdimc\dimexpr\xP@preclw/-2\relax
\@tempdimb\dimexpr\L@c+\R@c+\xP@preclw\relax
\xP@contfalse
\xP@setdottedpat
\dimen@\dimexpr\@tempdimb+\@tempdima/2+\@tempdimc\relax
\xP@stroke{\xP@dim\@tempdimc0 m \xP@dim\dimen@0 l \xP@coor\@tempdimc\dimen@ii m \xP@coor\dimen@\dimen@ii l}\let\xP@testcont\xP@alwaysconttrue
\@tempdimb\dimen@ii
\xP@setdottedpat
\dimen@\dimexpr\L@c+\R@c\relax
\advance\dimen@ii\dimexpr\@tempdimc-\@tempdima/2\relax
\multiply\@tempdimc\m@ne
\xP@stroke{0 \xP@dim\@tempdimc m 0 \xP@dim\dimen@ii l \xP@coor\dimen@\@tempdimc m \xP@coor\dimen@\dimen@ii l}}}
\newcommand*\xP@dottedoval{\def\xP@fillorstroke{\xP@setcldottedpat\xP@stroke}\xP@oval
}
\xP@hook{frame}{frm[o]{.}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{.}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldottedpat}}
\xP@hook{frame}{frm{--}}
\expandafter\newcommand\expandafter*\csname xP@frm{--}\endcsname{\xP@framedrop\xP@rectframedashed
}
\newcommand*\xP@rectframedashed[1]{\R@#1\relax
\xP@frameifnotzero{\ifdim\R@=\z@
\xP@dashedrect
\else
\xP@dashedoval
\fi
}}
\newcommand*\xP@dashedrect{\hskip-\L@c
\lower\D@c\hbox{\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\@tempdimb\dimen@
\xP@contfalse
\xP@setdashpat
\xP@stroke{0 0 m \xP@dim\dimen@0 l 0 \xP@dim\dimen@ii m \xP@coor\dimen@\dimen@ii l}\@tempdimb\dimen@ii
\xP@setdashpat
\xP@stroke{0 0 m 0 \xP@dim\dimen@ii l \xP@dim\dimen@0 m \xP@coor\dimen@\dimen@ii l}}}
\newcommand*\xP@dashedoval{\def\xP@fillorstroke{\xP@setcldashpat\xP@stroke}\xP@oval
}
\xP@hook{frame}{frm[o]{--}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{--}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldashpat}}
\xP@hook{frame}{frm{,}}
\expandafter\newcommand\expandafter*\csname xP@frm{,}\endcsname{\xP@framedrop\xP@frameshadow
}
\newcommand*\xP@frameshadow[1]{\R@#1\relax
\ifdim\R@=\z@\R@1.2pt\relax\fi
\xP@frameifnotzero\xP@shadow
}
\newcommand*\xP@shadow{\hskip\dimexpr\R@c+\R@/2\relax
\lower\dimexpr\D@c+\R@/2\relax\hbox{\def\xP@pattern{0 J 0 j []0 d}\edef\xP@lw{\xP@dim\R@}\xP@stroke{\xP@dim{\R@/2-\L@c-\R@c} 0 m 0 0 l 0 \xP@dim{\D@c+\U@c-\R@/2}l}}}
\xP@hook{frame}{frm{o-}}
\expandafter\newcommand\expandafter*\csname xP@frm{o-}\endcsname{\xP@framedrop\xP@roundedrectframe
}
\newcommand*\xP@roundedrectframe[1]{\R@#1\relax
\ifdim\R@=\z@\R@\xydashl@\relax\fi
\xP@frameifnotzero\xP@roundedrectangle
}
\newcommand*\xP@roundedrectangle{\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\R@\xP@min\R@{.5\dimen@}\R@\xP@min\R@{.5\dimen@ii}\hskip-\L@c
\lower\D@c\hbox{\@tempdimb\dimexpr2\dimen@+2\dimen@ii-\R@*696621973/405764219\relax
\def\@tempa{*119763188/267309217}\xP@setsolidpat
\xP@stroke{\xP@dim\R@0 m \xP@dim{\R@\@tempa}0 0 \xP@dim{\R@\@tempa}0 \xP@dim\R@ c \ifdim2\R@=\dimen@ii\else
0 \xP@dim{\dimen@ii-\R@}m \fi
0 \xP@dim{\dimen@ii-\R@\@tempa}\xP@coor{\R@\@tempa}\dimen@ii
\xP@coor\R@\dimen@ii c \ifdim2\R@=\dimen@\else
\xP@coor{\dimen@-\R@}\dimen@ii m \fi
\xP@coor{\dimen@-\R@\@tempa}\dimen@ii
\xP@coor\dimen@{\dimen@ii-\R@\@tempa}\xP@coor\dimen@{\dimen@ii-\R@} c \ifdim2\R@=\dimen@ii\else
\xP@coor\dimen@\R@ m \fi
\xP@coor\dimen@{\R@\@tempa}\xP@dim{\dimen@-\R@\@tempa}0 \xP@dim{\dimen@-\R@}0 c}\xP@contfalse
\@tempdimb\dimexpr\L@c+\R@c-2\R@\relax
\ifdim\@tempdimb<\z@\@tempdimb\z@\fi
\xP@setdashpat
\ifdim\@tempdima>\z@
\dimen@\dimexpr\@tempdimb+\R@-\@tempdima/2\relax
\dimen@ii\dimexpr\U@c+\D@c\relax
\xP@stroke{\xP@dim{\R@+\@tempdima}0 m \xP@dim\dimen@ 0 l \xP@coor{\R@+\@tempdima}\dimen@ii m \xP@coor\dimen@\dimen@ii l}\fi
\@tempdimb\dimexpr\U@c+\D@c-2\R@\relax
\ifdim\@tempdimb<\z@\@tempdimb\z@\fi
\xP@setdashpat
\ifdim\@tempdima>\z@
\dimen@\dimexpr\L@c+\R@c\relax
\dimen@ii\dimexpr\@tempdimb+\R@-\@tempdima/2\relax
\xP@stroke{0 \xP@dim{\R@+\@tempdima}m 0 \xP@dim\dimen@ii l \xP@coor\dimen@{\R@+\@tempdima}m \xP@coor\dimen@\dimen@ii l}\fi
}}
\xP@hook{frame}{frm{=}}
\expandafter\newcommand\expandafter*\csname xP@frm{=}\endcsname{\xP@framedrop\xP@dsframe
}
\newcommand*\xP@dsframe[1]{\R@#1\relax
\xP@frameifnotzero\xP@dsoval
}
\newcommand*\xP@dsoval{\dimen@\dimexpr(\L@c+\R@c)/2\relax
\ifdim\dimen@<\xydashh@\dimen@\xydashh@\fi
\dimen@ii\dimexpr(\U@c+\D@c)/2\relax
\ifdim\dimen@ii<\xydashh@\dimen@ii\xydashh@\fi
\R@\xP@min\R@\dimen@
\R@\xP@min\R@\dimen@ii
\xP@setsolidpat
\let\xP@fillorstroke\xP@stroke
\xP@oval
\hskip\L@c
\advance\L@c-\xydashh@
\advance\R@c-\xydashh@
\advance\U@c-\xydashh@
\advance\D@c-\xydashh@
\advance\R@-\xydashh@
\ifdim\R@<\z@\R@\z@\fi
\xP@oval
}
\xP@hook{frame}{frm[o]{=}}
\expandafter\newcommand\expandafter*\csname xP@frm[o]{=}\endcsname{\xP@framedrop\xP@dsellframe
}
\xP@hook{frame}{frm{ee}}
\expandafter\newcommand\expandafter*\csname xP@frm{ee}\endcsname{\xP@framedrop\xP@dsellframe
}
\newcommand*\xP@dsellframe[1]{\xP@getradii{#1}\xP@frameifnotzero\xP@dsellipse
}
\@ifdefinable\xP@temppath\relax
\newcommand*\xP@dsellipse{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\advance\A@-\xydashh@
\advance\B@-\xydashh@
\ifdim\A@<\z@\A@\z@\fi
\ifdim\B@<\z@\B@\z@\fi
\def\xP@fillorstroke{\edef\xP@temppath}\xP@ellipse@
\xP@inibigdim
\let\@tempa\xydashh@
\xP@offsetellipse
\xP@setsolidpat
\xP@stroke{\xP@temppath\space\the\@temptokena}}}
\newcommand*\xP@offsetellipse{\xP@movetotrue
\@temptokena{}\xP@offsetelliptseg\A@\z@\A@{\B@*173517671/654249180}{\A@*554561898/619869377}{\B@*34221476/65864945}{\A@*543339720/768398401}{\B@*543339720/768398401}\xP@offsetelliptseg{\A@*543339720/768398401}{\B@*543339720/768398401}{\A@*34221476/65864945}{\B@*554561898/619869377}{\A@*173517671/654249180}\B@\z@\B@
\xP@mirrorpath
}
\newcommand*\xP@mirrorpath{\edef\@tempa{\the\@temptokena\relax\space\space\space\space}\let\@tempb\@empty
\let\@tempc\@empty
\expandafter\xP@mirrorpath@\@tempa
}
\@ifdefinable\xP@mirrorpath@\relax
\def\xP@mirrorpath@#1 #2 #3 #4 #5 #6 #7 {\ifx\relax#4\xP@append\@temptokena{\@tempb\xP@minus#1 \xP@minus#2 #3 \@tempc h}\else
\edef\@tempb{\xP@minus#6 #7 \xP@minus#4 #5 \xP@minus#1 #2 c \@tempb\if#3m\else\xP@minus#1 \xP@minus#2 #3 \fi\xP@minus#4 \xP@minus#5 \xP@minus#6 \xP@minus#7 }\edef\@tempc{#6 \xP@minus#7 #4 \xP@minus#5 #1 \xP@minus#2 c \@tempc}\expandafter\xP@mirrorpath@
\fi
}
\@ifdefinable\xP@minus\relax
\def\xP@minus#1 {\if-#1 \else\ifdim\dimexpr#1pt\relax=\z@\else-\fi#1 \fi}
\newcommand*\xP@insertbefore[2]{{\edef\@tempa{#1{#2\the#1}}\expandafter}\@tempa}
\newcommand*\xP@offsetelliptseg[8]{\X@p\dimexpr#1\relax
\Y@p\dimexpr#2\relax
\L@c\dimexpr#3\relax
\U@c\dimexpr#4\relax
\R@c\dimexpr#5\relax
\D@c\dimexpr#6\relax
\X@c\dimexpr#7\relax
\Y@c\dimexpr#8\relax
\xP@savepts
\xP@a\z@
\xP@c\xP@bigdim
\xP@paintsolid@
}
\newcommand*\xP@getradii[1]{\edef\@tempa{#1}\expandafter\xP@getradii@\@tempa,\maxdimen,@}
\@ifdefinable\xP@getradii@\relax
\def\xP@getradii@#1,#2,#3@{\A@#1\relax
\B@#2\relax
\ifdim\B@=\maxdimen
\A@\dimexpr(\L@c+\R@c)/2\relax
\B@\dimexpr(\U@c+\D@c)/2\relax
\fi
}
\xP@hook{frame}{frm{o}}
\expandafter\newcommand\expandafter*\csname xP@frm{o}\endcsname{\xP@framedrop{\xP@circleframe\xP@setsolidpat}}
\xP@hook{frame}{frm{-o}}
\expandafter\newcommand\expandafter*\csname xP@frm{-o}\endcsname{\xP@framedrop{\xP@circleframe\xP@setcldashpat}}
\xP@hook{frame}{frm{.o}}
\expandafter\newcommand\expandafter*\csname xP@frm{.o}\endcsname{\xP@framedrop{\xP@circleframe\xP@setcldottedpat}}
\newcommand*\xP@circleframe[2]{\R@#2\relax
\def\xP@fillorstroke{#1\xP@stroke}\xP@ifzerosize{\ifdim\R@>\z@
\xP@circleframe@
\fi
}{\ifdim\R@=\z@
\A@\dimexpr(\L@c+\R@c)/2\relax
\B@\dimexpr(\U@c+\D@c)/2\relax
\R@\xP@max\A@\B@
\fi
\xP@circleframe@
}}
\newcommand*\xP@circleframe@{\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\xP@circle}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
}
\xP@hook{frame}{frm{e}}
\expandafter\newcommand\expandafter*\csname xP@frm{e}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setsolidpat}}
\xP@hook{frame}{frm{-e}}
\expandafter\newcommand\expandafter*\csname xP@frm{-e}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldashpat}}
\xP@hook{frame}{frm{.e}}
\expandafter\newcommand\expandafter*\csname xP@frm{.e}\endcsname{\xP@framedrop{\xP@ellipseframe\xP@setcldottedpat}}
\xP@hook{frame}{frm2{.e}}
\expandafter\newcommand\expandafter*\csname xP@frm2{.e}\endcsname{\xP@framedrop\xP@dsdottedellframe
}
\newcommand*\xP@dsdottedellframe[1]{\xP@getradii{#1}\xP@frameifnotzero\xP@dsdottedellipse
}
\newcommand*\xP@dsdottedellipse{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\@tempdima.5\xydashh@\relax
\advance\A@-\@tempdima
\advance\B@-\@tempdima
\ifdim\A@<\@tempdima\A@\@tempdima\fi
\ifdim\B@<\@tempdima\B@\@tempdima\fi
\let\xP@normalmult\@ne
\xP@specialellipse{\xP@splinemultdotted\xP@doublestroke}}}
\newcommand*\xP@specialellipse[1]{\def\@tempa{*147546029/267309217}\X@p\A@
\Y@p\z@
\L@c\A@
\U@c\dimexpr\B@\@tempa\relax
\R@c\dimexpr\A@\@tempa\relax
\D@c\B@
\X@c\z@
\Y@c\B@
\xP@bezierlength
\let\xP@testcont\xP@alwaysconttrue
#1\X@p\z@
\Y@p\B@
\L@c-\R@c
\D@c\U@c
\U@c\B@
\R@c-\A@
\X@c-\A@
\Y@c\z@
#1\X@p-\A@
\Y@p\z@
\R@c\L@c
\L@c-\A@
\U@c-\D@c
\D@c-\B@
\X@c\z@
\Y@c-\B@
#1\X@p\z@
\Y@p-\B@
\L@c-\R@c
\D@c\U@c
\U@c-\B@
\R@c\A@
\X@c\A@
\Y@c\z@
#1}
\newcommand*\xP@alwaysconttrue[1]{\xP@splineconttrue}
\xP@hook{frame}{frm2{-e}}
\expandafter\newcommand\expandafter*\csname xP@frm2{-e}\endcsname{\xP@framedrop\xP@dsdashellframe
}
\newcommand*\xP@dsdashellframe[1]{\xP@getradii{#1}\xP@frameifnotzero\xP@dsdashellipse
}
\newcommand*\xP@dsdashellipse{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\advance\A@-\xydashh@
\advance\B@-\xydashh@
\ifdim\A@<\z@\A@\z@\fi
\ifdim\B@<\z@\B@\z@\fi
\xP@specialellipse{\xP@splinemultdashed\xP@elldoublestroke}}}
\newcommand*\xP@elldoublestroke{\z@,\xydashh@}
\newcommand*\xP@fill[1]{\xP@literal{#1 f}}
\newcommand*\xP@fillstroke[1]{\xP@literal{\xP@dim{\xP@preclw/2}w 1 j 0 G #1 b}}
\newcommand*\xP@fillorstroke{}
\xP@hook{frame}{frm{*}}
\expandafter\newcommand\expandafter*\csname xP@frm{*}\endcsname{\xP@framedrop{\let\xP@fillorstroke\xP@fill\xP@framefill}}
\xP@hook{frame}{frm{**}}
\expandafter\newcommand\expandafter*\csname xP@frm{**}\endcsname{\xP@framedrop{\let\xP@fillorstroke\xP@fillstroke\xP@framefill}}
\newcommand*\xP@framefill[1]{\R@#1\relax
\xP@setsolidpat
\setboxz@h{\hskip\X@c\raise\Y@c\hbox{\DN@{\rectangleEdge}\ifx\next@\prevEdge@@
\DN@{\xP@oval}\else
\DN@{\circleEdge}\ifx\next@\prevEdge@@
\ifdim\R@=\z@
\DN@{\xP@filledellipse}\else
\DN@{\restR@max\xP@circle}\fi
\else
\ifdim\R@=\z@
\DN@{\xP@oval}\else
\DN@{\xP@circle}\fi
\fi
\fi
\next@
}}\wd\z@\z@\ht\z@\z@\dp\z@\z@
\boxz@
}
\newcommand*\xP@circle{\xP@ellipse\R@\R@
}
\newcommand*\xP@filledellipse{\xP@ellipse{\dimexpr(\L@c+\R@c)/2\relax}{\dimexpr(\U@c+\D@c)/2\relax}}
\newcommand*\xP@framedellipse{\xP@ellipse\A@\B@
}
\newcommand*\xP@ellipse[2]{\hskip\dimexpr(\R@c-\L@c)/2\relax
\lower\dimexpr(\D@c-\U@c)/2\relax
\hbox{\A@#1\relax
\B@#2\relax
\xP@ellipse@
}}
\newcommand*\xP@ellipse@{\X@p\dimexpr\A@*543339720/768398401\relax
\Y@p\dimexpr\B@*543339720/768398401\relax
\L@c\dimexpr\A@*34221476/65864945\relax
\U@c\dimexpr\B@*554561898/619869377\relax
\R@c\dimexpr\A@*173517671/654249180\relax
\D@c\B@
\X@c\z@
\Y@c\B@
\xP@bezierlength
\@tempdima\@tempdimb
\X@p\A@
\Y@p\z@
\L@c\A@
\U@c\dimexpr\B@*173517671/654249180\relax
\R@c\dimexpr\A@*554561898/619869377\relax
\D@c\dimexpr\B@*34221476/65864945\relax
\X@c\dimexpr\A@*543339720/768398401\relax
\Y@c\dimexpr\B@*543339720/768398401\relax
\xP@bezierlength
\@tempdimb4\dimexpr\@tempdima+\@tempdimb\relax
\edef\@tempa{\xP@dim\A@0 m
\xP@coor\L@c\U@c
\xP@coor\R@c\D@c
\xP@coor\X@c\Y@c c \xP@coor{\A@*34221476/65864945}{\B@*554561898/619869377}\xP@coor{\A@*173517671/654249180}\B@
0 \xP@dim\B@ c }\@temptokena\expandafter{\@tempa}\xP@mirrorpath
\xP@fillorstroke{\the\@temptokena}}
\xyendinput





%%
%% End of file `xypdf-fr.tex'.


==> xypdf-li.tex <==
%%
%% This is file `xypdf-li.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `line')
%% 
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://math.stanford.edu/~muellner>
%% --------------------------------------------------------------------------
%% 
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%% 
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%% 
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%% 
%% --------------------------------------------------------------------------
%% 
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%% 
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%% 
%% The files with the TeX code are generated by the following command:
%% 
%%    latex xypdf.ins
%% 
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%% 
%% --------------------------------------------------------------------------
%% 
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%% 
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%% 
\xycatcodes
\expandafter\let\csname xypdf-li@loaded\endcsname\@empty
\xyendinput





%%
%% End of file `xypdf-li.tex'.


==> xypdf-ro.tex <==
%%
%% This is file `xypdf-ro.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `rotate')
%% 
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://math.stanford.edu/~muellner>
%% --------------------------------------------------------------------------
%% 
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%% 
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%% 
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%% 
%% --------------------------------------------------------------------------
%% 
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%% 
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%% 
%% The files with the TeX code are generated by the following command:
%% 
%%    latex xypdf.ins
%% 
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%% 
%% --------------------------------------------------------------------------
%% 
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%% 
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%% 
\xycatcodes
\expandafter\let\csname xypdf-ro@loaded\endcsname\@empty
\xP@hook{rotate}{xyscale@@}
\newcommand*\xP@xyscale@@[2]{\setboxz@h{\hskip\L@c
\hskip-\R@p
\lower\U@p\hbox{\xP@cm{#1}00{#2}{\raise\U@p\hb@xt@\z@{\hskip-\L@c\hskip\R@p\boxz@\hss}}}}\global\let\xP@lastpattern\@empty
}
\xP@hook{rotate}{xyRotate@@}
\newcommand\xP@xyRotate@@{\xP@rotate@\xP@trigfromdir}
\xP@hook{rotate}{doSpecialRotate@@}
\@ifdefinable\xP@doSpecialRotate@@\relax
\def\xP@doSpecialRotate@@#1@@{\xP@rotate@\xP@trig{#1}}
\newcommand*\xP@rotate@[2]{\setboxz@h{#1{#2}\hskip\L@c
\hskip-\R@p
\lower\U@p\hbox{\xP@cm\cosDirection\sinDirection
{\if-\sinDirection\else-\sinDirection\fi}\cosDirection
{\raise\U@p\hb@xt@\z@{\hskip-\L@c\hskip\R@p\boxz@\hss}}}}\global\let\xP@lastpattern\@empty
}
\newcommand*\xP@trig[1]{\@tempdima\dimexpr#1pt\relax
\@tempdimb\@tempdima
\divide\@tempdimb23592960
\advance\@tempdima-23592960\@tempdimb
\ifdim\@tempdima<\z@\advance\@tempdima360pt\fi
\@tempdimb\@tempdima
\divide\@tempdimb5898240
\ifcase\@tempdimb
\xP@sinpoly
\edef\sinDirection{\xP@EARPT\@tempdimb}\@tempdima\dimexpr90pt-\@tempdima\relax
\xP@sinpoly
\edef\cosDirection{\xP@EARPT\@tempdimb}\or
\@tempdima\dimexpr180pt-\@tempdima\relax
\xP@sinpoly
\edef\sinDirection{\xP@EARPT\@tempdimb}\@tempdima\dimexpr90pt-\@tempdima\relax
\xP@sinpoly
\edef\cosDirection{\xP@EARPT\dimexpr-\@tempdimb\relax}\or
\@tempdima\dimexpr\@tempdima-180pt\relax
\xP@sinpoly
\edef\sinDirection{\xP@EARPT\dimexpr-\@tempdimb\relax}\@tempdima\dimexpr90pt-\@tempdima\relax
\xP@sinpoly
\edef\cosDirection{\xP@EARPT\dimexpr-\@tempdimb\relax}\or
\@tempdima\dimexpr360pt-\@tempdima\relax
\xP@sinpoly
\edef\sinDirection{\xP@EARPT\dimexpr-\@tempdimb\relax}\@tempdima\dimexpr90pt-\@tempdima\relax
\xP@sinpoly
\edef\cosDirection{\xP@EARPT\@tempdimb}\else
\PackageError{xypdf}{Unexpected case in sin/cos calculation}{Feel free to contact the author of the xypdf package with a minimal example.}\fi
}
\newcommand*\xP@sinpoly{{\ifdim\@tempdima<49pt
\ifdim\@tempdima<27pt
\@tempdimb\dimexpr((\@tempdima*-529771058/16039085-1384933sp)*\@tempdima/268756075+10714164sp)*\@tempdima/613777813\relax
\else
\advance\@tempdima-27pt
\@tempdimb\dimexpr(((\@tempdima*-743101305/20672414-238989613sp)*\@tempdima/80975565+42661556sp)*\@tempdima/622461739+2\p@)*157520747/693945047\relax
\fi
\else
\ifdim\@tempdima<70pt
\advance\@tempdima-49pt
\@tempdimb\dimexpr(((\@tempdima*-348406699/107952940-55079229sp)*\@tempdima/866635628+408805sp)*\@tempdima/26926757+\p@)*135751711/179873976\relax
\else
\advance\@tempdima-70pt
\@tempdimb\dimexpr(((\@tempdima*-1015850353/137849442-460519207sp)*\@tempdima/8742349+142263941sp)*\@tempdima/972432199+23\p@)*31253604/764969669\relax
\fi
\fi
\global\dimen@i\@tempdimb
}\@tempdimb\dimen@i
}
\xyendinput





%%
%% End of file `xypdf-ro.tex'.


==> xypdf.tex <==
%%
%% This is file `xypdf.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xypdf.dtx  (with options: `basic')
%% 
%% The xypdf package for TeX and LaTeX
%% Copyright (c) 2010 by Daniel Müllner (M\"ullner)
%% <http://math.stanford.edu/~muellner>
%% --------------------------------------------------------------------------
%% 
%% This program is free software: you can redistribute it and/or modify it
%% under the terms of the GNU General Public License as published by the Free
%% Software Foundation, either version 2 of the License, or (at your option)
%% any later version.
%% 
%% This program is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%% 
%% The GNU General Public License is available at
%% <http://www.gnu.org/licenses/>.
%% 
%% --------------------------------------------------------------------------
%% 
%% This file is part of the xypdf package for TeX and LaTeX2e. The xypdf
%% package may be distributed and/or modified under the conditions of the
%% GNU General Public License as published by the Free Software Foundation,
%% either version 2 of the License, or (at your option) any later version.
%% The distribution consists of the following files:
%% 
%%    xypdf.dtx  -  Documented source code
%%    xypdf.ins  -  Installation script
%%    xypdf.pdf  -  Documentation (generated from xypdf.dtx)
%% 
%% The files with the TeX code are generated by the following command:
%% 
%%    latex xypdf.ins
%% 
%% This generates the files xypdf.tex, xypdf-co.tex, xypdf-cu.tex,
%% xypdf-fr.tex, xypdf-li.tex and xypdf-ro.tex.
%% 
%% --------------------------------------------------------------------------
%% 
%% The xypdf package improves the output quality of the Xy-pic package when
%% PDF documents are generated. It produces generic PDF code for graphical
%% elements like lines, curves and circles instead of approximating these
%% elements with glyphs in special fonts as the original Xy-pic package does.
%% The xypdf package works with both TeX and LaTeX in the occurrences of
%% pdfTeX, XeTeX and eTeX with dvipdfm(x) to generate PDF files. It is being
%% integrated and distributed together with Xy-pic, starting with Xy-pic
%% version 3.8.
%% 
%% The copyright for the xypdf package is by its author, Daniel Müllner
%% (Muellner, M\"ullner).
%% 
\ifx\xyloaded\undefined\input xy \fi
\xyprovide{pdf}{PDF driver}{1.7}{Daniel M\"ullner\newline}{\url{http://math.stanford.edu/~muellner}}{}
\ifx\makeatletter\undefined\input miniltx \fi
\newcommand*\xypdfdate{2011/03/20}
\newdriver{\xyaddsupport{pdf}\xP@pdf@on
\xyaddsupport{color}\xP@color@on
\xyaddsupport{curve}\xP@curve@on
\xyaddsupport{frame}\xP@frame@on
\xyaddsupport{rotate}\xP@rotate@on
}
\xyaddunsupport{pdf}\xP@pdf@off
\xyaddunsupport{color}\xP@color@off
\xyaddunsupport{curve}\xP@curve@off
\xyaddunsupport{frame}\xP@frame@off
\xyaddunsupport{rotate}\xP@rotate@off
\newcommand*\xypdfon{\xP@pdf@on
\xP@color@on
\xP@curve@on
\xP@frame@on
\xP@line@on
\xP@rotate@on
}
\newcommand*\xypdfoff{\xP@pdf@off
\xP@color@off
\xP@curve@off
\xP@frame@off
\xP@line@off
\xP@rotate@off
}
\ifx\unexpanded\@undefined
\PackageError{xypdf}{eTeX is needed for the xypdf package}{}
\fi
\newcommand*\xP@testpdfsave{\ifpdf
\ifx\pdfsave\@undefined
\PackageError{xypdf}{pdfTeX version 1.40.0 or higher is needed for the xypdf^^Jpackage with PDF output}{}\fi
\fi
\let\xP@testpdfsave\@undefined
}
\ifx\PackageWarning\@undefined
\newcommand*\xP@warning[2]{{\newlinechar`\^^J\@warning{Package #1 Warning: #2\@empty.}}}
\else
\newcommand*\xP@warning{\PackageWarning}
\fi
\newcommand*\xP@pdf@on{}
\newcommand*\xP@pdf@off{}
\newcommand*\xP@color@on{}
\newcommand*\xP@color@off{}
\newcommand*\xP@curve@on{}
\newcommand*\xP@curve@off{}
\newcommand*\xP@frame@on{}
\newcommand*\xP@frame@off{}
\newcommand*\xP@line@on{}
\newcommand*\xP@line@off{}
\newcommand*\xP@rotate@on{}
\newcommand*\xP@rotate@off{}
\newcommand*\xP@hook[2]{\edef\next@{\let\expandafter\noexpand\csname xP@old@#2\endcsname
\expandafter\noexpand\csname#2\endcsname}\next@
\expandafter\edef\csname xP@#1@on\endcsname{\unexpanded\expandafter\expandafter\expandafter{\csname xP@#1@on\endcsname}\let\expandafter\noexpand\csname#2\endcsname
\expandafter\noexpand\csname xP@#2\endcsname
}\expandafter\edef\csname xP@#1@off\endcsname{\unexpanded\expandafter\expandafter\expandafter{\csname xP@#1@off\endcsname}\let\expandafter\noexpand\csname#2\endcsname
\expandafter\noexpand\csname xP@old@#2\endcsname
}}
\newcommand*\xP@defpdfliteral{\ifpdf
\newcommand*\xP@literal[1]{\pdfsave\pdfliteral{##1}\pdfrestore}
\newcommand*\xP@cm[5]{\pdfsave
\pdfsetmatrix{##1 ##2 ##3 ##4}##5\pdfrestore
}
\@ifundefined{@pdfcolorstack}{\def\@pdfcolorstack{\z@}}{}\newcommand*\xP@setcolor[3]{\pdfcolorstack\@pdfcolorstack push{##1 ##2 ##1 ##3}}
\newcommand*\xP@resetcolor{\pdfcolorstack\@pdfcolorstack pop\relax}\else
\newcommand*\xP@literal{\xP@warning{xypdf}{The produced DVI file is NOT PORTABLE. Convert it with^^Jdvipdfm(x) to the PDF format but do not expect the DVI file itself to be^^Jdisplayed correctly\@gobble}\global\let\xP@literal\xP@literal@
\xP@literal
}
\newcommand*\xP@literal@[1]{\special{pdf:content ##1}}
\newcommand*\xP@cm[5]{\special{pdf:btrans matrix ##1 ##2 ##3 ##4 0 0}##5\special{pdf:etrans}}
\newcommand*\xP@setcolor[3]{\special{pdf:bcolor[##1]}}
\newcommand*\xP@resetcolor{\special{pdf:ecolor}}\fi
\let\xP@defpdfliteral\@undefined
}
\DN@{\@firstofone}
\DNii@{xy}
\ifx\@currname\nextii@
\ifx\AtEndOfPackage\@undefined
\else
\DN@{\AtEndOfPackage}\fi
\fi
\next@
{\RequirePackage{ifpdf}\xP@testpdfsave
\xP@defpdfliteral}
\ifx\pdfdecimaldigits\@undefined
\newcommand*\xP@digits{2}
\else
\@ifdefinable\xP@digits\relax
\xdef\xP@digits{\the\pdfdecimaldigits}
\ifnum\pdfdecimaldigits<2
\xP@warning{xypdf}{The precision in \string\pdfdecimaldigits\space is only \xP@digits\space
decimals.^^JIt is recommended to set \string\pdfdecimaldigits\space to 2 or 3 for best output quality\@gobble}
\fi
\fi
\newcommand*\xP@dim[1]{\expandafter\xP@removePT\the\dimexpr(#1)*800/803\relax\space}
\newcommand*\xP@precdim[1]{\xP@EARPT\dimexpr(#1)*800/803\relax\space}
\newcommand*\xP@EARPT{\expandafter\removePT@\the}
\newcommand*\xP@coor[1]{\xP@dim{#1}\xP@dim}
\@ifdefinable\xP@removePT\relax
{\@makeother\p\@makeother\t\gdef\xP@removePT#1pt{\xP@removePT@#10000@}}
\@ifdefinable\xP@removePT@\relax
\ifcase\xP@digits
\def\xP@removePT@#1.#2#3@{\ifnum#2<5
#1\else
\the\numexpr-\if-#1-\else-#1+\fi\@ne\relax
\fi
}
\or
\def\xP@removePT@#1#2.#3#4#5@{\ifnum#4<5
#1#2\if#30\else
.#3\fi
\else
\expandafter\xP@removePT
\the\dimexpr#1#2.#3pt+\if#1--\fi.12pt\relax
\fi
}
\or
\def\xP@removePT@#1#2.#3#4#5#6@{\ifnum#5<5
#1#2\if#40\if#30\else
.#3\fi
\else
.#3#4\fi
\else
\expandafter\xP@removePT
\the\dimexpr#1#2.#3#4pt+\if#1--\fi786sp\relax
\fi
}
\or
\def\xP@removePT@#1#2.#3#4#5#6#7@{\ifnum#6<5
#1#2\if#50\if#40\if#30\else
.#3\fi
\else
.#3#4\fi
\else
.#3#4#5\fi
\else
\expandafter\xP@removePT
\the\dimexpr#1#2.#3#4#5pt+\if#1--\fi79sp\relax
\fi
}
\or
\def\xP@removePT@#1#2.#3#4#5#6#7#8@{\ifnum#7<5
#1#2\if#60\if#50\if#40\if#30\else
.#3\fi
\else
.#3#4\fi
\else
.#3#4#5\fi
\else
.#3#4#5#6\fi
\else
\expandafter\xP@removePT
\the\dimexpr#1#2.#3#4#5#6pt+\if#1--\fi8sp\relax
\fi
}
\else
\let\xP@dim\xP@precdim
\fi
\AtBeginDocument{{\setboxz@h{$ $}}\@ifdefinable\xP@lw\relax
\@ifdefinable\xP@preclw\relax
\edef\xP@preclw{\the\fontdimen8\textfont3}\edef\xP@lw{\xP@dim\xP@preclw}\PackageInfo{xypdf}{Line width: \xP@preclw}}
\xP@hook{pdf}{line@}
\newcommand*\xP@line@{\setboxz@h{\xP@setsolidpat
\xP@stroke{0 0 m \xP@coor{\cosDirection\xydashl@}{\sinDirection\xydashl@}l}}\U@c\sinDirection\xydashl@
\D@c\z@
\ifdim\U@c<\z@
\multiply\U@c\m@ne
\xP@swapdim\U@c\D@c
\fi
\ht\z@\U@c
\dp\z@\D@c
\R@c\cosDirection\xydashl@
\L@c\z@
\ifdim\R@c<\z@
\multiply\R@c\m@ne
\xP@swapdim\L@c\R@c
\fi
\hskip\L@c\boxz@\hskip\R@c
\edef\tmp@{\egroup\U@c\the\U@c\D@c\the\D@c\L@c\the\L@c\R@c\the\R@c}\tmp@
\Edge@c={\rectangleEdge}\edef\Upness@{\ifdim\z@<\U@c1\else0\fi}\edef\Leftness@{\ifdim\z@<\L@c1\else0\fi}\def\Drop@@{\styledboxz@}\def\Connect@@{\solid@}}
\xP@hook{pdf}{solid@}
\newcommand*\xP@solid@{\straight@\xP@solidSpread}
\@ifdefinable\xP@solidSpread\relax
\def\xP@solidSpread#1\repeat@{{\@tempswatrue
\ifdim\X@p=\X@c
\ifdim\Y@p=\Y@c
\@tempswafalse
\fi
\fi
\if@tempswa
\xP@setsolidpat
\xP@stroke{\xP@coor\X@p\Y@p m \xP@coor\X@c\Y@c l}\fi
}}
\newcommand*\xP@pattern{}
\newcommand*\xP@setsolidpat{\def\xP@pattern{1 J 1 j []0 d}\global\let\xP@lastpattern\xP@solidmacro
}
\newcommand*\xP@stroke[1]{\xP@literal{\xP@lw w \xP@pattern\space#1 S}}
\xP@hook{pdf}{dash@}
\newcommand\xP@dash@{\line@\def\Connect@@{\straight@\xP@dashedSpread}}
\@ifdefinable\xP@dashedSpread\relax
\def\xP@dashedSpread#1\repeat@{{\xP@veclen
\ifdim\@tempdimb>\z@
\xP@setdashpat
\xP@savec
\xP@stroke{\xP@coor\X@p\Y@p m \xP@coor\X@c\Y@c l}\fi
}}
\newcommand*\xP@setdashpat{\xP@testcont\xP@dashmacro
\ifxP@splinecont
{\count@\numexpr2*((\@tempdimb-\xydashl@/3)/(2*\xydashl@))\relax
\global\dimen@i
\ifnum\count@>\z@
\dimexpr\@tempdimb/\count@\relax
\else
\z@
\fi
}\@tempdima\dimen@i
\edef\xP@pattern{1 J 1 j [\ifdim\@tempdima>\z@
\xP@precdim\@tempdima]\xP@precdim\@tempdima
\else
]0 \fi
d}\else
\@tempdima
\ifdim\@tempdimb>\xydashl@
\dimexpr\@tempdimb/(2*((\@tempdimb+\xydashl@)/(2*\xydashl@))-1)\relax
\else
\z@
\fi
\edef\xP@pattern{1 J 1 j [\ifdim\@tempdima>\z@\xP@precdim\@tempdima\fi
]0 d}\fi
\global\let\xP@lastpattern\xP@dashmacro
}
\newcommand*\xP@setcldashpat{{\count@\numexpr2*((\@tempdimb-\xydashl@/3)/(2*\xydashl@))\relax
\xdef\@gtempa{1 J 1 j [\ifnum\count@>\z@\xP@precdim{\@tempdimb/\count@}\fi]\ifnum\count@>\z@\xP@precdim{\@tempdimb*3/2/\count@}\else0 \fi d}}\edef\xP@pattern{\@gtempa}}
\xP@hook{pdf}{point@}
\newcommand*\xP@point@{\xP@zerodot\egroup\Invisible@false
\Hidden@false\def\Leftness@{.5}\def\U@pness@{.5}\ctipEdge@
\def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\xP@dottedSpread}}
\newcommand*\xP@zerodot{\hb@xt@\z@{\hss
\vbox to\z@{\vss\hrule\@width\xP@preclw\@height\xP@preclw\vss}\hss}}
\@ifdefinable\xP@dottedSpread\relax
\def\xP@dottedSpread#1\repeat@{{\xP@veclen
\ifdim\@tempdimb>\z@
\xP@setdottedpat
\xP@savec
\xP@stroke{\xP@coor\X@p\Y@p m \xP@coor\X@c\Y@c l}\fi
}}
\newcommand*\xP@setdottedpat{\xP@testcont\xP@dotmacro
\ifxP@splinecont
\@tempdima\dimexpr\@tempdimb/(\@tempdimb/131072+1)-\xP@preclw\relax
\edef\xP@pattern{0 J [\ifdim\@tempdima>\z@
\xP@precdim\xP@preclw\xP@precdim\@tempdima
\fi
]\xP@precdim{\xP@preclw+1sp}d}\else
\advance\@tempdimb-\xP@preclw
\ifdim\@tempdimb<\z@\@tempdimb\z@\fi
\@tempdima\dimexpr\@tempdimb/(\@tempdimb/131072+1)-\xP@preclw\relax
\edef\xP@pattern{0 J [\ifdim\@tempdima>\z@
\xP@precdim\xP@preclw\xP@precdim\@tempdima
\fi
]0 d}\fi
\global\let\xP@lastpattern\xP@dotmacro
}
\newcommand*\xP@setcldottedpat{\@tempdima\dimexpr\@tempdimb/(\@tempdimb/131072+1)-\xP@preclw\relax
\edef\xP@pattern{0 J [\ifdim\@tempdima>\z@
\xP@precdim\xP@preclw\xP@precdim\@tempdima
\fi
]\xP@precdim{\dimexpr\xP@preclw+\@tempdima/2\relax}d}}
\newcommand*\xP@abs[1]{\ifdim#1<\z@\multiply#1\m@ne\fi}
\newcommand*\xP@ifabsless[2]{\ifpdfabsdim#1<#2}
\ifx\ifpdfabsdim\@undefined
\renewcommand*\xP@ifabsless[2]{\ifdim\ifdim#1<\z@-\fi#1<\ifdim#2<\z@-\fi#2}
\@gobble\fi
\fi
\newcommand*\xP@swapdim[2]{\@tempdima#1#1#2#2\@tempdima}
\newcommand*\xP@swapnum[2]{\@tempcnta#1#1#2#2\@tempcnta}
\newcommand*\xP@min[2]{\ifdim#1<#2#1\else#2\fi}
\newcommand*\xP@max[2]{\ifdim#1>#2#1\else#2\fi}
\newcommand*\xP@Max[2]{#1\ifdim#2<\z@\xP@max#1{-#2}\else\xP@max#1#2\fi}
\newcommand*\xP@sqrt{\loop
\@tempdimb\dimexpr(\@tempdimc+(\@tempdima*\p@/\@tempdimc))/2\relax
\unless\ifdim\@tempdimc=\@tempdimb
\@tempdimc\@tempdimb\relax
\repeat
}
\newcommand*\xP@veclen{{\xP@veclen@
\global\dimen@i\@tempdimb
}\@tempdimb\dimen@i
}
\newcommand*\xP@veclen@{\xP@abs\d@Y
\ifdim\d@X=\z@
\@tempdimb\d@Y
\else
\xP@abs\d@X
\ifdim\d@Y=\z@
\@tempdimb\d@X
\else
\@tempswatrue
\ifdim\d@X>5931641sp\relax\@tempswafalse\fi
\ifdim\d@Y>5931641sp\relax\@tempswafalse\fi
\if@tempswa
\count@\@ne
\loop
\@tempdima\dimexpr\d@X*\d@X/\p@+\d@Y*\d@Y/\p@\relax
\ifdim\@tempdima<4096pt
\@tempcnta\ifdim\@tempdima<1024pt\ifdim\@tempdima<256pt8\else4\fi\else\tw@\fi
\multiply\d@X\@tempcnta
\multiply\d@Y\@tempcnta
\multiply\count@\@tempcnta
\repeat
\@tempdimc\dimexpr(\d@X+\d@Y)*3/4\relax
\xP@sqrt
\@tempdimb\dimexpr\@tempdimb/\count@\relax
\else
\ifdim\d@X>83042982sp\relax\@tempswatrue\fi
\ifdim\d@Y>83042982sp\relax\@tempswatrue\fi
\if@tempswa
\@tempdima\dimexpr\d@X/182*\d@X/11927552+\d@Y/182*\d@Y/11927552\relax
\@tempdimc\dimexpr(\d@X+\d@Y)*3/728\relax
\xP@sqrt
\multiply\@tempdimb182\relax
\else
\@tempdima\dimexpr\d@X*\d@X/12845056+\d@Y*\d@Y/12845056\relax
\@tempdimc\dimexpr(\d@X+\d@Y)*3/56\relax
\xP@sqrt
\multiply\@tempdimb14\relax
\fi
\fi
\fi
\fi
}
\xP@hook{pdf}{squiggledSpread@}
\@ifdefinable\xP@squiggledSpread@\relax
\def\xP@squiggledSpread@#1\repeat@{{\xP@veclen
\ifdim\@tempdimb>\z@
\edef\@tempa{\xP@coor\X@p\Y@p m }\toks@\expandafter{\@tempa}\@tempcnta\numexpr\@tempdimb/\xybsqll@\relax
\ifnum\@tempcnta<\tw@\@tempcnta\tw@\fi
\@tempdima\dimexpr\d@X/\@tempcnta\relax
\@tempdimc\dimexpr\d@Y/\@tempcnta\relax
\xP@testcont\xP@oddsquigglemacro
\ifxP@splinecont
\def\xP@squigsign{-}\else
\let\xP@squigsign\@empty
\fi
\count@\z@
\loop
\xP@append\toks@{\xP@coor{\X@p+\d@X*\count@/\@tempcnta+(\@tempdima
-\xP@squigsign\ifodd\count@-\fi\@tempdimc)*147546029/534618434}{\Y@p+\d@Y*\count@/\@tempcnta+(\@tempdimc
+\xP@squigsign\ifodd\count@-\fi\@tempdima)*147546029/534618434}}\advance\count@\@ne
\xP@append\toks@{\xP@coor{\X@p+\d@X*\count@/\@tempcnta-(\@tempdima
-\xP@squigsign\ifodd\count@-\fi\@tempdimc)*147546029/534618434}{\Y@p+\d@Y*\count@/\@tempcnta-(\@tempdimc
+\xP@squigsign\ifodd\count@-\fi\@tempdima)*147546029/534618434}\xP@coor{\X@p+\d@X*\count@/\@tempcnta}{\Y@p+\d@Y*\count@/\@tempcnta}c }\ifnum\count@<\@tempcnta
\repeat
\xP@setsolidpat
\global\expandafter\let\expandafter\xP@lastpattern
\ifodd\numexpr\count@\if\xP@squigsign-+1\fi\relax
\xP@oddsquigglemacro
\else
\xP@evensquigglemacro
\fi
\xP@savec
\xP@stroke{\the\toks@}\fi
}}
\newcommand*\xP@squigsign{}
\newcommand*\xP@append[2]{{\edef\@tempa{#1{\the#1#2}}\expandafter}\@tempa
}
\xP@hook{pdf}{circhar@@}
\newcommand*\xP@circhar@@[1]{\expandafter\xP@circhar@@@\ifcase#1 000{-173517671/654249180}{65307479/619869377}{-34221476/65864945}{225058681/768398401}{-543339720/768398401}\or
0{-543339720/768398401}{181455824/967576667}{-554561898/619869377}{826676217/1870772527}{-1}{543339720/768398401}{-1}\or
0{-1}{173517671/654249180}{-1}{34221476/65864945}{-554561898/619869377}{543339720/768398401}{-543339720/768398401}\or
0{-543339720/768398401}{181455824/967576667}{-34221476/65864945}{225058681/768398401}{-173517671/654249180}{225058681/768398401}0\or
0{543339720/768398401}{181455824/967576667}{34221476/65864945}{225058681/768398401}{173517671/654249180}{225058681/768398401}0\or
01{173517671/654249180}1{34221476/65864945}{554561898/619869377}{543339720/768398401}{543339720/768398401}\or
0{543339720/768398401}{181455824/967576667}{554561898/619869377}{826676217/1870772527}1{543339720/768398401}1\or
000{173517671/654249180}{65307479/619869377}{34221476/65864945}{225058681/768398401}{543339720/768398401}\fi}
\newcommand\xP@circhar@@@[8]{\xP@setsolidpat
\xP@stroke{\xP@coor{\R@*#1}{\R@*#2}m
\xP@coor{\R@*#3}{\R@*#4}\xP@coor{\R@*#5}{\R@*#6}\xP@coor{\R@*#7}{\R@*#8}c}\vrule width\z@ height\R@ depth\R@
\kern\dimexpr\R@*#7\relax
}
\xP@hook{pdf}{cirrestrict@@}
\newcommand*\xP@cirrestrict@@{\count@\z@\relax}
\newcommand*\xP@trigfromdir[1]{{\Direction#1\relax
\count@-\Direction
\advance\count@4096
\divide\count@2048
\ifcase\count@
\d@X\K@\p@
\d@Y\numexpr\Direction-3*\K@\relax\p@
\or
\d@X\numexpr\Direction-\K@\relax\p@
\d@Y-\K@\p@
\or
\d@X-\K@\p@
\d@Y\numexpr-\Direction-\K@\relax\p@
\or
\d@X\numexpr-\Direction-3*\K@\relax\p@
\d@Y\K@\p@
\else
\PackageError{xypdf}{Unexpected case in direction calculation}{Feel free to contact the author of the xypdf package with a minimal example.}\fi
\xP@veclen
\xdef\@gtempa{\def\noexpand\cosDirection{\xP@EARPT\dimexpr\d@X*\p@/\@tempdimb\relax}\def\noexpand\sinDirection{\xP@EARPT\dimexpr\d@Y*\p@/\@tempdimb\relax}}}\@gtempa
}
\outer\def\@tempa{\alloc@1\dimen\dimendef\insc@unt}
\let\xP@newdimen\newdimen
\ifx\newdimen\@tempa
\def\xP@newdimen{\alloc@1\dimen\dimendef\insc@unt}
\fi
\outer\def\@tempa#1{\count@=\escapechar\escapechar=-1
\expandafter\expandafter\expandafter
\def\@if#1{true}{\let#1=\iftrue}\expandafter\expandafter\expandafter
\def\@if#1{false}{\let#1=\iffalse}\@if#1{false}\escapechar=\count@}
\let\@tempa\relax
\newcommand*\xP@lastX{}
\newcommand*\xP@lastY{}
\newcommand*\xP@lastpattern{}
\newcommand*\xP@solidmacro{solid}
\newcommand*\xP@dotmacro{dot}
\newcommand*\xP@dashmacro{dash}
\newcommand*\xP@evensquigglemacro{evensquiggle}
\newcommand*\xP@oddsquigglemacro{oddsquiggle}
\newcommand*\xP@brokensquigglemacro{brokensquiggle}
\renewcommand*\xyinside@{\global\let\xP@lastpattern\@empty
\saveXyStyle@ \aftergroup\xycheck@end
\setboxz@h\bgroup
\plainxy@
\X@c=\z@\Y@c=\z@\czeroEdge@
\X@p=\z@\Y@p=\z@\U@p=\z@\D@p=\z@\L@p=\z@\R@p=\z@\Edge@p={\zeroEdge}\X@min=\hsize\X@max=-\hsize\Y@min=\hsize\Y@max=-\hsize
\mathsurround=\z@
\expandafter\POS\everyxy@@
}
\newcommand*\xP@savec{\xdef\xP@lastX{\the\X@c}\xdef\xP@lastY{\the\Y@c}}
\@ifdefinable\ifxP@splinecont\relax
\@ifdefinable\xP@splineconttrue\relax
\@ifdefinable\xP@splinecontfalse\relax
\newif\ifxP@splinecont
\newcommand*\xP@testcont[1]{\xP@splinecontfalse
\ifxP@cont
\ifx\xP@lastpattern#1\ifdim\xP@lastX=\X@p
\ifdim\xP@lastY=\Y@p
\xP@splineconttrue
\fi
\fi
\fi
\fi
}
\@ifdefinable\ifxP@cont\relax
\@ifdefinable\xP@conttrue\relax
\@ifdefinable\xP@contfalse\relax
\newif\ifxP@cont
\newcommand*\xypdfcontpatternon{\xP@conttrue}
\newcommand*\xypdfcontpatternoff{\xP@contfalse}
\xP@conttrue
\let\@tempa\@undefined
\let\nextii@\@undefined
\DN@{\xywithoption{color}{\message{Xy-pic pdf driver: `color' extension support}\@ifundefined{xypdf-co@loaded}{\input xypdf-co\relax}{\message{not reloaded}}}\xywithoption{curve}{\message{Xy-pic pdf driver: `curve' extension support}\@ifundefined{xypdf-cu@loaded}{\input xypdf-cu\relax}{\message{not reloaded}}}\xywithoption{frame}{\message{Xy-pic pdf driver: `frame' extension support}\@ifundefined{xypdf-fr@loaded}{\input xypdf-fr\relax}{\message{not reloaded}}}\xywithoption{line}{\message{Xy-pic pdf driver: `line' extension support}\@ifundefined{xypdf-li@loaded}{\input xypdf-li\relax}{\message{not reloaded}}}\xywithoption{rotate}{\message{Xy-pic pdf driver: `rotate' extension support}\@ifundefined{xypdf-ro@loaded}{\input xypdf-ro\relax}{\message{not reloaded}}}}
\next@
\xyendinput
%%
%% End of file `xypdf.tex'.


==> xypic.tex <==
%% xypic.tex from $Id: xypic.doc,v 3.6 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic v2 compatibility loading.
%% Copyright (c) 1993-1996 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\input xyv2
\endinput


==> xypicture.tex <==
%% xypicture.tex from $Id: xypicture.doc,v 3.6 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``LaTeX Picture Mode'' option.
%% Copyright (c) 199802011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-1998 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{picture}{LaTeX Picture extension}{\stripRCS$Revision: 3.6 $}%
 {Kristoffer H.~Rose}{krisrose@tug.org}%
 {IBM T.J.Watson Research Center, P.O.Box 704, Yorktown Heights, NY 10598, USA}
\xynew@{dimen}\xyp@xsize
\xynew@{dimen}\xyp@ysize
\xylet@\xyp@arrow=\relax
{\xyuncatcodes\makeatletter
 \gdef\xyp@tail{}
 \gdef\xyp@mid{-}
 \gdef\xyp@head{>}
}
\xydef@\xyvector(#1,#2)#3{%
 \xyp@xsize#3\relax
 \ifnum#1<\z@\multiply\xyp@xsize\m@ne\fi
 \xyp@ysize\xyp@xsize\relax
 \ifnum#1=\z@
 \xyp@xsize\z@
 \ifnum#2<\z@\multiply\xyp@ysize\m@ne\fi
 \else
 \multiply\xyp@ysize#2\relax\divide\xyp@ysize#1\relax
 \fi
 \edef\xyp@arrow{\noexpand\arAT{\xyp@tail\xyp@mid\xyp@head}}%
 \ifnum#1<\z@
 \makebox(\xyp@xsize,\xyp@ysize){%
 \begin{xy} 0;<\unitlength,\z@>:%
 \xyp@arrow(\xyp@xsize,\xyp@ysize)
 \end{xy}}%
 \else
 \xyp@arrow(\xyp@xsize,\xyp@ysize)\relax
 \fi
}
\xyendinput


==> xypoly.tex <==
%% xypoly.tex from $Id: xypoly.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Polygon'' feature.
%% Copyright (c) 1994-1997 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this macro package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{poly}{Polygon feature}{\stripRCS$Revision: 3.11 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xyrequire{arrow}\xycatcodes
\message{polygons,}
\xynew@{count}\xypolynode@\xypolynode@=\m@ne
\xydef@\xypolynode{\the\xypolynode@}
\xydef@\xypolyNUMSIDES@{}
\xydef@\xypolynum{\xypolyNUMSIDES@}
\xydef@\xypolygon{\xypoly@}%
\xydef@\xypoly@{%
 \if\inxy@ 
 \if\inxypoly@
 \edef\next@{\noexpand\xy@@{\noexpand\nter@{\xypolynode@=\the\xypolynode@
 \noexpand\def\noexpand\xypolyNUMSIDES@{\xypolyNUMSIDES@}}}}%
 \else
 \DN@{\xy@@{\def\inxypoly@{TT}%
 \nter@{\def\inxypoly@{TF}\xypolynode@=\m@ne}}}%
 \fi
 \else
 \if\inxypoly@
 \edef\next@{\noexpand\xy 
 \noexpand\xy@@{\noexpand\nter@{\xypolyside=\the\xypolyside
 \noexpand\def\noexpand\xypolyNUMSIDES@{\xypolyNUMSIDES@}\endxy}}}%
 \else
 \DN@{\xy \xy@@{\def\inxypoly@{TT}%
 \nter@{\def\inxypoly@{TF}\xypolynode@=\m@ne \endxy}}}%
 \fi
 \fi
 \next@ \count@=\z@ \xyFN@\xypoly@n}
\xydef@\inxypoly@{TF}%
\xydef@\xypoly@x{\xy@@{\leave@\leave@}}
\xydef@\xypoly@n{%
 \DN@##1{\multiply\count@10\relax \advance\count@##1\relax \xyFN@\xypoly@n}%
 \ifx \space@\next
 \ifnum\count@>\z@ \expandafter\DN@\space@{\xyFN@\xypoly@i}%
 \else \expandafter\DN@\space@{\xyFN@\xypoly@n}\fi
 \else\ifx 0\next \else\ifx 1\next \else\ifx 2\next \else\ifx 3\next
 \else\ifx 4\next \else\ifx 5\next \else\ifx 6\next \else\ifx 7\next
 \else\ifx 8\next \else\ifx 9\next
 \else \let\next@=\xypoly@i \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi \next@}
\xydef@\xypoly@i{\edef\xypolyNUMSIDES@{\the\count@}\xyFN@\xygetpolyprefix@}
\xydef@\xypolyPREFIX@{}%
\xydef@\xypolyPREFIX@@{}%
\xydef@\xypolyname{\xypolyPREFIX@}%
\xydef@\xygetpolyprefix@{%
 \ifx\next"\DN@"##1"{\def\xypolyPREFIX@@{##1}\expandafter
 \edef\csname\xypolyPREFIX@@ NUMSIDES\endcsname{\xypolyNUMSIDES@}%
 \xypolyprefix@@ }%
 \else 
 \ifnum\xypolynode@<\z@\def\xypolyPREFIX@@{}%
 \else
 \edef\xypolyPREFIX@@{\xypolyPREFIX@\the\xypolynode@,}%
 \fi \DN@{\xypolyprefix@@}%
 \fi \next@ }
\xydef@\xypolyprefix@@{%
 \expandafter\toks@\expandafter{\addEQ@\POS"}%
 \expandafter\addtotoks@\expandafter{\xypolyPREFIX@@0"\relax}%
 \the\toks@ 
 \ifnum\xypolynode@<\z@
 \expandafter\def\expandafter\xypolyPREFIX@\expandafter{\xypolyPREFIX@@}%
 \xy@@{\enter@{\xypolynode@=\the\xypolynode@
 \noexpand\def\noexpand\xypolyPREFIX@{\xypolyPREFIX@}}\xypolynode@=\z@ }%
 \else
 \xy@@{\enter@{\xypolynode@=\the\xypolynode@
 \noexpand\def\noexpand\xypolyPREFIX@{\xypolyPREFIX@}}\xypolynode@=\z@ }%
 \expandafter\def\expandafter\xypolyPREFIX@\expandafter{\xypolyPREFIX@@}%
 \fi
 \xypoly@@i }
\xydef@\xypoly@@i#1#{\begingroup
 \DN@{#1}\ifx\next@\empty\else
 \xywarning@{discarding unused tokens: #1}\fi \xypoly@@ }
\xydef@\xypoly@@#1{\xypolydefaults@
 \DN@{#1}\ifx\next@\empty\DN@{\xypoly@@@}%
 \else \DN@{\xyFN@\xypolyparams@#1~!}\fi \next@}
\xydef@\xypolydefaults@{\def\xypolySCALE@{}%
 \def\xypolySPOKES@{{}}\def\xypostSPOKES@{}\let\xypreSPOKES@\relax
 \def\xypolySIDES@{{-}}\def\xypostSIDES@{}\let\xypreSIDES@\relax
 \def\xypolyVERTEX@{}\def\xypolyALIGN@{}}
{\xyuncatcodes \gdef\next{*=0}}
\xylet@\xypolynullvertex@=\next
{\xyuncatcodes \gdef\next{*[o]}}
\xylet@\xypolyvertex@=\next
{\xyuncatcodes \gdef\next{*+[o]}}
\xylet@\xypolywidevertex@=\next
\xydef@\xypolyparams@{%
 \ifx\space@\next \expandafter\DN@\space{\xyFN@\xypolyparams@}%
 \else\ifx\next~\DN@~{\xyFN@\xypolywhich@}%
 \else\ifx\next\bgroup\DN@##1~!{%
 \ifx\empty\xypolyVERTEX@\expandafter
 \def\expandafter\xypolyVERTEX@\expandafter{\xypolyvertex@{##1}}%
 \else\xypolyVERTEXerror@{##1}\fi \xypoly@@@}%
 \else\DN@##1~!{\DN@{##1}\ifx\next@\empty\else
 \ifx\empty\xypolyVERTEX@\def\xypolyVERTEX@{*##1}%
 \expandafter\checkpolytok@\expandafter\xypolyVERTEX@
 \expandafter{\xypolynullvertex@}##1@@!\relax
 \else\xypolyVERTEXerror@{##1}\fi\fi \xypoly@@@}%
 \fi\fi\fi \next@ }
\xydef@\xypolyVERTEXerror@#1{\xywarning@{%
 vertex already specified, discarding unused tokens:#1}}
\xydef@\xypolywhich@{%
 \ifx\next!\DN@!{\xypoly@@@}%
 \else \addLT@\ifx\next \addLT@\DN@{\xyFN@\xypoly@SPOKES@}%
 \else \addGT@\ifx\next \addGT@\DN@{\xyFN@\xypoly@SIDES@}%
 \else \addEQ@\ifx\next \addEQ@\DN@##1{%
 \def\xypolyALIGN@{##1}\xyFN@\xypolyparams@ }%
 \else \ifx :\next \DN@:##1{%
 \def\xypolySCALE@{##1}\xyFN@\xypolyparams@ }%
 \else\ifx\next*\DN@*##1{\expandafter
 \def\expandafter\xypolyVERTEX@\expandafter{\xypolywidevertex@{##1}}%
 \xyFN@\xypolyparams@}%
 \fi\fi\fi\fi\fi\fi \next@ }
\xydef@\xypoly@SPOKES@{%
 \addLT@\ifx\next \addLT@\DN@##1{%
 \def\xypreSPOKES@{##1}\def\xypolySPOKES@{}\xyFN@\xypolyparams@ }%
 \else \addGT@\ifx\next \addGT@\DN@##1{%
 \def\xypostSPOKES@{##1}\xyFN@\xypolyparams@ }%
 \else \ifx\next\bgroup \DN@##1{%
 \def\xypolySPOKES@{##1}\let\xypreSPOKES@\relax
 \checkpolytok@\xypolySPOKES@{}##1@@!{\xyFN@\xypolyparams@}}%
 \else \DN@##1{%
 \let\xypreSPOKES@\relax \def\xypolySPOKES@{{##1}}\xyFN@\xypolyparams@}%
 \fi\fi\fi \next@ }
\xydef@\xypoly@SIDES@{%
 \addLT@\ifx\next \addLT@\DN@##1{%
 \def\xypreSIDES@{##1}\def\xypolySIDES@{}\xyFN@\xypolyparams@ }%
 \else \addGT@\ifx\next \addGT@\DN@ ##1{%
 \def\xypostSIDES@{##1}\xyFN@\xypolyparams@ }%
 \else \ifx\next\bgroup \DN@##1{%
 \def\xypolySIDES@{##1}\let\xypreSIDES@\relax
 \checkpolytok@\xypolySIDES@{}##1@@!{\xyFN@\xypolyparams@}}%
 \else \DN@##1{%
 \let\xypreSIDES@\relax \def\xypolySIDES@{{##1}}\xyFN@\xypolyparams@}%
 \fi\fi\fi \next@ }
\xydef@\checkpolytok@#1#2#3#4@!#5{\DNii@{#1}\DN@{#4}%
 \ifx\next@\empty\expandafter\def\nextii@{{}}%
 \else\ifx#4@\expandafter\def\nextii@{#2{#3}}\fi\fi #5}
\xydef@\xytrigerror@#1#2{\string#1 only works from 0 to 12}
\xydef@\cosPIon#1{\ifcase#1 1\or-1\or0\or.5\or\halfroottwo\or
 .809017\or\halfrootthree\or.900969\or.92388\or.939693\or.951057\or
 .959493\or.965926\else1\xytrigerror@\cosPIon{#1}\fi}
\xydef@\sinPIon#1{\ifcase#1 0\or0\or1\or\halfrootthree\or\halfroottwo\or
 .587785\or.5\or.433884\or.382683\or.34202\or.309017\or
 .281733\or.258819\else0\xytrigerror@\sinPIon{#1}\fi}
\xydef@\cosTwoPIon#1{\ifcase#1 1\or1\or-1\or-\cosPIon3\or\cosPIon2\or
 \sinPIon{10}\or\cosPIon3\or.62349\or\cosPIon4\or
 .766044\or\cosPIon5\or.841254\or\cosPIon6%
 \else1\xytrigerror@\cosTwoPIon{#1}\fi}
\xydef@\sinTwoPIon#1{\ifcase#1 0\or0\or0\or-\sinPIon3\or\sinPIon2\or
 \cosPIon{10}\or\sinPIon3\or.781831\or\sinPIon4\or
 .642788\or\sinPIon5\or.540641\or\sinPIon6%
 \else0\xytrigerror@\sinTwoPIon{#1}\fi}
\xydef@\cosThreePIon#1{\ifcase#1 1\or-1\or0\or-1\or-\cosPIon4\or
 -\cosPIon5\or\cosPIon2\or.222521\or\sinPIon8\or\cosPIon3\or
 \sinTwoPIon5\or.654861\or\cosPIon4%
 \else1\xytrigerror@\cosThreePIon{#1}\fi}
\xydef@\sinThreePIon#1{\ifcase#1 0\or0\or1\or0\or\sinPIon4\or
 \sinTwoPIon5\or\sinPIon2\or.974928\or\cosPIon8\or\sinPIon3\or
 \cosTwoPIon5\or.75575\or\sinPIon4%
 \else0\xytrigerror@\sinThreePIon{#1}\fi}
\xydef@\cosFourPIon#1{\ifcase#1 1\or1\or1\or-\cosPIon3\or-1\or-\cosPIon5\or
 \cosTwoPIon3\or-\cosThreePIon7\or0\or.173648\or\cosTwoPIon5\or
 .415415\or\cosPIon3%
 \else1\xytrigerror@\cosFourPIon{#1}\fi}
\xydef@\sinFourPIon#1{\ifcase#1 0\or0\or0\or-\sinPIon3\or0\or\sinPIon5\or
 \sinTwoPIon3\or\sinThreePIon7\or1\or.984808\or\sinTwoPIon5\or
 .909632\or\sinPIon3%
 \else0\xytrigerror@\sinFourPIon{#1}\fi}
\xydef@\cosFivePIon#1{\ifcase#1 1\or-1\or0\or\cosPIon3\or-\cosPIon4\or
 -1\or-\cosPIon6\or-\cosTwoPIon7\or-\cosThreePIon8\or-\cosFourPIon9\or
 0\or.142315\or\sinPIon{12}%
 \else1\xytrigerror@\cosFivePIon{#1}\fi}
\xydef@\sinFivePIon#1{\ifcase#1 0\or0\or1\or-\sinPIon3\or-\sinPIon4\or
 0\or\sinPIon6\or\sinTwoPIon7\or\sinThreePIon8\or\sinFourPIon9\or1\or
 .989821\or\cosPIon{12}%
 \else0\xytrigerror@\sinFivePIon{#1}\fi}
\xydef@\xypoly@@@{\count@=\xypolyNUMSIDES@\relax
 \ifx\xypolyALIGN@\empty
 \ifnum\count@<\thr@@\relax\DN@{\xypolytoosmall@{\the\count@}}%
 \else \advance\count@-\thr@@
 \ifcase\count@ \DN@{\xyPolygon@@@\xytriangle@@}%
 \or \DN@{\xyPolygon@@@\xysquare@@}%
 \or \DN@{\xyPolygon@@@\xypentagon@@}%
 \or \DN@{\xyPolygon@@@\xyhexagon@@}%
 \or \DN@{\xyPolygon@@@\xyheptagon@@}%
 \or \DN@{\xyPolygon@@@\xyoctagon@@}%
 \or \DN@{\xyPolygon@@@\xynonagon@@}%
 \or \DN@{\xyPolygon@@@\xydecagon@@}%
 \or \DN@{\xyPolygon@@@\xyundecagon@@}%
 \or \DN@{\xyPolygon@@@\xydodecagon@@}%
 \else \DN@{\xylargePolygon@{0}{\xypolyNUMSIDES@}}%
 \fi\fi
 \else 
 \DN@{\xylargePolygon@{\xypolyALIGN@}{\xypolyNUMSIDES@}}%
 \fi \next@ \xypoly@@@x}
\xydef@\xypoly@@@x{\restore\xypoly@x}
\xydef@\xypolytoosmall@#1{\xyerror@{#1 sides is too few for a polygon}}
\xydef@\xyPolygon@@@#1{%
 \toks@={\def\xypolyNUMSIDES@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyNUMSIDES@}\save}%
 \ifx\empty\xypolySCALE@ \addtotoks@{\POS"}%
 \else \addtotoks@{\POS;0;}%
 \expandafter\addtotoks@\expandafter{\xypolySCALE@\relax\POS"}%
 \fi
 \expandafter\addtotoks@\expandafter{\xypolyPREFIX@0"\relax}%
 \ifx\xypreSPOKES@\relax
 \addtotoks@{#1{;}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyVERTEX@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyPREFIX@}}%
 \DN@##1\next@{\def\tmp@{**\dir##1}}%
 \expandafter\next@\expandafter{\xypolySPOKES@}\next@
 \expandafter\addtotoks@\expandafter{\expandafter{\tmp@}}%
 \else
 \expandafter\DN@\expandafter{\expandafter\ar\xypreSPOKES@}%
 \addtotoks@{#1}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyVERTEX@}}%
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyPREFIX@}{}}%
 \fi
 \expandafter\addtotoks@\expandafter{\expandafter{\xypostSPOKES@}}%
 \ifx\xypreSIDES@\relax
 \addtotoks@{{;}}%
 \DN@##1\next@{\def\tmp@{**\dir##1}}%
 \expandafter\next@\expandafter{\xypolySIDES@}\next@
 \expandafter\addtotoks@\expandafter{\expandafter{\tmp@}}%
 \else
 \expandafter\DN@\expandafter{\expandafter\ar\xypreSIDES@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\next@}{}}%
 \fi
 \expandafter\addtotoks@\expandafter{\expandafter{\xypostSIDES@}}%
 \ifx\xypolyALIGN@\empty
 \ifnum\xypolyNUMSIDES@>12\addtotoks@{{0}}\fi
 \else
 \expandafter\addtotoks@\expandafter{\expandafter{\xypolyALIGN@}}%
 \fi
 \expandafter\DN@\expandafter{\expandafter\endgroup\the\toks@ }%
 \next@}
\xydef@\xytriangle@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(0,1)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(-\cosPIon6, -.5)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\cosPIon6,-.5)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#33"#6"#31"#7#8\relax }
\xydef@\xysquare@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\halfroottwo,\halfroottwo)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(-\halfroottwo,\halfroottwo)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\halfroottwo,\halfroottwo)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(-\halfroottwo,\halfroottwo)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#34"#6"#31"#7#8\relax }
\xydef@\xypentagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\cosPIon{10},\sinPIon{10})#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(0,1)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\cosPIon{10},\sinPIon{10})#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon5,\cosPIon5)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon5,-\cosPIon5)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#35"#6"#31"#7#8\relax }
\xydef@\xyhexagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(1,0)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(.5,\halfrootthree)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-.5,\halfrootthree)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(1,0)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(.5,\halfrootthree)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(-.5,\halfrootthree)#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#36"#6"#31"#7#8\relax }
\xydef@\xyheptagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\sinTwoPIon7,\cosTwoPIon7)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(0,1)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\sinTwoPIon7,\cosTwoPIon7)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinThreePIon7,\cosThreePIon7)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon7,\cosPIon7)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon7,-\cosPIon7)#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinThreePIon7,-\cosThreePIon7)#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#37"#6"#31"#7#8\relax }
\xydef@\xyoctagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\cosPIon8,\sinPIon8)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(\sinPIon8,\cosPIon8)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon8,-\cosPIon8)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon8,-\sinPIon8)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon8,\sinPIon8)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon8,\cosPIon8)#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon8,-\cosPIon8)#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\cosPIon8,-\sinPIon8)#2="#38"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#37"#6"#38"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#38"#6"#31"#7#8\relax }
\xydef@\xynonagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\sinFourPIon9,\cosFourPIon9)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(\sinTwoPIon9,\cosTwoPIon9)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(0,1)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\sinTwoPIon9,\cosTwoPIon9)#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\sinFourPIon9,\cosFourPIon9)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon6,\sinPIon6)#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon9,\cosPIon9)#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon9,-\cosPIon9)#2="#38"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#37"#6"#38"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\cosPIon6,-\sinPIon6)#2="#39"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#38"#6"#39"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#39"#6"#31"#7#8\relax }
\xydef@\xydecagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(1,0)#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(\cosPIon5,\sinPIon5)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon{10},\cosPIon{10})#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon{10},-\cosPIon{10})#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon5,-\sinPIon5)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(1,0)#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon5,\sinPIon5)#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon{10},\cosPIon{10})#2="#38"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#37"#6"#38"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon{10},-\cosPIon{10})#2="#39"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#38"#6"#39"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\cosPIon5,-\sinPIon5)#2="#310"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#39"#6"#310"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#310"#6"#31"#7#8\relax }
\xydef@\xyundecagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\sinFourPIon{11},\cosFourPIon{11})#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(\sinTwoPIon{11},\cosTwoPIon{11})#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(0,1)#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\sinTwoPIon{11},\cosTwoPIon{11})#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(-\sinFourPIon{11},\cosFourPIon{11})#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinFivePIon{11},\cosFivePIon{11})#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinThreePIon{11},\cosThreePIon{11})#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon{11},\cosPIon{11})#2="#38"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#37"#6"#38"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon{11},-\cosPIon{11})#2="#39"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#38"#6"#39"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinThreePIon{11},-\cosThreePIon{11})#2="#310"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#39"#6"#310"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinFivePIon{11},-\cosFivePIon{11})#2="#311"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#310"#6"#311"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#311"#6"#31"#7#8\relax }
\xydef@\xydodecagon@@#1#2#3#4#5#6#7#8{%
 \xy@@{\xypolynode@=\@ne}%
 \POS#1"#30"+(\cosPIon{12},\sinPIon{12})#2="#31"#4#5\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#30"#1"#30"+(\halfroottwo,\halfroottwo)#2="#32"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#31"#6"#32"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon{12},\cosPIon{12})#2="#33"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#32"#6"#33"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon{12},-\cosPIon{12})#2="#34"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#33"#6"#34"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\halfroottwo,-\halfroottwo)#2="#35"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#34"#6"#35"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon{12},-\sinPIon{12})#2="#36"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#35"#6"#36"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\cosPIon{12},\sinPIon{12})#2="#37"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#36"#6"#37"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\halfroottwo,\halfroottwo)#2="#38"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#37"#6"#38"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"-(\sinPIon{12},\cosPIon{12})#2="#39"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#38"#6"#39"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\sinPIon{12},-\cosPIon{12})#2="#310"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#39"#6"#310"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\halfroottwo,-\halfroottwo)#2="#311"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#310"#6"#311"#7#8\relax
 \xy@@{\advance\xypolynode@\tw@}%
 \POS"#30"#1"#30"+(\cosPIon{12},-\sinPIon{12})#2="#312"#4#5\relax
 \xy@@{\advance\xypolynode@\m@ne}%
 \POS"#311"#6"#312"#7#8\relax
 \xy@@{\advance\xypolynode@\@ne}%
 \POS"#312"#6"#31"#7#8\relax }
\xydef@\xylargePolygon@#1#2{%
 \dimen@=#1\p@
 \xyPolygon@@@\xypolygon@@}
\xydef@\xypolyrepeat@{\fi}
\xydef@\xypolybody@{}
\xydef@\xypolyiterate@{\xypolybody@\expandafter\xypolyiterate@\else\fi}
\xydef@\xypolyloop@#1\xypolyrepeat@{\def\xypolybody@{#1}\xypolyiterate@}
\xydef@\xypolygon@@#1#2#3#4#5#6#7#8#9{\save
 \vfromcartesianangle@{#9}\edef\next@{\the\X@c,\the\Y@c\addGT@\empty}%
 \xy@@{\xypolynode@=\@ne}%
 \toks@={\POS#1"#30"+}%
 \expandafter\expandafter\expandafter\addtotoks@\expandafter
 \expandafter\expandafter{\addLT@\empty}%
 \expandafter\addtotoks@\expandafter{\next@#2="#31"#4#5\relax}%
 \xy@@\dontleave@ \the\toks@
 \xypolyloop@
 \dimen@=360\p@ \count@@=\xypolyNUMSIDES@\relax \advance\dimen@ .5\count@@
 \divide\dimen@ \xypolyNUMSIDES@ \relax 
 \multiply\dimen@\xypolynode@ \relax \advance\dimen@ #9\p@ 
 \edef\tmp@{%
 \noexpand\vfromcartesianangle@{\expandafter\removePT@\the\dimen@}}%
 \tmp@ \edef\next@{\the\X@c,\the\Y@c\addGT@\empty}%
 \xy@@{\advance\xypolynode@\@ne}\count@=\xypolynode@
 \toks@={\POS"#30"#1"#30"+}\edef\nextii@{\the\count@}%
 \expandafter\expandafter\expandafter\addtotoks@\expandafter
 \expandafter\expandafter{\addLT@\space}%
 \expandafter\addtotoks@\expandafter{\next@#2="#3}%
 \expandafter\addtotoks@\expandafter{\nextii@"#4#5\relax}%
 \the\toks@ 
 \count@=\xypolynode@ \xy@@{\advance\xypolynode@\m@ne}%
 \toks@={\POS"#3}\expandafter\addtotoks@\expandafter{\the\xypolynode@"#6"#3}%
 \expandafter\addtotoks@\expandafter{\the\count@"#7#8\relax}%
 \the\toks@
 \xy@@{\advance\xypolynode@\@ne}\count@=\xypolyNUMSIDES@ \relax
 \ifnum\xypolynode@<\count@ \relax \xypolyrepeat@
 \toks@={\POS"#3}%
 \expandafter\addtotoks@\expandafter{\xypolyNUMSIDES@"#6"#31"#7#8\relax}%
 \the\toks@ \restore }
\xyendinput


==> xyps-c.tex <==
%% xyps-c.tex from $Id: xyps-c.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Colour extension'' PostScript backend support.
%% Copyright (c) 1993-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-cloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-cloaded\endcsname=\empty \xycatcodes
\expandafter\ifx \csname xyps-sloaded\endcsname\empty\else
 \xyinputorelse@{xyps-s}{\xyerror@{Could not load xyps-s}{}}%
 \xycatcodes\fi
\xydef@\UsePScolor{\installPScolor@}
\xydef@\NoPScolor{\UnloadColor@}
\xydef@\installPScolor@{\installPSstyle@
 \let\xymath@=\xyPSmath@ \let\xynomath@=\xyPSnomath@
 \let\checkxyPScolor@=\checkxyPScolor@@
 \let\xycolor@@=\xyPScolor@@
 \xystandardcolors@ 
 \xyuncatcodes }
\xydef@\xyPSmath@{\hbox\bgroup\dimen@=.55ex \checkxyPScolor@ \xyinside@}
\xydef@\xyPSnomath@{\hbox\bgroup\dimen@=\z@ \checkxyPScolor@ \xyinside@}
\xydef@\checkxyPScolor@@{\xycolor@raw@@{}\let\checkxyPScolor@=\relax}
\xylet@\checkxyPScolor@=\relax
\xydef@\xyPSnewcolor@#1#2#3#4#5{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@\newxycolor{#1}{}\relax\fi
 \DNii@{#4}\ifx\nextii@\empty
 \expandafter\DNii@\expandafter{\csname xyPSshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPScolor@{#2 #3}}\else
 \expandafter\DNii@\expandafter{\csname xyPSshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPScolor@{#4}}\fi
 \ifx\nextii@\empty\expandafter\def\next@{\xyPSnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}\expandafter\tmp@\fi }
\xydef@\xyPScolor@{\ifPSspecials@\expandafter\xyPScolor@@
 \else\expandafter\eat@\fi}
\xydef@\xyPScolor@@#1{\bgroup \checkXyStyle@ 
 \def\preStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPSpre@}}%
 \def\postStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPSpost@}}%
 \let\modPSboxz@=\modXYstyle@ \xyPS@color@@{#1}%
 \toks@={\egroup\let\xy@style@=\relax \def\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Drop@@}\def\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Connect@@}}%
 \the\toks@ }
\xydef@\xyPS@color@@#1{\xyPSsplitPS@{{#1}cc}{}}
\xydef@\xycolor@raw@@#1{\PSraw@@{xyc}}
\endinput


==> xyps-col.tex <==
%% xyps-col.tex from $Id: xyps-col.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Crayola colour names'' PostScript colour support.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyrequire{color}\xycatcodes
\newxycolor@{GreenYellow}{0.15 0 0.69 0}{cmyk}{}{}%
\newxycolor@{Yellow}{0 0 1. 0}{cmyk}{}{}%
\newxycolor@{Goldenrod}{0 0.10 0.84 0}{cmyk}{}{}%
\newxycolor@{Dandelion}{0 0.29 0.84 0}{cmyk}{}{}%
\newxycolor@{Apricot}{0 0.32 0.52 0}{cmyk}{}{}%
\newxycolor@{Peach}{0 0.50 0.70 0}{cmyk}{}{}%
\newxycolor@{Melon}{0 0.46 0.50 0}{cmyk}{}{}%
\newxycolor@{YellowOrange}{0 0.42 1. 0}{cmyk}{}{}%
\newxycolor@{Orange}{0 0.61. 0.87 0}{cmyk}{}{}%
\newxycolor@{BurntOrange}{0 0.51 1. 0}{cmyk}{}{}%
\newxycolor@{Bittersweet}{0 0.75 1. 0.24}{cmyk}{}{}%
\newxycolor@{RedOrange}{0 0.77 0.87 0}{cmyk}{}{}%
\newxycolor@{Mahogany}{0 0.85 0.87 0.35}{cmyk}{}{}%
\newxycolor@{Maroon}{0 0.87 0.68 0.32}{cmyk}{}{}%
\newxycolor@{BrickRed}{0 0.89 0.94 0.28}{cmyk}{}{}%
\newxycolor@{Red}{0 1. 1. 0}{cmyk}{}{}%
\newxycolor@{OrangeRed}{0 1. 0.50 0}{cmyk}{}{}%
\newxycolor@{RubineRed}{0 1. 0.13 0}{cmyk}{}{}%
\newxycolor@{WildStrawberry}{0 0.96 0.39 0}{cmyk}{}{}%
\newxycolor@{Salmon}{0 0.53 0.38 0}{cmyk}{}{}%
\newxycolor@{CarnationPink}{0 0.63 0 0}{cmyk}{}{}%
\newxycolor@{Magenta}{0 1. 0 0}{cmyk}{}{}%
\newxycolor@{VioletRed}{0 0.81 0 0}{cmyk}{}{}%
\newxycolor@{Rhodamine}{0 0.82 0 0}{cmyk}{}{}%
\newxycolor@{Mulberry}{0.34 0.90 0 0.02}{cmyk}{}{}%
\newxycolor@{RedViolet}{0.07 0.90 0 0.34}{cmyk}{}{}%
\newxycolor@{Fuchsia}{0.47 0.91 0 0.08}{cmyk}{}{}%
\newxycolor@{Lavender}{0 0.48 0 0}{cmyk}{}{}%
\newxycolor@{Thistle}{0.12 0.59 0 0}{cmyk}{}{}%
\newxycolor@{Orchid}{0.32 0.64 0 0}{cmyk}{}{}%
\newxycolor@{DarkOrchid}{0.40 0.80 0.20 0}{cmyk}{}{}%
\newxycolor@{Purple}{0.45 0.86 0 0}{cmyk}{}{}%
\newxycolor@{Plum}{0.50 1. 0 0}{cmyk}{}{}%
\newxycolor@{Violet}{0.79 0.88 0 0}{cmyk}{}{}%
\newxycolor@{RoyalPurple}{0.75 0.90 0 0}{cmyk}{}{}%
\newxycolor@{BlueViolet}{0.86 0.91 0 0.04}{cmyk}{}{}%
\newxycolor@{Periwinkle}{0.57 0.55 0 0}{cmyk}{}{}%
\newxycolor@{CadetBlue}{0.62 0.57 0.23 0}{cmyk}{}{}%
\newxycolor@{CornflowerBlue}{0.65 0.13 0 0}{cmyk}{}{}%
\newxycolor@{MidnightBlue}{0.98 0.13 0 0.43}{cmyk}{}{}%
\newxycolor@{NavyBlue}{0.94 0.54 0 0}{cmyk}{}{}%
\newxycolor@{RoyalBlue}{1. 0.50 0 0}{cmyk}{}{}%
\newxycolor@{Blue}{1. 1. 0 0}{cmyk}{}{}%
\newxycolor@{Cerulean}{0.94 0.11 0 0}{cmyk}{}{}%
\newxycolor@{Cyan}{1. 0 0 0}{cmyk}{}{}%
\newxycolor@{ProcessBlue}{0.96 0 0 0}{cmyk}{}{}%
\newxycolor@{SkyBlue}{0.62 0 0.12 0}{cmyk}{}{}%
\newxycolor@{Turquoise}{0.85 0 0.20 0}{cmyk}{}{}%
\newxycolor@{TealBlue}{0.86 0 0.34 0.02}{cmyk}{}{}%
\newxycolor@{Aquamarine}{0.82 0 0.30 0}{cmyk}{}{}%
\newxycolor@{BlueGreen}{0.85 0 0.33 0}{cmyk}{}{}%
\newxycolor@{Emerald}{1. 0 0.50 0}{cmyk}{}{}%
\newxycolor@{JungleGreen}{0.99 0 0.52 0}{cmyk}{}{}%
\newxycolor@{SeaGreen}{0.69 0 0.50 0}{cmyk}{}{}%
\newxycolor@{Green}{1. 0 1. 0}{cmyk}{}{}%
\newxycolor@{ForestGreen}{0.91 0 0.88 0.12}{cmyk}{}{}%
\newxycolor@{PineGreen}{0.92 0 0.59 0.25}{cmyk}{}{}%
\newxycolor@{LimeGreen}{0.50 0 1. 0}{cmyk}{}{}%
\newxycolor@{YellowGreen}{0.44 0 0.74 0}{cmyk}{}{}%
\newxycolor@{SpringGreen}{0.26 0 0.76 0}{cmyk}{}{}%
\newxycolor@{OliveGreen}{0.64 0 0.95 0.40}{cmyk}{}{}%
\newxycolor@{RawSienna}{0 0.72 1. 0.45}{cmyk}{}{}%
\newxycolor@{Sepia}{0 0.83 1. 0.70}{cmyk}{}{}%
\newxycolor@{Brown}{0 0.81 1. 0.60}{cmyk}{}{}%
\newxycolor@{Tan}{0.14 0.42 0.56 0}{cmyk}{}{}%
\newxycolor@{Gray}{0 0 0 0.50}{cmyk}{}{}%
\newxycolor@{Black}{0 0 0 1.}{cmyk}{}{}%
\newxycolor@{White}{0 0 0 0}{cmyk}{}{}%
\endinput


==> xyps-f.tex <==
%% xyps-f.tex from $Id: xyps-f.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Frame extension'' PostScript backend support.
%% Copyright (c) 1995-1997 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-floaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-floaded\endcsname=\empty \xycatcodes
\xydef@\installPSframes@{%
 \let\framed@body@@=\xyPSframed@body@
 \let\circled@x@@=\xyPScircled@x@
 \let\ellipsed@x@@=\xyPSellipsed@x@
 \installPSfills@
 \xyuncatcodes}
\xydef@\UsePSframes{\installPSframes@}
\xydef@\NoPSframes{\UnloadFrames@}
\xydef@\xyPSframed@body@{\DN@{\framed@body@}%
 \ifx\framehfill\frm@solidh@@
 \DN@{\xyPSframed@oval@\xyPSoval@Special}%
 \else\ifdim\R@=\z@\else
 \ifx\framehfill\frm@dashh@@
 \DN@{\xyPSframed@oval@\xyPSdashoval@Special}%
 \else\ifx\framehfill\frm@doth@@
 \DN@{\xyPSframed@oval@\xyPSdotoval@Special}%
 \fi\fi
 \fi\fi \next@ }
\xydef@\xyPSframed@oval@#1{\vglue\U@c
 \hbox{\hglue\L@c\xypsoval@#1\hglue\R@c}\vglue\D@c}
\xydef@\xyPScircled@x@{\DN@{\xyPScircled@x@@\xyPScirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPScircled@x@@\xyPSdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPScircled@x@@\xyPSdashcirc@Special}%
 \fi\fi \next@ }
\xydef@\xyPScircled@x@@#1{\vglue2\R@
 \hbox{\hglue2\R@\xypscircle@#1\hglue2\R@}%
 \vglue2\R@}
\xydef@\xyPSellipsed@x@#1#2{%
 \DN@{\xyPSellipsed@x@@\xyPScirc@Special}%
 \ifx\framehfill\frm@doth@@
 \DN@{\xyPSellipsed@x@@\xyPSdotcirc@Special}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyPSellipsed@x@@\xyPSdashcirc@Special}%
 \fi\fi \next@{#1}{#2}}
\xydef@\xyPSellipsed@x@@#1#2#3{\vglue #3\vglue #3\relax
 \hbox{\L@c = #2\relax \R@c=\L@c \D@c = #3\relax \U@c=\D@c 
 \hglue#2\hglue#2\relax\xypsellipse@#1\hglue#2\hglue#2\relax}%
 \vglue #3\vglue #3\relax}
\xydef@\xyPSdashhfill@{{\SemiDirectionChar=95 \Direction=3072 \xyPSdash@}}
\xydef@\xyPSdashvfill@{{\SemiDirection=31 \Direction=1023 \xyPSdash@}}
\xydef@\xypsoval@#1{%
 \dimen@=\L@c \advance\dimen@\R@c
 \dimen@ii=\U@c \advance\dimen@ii\D@c 
 \ifdim\dimen@ii<\dimen@ \relax \dimen@=\dimen@ii\fi \divide\dimen@\tw@
 \ifdim\R@>\dimen@ \relax \R@=\dimen@ \fi
 \D@c=-\D@c \L@c=-\L@c 
 \edef\tmp@{\expandafter\removePT@\the\R@
 \space\expandafter\removePT@\the\R@c 
 \space\expandafter\removePT@\the\D@c 
 \space\expandafter\removePT@\the\L@c 
 \space\expandafter\removePT@\the\U@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypscircle@#1{\dimen@=\R@
 \edef\tmp@{\expandafter\removePT@\the\dimen@}%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xypsellipse@#1{\edef\tmp@{%
 \expandafter\removePT@\the\U@c \space
 \expandafter\removePT@\the\D@c \space
 \expandafter\removePT@\the\L@c \space
 \expandafter\removePT@\the\R@c }%
 \expandafter#1\expandafter{\tmp@}}
\xydef@\xyPSoval@Special#1{\PSmacro@{#1 ov}}
\xydef@\xyPScirc@Special#1{\PSmacro@{#1 ox}}
\xydef@\xyPSdotcirc@Special#1{\PSmacro@{#1 ot}}
\xydef@\xyPSdashcirc@Special#1{\PSmacro@{#1 od}}
\xydef@\xyPSdotoval@Special#1{\PSmacro@{#1 vt}}
\xydef@\xyPSdashoval@Special#1{\PSmacro@{#1 vd}}
\xydef@\xyPSfilledRegion#1#2{\setboxz@h{\lower\D@c\vbox{%
 \vglue\U@c\hbox{#1#2\empty\hglue\L@c\hglue\R@c}\vglue\D@c}}%
 \ht\z@=\z@ \dp\z@=\z@ \wd\z@=\z@ \boxz@}
\xydef@\filledRectangle@PS{%
 \xyPSfilledRegion{\xypsoval@\xyPSfilloval@Special}}
\xydef@\filledCircle@PS#1{{\R@c=\R@ \L@c=\R@ \U@c=\R@ \D@c=\R@
 \xyPSfilledRegion{\xypscircle@\xyPSfillcirc@Special}#1}}
\xydef@\filledEllipse@PS{%
 \xyPSfilledRegion{\xypsellipse@\xyPSfillellipse@Special}}
\xydef@\filledOval@PS{%
 \xyPSfilledRegion{\xypsoval@\xyPSfilloval@Special}}
\xydef@\frame@emph@PS#1{\filled@{#1}\relax}
\xydef@\installPSfills@{%
 \let\frame@emph@@=\frame@emph@PS
 \let\filledRectangle@@=\filledRectangle@PS
 \let\filledOval@@=\filledOval@PS
 \let\filledCircle@@=\filledCircle@PS
 \let\filledEllipse@@=\filledEllipse@PS
}
\xydef@\xyPSfilloval@Special#1#2{%
 \ifx#2\relax\PSmacro@{#1 sfo}%
 \else\PSmacro@{#1 fo}\fi}
\xydef@\xyPSfillcirc@Special#1#2{%
 \ifx#2\relax\PSmacro@{#1 sfc}%
 \else\PSmacro@{#1 fc}\fi}
\xydef@\xyPSfillellipse@Special#1#2{%
 \ifx#2\relax\PSmacro@{#1 sfe}%
 \else\PSmacro@{#1 fe}\fi}
\endinput


==> xyps-l.tex <==
%% xyps-l.tex from $Id: xyps-l.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Line extension'' PostScript backend support.
%% Copyright (c) 1993-1997 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-lloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-lloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xyps-sloaded\endcsname\empty\else
 \xyinputorelse@{xyps-s}{\xyerror@{Could not load xyps-s}{}}%
 \xycatcodes\fi
\xydef@\installPSline@{\installPSstyle@
 \installPSlinestyles@ \installPSpolylines@ }
\xydef@\UsePSlines{\installPSline@}
\xydef@\NoPSlines{\UnloadLine@\relax}
\xydef@\xyPSlineSpecial@#1{\addtostyletoks@{ #1 lw}}
\xydef@\xyPScapSpecial@#1{\addtostyletoks@{ #1 lc}}
\xydef@\xyPSjoinSpecial@#1{\addtostyletoks@{ #1 lj}}
\xydef@\xyPSmiterSpecial@#1{\addtostyletoks@{ #1 ml}}
\xydef@\installPSlinestyles@{%
 \let\xylinewidth@@=\xylinewidth@
 \let\transxyline@@=\transxyline@
 \let\xylineSpecial@@=\xyPSlineSpecial@
 \let\resetxyline@@=\resetxyline@i
 \let\xy@linecap@@=\xy@linecap@
 \let\xycapSpecial@@=\xyPScapSpecial@
 \let\resetxylinecap@@=\resetxylinecap@i
 \let\xy@linejoin@@=\xy@linejoin@
 \let\xyjoinSpecial@@=\xyPSjoinSpecial@
 \let\resetxylinejoin@@=\resetxylinejoin@i
 \let\xy@linemiter@@=\xy@linemiter@
 \let\xymiterSpecial@@=\xyPSmiterSpecial@
 \let\resetxylinemiter@@=\resetxylinemiter@i
}
\xydef@\xypolylinePS@Special#1{\PSmacro@{#1 pl}}
\xydef@\xypolydotPS@Special#1{\PSmacro@{#1 pt}}
\xydef@\xypolydashPS@Special#1{\PSmacro@{#1 pd}}
\xydef@\xypolyfillPS@Special#1{\PSmacro@{#1 pf}}
\xydef@\xypolyeofillPS@Special#1{\PSmacro@{#1 pe}}
\xydef@\installPSpolylines@{%
 \let\xypolyline@Special=\xypolylinePS@Special
 \let\xypolydot@Special=\xypolydotPS@Special
 \let\xypolydash@Special=\xypolydashPS@Special
 \let\xypolyfill@Special=\xypolyfillPS@Special
 \let\xypolyeofill@Special=\xypolyeofillPS@Special
 \let\xy@polystyle@@=\xy@polystyle@ }
\endinput


==> xyps-pro.tex <==
%% xyps-pro.tex from $Id: xyps-pro.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``PostScript Prolog'' for PostScript support.
%% Copyright (c) 1993-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
\begingroup \xycatcodes%
 \count@=\xydashl@\relax \count@@=\xydashw@\relax%
 \let\firstPS@@=\relax%
 \xyPSobeylines@@%
\PSspecialdict@@{%
/XYdict where not{250 dict /XYdict exch def 
 /xy{mark exch XYdict begin countdictstack /xylevel exch def
 xyopen xycolor mark xypatt xypattern stopped xyclose end
 cleartomark}def /xyg{gsave xy}def 
 /xyf{currentfont exch xy grestore setfont}def
 /xycc{{xychgcol}xy}def /xyc{XYdict begin xycolstore end}def
 /xyx{/xyYpos exch def /xyXpos exch def}def 
 /xyp{currentpoint xyx}def
 /xyd{setupDirection XYdirection 2 mul}def 
 /xyct{currentpoint xyt 2 copy 6 2 roll}def
 /xyt{xyXpos xyYpos 2 copy translate}def /xyr{neg rotate xynt}def
 /xyrs{neg rotate 3 -1 roll sub neg 3 1 roll sub exch moveto xynt}def
 /xynt{neg exch neg exch translate}def /xys{scale xynt}def
 /xyss{scale 3 -1 roll sub neg 3 1 roll sub exch moveto xynt}def
 /xyi{0 0 transform grestore gsave itransform}def
 }if}%
\tmp@false\def\do#1{\DN@{#1}\ifx\next@\nextii@\tmp@true\fi}%
\DNii@{17oztex}\xydriversselected@@\iftmp@\PSspecialdict@@{%
 /@boxy{prespecialVM restore grestore}def
 /@eoxy{gsave /prespecialVM save def}def
 }%
\else \DNii@{oztex}\xydriversselected@@\iftmp@\PSspecialdict@@{%
 /@oxy{prespecialVM restore grestore}def
 /@oxy{gsave /prespecialVM save def}def
 }\fi\fi% 
\PSdict@@{/XYdict where pop begin XYdict begin}%
\PSdict@@{%
 /xyopen{currentdict /XYddict known{XYddict null eq{}
 {XYddict begin xyopen}ifelse}if}def
 /xyclose{countdictstack -1 xylevel 1 add{pop end}for}def
 /xychgcol{/xycolor exch def}def /xysetcol{xypush xychgcol}def 
}%
\PSdict@@{%
 /xypush{16 dict /XYddict exch def XYddict begin}def
 /undef where
 {pop /xypop{countdictstack xylevel eq{}{end}ifelse
 currentdict /XYddict undef}def}
 {/xypop{countdictstack xylevel eq{}{end}ifelse
 /XYddict null def}def}ifelse
 /pu /xypush load def /pp /xypop load def}%
\PSdict@@{%
 /xypspt{72 72.27 div dup scale}bind def /pscorrect{.85 mul}bind def 
 /gstartxy{gsave xypspt xywidth xycap xyjoin xymiter newpath 0 0 moveto}def 
 /xypath{gstartxy rmoveto counttomark 2 idiv -1 1{pop lineto}for}def 
 /xystroke{stroke grestore}bind def 
 /xyfill{closepath fill grestore}bind def
 /xystfil{closepath gsave fill grestore 0 setgray 
 0 setlinewidth xystroke}bind def
 /xyeofill{closepath eofill grestore}bind def
}%
\PSdict@@{%
 /xypolyline{xypath xystroke}def /xypolyfill{xypath xyfill}def
 /xydotsep{/@ currentlinewidth 2 mul def}def
 /xypolydot{xypath xydotsep [xydt @] 0 setdash xystroke}def
 /xypolydash{xypath xydotsep [@ @] 0 setdash xystroke}def
 /xypolyeofill{xypath xyeofill}def /pe /xypolyeofill load def 
 /pl /xypolyline load def /pf /xypolyfill load def 
 /pt /xypolydot load def /pd /xypolydash load def }%
\PSdict@@{%
 /arc4pop{arcto 4{pop}repeat}bind def 
 /xyoval{gstartxy oval closepath xystroke}def
 /xycircle{gstartxy circle xystroke}def
 /circle{dup 0 moveto 0 0 3 -1 roll 0 360 arc}def
 /oval{newpath 2 copy exch 5 index add 2 div exch 3 copy 10 3 roll 
 moveto 1 index dup 5 1 roll 3 index 7 index arc4pop
 dup dup 4 1 roll 4 index exch 6 index arc4pop
 1 index dup 8 1 roll 4 index 4 index arc4pop
 arc4pop closepath}def
 /xyellipse{gstartxy counttomark 1 gt{squarify pop pop 1}if
 circle xystroke}def
 /ov /xyoval load def /ox /xyellipse load def }%
\PSdict@@{%
 /dotit{dup currentlinewidth 6 mul div round div
 /@ exch def [xydt @] 0 setdash}def
 /elldash{dup 4 -1 roll 10 exch div dashit}def
 /ovdash{dup 10 dashit}def
 /dashit{div round 2 mul div /@ exch def [@ @] 0 setdash}def
 /dotcirc{gstartxy cirlen dotit circle xystroke}def
 /dashcirc{gstartxy cirlen dashit circle xystroke}def
 /dotoval{gstartxy 5 copy ovlen dotit oval xystroke}def
 /dashoval{gstartxy 5 copy ovlen ovdash oval xystroke}def
 /cirlen{dup 6.283185 mul}bind def
 /ovlen{3 -1 roll sub 3 1 roll sub add exch 1.716815 mul sub}def
 /dotellipse{gstartxy counttomark 1 gt{squarify pop pop 1}if
 cirlen dotit circle closepath xystroke}def
 /dashellipse{gstartxy counttomark 1 gt{squarify add 2 div 1}
 {1 exch 1 exch}ifelse cirlen elldash circle xystroke}def
 /ot /dotellipse load def /od /dashellipse load def 
 /vt /dotoval load def /vd /dashoval load def }%
\PSdict@@{%
 /filloval{gstartxy oval xyfill}def
 /stfiloval{gstartxy oval xystfil}def
 /fillcircle{gstartxy circle xyfill}def 
 /stfilcircle{gstartxy circle xystfil}def 
 /fillellipse{gstartxy squarify pop pop 1 circle xyfill}def
 /stfilellipse{gstartxy squarify pop pop 1 circle xystfil}def
 /squarify{4 copy sub 2 div 3 1 roll sub 2 div translate
 add 2 div 3 1 roll add 2 div 2 copy scale
 2 copy add 2 div currentlinewidth exch div setlinewidth
 newpath}def
 /fe /fillellipse load def /sfe /stfilellipse load def 
 /fo /filloval load def /sfo /stfiloval load def
 /fc /fillcircle load def /sfc /stfilcircle load def }%
\PSdict@@{%
 /xywidth{.4 pscorrect setlinewidth}bind def
 /xydash{[] 0 setdash}bind def /xycap{1 setlinecap}bind def
 /xyjoin{1 setlinejoin}bind def /xymiter{10 setmiterlimit}bind def
}%
\PSdict@@{%
 /cc{dup exec xychgcol}def
 /lw{dup setlinewidth /@l exch def
 /xywidth{@l setlinewidth}bind def}def
 /lc{dup setlinecap /@c exch def
 /xycap{@c setlinecap}bind def}def
 /lj{dup setlinejoin /@j exch def
 /xyjoin{@j setlinejoin}bind def}def
 /ml{dup setmitrelimit /@m exch def
 /xymiter{@m setmitrelimit}bind def}def
}%
\PSdict@@{%
 /setupDirection{dup -2048 lt{3072 add neg 1024 exch}
 {dup 0 lt{1024 add neg -1024}{dup 2048 lt{1024 sub -1024 exch}
 {3072 sub 1024}ifelse}ifelse}ifelse atan 
 dup 180 gt{360 sub}if dup /XYdirection exch def rotate}def
 }%
\PSdict@@{%
 userdict begin 
 /gray{setgray}bind def /gray@{setgray}bind def
 /rgb{setrgbcolor}bind def /rgb@{setrgbcolor}bind def
 /hsb{sethsbcolor}bind def /hsb@{sethsbcolor}bind def
 /setcmykcolor where{pop}{/setcmykcolor{dup 3 1 roll dup 5 1 roll
 exch sub 1 add 5 1 roll exch sub 1 add 4 1 roll 
 exch sub 1 add 3 1 roll setrgbcolor}bind def}ifelse
 /cmyk{setcmykcolor}bind def /cmyk@{setcmykcolor}bind def
 /sethalftone where{/sethalftone load /tone exch def}if
 /xycolarray 3 array def /xycolstore{currentrgbcolor 2 -1 0
 {exch xycolarray 3 1 roll put}for}def xycolstore
 /xycolor{0 1 2{xycolarray exch get}for setrgbcolor}def
 /xypatt{}def /xypattern{cleartomark}bind def
 end}%
\PSdict@@{end end}%
\endgroup%
\endinput


==> xyps-ps.tex <==
%% xyps-ps.tex from $Id: xyps-ps.doc,v 3.12 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``PS-PS'' PostScript support.
%% Copyright (c) 1993-1997 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-psloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-psloaded\endcsname=\empty \xycatcodes
\xylet@\PSmacro@@=\eat@
\xylet@\PSdict@@=\eat@
\xylet@\PSspecial@@=\eat@
\xylet@\PSread@@=\eat@
\xylet@\PSinclude@@=\eat@
\xylet@\PSraw@@=\eat@
\xylet@\xyPSobeylines@@=\relax
\xylet@\PSspecialdict@@=\eat@
\xydef@\UnloadPSps@{%
 \let\PSmacro@@=\eat@
 \let\PSdict@@=\eat@
 \let\PSspecial@@=\eat@
 \let\PSread@@=\eat@
 \let\PSinclude@@=\eat@
 \let\PSraw@@=\eat@
 \let\xyPSobeylines@@=\relax
 \let\PSspecialdict@@=\eat@
}
\xydef@\UnloadPS@{\UnloadPSps@
 \expandafter\ifx\csname xypsloaded\endcsname\unknown\PSspecials@false
 \else\expandafter\NoPSspecials\fi}
\xylet@\UnloadPS@@=\UnloadPS@
\ifx\undefined\dvitype@\xydef@\dvitype@{null}\fi
\xylet@\xyrealshipout@=\shipout
\xydef@\xyPSshipout@{\setbox9=\copy\voidb@x
 \afterassignment\xyPSshipout@i\setbox9=}
\xydef@\xyPSshipout@i{\ifvoid9 \expandafter\aftergroup\fi\xyPSshipout@ii}
\xydef@\xyPSshipout@ii{\xyrealshipout@\vbox{\XYpredict@@\box9}}
\xydef@\@PSshipout{\global\let\shipout=\xyPSshipout@ }
\xydef@\xyPSshipout@PSii{%
 \ifUsePSdict@@\let\XYshipdict@=\includeXYPSdict@@
 \else\def\XYshipdict@{\XYpredict@@\XYdict@@}\fi
 \xyrealshipout@\vbox{\XYshipdict@\box9}}
\xydef@\firstPS@{%
 \global\let\firstPS@@=\relax \global\let\firstPS@=\relax}
\xylet@\firstPS@@=\firstPS@
\ifx\undefined\dumpPSdict@@ \xylet@\dumpPSdict@@=\relax \fi
\xydef@\installxyps@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}\xycatcodes
 \installxyps@@ \installxyps@x }
\xylet@\installxyps@@=\relax
\xylet@\setupxyPS@@=\relax
\xywithoption{ps}{\let\setupxyPS@@=\setupxyPS@}
\xydef@\installxyps@x{\dumpPSdict@@ 
 \ifx\xyrealshipout@\undefined \let\xyrealshipout@=\shipout\fi
 \ifx \shipout \xyrealshipout@ 
 \ifUsePSdict@@ \DN@{\includePSmessage@\includeXYPSdict@\message{>}}%
 \else \DN@{\XYdict@\endXYdict@}\fi
 \else \DN@{\let\xyPSshipout@ii=\xyPSshipout@PSii \@PSshipout}\fi
 \let\firstPS@=\relax \next@
 \let\XYpredict@=\relax
 \setupxyPS@@ }
\let\realinstallxyps@x=\installxyps@x
\ifx\undefined\AfterBeginDocument
 \def\installxyps@x{\xysetup@@{\realinstallxyps@x}}%
\else
 \def\installxyps@x{\AfterBeginDocument{\realinstallxyps@x}}%
\fi
\xydef@\xydefaultdriver@{dvips}
\xydef@\xyPSdriver#1{\def\xydefaultdriver@{#1}}
\xydef@\installxyps@orig{\DN@{}%
 \ifx\xydriversselected@@\empty
 \DN@{\expandafter\defaultinstallps@\expandafter{\xydefaultdriver@}}%
 \else \def\do##1{%
 \expandafter\ifx\csname##1@xy@ps\endcsname\relax
 \DN@{\defaultinstallps@{##1}}}%
 \xydriversselected@@ 
 \else \DN@##1{}\fi\fi \next@ }
\xydef@\defaultinstallps@#1#2{%
 \xywarning@{no driver specified, using #1 }%
 \xyrequire{#1}\csname #1@xy@ps\endcsname{}}
\xydef@\null@xy@ps{\installxyps@}
\xydefcsname@{shape [!...]}#1{%
 \expandafter\ifx\csname xyps-sloaded\endcsname\empty \DN@{\xyPSescapestyle@{#1}@@}%
 \else\ifxyPSshapes@\DN@{\xyPSshapechar@{#1}@@}%
 \else \DN@{\xyPScharwarning@}\fi\fi \next@ }
\xydefcsname@{shape [psxy]}{\ifxyPSshapes@\DN@{\xyPSpsxy@}%
 \else \DN@{\xyPScharwarning@}\fi \next@ }
\xydef@\xyPSpsxy@{%
 \setboxz@h{\dimen@=\L@p \advance\dimen@-\R@p 
 \dimen@ii=-\U@p \raise\dimen@ii\hbox to\z@{%
 \kern\dimen@\xyPScurrpt@\kern-\dimen@}\boxz@}}%
\xydef@\xyPScurrpt@{\ifxyPSshapes@\expandafter\xyPScurrpt@@\fi}
\xydef@\xyPScurrpt@@@{\PSspecial@@{xyi}\PSraw@@{userdict begin xyx end}}
\ifx\undefined\xyPScurrpt@@ \xylet@\xyPScurrpt@@=\xyPScurrpt@@@ \fi
\xywarnifdefined\xyPSshapechar@
\xywarnifdefined\xyPSsplitshape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPSshapechar@#1@@{\xyPSsplitshape@#1<><>@@}%
 \gdef\xyPSsplitshape@#1<>#2<>#3@@{\xyPSsplitPS@{#1}{#2}}}
\xydef@\xyPSrawA@#1{\expandafter\xyPSrawAA@ #1{}}%
\xydef@\xyPSrawAA@#1#2{\PSraw@@{{pu #1}xyg #2}%
 \PSmessage{{pu #1}xyg #2}}%
\xydef@\xyPSrawZ@#1{\PSraw@@{{#1 pp}xyf}\PSmessage{{#1 pp}xyf}}%
\xydef@\modPSboxz@{%
 \expandafter\DN@\expandafter{\xyPSpre@{}}\ifx\next@\empty\else
 \setboxz@h{\expandafter\xyPSrawA@\expandafter{\xyPSpre@{}}\boxz@
 \expandafter\xyPSrawZ@\expandafter{\xyPSpost@}}\DN@{}\fi}%
\xydef@\modPSdrop@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPSrawA@\expandafter{\xyPSpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Drop@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPSrawZ@\expandafter{\xyPSpost@}}%
 \DN@##1{\expandafter\def\expandafter\Drop@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\modPSconnect@{%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPSrawA@\expandafter{\xyPSpre@{}}}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{\nextii@ ##1}}%
 \expandafter\next@\expandafter{\Connect@@}%
 \expandafter\DNii@\expandafter{%
 \expandafter\xyPSrawZ@\expandafter{\xyPSpost@}}%
 \DN@##1{\expandafter\def\expandafter\Connect@@\expandafter{\tmp@ ##1}}%
 \expandafter\next@\expandafter{\nextii@}}%
\xydef@\xyPSpre@{{}{}}
\xydef@\xyPSpost@{}
\xydef@\PSmessage@#1{\W@{PS: #1, direction=\the\Direction}}
\xydef@\PSignore@#1{}%
\xydef@\showPSmessages{\let\PSmessage=\PSmessage@}
\xydef@\hidePSmessages{\let\PSmessage=\PSignore@}
\xylet@\PStracing=\showPSmessages
\hidePSmessages
\xydef@\PSmacro@#1{\PSmacro@@{#1}\PSmessage{#1}}
\xydef@\includeXYPSdict@@{%
 \expandafter\PSinclude@@\expandafter{\xyPSdictname}}
\xydef@\includeXYPSdict@r{\message{PS: includeXYPSdict}\includeXYPSdict@@
 \let\includeXYPSdict@=\relax}
\xylet@\includeXYPSdict@\includeXYPSdict@r
\xydef@\endXYdict@{}
\xydef@\includePSmessage@@{\message{<xyps: including \xyPSdictname}}
\xylet@\includePSmessage@=\includePSmessage@@ 
\xydef@\xyPSdictknown@{%
 \immediate\closein\xyread@
 \xywarning@{File \xyPSdictname\space already exists}
 \message{ Do you wish to overwrite it \string? y/n }%
 \read16 to \next
 \DNii@{\xywarning@{You did not type Y or N -- try again please}%
 \xyPSdictknown@}%
 \DN@{Y }\ifx\next@\next \DNii@{\writePSdict@@}%
 \else\DN@{y }\ifx\next@\next \DNii@{\writePSdict@@}%
 \else\DN@{n }\ifx\next@\next \DNii@{\cancelPSdict@}%
 \else\DN@{N }\ifx\next@\next \DNii@{\cancelPSdict@}%
 \fi\fi\fi\fi \nextii@ }
\xydef@\cancelPSdict@{%
 \xywarning@{cancelling dump of PostScript dictionary}}
\xydef@\noDictmessage@{%
 \xywarning@{\dvitype@\space does not support the use of a header file}}
\DN@{\csname newif\endcsname\ifUsePSdict@@\DN@{}}
 \ifx\undefined\UsePSdict@@true\else\DN@{}\fi \next@
\ifx\undefined\xyPSdefaultdict
 \xydef@\xyPSdefaultdict{%
 \DN@##1.##2.##3@{\gdef\xyPSdictname{xy##1##2dict.pro}}%
 \expandafter\next@\xyversion.@}%
\fi
\ifx\undefined\UsePSheader@
 \xydef@\UsePSheader@#1{%
 \DN@{#1}\ifx\next@\empty
 \else \gdef\xyPSdictname{#1}\fi
 \ifx\xyPSdictname\undefined\xyPSdefaultdict\fi
 \gdef\xyHeaderMessage@{%
 It includes a reference to the PostScript file \xyPSdictname.^^J}%
 \UsePSdict@@true}%
 \let\UsePSheader=\UsePSheader@
\fi
\xywarnifdefined\xyPS@@
\xywarnifdefined\xyPS@@@
{\catcode`|=14 \catcode`\%=12 \catcode`\<=1 \catcode`\>=2 |
 \gdef\xyPS@@<%%>\gdef\xyPS@@@<%!>}
\xydef@\writePSdict@@{\message{PS: writePSdict@@}\writePSdict@ 
 \def\writePSdict@@{\message{write PS relaxed}}}
{\catcode`|=14 \catcode`\%=12 
 \gdef\writePSdict@{{\begingroup|
 \immediate\openout\xywrite@=\xyPSdictname \relax
 \message{<xyps: dumping \xyPSdictname}|
 \def\PSdict@@@##1{\immediate\write\xywrite@{##1}}|
 \let\xyPSobeylines@@=\obeyoutlines@
 \let\firstPS@@=\relax
 \let\endXYdict@=\relax
 \PSdict@@@{\xyPS@@@ PS-Adobe-3.0 Resource-procset}|
 \PSdict@@@{\xyPS@@ Title: \xyPSdictname}|
 \PSdict@@@{\xyPS@@ Version: 3.8.6}|
 \PSdict@@@{\xyPS@@ Creator: Xy-ps backend to Xy-pic}|
 \PSdict@@@{\xyPS@@ DocumentSuppliedProcSets: XYdict}|
 \ifx\dvitype@\undefined
 \PSdict@@@{\xyPS@@ For: use with Xy-pic}\else
 \PSdict@@@{\xyPS@@ For: \dvitype@ use of Xy-pic}\fi
 \PSdict@@@{\xyPS@@ BeginResource: procset XYdict}|
 \def\PSspecialdict@@##1{\PSdict@@@{##1^^J}}|
 \let\PSdict@@=\PSdict@@@ \let\xy@begindvi=\literal@|
 \UsePSdict@@false\XYpredict@@|
 \XYdict@@|
 \PSdict@@@{\xyPS@@ EndResource}|
 \immediate\closeout\xywrite@
 \message{>}|
 \endgroup}}}
\xywarnifdefined\obeyoutlines@
{\catcode`\^^M=\active%
 \gdef\obeyoutlines@{\catcode`\^^M=\active \def^^M{^^J}%
 \newlinechar=`\^^J\obeyspaces}}
\xydef@\XYpredict@@{\ifUsePSdict@@\DN@{}\else
 \DN@{\xy@begindvi{\xyinputorelse@{xyps-pro}%
 {\xyerror@{Could not load xyps-pro}{}}\xyuncatcodes}}%
 \next@
 \DN@{\xy@begindvi{\xyinputorelse@{xypspatt}%
 {\xyerror@{Could not load xypspatt}{}}\xyuncatcodes}}\fi
 \next@ }
\xydef@\XYpredict@r{\XYpredict@@ \let\XYpredict@=\relax \installxyps@}
\xylet@\XYpredict@\XYpredict@r
\xydef@\XYdict@{\XYdict@@\def\XYdict@{\message{PS relaxed}}}%
\xydef@\XYdict@@{\DN@{\xyinputorelse@{xypsdict}%
 {\xyerror@{Could not load xypsdict}{}}\xyuncatcodes}%
 \expandafter\xy@begindvi\expandafter{\next@}}
\xydef@\forceload@XYdict{%
 \let\includeXYPSdict@=\includeXYPSdict@r
 \let\XYpredict@=\XYpredict@r
 \let\XYdict@=\XYdict@@ \expandafter\installxyps@ }
\xynew@{if}\ifxyPSshapes@ \xyPSshapes@true 
\xydef@\xyPScharwarning@@{\xyPScharmessage@
 \gdef\xyPScharwarning@@{\xyPScharmessage@
 \xywarning@{...no further PostScript warnings will be given}%
 \global\let\xyPScharwarning@@=\relax }}
\xydef@\xyPScharmessage@{\xywarning@{%
 the current <driver> does not fully support PostScript effects}}%
\xydef@\newxyshape#1#2#3{%
 \DN@{#3}\ifx\next@\empty
 \xydefcsname@{shape [#1]}{\csname xyshape@#1@\endcsname}%
 \else \expandafter\def\csname shape [#1]\endcsname{%
 \csname xyshape@#1@\endcsname}\fi
 \DN@{#2}\ifx\next@\empty
 \expandafter\def\csname xyshape@#1@\endcsname{%
 \xyundefinedEffect@{#1}{}@@}%
 \else \expandafter\def\csname xyshape@#1@\endcsname{#2}\fi }
\xydef@\xyundefinedEffect@#1#2@@{%
 \xywarning@{The #1 #2 effect is not implemented with the current driver}}%
\xydef@\newxyPSshape#1#2{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@ \newxyshape{#1}{}\relax\fi
 \expandafter\DNii@\expandafter{\csname xyPSshape@#1@\endcsname}%
 \expandafter\def\nextii@{#2}%
 \ifx\nextii@\empty\expandafter\def\next@{\xyPSnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}%
 \expandafter\tmp@\fi }
\xydef@\xyPSnotimplemented@@#1@@{%
 \xywarning@{This PostScript effect is not implemented yet}}%
\xydef@\xyPSnotfinished@@{%
 \xywarning@{This effect is not reliable yet; box sizes may be wrong}}%
\endinput


==> xyps-r.tex <==
%% xyps-r.tex from $Id: xyps-r.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``PostScript Rotations and Scaling''.
%% Copyright (c) 1993-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-rloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-rloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xyps-sloaded\endcsname\empty\else
 \xyinputorelse@{xyps-s}{\xyerror@{Could not load xyps-s}{}}%
 \xycatcodes\fi
\xydef@\installPSrotscale@{\installPSstyle@
 \let\xyRotate@@=\xyPSrotate@@
 \let\doSpecialRotate@@=\doPSspecialRotate@@
 \let\xyscale@@=\xyPSscale@@
 \xyPSshapes@true
 \xyuncatcodes }
\xydef@\UsePSrotate{\installPSrotscale@}
\xydef@\NoPSrotate{\UnloadRotate@\relax}
\xydef@\xyPSpretransform@{\xyPSrawA@{\preXYtransform@@}}
\xydef@\xyPSposttransform@{\xyPSrawZ@{\postXYtransform@@}}
\let\preXYtransform@=\xyPSpretransform@
\let\postXYtransform@=\xyPSposttransform@
\xydef@\xyPSrotSplit@{%
 \expandafter\def\expandafter\preShape@@\expandafter{\xyPSpre@}%
 \expandafter\def\expandafter\postShape@@\expandafter{\xyPSpost@}}
\xydef@\xyPSscale@@#1#2{%
 \xyPSsplitPS@{\xyscale@start(#1,#2)}{\xyscale@end}%
 \xyPSrotSplit@\xyPSpsxy@ }
\xydef@\xyPSrotate@@#1{%
 \xyPSsplitPS@{\xyrot@start(#1 xyd)}{\xyrot@end}%
 \xyPSrotSplit@\xyPSpsxy@ }
\xydef@\xyPSspecialRotate@#1{%
 \xyPSsplitPS@{\xyrot@start(#1)}{\xyrot@end}\xyPSrotSplit@\xyPSpsxy@ }
\xydef@\doPSspecialRotate@@#1@@{\xyPSspecialRotate@{#1}}
\xydef@\xyRotScale@@{%
 \def\xyrot@start(##1){{xyt ##1\space xyr}}%
 \def\xyscale@start(##1,##2){{xyt ##1\space##2\space xys}}%
 \def\xyrot@end{}\def\xyscale@end{}}
\endinput


==> xyps-s.tex <==
%% xyps-s.tex from $Id: xyps-s.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Style extension'' PostScript support.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-sloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-sloaded\endcsname=\empty \xycatcodes
\xydef@\xykillstyles@@{\Unloadstyle@}%
\xywarnifdefined\xyPSescapestyle@
\xywarnifdefined\xyPSsplitescape@
{\xyuncatcodes \catcode`@=11
 \gdef\xyPSescapestyle@#1@@{\xyPSsplitescape@#1<><>@@}%
 \gdef\xyPSsplitescape@#1<>#2<>#3@@{\xyescape@@{#1}{#2}}}
\xydef@\xyPSsplitPS@#1#2{%
 \def\xyPSpre@{#1}\def\xyPSpost@{#2}\modPSboxz@ }
\xydef@\xyescape@@#1#2{\checkXyStyle@ 
 \applyFIFOstyle@\prexyescape@{#1}\postxyescape@{#2}}
\xydef@\prexyescape@{\xyescapeSpecial@}
\xydef@\postxyescape@{\xyescapeSpecial@}
\xylet@\xyescapeSpecial@=\eat@
\let\xyescapeSpecial@=\addtostyletoks@
\xydef@\installPSstyle@{%
 \def\preXYstyle@@{\xyPSpre@}%
 \let\xydoprestyles@=\xyPSrawstyleA@
 \let\xydopoststyles@=\xyPSrawZ@
 \let\xykillstyles@=\xykillstyles@@
 }
\xydef@\xyPSrawstyleA@#1{\xyPSrawA@{{#1}{}}}
\endinput


==> xyps-t.tex <==
%% xyps-t.tex from $Id: xyps-t.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Pattern and Tile extension'' PostScript support.
%% Copyright (c) 1993-1997 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\expandafter\ifx\csname xyps-tloaded\endcsname\empty
 \message{not reloaded}\endinput \fi
\expandafter\let\csname xyps-tloaded\endcsname=\empty \xycatcodes
\expandafter\ifx\csname xyps-sloaded\endcsname\empty\else
 \xyinputorelse@{xyps-s}{\xyerror@{Could not load xyps-s}{}}%
 \xycatcodes\fi
\xydef@\installPSpatterns@{\installPSstyle@
 \let\xypattern@=\xyPSpattern@@
 \let\xypatternwarning@=\relax
 \xystandardpatterns@
 \xyuncatcodes }
\xylet@\UnloadPSpatterns@=\Unloadpattern@
\xydef@\UsePStiles{\installPSpatterns@}
\xydef@\NoPStiles{\UnloadPSpatterns@\relax}
\xydef@\xyPSnewpattern@#1#2#3#4#5{%
 \expandafter\DN@\expandafter{\csname shape [#1]\endcsname}%
 \DNii@{\relax}\ifx\next@\nextii@\newxypattern{#1}{}\relax\fi
 \DNii@{#4}\ifx\nextii@\empty
 \expandafter\DNii@\expandafter{\csname xyPSshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPSpattern@{#2 #3}}\else
 \expandafter\DNii@\expandafter{\csname xyPSshape@#1@\endcsname}%
 \expandafter\def\nextii@{\xyPSpattern@{#4}}\fi
 \ifx\nextii@\empty\expandafter\def\next@{\xyPSnotimplemented@@`#1'@@}%
 \else
 \edef\tmp@{\noexpand\let\expandafter\noexpand\next@
 \expandafter\noexpand\nextii@}\expandafter\tmp@\fi }
\xydef@\xyPSpattern@{\ifPSspecials@\expandafter\xyPSpattern@@
 \else\expandafter\eat@\fi}%
\xydef@\xyPSpattern@@#1{\bgroup \checkXyStyle@ 
 \def\preStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPSpre@}}%
 \def\postStyle@@{\expandafter\addtostyletoks@\expandafter{\xyPSpost@}}%
 \let\modPSboxz@=\modXYstyle@ \xyPS@pattern@@{#1}%
 \toks@={\egroup\let\xy@style@=\relax \def\Drop@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Drop@@}\def\Connect@@}%
 \expandafter\addtotoks@\expandafter{\expandafter{\Connect@@}}%
 \the\toks@ }
\xydef@\xyPS@pattern@@#1{\xyPSsplitPS@{{#1}sp}{}}
\endinput


==> xyps.tex <==
%% xyps.tex from $Id: xyps.doc,v 3.12 2011/05/27 04:51:17 krisrose Exp $
%%
%% Xy-pic ``PostScript backend''.
%% Copyright (c) 1993-1997 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{ps}{PostScript backend}{\stripRCS$Revision: 3.12 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\UsePSspecials{\DNii@{{[4]}}\xyFN@\UsePSspecials@i}
\xydef@\UsePSspecials@i{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\UsePSspecials@i}%
 \else\ifx [\next \DN@[##1]{\DNii@{{[##1]}}\xyFN@\UsePSspecials@i}%
 \else\ifcat 5\noexpand\next \DN@##1{\DNii@{{[##1]}}\xyFN@\UsePSspecials@i}%
 \else\ifx\bgroup\next \DN@{\expandafter\UsePS@specials\nextii@}%
 \else \DN@{\UsePS@specials{[4]}}%
 \fi\fi\fi\fi \next@ }
\xydef@\UsePS@specials#1#2{%
 \ifx\empty\whichPSspecials@
 \DN@{#2}\ifx\next@\empty
 \else
 \expandafter\let\expandafter\next\csname#2@\endcsname
 \ifx\next\relax \DN@{\UsePSspecials@{#2}{}}%
 \else \DN@{\UsePSspecials@{#2}{#1}}\fi
 \fi
 \else
 \DN@{#2}\ifx\next@\empty \DN@{\PSspecials@true}%
 \else
 \DN@{#2}%
 \edef\nextii@{\expandafter\string\whichPSspecials@}%
 \ifx\next@\nextii@\DN@{\PSspecials@true}%
 \else
 \ifx\firstPS@@\relax
 \DN@{\xyerror@{Only one PS <driver> allowed: \dvitype@ already loaded}{}}%
 \else
 \expandafter\let\expandafter\next\csname#2@\endcsname
 \ifx\next\relax
 \DN@{\xyerror@{PostScript specials for `#2' not supported}{}}%
 \else 
 \xywarning@{Changing PS <driver> to #2 }%
 \DN@{\UsePSspecials@{#2}{#1}}%
 \fi
 \fi
 \fi
 \fi
 \fi \next@}
\xydef@\UseDVIPSspecials{\UsePSspecials@\dvips@}
\xydef@\UseTexturesPSspecials{\UsePSspecials@\Textures@}
\xydef@\UseTexturesSpecials{\UsePSspecials@\Textures@}
\xydef@\UsePostScriptSpecials{\UsePSspecials@\dvips@}
\xydef@\UseOzTeXspecials{\UsePSspecials@\OzTeX@}
\xydef@\UseDVITOPSspecials{\UsePSspecials@\dvitops@}
\message{drivers,}
\xydef@\loadPSdriver@#1#2{\xyinputorelse@{xy#1}%
 {\xyrequire{#2}\expandafter\ifx\csname xy#2loaded\else
 {\xyerror@{Unable to load xy#1.tex for #2 driver}{}}\fi}}
\xydef@\dvips@{\loadPSdriver@{ps-dvi}{dvips}}
\xydef@\Textures@{\loadPSdriver@{ps-txt}{Textures}}
\xydef@\OzTeX@{\loadPSdriver@{ps-oz}{OzTeX}}
\xydef@\dvitops@{\loadPSdriver@{ps-dto}{dvitops}}
\xydef@\dvipsone@{\loadPSdriver@{ps-one}{dvipsone}}
\global\newif\ifPSspecials@ 
\xydef@\UsePSspecials@#1{\def\whichPSspecials@{#1}%
 \DN@{\Textures@}\ifx\next@\whichPSspecials@
 \DN@##1{\xyrequire{textures}%
 \def\whichPSspecials@{textures}\xyps@options}%
 \else\DN@{\dvips@}\ifx\next@\whichPSspecials@
 \DN@##1{\xyrequire{dvips}%
 \def\whichPSspecials@{dvips}\xyps@options}%
 \else\DN@{\OzTeX@}\ifx\next@\whichPSspecials@
 \DN@##1{\xyrequire{oztex}%
 \def\whichPSspecials@{oztex}\xyps@options}%
 \else\DN@{\dvitops@}\ifx\next@\whichPSspecials@
 \DN@##1{\xyrequire{dvitops}%
 \def\whichPSspecials@{dvitops}\xyps@options}%
 \else
 \DN@##1{\xyrequire{ps}\xyrequire{#1}\xyps@options}%
 \fi\fi\fi\fi \next@ }
\xydef@\xyps@options{%
 \xyrequire{ps}\xyrequire{line}\xyrequire{color}\xyrequire{crayon}%
 \xyrequire{rotate}\xyrequire{tile}\xyrequire{frame}\xyuncatcodes }
\xydef@\whichPSspecials@{}
\xydef@\NoPSspecials{\xyPSwarning@{off}%
 \PSspecials@false\aftergroup\resetPS@}
\xydef@\resetPS@{\ifPSspecials@\xyPSwarning@{back on}\fi}
\xydef@\UsePSspecials@x{\PSspecials@true\resetPS@}
\xydef@\xyPSwarning@#1{\xywarning@{PostScript switched #1}}
\xyaddunsupport{ps}{\csname UnloadPS@@\endcsname}
\xydef@\PSspecials@{%
 \ifx\next[\DN@[##1]{\setxyPSlevel@{##1}\xyFN@\PSspecials@}%
 \else\DN@{\whichPSspecials@\PSspecials@@}%
 \fi \next@ }%
\xydef@\PSspecials@@{%
 \ifx\und@fined\PSmessage\hidePSmessages\fi \setupxyPS@}
\xydef@\setupxyPSlevelO@{\relax}
\xydef@\setxyPSlevel@#1{\ifcase#1%
 \gdef\setupxyPS@{\setupxyPSlevelO@}%
 \or\gdef\setupxyPS@{\setupxyPSlevelA@}%
 \or\gdef\setupxyPS@{\setupxyPSlevelB@}%
 \or\gdef\setupxyPS@{\setupxyPSlevelC@}%
 \or\gdef\setupxyPS@{\setupxyPSlevelD@}%
 \else\gdef\setupxyPS@{\setupxyPSlevelD@}\fi }
\xywarnifdefined\setupxyPS@ 
 \gdef\setupxyPS@{\setupxyPSlevelD@ \gdef\setupxyPS@{\PSspecials@true}}
\xydef@\PSincrease@#1{%
 \xywarning@{The PS level may only increase: #1 is already active}}
\DN@{\csname newif\endcsname\ifUsePSdict@@\DN@{}}
 \ifx\undefined\UsePSdict@@true\else\DN@{}\fi \next@
\ifx\undefined\xyPSdefaultdict
 \xydef@\xyPSdefaultdict{%
 \DN@##1.##2.##3@{\gdef\xyPSdictname{xy##1##2dict.pro}}%
 \expandafter\next@\xyversion.@}%
\fi
\ifx\undefined\UsePSheader@
 \xydef@\UsePSheader@#1{%
 \DN@{#1}\ifx\next@\empty
 \else \gdef\xyPSdictname{#1}\fi
 \ifx\xyPSdictname\undefined\xyPSdefaultdict\fi
 \gdef\xyHeaderMessage@{%
 It includes a reference to the PostScript file \xyPSdictname.^^J}%
 \UsePSdict@@true}%
 \let\UsePSheader=\UsePSheader@
\fi
\xydef@\dumpPSdict#1{\DN@{#1}\ifx\next@\empty
 \ifx\undefined\xyPSdictname\xyPSdefaultdict\fi
 \else\gdef\xyPSdictname{#1}\fi
 \def\dumpPSdict@@{\writePSdict@@}%
 \ifx\xydriversselected@@\empty\DN@{\xysetup@@\null@xy@ps}%
 \else \DN@{\installxyps@x}\fi \next@}
\message{hooks,}
\gdef\xyPSalternative@#1#2{%
\expandafter\global\expandafter\let\csname origxy#2@\endcsname=#1%
 \xdef#1{\noexpand\ifPSspecials@
 \noexpand\expandafter\expandafter\noexpand\csname xyPS#2@\endcsname
 \noexpand\else
 \noexpand\expandafter\expandafter\noexpand\csname origxy#2@\endcsname
 \noexpand\fi}}%
\xydef@\setupxyPSlevelA@{\xyPStips@%
 \xyPSalternative@{\Tip@@}{Tip}%
 \xyPSalternative@{\Ttip@@}{Ttip}%
 \xyPSalternative@{\Tip@@eu}{Tip@eu}%
 \xyPSalternative@{\Ttip@@eu}{Ttip@eu}%
 \xyPSalternative@{\hook@@}{hook}%
 \xyPSalternative@{\ahook@@}{ahook}%
 \xyPSalternative@{\bhook@@}{bhook}%
 \xyPSalternative@{\aturn@@}{aturn}%
 \xyPSalternative@{\bturn@@}{bturn}%
 \xyPSalternative@{\squiggle@@}{squiggle}%
 \xyPSalternative@{\stopper@@}{stopper}%
 \xyPSalternative@{\line@@}{dash}%
 \xyPSalternative@{\circhar@@}{circhar@}%
 \gdef\setupxyPSlevelA@{\PSincrease@{1}}%
 \global\let\UsePSspecials=\UsePSspecials@x \PSspecials@true}
\xydef@\setupxyPSlevelB@{%
 \let\xyPSfont@=\empty \let\xyPSsemifont@=\empty
 \xyPSalternative@{\cirrestrict@@}{cirrest}%
 \gdef\setupxyPSlevelB@{\PSincrease@{2}}%
 \setupxyPSlevelA@ }
\xydef@\setupxyPSlevelC@{%
 \xyPSalternative@{\cirbuild@}{cirbuild}%
 \xyPSalternative@{\CIRfull@}{CIRfull}%
 \xyPSalternative@{\solid@}{solid}%
 \xyPSalternative@{\point@}{point}%
 \xywithoption{curve}{%
 \xyPSalternative@{\splinesolid@}{splinesolid}}%
 \gdef\setupxyPSlevelC@{\PSincrease@{3}}%
 \setupxyPSlevelB@ }%
\xydef@\setupxyPSlevelD@{%
 \xyPSalternative@{\dash@}{dashed}%
 \xywithoption{curve}{%
 \xyPSalternative@{\splinedashed@}{splinedashed}%
 \xyPSalternative@{\splinedotted@}{splinedotted}}%
 \gdef\setupxyPSlevelD@{}%
 \setupxyPSlevelC@ }
\xydef@\xyPSchar@#1{%
 \PSmacro@{\the\Direction\space \xyPSfont@ #1}}
\xydef@\xyPSsemichar@#1{%
 \PSmacro@{\the\Direction\space \xyPSsemifont@ #1}}
\xydef@\xyPSfont@{f }%
\xydef@\xyPSsemifont@{fs }%
\xydef@\xyPStip@{\xyPSchar@{t}}%
\xydef@\xyPSTip@{\xyPSchar@{/XT tt}}%
\xydef@\xyPSTtip@{\setboxz@h\bgroup 
 \reverseDirection@\line@ \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ 
 \kern-\L@c \boxz@ \kern\L@c \xyPSchar@{/Xt tT}}%
\xydef@\xyPSTip@eu@{\xyPSchar@{/ET tt}}%
\xydef@\xyPSTtip@eu@{\setboxz@h\bgroup 
 \reverseDirection@\line@ \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ 
 \kern-\L@c \boxz@ \kern\L@c \xyPSchar@{/ET tT}}%
\xydef@\xyPScm@\tip@x{\xyFN@\xyPScm@@}%
\xydef@\xyPScm@@{%
 \ifx\next\tip@@ \DN@\tip@@{\tip@x\xyPScmtip@}%
 \else\ifx\next\atip@@ \DN@\atip@@{\tip@x\xyPScmatip@}%
 \else\ifx\next\btip@@ \DN@\btip@@{\tip@x\xyPScmbtip@}%
 \else\DN@{}%
 \fi\fi\fi \next@}%
\xydef@\xyPScmtip@{\xyPSchar@{ct}}%
\xydef@\xyPScmatip@{\xyPSchar@{ca}}%
\xydef@\xyPScmbtip@{\xyPSchar@{cb}}%
\xydef@\xyPStips@{%
 \xyPSalternative@{\atip@@}{atip}%
 \xyPSalternative@{\btip@@}{btip}%
 \xyPSalternative@{\tip@@}{abtip}%
}%
\xydef@\xyPSatip@{\xyPSwhichatip@ 
 \expandafter\xyPSchar@\expandafter{\xyPSfont@@}}%
\xydef@\xyPSbtip@{\xyPSwhichbtip@
 \expandafter\xyPSchar@\expandafter{\xyPSfont@@}}%
\xydef@\xyPSabtip@{\xyPSwhichabtip@
 \expandafter\xyPSchar@\expandafter{\xyPSfont@@}}%
\xydef@\xyPSwhichatip@{\ifx\xyatipfont\xy@@atfont
 \expandafter\xyPSatip@i \else\def\xyPSfont@@{10 /xy A}\fi }%
\xydef@\xyPSwhichbtip@{\ifx\xybtipfont\xy@@btfont
 \expandafter\xyPSbtip@i \else\def\xyPSfont@@{10 /xy B}\fi }%
\xydef@\xyPSwhichabtip@{\ifx\xyatipfont\xy@@atfont
 \expandafter\xyPSabtip@i \else\def\xyPSfont@@{10 /xy AB}\fi }%
\xydef@\xyPSatip@i{%
 \edef\xyPSfont@@{\tipsize@@\space/\tipfamily@@\space A}} 
\xydef@\xyPSbtip@i{%
 \edef\xyPSfont@@{\tipsize@@\space/\tipfamily@@\space B}} 
\xydef@\xyPSabtip@i{%
 \edef\xyPSfont@@{\tipsize@@\space/\tipfamily@@\space AB}} 
\xydef@\xyPSTtips@{%
 \let\Ttip@xy=\Ttip@
 \let\Ttip@cm=\Ttip@
 \let\Ttip@eu=\Ttip@ }
\xydef@\xyPShook@{\xyPSchar@{h}}%
\xydef@\xyPSahook@{\xyPSchar@{ha}}%
\xydef@\xyPSbhook@{\xyPSchar@{hb}}%
\xydef@\xyPSaturn@{\xyPSchar@{ta}}%
\xydef@\xyPSbturn@{\xyPSchar@{tb}}%
\xydef@\xyPSsquiggle@{\xyPSchar@{g}}%
\xydef@\xyPSstopper@{\xyPSchar@{st}}%
\xydef@\xyPSfliptrue@{\DN@{\xyPSsemichar@{T d}}}
\xydef@\xyPSdash@{%
 \DN@{\xyPSsemichar@{F d}}%
 \ifnum\SemiDirectionChar=31
 \ifdim\d@Y<\z@ 
 \ifdim\d@X<\z@ \ifx\xyPSsemifont@\empty\xyPSfliptrue@\fi\fi
 \else
 \ifdim\z@>\d@X 
 \ifx\xyPSsemifont@\empty\else\xyPSfliptrue@\fi
 \else\xyPSfliptrue@\fi
 \fi\fi
 \next@ \setboxz@h{\origxydash@}\kern\wdz@ 
 \setbox\z@=\box\voidb@x }
\xydef@\xyPScirchar@#1{\count@=#1\edef\tmp@{\the\count@}%
 \ifcase#1%
 \xyPScirchar@@@{-180}{-135}{\tmp@}\dimen@=\partroottwo\R@
 \or\xyPScirchar@@@{-135}{-90}{\tmp@}\dimen@=\halfroottwo\R@
 \or\xyPScirchar@@@{-90}{-45}{\tmp@}\dimen@=\halfroottwo\R@
 \or\xyPScirchar@@@{-45}0{\tmp@}\dimen@=\partroottwo\R@
 \or\xyPScirchar@@@0{45}{\tmp@}\dimen@=\partroottwo\R@
 \or\xyPScirchar@@@{45}{90}{\tmp@}\dimen@=\halfroottwo\R@
 \or\xyPScirchar@@@{90}{135}{\tmp@}\dimen@=\halfroottwo\R@
 \or\xyPScirchar@@@{135}{180}{\tmp@}\dimen@=\partroottwo\R@
 \fi}
\xydef@\xyPScirrest@{\relax}%
\xydef@\xyPScirchar@@#1{\relax\count@=#1\edef\tmp@{\the\count@}%
 \expandafter\xyPScirchar@@@\ifcase#1%
 {-180}{-135}{\tmp@}\kern\partroottwo\R@
 \or{-135}{-90}{\tmp@}\kern\halfroottwo\R@
 \or{-90}{-45}{\tmp@}\kern\halfroottwo\R@
 \or{-45}0{\tmp@}\kern\partroottwo\R@
 \or 0{45}{\tmp@}\kern\partroottwo\R@
 \or{45}{90}{\tmp@}\kern\halfroottwo\R@
 \or{90}{135}{\tmp@}\kern\halfroottwo\R@
 \or{135}{180}{\tmp@}\kern\partroottwo\R@
 \fi}
\xydef@\xyPScirchar@@@#1#2#3{\edef\tmp@{#1\space#2\space
 \expandafter\removePT@\the\R@\space #3\space c}%
 \PSmacro@{\tmp@}}
\xydef@\xyPScirc@#1#2{\edef\tmp@{\expandafter\removePT@\the\R@}%
 \PSmacro@{\tmp@\space #1 #2 o}}
\xydef@\xyPSCIRfull@{\setboxz@h{\kern\R@\xyPScirc@0{360}\kern\R@}%
 \wd\z@=\z@ \ht\z@=\R@ \dp\z@=\R@ \boxz@}%
\xydef@\xyPScirbuild@{{%
 \count@=\CIRlo@@ \count@@=\CIRhi@@ 
 \multiply\count@ by45 \advance\count@-180 \relax
 \multiply\count@@ by45 \advance\count@@-180 \relax
 \def\tmp@{}%
 \ifx\CIRtest@@\CIRtest@inside 
 \ifnum\count@@>\count@
 \edef\tmp@{\noexpand\xyPScirc@{\the\count@}{\the\count@@}}\fi
 \else\ifx\CIRtest@@\CIRtest@outside
 \ifnum\count@>-180 \advance\count@ by360 \relax
 \edef\tmp@{\noexpand\xyPScirc@{\the\count@@}{\the\count@}}%
 \else
 \ifnum\count@@<180 \relax
 \edef\tmp@{\noexpand\xyPScirc@{\the\count@@}{180}}%
 \fi\fi
 \fi\fi
 \kern\R@\tmp@\kern\R@}}
\xydef@\xyPSstraight@#1{\setupDirection@
 \edef\Creset@@{\cfromthec@ \pfromthep@ \DirectionfromtheDirection@}%
 \DN@##1##2{\def\checkoverlap@@{%
 \ifdim##1\X@p>##1\X@c \let\next@=\relax \fi
 \ifdim##2\Y@p>##2\Y@c \let\next@=\relax \fi}}%
 \edef\nextii@{{\sd@X}{\sd@Y}}\expandafter\next@\nextii@
 \noCshavep@@
 \edef\Cshavep@@{\pfromthep@ \noexpand\resetDirection@}%
 \noCshavec@@
 \edef\Cshavec@@{\cfromthec@ \noexpand\resetDirection@}%
 \ifHidden@\else
 \ifdim\Y@c>\Y@max \Y@max=\Y@c \fi \ifdim\Y@p>\Y@max \Y@max=\Y@p \fi
 \ifdim\Y@c<\Y@min \Y@min=\Y@c \fi \ifdim\Y@p<\Y@min \Y@min=\Y@p \fi
 \ifdim\X@c>\X@max \X@max=\X@c \fi \ifdim\X@p>\X@max \X@max=\X@p \fi
 \ifdim\X@c<\X@min \X@min=\X@c \fi \ifdim\X@p<\X@min \X@min=\X@p \fi \fi
 \ifInvisible@\let\next@=\relax \else
 \DN@{\setboxz@h{\kern\X@c \raise\Y@c\hbox{#1}}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ {\xykillstyles@\Drop@@}}%
 \fi 
 \checkoverlap@@
 \ifdim\d@X=\z@ \ifdim\d@Y=\z@ \DN@{\relax}\fi\fi \next@
 \def\Cslidep@@{\noCslidep@@}\def\Cslidec@@{\noCslidec@@}%
 \def\Calong@@{\noCalong@@}\Creset@@ }
\xylet@\xykillstyles@=\relax
\xydef@\xyPSsolid@{\straight@\xyPSsolidSpread@}%
\xydef@\xyPSsolidSpread@{\xyPSspread@{solid}{l}@@}%
\xydef@\xyPSdottedSpread@{\xyPSspread@{dotted}{dt}@@}%
\xydef@\xyPSdashed@{\line@ \def\Connect@@{\straight@\xyPSdashedSpread@}}
\xydef@\xyPSdashedSpread@{\xyPSspread@{dashed}{dd}@@}%
\xydef@\xyPSspread@#1#2@@#3\repeat@{\edef\tmp@{%
 \expandafter\removePT@\the\d@X\space\expandafter\removePT@\the\d@Y}%
 \setboxz@h{\kern\X@c \raise\Y@c\hbox{%
 \PSmessage{#1 line:}\PSmacro@{\tmp@\space #2}}}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\xyPSpoint@{\xyPSzerodot@\egroup
 \Invisible@false \Hidden@false \def\Leftness@{.5}\def\U@pness@{.5}\ctipEdge@
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@\xyPSdottedSpread@}}
\xydef@\xyPSzerodot@{\PSmessage{dot:}\PSmacro@{p}}
\xydef@\xyPScubic@#1{\readsplineparams@
 \PSmessage{CUBIC:}%
 \DN@{#1}\ifx\next@\empty\PSmacro@{mark \cubicinfo@\space bz}%
 \else\PSmacro@{mark \cubicinfo@\space b#1}\fi}
\xydef@\xyPSsquine@#1{\readsplineparams@
 \PSmessage{SQUINE:}%
 \DN@{#1}\ifx\next@\empty\PSmacro@{mark \squineinfo@\space q#1}%
 \else\PSmacro@{mark \squineinfo@\space q#1}\fi}
\xydef@\xyPSsplinesolid@{\ifx\splineinfo@\squineinfo@
 \expandafter\xyPSsquine@\else\expandafter\xyPScubic@\fi{}}
\xydef@\xyPSsplinedashed@{\ifx\splineinfo@\squineinfo@
 \expandafter\xyPSsquine@\else\expandafter\xyPScubic@\fi{d}}
\xydef@\xyPSsplinedotted@{\ifx\splineinfo@\squineinfo@
 \expandafter\xyPSsquine@\else\expandafter\xyPScubic@\fi{t}}
\xyendinput


==> xypsdict.tex <==
%% xypsdict.tex from $Id: xypsdict.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``PostScript backend prolog''.
%% Copyright (c) 1995-1997 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
\begingroup \xycatcodes%
 \count@=\xydashl@\relax \count@@=\xydashw@\relax%
 \XYpredict@\relax \xycatcodes \xyPSobeylines@@%
\PSdict@@{/XYdict where pop begin XYdict begin}%
\PSdict@@{%
 /xysize 10 def /T true def /F false def
 /dimendiv{65536 div}bind def 
 /xysegl \number\count@\space dimendiv def 
 /xyopp{1 -1 scale}bind def 
 /xynormwidth{\number\count@@\space dimendiv pscorrect}bind def
 /xywidth{xynormwidth setlinewidth}bind def 
}%
\PSdict@@{%
 /xyfont{4096 add 64 div round 64 mul 4096 sub}def /xydt 0.01 def
 /xysdfont{4096 add 32 div round 32 mul 4096 sub}def 
 /xydots{xywidth 1 setlinecap [xydt 2] 0 setdash}bind def 
 /f /xyfont load def /fs /xysdfont load def}%
\PSdict@@{%
 /xyCheckDir{dup 8 div 3 mul 3 -1 roll sub neg exch div 360 mul 
 dup dup XYdirection sub 180 div round 180 mul XYdirection add 
 dup 3 -1 roll sub abs 10 gt not{exch}if pop}def 
}%
\ifdim\xydashw@=0pt\xydashw@=.4pt\fi\count@@=\xydashw@\relax%
\PSdict@@{%
 /xyrulth{\number\count@@\space dimendiv pscorrect setlinewidth 
 0 setlinecap}bind def
}%
\PSdict@@{%
 /gsavexy{gsave xypspt XYdirection rotate xywidth newpath 0 0 moveto}def 
 /gchksavexy{gsave xypspt setupDirection xywidth newpath 0 0 moveto}def 
}%
\PSdict@@{%
 /xyswap{XYdirection 180 add /XYdirection exch def}def 
 /xyline{gstartxy setupDirection rlineto xystroke}def 
}%
\PSdict@@{%
 /dash{exch gchksavexy xysegl XYdirection dup 
 -90 lt{pop neg}{90 gt{neg}if}ifelse exch{neg}if
 0 rlineto xystroke}def 
 /stopper{gstartxy setupDirection 0 xysegl 2 div rmoveto 
 0 xysegl neg rlineto xystroke }def 
 /d /dash load def /st /stopper load def}%
\PSdict@@{%
 /solid{gstartxy xydash neg exch neg exch rlineto xystroke}def 
 /dashed{gstartxy 2 copy dup mul exch dup mul add sqrt dup 
 xysegl add xysegl 2 mul div round 2 mul 1 sub div [ exch dup ] 0 setdash 
 neg exch neg exch rlineto xystroke}def
 /l /solid load def /dd /dashed load def}%
\PSdict@@{%
 /dot{gstartxy 2 setlinecap [xydt 2] 0 setdash 
 1 0 rlineto xystroke}def 
 /dotted{gstartxy 2 copy dup mul exch dup mul add sqrt dup 
 2 div round 1 add div 2 setlinecap [xydt 3 -1 roll] 0 setdash 
 neg exch neg exch rlineto 0 0 rlineto xystroke}def
 /p /dot load def /dt /dotted load def}%
\PSdict@@{%
 /cubic{gstartxy docubic} def 
 /docubic{chkvalid 
 {chkcubedge 8 -2 roll moveto curveto xystroke pop}
 {cleartomark grestore}ifelse}def 
 /chkcubedge{2 copy 1.0 eq{0.0 eq{pop pop}{cubicedge}ifelse}
 {pop cubicedge}ifelse}def
 /bz /cubic load def}%
\PSdict@@{%
 /dotcubic{gstartxy 1 setlinecap [xydt 2] 0 setdash docubic}def 
 /dashcubic{gstartxy [5 5] 0 setdash docubic}def 
 /bt /dotcubic load def /bd /dashcubic load def}%
\PSdict@@{%
 /squine{gstartxy dosquine}def 
 /dosquine{chkvalid 
 {chksquedge 2 copy moveto xysq2cub curveto xystroke pop}
 {cleartomark grestore}ifelse}def
 /q /squine load def}%
\PSdict@@{%
 /chkvalid{2 copy lt{dup 1 gt{false}{true}ifelse}{false}ifelse}def 
}%
\PSdict@@{%
 /chksquedge{2 copy 1.0 eq{0.0 eq{pop pop}{squineedge}ifelse}
 {pop squineedge}ifelse}def 
 /xysq2cub{xysq2cubit 6 1 roll xysq2cubit 6 1 roll 3 index 3 index 
 xysq2cubit 6 1 roll xysq2cubit 6 1 roll pop pop}def 
 /xysq2cubit{2 index 2 mul add 3 div}def 
}%
\PSdict@@{%
 /dotsquine{gstartxy 1 setlinecap [xydt 2] 0 setdash dosquine}def 
 /dashsquine{gstartxy [5 5] 0 setdash dosquine}def 
 /qt /dotsquine load def /qd /dashsquine load def}%
\PSdict@@{%
/xy4mul{8 copy 
 5 -1 roll mul 5 1 roll 6 -1 roll mul 6 1 roll 
 3 -1 roll mul exch 4 -1 roll mul 3 1 roll 
 add 3 1 roll add exch 10 2 roll 
 7 -1 roll mul 7 1 roll 4 -1 roll mul 5 1 roll 
 4 -1 roll mul 4 1 roll mul add 3 1 roll add 
 exch 3 -1 roll }def 
}%
\PSdict@@{%
 /xy44mul{4 copy 16 4 roll exch 3 1 roll 4 copy 12 4 roll
 xy4mul 12 4 roll xy4mul 12 -4 roll 4 copy 16 4 roll
 8 4 roll xy4mul 12 4 roll xy4mul}def
}%
\PSdict@@{%
 /cubicedge{10 2 roll exch 8 1 roll 3 -1 roll dup dup 9 2 roll
 5 -1 roll dup dup 9 1 roll 8 3 roll
 4 1 roll dup dup 5 3 roll dup dup 5 1 roll 3 -1 roll
 18 -2 roll 2 copy 1 sub neg 4 1 roll 1 sub neg exch 4 1 roll
 xy444mul
 pop pop pop 13 1 roll pop pop pop 9 1 roll 10 1 roll
 pop 8 1 roll 7 1 roll 8 1 roll pop 5 1 roll 3 1 roll}def
}%
\PSdict@@{%
 /xy444mul{4 copy 24 4 roll 12 -4 roll 16 4 roll 4 copy 16 4 roll
 xy44mul 20 8 roll xy44mul
 12 -4 roll 4 -1 roll 7 1 roll exch 4 1 roll exch 6 -1 roll exch
 4 2 roll 16 8 roll 8 4 roll
 4 -1 roll 7 1 roll exch 4 1 roll exch 6 -1 roll exch 4 2 roll
 8 4 roll 16 4 roll 8 4 roll 20 -4 roll exch 3 1 roll
 4 copy 20 4 roll 4 copy 16 4 roll 4 copy 12 4 roll
 xy4mul 28 4 roll xy4mul 20 4 roll xy4mul 12 4 roll xy4mul}def
}%
\PSdict@@{%
 /squineedge{8 2 roll
 exch 5 1 roll 3 -1 roll dup 6 2 roll 1 index exch
 10 -2 roll 2 copy 1 sub neg 4 1 roll 1 sub neg exch 4 1 roll
 xy44mul 4 1 roll pop 5 1 roll 6 1 roll 3 -1 roll pop}def
}%
\PSdict@@{%
 /xyshort{2 copy abs exch abs add xysegl .5 mul lt
 {pop pop grestore}{rlineto xystroke}ifelse}def
}%
\PSdict@@{%
 /tipwidth{xywidth xynormwidth dup currentlinewidth exch div 
 sqrt dup dup scale mul setlinewidth 1 setlinecap}def
}%
\PSdict@@{%
 /halftip{tipwidth xysize 10 div 0 0 moveto
 -.25 0 3 -1 roll -2.5 mul 0 xysize 2 div neg
 dup .62 mul 2 div neg curveto}bind def
}%
\PSdict@@{/atip{gchksavexy halftip xystroke}def
 /btip{gchksavexy xyopp halftip xystroke}def
 /tip{gchksavexy gsave halftip stroke grestore
 xyopp halftip xystroke}def
 /t /tip load def /a /atip load def /b /btip load def}%
\PSdict@@{/cmatip{gchksavexy halfcmtip xystroke}def 
 /cmbtip{gchksavexy xyopp halfcmtip xystroke}def
 /cmtip{gchksavexy gsave halfcmtip stroke grestore
 xyopp halfcmtip xystroke}def
 /halfcmtip{tipwidth 0 0 moveto
 -.1333 0 .25 neg dup .125 3 -1 roll .25 curveto}bind def
 /ct /cmtip load def /ca /cmatip load def /cb /cmbtip load def}%
\PSdict@@{%
 /xyfscale{/xyfsize exch def}def /xyfsize{10}def
 /eu{-0.0551 0.0643 -0.0976 0.1386 -0.125 0.2188}def
 /cm{-0.105 0.0437 -0.1804 0.1380 -0.2 0.25}def
 /XY{-0.1753 0.0181 -0.3452 0.0708 -0.5 0.155}def
 /tipstart{3 -1 roll gchksavexy exch xyfscale tipwidth dup XYdict exch 
 known{dup /xy eq{pop /XY}if}{pop /XY}ifelse XYdict exch get}def
 /tipend{halfxytip xystroke}def 
 /halfxytip{1 1 6{pop xyfsize mul 6 1 roll}for 0 0 moveto curveto}def
 /A{tipstart D}def /B{tipstart C}def /C{xyopp D}def /D{exec tipend}def
 /AB{tipstart dup gsave exec halfxytip stroke grestore C}def
}%
\PSdict@@{%
 /Tip{exch gchksavexy /xyfsize{10}def tipwidth gsave 
 dup XYdict exch known{dup /xy eq{pop /XT}if}{pop /XT}ifelse
 XYdict exch get dup
 halfTip stroke grestore xyopp halfTip xystroke}def
 /XT{360 32 div neg}def /Xt{-1 .31 mul 1 atan}def
 /ET{360 64 div 5 mul neg}def /Et{-1 .31 mul 1 atan}def
 /halfTip{exec rotate XY halfxytip}def /halfTtip{halfTip}def
 /Ttip{exch gchksavexy /xyfsize{10}def tipwidth gsave 
 dup XYdict exch known{dup /xy eq{pop /Xt}if}{pop /Xt}ifelse
 XYdict exch get dup
 halfTtip stroke grestore xyopp halfTtip xystroke}def
 /tt /Tip load def /tT /Ttip load def}%
\PSdict@@{/halfturn{xysegl 2 div dup dup neg exch rmoveto
 0 exch dup exch -180 -90 arc}bind def
 /aturn{gchksavexy halfturn xystroke}def
 /bturn{gchksavexy xyopp halfturn xystroke}def
 /ta /aturn load def /tb /bturn load def}%
\dimen@=\xybsqll@\relax\count@=\dimen@%
\PSdict@@{%
 /xysqll \the\count@\space dimendiv def 
 /squigl{gchksavexy xysqll dup neg 0 rmoveto
 2 div dup dup neg dup 3 -1 roll
 2 sqrt mul dup 5 1 roll
 135 45 arcn dup 3 -1 roll -135 -45 arc
 xystroke}def
 /g /squigl load def}%
\PSdict@@{/fullhook{0 xysegl 2 div dup -90 90 arcn}bind def
 /halfhook{xysegl 2 div dup 0 exch 180 90 arcn}bind def
}%
\PSdict@@{/ahook{gchksavexy fullhook xystroke}def
 /bhook{gchksavexy xyopp fullhook xystroke}def
 /hook{gchksavexy gsave halfhook stroke grestore
 xyopp halfhook xystroke}def
 /h /hook load def /ha /ahook load def /hb /bhook load def}%
\PSdict@@{%
 /xyqcirc{dup dup neg exch translate newpath 
 dup neg 0 exch moveto 0 0 3 -1 roll -90 0 arc}bind def
}%
\PSdict@@{%
 /circ{gstartxy 
 3 copy pop 2 copy cos mul 3 1 roll sin mul
 rmoveto 0 0 5 2 roll arc xystroke}bind def
 /o /circ load def}%
\PSdict@@{%
 /circhar{gsave dup 3 gt{7 sub neg}if dup
 3 eq{pop dup 2 sqrt -2 div mul}{dup 1 eq{pop dup 2 sqrt 2 div mul}
 {0 eq{dup}{0}ifelse}ifelse}ifelse 
 0 translate 3 1 roll circ grestore}bind def
 /c /circhar load def}%
\PSdict@@{end end}%
\endgroup%
\endinput


==> xypspatt.tex <==
%% xypspatt.tex from $Id: xypspatt.doc,v 3.11 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``PostScript pattern prolog''.
%% Copyright (c) 1995-1998 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
%% As a special exception, you may use this file and all files derived
%% from it without restrictions. This special exception was added with
%% version 3.7 of Xy-pic.
%%
\begingroup \xycatcodes \xyPSobeylines@@%
\PSdict@@{/XYdict where pop begin XYdict begin}%
\PSdict@@{/:patt
{XYddict begin 
14 dict begin
/BGnd exch def
/FGnd exch def
/PaintData exch def
/PatternType 1 def
/PaintType 1 def
/BBox[0 0 1 1]def
/TilingType 1 def
/XStep 1 def
/YStep 1 def
/PatternMtx[24 0 0 24 0 0]def
/PaintProc BGnd null ne
 {{begin BGnd aload pop setrgbcolor 0 0 1 1 rF
 FGnd aload pop setrgbcolor
 24 24 true PatternMtx PaintData imagemask end}}
 {{begin FGnd aload pop setrgbcolor
 24 24 true PatternMtx PaintData imagemask end}}
 ifelse def
 currentdict PatternMtx end
 gsave patangle xyland{180 add}if
 rotate macfreq patfreq div dup neg exch scale matrix currentmatrix 
 grestore gsave setmatrix /DeviceRGB setcolorspace makepattern grestore
 end}def}%
\PSdict@@{%
/rF{gsave
 newpath 4 2 roll moveto 1 index 0 rlineto 0 exch rlineto neg 0 rlineto
 fill grestore}bind def }%
\PSdict@@{%
 /setpatscreen{/pattstring exch store patfreq
 patangle xyport not{90 add}if
 {1 add 4 mul cvi pattstring exch get exch 1 add 4 mul cvi 7 sub 
 bitshift 1 and}setscreen}bind def 
 /setcolpattern{setpatscreen 64 div 1 exch sub currentrgbcolor
 1 1 3{pop 1 exch sub 3 index mul 1 exch sub 3 1 roll}for
 setrgbcolor pop}def
 /setgraypattern{setpatscreen 64 div setgray}def
 /macfreq 9.375 def /patangle 0 def /patfreq 12.5 def}%
\PSdict@@{/checkland{%
 /normland where{pop normland not}{false}ifelse
 /xyland exch def
 /por where{pop por}{/isls where{pop isls not /xyland true def}
 {/land where{pop land not}{true}
 ifelse}ifelse}ifelse /xyport exch def}def }%
\PSdict@@{%
 /setpatfreq{/patfreq exch def}def
 /setpatangle{/patangle exch def}def
 /setbackcolor{/backcolor exch def}def
 /setforecolor{/forecolor exch def}def
 [1 1 1] setbackcolor xycolarray setforecolor
 /bg /setbackcolor load def /fg /setforecolor load def 
 /pa /setpatangle load def /pq /setpatfreq load def }%
\PSdict@@{%
 /xypattern{checkland counttomark dup 0 eq{pop}
 {dup 1 eq{pop setpatscreen}
 {dup 2 eq{pop setcolpattern}
 {dup 3 eq{pop 
 /setcolorspace where {
 /.setcolorspace where{pop pop pop setcolpattern}
 {/.buildpattern where {pop
 forecolor backcolor :patt setpattern
 }{pop pop setcolpattern}ifelse}ifelse}
 {pop setcolpattern}ifelse}
 {5 eq{/setcolorspace where{
 /.setcolorspace where{pop pop pop pop pop setcolpattern}
 {/.buildpattern where {pop
 :patt setpattern
 }{pop pop pop pop setcolpattern}ifelse}ifelse}
 {pop pop pop setcolpattern}ifelse
 }{}ifelse}ifelse}ifelse}ifelse}ifelse cleartomark }def 
 /xysetpattern{/xypatt exch def}def
 /sp /xysetpattern load def }%
\PSdict@@{end end}%
\endgroup%
\endinput


==> xyrecat.tex <==
%% xyrecat.tex from $Id: xyrecat.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Reset Category Codes'' utility.
%% Copyright (c) 1994-1996 Kristoffer H. Rose <krisrose@tug.org>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\xyuncatcodes
\xyrecat @ 64 \catcode 64 11
\xymakeADD@\addHASH@ # 35
\xymakeADD@\addDOLL@ $ 36
\xymakeADD@\addAND@ & 38
\xymakeADD@\addRQ@ ' 39
\xymakeADD@\addPLUS@ + 43
\xymakeADD@\addDASH@ - 45
\xymakeADD@\addDOT@ . 46
\xymakeADD@\addLT@ < 60
\xymakeADD@\addEQ@ = 61
\xymakeADD@\addGT@ > 62
\xymakeADD@\addLQ@ ` 96
\endinput


==> xyrotate.tex <==
%% xyrotate.tex from $Id: xyrotate.doc,v 3.8 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Rotate and Scale extension'' option.
%% Copyright (c) 1993-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{rotate}{Rotate and Scale extension}{\stripRCS$Revision: 3.8 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\xyundefinedRotate@#1#2@@{%
 \xywarning@{The #1 #2 effect is not implemented with the current driver.}}%
\xydef@\NoResizing{\xyNoResizing@}
\xydef@\UseResizing{\xyUseResizing@}
\xydef@\xyNoResizing@{%
 \global\let\origxyrescale@=\xyrescale@
 \global\let\origxyrotSizeMod@=\xyrotateSizeMod@
 \global\let\xyNoResizing@=\xyNoResizing@@
 \global\let\xyUseResizing@=\xyUseResizing@@
 \xyNoResizing@@ }
\xydef@\xyNoResizing@@{%
 \global\let\xyrescale@=\xyignorescale@
 \global\let\xyrotateSizeMod@=\xyignoreSizeMod@
 }
\xylet@\xyUseResizing@=\relax
\xydef@\xyUseResizing@@{%
 \global\let\xyrescale@=\origxyrescale@
 \global\let\xyrotateSizeMod@=\origxyrotSizeMod@
 }
\xydefcsname@{shape [@...]}#1{\xyrotatechar@#1@@}%
\xydefcsname@{shape [<...]}#1{\xyshearchar@{#1}@@}%
\xydefcsname@{shape [*...]}#1{\xyscalechar@{#1}@@}%
\xydefcsname@{shape [left]}{\xyshape@left@}
\xydefcsname@{shape [right]}{\xyshape@right@}
\xydefcsname@{shape [flip]}{\xyshape@flip@}
\xydefcsname@{shape [halfsize]}{\xyshape@halfsize@}
\xydefcsname@{shape [dblsize]}{\xyshape@dblsize@}
\xydefcsname@{shape [vflip]}{\xyshape@vflip@}
\xydefcsname@{shape [hflip]}{\xyshape@hflip@}
\xydef@\preXYtransform@{}
\xydef@\postXYtransform@{}
\xywarnifdefined\preXYtransform@@
\xywarnifdefined\postXYtransform@@
 \gdef\preXYtransform@@{}
 \gdef\postXYtransform@@{}
\xydef@\xy@transform@{}
\xydef@\preShape@@{}
\xydef@\postShape@@{}
\xydef@\modXYtransform@{%
 \ifx\xy@transform@\empty
 \transformDrop@\transformConnect@\resetTransform@\fi
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{##1}}%
 \expandafter\next@\expandafter{\preShape@@}%
 \DN@##1{\expandafter\gdef\expandafter\preXYtransform@@\expandafter{%
 \tmp@ ##1}}\expandafter\next@\expandafter{\preXYtransform@@}%
 \DN@##1{\expandafter\def\expandafter\tmp@\expandafter{##1}}%
 \expandafter\next@\expandafter{\postShape@@}%
 \DN@##1{\expandafter\gdef\expandafter\postXYtransform@@\expandafter{%
 \postXYtransform@@ ##1}}\expandafter\next@\expandafter{\tmp@}}%
\xydef@\transformDrop@{\let\xy@transform@=\relax
 \expandafter\def\expandafter\Drop@@\expandafter{%
 \expandafter\preXYtransform@\Drop@@\postXYtransform@}}
\xydef@\transformConnect@{\let\xy@transform@=\relax
 \expandafter\def\expandafter\Connect@@\expandafter{%
 \expandafter\preXYtransform@\Connect@@\postXYtransform@}}
\xydef@\resetTransform@{\gdef\preXYtransform@@{}\gdef\postXYtransform@@{}}
\xydef@\xynametransform@#1{%
 \DN@{\expandafter\gdef\expandafter#1\expandafter{\the\toks@}}\next@ }
\xydef@\xyscalechar@#1@@{\xyscalechars@#1,#1,@@}
\xydef@\xyscalechars@#1,#2,#3@@{%
 \DN@{\xyrescale@(#1,#2)}%
 \dimen@=#1\p@
 \ifdim\dimen@>\z@ \else \ifdim\dimen@<\z@ \else
 \DN@{\xywarning@{invalid scaling factors #1, #2}}%
 \fi\fi \dimen@=#2\p@
 \ifdim\dimen@>\z@ \else \ifdim\dimen@<\z@ \else
 \DN@{\xywarning@{invalid scaling factors #1, #2 }}%
 \fi\fi \next@ }
\xydef@\xyrescale@(#1,#2){%
 \setboxz@h{\xyscale@@{#1}{#2}%
 \dimen@=\ifx-#1\R@c\advance\dimen@-\R@c \dimen@=-\dimen@
 \else#1\L@c \advance\dimen@-\L@c\fi
 \kern\dimen@\boxz@\kern-\dimen@}%
 \R@c=\if-#1\L@c\else#1\R@c\fi
 \L@c=\if-#1\R@c\else#1\L@c\fi
 \U@c=\if-#2\D@c\else#2\U@c\fi
 \D@c=\if-#2\U@c\else#2\D@c\fi }
\xydef@\xyignorescale@(#1,#2){\xywarning@{Ignoring rescale: #1,#2}%
 \setboxz@h{\xyscale@@{#1}{#2}\boxz@}}%
\xydef@\xyshape@halfsize@{\xyrescale@(.5,.5)}
\xydef@\xyshape@dblsize@{\xyrescale@(2,2)}
\xydef@\xyshape@flip@{\xyrescale@(-1,-1)}
\xydef@\xyshape@vflip@{\xyrescale@(1,-1)}
\xydef@\xyshape@hflip@{\xyrescale@(-1,1)}
\xydef@\xyrotatechar@{\bgroup
 \afterDIRECTIONorEMPTY{\xyrotateSizeMod@}{\xyFN@\xySpecialRotate@i}}
\xydef@\xySpecialRotate@i{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\xySpecialRotate@i}%
 \else\ifx @\next \let\next@=\xyrotateSizeMod@
 \else\addEQ@\ifx \next
 \addEQ@\DN@##1@@{%
 \expandafter\xynametransform@\csname shape [##1]\endcsname\egroup}%
 \else\ifx !\next \DN@!{\egroup\getSpecialRotate@}%
 \else\ifx *\next \DN@*@@{\egroup\transformDrop@}%
 \else \DN@{\xySpecialRotate@@}%
 \fi\fi\fi\fi\fi \next@ }
\xydef@\getSpecialRotate@{\doSpecialRotate@@}
\xydef@\xyRotate@#1{\xyundefinedRotate@{rotate}{#1}@@}
\xydef@\xySpecialRotate@#1@@{\xyundefinedRotate@{rotate}{#1}@@\egroup}
\xydef@\doSpecialRotate@#1@@{\xyundefinedRotate@{special rotate}{#1}@@}
\xydef@\xyscale@#1#2{\xyundefinedRotate@{scale}{#1,#2}@@}
\xydef@\UnloadRotate@#1{%
 \ifx#1\relax\else\xyunload@{rotation extension}\fi
 \let\xyRotate@@=\xyRotate@
 \let\xySpecialRotate@@=\xySpecialRotate@
 \let\doSpecialRotate@@=\doSpecialRotate@
 \let\xyscale@@=\xyscale@ }
\UnloadRotate@\relax
\xyaddunsupport{rotate}{\UnloadRotate@\relax}
\xydef@\xyrotateSizeMod@ @@{%
 \L@p=\L@c \R@p=\R@c \U@p=\U@c \D@p=\D@c 
 \ifdim\cosDirection\p@>\z@ 
 \R@c=\cosDirection\R@p \L@c=\cosDirection\L@p
 \U@c=\cosDirection\U@p \D@c=\cosDirection\D@p 
 \else
 \R@c=\cosDirection\L@p \L@c=\cosDirection\R@p
 \U@c=\cosDirection\D@p \D@c=\cosDirection\U@p 
 \fi
 \advance\L@c \if-\sinDirection\D@p\else\sinDirection\U@p\fi
 \advance\R@c \if-\sinDirection\U@p\else\sinDirection\D@p\fi
 \advance\U@c \if-\sinDirection\L@p\else\sinDirection\R@p\fi
 \advance\D@c \if-\sinDirection\R@p\else\sinDirection\L@p\fi
 \dimen@ii=\L@c \advance\dimen@ii-\L@p
 \edef\tmp@{\egroup \L@c=\the\L@c \R@c=\the\R@c \U@c=\the\U@c \D@c=\the\D@c
 \dimen@ii=\the\dimen@ii \noexpand\setboxz@h\bgroup
 \noexpand\xyRotate@@{\the\Direction}}\tmp@
 \xydropRotated@ }
\xydef@\xydropRotated@@{%
 \kern\dimen@ii \boxz@ \kern-\dimen@ii \modXYtransform@ \egroup }
\xylet@\xydropRotated@=\xydropRotated@@
\xydef@\xyignoreSizeMod@ @@{\xywarning@{Ignoring rotation}}
\xydef@\xyshape@left@{\xyrotatechar@ v(0,1)@@}
\xydef@\xyshape@right@{\xyrotatechar@ v(0,-1)@@}
\xydef@\xyshearchar@{\xyundefinedRotate@{shearing}}
\xyendinput


==> xysmart.tex <==
%% xysmart.tex from $Id: xysmart.doc,v 3.6 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Smart Path feature'' option.
%% Copyright (c) 1998 George C. Necula <necula@cs.cmu.edu>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{smart}{Smart Path option}{\stripRCS$Revision: 3.6 $}%
 {George C. Necula}{necula@cs.cmu.edu}%
 {School of Computer Science,
 Carnegie Mellon University,
 5000 Forbes Avenue,
 Pittsburgh, PA 15213-3891, USA}
\xyrequire{arrow}\xycatcodes
\let\origPATHturn@=\PATHturn@
\def\PATHturn@{%
 \ifx \space@\next \expandafter\DN@\space{\xyFN@\PATHturn@}%
 \else\ifx s\next
 \let\origPATHturn@i=\PATHturn@i\let\PATHturn@i=\PATHsmartturn@i
 \let\origPATHturn@cir=\PATHturn@cir\let\PATHturn@cir=\PATHsmartturn@cir
 \DN@ s{\xyFN@\origPATHturn@}%
 \else
 \DN@{\origPATHturn@}%
 \fi\fi
 \next@}
\xydef@\PATHsmartturn@cir{%
 \edef\next@{{\CIRin@@}{\expandafter\noexpand\CIRorient@@}{\CIRout@@}}%
 \expandafter\PATHturn@i\next@}
\xydef@\PATHsmartturn@i#1#2#3{%
 \DN@##1{%
 \def\PATHinit@@{%
 \xy@@{%
 \def\sm@CIRin{#1}\def\sm@CIRout{#3}%
 \ifx\sm@CIRout\empty
 \let\sm@CIRout=\sm@CIRin
 \let\sm@CIRin=\PATHlastout@@
 \fi
 ##1\relax}%
 \xy@@{\enter@{\basefromthebase@}}%
 \xy@@{\sm@conn}%
 \xy@@{\X@p=\X@c \Y@p=\Y@c \czeroEdge@% Save the start of the segment
 \count@=\sm@CIRout\count@=\the\count@% Move forward a dash to
 \dimen@=\xydashl@ \ABfromdiag@ \advance\X@c\A@ \advance\Y@c\B@
 \edef\PATHpostpos@@{\X@c=\the\X@c \Y@c=\the\Y@c \noexpand\czeroEdge@
 \noexpand\PATHomitslide@@true}}%
 \xy@@{\leave@
 \edef\PATHlastout@@{\sm@CIRout}%
 \count@=\sm@CIRout \dimen@=\xydashl@ \Directionfromdiag@}}}%
 \expandafter\next@\expandafter{\the\toks@}\toks@={}%
 \let\PATHextra@@=\empty
 \def\PATHpost@@{\xy@@\PATHpostpos@@}%
 \let\PATHlabelsextra@@=\relax
 \let\PATHturn@i=\origPATHturn@i
 \let\PATHturn@cir=\origPATHturn@cir
 \xyFN@\PATHturn@ii}
\xydef@\sm@nil{}
\xydef@\sm@nnil{\sm@nil}
\xydef@\sm@maxcost{1000mm}%
\xydef@\sm@conn{
 \enter@{\cfromthec@ \DirectionfromtheDirection@}\cfromp@% Adjust p
 \count@=\sm@CIRin\count@=\the\count@
 \dimen@=\xydashl@ \ABfromdiag@ \advance\X@p\A@\advance\Y@p\B@
 \setupDirection@ \the\Edge@c\z@ \czeroEdge@
 \pfromc@
 \reverseDirection@
 \count@=\sm@CIRin\count@=\the\count@
 \dimen@=\xydashl@ \ABfromdiag@
 \edef\tmp@{\noexpand\dir\artail@@}\expandafter\sm@drop@\tmp@
 \X@c=\X@p\advance\X@c\A@ \Y@c=\Y@p\advance\Y@c\B@ \czeroEdge@
 \sm@stri
 \X@p=\X@c \Y@p=\Y@c
 \leave@
 \enter@{\pfromthep@ \DirectionfromtheDirection@}\pfromc@% Adjust c
 \count@=\sm@CIRout\count@=\the\count@
 \dimen@=\xydashl@ \ABfromdiag@ \advance\X@p-\A@\advance\Y@p-\B@
 \setupDirection@ \the\Edge@c\z@
 \advance\X@c-\A@\advance\Y@c-\B@% Leave room for a dash to terminate the seg
 \czeroEdge@
 \def\PATHlabelsnext@@{}%
 \leave@
 \R@=\turnradius@
 \cirrestrict@@%Adjust the radius to fit the circles
 \let\sm@circles=\sm@nil
 \edef\sm@bestcost{\sm@maxcost}%
 \sm@trycircles 1%Try counter clockwise first
 \sm@trycircles{-1}%
 \ifdim\sm@bestcost<\sm@maxcost
 \cfromp@
 \expandafter\sm@conndraw\sm@bestconn
 \else
 \xyerror@{Cannot draw the smart connector}{}%
 \fi
}
\xydef@\sm@trycircles#1{%
 \ifnum #1>0% Compute the opposite orientation
 \def\sm@CIRorienti{-1}%
 \else
 \def\sm@CIRorienti{1}%
 \fi
 \edef\tmp@{{{\sm@CIRin}{#1}{\sm@CIRout}}}%
 \expandafter\sm@trycirclelist\expandafter{\tmp@\sm@nil}%
 \count@@=\sm@CIRin\count@@=\the\count@@\count@=\count@@
 \sm@roundcount@{#1}%
 \edef\sm@savecount@{\the\count@}%
 \ifnum\the\count@=\the\count@@ \else
 \edef\tmp@{{{\sm@CIRin}{#1}{\the\count@}}%
 {{\the\count@}{\sm@CIRorienti}{\sm@CIRout}}}%
 \expandafter\sm@trycirclelist\expandafter{\tmp@\sm@nil}%
 \fi
 \count@=\sm@savecount@\count@=\the\count@
 \sm@advancecount@ 2{#1}\edef\sm@savecount@{\the\count@}%
 \edef\tmp@{{{\sm@CIRin}{#1}{\the\count@}}%
 {{\the\count@}{\sm@CIRorienti}{\sm@CIRout}}}%
 \expandafter\sm@trycirclelist\expandafter{\tmp@\sm@nil}%
 \count@=\sm@savecount@\count@=\the\count@
 \sm@advancecount@ 2{#1}\edef\sm@savecount@{\the\count@}%
 \edef\tmp@{{{\sm@CIRin}{#1}{\the\count@}}%
 {{\the\count@}{\sm@CIRorienti}{\sm@CIRout}}}%
 \expandafter\sm@trycirclelist\expandafter{\tmp@\sm@nil}%
 \count@=\sm@savecount@\count@=\the\count@
 \sm@advancecount@ 2{#1}\edef\sm@savecount@{\the\count@}%
 \edef\tmp@{{{\sm@CIRin}{#1}{\the\count@}}%
 {{\the\count@}{\sm@CIRorienti}{\sm@CIRout}}}%
 \expandafter\sm@trycirclelist\expandafter{\tmp@\sm@nil}%
}
\xydef@\sm@advancecount@#1#2{%
 \ifnum #2>0
 \edef\tmp@{#1}%
 \else
 \edef\tmp@{-#1}%
 \fi
 \advance\count@\tmp@\count@=\the\count@
 \ifnum\the\count@<0 \advance\count@ 8\fi
 \ifnum\the\count@>7 \advance\count@ -8\fi
 \count@=\the\count@
}
\xydef@\sm@roundcount@#1{%
 \ifcase\the\count@
 \advance\count@ #1\or
 \or \advance\count@ #1\or
 \or \advance\count@ #1\or
 \or \advance\count@ #1\fi
 \count@=\the\count@
 \ifnum\the\count@<0 \advance\count@ 8\fi
 \ifnum\the\count@>7 \advance\count@ -7\fi
 \count@=\the\count@
}
\newif\ifsm@firstseg
\newif\ifsm@acceptable
\xydef@\sm@trycirclelist#1{%
 \R@p=\z@\U@p=\R@p% Clear the deltas
 \def\sm@exthp{0}\def\sm@exthm{0}%
 \def\sm@extvp{0}\def\sm@extvm{0}%
 \def\sm@dxp{0pt}\def\sm@dxm{0pt}%
 \def\sm@dyp{0pt}\def\sm@dym{0pt}%
 \def\sm@segs{}%
 \sm@firstsegtrue
 \def\sm@connlen{0pt}%
 \let\sm@tryclcont=\sm@trycirclelist@i
 \sm@trycirclelist@i #1%Strip {} to expose the list elements
 \count@@=\sm@CIRout\count@@=\the\count@\count@=\the\count@
 \sm@roundcount@{1}%
 \ifnum\count@=\count@@
 \edef\sm@segs{\sm@segs{{\the\count@}{1}{\the\count@}}}%
 \fi
 \A@=\X@p\advance\A@\R@p\advance\A@ -\X@c\A@=-\A@
 \B@=\Y@p\advance\B@\U@p\advance\B@ -\Y@c\B@=-\B@
 \sm@acceptabletrue
 \ifdim\A@>0pt
 \ifnum\sm@exthp>0 \dimen@=\A@ \divide\dimen@\sm@exthp
 \edef\sm@dxp{\the\dimen@}%
 \else \sm@acceptablefalse\fi\fi
 \ifdim\A@<0pt
 \ifnum\sm@exthm>0 \dimen@=\A@ \divide\dimen@\sm@exthm
 \edef\sm@dxm{\the\dimen@}%
 \else \sm@acceptablefalse\fi
 \A@=-\A@%Make it positive
 \fi
 \ifdim\B@>0pt
 \ifnum\sm@extvp>0 \dimen@=\B@ \divide\dimen@\sm@extvp
 \edef\sm@dyp{\the\dimen@}%
 \else \sm@acceptablefalse\fi\fi
 \ifdim\B@<0pt
 \ifnum\sm@extvm>0 \dimen@=\B@ \divide\dimen@\sm@extvm
 \edef\sm@dym{\the\dimen@}%
 \else \sm@acceptablefalse\fi
 \B@=-\B@
 \fi
 \ifsm@acceptable
 \dimen@=\sm@connlen\advance\dimen@\A@\advance\dimen@\B@
 \ifdim\dimen@<\sm@bestcost
 \edef\sm@bestcost{\the\dimen@}%
 \edef\sm@bestconn{{\sm@dxp}{\sm@dxm}{\sm@dyp}{\sm@dym}{\sm@segs}}%
 \fi
 \fi
}
\xydef@\sm@showext#1{%
 \W@{#1\space hp=\sm@exthp,hm=\sm@exthm,vp=\sm@extvp
 ,vm=\sm@extvm,len=\sm@connlen}}
\xydef@\sm@trycirclelist@i#1{%
 \def\@tmp{#1}%
 \ifx \@tmp\sm@nnil \let\sm@tryclcont=\relax\else
 \expandafter\sm@tryclcar\@tmp \fi
 \sm@tryclcont}
\xydef@\sm@tryclcar#1#2#3{%
 \dimen@=\ifnum #2<0 -\fi\R@
 \count@=#1\count@=\the\count@ \ABfromdiag@
 \advance\R@p -\B@ \advance\U@p \A@
 \count@=#3\count@=\the\count@ \ABfromdiag@
 \advance\R@p \B@ \advance\U@p -\A@
 \sm@computeext{#1}{#2}{#3}%
}
\xydef@\sm@computeext#1#2#3{%
 \ifsm@firstseg
 \sm@accumext#1%
 \sm@firstsegfalse
 \fi
 \count@@=#1\count@@=\the\count@@\count@=\count@@
 \dimen@=\sm@connlen
 \sm@roundcount@{#2}%
 \ifnum \count@=\count@@
 \sm@advancecount@ 1{#2}%
 \advance\dimen@ 0.7854\R@% It was incremented with 1/8 circle
 \ifnum \count@=#3% Check if done
 \else
 \sm@advancecount@ 1{#2}%
 \advance\dimen@ 0.7854\R@% It was incremented with 1/8 circle
 \fi
 \else
 \advance\dimen@ 0.7854\R@% It was incremented with 1/8 circle
 \fi
 \edef\sm@connlen{\the\dimen@}%
 \sm@accumext{\the\count@}%
 \edef\sm@segs{\sm@segs{{#1}{#2}{\the\count@}}}%
 \ifnum\the\count@=#3 \else
 \edef\tmp@{{\the\count@}{#2}{#3}}%
 \expandafter\sm@computeext\tmp@
 \fi
}
\xydef@\sm@accumext#1{%
 \ifcase #1%
 \or \count@@=\sm@extvm\advance\count@@ by1%
 \edef\sm@extvm{\the\count@@}%
 \or\or \count@@=\sm@exthp\advance\count@@ by1%
 \edef\sm@exthp{\the\count@@}%
 \or\or \count@@=\sm@extvp\advance\count@@ by1%
 \edef\sm@extvp{\the\count@@}%
 \or\or \count@@=\sm@exthm\advance\count@@ by1%
 \edef\sm@exthm{\the\count@@}%
 \fi
}
\xydef@\sm@conndraw#1#2#3#4#5{%
 \def\sm@contlist{\sm@drawseglist}%
 \edef\sm@dxp{#1}%
 \edef\sm@dxm{#2}%
 \edef\sm@dyp{#3}%
 \edef\sm@dym{#4}%
 \sm@drawseglist #5\sm@nil}
\xydef@\sm@drawseglist#1{%
 \ifx #1\sm@nil \def\sm@contlist{}\else
 \sm@drawseg #1\fi
 \sm@contlist}
\xydef@\sm@drawseg#1#2#3{%
 \def\CIRin@@{#1}\def\CIRout@@{#3}%
 \sm@straight%See if a straight line is needed here. Insert it and
 \ifnum\CIRin@@=\CIRout@@ \else
 \count@=\CIRin@@
 \dimen@=\ifnum #2<0 -\fi\R@
 \ABfromdiag@
 \advance\X@c -\B@ \advance\Y@c \A@
 \ifnum #2>0 \def\CIRorient@@{\CIRacw@}%
 \else \def\CIRorient@@{\CIRcw@}\fi
 \drop@\literal@{\hbox\bgroup\cir@i}%
 \dimen@=\ifnum #2<0 -\fi\R@
 \count@=\CIRout@@\count@=\count@%Wierd. If I remove this last assignm
 \ABfromdiag@
 \advance\X@c\B@ \advance\Y@c-\A@
 \fi
}
\xydef@\sm@straight{%
 \U@c=\z@\D@c=\U@c\L@c=\U@c\R@c=\U@c
 \pfromc@
 \ifcase \CIRin@@ \or% 1 is V-
 \A@=\sm@dym\advance \Y@c\A@
 \or\or
 \A@=\sm@dxp\advance \X@c\A@
 \or\or
 \A@=\sm@dyp\advance \Y@c\A@
 \or\or
 \A@=\sm@dxm\advance \X@c\A@ \fi
 \ifdim\X@c=\X@p\ifdim\Y@c=\Y@p\else \sm@stri \fi\else \sm@stri \fi
}
\xydef@\sm@stri{%
 \edef\tmp@{\expandafter\noexpand\arstemprefix@@\arstem@@}%
 \expandafter\sm@connect@\tmp@}
\xydef@\sm@connect@#1#{%
 \DN@##1{\connect@{#1}{##1}}\next@}
\xydef@\sm@drop@#1#{%
 \DN@##1{\drop@{#1}{##1}}\next@}
\xydef@\smconn#1#2#3{%
 \edef\sm@CIRin{#1}\edef\sm@CIRout{#2}%
 \R@=#3\R@=\the\R@
 \sm@conn}
\xyendinput


==> xytextures.tex <==
%% xytextures.tex from $Id: xytextures.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Textures'' driver interface option.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{textures}{Textures driver}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\Textures@@#1{\dvimessage@{Textures}{#1}}
\newdriver{%
 \xyaddsupport{color}\texturesColor@@
 \xyaddsupport{crayon}\texturesCrayon@@
 \xyaddsupport{ps}\texturesPS@@
 \xyaddsupport{rotate}\texturesRotate@@
 \xyaddsupport{line}\texturesLine@@
 \xyaddsupport{frame}\texturesFrames@@
 \xyaddsupport{tile}\texturesTiles@@
 \xyaddsupport{cmtip}\relax
}
\xydef@\TexturesColor@push#1{\special{color push}\special{color #1}}
\xydef@\TexturesColours@{\texturesPStypes@
 \let\xylocalColor@=\xystackcolor@
 \let\xycolor@push=\TexturesColor@push
 \def\xycolor@{\xycolor@@}%
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}%
 \installPScolor@ }\else\DN@{}\fi \next@
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\texturesCrayon@@{}}%
 \else\let\next@=\xystandardcolors@ \fi \next@ 
 \let\xycolorwarning@=\relax \Textures@@{color}%
 \let\texturesColor@@=\relax
 \let\UnloadColor@@=\NoTexturesColor@
 }
\xydef@\texturesColor@@{\TexturesColours@}
\xydef@\NoTexturesColor@{%
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolor@=\xyNoColor@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\texturesColor@@=\TexturesColours@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\texturesCrayon@@{\texturesColor@@\texturesCrayon@}
\xydef@\texturesCrayon@{\installCrayolaColors@}%
\xydef@\texturesPS@@{\texturesPS@}
\xydef@\texturesPSunload@{\UnloadPS@
 \let\UnloadPS@@=\UnloadPS@
 \let\texturesPS@@=\texturesPS@ }
\xydef@\texturesPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\TexturesSpecial@\else
 \let\PSspecial@@=\TexturesSpecial@
 \let\PSmacro@@=\TexturesMacro@
 \let\PSdict@@=\TexturesDict@
 \let\PSraw@@=\TexturesRaw@
 \let\PSinclude@@=\TexturesInclude@
 \let\PSspecialdict@@=\TexturesSpecialDict@
 \let\xyPSobeylines@@=\obeyTextureslines@
 \Textures@@{PostScript}%
 \fi \texturesCurrpt@ \XYpredict@ }
\xydef@\TexturesSpecial@#1{\firstPS@@\special{postscript #1}}
\xydef@\TexturesMacro@#1{\special{postscript {#1}xy}}
\xydef@\TexturesDict@#1{\special{prePostScript #1}}
\xydef@\TexturesSpecialDict@#1{\special{prePostScript #1}}
\xydef@\TexturesInclude@#1{\firstPS@@\special{prePostScriptfile #1}}
\xydef@\TexturesRaw@#1{\firstPS@@\special{rawpostscript #1}}%
{\catcode`\^^M=\active%
 \gdef\next{\catcode`\^^M=\active \let^^M=\par%
 \let\PSspecial@@=\TexturesDict@ \obeyspaces}}
\xylet@\obeyTextureslines@=\next
\xydef@\texturesCurrpt@{\let\xyPScurrpt@@=\texturesCurrpt@@}%
\xydef@\texturesCurrpt@@{\PSspecial@@{xyi}\PSraw@@{userdict begin xyx end}}
\xydef@\texturesPS@{\texturesPStypes@
 \let\texturesPS@@=\relax
 \let\UnloadPS@@=\texturesPSunload@ 
 \let\installxyps@@=\relax \installxyps@ }
\xydef@\texturesRotate@@{\texturesRotate@}
\xydef@\texturesRotate@{\texturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \xyRotScale@@ \installPSrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}\UnloadRotate@\relax}\fi
 \next@}
\xydef@\texturesLine@@{\texturesLine@}
\xydef@\texturesLine@{\texturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}%
 \installPSline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\texturesFrames@@{\texturesFrames@}
\xydef@\texturesFrames@{\texturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}%
 \installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadPSFrames@\relax}\fi
 \next@ }
\xydef@\texturesTiles@@{\texturesTiles@}
\xydef@\texturesTiles@{\texturesPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}%
 \installPSpatterns@ \xystandardpatterns@}%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xyendinput


==> xytile.tex <==
%% xytile.tex from $Id: xytile.doc,v 3.8 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Pattern and Tile extension'' option.
%% Copyright (c) 1993-1997 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{tile}{Pattern and Tile extension}{\stripRCS$Revision: 3.8 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\xypatternwarning@@{\xypatternmessage@
 \gdef\xypatternwarning@{\xypatternmessage@
 \xywarning@{...no further pattern warnings will be given.}%
 \global\let\xypatternwarning@=\relax }}
\xylet@\xypatternwarning@=\xypatternwarning@@
\xydef@\xypatternmessage@{%
 \xywarning@{Current driver does not support patterns.}}%
\xydef@\newxypattern{\begingroup\xycatcodes\newxypattern@i}
\xydef@\newxypattern@i#1#2{\edef\next@{\endgroup
 \noexpand\newxyPattern{#1}{}{#2}{}}\next@}
\xydef@\newxyPattern#1#2#3#4{\newxypattern@{#1}{#2}{#3}{#4}{}}
\xydef@\newxypattern@#1#2#3#4#5{%
 \expandafter\let\expandafter\next@\csname shape [#1]\endcsname
 \ifx\next@\relax
 \DN@{#4}\ifx\next@\empty
 \DN@{#2}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalpattern@{}{#3}\xypattern@{#3}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalpattern@{#2}{#3}\xypattern@{#2 #3}}}%
 \fi
 \else\DN@{#2#3}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalpattern@{#4}{}\xypattern@{#4}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalpattern@{#2}{#3}\xypattern@{#4}}}%
 \fi\fi 
 \else \def\tmp@{\relax}\DNii@{#5}%
 \ifx\nextii@\tmp@
 \DN@{#4}\ifx\next@\empty
 \DN@{#2}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalpattern@{}{#3}\xypattern@{#3}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalpattern@{#2}{#3}\xypattern@{#2 #3}}}%
 \fi
 \else
 \DN@{#2#3}\ifx\next@\empty
 \DN@{\newxystyle{#1}{\xylocalpattern@{#4}{}\xypattern@{#4}}}%
 \else
 \DN@{\newxystyle{#1}{\xylocalpattern@{#2}{#3}\xypattern@{#4}}}%
 \fi\fi 
 \else\DN@{}\fi\fi \next@\relax }
\xydef@\xyNopattern@#1{}
\xylet@\xypattern@@=\xyNopattern@
\xydef@\xyNopattern@@#1#2{\xypatternwarning@}
\xylet@\xypattern@=\xypattern@@
\xylet@\xylocalpattern@=\xyNopattern@@
\xydef@\Unloadpattern@{%
 \let\xylocalpattern@=\xyNopattern@@
 \let\xypattern@=\xyNopattern@
 \let\xypatternwarning@=\xypatternwarning@@ }
\Unloadpattern@
\xydef@\xystandardpatterns@{}%
\xynew@{read}{\xypatread@}
\xydef@\defaultpattfile@{}
\xydef@\xygetfilepatterns@#1{\DN@{#1}%
 \ifx\next@\empty
 \ifx\defaultpattfile@\empty \xywarning@{No pattern file specified.}%
 \else \DN@{\expandafter\openpattfile@\expandafter{\defaultpattfile@}}\fi
 \else \DN@{\openpattfile@{#1}}\fi \next@ }
\xydef@\openpattfile@#1{\openin\xypatread@=#1.xyp
 \ifeof\xypatread@\xywarning@{No patterns in file: #1.xyp}%
 \closein\xypatread@
 \else \expandafter \xyreadpatfile@ \fi }%
\xydef@\UsePatternFile#1{\def\defaultpattfile@{#1}}
\xydef@\LoadAllPatterns{\let\parsepattern@=\parsepattern@@
 \xygetfilepatterns@ }
\xydef@\LoadPattern#1{\let\parsepattern@=\filepattern@@
 \def\pattname@{#1}\xygetfilepatterns@}
\xydef@\AliasPattern#1#2{\let\parsepattern@=\aliaspattern@@
 \def\aliasname@{#1}\def\pattname@{#2}\xygetfilepatterns@}
\xydef@\xyreadpatfile@{%
 \loop@ \bgroup\xycatcodes
 \global\read\xypatread@ to\xypatline@
 \ifeof\xypatread@ \aftergroup\endpatread@
 \else\aftergroup\morepatread@\fi \edef\next@{%
 \egroup\noexpand\getxypattern@{\xypatline@!!!}\relax}\next@
 \repeat@ }
\xydef@\endpatread@{\closein\xypatread@\iffalse}
\xydef@\morepatread@{\iftrue}
\xydef@\getxypattern@#1{\def\next{#1}\getxypattern@@}
\xydef@\getxypattern@@{\DN@{!!!}\ifx\next\next@\DN@{}%
 \else\DN@{\expandafter\parsepattern@\next}\fi \next@ }
\xydef@\parsepattern@@#1 #2!#3\relax{\newxypattern{#1}{#2}}
\xydef@\filepattern@@#1 #2!#3\relax{\DN@{#1}%
 \ifx\next@\pattname@
 \DN@{\expandafter\foundpattern@\expandafter{\pattname@}{#2}}%
 \else\DN@{}\fi \next@ }
\xydef@\foundpattern@#1#2{\newxypattern{#1}{#2}\endpatread@\fi
 \expandafter\eat@}
\xydef@\aliaspattern@@#1 #2!#3\relax{\DN@{#1}%
 \ifx\next@\pattname@
 \DN@{\expandafter\foundpattern@\expandafter{\aliasname@}{#2}}%
 \else\DN@{}\fi \next@ }
\DN@{\xyaddunsupport{tile}\Unloadpattern@}%
\ifx\xyeverywithoption@tile@\undefined
\else\ifx\xyeverywithoption@tile@\empty
\else
 \DN@{\xysetup@@{\xywithoption{tile}{\xyeverywithoption@tile@\xydriversloaded@@}}}%
\fi\fi \next@
\xyendinput


==> xytips.tex <==
%auto-ignore
%% xytips.tex from $Id: xytips.doc,v 3.9 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``More Tips'' extension.
%% Copyright (c) 1992-1996 Kristoffer H. Rose <kris@diku.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <kris@diku.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{tips}{More Tips extension}{\stripRCS$Revision: 3.9 $}%
 {Kristoffer H.~Rose}{kris@diku.dk}%
 {IBM T.~ J.\ Watson Research Center, P.O.~Box 704, Yorktown Heights, NY 10598 (USA)}
\xylet@\tip@xy=\tip@
\xylet@\atip@xy=\atip@
\xylet@\btip@xy=\btip@
\xylet@\Tip@xy=\Tip@
\xylet@\Ttip@xy=\Ttip@
\xylet@\tipjot@xy=\tipjot@
\xyfont@\xy@@atfont=xycmat10
\xyfont@\xy@@btfont=xycmbt10
\xyfont@\xy@@alfont=xyluat10
\xyfont@\xy@@blfont=xylubt10
\xydef@\tipfamily@@{cm}
\xydef@\tipsize@@{10}
\xydef@\SelectTips#1#2{%
 \DN@{#1}\ifx\next@\empty\else \def\tipfamily@@{#1}\fi
 \DN@{#2}\ifx\next@\empty\else \def\tipsize@@{#2}\fi
 \csname tipfamily \tipfamily@@\endcsname \ignorespaces}
\xydefcsname@{tipfamily cm}{\loadtipfonts@
 \let\tip@=\tip@cm \let\atip@=\atip@cm \let\btip@=\btip@cm
 \let\Tip@=\Tip@xy \let\Ttip@=\Ttip@xy \def\tipjot@{.2em}}
\xydef@\loadtipfonts@{\edef\next##1##2{##1=xy\tipfamily@@##2\tipsize@@}%
 \next{\font\xy@@atfont}{at}
 \next{\font\xy@@btfont}{bt}
}
\xydef@\tip@cm{\activatetips@ \tip@x\tip@@}
\xydef@\atip@cm{\activatetips@ \tip@x\atip@@}
\xydef@\btip@cm{\activatetips@ \tip@x\btip@@}
\xydef@\activatetips@{\let\xyatipfont=\xy@@atfont \let\xybtipfont=\xy@@btfont}
\xydefcsname@{tipfamily eu}{\loadtipfonts@
 \let\tip@=\tip@cm \let\atip@=\atip@cm \let\btip@=\btip@cm
 \let\Tip@=\Tip@eu \let\Ttip@=\Ttip@eu \def\tipjot@{.15em}}
\xydef@\Tip@eu{\kern1.5pt \vrule height1.5pt depth1.5pt width\z@
 \Tip@@eu \kern1.5pt \egroup
 \U@c=1.5pt \D@c=1.5pt \L@c=1.5pt \R@c=1.5pt \Edge@c={\circleEdge}%
 \Invisible@false \Hidden@false \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@\jot}}}
\xydef@\Tip@@eu{\count@=\DirectionChar
 \advance\count@-10 \ifnum\count@<\z@ \advance\count@128 \fi
 \xyatipfont\char\count@
 \advance\count@ 20 \ifnum127<\count@ \advance\count@-128 \fi
 \xybtipfont\char\count@}
\xydef@\Ttip@eu{\kern2.4pt \vrule height2.4pt depth2.4pt width\z@
 \Ttip@@eu \kern2.4pt \egroup
 \U@c=2.4pt \D@c=2.4pt \L@c=2.4pt \R@c=2.4pt \Edge@c={\circleEdge}%
 \Invisible@false \Hidden@false
 \def\Leftness@{.5}\def\Upness@{.5}%
 \def\Drop@@{\styledboxz@}\def\Connect@@{\straight@{\dottedSpread@\jot}}}
\xydef@\Ttip@@eu{%
 \setboxz@h\bgroup\reverseDirection@\line@ \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@
 \kern-\L@c \boxz@ \kern\L@c \Tip@@eu}
\xydefcsname@{tipfamily lu}{\loadtipfonts@
 \let\tip@=\tip@cm \let\atip@=\atip@cm \let\btip@=\btip@cm
 \let\Tip@=\Tip@xy \let\Ttip@=\Ttip@xy \def\tipjot@{.2em}}
\xydef@\UseTips{\csname tipfamily \tipfamily@@\endcsname}
\xydef@\NoTips{\let\tip@=\tip@xy \let\atip@=\atip@xy \let\btip@=\btip@xy
 \let\Tip@=\Tip@xy \let\Ttip@=\Ttip@xy \let\tipjot@=\tipjot@xy}
\xyendinput


==> xytp-f.tex <==
%% xytp-f.tex from $Id: xytp-f.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Frame extension'' TPIC backend support.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xytpfloaded\empty \message{not reloaded}\endinput \fi
\let\xytpfloaded=\empty \xycatcodes
\xydef@\installTPICframes@{%
 \let\framed@body@@=\xyTPICframed@body@
 \let\circled@x@@=\xyTPICcircled@x@
 \let\ellipsed@x@@=\xyTPICellipsed@x@
 \installTPICfills@
 \xyuncatcodes}
\xydef@\UseTPICframes{\installTPICframes@}
\xydef@\NoTPICframes{\UnloadFrames@}
\xydef@\xyTPICframed@body@{\DN@{\framed@body@}%
 \ifdim\R@=\z@ 
 \ifx\framehfill\frm@solidh@@
 \DN@{\xyTPICframed@rect@i\xytpic@solid@@}%
 \else\ifx\framehfill\frm@dashh@@
 \DN@{\xyTPICframed@rect@i\xytpic@dashed@@}%
 \else\ifx\framehfill\frm@doth@@
 \DN@{\xyTPICframed@rect@i\xytpic@dotted@@}%
 \fi\fi\fi\fi \next@ }
\xydef@\xyTPICframed@rect@i#1{\vglue\U@c
 \hbox{\hglue\L@c\xyTPICrect@{#1}\hglue\R@c}\vglue\D@c}
\xydef@\xyTPICcircled@x@{\DN@{\xyTPICcircled@xx{}}%
 \ifx\framehfill\frm@doth@@ \DN@{\xyTPICdotcirc@}%
 \else\ifx\framehfill\frm@dashh@@\DN@{\xyTPICdashcirc@}%
 \fi\fi \next@ }
\xydef@\xyTPICcircled@xx#1{\vglue2\R@
 \hbox{\hglue2\R@\xyTPICfullcircle@#1\hglue2\R@}\vglue2\R@}
\xydef@\xyTPICdotcirc@{\let\zerodot=\framezerodot@@ 
 \L@=\R@ \circled@x@@ }
\xydef@\xyTPICdashcirc@{\L@=\R@ \circled@x@@ }
\xydef@\xyTPICdotellip@{\ellipsed@x@@ }
\xydef@\xyTPICdashellip@{\ellipsed@x@@ }
\xydef@\xyTPICellipsed@x@#1#2{\DN@{\xyTPICellipsed@xx{}}%
 \ifx\framehfill\frm@doth@@\DN@{\xyTPICdotellip@}%
 \else\ifx\framehfill\frm@dashh@@\DN@{\xyTPICdashellip@}%
 \fi\fi \next@{#1}{#2}}
\xydef@\xyTPICellipsed@xx#1#2#3{\vglue #3\vglue #3\relax
 \hbox{\L@c = #2\relax \R@c=\L@c \D@c = #3\relax \U@c=\D@c 
 \hglue#2\hglue#2\relax \R@=#2\relax \L@=#3\relax
 \xyTPICfullcircle@#1\hglue#2\hglue#2\relax}%
 \vglue #3\vglue #3\relax}
\xydef@\xyTPICrect@#1{\DNii@{\relax}\DN@{#1}\toks@={}%
 \ifx\next@\nextii@ \xytpic@pn0\relax\xytpic@bk
 \def\xytpic@style@@{\xytpic@fp}%
 \else\DNii@{\empty}%
 \ifx\next@\nextii@\def\xytpic@style@@{\xytpic@ip}\xytpic@bk
 \else\ifx\next@\empty\def\xytpic@style@@{\xytpic@ip}\xytpic@bk
 \else#1\fi\fi\fi 
 \xytpic@pt\R@c 
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \xytpic@pt\D@c 
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \xytpic@pt{\L@c}%
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \xytpic@pt{\U@c}%
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \expandafter\xyTPICrect@x\the\toks@
 \DNii@{\relax}\DN@{#1}\ifx\next@\nextii@
 \def\xytpic@style@@{\xytpic@fp}\expandafter\xyTPICrect@x\the\toks@\fi }
\xydef@\xyTPICrect@x#1#2#3#4{\xyTPIC@special{pa -#3 -#4}%
 \xyTPIC@special{pa -#3 #2}\xyTPIC@special{pa #1 #2}%
 \xyTPIC@special{pa #1 -#4}\xyTPIC@special{pa -#3 -#4}%
 \xytpic@style@@ }
\xydef@\xyTPICoval@#1{\DN@{#1}\DNii@{\relax}%
 \ifx\next@\nextii@ \DN@{\xyTPICfilledoval@\relax}%
 \else\DNii@{\empty}\ifx\next@\nextii@ \DN@{\xyTPICfilledoval@\empty}%
 \else\DN@{\xyTPICoval@i{#1}}\fi\fi \next@ }
\xylet@\xyTPICoval@i=\eat@
\xydef@\xyTPICfilledoval@#1{%
 {\advance\L@c-\R@ \advance\R@c-\R@ \xyTPICrect@{\empty}}%
 {\advance\U@c-\R@ \advance\D@c-\R@ \xyTPICrect@{\empty}}%
 \L@=\R@ \bgroup 
 \dimen@=-\U@c \advance\dimen@\R@ \xytpic@pt\dimen@ 
 \edef\tmp@{\the\count@}%
 \dimen@=-\L@c \advance\dimen@\R@ \xytpic@pt\dimen@
 \edef\tmp@{\noexpand\toks@={{\the\count@}{\tmp@}}}%
 \setTPICcircstyle@ \xyTPICcircle@{\tmp@}\egroup
 \bgroup 
 \dimen@=-\U@c \advance\dimen@\R@ \xytpic@pt\dimen@ 
 \edef\tmp@{\the\count@}%
 \dimen@=\R@c \advance\dimen@-\R@ \xytpic@pt\dimen@
 \edef\tmp@{\noexpand\toks@={{\the\count@}{\tmp@}}}%
 \setTPICcircstyle@ \xyTPICcircle@{\tmp@}\egroup
 \bgroup 
 \dimen@=\D@c \advance\dimen@-\R@ \xytpic@pt\dimen@ 
 \edef\tmp@{\the\count@}%
 \dimen@=-\L@c \advance\dimen@\R@ \xytpic@pt\dimen@
 \edef\tmp@{\noexpand\toks@={{\the\count@}{\tmp@}}}%
 \setTPICcircstyle@ \xyTPICcircle@{\tmp@}\egroup
 \bgroup 
 \dimen@=\D@c \advance\dimen@-\R@ \xytpic@pt\dimen@ 
 \edef\tmp@{\the\count@}%
 \dimen@=\R@c \advance\dimen@-\R@ \xytpic@pt\dimen@
 \edef\tmp@{\noexpand\toks@={{\the\count@}{\tmp@}}}%
 \setTPICcircstyle@ \xyTPICcircle@{\tmp@}\egroup
 \DN@{#1}\DNii@{\relax}\ifx\next@\nextii@
 \def\tmp@{{\xytpic@pn0\def\xytpic@style@@{\xytpic@fp}}}%
 \DN@{\expandafter\xyTPICoval@i\tmp@}%
 \else\DN@{}\fi \next@ }
\xydef@\setTPICcircstyle@{%
 \def\xytpic@circstyle@@{\xytpic@ia}\xytpic@bk}
\xydef@\xyTPICcircle@#1{\DNii@{\relax}%
 \DN@{#1}\toks@={00}\ifx\next@\nextii@ 
 \xytpic@pn0\relax\xytpic@bk \def\xytpic@circstyle@@{\xytpic@ar}%
 \else\DNii@{\empty}%
 \ifx\next@\nextii@ \setTPICcircstyle@
 \else\ifx\next@\empty \setTPICcircstyle@
 \else#1\fi\fi\fi 
 \xytpic@pt\R@ 
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \xytpic@pt\L@ 
 \expandafter\addtotoks@\expandafter{\expandafter{\the\count@}}%
 \expandafter\xytpic@circstyle@@\the\toks@ 0\twoPi@}
\xydef@\xyTPICellipse@{%
 \X@p=\R@c \advance\X@p-\L@c \divide\X@p\tw@ \R@=\R@c \advance\R@-\X@p
 \Y@p=\D@c \advance\Y@p-\U@c \divide\Y@p\tw@ \L@=\D@c \advance\L@-\Y@p
 \xyTPICcircle@}
\xydef@\xyTPICrect@Special#1#2#3#4{\TPICmacro@@{#1 fp}}
\xydef@\xyTPICdotrect@Special#1{\TPICmacro@@{#1 fp}}
\xydef@\xyTPICdashrect@Special#1{\TPICmacro@@{#1 fp}}
\xydef@\xyTPICcirc@Special#1{\TPICmacro@@{#1 ar}}
\xydef@\xyTPICdotcirc@Special#1{\TPICmacro@@{#1 ar}}
\xydef@\xyTPICdashcirc@Special#1{\TPICmacro@@{#1 ar}}
\xydef@\xyTPICfilledRegion#1#2{\vglue\U@c
 \hbox{\hglue\L@c#1#2\empty\hglue\R@c}\vglue\D@c}
\xydef@\filledRectangle@TPIC@@{%
 \ifdim\R@=\z@ \DN@{\xyTPICfilledRegion\xyTPICrect@}%
 \else \DN@{\xyTPICfilledRegion\xyTPICoval@}%
 \fi \next@ }
\xydef@\filledCircle@TPIC@@#1{{\R@c=\R@ \L@c=\R@ \U@c=\R@ \D@c=\R@
 \xyTPICfilledRegion\xyTPICcircle@#1{}}}
\xydef@\filledEllipse@TPIC@@{\xyTPICfilledRegion\xyTPICellipse@}
\xydef@\filledOval@TPIC@@{\xyTPICfilledRegion\xyTPICoval@}
\xydef@\installTPICfills@{%
 \let\filledRectangle@@=\filledRectangle@TPIC@@
 \let\filledOval@@=\filledOval@TPIC@@
 \let\filledCircle@@=\filledCircle@TPIC@@
 \let\filledEllipse@@=\filledEllipse@TPIC@@
}
\xydef@\xyTPICfillrect@Special#1#2{%
 \ifx#2\relax\TPICmacro@@{#1 fp}%
 \else\TPICmacro@@{#1 ip}\fi}
\xydef@\xyTPICfilloval@Special#1#2{%
 \ifx#2\relax\TPICmacro@@{#1 fp}%
 \else\TPICmacro@@{#1 ip}\fi}
\xydef@\xyTPICfillcirc@Special#1#2{%
 \ifx#2\relax\TPICmacro@@{#1 ar}%
 \else\TPICmacro@@{#1 ai}\fi}
\xydef@\xyTPICfillellipse@Special#1#2{%
 \ifx#2\relax\TPICmacro@@{#1 ar}%
 \else\TPICmacro@@{#1 ai}\fi}
\endinput


==> xytpic.tex <==
%% xytpic.tex from $Id: xytpic.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``tpic'' TPIC backend, for lines, curves and fills.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{tpic}{TPIC backend}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xynew@{if}\ifTPICspecials@
\xydef@\UseTPICspecials{\TPICspecials@true}
\xydef@\NoTPICspecials{\TPICspecials@false}
\xynew@{count}\xytpic@cnt
\xydef@\xytpic@max{300}
\xydef@\maxTPICpoints#1{\count@=#1 \relax
 \ifnum\count@>\tw@ \edef\xytpic@max{\the\count@}%
 \else\expandafter\xyTPICmaxwarning@\expandafter{\the\count@}\fi}
\xydef@\xyTPICmaxwarning@#1{max points must be at least 2, #1 invalid}
\xydef@\xytpic@style@@{\xytpic@fp}
\xydef@\xytpic@reset@{\gdef\xytpic@style@@{\xytpic@fp}%
 \global\xytpic@cnt=\z@ }
\xydef@\xytpic@set@#1{\xdef\xytpic@style@@{\noexpand#1}}
\xydef@\xytpic@pn#1{\xyTPIC@special{pn #1}}
\xydef@\xytpic@pa#1#2{\global\advance\xytpic@cnt\@ne\relax
 \ifnum\xytpic@cnt=\xytpic@max\relax \xyTPIC@special{pa #1 #2}%
 \kern-\X@c\raise-\Y@c\hbox{\xytpic@style@@}\kern\X@c
 \global\xytpic@cnt=\@ne \relax\fi \xyTPIC@special{pa #1 #2}}
\xydef@\xytpic@fp{\xyTPIC@special{fp}}
\xydef@\xytpic@ip{\xyTPIC@special{ip}}
\xydef@\xytpic@da#1{\xyTPIC@special{da #1}}
\xydef@\xytpic@dt#1{\xyTPIC@special{dt #1}}
\xydef@\xytpic@sp#1{\xyTPIC@special{sp #1}}
\xydef@\xytpic@ar#1#2#3#4#5#6{\xyTPIC@special{ar #1 #2 #3 #4 #5 #6}}
\xydef@\xytpic@ia#1#2#3#4#5#6{\xyTPIC@special{ia #1 #2 #3 #4 #5 #6}}
\xydef@\xytpic@sh#1{\xyTPIC@special{sh #1}}
\xydef@\xytpic@wh{\xyTPIC@special{sh 0}}
\xydef@\xytpic@bk{\xyTPIC@special{sh 1}}
\xydef@\xyTPIC@special#1{\special{#1}}
\xydef@\xyTPIC@noisy#1{\W@{TPIC: #1}\special{#1}}
\xydef@\NoisyTPIC{\let\xyTPIC@special=\xyTPIC@noisy}
\xydef@\xyTPICsplit@#1#2{\setboxz@h{#1\boxz@#2}}%
\xydef@\xytpic@pt#1{\dimen@=#1\divide\dimen@ by72
 \multiply\dimen@ by 1000 \advance\dimen@.5\p@
 \count@=\dimen@ \divide\count@\p@ }
\xydef@\xytpic@in#1{\dimen@=#1\divide\dimen@ by72
 \edef\next@{\expandafter\removePT@\the\dimen@}}%
\xydef@\xytpic@dot@@{\xytpic@pa00}
\xydef@\xytpic@width@{\xytpic@pt{\xylinethick@}%
 \expandafter\xytpic@pn\expandafter{\the\count@}}
\xydef@\xytpic@line{%
 \xytpic@dot@@ \xytpic@pt{-\d@X}\count@@=\count@
 \xytpic@pt\d@Y \edef\next@{{\the\count@@}{\the\count@}}%
 \expandafter\xytpic@pa\next@ \xytpic@style@@ \xytpic@reset@ }
\xydef@\xytpic@solid@@{\xytpic@set@\xytpic@fp}
\xydef@\xytpic@dashed@@{\xytpic@in\xydashl@ \xytpic@dad}
\xydef@\xytpic@dotted@@{\dimen@=.5\xydashl@ \xytpic@in\dimen@ \xytpic@dtd}
\xydef@\xytpic@dad{\expandafter\xytpic@set@\expandafter{%
 \expandafter\xytpic@da\expandafter{\next@}}}
\xydef@\xytpic@dtd{\expandafter\xytpic@set@\expandafter{%
 \expandafter\xytpic@dt\expandafter{\next@}}}
\xydef@\xytpic@polysolid@{\xytpic@set@\xytpic@fp}
\xydef@\xytpic@polydashed@#1{\count@=#1 \xytpic@dad}
\xydef@\xytpic@polydotted@#1{\count@=#1 \xytpic@dtd}
\xydef@\xytpic@postpoly@{\xytpic@style@@ \xytpic@reset@}
\xydef@\TPICalternative@#1#2{%
\expandafter\global\expandafter\let\csname origxy#2@\endcsname=#1%
 \xdef#1{\noexpand\ifTPICspecials@
 \noexpand\expandafter\expandafter\noexpand\csname xytpic@#2@\endcsname
 \noexpand\else
 \noexpand\expandafter\expandafter\noexpand\csname origxy#2@\endcsname
 \noexpand\fi}}%
\xydef@\setupxyTPIC@{\xywarning@{using TPIC specials}%
 \TPICalternative@{\solid@}{solid}%
 \TPICalternative@{\dash@}{dashed}%
 \TPICalternative@{\point@}{point}%
 \TPICalternative@{\circhar@@}{circhar}%
 \TPICalternative@{\splinesolid@}{splinesolid}%
 \xywithoption{frame}{\xyinputorelse@{xytp-f}{}\xyuncatcodes}%
 \let\setupxyTPIC@=\reloadxyTPIC@ 
 \activateTPIC@ }
\xydef@\xyunloadTPIC@{\xywarning@{TPIC specials turned off}%
 \xywithoption{curve}{\xysetup@@\uninstallTPICcurves@ }%
 \xywithoption{line}{\xysetup@@\uninstallTPICline@ }%
 \xywithoption{frame}{\xysetup@@\uninstallTPICframes@ }%
 \TPICspecials@false
 \let\setupxyTPIC@=\reloadxyTPIC@ }
\xydef@\activateTPIC@{%
 \xywithoption{line}{\xysetup@@\installTPICline@}%
 \xywithoption{curve}{\xysetup@@\installTPICcurves@}%
 \xywithoption{frame}{\xysetup@@\installTPICframes@}%
 \TPICspecials@true }
\xydef@\reloadxyTPIC@{\xywarning@{TPIC specials back on}\activateTPIC@ }
\xydef@\xytpic@solid@{%
 \ifInvisible@ \let\next@=\no@@
 \else \DN@{\xyTPICstraight@{\xytpic@solid@@ \xytpic@line}}\fi
 \next@ }
\xydef@\xytpic@dashed@{\line@
 \def\Connect@@{\xyTPICstraight@{\xytpic@dashed@@ \xytpic@line}}}
\xydef@\xytpic@point@{\xytpic@dot@@\xytpic@fp\egroup
 \Invisible@false \Hidden@false \def\Leftness@{.5}\def\Upness@{.5}\ctipEdge@
 \def\Drop@@{\styledboxz@}%
 \def\Connect@@{\xyTPICstraight@{\xytpic@dotted@@ \xytpic@line}}}
\xydef@\xyTPICstraight@#1{\setupDirection@
 \edef\Creset@@{\cfromthec@ \pfromthep@ \DirectionfromtheDirection@}%
 \DN@##1##2{\def\checkoverlap@@{%
 \ifdim##1\X@p>##1\X@c \let\next@=\relax \fi
 \ifdim##2\Y@p>##2\Y@c \let\next@=\relax \fi}}%
 \edef\nextii@{{\sd@X}{\sd@Y}}\expandafter\next@\nextii@
 \noCshavep@@ \edef\Cshavep@@{\pfromthep@ \noexpand\resetDirection@}%
 \noCshavec@@ \edef\Cshavec@@{\cfromthec@ \noexpand\resetDirection@}%
 \ifHidden@\else
 \ifdim\Y@c>\Y@max \Y@max=\Y@c \fi \ifdim\Y@p>\Y@max \Y@max=\Y@p \fi
 \ifdim\Y@c<\Y@min \Y@min=\Y@c \fi \ifdim\Y@p<\Y@min \Y@min=\Y@p \fi
 \ifdim\X@c>\X@max \X@max=\X@c \fi \ifdim\X@p>\X@max \X@max=\X@p \fi
 \ifdim\X@c<\X@min \X@min=\X@c \fi \ifdim\X@p<\X@min \X@min=\X@p \fi \fi
 \ifInvisible@\let\next@=\relax \else
 \DN@{\setboxz@h{\kern\X@c \raise\Y@c\hbox{#1}}%
 \ht\z@=\z@ \wd\z@=\z@ \dp\z@=\z@ {\Drop@@}}%
 \fi 
 \checkoverlap@@
 \ifdim\d@X=\z@ \ifdim\d@Y=\z@ \DN@{\relax}\fi\fi \next@
 \def\Cslidep@@{\noCslidep@@}\def\Cslidec@@{\noCslidec@@}%
 \def\Calong@@{\noCalong@@}\Creset@@ }
\xydef@\xytpic@splinesolid@{\xyTPICspline@\xytpic@fp }
\xydef@\xytpic@splinedashed@{\xytpic@in\xydashl@\expandafter\xyTPICspline@
 \expandafter{\expandafter\xytpic@da\expandafter{\next@}}}
\xydef@\xytpic@splinedotted@{\xytpic@in{.5\xydashl@}\expandafter\xyTPICspline@
 \expandafter{\expandafter\xytpic@dt\expandafter{\next@}}}
\xydef@\xyTPICspline@#1{\setbox\splinebox@=\copy\voidb@x
 \SloppyCurves
 \global\xytpic@cnt=\@ne \xytpic@set@{#1}%
 \def\splineextra@@{\xyTPICspline@dot}%
 \def\xycrvdrop@{ }\def\xycrvconn@{}\splineset@@ \xytpic@style@@}
\xydef@\xyTPICspline@dot{\xytpic@pt{\X@c}\count@@=\count@
 \xytpic@pt{-\Y@c}\edef\next@{{\the\count@@}{\the\count@}}%
 \expandafter\xytpic@pa\next@ }
\xydef@\xyTPIClinewidth@#1{\xytpic@pt{#1}\edef\next@{\the\count@}}
\xydef@\installTPICline@{%
 \let\xylinewidth@@=\xylinewidth@
 \let\xylineSpecial@@=\xytpic@pn
 \let\transxyline@@=\xyTPIClinewidth@ }
\xydef@\uninstallTPICline@{\UnloadLine@}%
\xydef@\xydoTPICcircle@#1{\DN@{#1}%
 \ifx\next@\empty\DN@{\xyTPICfullcircle@}%
 \else\expandafter\DNii@\expandafter{\addDASH@{}}%
 \ifx\next@\nextii@\DN@{\L@=\R@ \xyTPICfullcircle@}%
 \else\DN@{\dosolidcircle@{#1}}\fi\fi \next@ }
\xydef@\xyTPICfullcircle@{\xyTPICpartcircle@{00}0\twoPi@}%
\xydef@\xyTPICpartcircle@#1#2#3{%
 \xytpic@pt{\R@}\expandafter\DNii@\expandafter{\the\count@}%
 \xytpic@pt{\L@}\edef\next@{#1{\nextii@}{\the\count@}{#2}{#3}}%
 \expandafter\xytpic@ar\next@ }
\xydef@\qartPi@{0.7853981}
\xydef@\tartPi@{2.3561944}
\xydef@\xytpic@circhar@#1{\xytpic@width@\ifcase#1%
 \xytpic@pt{\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{\tartPi@}{\fullPi@}\kern\partroottwo\R@
 \or
 \xytpic@pt{\halfroottwo\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{\halfPi@}{\tartPi@}\kern\halfroottwo\R@
 \or
 \xytpic@pt{\z@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{\qartPi@}{\halfPi@}\kern\halfroottwo\R@
 \or
 \xytpic@pt{-\halfroottwo\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@0{\qartPi@}\kern\partroottwo\R@
 \or
 \xytpic@pt{-\halfroottwo\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{-\qartPi@}0\kern\partroottwo\R@
 \or
 \xytpic@pt{\z@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{-\halfPi@}{-\qartPi@}\kern\halfroottwo\R@
 \or
 \xytpic@pt{\halfroottwo\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{-\tartPi@}{-\halfPi@}\kern\halfroottwo\R@
 \or
 \xytpic@pt{\R@}\edef\next@{{{\the\count@}0}}%
 \expandafter\xyTPICcirchar@i\next@{-\fullPi@}{-\tartPi@}\kern\partroottwo\R@
 \fi}
\xydef@\xyTPICcirchar@i#1#2#3{\L@=\R@ \xyTPICpartcircle@{#1}{#2}{#3}}
\xydef@\xyTPIC@spline@ii@{\DN@{\xy@spline@ii}%
 \ifx\splineSTYLE@\empty\DN@{\xyTPICqspline@{0}}%
 \else\expandafter\DNii@\expandafter{\addDASH@{}}%
 \ifx\splineSTYLE@\nextii@\DN@{\xyTPICqspline@{0}}%
 \else\expandafter\DNii@\expandafter{\addDOT@{}}%
 \ifx\splineSTYLE@\nextii@\DN@{\xyTPICqspline@{-.5}}%
 \else\expandafter\expandafter\expandafter\DNii@\expandafter\expandafter
 \expandafter{\expandafter\addDASH@\addDASH@{}}%
 \ifx\splineSTYLE@\nextii@\DN@{\xyTPICqspline@{}}%
 \fi\fi\fi\fi
 \next@ }%
\xydef@\xyTPIC@accumulate{\xytpic@pt\X@c \count@@=\count@ 
 \xytpic@pt{-\Y@c}\edef\next@{{\the\count@@}{\the\count@}}%
 \expandafter\xytpic@pa\next@ }
\xydef@\xyTPICqspline@#1{\xytpic@width@
 \xytpic@in{#1\xydashl@}\expandafter\gdef\expandafter\xytpic@style@@
 \expandafter{\expandafter\xytpic@sp\expandafter{\next@}}%
 \save@ \cfromp@ \xyTPIC@accumulate
 \edef\smapp@@{\s@bot}\smapxy@i{\xyTPIC@accumulate}%
 \leave@ \xyTPIC@accumulate \xytpic@style@@ \xytpic@reset@
 \enter@{}\xy@spline@x }
\xydef@\installTPICcurves@{%
 \let\dosolidcircle@@=\xydoTPICcircle@
 \let\xy@spline@ii@@=\xyTPIC@spline@ii@
 }
\xydef@\uninstallTPICcurves@{%
 \let\dosolidcircle@@=\dosolidcircle@
 \let\xy@spline@ii@@=\xy@spline@ii }
 \xywithoption{frame}{\xyinputorelse@{xytp-f}{}}
\xydef@\uninstallTPICframes@{\UnloadFrames@}
\xyendinput


==> xyv2.tex <==
%% xyv2.tex from $Id: xyv2.doc,v 3.8 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Version 2 compatibility'' feature.
%% Copyright (c) 1993-1995 Kristoffer H. Rose <kris@diku.dk>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <kris@diku.dk>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{v2}{Version 2 Compatibility}{\stripRCS$Revision: 3.8 $}%
 {Kristoffer H.~Rose}{krisrose@tug.org}%
 {IBM T.~ J.\ Watson Research Center, P.O.~Box 704, Yorktown Heights, NY 10598 (USA)}
\xylet@\XY=\Xy
\ifx\redefine\undefined \let\redefine=\def \fi
\ifx\define\undefined \let\define=\xydef@ \fi
\ifx\dsize\undefined \let\dsize=\displaystyle \fi
\ifx\tsize\undefined \let\dsize=\textstyle \fi
\ifx\ssize\undefined \let\ssize=\scriptstyle \fi
\ifx\sssize\undefined \let\sssize=\scriptscriptstyle \fi
\ifx\text\undefined
 \def\text{\relax\textC}%
 \xydef@\textC#1{\relax
 \ifmmode\mathchoice
 {\hbox{\the\textfont0\relax#1}}%
 {\hbox{\the\textfont0\relax#1}}%
 {\hbox{\the\scriptfont0\relax#1}}%
 {\hbox{\the\scriptscriptfont0\relax#1}}%
 \else{\relax#1}\fi}
\fi
\xydef@\Text{\relax\xyFN@\Text@}
\xydef@\TextC{\relax\textC}%
\xydef@\Text@{%
 \addLT@\ifx\next \addGT@{\addLT@\DN@##1}{\A@=##1\Text@i}%
 \else \DN@{\A@=\maxdimen \Text@i}\fi \next@}
\xydef@\Text@i#1{%
 \ifmmode \mathchoice
 {\expandafter\Text@ii\the\textfont0{#1}}%
 {\expandafter\Text@ii\the\textfont0{#1}}%
 {\expandafter\Text@ii\the\scriptfont0{#1}}%
 {\expandafter\Text@ii\the\scriptscriptfont0{#1}}%
 \else
 \leavevmode \expandafter\Text@ii\the\textfont0{#1}%
 \fi\ignorespaces}
\xydef@\Text@ii{\hbox\bgroup \txt@i}
\xylet@\cL=\L@c
\xylet@\cR=\R@c
\xylet@\cD=\D@c
\xylet@\cH=\U@c
\xylet@\Xc=\X@c
\xylet@\Yc=\Y@c
\xylet@\Uc=\U@c
\xylet@\Dc=\D@c
\xylet@\Lc=\L@c
\xylet@\Rc=\R@c
\xylet@\Xp=\X@p
\xylet@\Yp=\Y@p
\xylet@\Up=\U@p
\xylet@\Dp=\D@p
\xylet@\Lp=\L@p
\xylet@\Rp=\R@p
\xylet@\dX=\d@X
\xylet@\dY=\d@Y
\xylet@\Xorigin=\X@origin
\xylet@\Yorigin=\Y@origin
\xylet@\Xxbase =\X@xbase 
\xylet@\Yxbase =\Y@xbase 
\xylet@\Xybase =\X@ybase 
\xylet@\Yybase =\Y@ybase 
\xylet@\Xmin=\X@min
\xylet@\Ymin=\Y@min
\xylet@\Xmax=\X@max
\xylet@\Ymax=\Y@max
\xydef@\go{\aftergo{}}
\xydef@\aftergo#1{\xy@\aftergo{\enter@\pfromthec@}\afterPOS{\xy@@\leave@#1}}
\xydef@\merge{\POS.p\relax}
\xydef@\swap{\xy@\swap\swap@}
\xydef@\Drop{\expandafter\drop\entrymodifiers@}
\xydef@\none{\xy@\none{}\ignorespaces}
\xydef@\solid{\connect h\dir{-}}
\xydef@\Solid{\connect h\dir2{-}}
\xydef@\Ssolid{\connect h\dir3{-}}
\xydef@\dashed{\connect h\dir{--}}
\xydef@\Dashed{\connect h\dir2{--}}
\xydef@\Ddashed{\connect h\dir3{--}}
\xydef@\dotted{\connect h\dir{.}}
\xydef@\Dotted{\connect h\dir2{.}}
\xydef@\Ddotted{\connect h\dir3{.}}
\xydef@\dottedwith#1{\connect h{#1}}
\xydef@\notip{\dir{}}
\xydef@\stop{\dir{|}}
\xydef@\astop{\dir^{|}}
\xydef@\bstop{\dir_{|}}
\xydef@\tip{\dir{>}}
\xydef@\atip{\dir^{>}}
\xydef@\btip{\dir_{>}}
\xydef@\Tip{\dir2{>}}
\xywarnifdefined\aTip
\xywarnifdefined\bTip
{\xyuncatcodes
 \gdef\aTip{\object=<5pt>:(32,-1)\dir^{>}}
 \gdef\bTip{\object=<5pt>:(32,+1)\dir_{>}}}
\xydef@\Ttip{\dir3{>}}
\xydef@\ahook{\dir^{(}}
\xydef@\bhook{\dir_{(}}
\xydef@\aturn{\dir^{'}}
\xydef@\bturn{\dir_{'}}
\xydef@\rotate{\hbox\bgroup
 \DN@{\ifx (\next
 \DN@(####1){\rotate@ii{####1}}%
 \else \DN@{\rotate@i}\fi\next@}\xyFN@\next@}
\xydef@\rotate@i#1{\reverseDirection@ #1\OBJECT@x}
\xydef@\rotate@ii#1#2{\dimen@=#1\p@
 \ifdim \dimen@=-\p@ \aboveDirection@\xydashl@
 \else\ifdim\dimen@= \p@ \belowDirection@\xydashl@
 \else\ifdim\dimen@<-1.5\p@ \advance\dimen@-2\p@
 \edef\next@{\expandafter\removePT@\the\dimen@}\vDirection@(-1,\next@){1pc}%
 \else\ifdim\dimen@<-.5\p@ \vDirection@(#1,-1){1pc}%
 \else\ifdim\dimen@< .5\p@ \vDirection@( 1,#1){1pc}%
 \else\ifdim\dimen@<1.5\p@ \vDirection@(#1, 1){1pc}%
 \else \dimen@=-\dimen@ \advance\dimen@2\p@
 \edef\next@{\expandafter\removePT@\the\dimen@}\vDirection@(-1,\next@){1pc}%
 \fi\fi\fi\fi\fi\fi
 #2\OBJECT@x}
\xydef@\squash#1{%
 \ifmmode\setboxz@h{\m@th${\mathstrut}#1{\mathstrut}$}\else\setboxz@h{#1}\fi
 \setboxz@h{\kern-.5\wdz@ \dimen@=.5\ht\z@ \advance\dimen@-.5\dp\z@
 \lower\dimen@\boxz@}%
 \wdz@=\z@ \ht\z@=\z@ \dp\z@=\z@ \boxz@}
\xydef@\grow{%
 \DN@{\ifx <\next \DN@<####1>{\dimen@=####1\grow@\empty}%
 \else \DN@{\dimen@=2\p@ \grow@\empty}\fi\next@}\xyFN@\next@}
\xydef@\grow@#1#{\grow@@{#1}}
\xydef@\grow@@#1#2{\relax
 \ifmmode \setboxz@h{\kern\dimen@ \m@th$#2$\kern\dimen@}%
 \else \setboxz@h{\kern\dimen@ {#2}\kern\dimen@}\fi
 \dimen@ii=\ht\z@ \advance\dimen@ii\dimen@ \ht\z@=\dimen@ii
 \dimen@ii=\dp\z@ \advance\dimen@ii\dimen@ \dp\z@=\dimen@ii \boxz@}
\xydef@\squarify{\addEQ@{\addPLUS@\object}}
\xydef@\qc{\corn@@}
\xyrequire{frame}\xycatcodes
\xydef@\framed{\relax\convertframed{-}}
\xydef@\Framed{\relax\convertframed{=}}
\xydef@\circled{\relax\convertframed{o}}
\xydef@\Circled{\relax\convertframed{oo}}
\xydef@\convertframed#1{\DNii@##1@{\drop\frm##1{#1}}\xyFN@\convertframed@i}
\xydef@\convertframed@i{%
 \addLT@\ifx \next
 \addGT@{\addLT@\DN@##1}{\addGT@{\addLT@{\nextii@}##1}@}%
 \else \DN@{\nextii@ @}\fi \next@}
\xydef@\dotframed{\relax\drop\frm{.}}
\xydef@\dashframed{\relax\drop\frm{--}}
\xydef@\rounddashframed{\relax\drop\frm{o-}}
\xydef@\filled{\DN@{%
 \addLT@\ifx \next
 \addGT@{\addLT@\DN@####1}{\xy@@{\frame@fill@@{####1}}}%
 \else \DN@{\xy@@{\frame@fill@@\z@}}%
 \fi\next@}\xyFN@\next@}
\xydef@\Filled{\DN@{%
 \addLT@\ifx \next
 \addGT@{\addLT@\DN@####1}{\xy@@{\frame@emph@@{####1}}}%
 \else \DN@{\xy@@{\frame@emph@@\z@}}%
 \fi\next@}\xyFN@\next@}
\xyrequire{matrix}\xycatcodes
\xydef@\diagram#1\enddiagram{\relax\diagram@\diagram@@{#1}}
\xydef@\diagram@{\relax
 \ifmmode \DN@##1##2{\vcenter{\oldxymatrix@true \xy##1{\xymatrix{##2}}\endxy}}%
 \else\DN@##1##2{{\oldxymatrix@true \xy/u.8ex/##1{\xymatrix{##2}}\endxy}}%
 \fi \next@}
\xydef@\LaTeXdiagrams{\def\diagram{\ltxdiagram@\diagram@@}%
 \def\diagramnocompile{\ltxdiagram@\literal@}%
 \def\diagramcompileto##1{\ltxdiagram@{\NoCompileMatrices\xycompileto{##1}}}}
\xydef@\ltxdiagram@#1#2\end#3{\relax
 \DN@{#3}\DNii@{diagram}\ifx\next@\nextii@\diagram@{#1}{#2}\end{diagram}%
 \else\xyerr@{Put \string{\string} around \string\begin...\string\end\space
 within diagrams}\fi}
\xylet@\diagram@@=\literal@
\xydef@\NoisyDiagrams{}
\xydef@\spreaddiagramrows#1{\addPLUS@\xymatrixrowsep{#1}}
\xydef@\spreaddiagramcolumns#1{\addPLUS@\xymatrixcolsep{#1}}
\xyrequire{arrow}\xycatcodes
\xylet@\arrow=\ar
{\xyuncatcodes
 \gdef\morPHISM#1#2#3{\PATH~={\oldconnect{#1}}~<{|<*{#3}}~>{|>*{#2}}}}
\xydef@\morphism{\relax\morPHISM}
\xylet@\connect@iii=\connect
\xydef@\oldconnect#1{%
 \let\PATHlabelabove@@=\PATHlabelabove@
 \let\PATHlabelbelow@@=\PATHlabelbelow@
 \let\connect=\preconnect#1\let\connect=\connect@iii}
\xydef@\definemorphism#1#2#3#4{%
 \xydefcsname@{x#1}{\morphism{#2}{#3}{#4}}%
 \xydefcsname@{u#1}{\morphism{#2}{#3}{#4}[u]}%
 \xydefcsname@{d#1}{\morphism{#2}{#3}{#4}[d]}%
 \xydefcsname@{l#1}{\morphism{#2}{#3}{#4}[l]}%
 \xydefcsname@{r#1}{\morphism{#2}{#3}{#4}[r]}%
 \xydefcsname@{uu#1}{\morphism{#2}{#3}{#4}[uu]}%
 \xydefcsname@{dd#1}{\morphism{#2}{#3}{#4}[dd]}%
 \xydefcsname@{ll#1}{\morphism{#2}{#3}{#4}[ll]}%
 \xydefcsname@{rr#1}{\morphism{#2}{#3}{#4}[rr]}%
 \xydefcsname@{ur#1}{\morphism{#2}{#3}{#4}[ur]}%
 \xydefcsname@{ul#1}{\morphism{#2}{#3}{#4}[ul]}%
 \xydefcsname@{dr#1}{\morphism{#2}{#3}{#4}[dr]}%
 \xydefcsname@{dl#1}{\morphism{#2}{#3}{#4}[dl]}%
 \xydefcsname@{uul#1}{\morphism{#2}{#3}{#4}[uul]}%
 \xydefcsname@{uur#1}{\morphism{#2}{#3}{#4}[uur]}%
 \xydefcsname@{ull#1}{\morphism{#2}{#3}{#4}[ull]}%
 \xydefcsname@{urr#1}{\morphism{#2}{#3}{#4}[urr]}%
 \xydefcsname@{ddl#1}{\morphism{#2}{#3}{#4}[ddl]}%
 \xydefcsname@{ddr#1}{\morphism{#2}{#3}{#4}[ddr]}%
 \xydefcsname@{dll#1}{\morphism{#2}{#3}{#4}[dll]}%
 \xydefcsname@{drr#1}{\morphism{#2}{#3}{#4}[drr]}%
 \xydefcsname@{uull#1}{\morphism{#2}{#3}{#4}[uull]}%
 \xydefcsname@{uurr#1}{\morphism{#2}{#3}{#4}[uurr]}%
 \xydefcsname@{ddll#1}{\morphism{#2}{#3}{#4}[ddll]}%
 \xydefcsname@{ddrr#1}{\morphism{#2}{#3}{#4}[ddrr]}}
\definemorphism{to}\solid\tip\notip
\definemorphism{line}\solid\notip\notip
\definemorphism{dashed}\dashed\notip\notip
\definemorphism{dotted}\dotted\notip\notip
\definemorphism{double}\Solid\notip\notip
\xywarnifdefined\xyviitoi
\xywarnifdefined\xyviitoii
\xydef@\XXtoY@#1#2#3#4#5{\save;[#3]\relax
 \xy@@{%
 \dimen@=\turnradius@ \ifdim#1<#2\relax \dimen@ii=#2\else\dimen@ii=#1\fi
 \advance\dimen@\ifdim\dimen@>\dimen@ii +\dimen@\else +\dimen@ii\fi
 \edef\xyviitoi{\the\dimen@}\leave@}%
 \xto ~{[#3]} `#4[#3]#5/#4\xyviitoi/ `[#3]}
\xydef@\toXY@#1#2#3#4#5{\xy@@{\idfromc@{@}%
 \dimen@=\turnradius@ \dimen@ii=#1\relax
 \advance\dimen@\ifdim\dimen@>\dimen@ii +\dimen@\else +\dimen@ii\fi
 \edef\xyviitoi{\the\dimen@}%
 \dimen@=\turnradius@ \dimen@ii=#2\relax
 \advance\dimen@\ifdim\dimen@>\dimen@ii +\dimen@\else +\dimen@ii\fi
 \edef\xyviitoii{\the\dimen@}}%
 \morphism\solid{\object #4:(-1,0)\dir{>}}\notip
 ~{`"@" "@"} `#3"@"#5/#3\xyviitoi/#5/#4\p@/ `"@"#5/#4\xyviitoii/}
\xyuncatcodes \catcode64=11
\xydef@\lltod{\XXtoY@\D@c\D@p{ll}{d}+}
\xydef@\lltou{\XXtoY@\U@c\U@p{ll}{u}+}
\xydef@\rrtod{\XXtoY@\D@c\D@p{rr}{d}+}
\xydef@\rrtou{\XXtoY@\U@c\U@p{rr}{u}+}
\xydef@\ddtol{\XXtoY@\L@c\L@p{dd}{l}+}
\xydef@\ddtor{\XXtoY@\R@c\R@p{dd}{r}+}
\xydef@\uutol{\XXtoY@\L@c\L@p{uu}{l}+}
\xydef@\uutor{\XXtoY@\R@c\R@p{uu}{r}+}
\xydef@\told{\toXY@\L@c\D@c{l}{d}+}
\xydef@\tolu{\toXY@\L@c\U@c{l}{u}+}
\xydef@\tord{\toXY@\R@c\D@c{r}{d}+}
\xydef@\toru{\toXY@\R@c\U@c{r}{u}+}
\xydef@\todl{\toXY@\D@c\L@c{d}{l}+}
\xydef@\todr{\toXY@\D@c\R@c{d}{r}+}
\xydef@\toul{\toXY@\U@c\L@c{u}{l}+}
\xydef@\tour{\toXY@\U@c\R@c{u}{r}+}
\xycatcodes
\xydef@\TurnRadius{\addEQ@\turnradius}
\xydef@\diagramcompileto#1#2\enddiagram{\relax
 \diagram@{\NoCompileMatrices\xycompileto{#1}}{#2}}
\xydef@\diagramnocompile#1\enddiagram{\relax\diagram@\literal@{#1}}
\xydef@\CompileAllDiagrams#1{\CompilePrefix{#1}\CompileMatrices}
\xydef@\NoCompileAllDiagrams{\NoCompileMatrices}
\xydef@\ReCompileAllDiagrams{\CompileMatrices}
\xyendinput


==> xyweb.tex <==
%% xyweb.tex from $Id: xyweb.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``Lattice and web'' feature.
%% Copyright (c) 1994-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{web}{Lattice and web feature}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\message{lattices,}
\xynew@{count}\lattice@A
\xynew@{count}\lattice@B
\xydef@\latticeA{\lattice@A}
\xydef@\latticeB{\lattice@B}
\xydef@\xylattice#1#2#3#4{\xy@{LATTICE}{\xylattice@{#1}{#2}{#3}{#4}}}%
\xydef@\xylattice@#1#2#3#4{%
 \lattice@A=#1\relax
 \loop \bgroup\lattice@B=#3\relax
 \innerlatticeloop@{#4}%
 \edef\tmp@{\egroup
 \X@min=\the\X@min \X@max=\the\X@max
 \Y@min=\the\Y@min \Y@max=\the\Y@max 
 }\tmp@ \ifnum\lattice@A<#2\relax \advance\lattice@A\@ne
 \repeat }
\xydef@\innerlatticeloop@#1{%
 \loop \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ \the\lattice@A,\the\lattice@B @%
 \edef\latticeX{\expandafter\removePT@\the\X@c}%
 \edef\latticeY{\expandafter\removePT@\the\Y@c}%
 \leave@ \latticebody \leave@
 \ifnum\lattice@B<#1\relax \advance\lattice@B\@ne
 \repeat }
\xydef@\croplattice#1#2#3#4#5#6#7#8{\xy@{LATTICE}%
 {\xycroplattice@{#1}{#2}{#3}{#4}{#5}{#6}{#7}{#8}}}%
\xydef@\xycroplattice@#1#2#3#4#5#6#7#8{%
 \enter@{\X@min=\the\X@min \X@max=\the\X@max 
 \Y@min=\the\Y@min \Y@max=\the\Y@max}%
 \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ #5,0 @\leave@ \X@min=\X@c \leave@
 \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ #6,0 @\leave@ \X@max=\X@c \leave@
 \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ 0,#7 @\leave@ \Y@min=\Y@c \leave@
 \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ 0,#8 @\leave@ \Y@max=\Y@c \leave@
 \lattice@A=#1\relax
 \loop
 \bgroup\lattice@B=#3\relax
 \enter@{\cfromthec@}\innercroplatticeloop@{#4}\leave@
 \egroup
 \ifnum\lattice@A<#2\relax \advance\lattice@A\@ne
 \repeat \mergecropextents@ }
\xydef@\innercroplatticeloop@#1{%
 \loop 
 \enter@{\cfromthec@}\enter@{\cplusthec@}%
 \vfromcartesian@@ \the\lattice@A,\the\lattice@B @%
 \edef\latticeX{\expandafter\removePT@\the\X@c}%
 \edef\latticeY{\expandafter\removePT@\the\Y@c}%
 \leave@ \DN@{\latticebody}%
 \ifdim\X@c<\X@min\DN@{}%
 \else\ifdim\X@c>\X@max\DN@{}%
 \else\ifdim\Y@c<\Y@min\DN@{}%
 \else\ifdim\Y@c>\Y@max\DN@{}%
 \fi\fi\fi\fi \next@ \leave@
 \ifnum\lattice@B<#1\relax \advance\lattice@B\@ne
 \repeat }
\xydef@\mergecropextents@{%
 \edef\tmp@{%
 \noexpand\ifdim\X@min>\the\X@min \X@min=\the\X@min\noexpand\fi
 \noexpand\ifdim\X@max<\the\X@max \X@max=\the\X@max\noexpand\fi
 \noexpand\ifdim\Y@min>\the\Y@min \Y@min=\the\Y@min\noexpand\fi
 \noexpand\ifdim\Y@max<\the\Y@max \Y@max=\the\Y@max\noexpand\fi}%
 \leave@ \tmp@ }
\xydef@\deflatticebody@{\def\latticebody{\drop{\bullet}}}
\xydef@\defaultlatticebody{\deflatticebody@}
\deflatticebody@
\xyendinput


==> xyxdvi.tex <==
%% xyxdvi.tex from $Id: xyxdvi.doc,v 3.7 2011/03/14 20:14:00 krisrose Exp $
%%
%% Xy-pic ``xdvi-driver'' option.
%% Copyright (c) 1995-1996 Ross Moore <ross.moore@mq.edu.au>
%%
%% This file is part of the Xy-pic package for graphs and diagrams in TeX.
%% See the companion README and INSTALL files for further information.
%% Copyright (c) 1991-2011 Kristoffer H. Rose <krisrose@tug.org>
%%
%% The Xy-pic package is free software; you can redistribute it and/or modify
%% it under the terms of the GNU General Public License as published by the
%% Free Software Foundation; either version 2 of the License, or (at your
%% option) any later version.
%%
%% The Xy-pic package is distributed in the hope that it will be useful, but
%% WITHOUT ANY WARRANTY; without even the implied warranty of MERCHANTABILITY
%% or FITNESS FOR A PARTICULAR PURPOSE. See the GNU General Public License
%% for more details.
%%
%% You should have received a copy of the GNU General Public License along
%% with this package; if not, see http://www.gnu.org/licenses/.
%%
\ifx\xyloaded\undefined \input xy \fi
\xyprovide{xdvi}{XDVI driver}{\stripRCS$Revision: 3.7 $}%
 {Ross Moore}{ross.moore@mq.edu.au}%
 {Mathematics Department, Macquarie University, NSW~2109, Australia}
\xydef@\xdvi@@#1{\dvimessage@{xdvi}{#1}}
\newdriver{%
 \xyaddsupport{color}\xdviColor@@
 \xyaddsupport{crayon}\xdviCrayola@@
 \xyaddsupport{ps}\xdviPS@@
 \xyaddsupport{rotate}\xdviRotate@@
 \xyaddsupport{line}\xdviLine@@
 \xyaddsupport{frame}\xdviFrames@@
 \xyaddsupport{tile}\xdviTiles@@
 \xyaddsupport{tpic}\xdviTPIC@ 
}
\xydef@\xdvi@Color@{\xdviPStypes@ 
 \let\xylocalColor@=\xyNoColor@@
 \def\xycolor@{\xycolor@@}\let\xycolorwarning@=\relax
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-c}{\xydrivernoload@{ps-c}}\installPScolor@ }%
 \else\DN@{}\fi \next@ 
 \ifx\xycolor@@\xyNoColor@ \let\xycolor@@=\xycolor@raw@@\fi
 \ifx\xycrayolaloaded\empty \DN@{\xystandardcolors@\xdviCrayola@{}}%
 \else \DN@{\xystandardcolors@}\fi \next@
 \let\xdviColor@@=\relax
 \let\UnloadColor@@=\NoXDVIcolor@
 }%
\xydef@\xdviColor@@{\xdvi@Color@}
\xydef@\NoXDVIcolor@{%
 \def\xycolor@{\xycolor@@}%
 \let\xycolor@@=\xyNoColor@
 \let\xylocalColor@=\xyNoColor@@
 \let\xycolorwarning@=\xycolorwarning@@
 \let\xdviColor@@=\xdvi@Color@
 \let\UnloadColor@@=\UnloadColor@
 }
\xydef@\NoXDVIcolordvi@{\xywarning@{%
 Neither colordvi.tex nor colordvi.sty could be found.}%
 \xyBEcolorcheck@}%
\xydef@\xdviCrayola@@{\xdviColor@@\xdviCrayola@}
\xydef@\xdviCrayola@{%
 \let\prevxycolor@=\newxycolor@
 \def\newxyXDVIcolor@##1##2##3{\prevxycolor@{##1}{}{##1}}%
 \let\newxycolor@=\newxyXDVIcolor@
 \installCrayolaColors@
 \let\newxycolor@=\prevxycolor@ }%
\xydef@\xdviPS@@{\xdviPS@}
\xydef@\xdviPS@unload{\UnloadPS@
 \let\UnloadPS@@=\UnloadPS@
 \let\xdviPS@@=\xdviPS@ }
\xydef@\xdviPStypes@{%
 \xyinputorelse@{xyps-ps}{\xydrivernoload@{ps-ps}}%
 \ifx\PSspecial@@\xdviSpecial@\else
 \let\PSspecial@@=\xdviSpecial@
 \let\PSmacro@@=\xdviMacro@
 \let\PSdict@@=\xdviDict@
 \let\PSspecialdict@@=\xdviDict@
 \let\PSraw@@=\xdviRaw@
 \let\PSinclude@@=\xdviInclude@
 \let\xyPSobeylines@@=\obeyXDVIlines@
 \let\xyPScurrpt@@=\xdviCurrpt@@
 \xdvi@@{PostScript}%
 \fi \XYpredict@ }
\xywarnifdefined\xdviSpecial@
\xywarnifdefined\xdviMacro@
\xywarnifdefined\xdviDict@
\xywarnifdefined\xdviInclude@
\xywarnifdefined\xdviRaw@
{\catcode`\"=11 \catcode`\!=11 \catcode`\:=11
 \gdef\xdviSpecial@#1{\special{ps:: SDict begin #1 end}}
 \gdef\xdviMacro@#1{\firstPS@@\special{" {#1}xy}}
 \gdef\xdviDict@#1{\special{! #1}}
 \gdef\xdviInclude@#1{\special{header=#1}}
 \gdef\xdviRaw@#1{\special{ps: SDict begin #1 end}}
\catcode`\^^M=\active
 \gdef\next{\catcode`\^^M=\active \let^^M=\space }}%
\xylet@\obeyXDVIlines@=\next
\xydef@\xdviCurrpt@{\let\xyPScurrpt@@=\xdviCurrpt@@}%
\xydef@\xdviCurrpt@@{\PSraw@@{xyp}}
\xydef@\xdviPS@{\xdviPStypes@ 
 \let\xdviPS@@=\PSspecials@true
 \let\UnloadPS@@=\xdviPS@unload 
 \let\installxyps@@=\relax \installxyps@ }
\xydef@\xdviRotate@@{\xdviRotate@}
\xydef@\xdviRotate@{\xdviPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-r}{\xydrivernoload@{ps-r}}%
 \xdviCurrpt@ \xdviRotScale@ \installPSrotscale@ }%
 \else\DN@{\xydriverfail@{rotations are}UnloadRotate@\relax}\fi
 \next@ }
\xydef@\xdviRotScale@{%
 \def\xyrot@start(##1){{xyct ##1\space xyrs }}%
 \def\xyrot@end{}%
 \def\xyscale@start(##1,##2){{xyct ##1\space##2\space xyss }}%
 \def\xyscale@end{}}
\xydef@\xdviLine@@{\xdviLine@}
\xydef@\xdviLine@{\xdviPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-l}{\xydrivernoload@{ps-l}}\installPSline@ }%
 \else\DN@{\xydriverfail@{line-widths are}\UnloadLine@\relax}\fi
 \next@ }
\xydef@\xdviFrames@@{\xdviFrames@}
\xydef@\xdviFrames@{\xdviPStypes@
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-f}{\xydrivernoload@{ps-f}}\installPSframes@ }%
 \else\DN@{\xydriverfail@{frames are}\UnloadFrames@\relax}\fi
 \next@ }
\xydef@\xdviTiles@@{\xdviTiles@}
\xydef@\xdviTiles@{\xdviPStypes@ 
 \expandafter\ifx\csname xyps-psloaded\endcsname\empty\DN@{%
 \xyinputorelse@{xyps-t}{\xydrivernoload@{ps-t}}\installPSpatterns@ }%
 \else\DN@{\xydriverfail@{Patterns are}\UnloadPSpatterns@\relax}\fi
 \next@ }
\xydef@\xdviTPIC@@{\xdviTPIC@}
\xydef@\xdviTPIC@{\setupxyTPIC@}
\xyendinput

